Spectral Properties of Cool Stars: Extended Abundance Analysis of Kepler Objects of Interest

Accurate stellar parameters and precise elemental abundances are vital pieces to correctly characterize discovered planetary systems, better understand planet formation, and trace galactic chemical evolution. We have performed a uniform spectroscopic analysis for 1127 stars, yielding accurate gravity, temperature, and projected rotational velocity in addition to precise abundances for 15 elements (C, N, O, Na, Mg, Al, Si, Ca, Ti, V, Cr, Mn, Fe, Ni, and Y). Most of the stars in this sample are Kepler Objects of Interest, observed by the California-Kepler Survey (CKS) and include 1,003 stars hosting 1,562 confirmed planets. This catalog extends the uniform analysis of our previous catalog, bringing the total of homogeneously analyzed stars to almost 2,700 F, G, and K dwarfs. To ensure consistency between the catalogs, we performed an analysis of our ability to recover parameters as a function of S/N ratio and present individual uncertainties as well as functions to calculate uncertainties for parameters derived from lower S/N ratio spectra. With the updated parameters, we used isochrone fitting to derived new radii, masses and ages for the stars. Finally, we look at the Mg/Si ratios of super-Earth and sub-Neptune hosts to test whether differences in initial composition might lead to differences in planet radius. We find no differences in the Mg/Si distribution as a function of planet radius.

==> table_03.tex <==
\begin{deluxetable*}{llllrrrrrrrrrrrrr}
\tablecaption{Spectroscopically determined stellar properties.
\label{table:stellar_properties}
}
\tablehead{\colhead{ID} & \colhead{Name} & \colhead{$\alpha$} & \colhead{$\delta$} & \colhead{$T_{\mathrm{eff}}$} & \colhead{$\log g$} & \colhead{{[M/H]}} & \colhead{S$_{\mathrm{HK}}$} & \colhead{$\log{R_{HK}}$} & \colhead{$v_{{broad}}$} & \colhead{$v\sin{i}$} & \colhead{$v_{\mathrm{{mac}}}$} & \colhead{$v_{\mathrm{{rad}}}$} & \colhead{S/N} & \colhead{C-rms} & \colhead{L-rms} & \colhead{N} \\
\colhead{ } & \colhead{ } & \colhead{J2000} & \colhead{J2000} & \colhead{(K)} & \colhead{(cm s$^{-2}$)} & \colhead{ } & \colhead{ } & \colhead{ } & \colhead{(km s$^{-1}$)} & \colhead{(km s$^{-1}$)} & \colhead{(km s$^{-1}$)} & \colhead{(km s$^{-1}$)} & \colhead{6000 \AA} & \colhead{ } & \colhead{ } & \colhead{ } \\
\colhead{(1)} & \colhead{(2)} & \colhead{(3)} & \colhead{(4)} & \colhead{(5)} & \colhead{(6)} & \colhead{(7)} & \colhead{(8)} & \colhead{(9)} & \colhead{(10)} & \colhead{(11)} & \colhead{(12)} & \colhead{(13)} & \colhead{(14)} & \colhead{(15)} & \colhead{(16)} & \colhead{(17)}}
\startdata
2281 & KOI-3248 & 19 21 51.6 & +48 19 56 & 5742 & 4.34 & -0.07 & 0.09 & nan & 3.7 & 1.4 & 3.4 & -7.1 & 50 & 0.02 & 0.02 & 1 \\
2361 & KOI-4273 & 19 36 50.4 & +46 28 48 & 6123 & 4.11 & 0.14 & 0.13 & -5.22 & 7.3 & 4.5 & 5.6 & -21.3 & 46 & 0.03 & 0.03 & 1 \\
2393 & KOI-3605 & 19 43 21.2 & +41 25 38 & 5252 & 4.39 & 0.05 & 0.14 & -5.18 & 3.1 & 2.1 & 2.1 & -0.1 & 51 & 0.02 & 0.03 & 1 \\
2405 & KOI-3197 & 19 45 09.7 & +44 25 24 & 6218 & 4.43 & -0.02 & 0.17 & -4.87 & 9.3 & 6.1 & 6.4 & 2.2 & 48 & 0.02 & 0.03 & 1 \\
2430 & KOI-1353 & 19 49 51.7 & +42 52 58 & 5951 & 4.46 & -0.02 & 0.25 & -4.60 & 7.3 & 5.5 & 4.4 & -19.1 & 47 & 0.03 & 0.03 & 1 \\
2435 & KOI-4323 & 19 50 19.7 & +40 31 53 & 6314 & 4.22 & -0.03 & 0.06 & nan & 12.9 & 9.4 & 7.4 & -52.7 & 41 & 0.03 & 0.04 & 1 \\
2445 & KOI-3384 & 19 52 22.9 & +44 44 13 & 5994 & 4.24 & 0.07 & 0.11 & -5.51 & 5.4 & 2.7 & 4.6 & -12.1 & 50 & 0.02 & 0.02 & 1 \\
2460 & KOI-4409 & 19 58 08.4 & +40 28 40 & 5872 & 4.26 & 0.21 & 0.17 & -4.94 & 5.4 & 3.5 & 3.9 & -11.9 & 52 & 0.09 & 0.04 & 1 \\
2464 & KOI-4226 & 20 02 15.0 & +46 02 16 & 5817 & 4.02 & 0.37 & 0.10 & -5.89 & 6.1 & 4.7 & 3.7 & -28.2 & 43 & 0.03 & 0.07 & 1 \\
2485 & K2-58 & 22 15 17.2 & -14 03 00 & 5038 & 4.50 & 0.19 & 0.34 & -4.67 & 2.9 & 2.2 & 1.8 & 2.0 & 94 & 0.02 & 0.02 & 1 \\
2914 & XO-1 & 16 02 11.8 & +28 10 10 & 5731 & 4.51 & -0.07 & 0.00 & 0.00 & 3.8 & 1.7 & 3.3 & 0.1 & 112 & 0.01 & 0.01 & 1 \\
2962 & TRES-4 & 17 53 13.1 & +37 12 42 & 6198 & 4.09 & 0.25 & 0.00 & 0.00 & 11.0 & 8.3 & 6.2 & -16.1 & 77 & 0.02 & 0.02 & 1 \\
2980 & KOI-104 & 18 44 46.7 & +47 29 50 & 4718 & 4.50 & 0.32 & 0.69 & -4.46 & 0.8 & 0.1 & 1.6 & -51.9 & 58 & 0.03 & 0.06 & 1 \\
2981 & KOI-263 & 18 45 05.8 & +47 46 28 & 5821 & 4.15 & -0.13 & 0.10 & -5.95 & 4.3 & 2.1 & 3.7 & -0.4 & 42 & 0.03 & 0.03 & 1 \\
2982 & KOI-10 & 18 45 09.2 & +42 27 04 & 6155 & 4.12 & -0.07 & 0.13 & -5.23 & 12.4 & 9.8 & 5.8 & -55.5 & 48 & 0.03 & 0.03 & 1 \\
2983 & KOI-82 & 18 45 55.9 & +47 12 29 & 4811 & 4.56 & 0.08 & 0.57 & -4.51 & 2.6 & 1.9 & 1.7 & -31.8 & 54 & 0.03 & 0.03 & 1 \\
2986 & KOI-274 & 18 49 58.1 & +43 58 49 & 6119 & 4.12 & 0.00 & 0.11 & -5.54 & 7.9 & 5.3 & 5.5 & -25.6 & 47 & 0.03 & 0.03 & 1 \\
2987 & KOI-22 & 18 50 31.1 & +46 19 24 & 5836 & 4.21 & 0.17 & 0.14 & -5.19 & 4.5 & 2.4 & 3.8 & -14.2 & 48 & 0.02 & 0.03 & 1 \\
2988 & KOI-42 & 18 52 36.2 & +45 08 23 & 6310 & 4.21 & 0.02 & 0.11 & nan & 15.5 & 12.0 & 7.4 & -41.2 & 48 & 0.02 & 0.03 & 1 \\
2989 & KOI-701 & 18 52 51.1 & +45 21 00 & 4838 & 4.53 & -0.31 & 0.22 & -4.96 & 2.0 & 0.8 & 1.7 & 16.6 & 52 & 0.02 & 0.03 & 1 \\
2997 & KOI-245 & 18 56 14.3 & +44 31 05 & 5400 & 4.59 & -0.28 & 0.14 & -5.18 & 2.8 & 1.2 & 2.4 & -31.8 & 51 & 0.02 & 0.02 & 1 \\
2998 & KOI-180 & 18 57 34.6 & +46 14 57 & 5614 & 4.57 & -0.03 & 0.26 & -4.64 & 4.1 & 2.8 & 2.9 & -2.9 & 50 & 0.02 & 0.02 & 1 \\
2999 & KOI-367 & 18 57 53.3 & +39 54 43 & 5688 & 4.42 & 0.10 & 0.15 & -5.04 & 4.0 & 2.4 & 3.2 & -42.0 & 88 & 0.02 & 0.02 & 2 \\
3000 & KOI-122 & 18 57 55.8 & +44 23 53 & 5650 & 4.18 & 0.24 & 0.15 & -5.06 & 4.1 & 2.6 & 3.0 & -36.2 & 48 & 0.02 & 0.03 & 1 \\
3001 & KOI-1612 & 18 59 08.7 & +48 25 24 & 6078 & 4.20 & -0.11 & 0.13 & -5.21 & 5.9 & 2.7 & 5.2 & -56.4 & 49 & 0.02 & 0.03 & 1 \\
3003 & KOI-2169 & 19 00 49.8 & +45 23 04 & 5326 & 4.51 & 0.08 & 0.23 & -4.80 & 3.5 & 2.6 & 2.2 & 5.2 & 53 & 0.02 & 0.03 & 1 \\
3006 & KOI-7 & 19 02 27.7 & +50 08 09 & 5782 & 4.06 & 0.14 & 0.19 & -4.86 & 4.4 & 2.5 & 3.5 & -65.2 & 46 & 0.03 & 0.03 & 1 \\
3007 & KOI-299 & 19 02 38.8 & +37 57 52 & 5497 & 4.49 & 0.11 & 0.19 & -4.89 & 3.2 & 1.7 & 2.6 & -30.7 & 51 & 0.02 & 0.02 & 1 \\
3011 & KOI-1442 & 19 04 08.7 & +49 36 52 & 5496 & 4.32 & 0.35 & 0.12 & -5.33 & 3.5 & 2.3 & 2.6 & -29.5 & 46 & 0.03 & 0.03 & 1 \\
3017 & KOI-244 & 19 06 33.2 & +39 29 16 & 6168 & 4.08 & -0.05 & 0.13 & -5.24 & 11.5 & 8.9 & 5.9 & -9.0 & 47 & 0.02 & 0.03 & 1 \\
3018 & KOI-1 & 19 07 14.0 & +49 19 00 & 5838 & 4.41 & -0.03 & 0.17 & -4.96 & 3.8 & 0.1 & 3.8 & -4.2 & 48 & 0.06 & 0.03 & 1 \\
3020 & KOI-1431 & 19 08 05.3 & +48 40 55 & 5478 & 4.42 & 0.20 & 0.10 & -5.50 & 3.7 & 2.6 & 2.5 & -38.5 & 51 & 0.02 & 0.02 & 1 \\
3022 & KOI-292 & 19 09 18.4 & +48 40 24 & 5800 & 4.48 & -0.20 & 0.12 & -5.31 & 3.8 & 0.9 & 3.6 & 5.4 & 49 & 0.02 & 0.02 & 1 \\
3024 & Kepler-174 & 19 09 45.4 & +43 49 56 & 4730 & 4.45 & -0.46 & 0.00 & 0.00 & 2.1 & 1.2 & 1.6 & -98.1 & 61 & 0.05 & 0.05 & 1 \\
3025 & KOI-273 & 19 09 54.9 & +38 13 44 & 5620 & 4.28 & 0.22 & 0.10 & -5.65 & 4.1 & 2.7 & 2.9 & -74.6 & 48 & 0.02 & 0.03 & 1 \\
3026 & KOI-111 & 19 10 25.1 & +42 10 00 & 5903 & 4.44 & -0.38 & 0.17 & -4.95 & 3.8 & 0.1 & 4.1 & -4.4 & 38 & 0.03 & 0.03 & 1 \\
3027 & KOI-1781 & 19 10 25.3 & +49 31 24 & 4825 & 4.48 & 0.10 & 0.28 & -4.83 & 4.7 & 4.3 & 1.7 & -21.7 & 57 & 0.03 & 0.03 & 1 \\
3031 & KOI-70 & 19 10 47.5 & +42 20 19 & 5482 & 4.47 & 0.03 & 0.17 & -4.98 & 3.4 & 2.1 & 2.6 & -25.3 & 46 & 0.03 & 0.03 & 1 \\
3032 & KOI-98 & 19 10 50.1 & +47 19 59 & 6392 & 3.99 & 0.08 & 0.12 & -5.46 & 11.1 & 4.8 & 9.8 & 2.6 & 45 & 0.03 & 0.03 & 1 \\
3034 & KOI-153 & 19 11 59.5 & +50 56 40 & 4715 & 4.47 & 0.14 & 0.15 & -5.19 & 1.7 & 0.3 & 1.6 & -0.9 & 56 & 0.02 & 0.03 & 1 \\
3036 & KOI-262 & 19 12 24.2 & +50 02 01 & 6205 & 4.08 & -0.04 & 0.14 & -5.14 & 12.2 & 9.4 & 6.3 & -4.5 & 48 & 0.02 & 0.03 & 1 \\
3040 & KOI-283 & 19 14 07.4 & +40 56 32 & 5749 & 4.46 & 0.13 & 0.15 & -5.05 & 3.8 & 1.6 & 3.4 & -25.4 & 48 & 0.02 & 0.03 & 1 \\
3041 & KOI-97 & 19 14 19.6 & +41 05 23 & 6067 & 4.03 & 0.23 & 0.10 & -6.16 & 5.1 & 0.0 & 5.1 & -0.0 & 49 & 0.02 & 0.03 & 1 \\
3042 & KOI-85 & 19 14 45.3 & +41 09 04 & 6145 & 4.14 & 0.15 & 0.12 & -5.34 & 10.7 & 8.2 & 5.7 & -19.5 & 49 & 0.02 & 0.03 & 1 \\
3043 & KOI-108 & 19 15 56.3 & +40 03 52 & 5882 & 4.16 & 0.12 & 0.15 & -5.09 & 5.4 & 3.5 & 4.0 & -33.2 & 46 & 0.02 & 0.03 & 1 \\
3045 & KOI-87 & 19 16 52.2 & +47 53 04 & 5614 & 4.59 & -0.25 & 0.14 & -5.14 & 3.3 & 1.5 & 2.9 & -8.5 & 47 & 0.03 & 0.03 & 1 \\
3046 & KOI-63 & 19 16 54.3 & +49 32 53 & 5477 & 4.45 & 0.09 & 0.35 & -4.44 & 6.6 & 5.8 & 2.5 & -26.3 & 74 & 0.02 & 0.03 & 2 \\
3048 & KOI-260 & 19 17 23.4 & +44 12 31 & 6285 & 4.23 & -0.10 & 0.12 & -5.33 & 11.0 & 7.6 & 7.1 & -22.7 & 48 & 0.02 & 0.03 & 1 \\
3054 & KOI-5 & 19 18 57.5 & +44 38 51 & 5834 & 4.08 & 0.12 & 0.10 & -5.96 & 10.5 & 8.8 & 3.8 & -39.7 & 48 & 0.03 & 0.03 & 1 \\
3055 & KOI-3158 & 19 19 00.6 & +41 38 05 & 5024 & 4.55 & -0.39 & 0.19 & -4.97 & 1.1 & 0.1 & 1.8 & -120.0 & 54 & 0.02 & 0.03 & 1 \\
3058 & KOI-123 & 19 21 34.3 & +40 17 05 & 5937 & 4.22 & -0.02 & 0.17 & -4.93 & 5.0 & 2.4 & 4.3 & -41.5 & 45 & 0.03 & 0.03 & 1 \\
3059 & KOI-84 & 19 21 41.0 & +37 51 06 & 5537 & 4.55 & -0.08 & 0.15 & -5.07 & 3.2 & 1.5 & 2.7 & -15.2 & 47 & 0.02 & 0.03 & 1 \\
3064 & KOI-277 & 19 25 00.0 & +49 13 55 & 5980 & 4.05 & -0.17 & 0.12 & -5.45 & 6.2 & 4.0 & 4.5 & 6.4 & 48 & 0.02 & 0.03 & 1 \\
3065 & KOI-41 & 19 25 32.6 & +41 59 25 & 5857 & 4.13 & 0.09 & 0.18 & -4.89 & 5.1 & 3.2 & 3.9 & -62.1 & 48 & 0.02 & 0.03 & 1 \\
3067 & KOI-69 & 19 25 40.4 & +38 40 20 & 5650 & 4.48 & -0.14 & 0.14 & -5.18 & 3.5 & 1.5 & 3.0 & 26.5 & 50 & 0.02 & 0.02 & 1 \\
3068 & KOI-75 & 19 25 59.3 & +42 43 42 & 5870 & 3.75 & -0.09 & 0.11 & -5.52 & 6.9 & 4.7 & 4.8 & -12.7 & 49 & 0.02 & 0.03 & 1 \\
3072 & KOI-103 & 19 26 44.0 & +37 45 06 & 5551 & 4.57 & -0.07 & 0.17 & -4.95 & 3.4 & 1.8 & 2.7 & 4.6 & 36 & 0.04 & 0.04 & 1 \\
3074 & KOI-321 & 19 27 23.5 & +44 58 06 & 5586 & 4.34 & 0.22 & 0.27 & -4.62 & 3.8 & 2.4 & 2.8 & -62.9 & 46 & 0.03 & 0.03 & 1 \\
3078 & KOI-2687 & 19 30 27.6 & +42 45 51 & 5746 & 4.50 & -0.01 & 0.17 & -4.92 & 4.8 & 3.2 & 3.4 & 7.9 & 49 & 0.02 & 0.02 & 1 \\
3084 & KOI-1925 & 19 34 43.0 & +46 51 10 & 5394 & 4.47 & 0.04 & 0.16 & -5.03 & 3.5 & 2.4 & 2.4 & -29.0 & 260 & 0.01 & 0.01 & 1 \\
3091 & KOI-1924 & 19 37 08.9 & +40 12 50 & 5898 & 3.90 & 0.31 & 0.09 & nan & 6.7 & 4.3 & 4.9 & -17.2 & 49 & 0.02 & 0.03 & 1 \\
3100 & KOI-99 & 19 41 44.2 & +44 31 52 & 4957 & 4.48 & -0.20 & 0.50 & -4.51 & 1.4 & 0.1 & 1.8 & -71.3 & 53 & 0.02 & 0.03 & 1 \\
3101 & KOI-2720 & 19 41 45.5 & +44 02 21 & 5931 & 4.03 & -0.14 & 0.13 & -5.24 & 5.2 & 2.9 & 4.3 & -11.6 & 49 & 0.02 & 0.03 & 1 \\
3103 & KOI-364 & 19 43 29.4 & +42 52 52 & 5770 & 4.15 & 0.23 & 0.14 & -5.19 & 4.3 & 2.4 & 3.5 & 2.4 & 50 & 0.02 & 0.02 & 1 \\
3105 & KOI-64 & 19 46 02.5 & +42 32 51 & 5257 & 3.77 & 0.00 & 0.12 & -5.27 & 4.1 & 1.8 & 3.6 & -28.7 & 52 & 0.02 & 0.02 & 1 \\
3110 & KOI-174 & 19 47 17.5 & +48 06 27 & 4703 & 4.35 & -0.18 & 0.19 & -5.08 & 2.1 & 1.2 & 1.6 & -100.5 & 49 & 0.03 & 0.03 & 1 \\
3111 & KOI-17 & 19 47 20.9 & +48 14 24 & 5638 & 4.24 & 0.30 & 0.09 & -6.49 & 3.7 & 2.1 & 3.0 & -50.2 & 51 & 0.02 & 0.02 & 1 \\
3113 & KOI-265 & 19 48 04.5 & +50 24 32 & 6041 & 4.32 & 0.18 & 0.14 & -5.14 & 4.7 & 0.1 & 4.9 & -9.2 & 47 & 0.02 & 0.03 & 1 \\
3114 & KOI-261 & 19 48 16.7 & +40 31 31 & 5740 & 4.53 & 0.04 & 0.17 & -4.95 & 3.9 & 1.9 & 3.4 & -48.1 & 49 & 0.02 & 0.02 & 1 \\
3117 & KOI-305 & 19 49 25.0 & +41 18 00 & 4786 & 4.56 & 0.23 & 0.37 & -4.72 & 1.2 & 0.1 & 1.6 & -25.8 & 57 & 0.02 & 0.03 & 1 \\
3118 & KOI-365 & 19 49 56.9 & +49 37 24 & 5486 & 4.53 & -0.16 & 0.16 & -5.01 & 3.0 & 1.2 & 2.6 & -39.0 & 49 & 0.02 & 0.03 & 2 \\
3123 & KOI-137 & 19 52 19.1 & +44 44 47 & 5361 & 4.38 & 0.19 & 0.11 & -5.39 & 3.1 & 2.0 & 2.3 & -21.8 & 47 & 0.03 & 0.03 & 1 \\
3130 & KOI-148 & 19 56 33.4 & +40 56 56 & 5169 & 4.46 & 0.20 & 0.23 & -4.83 & 2.7 & 1.7 & 2.0 & -14.8 & 54 & 0.02 & 0.02 & 1 \\
3131 & KOI-18 & 19 57 37.7 & +44 02 06 & 6344 & 4.10 & 0.08 & 0.11 & -5.54 & 6.4 & 0.1 & 7.8 & -18.4 & 50 & 0.02 & 0.03 & 1 \\
3133 & KOI-116 & 20 03 27.4 & +44 20 15 & 5933 & 4.46 & -0.07 & 0.17 & -4.89 & 4.0 & 0.1 & 4.3 & -58.1 & 49 & 0.02 & 0.02 & 1 \\
3239 & HD 240429 & 23 51 55.0 & +59 42 49 & 5883 & 4.43 & 0.01 & 0.00 & 0.00 & 4.3 & 1.2 & 4.0 & -20.7 & 250 & 0.01 & 0.01 & 2 \\
3240 & HD 240430 & 23 52 09.2 & +59 42 27 & 5819 & 4.36 & 0.18 & 0.00 & 0.00 & 4.6 & 2.6 & 3.7 & -20.4 & 250 & 0.01 & 0.01 & 2 \\
3248 & WASP-57 & 14 55 16.8 & -02 03 28 & 5799 & 4.42 & 0.06 & 0.00 & 0.00 & 4.6 & 2.7 & 3.6 & -23.5 & 80 & 0.02 & 0.02 & 1 \\
3249 & WASP-74 & 20 18 09.3 & -01 04 33 & 5892 & 4.18 & 0.39 & 0.00 & 0.00 & 6.7 & 5.0 & 4.0 & -14.2 & 178 & 0.01 & 0.01 & 1 \\
3250 & WASP-37 & 14 47 46.6 & +01 03 54 & 5908 & 4.50 & -0.21 & 0.00 & 0.00 & 4.3 & 0.9 & 4.1 & 7.0 & 78 & 0.01 & 0.04 & 1 \\
3251 & HAT-P-41 & 19 49 17.4 & +04 40 21 & 6419 & 4.15 & 0.18 & 0.00 & 0.00 & 24.9 & 19.9 & 8.8 & 33.2 & 109 & 0.02 & 0.02 & 1 \\
3252 & COROT-28 & 18 34 45.2 & +05 34 25 & 5323 & 3.73 & 0.24 & 0.00 & 0.00 & 4.3 & 2.2 & 3.6 & -76.6 & 75 & 0.02 & 0.02 & 1 \\
3253 & HAT-P-27 & 14 51 04.2 & +05 56 51 & 5233 & 4.43 & 0.27 & 0.00 & 0.00 & 3.2 & 2.4 & 2.1 & -18.2 & 119 & 0.02 & 0.02 & 1 \\
3254 & WASP-103 & 16 37 15.6 & +07 11 00 & 6047 & 4.20 & 0.20 & 0.00 & 0.00 & 12.1 & 9.7 & 5.0 & -44.7 & 110 & 0.02 & 0.03 & 1 \\
3255 & WASP-52 & 23 13 58.8 & +08 45 41 & 5085 & 4.42 & 0.23 & 0.00 & 0.00 & 3.8 & 3.2 & 1.9 & -1.4 & 123 & 0.01 & 0.02 & 1 \\
3256 & WASP-114 & 21 50 39.7 & +10 27 47 & 5945 & 4.25 & 0.30 & 0.00 & 0.00 & 6.6 & 4.7 & 4.3 & -4.3 & 97 & 0.02 & 0.02 & 1 \\
3257 & BD+1290 & 00 47 43.6 & +12 52 20 & 5855 & 4.13 & -0.06 & 0.14 & -5.10 & 4.5 & 2.3 & 3.9 & 12.5 & 174 & 0.02 & 0.04 & 1 \\
3258 & HD 4552 & 00 47 41.2 & +12 52 45 & 6124 & 4.17 & 0.00 & 0.15 & -5.07 & 9.7 & 7.3 & 5.6 & 12.8 & 171 & 0.02 & 0.02 & 1 \\
3259 & HD 209622 & 22 04 30.1 & +15 51 28 & 6035 & 4.14 & 0.29 & 0.00 & 0.00 & 10.2 & 8.1 & 4.9 & -29.5 & 179 & 0.01 & 0.02 & 1 \\
3260 & BD+15_4556 & 22 04 27.4 & +15 52 17 & 4859 & 2.83 & 0.13 & 0.00 & 0.00 & 4.5 & 2.0 & 4.0 & 21.7 & 197 & 0.01 & 0.02 & 1 \\
3261 & HAT-P-23 & 20 24 29.7 & +16 45 44 & 6027 & 4.49 & 0.20 & 0.00 & 0.00 & 10.0 & 8.0 & 4.8 & -13.3 & 140 & 0.01 & 0.01 & 1 \\
3262 & HAT-P-55 & 17 37 05.6 & +25 43 52 & 5783 & 4.39 & -0.05 & 0.00 & 0.00 & 3.6 & 0.1 & 3.5 & -12.5 & 94 & 0.02 & 0.02 & 1 \\
3263 & HAT-P-31 & 18 06 09.1 & +26 25 36 & 5966 & 4.12 & 0.09 & 0.00 & 0.00 & 4.9 & 1.8 & 4.5 & -3.3 & 111 & 0.01 & 0.02 & 1 \\
3264 & BD+28_4543S & 23 11 11.8 & +29 18 49 & 5080 & 3.18 & 0.03 & 0.00 & 0.00 & 4.4 & 2.5 & 3.5 & 11.3 & 247 & 0.01 & 0.02 & 1 \\
3265 & WASP-135 & 17 49 08.4 & +29 52 45 & 5116 & 4.34 & 0.36 & 0.00 & 0.00 & 3.8 & 3.2 & 1.9 & -31.7 & 94 & 0.03 & 0.02 & 1 \\
3266 & WASP-10 & 23 15 58.3 & +31 27 46 & 4755 & 4.46 & 0.12 & 0.00 & 0.00 & 3.8 & 3.4 & 1.6 & -11.9 & 126 & 0.02 & 0.03 & 1 \\
3267 & KELT-16 & 20 57 04.4 & +31 39 40 & 6277 & 4.08 & -0.02 & 0.00 & 0.00 & 7.6 & 3.0 & 7.0 & -29.2 & 108 & 0.01 & 0.02 & 1 \\
3268 & HAT-P-18 & 17 05 23.2 & +33 00 45 & 4785 & 4.50 & 0.13 & 0.00 & 0.00 & 2.5 & 1.8 & 1.6 & -13.5 & 117 & 0.02 & 0.02 & 1 \\
3269 & HAT-P-4 & 15 19 57.9 & +36 13 47 & 5904 & 4.14 & 0.27 & 0.00 & 0.00 & 7.3 & 5.5 & 4.1 & -2.7 & 112 & 0.01 & 0.02 & 1 \\
3270 & KELT-12 & 17 50 33.7 & +36 34 13 & 6232 & 4.04 & 0.28 & 0.00 & 0.00 & 13.3 & 10.3 & 6.5 & -23.1 & 171 & 0.01 & 0.01 & 1 \\
3271 & KOI-958 & 19 25 01.1 & +36 44 37 & 4835 & 4.50 & -0.05 & 0.33 & -4.76 & 3.1 & 2.5 & 1.7 & -30.0 & 53 & 0.03 & 0.03 & 1 \\
3272 & KOI-1010 & 19 25 25.0 & +36 47 04 & 6128 & 4.21 & -0.02 & 0.13 & -5.23 & 9.1 & 6.6 & 5.6 & -41.0 & 42 & 0.03 & 0.03 & 1 \\
3273 & KOI-984 & 19 24 11.7 & +36 50 24 & 5223 & 4.47 & 0.18 & 0.51 & -4.40 & 6.7 & 6.1 & 2.1 & -29.4 & 50 & 0.03 & 0.03 & 1 \\
3274 & KOI-4212 & 19 28 49.1 & +37 13 16 & 6118 & 4.24 & 0.13 & 0.10 & -5.81 & 8.3 & 5.7 & 5.5 & -17.2 & 48 & 0.02 & 0.03 & 1 \\
3275 & KOI-1002 & 19 22 43.7 & +37 21 18 & 5352 & 4.35 & 0.03 & 0.15 & -5.08 & 3.2 & 2.1 & 2.3 & -52.4 & 50 & 0.02 & 0.03 & 1 \\
3276 & KOI-2538 & 19 05 08.6 & +37 23 13 & 4948 & 4.46 & -0.21 & 0.10 & -5.39 & 7.4 & 6.8 & 1.8 & 29.4 & 47 & 0.02 & 0.03 & 1 \\
3277 & KOI-2534 & 19 05 22.6 & +37 24 43 & 6091 & 4.35 & 0.02 & 0.15 & -5.06 & 6.1 & 2.9 & 5.3 & -5.3 & 45 & 0.03 & 0.03 & 1 \\
3278 & KOI-3233 & 19 06 28.6 & +37 30 15 & 5758 & 4.49 & -0.04 & 0.10 & -6.06 & 3.8 & 1.4 & 3.4 & -36.5 & 50 & 0.02 & 0.02 & 1 \\
3279 & KOI-2403 & 19 06 30.2 & +37 32 14 & 6077 & 4.27 & 0.15 & 0.15 & -5.06 & 6.9 & 4.4 & 5.2 & -30.1 & 47 & 0.02 & 0.03 & 1 \\
3280 & KOI-2201 & 19 05 28.8 & +37 33 09 & 6009 & 4.08 & 0.18 & 0.13 & -5.25 & 9.2 & 7.2 & 4.7 & -9.5 & 49 & 0.02 & 0.03 & 1 \\
3281 & KOI-988 & 19 25 27.6 & +37 36 33 & 4997 & 4.51 & 0.02 & 0.34 & -4.67 & 3.7 & 3.2 & 1.8 & -25.6 & 52 & 0.02 & 0.03 & 1 \\
3282 & KOI-151 & 19 29 30.0 & +37 37 51 & 6194 & 4.20 & -0.05 & 0.12 & -5.39 & 11.0 & 8.2 & 6.2 & -20.0 & 48 & 0.02 & 0.03 & 1 \\
3283 & KOI-113 & 19 29 05.7 & +37 40 18 & 5464 & 4.06 & 0.31 & 0.13 & -5.26 & 3.6 & 2.5 & 2.5 & -87.1 & 51 & 0.02 & 0.02 & 1 \\
3284 & KOI-3201 & 19 28 19.3 & +37 40 29 & 5811 & 4.52 & -0.42 & 0.13 & -5.22 & 3.5 & 0.1 & 3.7 & -28.1 & 49 & 0.02 & 0.02 & 1 \\
3285 & KOI-2053 & 19 29 41.1 & +37 40 58 & 6061 & 4.15 & 0.03 & 0.14 & -5.13 & 8.5 & 6.3 & 5.1 & -45.8 & 48 & 0.02 & 0.03 & 1 \\
3286 & KOI-2033 & 19 26 58.0 & +37 41 20 & 5004 & 4.48 & -0.13 & 0.20 & -4.94 & 2.5 & 1.6 & 1.8 & -11.6 & 47 & 0.03 & 0.03 & 1 \\
3287 & KOI-1944 & 19 21 18.9 & +37 43 23 & 5700 & 4.55 & -0.01 & 0.22 & -4.76 & 4.7 & 3.3 & 3.2 & -38.2 & 50 & 0.02 & 0.05 & 1 \\
3288 & KOI-2603 & 19 25 49.8 & +37 44 35 & 6229 & 4.07 & -0.05 & 0.10 & -5.82 & 11.5 & 8.6 & 6.5 & 5.9 & 47 & 0.02 & 0.03 & 1 \\
3289 & KOI-440 & 19 21 11.2 & +37 44 58 & 5041 & 4.59 & 0.15 & 0.33 & -4.67 & 2.9 & 2.2 & 1.8 & -27.8 & 51 & 0.22 & 0.08 & 1 \\
3290 & KOI-166 & 19 24 05.2 & +37 46 11 & 5166 & 4.54 & -0.26 & 0.24 & -4.81 & 1.9 & 0.1 & 2.0 & -33.7 & 51 & 0.02 & 0.02 & 1 \\
3291 & KOI-379 & 19 28 13.6 & +37 46 34 & 6044 & 3.94 & 0.15 & 0.14 & -5.17 & 9.1 & 6.5 & 5.8 & -22.4 & 48 & 0.03 & 0.04 & 1 \\
3292 & KOI-2009 & 19 31 05.8 & +37 47 52 & 5780 & 4.54 & -0.20 & 0.12 & -5.32 & 3.4 & 0.1 & 3.5 & -4.8 & 49 & 0.02 & 0.04 & 1 \\
3293 & KOI-4581 & 19 22 25.9 & +37 48 07 & 5879 & 4.36 & 0.07 & 0.11 & -5.62 & 4.2 & 1.1 & 4.0 & -37.4 & 50 & 0.02 & 0.02 & 1 \\
3294 & KOI-3835 & 19 30 45.7 & +37 50 06 & 4896 & 4.45 & -0.04 & 0.62 & -4.43 & 5.3 & 4.9 & 1.7 & -24.3 & 54 & 0.02 & 0.03 & 1 \\
3295 & KOI-3681 & 19 30 30.6 & +37 51 36 & 6157 & 4.28 & 0.16 & 0.08 & nan & 9.9 & 7.3 & 5.8 & -27.3 & 47 & 0.03 & 0.03 & 1 \\
3296 & KOI-3853 & 19 09 52.3 & +37 58 00 & 4906 & 3.63 & -0.03 & 0.12 & -5.25 & 3.8 & 1.4 & 3.4 & -94.5 & 55 & 0.02 & 0.03 & 1 \\
3297 & KOI-2979 & 19 32 17.0 & +37 59 13 & 6040 & 4.27 & -0.13 & 0.10 & -6.24 & 4.2 & 0.1 & 4.9 & -30.1 & 48 & 0.02 & 0.03 & 1 \\
3298 & KOI-986 & 19 27 42.2 & +38 00 51 & 5435 & 4.45 & 0.18 & 0.31 & -4.59 & 3.7 & 2.7 & 2.4 & -27.4 & 47 & 0.03 & 0.03 & 1 \\
3299 & KOI-2896 & 19 26 57.6 & +38 00 54 & 6208 & 4.38 & 0.02 & 0.12 & -5.29 & 17.4 & 13.9 & 6.3 & -19.0 & 47 & 0.03 & 0.03 & 1 \\
3300 & KOI-4659 & 19 30 03.5 & +38 01 19 & 5610 & 4.46 & -0.08 & 0.15 & -5.06 & 3.5 & 1.8 & 2.9 & -27.9 & 41 & 0.03 & 0.03 & 1 \\
3301 & KOI-1118 & 19 26 36.2 & +38 01 41 & 6022 & 4.28 & -0.05 & 0.12 & -5.43 & 5.2 & 1.7 & 4.8 & 16.1 & 49 & 0.02 & 0.02 & 1 \\
3302 & KOI-4298 & 19 26 10.4 & +38 02 56 & 6150 & 4.09 & -0.34 & 0.12 & -5.41 & 5.2 & 0.1 & 5.8 & -50.2 & 44 & 0.03 & 0.03 & 1 \\
3303 & KOI-1113 & 19 27 54.3 & +38 03 18 & 6079 & 4.26 & 0.06 & 0.11 & -5.62 & 6.8 & 4.1 & 5.2 & 14.5 & 48 & 0.02 & 0.03 & 1 \\
3304 & KOI-1116 & 19 23 32.3 & +38 03 27 & 5775 & 4.40 & 0.02 & 0.11 & -5.48 & 4.2 & 2.2 & 3.5 & -22.3 & 48 & 0.03 & 0.03 & 1 \\
3305 & KOI-2081 & 19 26 55.0 & +38 04 12 & 4976 & 3.48 & 0.13 & 0.12 & -5.24 & 3.2 & 0.1 & 3.4 & -16.2 & 48 & 0.02 & 0.03 & 1 \\
3306 & KOI-4400 & 19 02 03.1 & +38 04 47 & 5843 & 4.51 & -0.00 & 0.17 & -4.94 & 4.0 & 1.1 & 3.8 & -18.1 & 50 & 0.02 & 0.05 & 1 \\
3307 & KOI-1824 & 19 25 31.7 & +38 07 39 & 5952 & 4.28 & -0.18 & 0.13 & -5.23 & 5.0 & 2.2 & 4.4 & 12.2 & 48 & 0.02 & 0.03 & 1 \\
3308 & KOI-2807 & 19 21 55.2 & +38 08 12 & 6288 & 4.15 & 0.15 & 0.09 & nan & 16.6 & 13.0 & 7.1 & -17.2 & 47 & 0.03 & 0.09 & 1 \\
3309 & KOI-2335 & 19 26 47.9 & +38 08 43 & 5586 & 4.51 & -0.07 & 0.18 & -4.93 & 3.5 & 1.9 & 2.8 & -10.3 & 48 & 0.02 & 0.03 & 1 \\
3310 & KOI-197 & 19 23 20.0 & +38 11 04 & 4849 & 4.49 & 0.04 & 0.25 & -4.88 & 2.8 & 2.2 & 1.7 & -17.7 & 35 & 0.05 & 0.06 & 1 \\
3311 & KOI-4144 & 19 21 20.9 & +38 12 18 & 5978 & 4.39 & -0.11 & 0.13 & -5.18 & 5.1 & 2.1 & 4.5 & 18.7 & 36 & 0.03 & 0.03 & 1 \\
3312 & KOI-1115 & 19 25 41.7 & +38 13 00 & 5577 & 3.96 & 0.04 & 0.09 & -6.12 & 4.0 & 0.4 & 4.0 & -38.3 & 50 & 0.03 & 0.06 & 1 \\
3313 & HAT-P-14 & 17 20 27.9 & +38 14 32 & 6534 & 4.08 & 0.01 & 0.00 & 0.00 & 10.6 & 2.3 & 10.6 & -20.0 & 239 & 0.01 & 0.01 & 1 \\
3314 & KOI-1878 & 19 04 53.6 & +38 15 29 & 6132 & 4.26 & 0.18 & 0.14 & -5.15 & 8.5 & 5.9 & 5.6 & -15.7 & 48 & 0.02 & 0.03 & 1 \\
3315 & KOI-3277 & 19 29 41.5 & +38 15 59 & 5905 & 3.75 & -0.04 & 0.13 & -5.25 & 9.0 & 6.9 & 5.0 & -48.7 & 49 & 0.02 & 0.03 & 1 \\
3316 & KOI-3203 & 19 31 34.1 & +38 16 14 & 6454 & 3.86 & -0.18 & 0.15 & -5.04 & 19.4 & 14.0 & 11.1 & -10.6 & 47 & 0.03 & 0.03 & 1 \\
3317 & KOI-3225 & 19 18 41.2 & +38 17 52 & 5312 & 4.49 & 0.08 & 0.14 & -5.12 & 3.5 & 2.6 & 2.2 & -20.6 & 52 & 0.05 & 0.03 & 1 \\
3318 & Kepler-24 & 19 21 39.2 & +38 20 38 & 6097 & 4.39 & -0.03 & 0.00 & 0.00 & 7.0 & 4.3 & 5.4 & 3.0 & 38 & 0.05 & 0.04 & 1 \\
3319 & KOI-490 & 19 30 38.0 & +38 20 43 & 4799 & 4.49 & 0.03 & 0.26 & -4.89 & 2.1 & 1.1 & 1.6 & -31.1 & 51 & 0.07 & 0.06 & 1 \\
3320 & KOI-1089 & 19 37 44.0 & +38 21 20 & 5858 & 4.49 & 0.09 & 0.18 & -4.89 & 4.0 & 0.9 & 3.9 & -15.6 & 28 & 0.05 & 0.05 & 1 \\
3321 & KOI-2863 & 19 32 18.7 & +38 21 33 & 5801 & 4.49 & -0.23 & 0.13 & -5.20 & 3.3 & 0.1 & 3.6 & -63.8 & 46 & 0.02 & 0.04 & 1 \\
3322 & KOI-3515 & 19 30 51.2 & +38 22 11 & 6299 & 4.23 & -0.22 & 0.06 & nan & 7.4 & 1.6 & 7.2 & -5.2 & 47 & 0.03 & 0.03 & 1 \\
3323 & KOI-401 & 19 03 24.9 & +38 23 03 & 5330 & 4.40 & 0.25 & 0.15 & -5.08 & 2.8 & 1.6 & 2.2 & -8.2 & 67 & 0.02 & 0.02 & 1 \\
3324 & KOI-2278 & 19 26 25.7 & +38 24 37 & 5907 & 4.19 & -0.14 & 0.14 & -5.12 & 4.3 & 1.1 & 4.1 & -56.1 & 46 & 0.03 & 0.03 & 1 \\
3325 & KOI-3172 & 19 20 08.0 & +38 25 38 & 6049 & 4.00 & -0.00 & 0.11 & -5.65 & 7.8 & 5.5 & 5.0 & 8.9 & 48 & 0.03 & 0.03 & 1 \\
3326 & KOI-2974 & 19 19 18.6 & +38 26 33 & 6361 & 3.87 & 0.11 & 0.17 & -4.91 & 16.2 & 11.7 & 9.3 & -65.3 & 44 & 0.03 & 0.03 & 1 \\
3327 & KOI-384 & 19 36 35.9 & +38 27 30 & 6090 & 3.90 & 0.03 & 0.12 & -5.36 & 7.4 & 4.0 & 6.1 & -17.1 & 49 & 0.02 & 0.03 & 1 \\
3328 & KOI-2740 & 19 19 49.4 & +38 27 49 & 6091 & 4.20 & -0.19 & 0.11 & -5.51 & 8.8 & 6.4 & 5.3 & -31.8 & 48 & 0.02 & 0.03 & 1 \\
3329 & KOI-1196 & 19 31 41.5 & +38 28 38 & 5711 & 4.25 & -0.18 & 0.12 & -5.36 & 3.8 & 1.7 & 3.2 & -60.3 & 36 & 0.03 & 0.03 & 1 \\
3330 & KOI-1845 & 19 22 11.7 & +38 29 43 & 4780 & 4.49 & 0.34 & 0.43 & -4.65 & 2.3 & 1.5 & 1.6 & -10.8 & 37 & 0.03 & 0.04 & 1 \\
3331 & KOI-3075 & 19 08 49.4 & +38 29 53 & 5435 & 4.58 & -0.43 & 0.19 & -4.91 & 2.4 & 0.1 & 2.5 & -93.2 & 49 & 0.02 & 0.02 & 1 \\
3332 & KOI-268 & 19 02 54.9 & +38 30 25 & 6382 & 4.29 & 0.03 & 0.12 & -5.30 & 10.5 & 6.0 & 8.3 & -43.1 & 48 & 0.02 & 0.03 & 1 \\
3333 & KOI-2043 & 19 30 21.1 & +38 31 19 & 5862 & 4.37 & 0.00 & 0.10 & -6.06 & 4.2 & 1.3 & 3.9 & -53.9 & 40 & 0.03 & 0.03 & 1 \\
3334 & KOI-3876 & 19 21 45.8 & +38 31 25 & 5642 & 4.46 & 0.04 & 0.47 & -4.30 & 12.0 & 10.4 & 3.0 & -25.1 & 51 & 0.06 & 0.03 & 1 \\
3335 & KOI-1218 & 19 24 04.6 & +38 32 44 & 5637 & 4.42 & -0.06 & 0.13 & -5.24 & 3.7 & 2.1 & 3.0 & -36.7 & 47 & 0.02 & 0.03 & 1 \\
3336 & KOI-385 & 19 28 51.6 & +38 32 55 & 5463 & 4.49 & 0.06 & 0.17 & -4.98 & 2.5 & 0.1 & 2.5 & -20.0 & 49 & 0.02 & 0.02 & 1 \\
3337 & KOI-3415 & 19 14 11.8 & +38 33 55 & 5253 & 4.54 & -1.07 & 0.18 & -4.97 & 6.6 & 5.4 & 2.1 & 7.8 & 50 & 0.05 & 0.06 & 1 \\
3338 & KOI-3340 & 19 06 02.5 & +38 37 06 & 6086 & 4.23 & -0.06 & 0.08 & nan & 8.3 & 5.9 & 5.3 & 13.4 & 50 & 0.08 & 0.04 & 1 \\
3339 & KOI-3641 & 19 13 18.7 & +38 37 39 & 6163 & 4.11 & -0.08 & 0.12 & -5.47 & 5.4 & 0.1 & 5.9 & -17.4 & 48 & 0.02 & 0.03 & 1 \\
3340 & KOI-118 & 19 09 27.1 & +38 38 59 & 5764 & 4.20 & 0.03 & 0.12 & -5.42 & 4.0 & 1.8 & 3.5 & -28.0 & 49 & 0.02 & 0.02 & 1 \\
3341 & KOI-2755 & 19 26 17.8 & +38 39 21 & 5815 & 4.49 & -0.17 & 0.14 & -5.13 & 4.2 & 1.8 & 3.7 & -23.9 & 50 & 0.02 & 0.03 & 1 \\
3342 & KOI-2194 & 19 29 18.4 & +38 39 27 & 5908 & 4.53 & -0.18 & 0.15 & -5.07 & 3.7 & 0.1 & 4.1 & 19.4 & 43 & 0.03 & 0.03 & 1 \\
3343 & KOI-6102 & 19 27 00.5 & +38 39 45 & 6530 & 3.77 & 0.13 & 0.15 & -5.00 & 14.3 & 6.0 & 12.9 & -11.4 & 48 & 0.03 & 0.07 & 1 \\
3344 & KOI-624 & 19 22 41.6 & +38 41 28 & 5573 & 4.51 & 0.01 & 0.21 & -4.81 & 4.5 & 3.4 & 2.8 & -25.2 & 50 & 0.02 & 0.02 & 1 \\
3345 & KOI-1221 & 19 20 25.7 & +38 42 08 & 4893 & 3.55 & 0.30 & 0.17 & -5.03 & 2.9 & 0.1 & 3.4 & -48.1 & 70 & 0.02 & 0.03 & 2 \\
3346 & KOI-386 & 19 36 26.6 & +38 42 37 & 5981 & 4.38 & 0.06 & 0.11 & -5.53 & 5.2 & 2.4 & 4.5 & 5.2 & 47 & 0.02 & 0.03 & 1 \\
3347 & KOI-975 & 19 09 26.8 & +38 42 50 & 6207 & 4.06 & -0.01 & 0.12 & -5.41 & 9.5 & 6.5 & 6.3 & -19.0 & 53 & 0.02 & 0.02 & 1 \\
3348 & KOI-2279 & 19 41 41.3 & +38 44 08 & 5919 & 4.27 & 0.04 & 0.12 & -5.32 & 4.7 & 2.0 & 4.2 & -14.2 & 46 & 0.03 & 0.03 & 1 \\
3349 & KOI-302 & 19 42 26.1 & +38 44 09 & 6578 & 4.08 & 0.14 & 0.17 & -4.90 & 19.3 & 13.7 & 11.4 & -23.7 & 46 & 0.03 & 0.03 & 1 \\
3350 & KOI-1901 & 19 05 36.6 & +38 44 19 & 6034 & 4.36 & 0.18 & 0.13 & -5.22 & 6.0 & 3.3 & 4.9 & -27.4 & 47 & 0.02 & 0.03 & 1 \\
3351 & KOI-1861 & 19 28 39.9 & +38 44 21 & 6004 & 4.54 & 0.03 & 0.26 & -4.57 & 9.5 & 7.5 & 4.7 & 14.8 & 47 & 0.02 & 0.03 & 1 \\
3352 & KOI-3308 & 19 08 56.6 & +38 45 15 & 5871 & 4.12 & 0.02 & 0.12 & -5.36 & 4.8 & 2.5 & 3.9 & -28.4 & 49 & 0.02 & 0.03 & 1 \\
3353 & KOI-301 & 19 21 58.8 & +38 47 44 & 6006 & 4.04 & -0.06 & 0.14 & -5.14 & 7.0 & 4.9 & 4.7 & -41.9 & 48 & 0.02 & 0.03 & 1 \\
3354 & KOI-2808 & 19 03 40.7 & +38 52 19 & 6617 & 4.59 & 0.06 & 0.12 & -5.41 & 14.3 & 3.9 & 12.2 & -2.5 & 48 & 0.03 & 0.09 & 1 \\
3355 & KOI-442 & 19 24 23.3 & +38 52 32 & 5846 & 4.43 & -0.06 & 0.13 & -5.26 & 3.8 & 0.1 & 3.8 & -42.2 & 49 & 0.02 & 0.03 & 1 \\
3356 & KOI-2261 & 19 10 07.1 & +38 53 40 & 5110 & 4.57 & -0.02 & 0.53 & -4.42 & 3.7 & 3.1 & 1.9 & -22.1 & 45 & 0.03 & 0.03 & 1 \\
3357 & KOI-1206 & 19 35 49.1 & +38 54 00 & 5693 & 3.70 & 0.02 & 0.12 & -5.29 & 6.6 & 4.8 & 4.2 & -50.9 & 50 & 0.02 & 0.02 & 1 \\
3358 & KOI-3002 & 19 28 19.7 & +38 54 54 & 5857 & 4.46 & -0.19 & 0.14 & -5.13 & 21.3 & 17.3 & 3.9 & -1.5 & 49 & 0.03 & 0.06 & 1 \\
3359 & KOI-388 & 18 58 49.7 & +38 56 13 & 5762 & 3.97 & 0.11 & 0.10 & -5.98 & 5.3 & 2.8 & 4.4 & -24.0 & 48 & 0.02 & 0.03 & 1 \\
3360 & KOI-444 & 19 22 07.1 & +38 56 34 & 5677 & 4.54 & -0.15 & 0.08 & nan & 2.9 & 0.1 & 3.1 & -23.3 & 47 & 0.03 & 0.03 & 1 \\
3361 & KOI-149 & 19 06 31.2 & +38 56 44 & 5546 & 3.54 & 0.03 & 0.12 & -5.30 & 5.1 & 3.1 & 3.9 & -23.8 & 49 & 0.21 & 0.04 & 1 \\
3362 & KOI-2289 & 19 42 48.3 & +38 56 45 & 5907 & 4.10 & 0.15 & 0.13 & -5.26 & 7.7 & 5.9 & 4.1 & -12.3 & 48 & 0.15 & 0.04 & 1 \\
3363 & KOI-4423 & 19 42 00.5 & +38 59 01 & 6316 & 4.10 & -0.08 & 0.12 & -5.33 & 11.1 & 7.5 & 7.4 & -27.9 & 48 & 0.02 & 0.03 & 1 \\
3364 & KOI-1216 & 19 12 32.1 & +38 59 49 & 5999 & 4.15 & -0.03 & 0.14 & -5.14 & 5.2 & 2.1 & 4.7 & -37.7 & 49 & 0.02 & 0.03 & 1 \\
3365 & KOI-1208 & 19 34 28.5 & +39 01 21 & 6294 & 3.89 & -0.05 & 0.10 & -5.82 & 10.4 & 5.8 & 8.3 & 5.0 & 47 & 0.02 & 0.03 & 1 \\
3366 & KOI-2904 & 19 41 30.6 & +39 02 53 & 6045 & 3.95 & 0.30 & 0.11 & -5.59 & 9.0 & 6.4 & 5.8 & -40.4 & 49 & 0.02 & 0.03 & 1 \\
3367 & KOI-393 & 19 36 07.0 & +39 03 07 & 6212 & 4.14 & -0.14 & 0.09 & nan & 10.2 & 7.2 & 6.3 & -18.8 & 47 & 0.02 & 0.03 & 1 \\
3368 & KOI-3180 & 19 02 11.3 & +39 03 48 & 6029 & 3.88 & 0.10 & 0.12 & -5.30 & 6.3 & 2.7 & 5.7 & 15.2 & 49 & 0.02 & 0.03 & 1 \\
3369 & KOI-392 & 19 11 54.2 & +39 05 14 & 5956 & 4.06 & 0.17 & 0.09 & nan & 5.9 & 3.7 & 4.4 & -3.8 & 49 & 0.25 & 0.05 & 1 \\
3370 & KOI-1336 & 19 45 26.1 & +39 06 55 & 5765 & 4.55 & 0.04 & 0.23 & -4.70 & 3.7 & 1.1 & 3.5 & -14.6 & 28 & 0.05 & 0.05 & 1 \\
3371 & KOI-4887 & 19 29 03.7 & +39 07 47 & 5846 & 3.86 & -0.00 & 0.11 & -5.49 & 6.0 & 3.5 & 4.7 & -24.5 & 48 & 0.02 & 0.03 & 1 \\
3372 & KOI-1222 & 19 29 59.2 & +39 11 35 & 4988 & 3.49 & 0.04 & 0.20 & -4.96 & 3.5 & 0.1 & 3.4 & -2.9 & 37 & 0.04 & 0.04 & 1 \\
3373 & KOI-280 & 19 06 45.5 & +39 12 43 & 6047 & 4.37 & -0.29 & 0.15 & -5.03 & 4.9 & 0.1 & 5.0 & -42.5 & 48 & 0.02 & 0.03 & 1 \\
3374 & KOI-1335 & 19 24 04.8 & +39 13 14 & 6328 & 4.05 & 0.17 & 0.15 & -5.04 & 15.6 & 11.9 & 7.6 & -16.9 & 49 & 0.02 & 0.03 & 1 \\
3375 & KOI-2202 & 19 11 46.9 & +39 13 50 & 5212 & 4.47 & 0.26 & 0.39 & -4.53 & 3.1 & 2.3 & 2.1 & -12.4 & 47 & 0.03 & 0.06 & 1 \\
3376 & KOI-1344 & 18 59 26.4 & +39 14 26 & 6061 & 4.18 & -0.30 & 0.09 & nan & 4.9 & 0.1 & 5.1 & -36.7 & 48 & 0.02 & 0.03 & 1 \\
3377 & KOI-281 & 19 10 37.2 & +39 14 39 & 5760 & 4.31 & -0.36 & 0.19 & -4.86 & 3.0 & 0.1 & 3.4 & -60.1 & 49 & 0.02 & 0.03 & 1 \\
3378 & KOI-2866 & 19 03 00.5 & +39 14 57 & 6310 & 4.31 & 0.15 & 0.10 & -5.93 & 7.3 & 0.0 & 7.4 & -10.2 & 48 & 0.03 & 0.03 & 1 \\
3379 & KOI-144 & 19 46 05.8 & +39 15 00 & 4828 & 4.45 & 0.25 & 0.12 & -5.30 & 2.6 & 1.9 & 1.7 & -9.0 & 55 & 0.02 & 0.03 & 1 \\
3380 & KOI-3864 & 19 33 22.8 & +39 15 28 & 4970 & 4.53 & 0.02 & 0.32 & -4.72 & 4.8 & 4.3 & 1.8 & 7.7 & 54 & 0.02 & 0.03 & 1 \\
3381 & KOI-3880 & 19 15 28.2 & +39 15 54 & 6143 & 4.27 & 0.06 & 0.22 & -4.67 & 17.5 & 14.2 & 5.7 & -4.2 & 48 & 0.02 & 0.03 & 1 \\
3382 & KOI-1864 & 19 17 45.2 & +39 16 13 & 5516 & 3.87 & 0.07 & 0.11 & -5.46 & 4.0 & 0.8 & 3.9 & -52.6 & 48 & 0.10 & 0.04 & 1 \\
3383 & KOI-3678 & 19 19 10.0 & +39 17 07 & 5431 & 4.50 & 0.08 & 0.16 & -5.01 & 3.0 & 1.7 & 2.4 & -4.8 & 49 & 0.02 & 0.02 & 1 \\
3384 & KOI-551 & 19 34 07.4 & +39 18 57 & 5721 & 4.47 & 0.09 & 0.15 & -5.07 & 3.7 & 1.5 & 3.3 & -40.7 & 40 & 0.04 & 0.03 & 1 \\
3385 & KOI-3202 & 19 26 01.7 & +39 19 25 & 5205 & 3.79 & -0.04 & 0.20 & -4.89 & 3.8 & 1.1 & 3.5 & -52.4 & 50 & 0.03 & 0.02 & 1 \\
3386 & KOI-2311 & 19 08 57.9 & +39 19 58 & 5625 & 4.57 & 0.11 & 0.27 & -4.63 & 14.8 & 12.5 & 3.0 & -0.5 & 52 & 0.04 & 0.03 & 1 \\
3387 & KOI-1619 & 19 39 57.7 & +39 20 47 & 4780 & 4.49 & -0.27 & 0.20 & -5.02 & 2.9 & 2.4 & 1.6 & -8.0 & 55 & 0.03 & 0.03 & 1 \\
3388 & KOI-5048 & 18 58 33.3 & +39 21 19 & 4872 & 3.26 & 0.06 & 0.10 & -5.42 & 3.3 & 0.1 & 3.4 & -40.5 & 39 & 0.03 & 0.03 & 1 \\
3389 & KOI-3358 & 19 27 33.4 & +39 21 42 & 5360 & 4.55 & -0.18 & 0.32 & -4.58 & 3.6 & 2.7 & 2.3 & -2.2 & 43 & 0.03 & 0.03 & 1 \\
3390 & KOI-3928 & 19 00 35.2 & +39 22 15 & 6146 & 4.27 & -0.02 & 0.13 & -5.19 & 8.3 & 5.6 & 5.7 & -20.7 & 47 & 0.02 & 0.03 & 1 \\
3391 & KOI-3528 & 19 18 47.3 & +39 22 18 & 6110 & 3.70 & -0.17 & 0.17 & -4.89 & 8.1 & 4.6 & 6.3 & -82.1 & 49 & 0.03 & 0.03 & 1 \\
3392 & KOI-1615 & 19 41 17.4 & +39 22 35 & 5994 & 4.38 & 0.23 & 0.26 & -4.57 & 9.8 & 7.8 & 4.6 & -25.8 & 52 & 0.02 & 0.03 & 1 \\
3393 & KOI-403 & 19 07 31.1 & +39 22 42 & 6341 & 4.13 & 0.18 & 0.09 & nan & 12.8 & 9.1 & 7.7 & -27.0 & 46 & 0.13 & 0.04 & 1 \\
3394 & KOI-4774 & 19 40 29.4 & +39 23 27 & 5230 & 4.57 & -0.04 & 0.16 & -5.03 & 2.6 & 1.3 & 2.1 & -1.7 & 52 & 0.02 & 0.03 & 1 \\
3395 & KOI-5057 & 19 01 22.4 & +39 24 50 & 4965 & 3.24 & 0.02 & 0.10 & -5.43 & 3.4 & 0.1 & 3.4 & 14.9 & 37 & 0.03 & 0.03 & 1 \\
3396 & KOI-2787 & 19 26 44.6 & +39 25 44 & 6244 & 4.01 & -0.20 & 0.11 & -5.59 & 21.0 & 17.5 & 6.7 & -0.2 & 49 & 0.03 & 0.03 & 1 \\
3397 & KOI-1738 & 19 26 59.6 & +39 26 49 & 5203 & 4.43 & 0.17 & 0.20 & -4.91 & 3.1 & 2.2 & 2.0 & -18.1 & 52 & 0.02 & 0.02 & 1 \\
3398 & KOI-3378 & 19 38 02.2 & +39 27 40 & 5687 & 4.55 & -0.40 & 0.12 & -5.30 & 2.6 & 0.1 & 3.2 & -39.0 & 47 & 0.02 & 0.03 & 1 \\
3399 & KOI-1803 & 19 06 32.5 & +39 29 19 & 4853 & 4.49 & 0.00 & 0.40 & -4.65 & 2.9 & 2.3 & 1.7 & -10.1 & 55 & 0.02 & 0.03 & 1 \\
3400 & KOI-4452 & 19 37 12.2 & +39 31 09 & 5800 & 4.13 & -0.29 & 0.08 & nan & 4.2 & 1.9 & 3.6 & -32.0 & 49 & 0.02 & 0.03 & 1 \\
3401 & KOI-3168 & 19 09 15.6 & +39 32 17 & 5805 & 4.07 & -0.19 & 0.13 & -5.22 & 4.4 & 2.3 & 3.6 & -38.5 & 109 & 0.01 & 0.01 & 1 \\
3402 & KOI-626 & 19 40 46.4 & +39 32 23 & 6071 & 4.26 & -0.16 & 0.14 & -5.17 & 5.9 & 2.6 & 5.2 & -16.3 & 47 & 0.02 & 0.03 & 1 \\
3403 & KOI-1338 & 19 29 06.3 & +39 33 01 & 5728 & 4.49 & -0.18 & 0.12 & -5.32 & 3.7 & 1.4 & 3.3 & -3.4 & 35 & 0.04 & 0.08 & 1 \\
3404 & KOI-1332 & 19 15 39.9 & +39 35 41 & 5789 & 4.48 & -0.25 & 0.11 & -5.62 & 3.2 & 0.1 & 3.6 & -36.8 & 40 & 0.03 & 0.04 & 1 \\
3405 & KOI-2547 & 19 45 49.4 & +39 35 55 & 6016 & 4.49 & -0.08 & 0.10 & -6.38 & 4.4 & 0.1 & 4.8 & 26.1 & 43 & 0.03 & 0.04 & 1 \\
3406 & KOI-4288 & 19 09 29.1 & +39 36 13 & 5921 & 4.15 & 0.08 & 0.13 & -5.26 & 5.3 & 3.2 & 4.2 & -8.6 & 49 & 0.02 & 0.02 & 1 \\
3407 & KOI-3181 & 19 42 43.9 & +39 37 07 & 5373 & 3.87 & 0.11 & 0.17 & -5.01 & 9.1 & 7.6 & 3.7 & -57.1 & 51 & 0.02 & 0.03 & 1 \\
3408 & KOI-627 & 19 28 36.1 & +39 38 15 & 5970 & 4.16 & 0.17 & 0.10 & -6.01 & 6.9 & 5.0 & 4.5 & 7.0 & 48 & 0.02 & 0.04 & 1 \\
3409 & KOI-4157 & 19 09 38.4 & +39 39 31 & 6209 & 4.31 & 0.00 & 0.14 & -5.11 & 12.2 & 9.4 & 6.3 & -15.6 & 49 & 0.03 & 0.05 & 1 \\
3410 & KOI-2025 & 19 01 40.7 & +39 42 22 & 6403 & 4.24 & 0.02 & 0.12 & -5.37 & 24.7 & 19.8 & 8.5 & -25.5 & 45 & 0.03 & 0.03 & 1 \\
3411 & Kepler-350 & 19 01 40.7 & +39 42 22 & 6336 & 4.24 & 0.01 & 0.13 & -5.26 & 24.7 & 20.5 & 7.7 & -24.9 & 67 & 0.02 & 0.05 & 1 \\
3412 & KOI-628 & 19 14 47.7 & +39 42 30 & 5800 & 4.53 & -0.35 & 0.12 & -5.45 & 3.4 & 0.1 & 3.6 & 34.3 & 43 & 0.03 & 0.03 & 1 \\
3413 & KOI-3811 & 19 04 36.8 & +39 42 54 & 5951 & 4.49 & -0.05 & 0.13 & -5.26 & 6.2 & 4.1 & 4.4 & -49.1 & 50 & 0.05 & 0.06 & 1 \\
3414 & KOI-629 & 19 28 25.0 & +39 46 04 & 6085 & 4.22 & -0.26 & 0.11 & -5.49 & 4.8 & 0.1 & 5.3 & 6.6 & 43 & 0.03 & 0.03 & 1 \\
3415 & KOI-1805 & 19 15 14.9 & +39 46 14 & 5506 & 4.56 & -0.07 & 0.32 & -4.55 & 4.6 & 3.7 & 2.6 & 7.9 & 50 & 0.02 & 0.02 & 1 \\
3416 & KOI-2393 & 19 38 39.5 & +39 47 02 & 4748 & 4.46 & -0.04 & 0.22 & -4.98 & 1.6 & 0.1 & 1.6 & 1.9 & 33 & 0.19 & 0.05 & 1 \\
3417 & KOI-1534 & 19 20 21.8 & +39 49 01 & 6154 & 4.23 & 0.07 & 0.12 & -5.47 & 10.0 & 7.4 & 5.8 & -4.7 & 43 & 0.03 & 0.03 & 1 \\
3418 & KOI-3184 & 19 13 34.9 & +39 52 21 & 5818 & 4.14 & 0.23 & 0.12 & -5.40 & 5.5 & 3.9 & 3.7 & 1.8 & 50 & 0.02 & 0.02 & 1 \\
3419 & KOI-4367 & 19 52 07.9 & +39 53 00 & 6231 & 4.06 & -0.02 & 0.11 & -5.69 & 9.8 & 6.7 & 6.5 & -28.9 & 48 & 0.02 & 0.03 & 1 \\
3420 & KOI-4004 & 18 55 58.8 & +39 55 01 & 5715 & 4.54 & -0.09 & 0.28 & -4.59 & 8.4 & 7.1 & 3.3 & -24.1 & 51 & 0.14 & 0.04 & 1 \\
3421 & KOI-2120 & 19 48 17.9 & +39 56 02 & 4964 & 4.55 & -0.12 & 0.51 & -4.49 & 2.9 & 2.3 & 1.8 & -51.9 & 50 & 0.02 & 0.03 & 1 \\
3422 & KOI-4639 & 19 15 23.3 & +39 56 04 & 6509 & 3.88 & 0.23 & 0.16 & -4.97 & 17.2 & 10.8 & 12.4 & 7.6 & 48 & 0.03 & 0.03 & 1 \\
3423 & KOI-633 & 19 33 42.5 & +39 56 33 & 5840 & 4.24 & -0.14 & 0.10 & -5.88 & 3.9 & 0.7 & 3.8 & -41.1 & 48 & 0.02 & 0.03 & 1 \\
3424 & KOI-632 & 19 17 40.3 & +39 56 42 & 5314 & 4.53 & 0.01 & 0.35 & -4.55 & 2.5 & 1.0 & 2.2 & -51.1 & 51 & 0.02 & 0.03 & 1 \\
3425 & KOI-232 & 19 24 26.9 & +39 56 57 & 6007 & 4.42 & -0.04 & 0.10 & -6.00 & 5.3 & 2.3 & 4.7 & 18.7 & 23 & 0.06 & 0.06 & 1 \\
3426 & Kepler-122 & 19 24 26.9 & +39 56 57 & 5938 & 4.13 & -0.04 & 0.00 & 0.00 & 5.8 & 3.7 & 4.3 & 18.4 & 54 & 0.13 & 0.03 & 1 \\
3427 & KOI-3823 & 19 07 05.2 & +39 59 02 & 5604 & 4.54 & 0.00 & 0.28 & -4.60 & 3.4 & 1.7 & 2.9 & 0.6 & 45 & 0.02 & 0.03 & 1 \\
3428 & KOI-3936 & 19 50 18.5 & +40 01 40 & 4954 & 4.40 & 0.09 & 0.74 & -4.32 & 6.4 & 5.9 & 1.8 & -29.4 & 54 & 0.02 & 0.03 & 1 \\
3429 & KOI-1665 & 19 36 41.1 & +40 03 19 & 5956 & 4.24 & 0.33 & 0.16 & -5.01 & 4.6 & 1.3 & 4.4 & -20.7 & 49 & 0.03 & 0.05 & 1 \\
3430 & KOI-4018 & 19 33 24.2 & +40 03 35 & 5448 & 4.57 & -0.12 & 0.18 & -4.93 & 3.2 & 1.9 & 2.5 & -24.1 & 35 & 0.03 & 0.04 & 1 \\
3431 & KOI-2635 & 19 16 07.9 & +40 05 13 & 6027 & 3.94 & -0.14 & 0.13 & -5.27 & 8.6 & 6.0 & 5.7 & -33.3 & 46 & 0.03 & 0.03 & 1 \\
3432 & KOI-5107 & 19 44 04.5 & +40 05 14 & 4939 & 3.09 & -0.05 & 0.11 & -5.36 & 4.1 & 2.1 & 3.4 & -14.0 & 37 & 0.03 & 0.04 & 1 \\
3433 & KOI-3770 & 19 23 44.8 & +40 07 30 & 6108 & 4.11 & -0.02 & 0.13 & -5.23 & 8.0 & 5.5 & 5.4 & -26.9 & 44 & 0.03 & 0.03 & 1 \\
3434 & KOI-5119 & 19 51 09.2 & +40 07 51 & 4909 & 3.13 & 0.07 & 0.21 & -4.97 & 4.2 & 2.3 & 3.4 & 7.9 & 39 & 0.03 & 0.03 & 1 \\
3435 & KOI-4546 & 19 49 05.6 & +40 08 12 & 5981 & 4.33 & 0.07 & 0.09 & nan & 5.1 & 2.1 & 4.5 & -15.9 & 43 & 0.03 & 0.03 & 1 \\
3436 & KOI-2951 & 18 57 50.3 & +40 08 33 & 5664 & 4.49 & -0.23 & 0.15 & -5.07 & 4.1 & 2.5 & 3.1 & 20.5 & 49 & 0.02 & 0.03 & 1 \\
3437 & KOI-3421 & 19 19 40.7 & +40 10 07 & 6248 & 4.10 & 0.09 & 0.12 & -5.39 & 9.6 & 6.3 & 6.7 & -3.6 & 49 & 0.02 & 0.03 & 1 \\
3438 & KOI-1666 & 19 24 04.7 & +40 10 39 & 6437 & 4.41 & 0.13 & 0.10 & -6.10 & 16.9 & 12.6 & 9.0 & -34.1 & 35 & 0.04 & 0.04 & 1 \\
3439 & KOI-635 & 19 37 29.6 & +40 11 41 & 6102 & 4.39 & 0.07 & 0.21 & -4.71 & 7.8 & 5.3 & 5.4 & -38.2 & 48 & 0.02 & 0.03 & 1 \\
3440 & KOI-161 & 19 08 12.4 & +40 12 42 & 4882 & 4.49 & 0.30 & 0.23 & -4.91 & 1.4 & 0.1 & 1.7 & -15.7 & 55 & 0.02 & 0.03 & 1 \\
3441 & KOI-639 & 19 47 32.6 & +40 13 42 & 6156 & 4.30 & 0.08 & 0.15 & -5.04 & 9.1 & 6.4 & 5.8 & -23.0 & 48 & 0.02 & 0.03 & 1 \\
3442 & KOI-3093 & 19 23 58.0 & +40 13 46 & 5891 & 4.42 & 0.03 & 0.21 & -4.74 & 3.5 & 0.1 & 4.0 & -16.7 & 49 & 0.02 & 0.03 & 1 \\
3443 & Kepler-130 & 19 13 48.2 & +40 14 43 & 6050 & 4.49 & -0.09 & 0.14 & -5.13 & 4.1 & 0.1 & 5.0 & 17.8 & 108 & 0.01 & 0.02 & 1 \\
3444 & KOI-282 & 19 13 48.2 & +40 14 43 & 5954 & 4.40 & -0.14 & 0.12 & -5.32 & 3.5 & 0.1 & 4.4 & 18.8 & 49 & 0.02 & 0.02 & 1 \\
3445 & KOI-4331 & 19 23 15.3 & +40 15 18 & 6360 & 4.13 & 0.06 & 0.14 & -5.12 & 14.2 & 10.2 & 8.0 & -24.7 & 48 & 0.02 & 0.03 & 1 \\
3446 & KOI-1822 & 19 51 45.6 & +40 16 43 & 6105 & 4.35 & -0.17 & 0.10 & -5.91 & 6.3 & 3.0 & 5.4 & -6.9 & 50 & 0.03 & 0.03 & 1 \\
3447 & KOI-640 & 19 49 00.6 & +40 17 19 & 5227 & 4.46 & 0.08 & 0.12 & -5.27 & 2.3 & 0.6 & 2.1 & -24.4 & 52 & 0.02 & 0.02 & 1 \\
3448 & KOI-2698 & 19 55 20.6 & +40 17 35 & 5898 & 4.26 & 0.09 & 0.11 & -5.59 & 4.8 & 2.4 & 4.1 & -11.0 & 50 & 0.02 & 0.02 & 1 \\
3449 & KOI-1563 & 19 56 53.8 & +40 20 35 & 4994 & 4.41 & 0.06 & 0.44 & -4.56 & 2.7 & 1.9 & 1.8 & -4.8 & 26 & 0.05 & 0.06 & 1 \\
3450 & KOI-3474 & 19 52 20.0 & +40 20 46 & 5965 & 4.25 & -0.11 & 0.11 & -5.58 & 6.3 & 4.1 & 4.5 & -50.1 & 48 & 0.02 & 0.03 & 1 \\
3451 & KOI-2158 & 19 50 36.3 & +40 21 09 & 5333 & 4.42 & -0.03 & 0.17 & -4.97 & 3.0 & 1.8 & 2.2 & -94.0 & 49 & 0.02 & 0.02 & 1 \\
3452 & KOI-2563 & 19 12 23.0 & +40 21 57 & 6076 & 3.98 & 0.11 & 0.11 & -5.72 & 9.1 & 6.4 & 6.0 & 7.8 & 48 & 0.02 & 0.05 & 1 \\
3453 & KOI-4246 & 19 16 17.8 & +40 21 58 & 5603 & 4.51 & 0.15 & 0.36 & -4.46 & 7.6 & 6.6 & 2.9 & -20.9 & 50 & 0.02 & 0.02 & 1 \\
3454 & KOI-1576 & 19 51 10.8 & +40 25 04 & 5456 & 4.39 & 0.13 & 0.18 & -4.95 & 3.6 & 2.5 & 2.5 & -45.7 & 49 & 0.05 & 0.04 & 1 \\
3455 & KOI-825 & 18 52 53.1 & +40 25 19 & 4828 & 4.50 & 0.20 & 0.11 & -5.32 & 1.5 & 0.1 & 1.7 & -27.2 & 31 & 0.04 & 0.05 & 1 \\
3456 & KOI-4713 & 18 55 21.3 & +40 25 19 & 5921 & 4.70 & 0.11 & 0.28 & -4.55 & 20.7 & 17.3 & 4.2 & -28.7 & 17 & 0.09 & 0.10 & 2 \\
3457 & KOI-4411 & 19 34 19.4 & +40 25 39 & 6042 & 4.31 & -0.16 & 0.13 & -5.20 & 6.0 & 3.2 & 4.9 & -13.9 & 48 & 0.02 & 0.02 & 1 \\
3458 & KOI-3239 & 19 55 35.1 & +40 28 37 & 5568 & 4.50 & -0.04 & 0.38 & -4.44 & 6.8 & 5.9 & 2.8 & -29.2 & 49 & 0.02 & 0.03 & 1 \\
3459 & KOI-2711 & 19 23 46.7 & +40 28 48 & 5903 & 4.46 & 0.05 & 0.21 & -4.74 & 5.5 & 3.5 & 4.1 & 12.5 & 46 & 0.03 & 0.03 & 1 \\
3460 & KOI-1589 & 19 53 00.5 & +40 29 46 & 6066 & 4.54 & -0.07 & 0.17 & -4.94 & 6.5 & 3.7 & 5.1 & 12.7 & 26 & 0.05 & 0.05 & 1 \\
3461 & KOI-408 & 19 12 56.2 & +40 31 15 & 5833 & 4.80 & 0.30 & 0.18 & -4.89 & 5.0 & 3.0 & 3.8 & -18.2 & 28 & 0.60 & 0.10 & 1 \\
3462 & KOI-644 & 19 19 52.0 & +40 31 58 & 5780 & 4.28 & -0.09 & 0.19 & -4.85 & 3.8 & 1.0 & 3.5 & -79.0 & 36 & 0.05 & 0.04 & 1 \\
3463 & KOI-2370 & 19 50 14.0 & +40 32 29 & 6392 & 4.18 & -0.14 & 0.13 & -5.22 & 23.3 & 18.6 & 8.4 & 12.7 & 47 & 0.02 & 0.03 & 1 \\
3464 & KOI-2555 & 19 11 25.7 & +40 32 50 & 6113 & 4.30 & -0.06 & 0.11 & -5.56 & 8.0 & 5.4 & 5.5 & -34.7 & 47 & 0.02 & 0.03 & 1 \\
3465 & KOI-2011 & 19 49 01.2 & +40 32 54 & 6347 & 4.21 & -0.06 & 0.13 & -5.26 & 18.3 & 14.4 & 7.8 & -29.4 & 50 & 0.03 & 0.03 & 1 \\
3466 & KOI-2219 & 19 21 03.7 & +40 32 55 & 4900 & 4.48 & 0.11 & 0.26 & -4.85 & 2.0 & 0.9 & 1.7 & -16.1 & 47 & 0.03 & 0.03 & 1 \\
3467 & KOI-1825 & 19 41 12.0 & +40 33 24 & 5293 & 4.52 & 0.02 & 0.39 & -4.51 & 5.1 & 4.5 & 2.2 & -22.9 & 38 & 0.04 & 0.04 & 1 \\
3468 & KOI-2440 & 18 52 00.0 & +40 33 27 & 5629 & 4.22 & 0.26 & 0.12 & -5.37 & 3.7 & 2.2 & 3.0 & -32.0 & 51 & 0.02 & 0.02 & 1 \\
3469 & KOI-1557 & 19 37 46.0 & +40 33 27 & 4726 & 4.57 & -0.02 & 0.60 & -4.52 & 3.1 & 2.6 & 1.6 & -27.5 & 28 & 0.04 & 0.05 & 1 \\
3470 & KOI-829 & 19 21 50.8 & +40 33 45 & 5852 & 4.49 & 0.02 & 0.21 & -4.74 & 4.2 & 1.4 & 3.8 & -60.0 & 29 & 0.04 & 0.04 & 1 \\
3471 & KOI-2556 & 19 40 24.6 & +40 34 21 & 5506 & 4.57 & -0.21 & 0.11 & -5.50 & 3.3 & 1.7 & 2.6 & -43.1 & 42 & 0.03 & 0.03 & 1 \\
3472 & KOI-2690 & 19 35 44.0 & +40 35 27 & 5393 & 4.51 & 0.01 & 0.49 & -4.36 & 4.6 & 3.9 & 2.4 & -12.5 & 51 & 0.02 & 0.02 & 1 \\
3473 & KOI-645 & 19 40 52.2 & +40 35 32 & 5835 & 4.16 & -0.24 & 0.12 & -5.36 & 4.4 & 2.1 & 3.8 & 2.0 & 48 & 0.02 & 0.03 & 1 \\
3474 & KOI-3039 & 19 23 48.0 & +40 36 19 & 5769 & 4.20 & -0.24 & 0.12 & -5.34 & 4.5 & 2.7 & 3.5 & -16.1 & 50 & 0.02 & 0.03 & 1 \\
3475 & KOI-1567 & 19 14 09.3 & +40 36 58 & 4884 & 4.46 & -0.07 & 0.22 & -4.46 & 2.2 & 1.1 & 1.7 & -22.0 & 27 & 0.07 & 0.06 & 2 \\
3476 & KOI-4907 & 19 13 35.4 & +40 37 37 & 5976 & 4.30 & 0.07 & 0.10 & -6.26 & 4.7 & 1.1 & 4.5 & -39.2 & 45 & 0.03 & 0.03 & 1 \\
3477 & KOI-834 & 19 11 35.3 & +40 38 16 & 5704 & 4.04 & 0.28 & 0.24 & -4.68 & 4.4 & 2.9 & 3.2 & -13.5 & 26 & 0.05 & 0.05 & 1 \\
3478 & KOI-3791 & 19 13 54.0 & +40 39 05 & 6197 & 4.26 & 0.11 & 0.12 & -5.41 & 6.7 & 2.3 & 6.2 & -9.0 & 48 & 0.02 & 0.03 & 1 \\
3479 & KOI-1601 & 19 15 05.0 & +40 39 51 & 5627 & 4.12 & -0.10 & 0.13 & -5.21 & 3.4 & 1.5 & 3.0 & -72.0 & 37 & 0.03 & 0.03 & 1 \\
3480 & KOI-2970 & 19 30 18.7 & +40 40 04 & 6140 & 4.35 & -0.07 & 0.12 & -5.32 & 6.8 & 3.5 & 5.7 & 17.6 & 47 & 0.02 & 0.03 & 1 \\
3481 & KOI-142 & 19 24 35.5 & +40 40 10 & 5393 & 4.41 & 0.18 & 0.17 & nan & 2.2 & 0.5 & 2.4 & -21.3 & 75 & 0.02 & 0.02 & 2 \\
3482 & KOI-2707 & 19 58 00.4 & +40 40 15 & 5640 & 4.56 & -0.12 & 0.15 & -5.07 & 3.5 & 1.6 & 3.0 & -13.2 & 36 & 0.03 & 0.03 & 1 \\
3483 & Kepler-399 & 19 58 00.4 & +40 40 15 & 5587 & 4.53 & -0.18 & 0.00 & 0.00 & 3.7 & 2.2 & 2.8 & -12.1 & 56 & 0.03 & 0.07 & 1 \\
3484 & KOI-4368 & 19 50 39.6 & +40 40 55 & 5848 & 3.81 & 0.03 & 0.10 & -6.22 & 5.4 & 2.4 & 4.7 & 24.0 & 50 & 0.02 & 0.03 & 1 \\
3485 & KOI-409 & 19 22 15.9 & +40 41 31 & 5841 & 4.41 & 0.16 & 0.12 & -5.34 & 4.0 & 1.2 & 3.8 & -1.4 & 44 & 0.03 & 0.03 & 1 \\
3486 & KOI-647 & 19 24 46.8 & +40 42 10 & 6130 & 4.20 & -0.37 & 0.14 & -5.08 & 5.2 & 0.1 & 5.6 & -54.4 & 48 & 0.02 & 0.03 & 1 \\
3487 & KOI-2741 & 18 57 28.6 & +40 43 07 & 5852 & 4.43 & 0.04 & 0.15 & -5.05 & 3.6 & 0.1 & 3.8 & -54.1 & 49 & 0.02 & 0.03 & 1 \\
3488 & KOI-257 & 18 58 32.4 & +40 43 11 & 6179 & 4.31 & 0.14 & 0.15 & -5.03 & 9.1 & 6.3 & 6.0 & -14.1 & 49 & 0.02 & 0.03 & 1 \\
3489 & KOI-1590 & 19 37 27.6 & +40 43 15 & 4833 & 4.53 & -0.11 & 0.30 & -4.79 & 2.9 & 2.2 & 1.7 & -37.1 & 24 & 0.06 & 0.07 & 1 \\
3490 & KOI-2854 E & 18 57 25.1 & +40 43 23 & 6200 & 4.18 & 0.08 & 0.11 & -5.54 & 9.7 & 6.8 & 6.2 & 0.6 & 46 & 0.03 & 0.03 & 1 \\
3491 & KOI-2854 W & 18 57 24.9 & +40 43 24 & 5956 & 4.43 & 0.07 & 0.34 & -4.40 & 4.5 & 0.7 & 4.4 & -0.9 & 55 & 0.03 & 0.02 & 1 \\
3492 & KOI-2668 & 18 55 40.8 & +40 44 24 & 5464 & 4.55 & -0.10 & 0.22 & -4.80 & 2.9 & 1.2 & 2.5 & -14.2 & 49 & 0.02 & 0.02 & 1 \\
3493 & KOI-837 & 19 24 38.1 & +40 45 01 & 4831 & 4.43 & 0.38 & 0.24 & -4.92 & 2.4 & 1.6 & 1.7 & -42.4 & 28 & 0.05 & 0.06 & 1 \\
3494 & KOI-1621 & 19 54 21.4 & +40 45 03 & 6086 & 4.02 & 0.06 & 0.11 & -5.62 & 7.5 & 5.0 & 5.3 & -49.0 & 50 & 0.02 & 0.03 & 1 \\
3495 & KOI-4067 & 19 22 38.0 & +40 46 43 & 5961 & 4.28 & 0.06 & 0.12 & -5.45 & 5.3 & 2.9 & 4.4 & -22.5 & 47 & 0.02 & 0.03 & 1 \\
3496 & Kepler-338 & 18 51 55.0 & +40 47 04 & 5892 & 4.00 & -0.03 & 0.14 & -5.19 & 6.3 & 4.6 & 4.0 & -17.6 & 85 & 0.02 & 0.02 & 1 \\
3497 & KOI-1930 & 18 51 55.0 & +40 47 04 & 5834 & 3.93 & -0.07 & 0.13 & -5.21 & 6.5 & 4.3 & 4.7 & -19.3 & 51 & 0.03 & 0.03 & 1 \\
3498 & KOI-2332 & 19 29 00.6 & +40 47 34 & 5181 & 3.91 & -0.07 & 0.13 & -5.19 & 3.1 & 0.1 & 3.5 & -57.6 & 50 & 0.02 & 0.02 & 1 \\
3499 & KOI-1962 & 18 56 56.2 & +40 47 40 & 5918 & 4.12 & -0.06 & 0.13 & -5.21 & 5.9 & 4.0 & 4.2 & -58.7 & 51 & 0.02 & 0.02 & 1 \\
3500 & KOI-649 & 19 19 05.6 & +40 48 03 & 6114 & 3.96 & 0.21 & 0.11 & -5.54 & 9.6 & 6.7 & 6.3 & -14.2 & 49 & 0.02 & 0.03 & 1 \\
3501 & KOI-2915 & 19 19 40.2 & +40 49 43 & 5602 & 4.48 & -0.06 & 0.15 & -5.06 & 3.0 & 0.6 & 2.9 & -24.2 & 50 & 0.02 & 0.02 & 1 \\
3502 & KOI-2790 & 19 58 38.3 & +40 50 38 & 5115 & 4.44 & -0.20 & 0.14 & -5.15 & 2.4 & 1.2 & 1.9 & -29.7 & 52 & 0.02 & 0.02 & 1 \\
3503 & KOI-371 & 19 58 42.3 & +40 51 23 & 5083 & 3.60 & 0.05 & 0.19 & -4.97 & 3.0 & 0.1 & 3.5 & -60.4 & 40 & 0.03 & 0.03 & 1 \\
3504 & KOI-2369 & 19 02 53.0 & +40 51 25 & 5769 & 4.22 & 0.07 & 0.28 & -4.57 & 4.6 & 2.9 & 3.5 & -17.5 & 27 & 0.04 & 0.09 & 1 \\
3505 & KOI-2676 & 19 55 55.3 & +40 52 19 & 6272 & 3.84 & -0.01 & 0.12 & -5.33 & 6.6 & 0.1 & 8.0 & -25.3 & 47 & 0.02 & 0.03 & 1 \\
3506 & KOI-2010 & 19 40 37.9 & +40 53 56 & 6319 & 4.05 & 0.02 & 0.12 & -5.38 & 12.6 & 9.0 & 7.5 & 9.6 & 47 & 0.03 & 0.03 & 1 \\
3507 & KOI-2752 & 19 41 17.8 & +40 54 08 & 6060 & 4.26 & 0.17 & 0.09 & -7.54 & 9.1 & 7.0 & 5.1 & -6.9 & 48 & 0.02 & 0.03 & 1 \\
3508 & KOI-2183 & 19 28 41.1 & +40 54 59 & 5610 & 4.43 & 0.05 & 0.10 & -5.70 & 2.8 & 0.1 & 2.9 & -36.4 & 34 & 0.04 & 0.04 & 1 \\
3509 & KOI-505 & 19 04 00.0 & +40 55 10 & 4945 & 4.53 & 0.11 & 0.45 & -4.56 & 3.0 & 2.3 & 1.8 & -43.4 & 46 & 0.03 & 0.03 & 1 \\
3510 & Kepler-169 & 19 04 00.0 & +40 55 10 & 4896 & 4.32 & 0.06 & 0.00 & 0.00 & 2.9 & 2.3 & 1.7 & -42.8 & 52 & 0.02 & 0.05 & 1 \\
3511 & KOI-555 & 19 32 29.6 & +40 56 05 & 5221 & 4.45 & 0.02 & 0.09 & -5.63 & 2.3 & 0.7 & 2.1 & -38.1 & 50 & 0.02 & 0.03 & 1 \\
3512 & KOI-4744 & 19 32 41.8 & +40 57 03 & 5737 & 4.19 & 0.22 & 0.10 & -5.81 & 4.5 & 2.9 & 3.3 & -16.7 & 39 & 0.03 & 0.03 & 1 \\
3513 & KOI-2358 & 19 40 33.4 & +40 58 45 & 6084 & 3.97 & 0.15 & 0.18 & -4.83 & 16.8 & 13.6 & 6.1 & -45.7 & 48 & 0.02 & 0.03 & 1 \\
3514 & KOI-1897 & 19 14 17.9 & +40 59 19 & 5917 & 4.31 & -0.11 & 0.11 & -5.50 & 4.4 & 1.1 & 4.2 & 22.2 & 47 & 0.02 & 0.03 & 1 \\
3515 & KOI-2675 & 19 31 53.1 & +41 02 09 & 5679 & 4.53 & 0.00 & 0.31 & -4.53 & 9.0 & 7.8 & 3.1 & -10.7 & 49 & 0.02 & 0.03 & 1 \\
3516 & KOI-3288 & 18 52 50.8 & +41 02 17 & 5346 & 4.54 & -0.02 & 0.29 & -4.64 & 3.6 & 2.8 & 2.3 & -15.7 & 50 & 0.02 & 0.02 & 1 \\
3517 & KOI-650 & 19 21 35.1 & +41 02 24 & 5015 & 4.54 & 0.04 & 0.16 & -5.10 & 1.5 & 0.1 & 1.8 & -21.8 & 52 & 0.02 & 0.03 & 1 \\
3518 & KOI-1928 & 18 55 14.3 & +41 02 28 & 5787 & 4.33 & 0.17 & 0.17 & -4.92 & 4.5 & 2.6 & 3.5 & -52.9 & 49 & 0.02 & 0.02 & 1 \\
3519 & KOI-4686 & 19 55 37.4 & +41 02 33 & 5656 & 3.93 & 0.28 & 0.11 & -5.50 & 4.9 & 2.6 & 4.1 & -25.3 & 51 & 0.02 & 0.02 & 1 \\
3520 & KOI-4002 & 19 01 19.6 & +41 03 50 & 5136 & 4.50 & 0.14 & 0.50 & -4.43 & 3.4 & 2.7 & 2.0 & -10.3 & 31 & 0.04 & 0.04 & 1 \\
3521 & KOI-652 & 19 34 22.1 & +41 05 43 & 5256 & 4.59 & 0.02 & 0.21 & -4.87 & 3.4 & 2.5 & 2.1 & -21.8 & 54 & 0.03 & 0.04 & 1 \\
3522 & KOI-4913 & 18 54 42.9 & +41 05 49 & 6346 & 4.23 & 0.07 & 0.13 & -5.22 & 23.7 & 19.1 & 7.8 & 13.5 & 47 & 0.03 & 0.03 & 1 \\
3523 & KOI-3422 & 19 50 51.6 & +41 06 15 & 5815 & 4.48 & 0.08 & 0.25 & -4.63 & 6.5 & 5.1 & 3.7 & 1.0 & 50 & 0.02 & 0.02 & 1 \\
3524 & KOI-4156 & 19 33 16.4 & +41 07 00 & 5780 & 4.11 & 0.23 & 0.12 & -5.36 & 4.7 & 3.0 & 3.5 & -35.4 & 47 & 0.02 & 0.03 & 1 \\
3525 & KOI-1060 & 19 32 20.3 & +41 08 08 & 6549 & 4.32 & -0.21 & 0.17 & -4.89 & 13.6 & 7.7 & 10.9 & -1.2 & 25 & 0.06 & 0.06 & 1 \\
3526 & Kepler-758 & 19 32 20.3 & +41 08 08 & 6450 & 4.10 & -0.20 & 0.00 & 0.00 & 14.6 & 10.0 & 9.2 & -3.4 & 59 & 0.06 & 0.04 & 1 \\
3527 & KOI-2801 & 19 56 38.5 & +41 08 37 & 5992 & 4.11 & 0.03 & 0.12 & -5.43 & 5.3 & 2.5 & 4.6 & 4.6 & 49 & 0.02 & 0.03 & 1 \\
3528 & KOI-1839 & 18 56 22.7 & +41 10 58 & 5443 & 4.57 & 0.03 & 0.39 & -4.46 & 8.2 & 7.3 & 2.5 & -23.1 & 47 & 0.03 & 0.05 & 1 \\
3529 & KOI-2498 & 19 26 30.9 & +41 12 31 & 5138 & 4.53 & -0.11 & 0.13 & -5.22 & 2.6 & 1.6 & 2.0 & -48.3 & 50 & 0.02 & 0.05 & 1 \\
3530 & KOI-4633 & 19 19 07.1 & +41 12 52 & 5942 & 4.14 & 0.09 & 0.16 & -4.96 & 7.1 & 5.3 & 4.3 & -21.6 & 38 & 0.03 & 0.04 & 1 \\
3531 & KOI-654 & 18 57 38.4 & +41 14 15 & 5824 & 4.49 & -0.05 & 0.17 & -4.92 & 3.9 & 0.9 & 3.7 & -42.4 & 49 & 0.03 & 0.03 & 1 \\
3532 & KOI-1052 & 19 22 02.5 & +41 14 41 & 5929 & 4.36 & -0.07 & 0.13 & -5.22 & 4.6 & 1.4 & 4.2 & -21.7 & 26 & 0.05 & 0.05 & 1 \\
3533 & KOI-3190 & 19 53 04.4 & +41 15 06 & 6091 & 4.36 & -0.10 & 0.13 & -5.24 & 4.4 & 0.1 & 5.3 & -0.7 & 47 & 0.02 & 0.03 & 1 \\
3534 & KOI-655 & 19 34 30.2 & +41 16 22 & 6144 & 4.22 & -0.02 & 0.13 & -5.28 & 4.8 & 0.1 & 5.7 & 6.6 & 47 & 0.02 & 0.03 & 1 \\
3535 & KOI-2479 & 19 31 32.5 & +41 16 45 & 5275 & 3.82 & -0.01 & 0.18 & -4.97 & 3.8 & 1.2 & 3.6 & 22.6 & 51 & 0.02 & 0.02 & 1 \\
3536 & KOI-2250 & 19 00 52.0 & +41 16 57 & 4845 & 4.44 & 0.07 & 0.36 & -4.71 & 2.9 & 2.3 & 1.7 & -11.3 & 29 & 0.05 & 0.09 & 1 \\
3537 & KOI-303 & 19 34 42.1 & +41 17 43 & 5659 & 4.48 & -0.16 & 0.18 & -4.92 & 3.2 & 0.4 & 3.1 & -76.8 & 49 & 0.02 & 0.02 & 1 \\
3538 & KOI-2733 & 19 18 12.7 & +41 17 52 & 4716 & 4.41 & -0.08 & 0.40 & -4.71 & 3.5 & 3.1 & 1.6 & 4.9 & 47 & 0.03 & 0.03 & 1 \\
3539 & KOI-2148 & 18 52 46.1 & +41 18 19 & 5541 & 3.99 & 0.36 & 0.12 & -5.35 & 4.3 & 1.9 & 3.9 & -71.2 & 50 & 0.02 & 0.02 & 1 \\
3540 & Kepler-363 & 18 52 46.1 & +41 18 19 & 5526 & 3.92 & 0.35 & 0.18 & -4.94 & 4.3 & 1.7 & 3.9 & -72.5 & 86 & 0.02 & 0.04 & 1 \\
3541 & KOI-1054 & 19 14 43.8 & +41 18 26 & 5551 & 3.28 & -0.68 & 0.16 & -5.04 & 6.2 & 4.8 & 3.9 & -143.3 & 50 & 0.03 & 0.05 & 1 \\
3542 & KOI-2167 & 19 26 25.1 & +41 18 34 & 5716 & 4.53 & 0.06 & 0.22 & -4.76 & 4.6 & 3.1 & 3.3 & 11.4 & 34 & 0.05 & 0.04 & 1 \\
3543 & KOI-2071 & 19 17 46.7 & +41 19 04 & 5205 & 4.53 & 0.11 & 0.25 & -4.78 & 2.8 & 1.7 & 2.0 & -14.6 & 46 & 0.03 & 0.03 & 1 \\
3544 & KOI-1684 & 19 34 08.3 & +41 19 48 & 6530 & 4.59 & -0.09 & 0.14 & -5.15 & 21.2 & 15.2 & 10.5 & 22.8 & 48 & 0.03 & 0.04 & 1 \\
3545 & KOI-1916 & 19 20 57.0 & +41 19 53 & 5884 & 4.40 & 0.19 & 0.20 & -4.78 & 7.1 & 5.5 & 4.0 & -30.7 & 48 & 0.02 & 0.02 & 1 \\
3546 & Kepler-336 & 19 20 57.0 & +41 19 53 & 5800 & 4.38 & 0.16 & 0.20 & -4.80 & 7.4 & 6.0 & 3.6 & -29.3 & 66 & 0.08 & 0.04 & 1 \\
3547 & KOI-2949 & 19 03 30.2 & +41 19 57 & 5871 & 4.18 & 0.04 & 0.11 & -5.54 & 4.5 & 2.1 & 3.9 & -24.2 & 50 & 0.02 & 0.02 & 1 \\
3548 & KOI-3500 & 19 45 25.1 & +41 20 08 & 5951 & 3.94 & 0.16 & 0.10 & -6.21 & 8.3 & 6.0 & 5.2 & -38.7 & 49 & 0.02 & 0.03 & 1 \\
3549 & Kepler-132 & 18 52 56.6 & +41 20 35 & 5964 & 4.36 & -0.20 & 0.14 & -5.15 & 5.6 & 3.3 & 4.4 & -30.2 & 85 & 0.02 & 0.02 & 1 \\
3550 & KOI-284 & 18 52 56.6 & +41 20 35 & 5989 & 4.37 & -0.14 & 0.13 & -5.26 & 5.6 & 3.0 & 4.6 & -33.5 & 43 & 0.03 & 0.03 & 1 \\
3551 & KOI-4276 & 19 03 52.5 & +41 21 49 & 6149 & 3.90 & 0.10 & 0.12 & -5.47 & 9.7 & 6.6 & 6.6 & -9.6 & 50 & 0.04 & 0.04 & 1 \\
3552 & KOI-304 & 19 08 21.6 & +41 22 26 & 5848 & 4.53 & -0.19 & 0.16 & -4.97 & 3.9 & 0.1 & 3.8 & 19.8 & 48 & 0.02 & 0.02 & 1 \\
3553 & KOI-2001 & 19 48 05.1 & +41 22 38 & 5048 & 4.51 & -0.00 & 0.40 & -4.58 & 3.6 & 3.1 & 1.9 & -16.2 & 50 & 0.03 & 0.03 & 1 \\
3554 & KOI-306 & 19 57 16.7 & +41 23 05 & 5220 & 4.51 & 0.06 & 0.25 & -4.76 & 3.6 & 2.9 & 2.1 & -23.9 & 52 & 0.02 & 0.02 & 1 \\
3555 & Kepler-203 & 19 48 21.6 & +41 23 17 & 5884 & 4.42 & 0.06 & 0.00 & 0.00 & 4.7 & 2.4 & 4.0 & -33.6 & 67 & 0.02 & 0.04 & 1 \\
3556 & KOI-659 & 19 29 40.1 & +41 25 01 & 6308 & 4.29 & -0.01 & 0.13 & -5.22 & 10.8 & 7.3 & 7.3 & -39.4 & 46 & 0.03 & 0.03 & 1 \\
3557 & KOI-2098 & 18 59 54.7 & +41 25 13 & 6342 & 4.24 & -0.11 & 0.09 & nan & 13.4 & 9.8 & 7.8 & -8.5 & 41 & 0.03 & 0.03 & 1 \\
3558 & KOI-3179 & 19 57 12.8 & +41 26 28 & 5695 & 4.50 & 0.01 & 0.15 & -5.05 & 4.0 & 2.4 & 3.2 & -42.7 & 49 & 0.02 & 0.02 & 1 \\
3559 & KOI-4123 & 19 45 25.6 & +41 27 19 & 6091 & 3.80 & 0.12 & 0.11 & -5.51 & 5.7 & 0.1 & 6.1 & -21.2 & 46 & 0.02 & 0.03 & 1 \\
3560 & KOI-2398 & 19 19 45.4 & +41 30 10 & 6225 & 4.08 & -0.26 & 0.12 & -5.42 & 9.9 & 6.8 & 6.5 & -11.0 & 47 & 0.02 & 0.03 & 1 \\
3561 & KOI-2829 & 19 17 27.5 & +41 32 00 & 5887 & 4.12 & -0.00 & 0.13 & -5.24 & 5.0 & 2.8 & 4.0 & -30.1 & 49 & 0.02 & 0.02 & 1 \\
3562 & Kepler-92 & 19 16 20.7 & +41 33 47 & 5935 & 4.07 & 0.18 & 0.00 & 0.00 & 5.9 & 3.8 & 4.3 & -42.1 & 111 & 0.04 & 0.02 & 1 \\
3563 & KOI-285 & 19 16 20.7 & +41 33 47 & 5910 & 4.06 & 0.18 & 0.14 & -5.13 & 5.3 & 3.2 & 4.1 & -42.0 & 49 & 0.02 & 0.03 & 1 \\
3564 & KOI-2252 & 19 28 56.1 & +41 34 31 & 6131 & 4.00 & 0.13 & 0.13 & -5.25 & 9.4 & 7.0 & 5.6 & -25.7 & 48 & 0.02 & 0.03 & 1 \\
3565 & KOI-3240 & 19 29 22.8 & +41 35 07 & 6052 & 3.91 & 0.24 & 0.12 & -5.34 & 6.3 & 2.4 & 5.8 & -25.5 & 49 & 0.02 & 0.09 & 1 \\
3566 & KOI-2636 & 19 18 44.8 & +41 35 20 & 5846 & 4.42 & 0.04 & 0.18 & -4.89 & 4.7 & 2.7 & 3.8 & -20.8 & 48 & 0.03 & 0.02 & 1 \\
3567 & KOI-1812 & 19 20 30.4 & +41 36 04 & 6011 & 4.32 & 0.01 & 0.15 & -5.01 & 4.5 & 0.1 & 4.7 & -18.7 & 45 & 0.03 & 0.03 & 1 \\
3568 & KOI-308 & 19 35 43.1 & +41 36 10 & 6121 & 4.09 & 0.02 & 0.15 & -5.01 & 12.7 & 10.1 & 5.5 & -38.9 & 47 & 0.02 & 0.03 & 1 \\
3569 & KOI-2608 & 19 02 51.2 & +41 36 21 & 6173 & 3.89 & -0.02 & 0.12 & -5.31 & 21.8 & 17.7 & 6.8 & -24.9 & 48 & 0.03 & 0.03 & 1 \\
3570 & KOI-415 & 19 33 13.5 & +41 36 23 & 5836 & 4.47 & -0.16 & 0.12 & -5.34 & 3.2 & 0.1 & 3.8 & -4.6 & 47 & 0.03 & 0.06 & 1 \\
3571 & KOI-4302 & 19 34 43.5 & +41 36 43 & 6103 & 4.11 & -0.08 & 0.13 & -5.28 & 7.3 & 4.6 & 5.4 & -1.8 & 48 & 0.02 & 0.05 & 1 \\
3572 & KOI-1688 & 19 53 55.5 & +41 36 55 & 5949 & 4.14 & 0.17 & 0.09 & nan & 7.2 & 5.4 & 4.4 & -28.3 & 36 & 0.03 & 0.09 & 1 \\
3573 & KOI-660 & 18 59 40.7 & +41 37 02 & 5311 & 3.92 & -0.13 & 0.15 & -5.10 & 2.9 & 0.1 & 3.6 & -57.3 & 51 & 0.02 & 0.03 & 1 \\
3574 & KOI-307 & 19 32 43.3 & +41 37 04 & 6008 & 4.41 & -0.11 & 0.13 & -5.21 & 6.9 & 4.7 & 4.7 & 19.6 & 47 & 0.02 & 0.03 & 1 \\
3575 & KOI-1613 & 19 01 54.4 & +41 37 58 & 6190 & 4.34 & -0.32 & 0.12 & -5.34 & 11.5 & 8.6 & 6.1 & 8.3 & 48 & 0.02 & 0.03 & 1 \\
3576 & KOI-3436 & 18 55 56.7 & +41 39 01 & 4948 & 4.48 & 0.14 & 0.51 & -4.50 & 3.6 & 3.1 & 1.8 & -28.6 & 52 & 0.02 & 0.03 & 1 \\
3577 & KOI-219 & 19 48 51.4 & +41 39 51 & 6005 & 4.14 & 0.13 & 0.13 & -5.27 & 16.0 & 13.2 & 4.7 & -8.4 & 50 & 0.03 & 0.03 & 1 \\
3578 & KOI-611 & 19 53 10.6 & +41 41 02 & 6267 & 4.24 & 0.09 & 0.12 & -5.32 & 14.8 & 11.5 & 6.9 & -19.2 & 46 & 0.03 & 0.03 & 1 \\
3579 & KOI-2753 & 18 56 10.2 & +41 41 57 & 5796 & 4.26 & 0.18 & 0.12 & -5.37 & 4.1 & 1.8 & 3.6 & 5.0 & 49 & 0.02 & 0.02 & 1 \\
3580 & KOI-1128 & 19 25 44.0 & +41 42 12 & 5357 & 4.53 & -0.08 & 0.10 & -5.49 & 2.5 & 0.6 & 2.3 & -4.7 & 50 & 0.02 & 0.03 & 1 \\
3581 & KOI-662 & 19 28 44.9 & +41 43 37 & 5891 & 4.12 & 0.02 & 0.14 & -5.17 & 3.9 & 0.1 & 4.0 & -18.6 & 49 & 0.02 & 0.03 & 1 \\
3582 & KOI-3503 & 19 32 36.2 & +41 43 45 & 6097 & 4.28 & -0.44 & 0.12 & -5.30 & 4.8 & 0.1 & 5.3 & -1.8 & 47 & 0.02 & 0.03 & 1 \\
3583 & KOI-661 & 19 01 23.3 & +41 45 43 & 5863 & 4.45 & 0.02 & 0.16 & -5.00 & 4.4 & 1.9 & 3.9 & 18.7 & 48 & 0.02 & 0.02 & 1 \\
3584 & KOI-1121 & 19 21 24.7 & +41 46 11 & 5826 & 4.32 & 0.06 & 0.15 & -5.08 & 6.4 & 4.6 & 3.7 & -49.7 & 57 & 0.02 & 0.04 & 1 \\
3585 & KOI-1127 & 19 20 51.6 & +41 46 33 & 5586 & 4.10 & 0.29 & 0.21 & -4.81 & 3.7 & 2.3 & 2.8 & -35.1 & 23 & 0.05 & 0.09 & 1 \\
3586 & KOI-2857 & 18 58 15.8 & +41 46 43 & 6117 & 4.15 & 0.26 & 0.11 & -5.54 & 8.0 & 5.4 & 5.5 & -13.9 & 48 & 0.02 & 0.03 & 1 \\
3587 & KOI-2948 & 19 17 34.7 & +41 46 56 & 5512 & 4.03 & 0.42 & 0.14 & -5.15 & 4.5 & 3.6 & 2.6 & -38.6 & 52 & 0.02 & 0.02 & 1 \\
3588 & KOI-3456 & 19 28 00.5 & +41 47 13 & 5663 & 4.59 & -0.28 & 0.21 & -4.80 & 9.3 & 8.0 & 3.1 & -56.6 & 50 & 0.02 & 0.03 & 1 \\
3589 & KOI-1230 & 19 55 47.6 & +41 48 44 & 4968 & 3.09 & -0.05 & 0.14 & -5.21 & 4.4 & 2.7 & 3.4 & -30.6 & 53 & 0.02 & 0.03 & 2 \\
3590 & KOI-2840 & 19 53 24.9 & +41 49 12 & 5700 & 4.22 & -0.02 & 0.15 & -5.06 & 3.7 & 1.6 & 3.2 & -17.7 & 50 & 0.02 & 0.09 & 1 \\
3591 & Kepler-172 & 18 53 28.4 & +41 49 19 & 5549 & 4.44 & 0.29 & 0.00 & 0.00 & 3.9 & 2.7 & 2.7 & -14.7 & 47 & 0.03 & 0.06 & 1 \\
3592 & KOI-664 & 19 26 32.3 & +41 50 02 & 5718 & 4.37 & 0.02 & 0.14 & -5.15 & 3.2 & 0.1 & 3.3 & -11.7 & 49 & 0.02 & 0.03 & 1 \\
3593 & Kepler-206 & 19 26 32.3 & +41 50 02 & 5763 & 4.39 & 0.03 & 0.00 & 0.00 & 4.1 & 2.0 & 3.4 & -12.6 & 75 & 0.02 & 0.02 & 1 \\
3594 & KOI-372 & 19 56 29.4 & +41 52 00 & 5778 & 4.53 & -0.09 & 0.24 & nan & 5.1 & 3.5 & 3.5 & 11.5 & 89 & 0.02 & 0.02 & 2 \\
3595 & KOI-1241 & 19 35 02.0 & +41 52 19 & 4790 & 3.27 & 0.38 & 0.14 & -5.17 & 3.2 & 0.1 & 3.4 & -55.1 & 183 & 0.02 & 0.03 & 1 \\
3596 & KOI-2408 & 19 08 15.9 & +41 52 30 & 5481 & 4.51 & -0.14 & 0.16 & -5.04 & 3.2 & 1.8 & 2.6 & 17.2 & 49 & 0.02 & 0.02 & 1 \\
3597 & KOI-511 & 19 38 35.2 & +41 53 03 & 5887 & 4.36 & 0.05 & 0.10 & -6.19 & 5.5 & 3.6 & 4.0 & 14.2 & 36 & 0.25 & 0.08 & 1 \\
3598 & KOI-176 & 19 26 35.2 & +41 53 05 & 6318 & 4.17 & -0.18 & 0.13 & -5.26 & 13.5 & 10.0 & 7.5 & -47.6 & 47 & 0.02 & 0.03 & 1 \\
3599 & KOI-94 & 19 49 19.9 & +41 53 28 & 6144 & 4.16 & 0.11 & 0.12 & -5.35 & 9.4 & 6.9 & 5.7 & -21.9 & 64 & 0.02 & 0.03 & 3 \\
3600 & KOI-270 & 19 34 55.9 & +41 54 03 & 5739 & 4.35 & -0.11 & 0.12 & -5.37 & 4.8 & 3.2 & 3.4 & 12.2 & 49 & 0.02 & 0.02 & 1 \\
3601 & KOI-3117 & 19 28 29.2 & +41 55 37 & 5501 & 4.47 & 0.01 & 0.25 & -4.69 & 3.6 & 2.4 & 2.6 & -43.5 & 51 & 0.02 & 0.05 & 1 \\
3602 & KOI-4657 & 19 33 10.3 & +41 59 51 & 5303 & 4.49 & -0.09 & 0.14 & -5.18 & 2.5 & 0.9 & 2.2 & -50.2 & 52 & 0.02 & 0.03 & 1 \\
3603 & KOI-3438 & 19 19 40.4 & +42 00 05 & 6013 & 4.27 & -0.16 & 0.13 & -5.26 & 5.5 & 2.6 & 4.8 & -50.6 & 48 & 0.02 & 0.03 & 1 \\
3604 & KOI-1239 & 19 28 42.9 & +42 00 21 & 5752 & 4.44 & -0.11 & 0.18 & -4.89 & 3.5 & 0.5 & 3.4 & -19.0 & 30 & 0.04 & 0.04 & 1 \\
3605 & KOI-3287 & 18 55 04.9 & +42 01 38 & 5892 & 4.27 & -0.12 & 0.11 & -5.57 & 4.6 & 2.2 & 4.0 & -39.1 & 41 & 0.03 & 0.03 & 1 \\
3606 & KOI-857 & 19 00 26.5 & +42 02 02 & 5068 & 4.48 & 0.19 & 0.23 & -4.87 & 2.9 & 2.1 & 1.9 & -48.7 & 37 & 0.03 & 0.03 & 1 \\
3607 & KOI-1242 & 19 28 54.8 & +42 02 07 & 6128 & 4.26 & -0.00 & 0.11 & -5.49 & 7.0 & 4.0 & 5.6 & -7.4 & 47 & 0.02 & 0.03 & 1 \\
3608 & KOI-2559 & 19 26 25.6 & +42 02 09 & 5847 & 4.39 & 0.10 & 0.10 & -5.84 & 4.4 & 2.1 & 3.8 & -37.1 & 45 & 0.03 & 0.04 & 1 \\
3609 & KOI-3237 & 19 01 19.4 & +42 02 26 & 5768 & 4.48 & 0.10 & 0.28 & -4.56 & 6.3 & 4.9 & 3.5 & -30.8 & 50 & 0.02 & 0.03 & 1 \\
3610 & KOI-2838 & 19 28 47.9 & +42 02 46 & 5616 & 3.98 & 0.07 & 0.14 & -5.16 & 3.8 & 0.1 & 4.0 & -38.9 & 49 & 0.02 & 0.02 & 1 \\
3611 & KOI-1227 & 19 50 49.7 & +42 02 51 & 6131 & 4.48 & -0.39 & 0.34 & -4.39 & 21.7 & 15.8 & 5.6 & 34.2 & 47 & 0.04 & 0.06 & 1 \\
3612 & KOI-2737 & 19 37 00.8 & +42 03 45 & 5570 & 4.07 & 0.28 & 0.11 & -5.42 & 3.9 & 2.6 & 2.8 & -88.1 & 50 & 0.02 & 0.02 & 1 \\
3613 & KOI-4159 & 19 29 08.8 & +42 04 21 & 5161 & 4.39 & 0.07 & 0.13 & -5.23 & 3.0 & 2.2 & 2.0 & -87.9 & 36 & 0.03 & 0.04 & 1 \\
3614 & KOI-1692 & 19 38 41.8 & +42 04 32 & 5289 & 4.40 & 0.26 & 0.23 & -4.81 & 3.6 & 2.8 & 2.2 & -23.9 & 54 & 0.02 & 0.06 & 1 \\
3615 & KOI-612 & 18 59 52.4 & +42 04 45 & 5085 & 4.50 & -0.04 & 0.14 & -5.17 & 2.6 & 1.7 & 1.9 & 20.5 & 45 & 0.03 & 0.03 & 1 \\
3616 & KOI-666 & 19 44 07.7 & +42 07 54 & 5568 & 4.45 & 0.06 & 0.16 & -5.00 & 3.5 & 2.0 & 2.8 & -41.6 & 49 & 0.02 & 0.03 & 1 \\
3617 & KOI-4651 & 19 52 20.9 & +42 09 52 & 5561 & 4.37 & -0.07 & 0.16 & -5.04 & 4.7 & 3.7 & 2.8 & -10.7 & 35 & 0.15 & 0.09 & 1 \\
3618 & KOI-665 & 19 20 07.3 & +42 09 58 & 5893 & 4.09 & 0.25 & 0.14 & -5.18 & 6.5 & 4.8 & 4.0 & -48.5 & 49 & 0.02 & 0.02 & 1 \\
3619 & Kepler-207 & 19 20 07.3 & +42 09 58 & 5896 & 4.05 & 0.26 & 0.13 & -5.22 & 7.0 & 5.4 & 4.1 & -49.8 & 84 & 0.01 & 0.03 & 1 \\
3620 & KOI-561 & 18 48 01.1 & +42 10 36 & 5028 & 4.51 & -0.13 & 0.19 & -4.97 & 1.2 & 0.1 & 1.8 & -31.5 & 52 & 0.02 & 0.03 & 1 \\
3621 & KOI-1240 & 19 25 33.7 & +42 10 50 & 5493 & 4.41 & 0.06 & 0.11 & -5.37 & 2.9 & 1.1 & 2.6 & 3.0 & 35 & 0.03 & 0.03 & 1 \\
3622 & KOI-2092 & 19 33 10.5 & +42 11 47 & 5659 & 4.61 & -0.33 & 0.21 & -4.78 & 3.1 & 0.1 & 3.1 & 4.7 & 27 & 0.05 & 0.08 & 1 \\
3623 & KOI-5324 & 19 11 37.6 & +42 12 31 & 4960 & 3.35 & -0.08 & 0.12 & -5.27 & 3.6 & 0.9 & 3.4 & -15.1 & 36 & 0.03 & 0.04 & 1 \\
3624 & KOI-4072 & 18 55 03.4 & +42 13 20 & 5855 & 4.30 & 0.12 & 0.12 & -5.33 & 4.5 & 2.1 & 3.9 & 2.9 & 48 & 0.02 & 0.05 & 1 \\
3625 & KOI-2678 & 19 29 33.3 & +42 14 00 & 5284 & 4.50 & -0.02 & 0.40 & -4.50 & 7.6 & 6.8 & 2.2 & -31.6 & 44 & 0.03 & 0.05 & 1 \\
3626 & KOI-177 & 19 52 42.5 & +42 14 13 & 5754 & 4.44 & -0.04 & 0.14 & -5.14 & 4.0 & 1.9 & 3.4 & -8.3 & 49 & 0.02 & 0.02 & 1 \\
3627 & KOI-1695 & 19 53 15.5 & +42 14 51 & 5915 & 4.30 & 0.15 & 0.10 & -5.72 & 5.1 & 2.9 & 4.2 & -16.9 & 44 & 0.03 & 0.03 & 1 \\
3628 & KOI-3980 & 18 44 58.3 & +42 15 18 & 5742 & 4.37 & 0.10 & 0.11 & -5.57 & 3.9 & 1.9 & 3.4 & -18.7 & 35 & 0.03 & 0.04 & 1 \\
3629 & KOI-1375 & 19 13 16.9 & +42 15 41 & 6245 & 4.19 & -0.15 & 0.12 & -5.40 & 10.9 & 7.7 & 6.7 & -3.3 & 47 & 0.02 & 0.03 & 1 \\
3630 & KOI-4850 & 19 37 20.0 & +42 15 51 & 5577 & 4.53 & -0.01 & 0.13 & -5.20 & 3.2 & 1.4 & 2.8 & -12.6 & 47 & 0.03 & 0.04 & 1 \\
3631 & KOI-2086 & 19 15 50.7 & +42 15 54 & 5887 & 4.20 & -0.04 & 0.11 & -5.48 & 4.5 & 2.0 & 4.0 & -37.4 & 49 & 0.02 & 0.03 & 1 \\
3632 & Kepler-60 & 19 15 50.7 & +42 15 54 & 5883 & 4.18 & -0.08 & 0.00 & 0.00 & 4.2 & 1.2 & 4.0 & -36.2 & 65 & 0.02 & 0.08 & 1 \\
3633 & KOI-4871 & 19 14 07.0 & +42 16 35 & 6354 & 4.36 & -0.06 & 0.12 & -5.42 & 8.5 & 3.0 & 7.9 & 6.4 & 45 & 0.03 & 0.03 & 1 \\
3634 & KOI-4184 & 18 47 35.5 & +42 17 09 & 4841 & 4.49 & -0.05 & 0.37 & -4.69 & 5.1 & 4.8 & 1.7 & -24.8 & 54 & 0.02 & 0.03 & 1 \\
3635 & KOI-864 & 19 08 58.2 & +42 18 05 & 5403 & 4.48 & -0.03 & 0.18 & -4.94 & 2.8 & 1.2 & 2.4 & -5.8 & 29 & 0.04 & 0.05 & 1 \\
3636 & KOI-3244 & 19 11 03.9 & +42 19 22 & 4900 & 3.03 & -0.03 & 0.13 & -5.24 & 4.1 & 2.3 & 3.4 & -10.5 & 53 & 0.02 & 0.03 & 1 \\
3637 & KOI-4188 & 19 44 25.0 & +42 20 33 & 6110 & 4.54 & 0.29 & 0.18 & -4.87 & 6.0 & 2.3 & 5.5 & 4.4 & 34 & 0.11 & 0.05 & 1 \\
3638 & KOI-4674 & 18 50 19.9 & +42 20 47 & 5654 & 4.27 & 0.11 & 0.15 & -5.06 & 3.5 & 1.7 & 3.0 & -61.6 & 47 & 0.02 & 0.02 & 1 \\
3639 & KOI-201 & 19 08 31.3 & +42 21 01 & 5408 & 4.29 & 0.33 & 0.16 & -5.03 & 3.7 & 2.8 & 2.4 & -61.9 & 33 & 0.05 & 0.08 & 1 \\
3640 & KOI-2571 & 19 32 32.9 & +42 21 02 & 5218 & 4.40 & 0.19 & 0.13 & -5.19 & 7.0 & 6.2 & 2.1 & -14.8 & 38 & 0.03 & 0.03 & 1 \\
3641 & KOI-163 & 19 12 16.2 & +42 21 19 & 5066 & 4.55 & -0.36 & 0.14 & -5.18 & 1.7 & 0.1 & 1.9 & -9.3 & 51 & 0.02 & 0.03 & 1 \\
3642 & KOI-2220 & 19 36 33.1 & +42 22 14 & 5762 & 4.31 & 0.15 & 0.10 & -5.67 & 4.2 & 2.2 & 3.4 & 3.8 & 35 & 0.04 & 0.03 & 1 \\
3643 & KOI-1366 & 19 05 25.9 & +42 24 23 & 5404 & 4.48 & 0.00 & 0.17 & -4.99 & 2.9 & 1.5 & 2.4 & -21.6 & 34 & 0.03 & 0.05 & 1 \\
3644 & KOI-2925 & 19 53 11.6 & +42 26 04 & 5357 & 4.48 & 0.09 & 0.17 & -4.98 & 3.0 & 1.8 & 2.3 & 13.8 & 52 & 0.02 & 0.02 & 1 \\
3645 & KOI-1363 & 19 11 39.9 & +42 26 14 & 5635 & 4.46 & 0.16 & 0.23 & -4.73 & 3.2 & 1.1 & 3.0 & -0.2 & 27 & 0.04 & 0.07 & 1 \\
3646 & KOI-2087 & 18 46 14.8 & +42 27 02 & 5958 & 4.45 & 0.01 & 0.10 & -6.23 & 5.3 & 2.8 & 4.4 & -17.6 & 47 & 0.03 & 0.03 & 1 \\
3647 & KOI-1628 & 19 53 35.0 & +42 27 35 & 6234 & 4.50 & 0.16 & 0.16 & -4.99 & 12.6 & 9.6 & 6.6 & -26.0 & 51 & 0.02 & 0.06 & 1 \\
3648 & KOI-1367 & 19 07 32.9 & +42 28 17 & 4905 & 4.57 & -0.13 & 0.13 & -5.21 & 1.8 & 0.1 & 1.7 & -27.5 & 38 & 0.03 & 0.04 & 1 \\
3649 & KOI-4382 & 19 12 39.4 & +42 28 52 & 6246 & 4.20 & -0.06 & 0.13 & -5.26 & 12.3 & 9.2 & 6.7 & 7.8 & 47 & 0.03 & 0.03 & 1 \\
3650 & KOI-2879 & 19 46 48.5 & +42 30 31 & 5407 & 4.47 & -0.11 & 0.17 & -4.99 & 3.5 & 2.4 & 2.4 & -6.9 & 50 & 0.02 & 0.02 & 1 \\
3651 & KOI-670 & 19 27 17.6 & +42 30 58 & 5543 & 4.03 & 0.11 & 0.12 & -5.34 & 3.8 & 2.6 & 2.7 & -71.3 & 50 & 0.02 & 0.02 & 1 \\
3652 & KOI-671 & 19 35 33.6 & +42 31 41 & 6033 & 4.21 & -0.00 & 0.09 & -3.67 & 6.6 & 4.2 & 4.9 & -6.9 & 53 & 0.03 & 0.03 & 2 \\
3653 & KOI-2215 & 19 45 01.2 & +42 31 49 & 6539 & 4.56 & -0.04 & 0.12 & -5.44 & 11.2 & 0.1 & 10.7 & -22.9 & 50 & 0.03 & 0.04 & 1 \\
3654 & KOI-3689 & 19 03 53.2 & +42 32 45 & 5971 & 4.25 & 0.03 & 0.14 & -5.13 & 5.7 & 3.3 & 4.5 & 19.3 & 42 & 0.03 & 0.03 & 1 \\
3655 & KOI-312 & 19 45 52.2 & +42 35 56 & 6178 & 4.13 & 0.08 & 0.14 & -5.10 & 11.7 & 9.0 & 6.0 & -39.8 & 48 & 0.02 & 0.03 & 1 \\
3656 & KOI-872 & 19 17 04.5 & +42 36 15 & 5091 & 4.49 & 0.11 & 0.32 & -4.68 & 2.2 & 1.0 & 1.9 & -21.3 & 32 & 0.04 & 0.04 & 1 \\
3657 & KOI-673 & 19 35 20.3 & +42 37 30 & 6194 & 4.16 & 0.02 & 0.17 & -4.92 & 15.7 & 12.5 & 6.2 & -29.6 & 47 & 0.03 & 0.03 & 1 \\
3658 & KOI-672 & 19 24 40.7 & +42 38 27 & 5519 & 4.48 & 0.05 & 0.14 & -5.11 & 2.9 & 1.1 & 2.7 & -14.2 & 49 & 0.02 & 0.02 & 1 \\
3659 & KOI-2083 & 18 57 57.7 & +42 38 54 & 5975 & 4.22 & -0.07 & 0.23 & -4.67 & 7.5 & 5.5 & 4.5 & -20.5 & 48 & 0.02 & 0.03 & 1 \\
3660 & KOI-3907 & 19 47 59.5 & +42 39 12 & 6473 & 4.34 & -0.13 & 0.16 & -4.95 & 21.6 & 16.9 & 9.6 & -9.6 & 48 & 0.03 & 0.04 & 1 \\
3661 & Kepler-1542 & 19 02 54.8 & +42 39 16 & 5615 & 4.41 & 0.04 & 0.00 & 0.00 & 3.4 & 1.6 & 2.9 & -10.7 & 109 & 0.02 & 0.02 & 1 \\
3662 & KOI-4032 & 19 02 54.8 & +42 39 16 & 5614 & 4.42 & 0.05 & 0.15 & -5.06 & 3.1 & 0.8 & 2.9 & -9.4 & 49 & 0.02 & 0.05 & 1 \\
3663 & KOI-3012 & 19 17 19.0 & +42 39 21 & 5639 & 4.33 & -0.43 & 0.15 & -5.08 & 3.2 & 0.9 & 3.0 & -63.5 & 49 & 0.02 & 0.03 & 1 \\
3664 & KOI-4473 & 19 44 14.4 & +42 39 22 & 5895 & 3.88 & 0.00 & 0.11 & -5.68 & 7.3 & 5.0 & 4.9 & -18.4 & 50 & 0.02 & 0.03 & 1 \\
3665 & KOI-3083 & 19 11 54.9 & +42 40 46 & 5785 & 4.35 & 0.28 & 0.14 & -5.11 & 4.1 & 2.0 & 3.5 & -26.0 & 50 & 0.02 & 0.02 & 1 \\
3666 & KOI-3100 & 19 13 58.4 & +42 41 33 & 5941 & 4.12 & 0.27 & 0.13 & -5.24 & 4.6 & 1.4 & 4.3 & -18.2 & 48 & 0.03 & 0.03 & 1 \\
3667 & KOI-1379 & 19 39 56.5 & +42 43 40 & 5733 & 4.37 & -0.11 & 0.14 & -5.19 & 3.7 & 1.4 & 3.3 & -29.2 & 43 & 0.03 & 0.03 & 1 \\
3668 & KOI-1618 & 19 44 11.4 & +42 44 35 & 6143 & 4.10 & 0.13 & 0.11 & -5.54 & 12.0 & 9.4 & 5.7 & -6.3 & 50 & 0.02 & 0.03 & 1 \\
3669 & KOI-5375 & 19 42 04.2 & +42 45 32 & 4936 & 2.99 & -0.19 & 0.13 & -5.20 & 7.3 & 5.6 & 4.0 & -28.6 & 36 & 0.03 & 0.10 & 1 \\
3670 & KOI-369 & 18 47 39.8 & +42 46 32 & 6161 & 4.24 & -0.12 & 0.14 & -5.13 & 8.8 & 6.1 & 5.9 & -3.4 & 47 & 0.02 & 0.03 & 1 \\
3671 & KOI-238 & 19 47 59.7 & +42 46 55 & 6121 & 4.26 & -0.06 & 0.10 & -5.76 & 7.5 & 4.8 & 5.5 & -22.1 & 41 & 0.03 & 0.03 & 1 \\
3672 & KOI-987 & 19 42 17.8 & +42 48 23 & 5459 & 4.54 & 0.03 & 0.16 & -5.04 & 2.8 & 0.9 & 2.5 & -8.5 & 49 & 0.02 & 0.02 & 1 \\
3673 & KOI-4136 & 18 47 17.6 & +42 48 40 & 5653 & 3.92 & 0.09 & 0.13 & -5.27 & 4.7 & 2.0 & 4.1 & -26.9 & 50 & 0.02 & 0.02 & 1 \\
3674 & KOI-2051 & 19 03 11.9 & +42 48 42 & 5786 & 4.32 & -0.09 & 0.12 & -5.42 & 3.8 & 1.1 & 3.5 & -43.5 & 34 & 0.03 & 0.03 & 1 \\
3675 & KOI-1961 & 19 10 17.1 & +42 48 50 & 5318 & 4.55 & -0.07 & 0.22 & -4.81 & 4.3 & 3.6 & 2.2 & -6.2 & 50 & 0.02 & 0.02 & 1 \\
3676 & KOI-2916 & 19 10 56.6 & +42 49 24 & 4928 & 4.52 & -0.00 & 0.16 & -5.10 & 2.1 & 1.0 & 1.7 & 2.4 & 43 & 0.03 & 0.03 & 1 \\
3677 & KOI-2561 & 18 51 49.7 & +42 49 32 & 6025 & 4.26 & 0.05 & 0.13 & -5.27 & 5.7 & 2.9 & 4.8 & -19.4 & 48 & 0.02 & 0.03 & 1 \\
3678 & KOI-2516 & 19 41 48.9 & +42 51 32 & 5356 & 3.90 & 0.21 & 0.12 & -5.27 & 3.7 & 0.0 & 3.7 & -52.7 & 47 & 0.03 & 0.03 & 1 \\
3679 & KOI-456 & 19 11 05.7 & +42 52 09 & 5575 & 4.40 & 0.15 & 0.11 & -5.48 & 3.4 & 1.7 & 2.8 & -24.9 & 36 & 0.03 & 0.03 & 1 \\
3680 & KOI-1979 & 19 16 10.1 & +42 52 57 & 5722 & 4.37 & 0.15 & 0.11 & -5.48 & 4.1 & 2.4 & 3.3 & -63.9 & 47 & 0.03 & 0.03 & 1 \\
3681 & KOI-5379 & 19 27 41.5 & +42 53 35 & 5004 & 3.30 & 0.02 & 0.14 & -5.17 & 3.7 & 1.2 & 3.4 & -45.6 & 37 & 0.03 & 0.03 & 1 \\
3682 & KOI-1862 & 19 32 22.6 & +42 53 47 & 5581 & 4.43 & 0.18 & 0.12 & -5.40 & 3.4 & 1.8 & 2.8 & 0.9 & 50 & 0.02 & 0.02 & 1 \\
3683 & KOI-674 & 19 21 18.6 & +42 53 54 & 4842 & 3.62 & 0.22 & 0.13 & -5.23 & 3.0 & 0.1 & 3.4 & -52.1 & 55 & 0.02 & 0.03 & 1 \\
3684 & KOI-373 & 19 28 56.4 & +42 54 34 & 5842 & 4.51 & -0.33 & 0.13 & -5.21 & 3.8 & 0.1 & 3.8 & 3.7 & 48 & 0.02 & 0.02 & 1 \\
3685 & KOI-1378 & 19 42 02.6 & +42 55 50 & 5712 & 4.21 & -0.24 & 0.17 & -4.96 & 3.7 & 1.6 & 3.2 & -39.9 & 48 & 0.03 & 0.05 & 1 \\
3686 & KOI-4864 & 19 01 50.1 & +42 55 52 & 5730 & 3.76 & -0.26 & 0.13 & -5.25 & 4.7 & 1.7 & 4.3 & -10.1 & 48 & 0.02 & 0.03 & 1 \\
3687 & KOI-4665 & 19 32 16.5 & +42 57 26 & 5738 & 4.24 & 0.03 & 0.12 & -5.30 & 4.0 & 2.1 & 3.3 & -56.1 & 49 & 0.02 & 0.02 & 1 \\
3688 & KOI-266 & 19 41 37.0 & +42 58 53 & 6126 & 4.29 & -0.03 & 0.12 & -5.47 & 7.5 & 4.6 & 5.6 & 13.9 & 46 & 0.03 & 0.03 & 3 \\
3689 & KOI-3096 & 19 39 48.3 & +43 00 45 & 5551 & 4.16 & -0.05 & 0.18 & -4.91 & 3.5 & 1.9 & 2.7 & -75.6 & 48 & 0.02 & 0.03 & 1 \\
3690 & KOI-313 & 18 48 32.5 & +43 02 21 & 5208 & 4.51 & 0.01 & 0.21 & -4.89 & 1.5 & 0.1 & 2.0 & -30.3 & 51 & 0.02 & 0.03 & 1 \\
3691 & KOI-884 & 19 14 34.2 & +43 02 21 & 4964 & 4.48 & 0.22 & 0.19 & -4.98 & 1.9 & 0.2 & 1.8 & -56.1 & 41 & 0.03 & 0.03 & 1 \\
3692 & KOI-1848 & 19 06 50.6 & +43 02 36 & 5970 & 4.26 & -0.10 & 0.15 & -5.06 & 8.0 & 6.1 & 4.5 & 16.7 & 46 & 0.02 & 0.03 & 1 \\
3693 & KOI-2357 & 19 32 48.9 & +43 03 25 & 5672 & 4.44 & -0.00 & 0.15 & -5.11 & 3.4 & 1.1 & 3.1 & -13.2 & 32 & 0.04 & 0.04 & 1 \\
3694 & KOI-5393 & 19 42 34.8 & +43 03 55 & 4777 & 3.15 & 0.04 & 0.12 & -5.31 & 3.7 & 1.4 & 3.4 & 1.7 & 38 & 0.03 & 0.05 & 1 \\
3695 & KOI-3193 & 19 08 18.9 & +43 04 08 & 4890 & 3.14 & 0.11 & 0.06 & -5.76 & 4.0 & 2.0 & 3.4 & -8.6 & 44 & 0.03 & 0.05 & 1 \\
3696 & KOI-1890 & 19 32 19.1 & +43 04 25 & 6038 & 4.09 & 0.11 & 0.13 & -5.22 & 8.6 & 6.5 & 4.9 & -47.5 & 49 & 0.02 & 0.06 & 1 \\
3697 & KOI-457 & 19 22 04.0 & +43 05 02 & 5018 & 4.51 & 0.18 & 0.35 & -4.66 & 2.8 & 2.0 & 1.8 & -35.0 & 52 & 0.03 & 0.03 & 1 \\
3698 & KOI-679 & 19 10 29.0 & +43 08 30 & 5826 & 4.14 & 0.18 & 0.09 & nan & 5.3 & 3.6 & 3.7 & -8.1 & 48 & 0.02 & 0.03 & 1 \\
3699 & KOI-678 & 19 01 45.4 & +43 10 07 & 5096 & 4.52 & 0.08 & 0.54 & -4.43 & 3.0 & 2.3 & 1.9 & -27.6 & 53 & 0.02 & 0.03 & 1 \\
3700 & KOI-4663 & 19 10 40.9 & +43 11 50 & 5468 & 3.86 & 0.23 & 0.12 & -5.30 & 4.6 & 2.5 & 3.8 & -23.1 & 52 & 0.14 & 0.04 & 1 \\
3701 & Kepler-435 & 19 29 09.0 & +43 11 50 & 6144 & 3.89 & 0.04 & 0.00 & 0.00 & 7.9 & 4.2 & 6.6 & -26.4 & 77 & 0.02 & 0.03 & 1 \\
3702 & KOI-150 & 19 47 55.4 & +43 12 35 & 5598 & 4.54 & -0.43 & 0.16 & -5.03 & 3.0 & 0.6 & 2.9 & -85.3 & 51 & 0.02 & 0.02 & 1 \\
3703 & KOI-4160 & 19 31 08.3 & +43 12 58 & 5723 & 4.52 & 0.17 & 0.27 & -4.60 & 4.8 & 3.4 & 3.3 & -18.6 & 51 & 0.02 & 0.02 & 1 \\
3704 & KOI-3128 & 19 29 55.1 & +43 13 37 & 6110 & 3.94 & -0.06 & 0.12 & -5.39 & 6.8 & 2.5 & 6.3 & -23.9 & 49 & 0.02 & 0.06 & 1 \\
3705 & Kepler-431 & 18 44 27.0 & +43 13 40 & 5901 & 4.04 & -0.06 & 0.13 & -5.22 & 6.5 & 4.7 & 4.1 & -10.9 & 85 & 0.03 & 0.02 & 1 \\
3706 & KOI-3097 & 18 44 27.0 & +43 13 40 & 5948 & 4.05 & -0.03 & 0.12 & -5.33 & 6.6 & 4.7 & 4.4 & -11.2 & 49 & 0.02 & 0.03 & 1 \\
3707 & KOI-2631 & 18 48 57.5 & +43 14 39 & 5859 & 4.21 & -0.38 & 0.12 & -5.33 & 4.2 & 1.1 & 3.9 & -29.2 & 48 & 0.02 & 0.03 & 1 \\
3708 & KOI-683 & 19 51 17.8 & +43 15 30 & 5860 & 4.38 & 0.13 & 0.09 & -6.73 & 3.8 & 0.1 & 3.9 & -8.4 & 47 & 0.03 & 0.03 & 1 \\
3709 & KOI-1706 & 19 47 48.5 & +43 16 19 & 5135 & 4.42 & 0.06 & 0.15 & -5.10 & 2.9 & 2.1 & 2.0 & -53.0 & 49 & 0.02 & 0.03 & 1 \\
3710 & KOI-568 & 19 09 10.9 & +43 16 48 & 5284 & 4.46 & -0.03 & 0.15 & -5.09 & 2.7 & 1.5 & 2.2 & -10.5 & 43 & 0.03 & 0.04 & 1 \\
3711 & KOI-4614 & 18 46 55.4 & +43 16 56 & 6012 & 4.14 & 0.08 & 0.11 & -5.54 & 7.2 & 5.1 & 4.7 & -27.4 & 49 & 0.02 & 0.03 & 1 \\
3712 & KOI-1898 & 19 05 08.6 & +43 19 14 & 5738 & 4.35 & -0.04 & 0.18 & -4.91 & 3.8 & 1.7 & 3.3 & -53.0 & 45 & 0.03 & 0.03 & 1 \\
3713 & KOI-3943 & 19 23 29.4 & +43 19 59 & 6178 & 4.18 & -0.02 & 0.11 & -5.51 & 9.7 & 6.9 & 6.0 & -43.9 & 49 & 0.02 & 0.03 & 1 \\
3714 & KOI-315 & 19 49 05.3 & +43 20 00 & 4734 & 4.46 & -0.24 & 0.33 & -4.79 & 1.9 & 0.9 & 1.6 & 16.8 & 53 & 0.02 & 0.03 & 1 \\
3715 & KOI-1528 & 19 38 36.0 & +43 20 08 & 5206 & 4.39 & -0.03 & 0.09 & -5.56 & 2.6 & 1.4 & 2.0 & 9.0 & 46 & 0.03 & 0.09 & 1 \\
3716 & KOI-2722 & 19 13 28.9 & +43 21 17 & 6138 & 4.38 & -0.05 & 0.14 & -5.08 & 7.8 & 4.9 & 5.7 & -3.0 & 46 & 0.03 & 0.03 & 1 \\
3717 & Kepler-402 & 19 13 28.9 & +43 21 17 & 6121 & 4.30 & -0.06 & 0.15 & -5.05 & 7.9 & 5.2 & 5.5 & -1.0 & 81 & 0.03 & 0.02 & 1 \\
3718 & KOI-892 & 19 21 34.4 & +43 21 50 & 5007 & 4.69 & -0.08 & 0.87 & -4.22 & 3.0 & 2.3 & 1.8 & 10.0 & 22 & 0.07 & 0.08 & 1 \\
3719 & KOI-2585 & 19 14 38.6 & +43 22 05 & 5990 & 4.31 & -0.37 & 0.17 & -4.90 & 4.6 & 0.1 & 4.6 & -72.4 & 48 & 0.02 & 0.03 & 1 \\
3720 & KOI-269 & 19 09 23.0 & +43 22 42 & 6324 & 4.20 & -0.03 & 0.13 & -5.24 & 14.1 & 10.6 & 7.5 & -13.8 & 47 & 0.02 & 0.03 & 1 \\
3721 & KOI-684 & 18 45 09.7 & +43 24 48 & 5217 & 3.81 & 0.04 & 0.22 & -4.84 & 3.5 & 0.1 & 3.5 & -81.0 & 52 & 0.02 & 0.02 & 1 \\
3722 & KOI-4561 & 19 19 30.0 & +43 25 15 & 5926 & 3.97 & -0.02 & 0.13 & -5.26 & 8.1 & 5.8 & 5.1 & -27.9 & 48 & 0.02 & 0.03 & 1 \\
3723 & KOI-1921 & 19 31 01.8 & +43 25 37 & 6382 & 4.07 & 0.04 & 0.13 & -5.22 & 22.5 & 17.9 & 8.3 & 9.0 & 46 & 0.03 & 0.03 & 1 \\
3724 & KOI-4482 & 19 56 22.9 & +43 26 21 & 6181 & 4.16 & -0.03 & 0.12 & -5.31 & 8.3 & 5.2 & 6.1 & 1.6 & 50 & 0.03 & 0.03 & 1 \\
3725 & KOI-3721 & 19 40 37.2 & +43 26 40 & 6415 & 4.15 & -0.20 & 0.10 & -5.83 & 6.9 & 0.1 & 8.7 & -8.7 & 48 & 0.03 & 0.03 & 1 \\
3726 & KOI-4022 & 18 52 30.9 & +43 27 25 & 5946 & 3.85 & -0.07 & 0.12 & -5.38 & 8.5 & 6.2 & 5.2 & -10.6 & 48 & 0.02 & 0.03 & 1 \\
3727 & KOI-1808 & 19 38 58.4 & +43 27 40 & 6118 & 4.34 & 0.03 & 0.13 & -5.28 & 8.3 & 5.7 & 5.5 & -6.0 & 50 & 0.03 & 0.03 & 1 \\
3728 & KOI-685 & 19 41 54.2 & +43 29 35 & 6378 & 3.88 & -0.07 & 0.14 & -5.15 & 18.4 & 13.7 & 9.6 & -31.0 & 43 & 0.03 & 0.03 & 1 \\
3729 & KOI-3023 & 18 49 00.4 & +43 29 38 & 6311 & 4.45 & -0.01 & 0.09 & nan & 8.8 & 4.4 & 7.4 & -33.0 & 47 & 0.02 & 0.03 & 1 \\
3730 & KOI-4725 & 19 56 33.1 & +43 29 55 & 4754 & 4.39 & -0.05 & 0.17 & -5.11 & 2.7 & 2.1 & 1.6 & -28.0 & 48 & 0.08 & 0.04 & 1 \\
3731 & KOI-2848 & 19 22 39.4 & +43 30 00 & 5636 & 4.14 & 0.23 & 0.16 & -5.01 & 4.2 & 2.9 & 3.0 & -82.5 & 51 & 0.02 & 0.02 & 1 \\
3732 & KOI-3787 & 19 13 45.4 & +43 30 19 & 5684 & 4.50 & 0.06 & 0.16 & -5.03 & 3.5 & 1.5 & 3.1 & -19.2 & 50 & 0.02 & 0.02 & 1 \\
3733 & KOI-171 & 19 38 58.1 & +43 32 13 & 6139 & 4.20 & 0.11 & 0.12 & -5.39 & 9.8 & 7.3 & 5.7 & -12.7 & 47 & 0.02 & 0.03 & 1 \\
3734 & KOI-1533 & 19 05 05.2 & +43 35 43 & 5890 & 4.42 & -0.23 & 0.10 & -6.33 & 3.9 & 0.1 & 4.0 & -0.1 & 47 & 0.02 & 0.03 & 1 \\
3735 & KOI-4582 & 19 45 20.8 & +43 36 00 & 5708 & 4.49 & -0.22 & 0.12 & -5.29 & 4.0 & 2.2 & 3.2 & -2.6 & 51 & 0.04 & 0.03 & 1 \\
3736 & KOI-1964 & 19 22 48.9 & +43 36 26 & 5503 & 4.48 & -0.03 & 0.19 & -4.87 & 4.0 & 2.9 & 2.6 & -21.8 & 52 & 0.02 & 0.02 & 1 \\
3737 & KOI-2984 & 19 58 49.7 & +43 37 21 & 6050 & 4.02 & 0.09 & 0.12 & -5.43 & 7.8 & 5.6 & 5.0 & -7.5 & 50 & 0.02 & 0.03 & 1 \\
3738 & KOI-1818 & 18 48 08.5 & +43 37 53 & 5492 & 4.56 & -0.05 & 0.30 & -4.60 & 4.0 & 2.9 & 2.6 & 14.0 & 50 & 0.02 & 0.02 & 1 \\
3739 & KOI-4257 & 19 40 32.0 & +43 37 53 & 5498 & 3.93 & -0.01 & 0.15 & -5.07 & 4.0 & 1.1 & 3.8 & 1.9 & 41 & 0.03 & 0.03 & 1 \\
3740 & KOI-686 & 19 47 21.8 & +43 38 50 & 5659 & 4.47 & -0.03 & 0.15 & -5.08 & 3.3 & 0.9 & 3.1 & -34.8 & 50 & 0.02 & 0.02 & 1 \\
3741 & KOI-3236 & 19 41 45.4 & +43 40 35 & 6312 & 4.26 & 0.12 & 0.12 & -5.30 & 16.1 & 12.4 & 7.4 & 9.9 & 46 & 0.02 & 0.03 & 1 \\
3742 & KOI-4109 & 19 48 19.9 & +43 40 48 & 4892 & 4.44 & 0.25 & 0.12 & -5.30 & 2.6 & 1.8 & 1.7 & -34.4 & 40 & 0.03 & 0.04 & 1 \\
3743 & KOI-4773 & 19 47 22.4 & +43 41 51 & 6152 & 3.90 & -0.19 & 0.09 & nan & 7.8 & 3.9 & 6.6 & -23.0 & 41 & 0.03 & 0.03 & 1 \\
3744 & KOI-687 & 19 48 28.1 & +43 42 41 & 5889 & 4.37 & 0.05 & 0.16 & -4.96 & 6.0 & 4.2 & 4.0 & -46.9 & 50 & 0.02 & 0.03 & 1 \\
3745 & KOI-459 & 19 49 06.9 & +43 43 26 & 5824 & 4.32 & 0.06 & 0.20 & -4.81 & 4.6 & 2.5 & 3.7 & -11.6 & 31 & 0.04 & 0.04 & 1 \\
3746 & KOI-92 & 18 53 30.0 & +43 47 18 & 5903 & 4.41 & 0.07 & 0.11 & -5.57 & 4.6 & 1.9 & 4.1 & -35.2 & 49 & 0.02 & 0.03 & 1 \\
3747 & KOI-3214 & 19 54 41.7 & +43 47 44 & 5889 & 4.01 & -0.09 & 0.12 & -5.41 & 6.4 & 4.7 & 4.0 & -15.3 & 49 & 0.03 & 0.03 & 1 \\
3748 & KOI-2674 & 19 18 36.3 & +43 49 28 & 5708 & 4.07 & 0.03 & 0.10 & -5.62 & 3.7 & 1.8 & 3.2 & -17.0 & 49 & 0.02 & 0.02 & 1 \\
3749 & KOI-2352 & 19 00 43.9 & +43 49 52 & 6410 & 4.14 & -0.10 & 0.10 & -6.02 & 9.1 & 3.0 & 8.6 & -5.6 & 47 & 0.02 & 0.03 & 1 \\
3750 & KOI-237 & 19 43 48.3 & +43 51 07 & 5755 & 4.44 & 0.23 & 0.13 & -5.27 & 4.3 & 2.6 & 3.4 & -23.6 & 39 & 0.03 & 0.04 & 1 \\
3751 & KOI-520 & 19 38 40.3 & +43 51 12 & 5026 & 4.51 & 0.08 & 0.37 & -4.62 & 2.5 & 1.6 & 1.8 & -5.7 & 35 & 0.04 & 0.08 & 1 \\
3752 & KOI-517 & 19 06 06.8 & +43 52 24 & 5400 & 4.47 & 0.15 & 0.28 & -4.67 & 3.9 & 3.1 & 2.4 & -16.4 & 39 & 0.04 & 0.04 & 1 \\
3753 & KOI-519 & 19 18 12.8 & +43 52 34 & 5787 & 4.28 & 0.04 & 0.12 & -5.35 & 4.2 & 2.1 & 3.5 & -30.0 & 29 & 0.04 & 0.05 & 1 \\
3754 & KOI-155 & 19 29 17.2 & +43 52 52 & 5821 & 4.31 & -0.14 & 0.12 & -5.38 & 3.2 & 0.1 & 3.7 & 4.1 & 48 & 0.02 & 0.03 & 1 \\
3755 & KOI-316 & 18 49 34.1 & +43 53 22 & 5547 & 4.27 & 0.27 & 0.10 & -5.62 & 3.2 & 1.6 & 2.7 & -28.8 & 51 & 0.02 & 0.02 & 1 \\
3756 & KOI-569 & 18 49 52.4 & +43 53 24 & 4956 & 4.54 & -0.18 & 0.55 & -4.46 & 2.2 & 1.2 & 1.8 & -49.0 & 32 & 0.04 & 0.04 & 1 \\
3757 & KOI-2743 & 19 24 06.9 & +43 54 49 & 5532 & 4.53 & -0.09 & 0.17 & -4.95 & 3.4 & 1.9 & 2.7 & -36.6 & 50 & 0.02 & 0.02 & 1 \\
3758 & KOI-3245 & 18 40 59.9 & +43 54 54 & 6069 & 4.23 & -0.08 & 0.15 & -5.07 & 5.5 & 1.9 & 5.1 & -18.9 & 50 & 0.03 & 0.03 & 1 \\
3759 & KOI-2486 & 18 42 45.7 & +43 55 09 & 6012 & 4.12 & 0.11 & 0.13 & -5.22 & 7.4 & 5.3 & 4.7 & -6.1 & 48 & 0.02 & 0.03 & 1 \\
3760 & KOI-2426 & 18 59 36.7 & +43 57 14 & 5319 & 4.42 & 0.02 & 0.13 & -5.23 & 2.4 & 0.4 & 2.2 & 17.9 & 51 & 0.02 & 0.03 & 1 \\
3761 & KOI-4343 & 19 12 18.4 & +43 57 31 & 5890 & 3.89 & -0.42 & 0.12 & -5.36 & 5.3 & 1.8 & 4.9 & -26.7 & 40 & 0.03 & 0.03 & 1 \\
3762 & KOI-1951 & 18 58 02.5 & +43 57 42 & 6051 & 4.19 & -0.15 & 0.12 & -5.33 & 6.5 & 3.9 & 5.0 & -42.1 & 48 & 0.02 & 0.03 & 1 \\
3763 & KOI-162 & 19 40 39.3 & +43 57 47 & 5811 & 4.32 & 0.19 & 0.10 & -5.91 & 4.7 & 2.8 & 3.6 & -22.7 & 50 & 0.02 & 0.02 & 1 \\
3764 & KOI-4656 & 19 40 58.1 & +43 58 21 & 6558 & 4.10 & 0.13 & 0.13 & -5.26 & 14.5 & 8.6 & 11.0 & 12.4 & 47 & 0.02 & 0.03 & 1 \\
3765 & KOI-4881 & 19 22 12.2 & +43 59 40 & 6211 & 4.16 & 0.03 & 0.14 & -5.14 & 11.4 & 8.6 & 6.3 & -22.8 & 46 & 0.03 & 0.03 & 1 \\
3766 & KOI-317 & 19 55 15.9 & +43 59 53 & 6372 & 3.87 & 0.04 & 0.14 & -5.11 & 19.5 & 14.8 & 9.5 & 9.4 & 48 & 0.02 & 0.03 & 1 \\
3767 & KOI-2073 & 19 24 58.3 & +44 00 31 & 4855 & 4.48 & 0.02 & 0.05 & -6.00 & 1.8 & 0.1 & 1.7 & 1.9 & 35 & 0.03 & 0.05 & 1 \\
3768 & KOI-1019 & 19 45 55.7 & +44 00 33 & 4934 & 3.45 & 0.13 & 0.09 & -5.46 & 3.6 & 0.9 & 3.4 & -22.2 & 53 & 0.02 & 0.03 & 1 \\
3769 & KOI-688 & 19 21 17.5 & +44 02 09 & 6208 & 4.22 & 0.03 & 0.11 & -5.54 & 10.8 & 8.1 & 6.3 & 17.7 & 48 & 0.12 & 0.04 & 1 \\
3770 & KOI-4634 & 20 02 35.9 & +44 03 21 & 6065 & 4.30 & 0.17 & 0.14 & -5.18 & 5.1 & 0.2 & 5.1 & -8.2 & 46 & 0.02 & 0.03 & 1 \\
3771 & KOI-3046 & 19 21 38.4 & +44 03 49 & 5631 & 4.29 & 0.20 & 0.09 & -5.88 & 3.9 & 2.5 & 3.0 & -37.1 & 50 & 0.02 & 0.02 & 1 \\
3772 & KOI-318 & 19 12 37.0 & +44 04 08 & 6326 & 4.17 & 0.31 & 0.17 & -4.88 & 16.4 & 12.6 & 7.6 & -6.1 & 47 & 0.03 & 0.03 & 1 \\
3773 & KOI-2781 & 19 56 13.7 & +44 04 30 & 5824 & 4.22 & -0.42 & 0.13 & -5.28 & 3.8 & 0.3 & 3.7 & -64.4 & 50 & 0.02 & 0.03 & 1 \\
3774 & KOI-2105 & 19 27 29.1 & +44 05 15 & 5919 & 4.46 & -0.03 & 0.15 & -5.05 & 4.8 & 2.2 & 4.2 & -6.6 & 45 & 0.03 & 0.03 & 1 \\
3775 & KOI-1985 & 18 43 42.3 & +44 05 17 & 4867 & 4.55 & -0.04 & 0.40 & -4.65 & 2.6 & 1.8 & 1.7 & -4.4 & 49 & 0.03 & 0.03 & 1 \\
3776 & KOI-572 & 19 59 11.2 & +44 05 22 & 6016 & 4.13 & -0.05 & 0.09 & nan & 5.9 & 3.2 & 4.8 & 3.5 & 48 & 0.03 & 0.03 & 1 \\
3777 & KOI-907 & 19 46 15.9 & +44 06 21 & 5552 & 4.55 & -0.11 & 0.14 & -5.19 & 3.2 & 1.4 & 2.7 & -5.6 & 25 & 0.05 & 0.05 & 1 \\
3778 & KOI-1809 & 19 37 48.9 & +44 08 45 & 5727 & 4.40 & 0.04 & 0.14 & -5.16 & 4.3 & 2.6 & 3.3 & -14.6 & 52 & 0.02 & 0.03 & 1 \\
3779 & KOI-1726 & 19 39 49.2 & +44 09 00 & 4710 & 4.42 & 0.07 & 0.52 & -4.60 & 2.5 & 1.8 & 1.6 & -43.1 & 54 & 0.03 & 0.03 & 1 \\
3780 & KOI-2593 & 18 47 20.5 & +44 09 21 & 6085 & 4.14 & 0.18 & 0.11 & -5.65 & 9.2 & 6.9 & 5.3 & -4.7 & 48 & 0.02 & 0.03 & 1 \\
3781 & KOI-4037 & 20 03 47.0 & +44 09 53 & 6253 & 4.40 & 0.01 & 0.12 & -5.47 & 9.3 & 6.0 & 6.7 & -7.9 & 49 & 0.02 & 0.06 & 1 \\
3782 & KOI-4426 & 19 37 48.1 & +44 10 00 & 6061 & 3.97 & 0.06 & 0.10 & -5.85 & 9.2 & 6.5 & 5.9 & -3.9 & 49 & 0.02 & 0.03 & 1 \\
3783 & KOI-4098 & 19 10 00.9 & +44 10 02 & 4929 & 4.49 & -0.12 & 0.28 & -4.79 & 3.4 & 2.8 & 1.7 & -6.7 & 47 & 0.03 & 0.03 & 1 \\
3784 & KOI-1069 & 19 10 22.4 & +44 10 46 & 5124 & 4.47 & 0.22 & 0.16 & -5.06 & 2.7 & 1.8 & 1.9 & -36.6 & 29 & 0.04 & 0.04 & 1 \\
3785 & KOI-3338 & 20 03 08.1 & +44 11 33 & 6099 & 4.21 & -0.17 & 0.14 & -5.12 & 5.1 & 0.1 & 5.4 & -2.6 & 49 & 0.16 & 0.07 & 1 \\
3786 & KOI-4834 & 19 27 10.7 & +44 11 37 & 4909 & 3.66 & 0.37 & 0.15 & -5.14 & 3.2 & 0.1 & 3.4 & 2.9 & 55 & 0.03 & 0.03 & 1 \\
3787 & KOI-4567 & 20 06 15.1 & +44 14 25 & 6461 & 4.28 & -0.03 & 0.12 & -5.32 & 12.5 & 7.6 & 9.4 & -14.3 & 49 & 0.02 & 0.03 & 1 \\
3788 & KOI-4435 & 18 47 49.4 & +44 15 42 & 6106 & 3.96 & 0.13 & 0.12 & -5.39 & 10.6 & 7.8 & 6.2 & -18.8 & 46 & 0.03 & 0.04 & 1 \\
3789 & KOI-1137 & 20 06 50.2 & +44 16 54 & 5542 & 4.68 & -0.25 & 0.14 & -5.12 & 4.5 & 3.4 & 2.7 & 7.6 & 38 & 0.04 & 0.05 & 2 \\
3790 & KOI-3301 & 19 30 31.1 & +44 17 00 & 5716 & 3.96 & 0.23 & 0.11 & -5.60 & 4.3 & 0.3 & 4.3 & -35.2 & 50 & 0.02 & 0.02 & 1 \\
3791 & Kepler-271 & 18 52 00.7 & +44 17 03 & 5515 & 4.50 & -0.21 & 0.00 & 0.00 & 3.5 & 2.0 & 2.6 & 11.5 & 75 & 0.06 & 0.03 & 1 \\
3792 & KOI-1150 & 18 47 03.9 & +44 17 33 & 5765 & 4.34 & 0.07 & 0.11 & -5.53 & 5.2 & 3.8 & 3.5 & -5.2 & 48 & 0.02 & 0.03 & 1 \\
3793 & KOI-1820 & 18 45 23.7 & +44 17 43 & 5268 & 4.47 & -0.01 & 0.27 & -4.72 & 3.7 & 3.0 & 2.1 & -26.0 & 50 & 0.02 & 0.06 & 1 \\
3794 & KOI-4399 & 18 48 30.9 & +44 18 11 & 5445 & 4.54 & -0.18 & 0.17 & -5.01 & 3.4 & 2.4 & 2.5 & -1.9 & 51 & 0.02 & 0.05 & 1 \\
3795 & KOI-574 & 19 10 15.5 & +44 18 18 & 5007 & 4.52 & -0.07 & 0.11 & -5.35 & 2.2 & 1.1 & 1.8 & -8.3 & 30 & 0.04 & 0.04 & 1 \\
3796 & KOI-4763 & 18 57 31.8 & +44 18 30 & 5680 & 3.99 & 0.14 & 0.11 & -5.51 & 4.9 & 2.4 & 4.2 & -18.7 & 43 & 0.03 & 0.03 & 1 \\
3797 & KOI-573 & 18 45 07.1 & +44 18 56 & 5648 & 4.41 & 0.07 & 0.13 & -5.21 & 3.8 & 2.1 & 3.0 & -8.4 & 36 & 0.04 & 0.04 & 1 \\
3798 & KOI-127 & 19 18 25.9 & +44 20 44 & 5492 & 4.36 & 0.26 & 0.16 & -5.04 & 3.4 & 2.1 & 2.6 & -27.0 & 47 & 0.03 & 0.03 & 1 \\
3799 & KOI-4407 & 20 04 37.6 & +44 22 46 & 6517 & 4.21 & -0.09 & 0.14 & -5.14 & 9.5 & 0.1 & 10.3 & 4.9 & 49 & 0.02 & 0.03 & 1 \\
3800 & Kepler-79 & 20 02 04.1 & +44 22 54 & 6177 & 4.13 & -0.01 & 0.11 & -4.90 & 16.9 & 13.9 & 6.0 & -26.7 & 50 & 0.15 & 0.06 & 2 \\
3801 & KOI-152 & 20 02 04.1 & +44 22 54 & 6313 & 4.21 & 0.08 & 0.12 & -5.30 & 17.0 & 13.4 & 7.4 & -26.6 & 49 & 0.02 & 0.03 & 1 \\
3802 & KOI-689 & 19 21 53.1 & +44 23 14 & 5417 & 4.59 & -0.48 & 0.18 & -4.93 & 2.2 & 0.1 & 2.4 & -95.6 & 50 & 0.03 & 0.02 & 1 \\
3803 & KOI-2730 & 18 58 42.1 & +44 25 04 & 5655 & 4.30 & -0.03 & 0.08 & nan & 3.7 & 2.0 & 3.0 & -60.3 & 50 & 0.02 & 0.03 & 1 \\
3804 & KOI-4693 & 19 02 48.8 & +44 25 19 & 5795 & 4.33 & -0.23 & 0.13 & -5.26 & 3.4 & 0.1 & 3.6 & -18.5 & 47 & 0.03 & 0.03 & 1 \\
3805 & KOI-1148 & 18 48 48.0 & +44 25 20 & 6048 & 4.26 & 0.15 & 0.12 & -5.38 & 7.0 & 4.6 & 5.0 & -41.1 & 49 & 0.02 & 0.03 & 1 \\
3806 & KOI-102 & 19 58 49.2 & +44 26 09 & 5730 & 4.37 & 0.17 & 0.13 & nan & 3.8 & 1.7 & 3.3 & -19.8 & 64 & 0.02 & 0.02 & 2 \\
3807 & KOI-4603 & 19 26 09.4 & +44 26 49 & 6071 & 4.08 & 0.17 & 0.12 & -5.33 & 9.8 & 7.6 & 5.2 & 26.7 & 39 & 0.03 & 0.03 & 1 \\
3808 & TYC 2810-1660-1 & 00 56 55.8 & +44 27 20 & 5766 & 4.60 & -0.06 & 0.33 & -4.48 & 7.6 & 6.3 & 3.5 & 4.8 & 177 & 0.02 & 0.03 & 1 \\
3809 & BD+43183 & 00 56 53.5 & +44 27 52 & 6172 & 4.36 & 0.03 & 0.26 & -4.54 & 16.4 & 13.2 & 6.0 & -0.3 & 170 & 0.02 & 0.01 & 1 \\
3810 & KOI-3497 & 19 17 05.9 & +44 28 13 & 4712 & 4.42 & 0.02 & 1.01 & -4.30 & 4.6 & 4.2 & 1.6 & -19.7 & 56 & 0.03 & 0.03 & 1 \\
3811 & KOI-3251 & 18 56 02.7 & +44 29 40 & 5909 & 4.25 & 0.07 & 0.10 & -5.75 & 5.2 & 3.0 & 4.1 & 14.7 & 50 & 0.02 & 0.06 & 1 \\
3812 & KOI-370 & 19 25 33.1 & +44 31 45 & 5973 & 3.94 & -0.04 & 0.11 & -5.64 & 7.4 & 5.0 & 5.3 & -28.0 & 48 & 0.02 & 0.10 & 1 \\
3813 & KOI-2389 & 19 26 19.0 & +44 31 54 & 5840 & 4.07 & -0.09 & 0.11 & -5.49 & 4.3 & 1.9 & 3.8 & -8.3 & 49 & 0.03 & 0.03 & 1 \\
3814 & KOI-4505 & 19 24 23.9 & +44 32 45 & 6101 & 4.21 & -0.08 & 0.12 & -5.37 & 7.3 & 4.7 & 5.4 & -25.2 & 41 & 0.03 & 0.03 & 1 \\
3815 & KOI-2016 & 19 22 24.3 & +44 33 23 & 5902 & 4.28 & 0.40 & 0.11 & -5.59 & 5.6 & 3.7 & 4.1 & -7.4 & 47 & 0.19 & 0.10 & 1 \\
3816 & KOI-691 & 18 59 09.2 & +44 35 30 & 5970 & 4.17 & -0.29 & 0.10 & -5.92 & 4.6 & 0.7 & 4.5 & -33.0 & 45 & 0.03 & 0.03 & 1 \\
3817 & KOI-3315 & 19 19 19.5 & +44 36 36 & 5734 & 4.71 & -0.43 & 0.18 & -4.89 & 2.6 & 0.1 & 3.3 & -96.3 & 49 & 0.02 & 0.04 & 1 \\
3818 & KOI-2022 & 19 34 42.4 & +44 36 56 & 5734 & 4.51 & 0.08 & 0.36 & -4.43 & 7.6 & 6.4 & 3.3 & -23.9 & 42 & 0.03 & 0.07 & 1 \\
3819 & KOI-3111 & 19 54 18.4 & +44 37 18 & 5915 & 4.34 & -0.08 & 0.13 & -5.23 & 4.7 & 2.0 & 4.2 & -19.3 & 49 & 0.02 & 0.02 & 1 \\
3820 & KOI-1792 & 19 15 53.2 & +44 37 28 & 5484 & 4.08 & -0.07 & 0.10 & -5.58 & 5.0 & 4.0 & 2.6 & -27.1 & 54 & 0.02 & 0.03 & 1 \\
3821 & KOI-3890 & 19 35 05.3 & +44 38 19 & 4760 & 3.15 & -0.04 & 0.12 & -5.28 & 3.4 & 0.1 & 3.4 & -26.5 & 54 & 0.02 & 0.03 & 1 \\
3822 & KOI-692 & 19 23 17.8 & +44 38 50 & 5623 & 4.28 & 0.09 & 0.09 & -6.00 & 3.8 & 2.2 & 2.9 & -78.4 & 50 & 0.02 & 0.03 & 1 \\
3823 & KOI-1270 & 19 34 33.9 & +44 39 25 & 5133 & 4.46 & 0.02 & 0.25 & -4.79 & 2.7 & 1.8 & 1.9 & -21.6 & 42 & 0.03 & 0.03 & 1 \\
3824 & KOI-2969 & 19 28 28.7 & +44 39 29 & 5877 & 3.92 & 0.16 & 0.13 & -5.25 & 6.8 & 4.6 & 4.8 & 3.5 & 50 & 0.25 & 0.08 & 1 \\
3825 & KOI-2488 & 19 25 53.8 & +44 41 01 & 5951 & 4.14 & -0.05 & 0.12 & -5.34 & 6.2 & 4.1 & 4.4 & 15.1 & 47 & 0.02 & 0.03 & 1 \\
3826 & KOI-139 & 19 26 36.8 & +44 41 18 & 5869 & 4.30 & 0.19 & 0.09 & nan & 4.6 & 2.3 & 3.9 & -19.8 & 49 & 0.02 & 0.03 & 1 \\
3827 & KOI-1275 & 19 56 53.2 & +44 41 38 & 5839 & 4.29 & 0.00 & 0.07 & nan & 4.6 & 2.4 & 3.8 & -26.8 & 44 & 0.03 & 0.03 & 1 \\
3828 & KOI-981 & 18 54 56.7 & +44 42 48 & 4969 & 3.18 & -0.16 & 0.13 & -5.21 & 3.4 & 0.3 & 3.4 & -34.1 & 78 & 0.02 & 0.02 & 2 \\
3829 & KOI-3946 & 19 43 54.1 & +44 42 48 & 6400 & 4.10 & -0.14 & 0.11 & -5.62 & 9.0 & 2.9 & 8.5 & -12.6 & 48 & 0.02 & 0.03 & 1 \\
3830 & KOI-4580 & 19 33 29.7 & +44 43 41 & 5906 & 4.13 & -0.23 & 0.15 & -5.03 & 4.2 & 0.7 & 4.1 & -55.8 & 49 & 0.02 & 0.03 & 1 \\
3831 & KOI-579 & 19 14 20.2 & +44 44 02 & 5083 & 4.58 & 0.01 & 0.37 & -4.60 & 2.6 & 1.6 & 1.9 & -43.0 & 47 & 0.03 & 0.04 & 1 \\
3832 & KOI-2503 & 19 37 33.9 & +44 45 47 & 4797 & 4.48 & 0.13 & 0.14 & -5.19 & 2.0 & 0.8 & 1.6 & -14.1 & 54 & 0.03 & 0.03 & 1 \\
3833 & KOI-1754 & 19 59 49.7 & +44 46 19 & 6194 & 4.33 & 0.01 & 0.14 & -5.08 & 8.7 & 5.7 & 6.2 & -11.7 & 50 & 0.02 & 0.03 & 1 \\
3834 & KOI-2111 & 19 05 08.3 & +44 46 54 & 5520 & 4.52 & 0.05 & 0.28 & -4.62 & 5.0 & 4.1 & 2.7 & -18.9 & 35 & 0.03 & 0.03 & 1 \\
3835 & KOI-4775 & 19 29 36.8 & +44 46 55 & 5093 & 3.73 & 0.41 & 0.11 & -5.35 & 3.3 & 0.1 & 3.5 & -88.3 & 55 & 0.02 & 0.03 & 1 \\
3836 & KOI-2414 & 19 04 06.3 & +44 46 58 & 5632 & 4.18 & -0.30 & 0.09 & -6.14 & 3.5 & 1.6 & 3.0 & -39.5 & 48 & 0.02 & 0.02 & 1 \\
3837 & KOI-1279 & 19 33 29.4 & +44 47 06 & 5741 & 4.39 & -0.07 & 0.04 & nan & 3.4 & 0.1 & 3.4 & -14.6 & 48 & 0.02 & 0.02 & 1 \\
3838 & KOI-1271 & 19 37 03.7 & +44 47 39 & 6326 & 4.11 & -0.21 & 0.12 & -5.46 & 9.0 & 4.6 & 7.6 & 4.2 & 48 & 0.02 & 0.03 & 1 \\
3839 & KOI-1278 & 18 58 42.6 & +44 47 52 & 5848 & 4.55 & -0.19 & 0.16 & -4.98 & 3.2 & 0.1 & 3.8 & -1.3 & 27 & 0.05 & 0.05 & 1 \\
3840 & Kepler-282 & 18 58 42.6 & +44 47 52 & 5787 & 4.52 & -0.21 & 0.00 & 0.00 & 3.6 & 0.1 & 3.5 & 0.6 & 38 & 0.05 & 0.05 & 1 \\
3841 & KOI-1891 & 19 13 47.4 & +44 48 06 & 4940 & 4.49 & 0.11 & 0.20 & -4.96 & 1.6 & 0.1 & 1.7 & -8.2 & 37 & 0.03 & 0.04 & 1 \\
3842 & KOI-4066 & 19 22 55.2 & +44 50 10 & 6213 & 4.13 & 0.08 & 0.13 & -5.25 & 15.2 & 12.1 & 6.3 & -25.0 & 48 & 0.02 & 0.03 & 1 \\
3843 & KOI-2758 & 19 46 53.7 & +44 51 11 & 5093 & 3.61 & 0.28 & 0.36 & -4.61 & 4.5 & 2.7 & 3.5 & -61.8 & 53 & 0.02 & 0.03 & 1 \\
3844 & KOI-1283 & 19 44 01.7 & +44 51 12 & 5864 & 4.26 & -0.22 & 0.29 & -4.53 & 3.4 & 0.1 & 3.9 & -66.8 & 50 & 0.02 & 0.02 & 1 \\
3845 & KOI-105 & 19 55 44.9 & +44 51 28 & 5754 & 4.62 & -0.32 & 0.21 & nan & 2.5 & 0.1 & 3.4 & -58.6 & 60 & 0.02 & 0.02 & 2 \\
3846 & KOI-921 & 19 27 22.1 & +44 51 29 & 5004 & 4.51 & 0.10 & 0.57 & -4.42 & 1.2 & 0.1 & 1.8 & -58.7 & 37 & 0.03 & 0.04 & 1 \\
3847 & KOI-172 & 19 33 02.6 & +44 52 08 & 5815 & 4.54 & -0.18 & 0.12 & -5.45 & 3.2 & 0.1 & 3.7 & -40.4 & 49 & 0.02 & 0.05 & 1 \\
3848 & KOI-319 & 19 20 28.2 & +44 52 23 & 5898 & 3.96 & 0.12 & 0.12 & -5.34 & 6.6 & 4.2 & 4.9 & -9.6 & 49 & 0.02 & 0.03 & 1 \\
3849 & KOI-374 & 19 22 30.1 & +44 52 26 & 5938 & 4.44 & -0.16 & 0.14 & -5.18 & 3.5 & 0.1 & 4.3 & 2.6 & 48 & 0.02 & 0.02 & 1 \\
3850 & KOI-1629 & 19 21 38.9 & +44 53 58 & 5791 & 4.24 & 0.24 & 0.10 & -6.05 & 4.7 & 2.9 & 3.6 & -29.4 & 49 & 0.02 & 0.02 & 1 \\
3851 & KOI-2749 & 19 24 00.7 & +44 53 58 & 6106 & 3.82 & -0.01 & 0.13 & -5.28 & 11.6 & 8.8 & 6.2 & -29.8 & 47 & 0.03 & 0.03 & 1 \\
3852 & KOI-2473 & 19 27 50.4 & +44 54 00 & 5000 & 4.55 & -0.10 & 0.29 & -4.76 & 2.3 & 1.3 & 1.8 & -57.5 & 31 & 0.23 & 0.06 & 1 \\
3853 & KOI-3891 & 19 44 37.4 & +44 55 12 & 5076 & 3.77 & -0.05 & 0.12 & -5.28 & 3.4 & 0.1 & 3.5 & -43.7 & 52 & 0.07 & 0.03 & 1 \\
3854 & KOI-4301 & 19 52 48.6 & +44 55 33 & 6028 & 4.18 & -0.22 & 0.08 & nan & 7.1 & 4.9 & 4.9 & -41.6 & 40 & 0.03 & 0.04 & 1 \\
3855 & KOI-1257 & 19 24 54.1 & +44 55 39 & 5314 & 4.10 & 0.15 & 0.15 & -5.11 & 4.4 & 3.7 & 2.2 & 6.6 & 32 & 0.04 & 0.05 & 1 \\
3856 & KOI-2017 & 19 21 56.8 & +44 55 57 & 5624 & 4.55 & -0.07 & 0.30 & -4.56 & 5.1 & 4.0 & 2.9 & -7.0 & 48 & 0.02 & 0.02 & 1 \\
3857 & KOI-1904 & 19 46 11.4 & +44 56 31 & 5003 & 4.54 & -0.04 & 0.29 & -4.75 & 3.1 & 2.4 & 1.8 & 8.2 & 43 & 0.03 & 0.03 & 1 \\
3858 & KOI-4251 & 19 05 24.8 & +44 57 40 & 5505 & 4.53 & -0.04 & 0.27 & -4.66 & 3.4 & 2.1 & 2.6 & -0.8 & 50 & 0.02 & 0.03 & 1 \\
3859 & KOI-2159 & 19 00 33.2 & +45 00 16 & 5719 & 4.41 & 0.05 & 0.14 & -5.15 & 4.1 & 2.4 & 3.3 & -36.0 & 45 & 0.03 & 0.03 & 1 \\
3860 & KOI-694 & 18 55 35.9 & +45 01 01 & 5642 & 4.43 & 0.13 & 0.15 & -5.09 & 3.7 & 1.9 & 3.0 & -22.5 & 47 & 0.02 & 0.03 & 1 \\
3861 & KOI-2039 & 19 01 33.0 & +45 02 57 & 5478 & 4.56 & 0.16 & 0.20 & -4.87 & 3.6 & 2.4 & 2.5 & -42.1 & 34 & 0.03 & 0.03 & 1 \\
3862 & KOI-1850 & 19 38 27.1 & +45 03 37 & 5865 & 4.24 & 0.01 & 0.14 & -5.15 & 4.7 & 2.5 & 3.9 & 0.4 & 46 & 0.02 & 0.05 & 1 \\
3863 & KOI-1276 & 19 00 08.7 & +45 04 16 & 5526 & 4.52 & 0.08 & 0.11 & -5.45 & 3.2 & 1.5 & 2.7 & -27.3 & 37 & 0.03 & 0.09 & 1 \\
3864 & KOI-695 & 19 02 37.4 & +45 04 46 & 5827 & 4.54 & -0.39 & 0.14 & -5.19 & 2.9 & 0.1 & 3.7 & -8.9 & 48 & 0.03 & 0.03 & 1 \\
3865 & KOI-3052 & 19 40 21.7 & +45 04 52 & 5345 & 4.55 & -0.22 & 0.21 & -4.84 & 4.3 & 3.6 & 2.3 & -14.5 & 49 & 0.02 & 0.02 & 1 \\
3866 & KOI-2956 & 18 53 48.8 & +45 05 03 & 6392 & 3.97 & 0.03 & 0.12 & -5.28 & 11.7 & 6.1 & 9.8 & 16.0 & 48 & 0.04 & 0.03 & 1 \\
3867 & KOI-3886 & 20 04 11.4 & +45 05 15 & 4711 & 2.83 & 0.25 & 0.17 & -5.13 & 6.2 & 4.3 & 4.0 & -24.1 & 59 & 0.03 & 0.04 & 1 \\
3868 & KOI-1274 & 18 53 01.6 & +45 05 16 & 5234 & 4.54 & -0.24 & 0.13 & -5.22 & 2.9 & 1.9 & 2.1 & -27.8 & 50 & 0.03 & 0.02 & 1 \\
3869 & KOI-4811 & 19 15 25.8 & +45 05 52 & 5589 & 3.98 & 0.04 & 0.12 & -5.30 & 4.0 & 0.2 & 4.0 & 0.7 & 46 & 0.16 & 0.04 & 1 \\
3870 & KOI-2659 & 18 59 11.3 & +45 05 57 & 4930 & 3.44 & 0.19 & 0.11 & -5.33 & 3.2 & 0.1 & 3.4 & 0.6 & 53 & 0.02 & 0.03 & 1 \\
3871 & KOI-464 & 19 34 59.3 & +45 06 26 & 5378 & 4.43 & 0.16 & 0.26 & -4.70 & 3.2 & 2.1 & 2.3 & -21.3 & 30 & 0.04 & 0.04 & 1 \\
3872 & KOI-3541 & 18 57 01.7 & +45 07 07 & 6139 & 3.91 & -0.21 & 0.11 & -5.54 & 8.5 & 5.1 & 6.5 & -13.0 & 48 & 0.02 & 0.03 & 1 \\
3873 & KOI-2641 & 19 39 59.0 & +45 07 10 & 5812 & 4.13 & -0.01 & 0.21 & -4.75 & 4.6 & 2.7 & 3.7 & -34.4 & 50 & 0.02 & 0.03 & 1 \\
3874 & KOI-465 & 19 35 42.8 & +45 08 33 & 6052 & 4.25 & 0.06 & 0.15 & nan & 6.0 & 3.1 & 5.0 & -27.4 & 37 & 0.05 & 0.05 & 2 \\
3875 & KOI-697 & 19 16 00.2 & +45 09 15 & 5796 & 4.18 & 0.09 & 0.25 & -4.65 & 3.9 & 1.5 & 3.6 & -63.4 & 48 & 0.02 & 0.03 & 1 \\
3876 & KOI-4269 & 19 35 11.3 & +45 09 39 & 4934 & 3.56 & 0.07 & 0.09 & -5.47 & 2.9 & 0.1 & 3.4 & -21.0 & 54 & 0.02 & 0.03 & 1 \\
3877 & WASP-58 & 18 18 48.3 & +45 10 19 & 5918 & 4.31 & -0.21 & 0.00 & 0.00 & 4.3 & 0.8 & 4.2 & -27.7 & 110 & 0.01 & 0.01 & 1 \\
3878 & KOI-3473 & 19 52 18.2 & +45 11 20 & 5054 & 4.51 & -0.06 & 0.43 & -4.54 & 5.8 & 5.3 & 1.9 & -19.6 & 44 & 0.03 & 0.08 & 1 \\
3879 & KOI-698 & 19 35 39.3 & +45 11 23 & 6195 & 4.24 & 0.04 & 0.11 & -5.73 & 10.9 & 8.1 & 6.2 & -34.2 & 47 & 0.03 & 0.03 & 1 \\
3880 & KOI-2595 & 19 23 58.9 & +45 11 32 & 6285 & 4.23 & 0.03 & 0.13 & -5.19 & 17.1 & 13.7 & 7.1 & -23.0 & 46 & 0.03 & 0.03 & 1 \\
3881 & KOI-2517 & 19 19 32.3 & +45 12 41 & 5569 & 4.59 & -0.20 & 0.17 & -4.98 & 3.2 & 1.3 & 2.8 & 8.1 & 35 & 0.03 & 0.03 & 1 \\
3882 & KOI-700 & 19 39 53.6 & +45 12 49 & 5779 & 4.57 & -0.45 & 0.12 & -5.41 & 3.4 & 0.1 & 3.5 & 15.9 & 47 & 0.02 & 0.03 & 1 \\
3883 & Kepler-215 & 19 39 53.6 & +45 12 49 & 5768 & 4.59 & -0.48 & 0.14 & -5.16 & 3.5 & 0.1 & 3.5 & 15.8 & 65 & 0.04 & 0.04 & 1 \\
3884 & KOI-1412 & 19 24 17.9 & +45 14 33 & 5925 & 4.13 & 0.14 & 0.12 & -5.44 & 5.3 & 3.1 & 4.2 & 13.7 & 48 & 0.02 & 0.02 & 1 \\
3885 & KOI-159 & 19 50 50.8 & +45 15 43 & 5993 & 4.35 & -0.03 & 0.16 & -5.00 & 5.4 & 2.6 & 4.6 & -56.8 & 48 & 0.02 & 0.03 & 1 \\
3886 & KOI-2038 & 19 23 53.6 & +45 17 25 & 5421 & 4.56 & 0.03 & 0.14 & -5.15 & 3.6 & 2.6 & 2.4 & -16.3 & 25 & 0.05 & 0.05 & 1 \\
3887 & KOI-3227 & 19 53 36.7 & +45 17 50 & 5950 & 4.36 & 0.02 & 0.10 & -5.97 & 4.8 & 1.9 & 4.4 & -6.6 & 47 & 0.02 & 0.03 & 1 \\
3888 & KOI-4585 & 19 06 10.5 & +45 18 18 & 6076 & 3.93 & -0.12 & 0.12 & -5.39 & 11.7 & 8.9 & 6.0 & 23.0 & 46 & 0.02 & 0.03 & 1 \\
3889 & KOI-582 & 19 24 44.0 & +45 19 23 & 5068 & 4.50 & 0.03 & 0.60 & -4.37 & 2.9 & 2.1 & 1.9 & 5.0 & 37 & 0.03 & 0.03 & 1 \\
3890 & KOI-2319 & 18 55 01.2 & +45 20 07 & 6036 & 4.24 & -0.04 & 0.11 & -5.59 & 6.4 & 3.8 & 4.9 & -7.3 & 45 & 0.02 & 0.03 & 1 \\
3891 & KOI-3196 & 18 53 24.1 & +45 20 21 & 6098 & 4.26 & -0.01 & 0.14 & -5.14 & 5.3 & 0.1 & 5.4 & -20.2 & 83 & 0.02 & 0.02 & 1 \\
3892 & KOI-2530 & 19 11 13.3 & +45 20 26 & 5866 & 4.00 & 0.09 & 0.13 & -5.24 & 5.9 & 3.3 & 4.8 & -29.4 & 48 & 0.02 & 0.03 & 1 \\
3893 & KOI-2768 & 19 05 35.7 & +45 20 37 & 5254 & 4.53 & -0.15 & 0.29 & -4.69 & 2.5 & 1.1 & 2.1 & -30.5 & 35 & 0.03 & 0.03 & 1 \\
3894 & KOI-4014 & 19 07 47.9 & +45 21 14 & 5939 & 4.37 & 0.07 & 0.15 & -5.08 & 5.0 & 2.5 & 4.3 & 10.9 & 42 & 0.03 & 0.06 & 1 \\
3895 & KOI-134 & 19 42 20.8 & +45 21 54 & 6143 & 4.03 & 0.32 & 0.13 & -5.24 & 13.5 & 10.8 & 5.7 & -22.3 & 43 & 0.03 & 0.03 & 1 \\
3896 & KOI-1413 & 19 01 23.0 & +45 22 04 & 5291 & 3.82 & -0.04 & 0.12 & -5.30 & 3.6 & 0.1 & 3.6 & -34.2 & 36 & 0.03 & 0.03 & 1 \\
3897 & KOI-1616 & 19 18 01.5 & +45 22 16 & 6043 & 4.34 & 0.17 & 0.14 & -5.16 & 6.6 & 4.2 & 5.0 & -29.5 & 50 & 0.02 & 0.03 & 1 \\
3898 & KOI-2564 & 19 34 17.8 & +45 23 04 & 6120 & 4.06 & -0.10 & 0.11 & -5.65 & 10.9 & 8.5 & 5.5 & -17.1 & 48 & 0.03 & 0.03 & 1 \\
3899 & KOI-2175 & 19 27 31.2 & +45 23 17 & 5416 & 3.90 & 0.05 & 0.17 & -4.98 & 4.1 & 1.5 & 3.7 & -2.5 & 51 & 0.02 & 0.02 & 1 \\
3900 & KOI-2833 & 19 52 51.7 & +45 24 25 & 6189 & 4.29 & -0.19 & 0.10 & -6.64 & 6.6 & 2.5 & 6.1 & 8.5 & 46 & 0.03 & 0.03 & 1 \\
3901 & KOI-2367 & 19 23 29.1 & +45 24 37 & 6068 & 4.13 & 0.20 & 0.12 & -5.41 & 7.9 & 5.6 & 5.1 & -13.6 & 48 & 0.02 & 0.03 & 1 \\
3902 & KOI-2470 & 19 51 08.8 & +45 25 03 & 5801 & 4.28 & 0.25 & 0.11 & -5.46 & 4.5 & 2.6 & 3.6 & -11.6 & 50 & 0.02 & 0.02 & 1 \\
3903 & KOI-3008 & 18 50 48.0 & +45 25 33 & 6005 & 4.07 & -0.07 & 0.12 & -5.45 & 6.8 & 4.7 & 4.7 & -30.5 & 48 & 0.02 & 0.03 & 1 \\
3904 & KOI-2640 & 19 27 14.4 & +45 26 08 & 4837 & 2.97 & -0.13 & 0.27 & -4.85 & 3.9 & 0.1 & 4.0 & -66.1 & 52 & 0.02 & 0.03 & 1 \\
3905 & KOI-4060 & 19 23 20.1 & +45 26 08 & 5798 & 4.21 & 0.14 & 0.17 & -4.93 & 4.5 & 2.6 & 3.6 & -68.4 & 39 & 0.03 & 0.03 & 1 \\
3906 & KOI-3249 & 19 19 02.5 & +45 27 20 & 6031 & 4.36 & 0.05 & 0.14 & -5.10 & 5.6 & 2.6 & 4.9 & -21.7 & 50 & 0.04 & 0.04 & 1 \\
3907 & HAT-P-40 & 22 22 03.1 & +45 27 27 & 6054 & 3.92 & 0.18 & 0.00 & 0.00 & 9.2 & 6.5 & 5.8 & -27.4 & 112 & 0.01 & 0.02 & 1 \\
3908 & KOI-4839 & 19 53 38.3 & +45 27 42 & 6145 & 4.15 & -0.06 & 0.09 & nan & 5.2 & 0.1 & 5.7 & -30.5 & 49 & 0.02 & 0.03 & 1 \\
3909 & KOI-4198 & 18 55 24.7 & +45 29 07 & 6146 & 3.89 & -0.34 & 0.09 & nan & 7.4 & 3.1 & 6.6 & -22.0 & 49 & 0.06 & 0.04 & 1 \\
3910 & KOI-3087 & 20 03 45.0 & +45 29 24 & 5206 & 4.47 & 0.20 & 0.22 & -4.84 & 2.4 & 1.2 & 2.0 & -18.2 & 53 & 0.02 & 0.02 & 1 \\
3911 & KOI-3425 & 20 01 15.9 & +45 29 43 & 6030 & 3.82 & -0.01 & 0.12 & -5.31 & 8.1 & 5.5 & 5.7 & -34.1 & 49 & 0.02 & 0.03 & 1 \\
3912 & KOI-2874 & 19 19 26.1 & +45 30 14 & 5244 & 4.54 & -0.11 & 0.20 & -4.90 & 2.7 & 1.6 & 2.1 & -28.3 & 35 & 0.03 & 0.03 & 1 \\
3913 & KOI-323 & 18 56 14.7 & +45 30 25 & 5397 & 4.54 & -0.04 & 0.40 & -4.46 & 5.7 & 4.9 & 2.4 & 6.6 & 50 & 0.02 & 0.02 & 1 \\
3914 & KOI-703 & 19 39 38.9 & +45 34 00 & 6236 & 3.99 & 0.26 & 0.12 & -5.42 & 9.5 & 5.4 & 7.5 & -16.9 & 48 & 0.02 & 0.03 & 1 \\
3915 & KOI-2522 & 19 57 31.6 & +45 35 32 & 4843 & 4.47 & 0.20 & 0.37 & -4.69 & 2.3 & 1.5 & 1.7 & -24.1 & 54 & 0.03 & 0.04 & 1 \\
3916 & KOI-584 & 19 11 40.3 & +45 35 34 & 5425 & 4.33 & 0.22 & 0.07 & nan & 3.2 & 2.0 & 2.4 & -11.3 & 47 & 0.03 & 0.03 & 1 \\
3917 & Kepler-192 & 19 11 40.3 & +45 35 34 & 5448 & 4.39 & 0.20 & 0.00 & 0.00 & 3.6 & 2.5 & 2.5 & -9.7 & 63 & 0.03 & 0.05 & 1 \\
3918 & KOI-4222 & 20 03 44.5 & +45 35 48 & 5612 & 4.57 & -0.11 & 0.26 & -4.66 & 4.3 & 3.0 & 2.9 & -4.6 & 45 & 0.03 & 0.09 & 1 \\
3919 & KOI-2443 & 19 11 11.6 & +45 39 24 & 5904 & 4.38 & -0.27 & 0.14 & -5.15 & 3.8 & 0.1 & 4.1 & -25.1 & 45 & 0.02 & 0.03 & 1 \\
3920 & KOI-2281 & 19 32 31.5 & +45 39 49 & 4992 & 4.53 & 0.12 & 0.26 & -4.82 & 2.4 & 1.4 & 1.8 & 1.2 & 54 & 0.02 & 0.06 & 1 \\
3921 & KOI-2162 & 19 02 46.1 & +45 41 22 & 5809 & 4.67 & -0.40 & 0.19 & -4.85 & 3.5 & 0.1 & 3.6 & -65.4 & 48 & 0.02 & 0.03 & 1 \\
3922 & KOI-4318 & 19 35 45.2 & +45 43 08 & 6367 & 4.19 & -0.04 & 0.16 & -4.94 & 22.0 & 17.7 & 8.1 & -10.5 & 48 & 0.06 & 0.03 & 1 \\
3923 & KOI-704 & 18 57 32.7 & +45 43 11 & 5233 & 4.52 & -0.16 & 0.28 & -4.70 & 2.9 & 1.9 & 2.1 & -30.1 & 50 & 0.02 & 0.02 & 1 \\
3924 & KOI-2657 & 19 31 02.8 & +45 43 38 & 5449 & 4.52 & -0.22 & 0.10 & -5.59 & 2.7 & 0.6 & 2.5 & -39.2 & 50 & 0.02 & 0.02 & 1 \\
3925 & KOI-3114 & 19 38 52.0 & +45 46 52 & 6103 & 3.92 & 0.19 & 0.10 & -6.31 & 10.6 & 7.9 & 6.2 & -21.4 & 47 & 0.03 & 0.03 & 1 \\
3926 & KOI-3867 & 19 44 13.0 & +45 49 37 & 5519 & 4.52 & 0.06 & 0.13 & -5.26 & 3.2 & 1.7 & 2.6 & -32.0 & 30 & 0.04 & 0.04 & 1 \\
3927 & KOI-4215 & 19 59 26.8 & +45 49 38 & 5483 & 4.16 & -0.25 & 0.09 & -5.85 & 3.5 & 2.1 & 2.6 & -73.9 & 39 & 0.03 & 0.03 & 1 \\
3928 & KOI-2137 & 19 56 56.9 & +45 50 05 & 5250 & 4.58 & -0.19 & 0.18 & -4.96 & 2.6 & 1.4 & 2.1 & -7.5 & 45 & 0.03 & 0.04 & 1 \\
3929 & KOI-1411 & 19 55 58.8 & +45 54 34 & 5582 & 4.24 & 0.25 & 0.35 & -4.48 & 4.1 & 2.9 & 2.8 & -63.8 & 51 & 0.02 & 0.02 & 1 \\
3930 & KOI-4640 & 19 40 42.1 & +45 55 51 & 6428 & 4.11 & 0.01 & 0.12 & -5.44 & 13.4 & 9.0 & 8.9 & -24.2 & 48 & 0.02 & 0.03 & 1 \\
3931 & KOI-1922 & 19 38 27.3 & +45 59 05 & 5730 & 4.37 & -0.03 & 0.13 & -5.26 & 4.1 & 2.2 & 3.3 & -4.5 & 30 & 0.05 & 0.05 & 1 \\
3932 & KOI-974 & 19 43 12.7 & +45 59 17 & 6217 & 3.91 & -0.02 & 0.12 & -5.44 & 9.8 & 6.0 & 7.3 & -21.6 & 47 & 0.02 & 0.03 & 1 \\
3933 & KOI-1835 & 19 37 18.1 & +46 00 08 & 5079 & 4.55 & 0.10 & 0.38 & -4.59 & 5.0 & 4.6 & 1.9 & -18.4 & 54 & 0.02 & 0.03 & 1 \\
3934 & KOI-707 & 19 16 18.6 & +46 00 19 & 5900 & 4.02 & 0.09 & 0.11 & -5.62 & 5.7 & 3.8 & 4.1 & 13.4 & 48 & 0.03 & 0.03 & 1 \\
3935 & Kepler-33 & 19 16 18.6 & +46 00 19 & 5910 & 4.04 & 0.10 & 0.00 & 0.00 & 6.2 & 4.4 & 4.1 & 12.3 & 60 & 0.06 & 0.04 & 1 \\
3936 & KOI-2079 & 19 39 54.9 & +46 00 20 & 5353 & 4.33 & 0.28 & 0.15 & -5.07 & 3.0 & 1.8 & 2.3 & -49.0 & 51 & 0.02 & 0.02 & 1 \\
3937 & KOI-2786 & 19 29 54.7 & +46 01 22 & 6394 & 4.14 & -0.10 & 0.12 & -5.44 & 9.1 & 3.5 & 8.4 & -12.1 & 47 & 0.02 & 0.03 & 1 \\
3938 & KOI-941 & 19 49 15.8 & +46 01 24 & 5058 & 4.50 & 0.34 & 0.38 & -4.61 & 2.7 & 1.9 & 1.9 & -5.8 & 25 & 0.06 & 0.06 & 1 \\
3939 & Kepler-127 & 19 00 45.6 & +46 01 41 & 6080 & 4.21 & 0.26 & 0.14 & -5.12 & 8.4 & 6.1 & 5.2 & -23.0 & 109 & 0.01 & 0.02 & 1 \\
3940 & KOI-271 & 19 00 45.6 & +46 01 41 & 6071 & 4.21 & 0.27 & 0.14 & -5.17 & 8.1 & 5.8 & 5.2 & -22.6 & 48 & 0.02 & 0.03 & 1 \\
3941 & KOI-4637 & 19 14 23.9 & +46 01 54 & 6286 & 3.96 & -0.14 & 0.12 & -5.32 & 7.2 & 0.1 & 8.2 & -19.7 & 49 & 0.02 & 0.03 & 1 \\
3942 & KOI-2029 & 19 59 35.2 & +46 03 07 & 5156 & 4.55 & -0.20 & 0.20 & -4.92 & 3.8 & 3.2 & 2.0 & -9.8 & 53 & 0.03 & 0.03 & 1 \\
3943 & KOI-2694 & 19 43 17.1 & +46 03 11 & 4716 & 4.53 & 0.25 & 0.46 & -4.65 & 1.7 & 0.1 & 1.6 & -12.5 & 32 & 0.04 & 0.05 & 1 \\
3944 & KOI-2246 & 19 15 41.8 & +46 03 27 & 5732 & 4.51 & -0.23 & 0.15 & -5.10 & 3.5 & 0.9 & 3.3 & -30.3 & 48 & 0.02 & 0.02 & 1 \\
3945 & KOI-119 & 19 38 14.2 & +46 03 44 & 5614 & 3.89 & 0.29 & 0.09 & -6.59 & 4.2 & 1.1 & 4.0 & -16.0 & 51 & 0.02 & 0.03 & 1 \\
3946 & KOI-110 & 18 58 13.4 & +46 03 50 & 6217 & 4.28 & -0.13 & 0.13 & -5.21 & 8.9 & 5.7 & 6.4 & -34.2 & 47 & 0.02 & 0.03 & 1 \\
3947 & KOI-1813 & 19 09 01.6 & +46 04 00 & 5331 & 4.53 & -0.05 & 0.34 & -4.56 & 3.5 & 2.6 & 2.2 & -2.2 & 46 & 0.05 & 0.03 & 1 \\
3948 & KOI-2082 & 19 38 16.1 & +46 04 33 & 5929 & 4.23 & 0.31 & 0.08 & nan & 5.6 & 3.5 & 4.2 & -29.7 & 47 & 0.03 & 0.03 & 1 \\
3949 & KOI-939 & 19 30 19.3 & +46 05 51 & 5542 & 4.32 & 0.16 & 0.50 & -4.30 & 3.5 & 2.2 & 2.7 & -12.2 & 25 & 0.05 & 0.05 & 1 \\
3950 & KOI-2717 & 19 31 29.3 & +46 05 56 & 6062 & 4.29 & 0.03 & 0.12 & -5.38 & 6.2 & 3.4 & 5.1 & 0.9 & 49 & 0.03 & 0.03 & 1 \\
3951 & KOI-1978 & 19 12 02.9 & +46 07 03 & 5476 & 4.53 & 0.06 & 0.17 & -4.98 & 3.3 & 2.0 & 2.5 & -22.2 & 34 & 0.04 & 0.03 & 1 \\
3952 & KOI-708 & 19 34 54.7 & +46 07 45 & 6108 & 4.14 & -0.08 & 0.12 & -5.39 & 8.6 & 6.2 & 5.4 & 4.0 & 48 & 0.02 & 0.03 & 1 \\
3953 & KOI-3132 & 19 49 19.1 & +46 08 10 & 6066 & 3.99 & 0.38 & 0.11 & -5.62 & 14.3 & 11.5 & 5.9 & -19.9 & 47 & 0.03 & 0.03 & 1 \\
3954 & KOI-49 & 19 28 59.8 & +46 09 54 & 5838 & 4.38 & -0.06 & 0.25 & -4.63 & 9.3 & 7.7 & 3.8 & -110.6 & 49 & 0.02 & 0.03 & 1 \\
3955 & KOI-1806 & 19 32 51.3 & +46 10 30 & 6117 & 4.25 & -0.03 & 0.13 & -5.22 & 8.6 & 6.1 & 5.5 & -48.1 & 43 & 0.03 & 0.03 & 1 \\
3956 & KOI-165 & 19 29 56.9 & +46 11 46 & 5118 & 4.43 & -0.27 & 0.14 & -5.18 & 2.8 & 1.8 & 1.9 & 13.7 & 52 & 0.02 & 0.02 & 1 \\
3957 & KOI-1886 & 19 58 38.5 & +46 11 54 & 6127 & 4.11 & 0.04 & 0.07 & nan & 12.7 & 10.2 & 5.6 & -52.4 & 48 & 0.03 & 0.03 & 1 \\
3958 & KOI-709 & 19 09 19.9 & +46 12 13 & 5343 & 4.51 & -0.20 & 0.12 & -5.29 & 2.3 & 0.1 & 2.3 & -39.2 & 49 & 0.02 & 0.02 & 1 \\
3959 & KOI-3165 & 19 10 33.0 & +46 12 16 & 6262 & 4.00 & -0.14 & 0.15 & -5.01 & 9.8 & 6.4 & 6.8 & -14.1 & 106 & 0.01 & 0.02 & 1 \\
3960 & KOI-3232 & 18 48 28.3 & +46 13 26 & 5809 & 4.58 & 0.00 & 0.23 & -4.68 & 5.2 & 3.5 & 3.6 & -26.5 & 50 & 0.02 & 0.09 & 1 \\
3961 & KOI-288 & 19 34 52.0 & +46 13 36 & 6072 & 3.92 & 0.20 & 0.10 & -5.90 & 9.5 & 6.9 & 6.0 & -18.3 & 49 & 0.02 & 0.03 & 1 \\
3962 & KOI-1819 & 19 41 15.2 & +46 14 15 & 5376 & 4.56 & -0.07 & 0.38 & -4.49 & 4.2 & 3.4 & 2.3 & -6.0 & 51 & 0.02 & 0.02 & 1 \\
3963 & KOI-3229 & 19 18 52.7 & +46 14 40 & 5767 & 4.56 & -0.36 & 0.16 & -5.03 & 3.6 & 0.5 & 3.5 & -73.8 & 50 & 0.02 & 0.03 & 1 \\
3964 & KOI-711 & 19 41 39.1 & +46 16 00 & 5500 & 4.30 & 0.29 & 0.11 & -3.46 & 3.4 & 2.1 & 2.6 & -56.7 & 56 & 0.02 & 0.02 & 2 \\
3965 & KOI-115 & 19 11 33.0 & +46 16 34 & 5957 & 4.42 & -0.10 & 0.13 & nan & 4.8 & 1.6 & 4.4 & -1.3 & 75 & 0.02 & 0.02 & 2 \\
3966 & KOI-710 & 19 32 09.1 & +46 16 39 & 6407 & 3.89 & -0.10 & 0.12 & -5.38 & 17.9 & 13.1 & 10.1 & -15.6 & 45 & 0.03 & 0.03 & 2 \\
3967 & Kepler-217 & 19 32 09.1 & +46 16 39 & 6555 & 4.07 & -0.06 & 0.00 & 0.00 & 18.0 & 12.7 & 11.0 & -15.9 & 83 & 0.02 & 0.03 & 1 \\
3968 & KOI-2612 & 19 48 35.7 & +46 17 49 & 5475 & 4.37 & 0.22 & 0.09 & -5.83 & 3.4 & 2.2 & 2.5 & -19.2 & 37 & 0.03 & 0.03 & 1 \\
3969 & KOI-2884 & 19 33 02.0 & +46 18 21 & 5747 & 3.92 & -0.06 & 0.12 & -5.37 & 4.7 & 1.7 & 4.4 & -41.5 & 51 & 0.02 & 0.02 & 1 \\
3970 & KOI-1970 & 19 30 00.0 & +46 19 28 & 5470 & 4.52 & 0.03 & 0.16 & -5.05 & 2.4 & 0.1 & 2.5 & -37.5 & 33 & 0.04 & 0.04 & 1 \\
3971 & KOI-4430 & 19 14 23.2 & +46 19 34 & 5008 & 4.48 & 0.03 & 0.60 & -4.40 & 2.8 & 2.1 & 1.8 & 14.4 & 36 & 0.03 & 0.04 & 1 \\
3972 & KOI-179 & 19 48 10.9 & +46 19 43 & 6058 & 3.96 & 0.22 & 0.11 & -5.62 & 11.0 & 8.5 & 5.9 & 8.0 & 44 & 0.03 & 0.03 & 1 \\
3973 & KOI-2049 & 19 28 10.7 & +46 19 44 & 5924 & 4.06 & 0.05 & 0.12 & -5.41 & 5.7 & 3.7 & 4.2 & -19.1 & 47 & 0.02 & 0.03 & 1 \\
3974 & KOI-712 & 19 11 57.9 & +46 21 25 & 5382 & 4.48 & -0.09 & 0.13 & -5.21 & 3.0 & 1.8 & 2.3 & -46.7 & 49 & 0.02 & 0.02 & 1 \\
3975 & KOI-1938 & 19 30 41.4 & +46 22 39 & 5095 & 4.57 & -0.24 & 0.11 & -5.32 & 2.7 & 1.7 & 1.9 & -22.6 & 48 & 0.03 & 0.03 & 1 \\
3976 & KOI-2815 & 19 51 26.4 & +46 23 11 & 5905 & 4.30 & -0.06 & 0.11 & -5.62 & 4.2 & 0.8 & 4.1 & -32.4 & 47 & 0.02 & 0.03 & 1 \\
3977 & Kepler-423 & 19 31 25.4 & +46 23 28 & 5648 & 4.44 & 0.04 & 0.00 & 0.00 & 3.8 & 2.1 & 3.0 & -2.5 & 67 & 0.04 & 0.03 & 1 \\
3978 & KOI-1854 & 19 47 50.1 & +46 23 39 & 5571 & 4.49 & -0.03 & 0.12 & -5.34 & 3.4 & 1.8 & 2.8 & -25.9 & 50 & 0.02 & 0.02 & 1 \\
3979 & KOI-4822 & 19 14 01.7 & +46 24 24 & 5819 & 4.09 & -0.02 & 0.14 & -5.12 & 4.4 & 2.2 & 3.7 & -106.4 & 47 & 0.02 & 0.03 & 1 \\
3980 & KOI-4617 & 19 11 44.9 & +46 25 07 & 5915 & 4.19 & -0.12 & 0.13 & -5.21 & 4.4 & 1.1 & 4.2 & -11.8 & 40 & 0.03 & 0.03 & 1 \\
3981 & KOI-2831 & 18 49 15.2 & +46 25 10 & 5715 & 3.87 & -0.07 & 0.11 & -5.58 & 5.9 & 3.8 & 4.3 & -24.3 & 50 & 0.02 & 0.03 & 1 \\
3982 & KOI-2706 & 19 00 18.6 & +46 25 11 & 6255 & 4.04 & 0.12 & 0.18 & -4.84 & 12.9 & 9.8 & 6.8 & -39.1 & 107 & 0.02 & 0.02 & 1 \\
3983 & KOI-2769 & 18 48 03.0 & +46 25 42 & 5766 & 3.94 & -0.08 & 0.12 & -5.35 & 4.4 & 0.1 & 4.4 & -19.6 & 49 & 0.02 & 0.03 & 1 \\
3984 & KOI-2545 & 18 58 22.5 & +46 27 00 & 6059 & 3.96 & 0.14 & 0.09 & nan & 8.3 & 5.5 & 5.9 & -11.0 & 48 & 0.03 & 0.03 & 1 \\
3985 & KOI-1751 & 19 54 25.9 & +46 27 13 & 5059 & 4.53 & -0.08 & 0.20 & -4.94 & 3.1 & 2.4 & 1.9 & -37.8 & 36 & 0.04 & 0.04 & 1 \\
3986 & KOI-1913 & 19 17 11.1 & +46 27 29 & 5426 & 4.53 & 0.12 & 0.35 & -4.53 & 3.8 & 2.8 & 2.4 & -11.5 & 49 & 0.03 & 0.03 & 1 \\
3987 & KOI-714 & 19 12 02.0 & +46 28 25 & 5298 & 4.50 & 0.05 & 0.26 & -4.72 & 2.4 & 0.6 & 2.2 & -52.6 & 50 & 0.02 & 0.02 & 1 \\
3988 & KOI-2913 & 18 50 31.5 & +46 28 52 & 5700 & 4.28 & 0.27 & 0.12 & -5.38 & 3.9 & 2.1 & 3.2 & -14.2 & 50 & 0.02 & 0.02 & 1 \\
3989 & KOI-2273 & 19 39 38.8 & +46 29 29 & 5985 & 4.29 & 0.23 & 0.13 & -5.23 & 6.1 & 3.8 & 4.6 & -55.9 & 49 & 0.02 & 0.03 & 1 \\
3990 & KOI-2035 & 19 55 28.0 & +46 30 08 & 5489 & 4.57 & -0.01 & 0.38 & -4.46 & 7.1 & 6.3 & 2.6 & -13.6 & 50 & 0.02 & 0.02 & 1 \\
3991 & KOI-2457 & 18 49 12.3 & +46 30 58 & 6398 & 4.09 & -0.03 & 0.12 & -5.28 & 13.8 & 9.5 & 8.5 & 0.8 & 47 & 0.03 & 0.03 & 1 \\
3992 & KOI-3871 & 18 48 47.6 & +46 31 13 & 5144 & 4.56 & 0.02 & 0.69 & -4.27 & 3.9 & 3.3 & 2.0 & -25.7 & 51 & 0.02 & 0.03 & 1 \\
3993 & KOI-3162 & 18 48 46.8 & +46 31 22 & 6024 & 4.41 & 0.01 & 0.18 & -4.86 & 20.0 & 15.7 & 4.8 & -25.3 & 109 & 0.02 & 0.03 & 1 \\
3994 & KOI-3465 & 19 14 14.8 & +46 32 10 & 5247 & 4.46 & -0.03 & 0.28 & -4.70 & 3.8 & 3.1 & 2.1 & -31.7 & 50 & 0.02 & 0.02 & 1 \\
3995 & KOI-3837 & 19 09 29.2 & +46 33 53 & 6393 & 4.43 & -0.08 & 0.13 & -5.24 & 11.8 & 7.4 & 8.4 & -38.8 & 48 & 0.02 & 0.03 & 1 \\
3996 & KOI-1852 & 19 13 40.3 & +46 35 26 & 6446 & 4.30 & -0.10 & 0.17 & -4.87 & 6.3 & 0.1 & 9.2 & -10.9 & 45 & 0.03 & 0.03 & 1 \\
3997 & KOI-1529 & 19 08 09.5 & +46 38 24 & 5873 & 4.19 & -0.23 & 0.11 & -5.54 & 4.0 & 0.2 & 3.9 & -38.6 & 31 & 0.04 & 0.04 & 1 \\
3998 & KOI-2943 & 19 39 19.5 & +46 39 35 & 5756 & 4.14 & 0.29 & 0.34 & -4.45 & 4.1 & 2.2 & 3.4 & -14.7 & 49 & 0.02 & 0.02 & 1 \\
3999 & KOI-135 & 19 00 57.8 & +46 40 06 & 5925 & 4.24 & 0.33 & 0.14 & -5.16 & 6.6 & 4.8 & 4.2 & -39.8 & 49 & 0.02 & 0.02 & 1 \\
4000 & KOI-4421 & 19 36 30.0 & +46 40 22 & 5944 & 4.11 & 0.03 & 0.13 & -5.25 & 6.6 & 4.7 & 4.3 & -7.9 & 46 & 0.02 & 0.03 & 1 \\
4001 & KOI-1715 & 19 37 06.6 & +46 40 31 & 5859 & 4.30 & -0.24 & 0.12 & -5.36 & 3.7 & 0.1 & 3.9 & -25.8 & 48 & 0.02 & 0.03 & 1 \\
4002 & KOI-1958 & 19 35 55.6 & +46 41 16 & 5789 & 4.50 & 0.01 & 0.29 & -4.55 & 5.6 & 4.1 & 3.6 & 6.8 & 26 & 0.05 & 0.05 & 1 \\
4003 & KOI-716 & 19 49 58.1 & +46 41 40 & 6067 & 4.17 & 0.15 & 0.09 & nan & 6.6 & 3.9 & 5.1 & -16.9 & 48 & 0.02 & 0.03 & 1 \\
4004 & KOI-1606 & 19 20 12.3 & +46 42 48 & 5352 & 4.46 & 0.04 & 0.18 & -4.95 & 2.7 & 1.2 & 2.3 & -19.7 & 53 & 0.02 & 0.02 & 1 \\
4005 & KOI-717 & 18 48 51.1 & +46 43 04 & 5549 & 4.27 & 0.26 & 0.12 & -5.38 & 3.1 & 1.2 & 2.7 & -8.5 & 51 & 0.02 & 0.02 & 1 \\
4006 & KOI-4230 & 18 47 35.4 & +46 43 21 & 5900 & 4.14 & -0.34 & 0.12 & -5.39 & 4.4 & 1.3 & 4.1 & -51.9 & 48 & 0.02 & 0.03 & 1 \\
4007 & KOI-3246 & 19 17 41.8 & +46 43 34 & 4715 & 4.44 & 0.04 & 0.70 & -4.46 & 3.3 & 2.9 & 1.6 & -32.0 & 55 & 0.03 & 0.03 & 1 \\
4008 & KOI-1955 & 19 30 42.7 & +46 43 36 & 6193 & 4.17 & 0.10 & 0.12 & -5.45 & 11.5 & 8.7 & 6.2 & -31.2 & 44 & 0.03 & 0.03 & 1 \\
4009 & Kepler-342 & 19 30 42.7 & +46 43 36 & 6177 & 4.15 & 0.11 & 0.00 & 0.00 & 11.8 & 9.1 & 6.0 & -26.6 & 76 & 0.02 & 0.02 & 1 \\
4010 & KOI-2135 & 19 47 12.8 & +46 44 28 & 6107 & 4.16 & 0.03 & 0.12 & -5.37 & 9.2 & 6.8 & 5.4 & 8.0 & 48 & 0.02 & 0.03 & 1 \\
4011 & KOI-2732 & 19 19 41.2 & +46 44 40 & 6007 & 4.01 & 0.07 & 0.11 & -5.51 & 6.5 & 4.2 & 4.7 & -35.4 & 47 & 0.02 & 0.03 & 1 \\
4012 & Kepler-403 & 19 19 41.2 & +46 44 40 & 5998 & 3.95 & 0.06 & 0.00 & 0.00 & 6.7 & 3.6 & 5.5 & -33.1 & 93 & 0.01 & 0.02 & 1 \\
4013 & KOI-4575 & 19 31 44.7 & +46 45 11 & 6157 & 3.90 & 0.03 & 0.11 & -5.51 & 7.5 & 3.3 & 6.7 & -22.2 & 48 & 0.02 & 0.03 & 1 \\
4014 & KOI-718 & 19 14 57.4 & +46 45 45 & 5846 & 4.34 & 0.33 & 0.13 & -5.28 & 5.0 & 3.1 & 3.8 & -18.8 & 44 & 0.03 & 0.03 & 1 \\
4015 & Kepler-219 & 19 14 57.4 & +46 45 45 & 5876 & 4.42 & 0.33 & 0.16 & -4.99 & 5.2 & 3.2 & 4.0 & -18.1 & 65 & 0.03 & 0.05 & 1 \\
4016 & KOI-327 & 19 09 28.7 & +46 46 06 & 6042 & 4.28 & -0.02 & 0.12 & -5.41 & 5.9 & 3.1 & 4.9 & -28.5 & 48 & 0.02 & 0.03 & 1 \\
4017 & KOI-4383 & 19 13 52.6 & +46 47 01 & 5749 & 4.57 & 0.01 & 0.21 & -4.79 & 4.3 & 2.6 & 3.4 & 5.9 & 45 & 0.03 & 0.03 & 1 \\
4018 & KOI-1537 & 18 45 50.8 & +46 47 24 & 6152 & 3.94 & -0.14 & 0.12 & -5.47 & 7.9 & 4.1 & 6.6 & -29.9 & 48 & 0.02 & 0.03 & 1 \\
4019 & KOI-2803 & 19 39 28.1 & +46 47 26 & 5582 & 4.44 & 0.09 & 0.10 & -5.62 & 3.9 & 2.6 & 2.8 & 10.6 & 51 & 0.02 & 0.05 & 1 \\
4020 & KOI-1779 & 19 53 55.9 & +46 47 37 & 5748 & 4.49 & 0.22 & 0.24 & -4.69 & 8.3 & 7.1 & 3.4 & -25.9 & 47 & 0.03 & 0.03 & 1 \\
4021 & KOI-721 & 19 48 16.4 & +46 50 03 & 5806 & 4.09 & 0.10 & 0.13 & -5.20 & 3.9 & 1.4 & 3.6 & -48.9 & 48 & 0.02 & 0.03 & 1 \\
4022 & KOI-720 & 19 46 37.1 & +46 50 07 & 5159 & 4.51 & -0.08 & 0.43 & -4.50 & 5.0 & 4.5 & 2.0 & 3.0 & 52 & 0.02 & 0.02 & 1 \\
4023 & KOI-722 & 19 49 02.2 & +46 50 35 & 6513 & 4.54 & 0.19 & 0.13 & -5.21 & 7.6 & 0.1 & 10.2 & -27.6 & 49 & 0.29 & 0.04 & 1 \\
4024 & KOI-4431 & 18 54 53.8 & +46 52 45 & 6152 & 3.95 & -0.16 & 0.11 & -5.62 & 11.9 & 8.8 & 6.6 & -7.3 & 48 & 0.02 & 0.03 & 1 \\
4025 & KOI-1875 & 19 51 45.2 & +46 52 53 & 5626 & 4.54 & -0.12 & 0.12 & -5.34 & 3.4 & 1.3 & 3.0 & -34.7 & 35 & 0.03 & 0.06 & 1 \\
4026 & KOI-4647 & 19 21 02.2 & +46 53 06 & 5051 & 3.70 & 0.16 & 0.17 & -5.03 & 3.5 & 0.1 & 3.5 & 10.9 & 42 & 0.03 & 0.03 & 1 \\
4027 & KOI-528 & 19 08 24.3 & +46 53 47 & 5370 & 4.57 & -0.07 & 0.11 & -5.41 & 2.4 & 0.2 & 2.3 & -28.0 & 32 & 0.04 & 0.04 & 1 \\
4028 & KOI-2748 & 19 45 06.7 & +46 54 00 & 5513 & 4.03 & -0.12 & 0.14 & -5.18 & 3.6 & 2.4 & 2.6 & -0.7 & 51 & 0.02 & 0.03 & 1 \\
4029 & KOI-2832 & 18 54 15.7 & +46 54 15 & 4983 & 4.51 & 0.07 & 0.20 & -4.96 & 1.9 & 0.3 & 1.8 & -35.0 & 54 & 0.02 & 0.03 & 1 \\
4030 & KOI-2312 & 19 49 08.0 & +46 54 16 & 6428 & 3.97 & -0.20 & 0.12 & -5.44 & 8.2 & 0.1 & 10.5 & -17.2 & 49 & 0.06 & 0.03 & 1 \\
4031 & KOI-4146 & 19 07 16.7 & +46 54 42 & 4987 & 4.49 & 0.16 & 0.49 & -4.50 & 4.0 & 3.5 & 1.8 & -27.1 & 53 & 0.02 & 0.03 & 1 \\
4032 & KOI-4706 & 19 49 05.0 & +46 55 42 & 5997 & 4.20 & -0.22 & 0.10 & -5.88 & 4.8 & 0.9 & 4.6 & -29.6 & 45 & 0.03 & 0.03 & 1 \\
4033 & KOI-3382 & 18 44 43.3 & +46 55 48 & 5363 & 4.49 & 0.12 & 0.13 & -5.19 & 2.6 & 0.9 & 2.3 & -49.0 & 29 & 0.04 & 0.04 & 1 \\
4034 & KOI-723 & 19 11 37.5 & +46 56 16 & 5211 & 4.52 & 0.21 & 0.51 & -4.39 & 4.6 & 4.0 & 2.1 & -21.5 & 36 & 0.03 & 0.03 & 1 \\
4035 & KOI-1796 & 19 39 39.9 & +46 56 42 & 5992 & 4.44 & -0.04 & 0.18 & -4.84 & 5.9 & 3.5 & 4.6 & -0.3 & 48 & 0.02 & 0.03 & 1 \\
4036 & KOI-2785 & 19 08 20.7 & +46 56 45 & 5886 & 4.42 & -0.01 & 0.11 & -5.65 & 4.2 & 1.1 & 4.0 & -6.1 & 46 & 0.03 & 0.03 & 1 \\
4037 & KOI-4469 & 19 19 01.6 & +46 57 10 & 4830 & 4.49 & 0.04 & 0.18 & -5.07 & 1.9 & 0.6 & 1.7 & -24.3 & 38 & 0.03 & 0.04 & 1 \\
4038 & WASP-113 & 14 59 29.5 & +46 57 36 & 5918 & 4.10 & 0.27 & 0.00 & 0.00 & 7.2 & 5.5 & 4.2 & -12.6 & 111 & 0.01 & 0.01 & 1 \\
4039 & KOI-1598 & 19 15 21.5 & +46 59 12 & 5429 & 4.58 & -0.19 & 0.07 & nan & 2.7 & 1.0 & 2.4 & -29.7 & 35 & 0.03 & 0.03 & 1 \\
4040 & Kepler-310 & 19 15 21.5 & +46 59 12 & 5432 & 4.54 & -0.22 & 0.00 & 0.00 & 3.1 & 1.7 & 2.4 & -28.0 & 62 & 0.02 & 0.05 & 1 \\
4041 & KOI-1783 & 19 17 22.0 & +46 59 18 & 5937 & 4.35 & 0.11 & 0.12 & -5.45 & 4.8 & 2.0 & 4.3 & -4.2 & 44 & 0.03 & 0.03 & 1 \\
4042 & KOI-2002 & 19 47 01.4 & +46 59 54 & 5990 & 4.46 & 0.02 & 0.18 & -4.86 & 6.4 & 4.1 & 4.6 & -3.1 & 48 & 0.02 & 0.03 & 1 \\
4043 & KOI-1984 & 19 53 58.4 & +47 00 47 & 5968 & 4.30 & 0.11 & 0.14 & -5.11 & 5.8 & 3.5 & 4.5 & -36.1 & 47 & 0.02 & 0.03 & 1 \\
4044 & HAT-P-44 & 14 12 34.6 & +47 00 53 & 5269 & 4.39 & 0.31 & 0.00 & 0.00 & 3.0 & 2.0 & 2.1 & -36.5 & 106 & 0.01 & 0.04 & 1 \\
4045 & KOI-4292 & 19 05 32.9 & +47 01 00 & 5567 & 4.48 & -0.00 & 0.35 & -4.48 & 3.1 & 1.2 & 2.8 & -75.1 & 50 & 0.02 & 0.07 & 1 \\
4046 & KOI-2891 & 19 15 23.3 & +47 01 22 & 6030 & 3.93 & 0.10 & 0.12 & -5.33 & 7.1 & 4.1 & 5.7 & -25.6 & 48 & 0.02 & 0.03 & 1 \\
4047 & KOI-1917 & 19 26 08.3 & +47 02 33 & 5935 & 4.31 & -0.09 & 0.13 & -5.23 & 4.9 & 2.3 & 4.3 & -7.1 & 48 & 0.02 & 0.02 & 1 \\
4048 & KOI-2964 & 19 58 42.2 & +47 04 33 & 6042 & 3.89 & -0.36 & 0.12 & -5.36 & 10.3 & 7.8 & 5.8 & -27.3 & 50 & 0.03 & 0.05 & 1 \\
4049 & KOI-1608 & 18 48 14.7 & +47 05 08 & 5932 & 4.34 & -0.03 & 0.14 & -5.17 & 4.5 & 1.3 & 4.3 & -39.3 & 47 & 0.02 & 0.03 & 1 \\
4050 & KOI-1888 & 19 06 44.5 & +47 05 54 & 6363 & 4.10 & 0.11 & 0.14 & -5.10 & 20.5 & 16.3 & 8.0 & -6.8 & 47 & 0.02 & 0.03 & 1 \\
4051 & KOI-1909 & 19 08 33.8 & +47 06 55 & 5883 & 4.42 & -0.01 & 0.15 & -5.05 & 4.4 & 1.7 & 4.0 & -36.7 & 48 & 0.02 & 0.02 & 1 \\
4052 & Kepler-334 & 19 08 33.8 & +47 06 55 & 5914 & 4.49 & 0.00 & 0.17 & -4.93 & 4.8 & 2.2 & 4.2 & -36.4 & 90 & 0.01 & 0.02 & 1 \\
4053 & KOI-1929 & 19 20 14.5 & +47 09 50 & 5613 & 3.93 & -0.00 & 0.15 & -5.09 & 3.8 & 0.1 & 4.0 & -63.8 & 50 & 0.02 & 0.02 & 1 \\
4054 & KOI-3195 & 18 44 29.5 & +47 09 54 & 6003 & 3.78 & -0.33 & 0.11 & -5.64 & 5.5 & 0.2 & 5.5 & -18.4 & 47 & 0.03 & 0.03 & 1 \\
4055 & KOI-1784 & 19 50 35.1 & +47 10 03 & 6028 & 4.54 & 0.02 & 0.16 & -4.99 & 7.9 & 5.6 & 4.9 & -16.1 & 49 & 0.02 & 0.03 & 1 \\
4056 & KOI-3208 & 19 46 43.3 & +47 10 23 & 5922 & 4.58 & -0.11 & 0.10 & -5.89 & 4.2 & 0.1 & 4.2 & -36.8 & 47 & 0.02 & 0.03 & 1 \\
4057 & KOI-991 & 19 45 59.1 & +47 10 58 & 5495 & 4.47 & -0.24 & 0.14 & -5.11 & 3.3 & 1.9 & 2.6 & -3.3 & 47 & 0.03 & 0.03 & 1 \\
4058 & KOI-4613 & 19 46 21.0 & +47 12 26 & 5469 & 4.58 & -0.17 & 0.12 & -5.28 & 2.9 & 1.2 & 2.5 & 32.0 & 50 & 0.02 & 0.02 & 1 \\
4059 & KOI-3218 & 18 55 24.4 & +47 14 37 & 5999 & 4.45 & 0.04 & 0.15 & -5.07 & 5.5 & 2.7 & 4.7 & -40.6 & 49 & 0.02 & 0.03 & 1 \\
4060 & KOI-4070 & 18 45 45.8 & +47 14 47 & 4836 & 4.51 & 0.05 & 0.21 & -4.98 & 2.2 & 1.2 & 1.7 & -14.4 & 38 & 0.03 & 0.04 & 1 \\
4061 & KOI-2342 & 19 34 54.2 & +47 14 49 & 5939 & 4.21 & -0.37 & 0.13 & -5.19 & 4.6 & 1.3 & 4.3 & -47.8 & 45 & 0.03 & 0.03 & 1 \\
4062 & KOI-427 & 18 52 05.5 & +47 15 40 & 5266 & 4.59 & 0.05 & 0.23 & -4.82 & 2.5 & 1.1 & 2.1 & 3.9 & 31 & 0.04 & 0.04 & 1 \\
4063 & KOI-3130 & 18 42 50.1 & +47 19 41 & 4886 & 4.58 & -0.43 & 0.29 & -4.79 & 2.2 & 1.3 & 1.7 & -17.6 & 53 & 0.08 & 0.07 & 1 \\
4064 & KOI-5782 & 19 25 27.1 & +47 19 43 & 5007 & 3.51 & 0.10 & 0.12 & -5.30 & 3.4 & 0.1 & 3.4 & -12.6 & 38 & 0.03 & 0.03 & 1 \\
4065 & KOI-331 & 19 44 44.0 & +47 21 32 & 5469 & 3.94 & 0.03 & 0.13 & -5.22 & 3.7 & 0.1 & 3.8 & -26.5 & 50 & 0.02 & 0.02 & 1 \\
4066 & KOI-2390 & 19 48 51.8 & +47 22 43 & 5849 & 3.79 & 0.04 & 0.05 & nan & 6.8 & 4.6 & 4.7 & 3.7 & 49 & 0.03 & 0.03 & 1 \\
4067 & KOI-732 & 19 13 18.7 & +47 22 54 & 5146 & 4.42 & 0.23 & 0.21 & -4.89 & 2.6 & 1.6 & 2.0 & -16.5 & 36 & 0.03 & 0.04 & 1 \\
4068 & KOI-4557 & 18 54 49.1 & +47 23 07 & 5925 & 4.05 & 0.02 & 0.13 & -5.24 & 5.6 & 3.4 & 4.2 & -18.2 & 45 & 0.03 & 0.10 & 1 \\
4069 & KOI-3608 & 18 59 15.7 & +47 23 33 & 5885 & 4.40 & -0.09 & 0.16 & -5.02 & 4.2 & 0.8 & 4.0 & -33.6 & 49 & 0.02 & 0.02 & 1 \\
4070 & KOI-332 & 19 50 36.2 & +47 23 47 & 5711 & 4.15 & 0.30 & 0.28 & -4.59 & 4.4 & 2.8 & 3.2 & -61.2 & 50 & 0.02 & 0.02 & 1 \\
4071 & KOI-2153 & 18 46 16.8 & +47 23 55 & 6051 & 4.17 & -0.03 & 0.12 & -5.31 & 7.3 & 5.0 & 5.0 & -9.2 & 48 & 0.02 & 0.03 & 1 \\
4072 & KOI-333 & 19 23 49.9 & +47 24 23 & 6140 & 4.27 & 0.11 & 0.14 & -5.11 & 10.1 & 7.6 & 5.7 & 7.5 & 47 & 0.02 & 0.03 & 1 \\
4073 & KOI-1905 & 19 06 39.1 & +47 24 49 & 4872 & 4.50 & -0.16 & 0.22 & -4.94 & 2.0 & 0.8 & 1.7 & -36.7 & 50 & 0.02 & 0.03 & 1 \\
4074 & KOI-3216 & 19 25 29.0 & +47 26 08 & 5676 & 4.46 & 0.01 & 0.51 & -4.25 & 16.5 & 14.0 & 3.1 & -60.6 & 49 & 0.03 & 0.03 & 1 \\
4075 & KOI-3908 & 19 58 20.0 & +47 26 53 & 5738 & 3.94 & -0.01 & 0.11 & -5.61 & 5.5 & 3.2 & 4.3 & 10.4 & 52 & 0.03 & 0.08 & 1 \\
4076 & KOI-1175 & 19 43 41.0 & +47 26 55 & 5550 & 3.72 & 0.00 & 0.12 & -5.30 & 5.4 & 3.5 & 3.9 & -2.7 & 49 & 0.02 & 0.07 & 1 \\
4077 & KOI-1169 & 18 46 12.3 & +47 28 12 & 5646 & 4.42 & 0.07 & 0.15 & -5.05 & 3.6 & 1.7 & 3.0 & -39.4 & 125 & 0.01 & 0.01 & 1 \\
4078 & KOI-1165 & 19 24 15.1 & +47 29 05 & 5330 & 4.46 & -0.11 & 0.09 & -5.69 & 2.6 & 1.2 & 2.2 & -12.8 & 50 & 0.02 & 0.02 & 1 \\
4079 & KOI-3991 & 19 46 00.9 & +47 29 13 & 5569 & 4.49 & -0.13 & 0.36 & -4.47 & 7.8 & 6.8 & 2.8 & -18.2 & 51 & 0.02 & 0.03 & 1 \\
4080 & KOI-4446 & 19 08 32.4 & +47 29 19 & 5135 & 3.91 & -0.25 & 0.08 & -5.72 & 3.6 & 0.1 & 3.5 & -41.2 & 52 & 0.02 & 0.03 & 1 \\
4081 & KOI-2147 & 19 27 05.2 & +47 31 48 & 5667 & 4.42 & -0.18 & 0.10 & -5.79 & 3.9 & 2.3 & 3.1 & -5.3 & 35 & 0.03 & 0.04 & 1 \\
4082 & KOI-2859 & 19 15 19.5 & +47 33 07 & 5227 & 4.49 & -0.12 & 0.18 & -4.97 & 2.7 & 1.6 & 2.1 & -30.1 & 51 & 0.02 & 0.03 & 1 \\
4083 & KOI-4556 & 19 18 28.5 & +47 33 29 & 5455 & 3.84 & -0.14 & 0.14 & -5.13 & 4.6 & 2.5 & 3.8 & -51.5 & 51 & 0.02 & 0.03 & 1 \\
4084 & KOI-289 & 18 51 47.0 & +47 34 30 & 6080 & 4.48 & -0.25 & 0.07 & nan & 5.1 & 0.1 & 5.2 & -0.5 & 46 & 0.03 & 0.07 & 1 \\
4085 & KOI-3224 & 18 45 18.6 & +47 35 06 & 5317 & 4.51 & -0.03 & 0.23 & -4.80 & 3.6 & 2.7 & 2.2 & -19.7 & 53 & 0.03 & 0.03 & 1 \\
4086 & KOI-2583 & 18 53 43.0 & +47 35 33 & 5576 & 4.45 & 0.03 & 0.14 & -5.13 & 2.9 & 0.5 & 2.8 & -29.4 & 49 & 0.02 & 0.02 & 1 \\
4087 & KOI-1161 & 19 56 30.6 & +47 35 38 & 5348 & 4.30 & -0.09 & 0.17 & -5.01 & 3.8 & 3.0 & 2.3 & 29.7 & 37 & 0.03 & 0.07 & 1 \\
4088 & KOI-1168 & 19 10 20.8 & +47 36 00 & 6073 & 3.96 & 0.07 & 0.12 & -5.31 & 8.2 & 5.2 & 6.0 & -9.3 & 47 & 0.02 & 0.03 & 1 \\
4089 & KOI-2040 & 19 43 10.1 & +47 36 00 & 5670 & 4.46 & -0.04 & 0.14 & -5.17 & 3.4 & 1.1 & 3.1 & -19.1 & 46 & 0.02 & 0.03 & 1 \\
4090 & KOI-474 & 19 11 07.4 & +47 37 48 & 5927 & 4.37 & -0.03 & 0.15 & -5.03 & 4.9 & 2.3 & 4.2 & 9.2 & 32 & 0.04 & 0.05 & 1 \\
4091 & Kepler-164 & 19 11 07.4 & +47 37 48 & 6018 & 4.49 & 0.04 & 0.00 & 0.00 & 5.3 & 2.1 & 4.8 & 11.6 & 64 & 0.06 & 0.04 & 1 \\
4092 & KOI-2484 & 18 55 32.4 & +47 38 14 & 5841 & 4.36 & -0.29 & 0.13 & -5.22 & 3.9 & 0.7 & 3.8 & -45.5 & 48 & 0.02 & 0.02 & 1 \\
4093 & KOI-3231 & 19 53 26.1 & +47 38 19 & 6211 & 4.41 & 0.05 & 0.13 & -5.25 & 11.1 & 7.7 & 6.3 & -21.1 & 47 & 0.03 & 0.03 & 1 \\
4094 & KOI-4480 & 19 23 06.4 & +47 38 54 & 5554 & 4.42 & 0.20 & 0.20 & -4.85 & 3.3 & 1.8 & 2.7 & -30.3 & 50 & 0.02 & 0.02 & 1 \\
4095 & KOI-2961 & 19 29 21.0 & +47 39 51 & 6003 & 4.28 & 0.09 & 0.13 & -5.29 & 6.6 & 4.4 & 4.7 & -14.9 & 49 & 0.14 & 0.09 & 1 \\
4096 & KOI-1163 & 19 25 12.5 & +47 41 52 & 5276 & 4.60 & -0.31 & 0.16 & -5.06 & 2.1 & 0.1 & 2.2 & -17.1 & 30 & 0.04 & 0.04 & 1 \\
4097 & KOI-2208 & 19 22 10.5 & +47 43 33 & 5862 & 4.36 & 0.08 & 0.15 & -5.08 & 4.6 & 2.3 & 3.9 & -58.9 & 50 & 0.02 & 0.03 & 1 \\
4098 & KOI-338 & 19 51 53.0 & +47 43 54 & 4910 & 4.46 & 0.30 & 0.24 & -4.88 & 2.0 & 0.7 & 1.7 & -19.7 & 54 & 0.02 & 0.03 & 1 \\
4099 & KOI-4345 & 19 26 00.3 & +47 44 52 & 5716 & 4.34 & -0.08 & 0.15 & -5.06 & 4.7 & 3.2 & 3.3 & -56.8 & 46 & 0.02 & 0.03 & 1 \\
4100 & KOI-337 & 19 42 44.4 & +47 44 53 & 5757 & 4.35 & 0.05 & 0.14 & -5.11 & 3.9 & 1.7 & 3.4 & -63.1 & 46 & 0.03 & 0.03 & 1 \\
4101 & KOI-263 B & 18 45 05.4 & +47 46 36 & 5901 & 4.31 & -0.11 & 0.14 & -5.15 & 4.2 & 0.3 & 4.1 & -0.4 & 47 & 0.02 & 0.03 & 1 \\
4102 & KOI-340 & 19 50 39.5 & +47 48 05 & 5593 & 3.96 & 0.28 & 0.27 & -4.64 & 8.4 & 6.9 & 4.0 & -92.9 & 51 & 0.02 & 0.02 & 1 \\
4103 & KOI-2300 & 18 56 23.4 & +47 48 38 & 5081 & 4.57 & -0.15 & 0.25 & -4.80 & 2.3 & 1.0 & 1.9 & -28.9 & 45 & 0.03 & 0.03 & 1 \\
4104 & KOI-203 & 19 53 34.9 & +47 48 54 & 5606 & 4.46 & 0.21 & 0.33 & -4.51 & 5.7 & 4.7 & 2.9 & -27.0 & 50 & 0.04 & 0.04 & 1 \\
4105 & KOI-4765 & 19 49 18.9 & +47 48 56 & 6115 & 4.23 & 0.13 & 0.14 & -5.16 & 8.5 & 6.0 & 5.5 & -23.9 & 47 & 0.03 & 0.03 & 1 \\
4106 & KOI-1308 & 19 01 41.8 & +47 50 05 & 5679 & 4.20 & -0.01 & 0.12 & -5.41 & 3.9 & 2.1 & 3.1 & -8.8 & 49 & 0.02 & 0.04 & 1 \\
4107 & KOI-275 & 19 01 14.7 & +47 50 55 & 5761 & 4.03 & 0.22 & 0.11 & -5.53 & 4.5 & 2.8 & 3.4 & -23.5 & 50 & 0.02 & 0.02 & 1 \\
4108 & KOI-4892 & 19 02 49.7 & +47 52 12 & 5651 & 3.84 & -0.38 & 0.16 & -5.04 & 4.3 & 0.8 & 4.1 & 42.0 & 49 & 0.03 & 0.03 & 1 \\
4109 & KOI-3032 & 19 00 37.7 & +47 52 24 & 5098 & 4.45 & 0.31 & 0.89 & -4.18 & 2.2 & 0.8 & 1.9 & -27.1 & 25 & 0.05 & 0.06 & 1 \\
4110 & KOI-4204 & 19 16 43.8 & +47 52 24 & 5896 & 4.28 & 0.16 & 0.13 & -5.29 & 4.8 & 2.4 & 4.1 & -52.5 & 43 & 0.03 & 0.03 & 1 \\
4111 & KOI-339 & 19 03 33.2 & +47 52 49 & 6040 & 4.39 & -0.15 & 0.11 & -5.56 & 6.6 & 4.0 & 4.9 & -15.4 & 48 & 0.02 & 0.02 & 1 \\
4112 & KOI-749 & 19 29 30.3 & +47 52 52 & 5257 & 4.41 & 0.01 & 0.15 & -5.09 & 2.4 & 0.9 & 2.1 & -37.9 & 35 & 0.04 & 0.03 & 1 \\
4113 & KOI-2149 & 19 51 08.8 & +47 53 10 & 6129 & 4.14 & 0.20 & 0.11 & -5.54 & 10.7 & 8.3 & 5.6 & -38.1 & 50 & 0.02 & 0.03 & 1 \\
4114 & KOI-4833 & 18 57 16.1 & +47 53 14 & 5725 & 4.09 & -0.02 & 0.14 & -5.19 & 4.0 & 2.1 & 3.3 & 54.1 & 50 & 0.02 & 0.02 & 1 \\
4115 & KOI-1837 & 19 13 29.4 & +47 56 01 & 5155 & 4.53 & 0.05 & 0.32 & -4.65 & 3.5 & 2.8 & 2.0 & -22.4 & 49 & 0.02 & 0.03 & 1 \\
4116 & KOI-1797 & 19 43 26.3 & +47 56 22 & 4857 & 4.47 & 0.06 & 0.46 & -4.59 & 4.3 & 3.9 & 1.7 & -25.7 & 57 & 0.02 & 0.04 & 1 \\
4117 & KOI-598 & 19 12 29.0 & +47 58 00 & 5182 & 4.50 & -0.03 & 0.20 & -4.92 & 2.2 & 0.7 & 2.0 & -21.3 & 36 & 0.03 & 0.04 & 1 \\
4118 & KOI-2 & 19 28 59.4 & +47 58 10 & 6234 & 3.92 & 0.19 & 0.06 & -3.28 & 6.9 & 0.1 & 7.5 & -10.6 & 69 & 0.02 & 0.03 & 3 \\
4119 & KOI-4366 & 18 51 39.4 & +47 58 13 & 5278 & 4.49 & -0.15 & 0.58 & -4.31 & 2.0 & 0.1 & 2.2 & -14.0 & 25 & 0.06 & 0.06 & 1 \\
4120 & KOI-211 & 19 11 52.9 & +47 58 20 & 5923 & 4.20 & -0.01 & 0.15 & -5.08 & 5.1 & 2.7 & 4.2 & -1.1 & 36 & 0.03 & 0.03 & 1 \\
4121 & KOI-2046 & 19 23 55.0 & +47 59 20 & 5551 & 4.11 & 0.18 & 0.11 & -5.44 & 4.0 & 2.8 & 2.7 & -1.8 & 49 & 0.02 & 0.02 & 1 \\
4122 & KOI-4312 & 19 12 55.9 & +48 00 08 & 5829 & 4.43 & -0.17 & 0.13 & -5.28 & 3.1 & 0.1 & 3.7 & -22.2 & 45 & 0.03 & 0.03 & 1 \\
4123 & KOI-4335 & 19 25 37.9 & +48 01 04 & 5849 & 4.43 & -0.27 & 0.15 & -5.05 & 3.5 & 0.1 & 3.8 & -38.1 & 49 & 0.02 & 0.02 & 1 \\
4124 & KOI-4024 & 18 55 08.9 & +48 01 46 & 5202 & 4.50 & -0.08 & 0.35 & -4.60 & 4.5 & 3.9 & 2.0 & -39.5 & 47 & 0.03 & 0.03 & 1 \\
4125 & KOI-209 & 19 15 10.3 & +48 02 25 & 6067 & 4.11 & 0.03 & 0.14 & -5.14 & 9.0 & 6.8 & 5.1 & -13.8 & 47 & 0.03 & 0.03 & 1 \\
4126 & KOI-1305 & 19 25 33.8 & +48 03 56 & 5231 & 4.55 & 0.09 & 0.22 & -4.85 & 2.1 & 0.1 & 2.1 & 6.8 & 38 & 0.03 & 0.03 & 1 \\
4127 & KOI-3 & 19 50 50.3 & +48 04 51 & 4763 & 4.47 & 0.29 & 0.50 & -4.58 & 2.6 & 2.0 & 1.6 & -63.7 & 57 & 0.03 & 0.03 & 1 \\
4128 & KOI-3889 & 19 30 28.7 & +48 04 53 & 5767 & 4.31 & 0.17 & 0.18 & -4.87 & 3.6 & 0.8 & 3.5 & -90.1 & 49 & 0.02 & 0.02 & 1 \\
4129 & KOI-1311 & 18 54 07.9 & +48 05 39 & 6385 & 4.89 & 0.06 & 0.12 & -5.35 & 4.4 & 0.1 & 8.3 & -5.3 & 48 & 0.46 & 0.06 & 1 \\
4130 & KOI-1639 & 19 51 36.1 & +48 05 41 & 6089 & 3.82 & 0.13 & 0.12 & -5.47 & 7.4 & 4.0 & 6.1 & -31.3 & 47 & 0.03 & 0.03 & 1 \\
4131 & KOI-2236 & 19 14 28.3 & +48 05 54 & 5504 & 4.47 & -0.07 & 0.15 & -5.10 & 2.7 & 0.1 & 2.6 & -24.8 & 33 & 0.03 & 0.04 & 1 \\
4132 & KOI-1316 & 19 22 12.6 & +48 07 35 & 5769 & 3.99 & 0.26 & 0.13 & -5.23 & 5.1 & 2.3 & 4.4 & -55.6 & 50 & 0.02 & 0.03 & 1 \\
4133 & KOI-1989 & 18 52 27.3 & +48 07 53 & 5669 & 4.54 & -0.01 & 0.18 & -4.89 & 3.7 & 2.0 & 3.1 & -7.5 & 46 & 0.03 & 0.03 & 1 \\
4134 & KOI-752 & 19 27 44.2 & +48 08 30 & 5518 & 4.49 & 0.03 & 0.12 & -5.36 & 3.0 & 1.2 & 2.6 & -33.1 & 33 & 0.04 & 0.04 & 1 \\
4135 & KOI-3451 & 19 21 22.7 & +48 08 50 & 5950 & 4.37 & -0.01 & 0.11 & -5.60 & 4.9 & 2.0 & 4.4 & -15.3 & 41 & 0.03 & 0.03 & 1 \\
4136 & KOI-3925 & 19 12 39.0 & +48 09 54 & 5280 & 4.54 & -0.03 & 0.77 & -4.17 & 3.7 & 2.9 & 2.2 & -38.2 & 43 & 0.03 & 0.03 & 1 \\
4137 & KOI-3683 & 19 23 53.8 & +48 10 41 & 6313 & 4.08 & -0.01 & 0.12 & -5.42 & 12.9 & 9.5 & 7.4 & -36.4 & 49 & 0.02 & 0.03 & 1 \\
4138 & KOI-4235 & 19 23 41.5 & +48 10 49 & 6226 & 4.10 & 0.07 & 0.14 & -5.07 & 16.7 & 13.4 & 6.5 & -26.8 & 47 & 0.02 & 0.03 & 1 \\
4139 & KOI-2228 & 19 33 40.3 & +48 11 56 & 6544 & 3.85 & -0.07 & 0.14 & -5.12 & 15.9 & 8.0 & 13.3 & -16.0 & 46 & 0.03 & 0.03 & 1 \\
4140 & KOI-117 & 19 48 06.8 & +48 12 31 & 5788 & 4.14 & 0.27 & 0.14 & -5.18 & 4.6 & 2.8 & 3.5 & 1.5 & 49 & 0.02 & 0.03 & 1 \\
4141 & Kepler-107 & 19 48 06.8 & +48 12 31 & 5800 & 4.13 & 0.27 & 0.13 & -5.27 & 4.9 & 3.2 & 3.6 & 3.1 & 87 & 0.02 & 0.02 & 1 \\
4142 & KOI-3602 & 18 54 12.6 & +48 13 23 & 6158 & 4.86 & -0.16 & 0.13 & -5.18 & 4.5 & 0.1 & 5.8 & -17.6 & 49 & 0.03 & 0.04 & 1 \\
4143 & KOI-756 & 19 45 08.7 & +48 13 29 & 5581 & 4.21 & 0.09 & 0.21 & -4.80 & 4.1 & 2.9 & 2.8 & -63.8 & 23 & 0.06 & 0.06 & 1 \\
4144 & KOI-2960 & 19 49 16.2 & +48 14 22 & 5943 & 4.24 & 0.08 & 0.12 & -5.36 & 4.8 & 2.0 & 4.3 & -43.2 & 48 & 0.02 & 0.03 & 1 \\
4145 & KOI-341 & 19 51 50.8 & +48 14 40 & 5485 & 4.52 & 0.08 & 0.25 & -4.72 & 3.5 & 2.3 & 2.6 & -29.1 & 50 & 0.02 & 0.02 & 1 \\
4146 & KOI-2075 & 19 20 24.5 & +48 15 04 & 6146 & 4.38 & -0.03 & 0.10 & -6.51 & 6.9 & 3.5 & 5.7 & 3.3 & 48 & 0.03 & 0.03 & 1 \\
4147 & KOI-431 & 18 49 50.5 & +48 15 26 & 5170 & 4.69 & -0.29 & 0.18 & -4.98 & 1.7 & 0.1 & 2.0 & 19.3 & 33 & 0.04 & 0.04 & 1 \\
4148 & KOI-1299 & 19 33 07.7 & +48 17 09 & 4926 & 3.33 & 0.06 & 0.16 & -5.02 & 3.2 & 0.1 & 3.4 & -35.5 & 65 & 0.02 & 0.02 & 1 \\
4149 & KOI-1306 & 19 22 42.3 & +48 17 39 & 5677 & 4.52 & -0.28 & 0.24 & -4.69 & 3.2 & 0.2 & 3.1 & 11.7 & 25 & 0.05 & 0.05 & 1 \\
4150 & KOI-3146 & 19 01 23.3 & +48 18 44 & 5625 & 4.02 & 0.14 & 0.29 & -4.59 & 3.9 & 2.5 & 3.0 & -74.0 & 49 & 0.02 & 0.02 & 1 \\
4151 & KOI-291 & 19 49 06.7 & +48 19 13 & 5663 & 4.13 & 0.23 & 0.14 & -5.19 & 5.1 & 3.9 & 3.1 & 5.2 & 50 & 0.02 & 0.02 & 1 \\
4152 & KOI-2623 & 19 20 06.2 & +48 20 09 & 6137 & 4.08 & 0.13 & 0.13 & -5.19 & 8.9 & 6.3 & 5.7 & -41.9 & 48 & 0.03 & 0.03 & 1 \\
4153 & KOI-46 & 18 53 01.3 & +48 21 19 & 5535 & 4.01 & 0.31 & 0.19 & -4.90 & 3.8 & 2.7 & 2.7 & -79.5 & 51 & 0.02 & 0.03 & 1 \\
4154 & KOI-1963 & 19 22 25.8 & +48 21 26 & 5947 & 4.29 & 0.18 & 0.27 & -4.67 & 12.6 & 9.9 & 4.3 & -36.3 & 27 & 0.08 & 0.09 & 2 \\
4155 & KOI-2754 & 18 54 59.0 & +48 22 24 & 5865 & 4.34 & -0.14 & 0.10 & -5.90 & 5.0 & 3.0 & 3.9 & -50.3 & 49 & 0.02 & 0.03 & 1 \\
4156 & KOI-757 & 19 07 59.9 & +48 22 33 & 4939 & 4.59 & -0.01 & 0.40 & -4.62 & 2.1 & 0.9 & 1.7 & 6.3 & 26 & 0.05 & 0.09 & 1 \\
4157 & KOI-601 & 19 23 23.8 & +48 24 58 & 5790 & 4.57 & 0.04 & 0.24 & -4.67 & 5.6 & 4.2 & 3.6 & 2.3 & 31 & 0.04 & 0.04 & 1 \\
4158 & KOI-1307 & 19 23 42.6 & +48 26 37 & 5503 & 4.49 & 0.03 & 0.13 & -5.24 & 2.9 & 1.2 & 2.6 & -16.3 & 32 & 0.04 & 0.10 & 1 \\
4159 & KOI-4374 & 19 52 44.0 & +48 26 38 & 5387 & 4.45 & -0.02 & 0.17 & -5.00 & 3.0 & 1.6 & 2.3 & -14.2 & 49 & 0.02 & 0.02 & 1 \\
4160 & KOI-1931 & 19 33 24.4 & +48 26 41 & 5366 & 4.52 & -0.10 & 0.23 & -4.79 & 3.6 & 2.6 & 2.3 & -16.9 & 41 & 0.03 & 0.03 & 1 \\
4161 & KOI-343 & 19 40 28.5 & +48 28 53 & 5769 & 4.36 & 0.02 & 0.18 & -4.89 & 4.0 & 1.8 & 3.5 & -48.4 & 48 & 0.02 & 0.03 & 1 \\
4162 & Kepler-142 & 19 40 28.5 & +48 28 53 & 5713 & 4.19 & -0.02 & 0.14 & -5.11 & 4.3 & 2.7 & 3.3 & -49.3 & 81 & 0.02 & 0.06 & 1 \\
4163 & KOI-112 & 19 42 35.7 & +48 29 44 & 5888 & 4.39 & -0.04 & 0.17 & -4.93 & 4.6 & 2.1 & 4.0 & -3.0 & 48 & 0.02 & 0.03 & 1 \\
4164 & KOI-759 & 19 02 52.5 & +48 30 21 & 5207 & 4.51 & -0.26 & 0.14 & -5.15 & 2.3 & 0.7 & 2.0 & -2.3 & 37 & 0.03 & 0.03 & 1 \\
4165 & KOI-3060 & 19 06 19.3 & +48 32 39 & 6208 & 4.04 & -0.02 & 0.14 & -5.13 & 7.9 & 4.6 & 6.3 & -52.3 & 49 & 0.04 & 0.05 & 1 \\
4166 & KOI-344 & 18 53 21.7 & +48 32 57 & 5629 & 4.53 & -0.27 & 0.16 & -5.01 & 2.6 & 0.1 & 3.0 & 10.8 & 49 & 0.02 & 0.02 & 1 \\
4167 & KOI-479 & 18 54 01.8 & +48 33 09 & 5552 & 4.47 & -0.16 & 0.15 & -5.09 & 2.9 & 0.4 & 2.7 & -54.5 & 48 & 0.02 & 0.05 & 1 \\
4168 & KOI-1645 & 19 52 50.6 & +48 33 33 & 5419 & 4.76 & -0.28 & 0.22 & -4.81 & 4.5 & 3.6 & 2.4 & -26.1 & 51 & 0.04 & 0.05 & 1 \\
4169 & KOI-1800 & 19 01 04.5 & +48 33 36 & 5503 & 4.50 & -0.04 & 0.40 & -4.42 & 8.3 & 7.3 & 2.6 & 0.7 & 51 & 0.02 & 0.03 & 1 \\
4170 & KOI-1444 & 19 49 34.0 & +48 33 38 & 6036 & 3.83 & 0.09 & 0.09 & nan & 10.4 & 7.8 & 5.7 & -19.6 & 40 & 0.03 & 0.04 & 1 \\
4171 & Kepler-299 & 18 52 49.7 & +48 34 50 & 5645 & 4.40 & 0.03 & 0.00 & 0.00 & 3.7 & 2.1 & 3.0 & 10.4 & 37 & 0.09 & 0.06 & 1 \\
4172 & KOI-124 & 19 31 43.0 & +48 36 10 & 5970 & 4.23 & -0.09 & 0.12 & -5.30 & 5.0 & 2.1 & 4.5 & -1.4 & 47 & 0.02 & 0.03 & 1 \\
4173 & KOI-1889 & 19 05 05.7 & +48 37 07 & 5399 & 4.60 & -0.08 & 0.20 & -4.87 & 3.3 & 2.2 & 2.4 & 3.0 & 34 & 0.03 & 0.05 & 1 \\
4174 & KOI-2007 & 18 51 42.0 & +48 37 35 & 5863 & 4.48 & 0.10 & 0.19 & -4.86 & 4.5 & 2.2 & 3.9 & -23.0 & 49 & 0.02 & 0.03 & 1 \\
4175 & KOI-2977 & 19 39 27.9 & +48 38 20 & 5915 & 4.13 & -0.08 & 0.13 & -5.30 & 4.7 & 1.9 & 4.2 & -32.9 & 47 & 0.02 & 0.03 & 2 \\
4176 & KOI-2885 & 19 55 03.4 & +48 38 42 & 5615 & 4.05 & -0.37 & 0.12 & -5.39 & 3.6 & 1.9 & 2.9 & -26.2 & 48 & 0.02 & 0.04 & 1 \\
4177 & KOI-2533 & 19 06 51.8 & +48 38 43 & 4941 & 3.52 & 0.01 & 0.14 & -5.16 & 3.5 & 0.7 & 3.4 & 12.1 & 53 & 0.02 & 0.02 & 1 \\
4178 & KOI-4287 & 19 21 50.0 & +48 39 41 & 6204 & 4.11 & -0.00 & 0.13 & -5.20 & 10.4 & 7.6 & 6.3 & -33.1 & 49 & 0.02 & 0.03 & 1 \\
4179 & KOI-2442 & 19 19 26.1 & +48 41 38 & 4968 & 4.47 & 0.03 & 0.29 & -4.77 & 2.4 & 1.6 & 1.8 & -13.5 & 26 & 0.05 & 0.06 & 1 \\
4180 & KOI-2712 & 19 50 59.3 & +48 41 39 & 6198 & 4.05 & 0.23 & 0.15 & -5.00 & 15.6 & 12.6 & 6.2 & -23.4 & 49 & 0.03 & 0.03 & 1 \\
4181 & KOI-2805 & 19 22 46.5 & +48 42 05 & 5880 & 4.22 & -0.23 & 0.09 & nan & 4.2 & 1.4 & 4.0 & -43.5 & 48 & 0.02 & 0.02 & 1 \\
4182 & KOI-276 & 19 18 39.5 & +48 42 22 & 5956 & 4.30 & -0.03 & 0.13 & -5.24 & 4.5 & 0.7 & 4.4 & -21.0 & 49 & 0.02 & 0.02 & 1 \\
4183 & KOI-1863 & 19 02 40.1 & +48 43 10 & 5511 & 4.91 & 0.02 & 0.18 & -4.95 & 6.2 & 5.2 & 2.6 & -22.0 & 48 & 0.16 & 0.06 & 1 \\
4184 & KOI-3371 & 19 01 15.3 & +48 43 31 & 5358 & 4.40 & -0.12 & 0.23 & -4.80 & 3.4 & 2.5 & 2.3 & -30.9 & 52 & 0.02 & 0.03 & 1 \\
4185 & KOI-2792 & 19 05 21.2 & +48 44 39 & 5895 & 4.23 & 0.17 & 0.10 & -5.87 & 5.6 & 3.7 & 4.1 & -32.2 & 50 & 0.02 & 0.02 & 1 \\
4186 & KOI-2333 & 18 49 34.7 & +48 45 33 & 6090 & 4.31 & -0.11 & 0.13 & -5.26 & 5.6 & 1.6 & 5.3 & -11.6 & 47 & 0.02 & 0.03 & 1 \\
4187 & KOI-1647 & 19 53 10.8 & +48 46 32 & 5670 & 4.23 & 0.21 & 0.11 & -5.54 & 4.9 & 3.6 & 3.1 & -38.2 & 48 & 0.02 & 0.03 & 1 \\
4188 & KOI-1426 & 18 52 50.2 & +48 46 40 & 5710 & 4.51 & -0.18 & 0.14 & -5.16 & 3.5 & 1.0 & 3.2 & -11.5 & 45 & 0.03 & 0.03 & 1 \\
4189 & KOI-1438 & 19 33 09.2 & +48 48 42 & 5632 & 3.91 & 0.11 & 0.14 & -5.18 & 5.2 & 3.1 & 4.1 & -40.1 & 46 & 0.03 & 0.03 & 1 \\
4190 & KOI-2813 & 19 41 22.1 & +48 51 22 & 4738 & 2.76 & -0.39 & 0.12 & -5.32 & 4.7 & 2.2 & 4.0 & -15.0 & 48 & 0.03 & 0.05 & 1 \\
4191 & KOI-481 & 19 32 38.4 & +48 52 52 & 5163 & 4.60 & -0.13 & 0.16 & -5.05 & 1.6 & 0.1 & 2.0 & -30.8 & 36 & 0.03 & 0.03 & 1 \\
4192 & KOI-2765 & 19 22 33.0 & +48 53 00 & 6129 & 3.94 & 0.12 & 0.11 & -5.54 & 5.4 & 0.1 & 6.4 & 1.0 & 49 & 0.03 & 0.05 & 1 \\
4193 & KOI-4653 & 19 06 14.5 & +48 53 35 & 6094 & 4.10 & 0.02 & 0.12 & -5.41 & 9.3 & 6.9 & 5.3 & -45.9 & 48 & 0.02 & 0.03 & 1 \\
4194 & KOI-294 & 19 53 04.6 & +48 55 00 & 6062 & 4.39 & 0.08 & 0.10 & -5.90 & 6.1 & 3.2 & 5.1 & -27.7 & 48 & 0.02 & 0.03 & 1 \\
4195 & KOI-2796 & 19 31 29.8 & +48 56 12 & 5745 & 4.44 & -0.03 & 0.15 & -5.08 & 3.6 & 1.1 & 3.4 & 16.2 & 31 & 0.04 & 0.04 & 1 \\
4196 & KOI-3103 & 19 13 07.2 & +48 57 02 & 5856 & 4.29 & 0.25 & 0.14 & -5.19 & 4.9 & 2.9 & 3.9 & -14.7 & 42 & 0.03 & 0.03 & 1 \\
4197 & KOI-2672 & 19 44 31.9 & +48 58 39 & 5561 & 4.51 & 0.06 & 0.32 & -4.53 & 4.7 & 3.7 & 2.8 & -14.8 & 80 & 0.02 & 0.02 & 2 \\
4198 & KOI-107 & 19 39 20.4 & +48 58 56 & 5853 & 4.07 & 0.22 & 0.12 & -5.36 & 5.3 & 3.5 & 3.8 & -52.5 & 48 & 0.02 & 0.03 & 1 \\
4199 & KOI-3346 & 19 22 32.8 & +48 59 46 & 5916 & 4.33 & -0.03 & 0.13 & -5.20 & 4.7 & 2.1 & 4.2 & -39.7 & 48 & 0.02 & 0.03 & 1 \\
4200 & KOI-1857 & 19 28 03.2 & +49 01 09 & 5738 & 4.36 & -0.10 & 0.17 & -4.97 & 4.6 & 3.0 & 3.3 & -32.1 & 45 & 0.03 & 0.03 & 1 \\
4201 & KOI-4716 & 19 13 22.8 & +49 01 19 & 5952 & 4.11 & 0.02 & 0.36 & -4.38 & 6.2 & 4.2 & 4.4 & -78.6 & 48 & 0.02 & 0.03 & 1 \\
4202 & KOI-246 & 19 24 07.8 & +49 02 25 & 5821 & 4.30 & 0.14 & 0.10 & -5.78 & 4.1 & 1.6 & 3.7 & -21.2 & 50 & 0.02 & 0.02 & 1 \\
4203 & KOI-1802 & 19 30 07.4 & +49 03 42 & 5900 & 4.47 & -0.01 & 0.22 & -4.72 & 4.9 & 2.6 & 4.1 & -8.4 & 42 & 0.03 & 0.03 & 1 \\
4204 & KOI-241 & 19 07 00.7 & +49 03 54 & 4991 & 4.57 & -0.34 & 0.10 & -5.41 & 1.9 & 0.1 & 1.8 & -69.5 & 45 & 0.03 & 0.03 & 1 \\
4205 & Kepler-124 & 19 07 00.7 & +49 03 54 & 4978 & 4.53 & -0.38 & 0.00 & 0.00 & 2.4 & 1.4 & 1.8 & -68.0 & 63 & 0.02 & 0.04 & 1 \\
4206 & KOI-2168 & 19 47 24.5 & +49 05 04 & 5866 & 4.21 & -0.10 & 0.19 & -4.83 & 5.4 & 3.6 & 3.9 & -45.8 & 28 & 0.04 & 0.06 & 1 \\
4207 & KOI-2422 & 19 46 12.0 & +49 06 08 & 5192 & 4.58 & -0.07 & 0.18 & -4.99 & 2.2 & 0.5 & 2.0 & 20.9 & 30 & 0.04 & 0.04 & 1 \\
4208 & KOI-2632 & 18 57 41.5 & +49 06 22 & 6136 & 3.84 & -0.04 & 0.16 & -4.99 & 12.2 & 9.3 & 6.5 & -33.2 & 48 & 0.02 & 0.03 & 1 \\
4209 & Kepler-15 & 19 44 48.1 & +49 08 24 & 5619 & 4.22 & 0.20 & 0.00 & 0.00 & 4.2 & 2.9 & 2.9 & -19.4 & 68 & 0.06 & 0.03 & 1 \\
4210 & KOI-128 & 19 44 48.1 & +49 08 24 & 5615 & 4.20 & 0.21 & 0.10 & -5.79 & 4.1 & 2.8 & 2.9 & -19.6 & 49 & 0.02 & 0.03 & 1 \\
4211 & KOI-2366 & 19 10 20.4 & +49 09 17 & 6143 & 4.24 & 0.03 & 0.13 & -5.27 & 8.2 & 5.5 & 5.7 & -31.2 & 47 & 0.02 & 0.03 & 1 \\
4212 & KOI-330 & 19 47 26.2 & +49 09 43 & 5822 & 4.07 & -0.01 & 0.12 & -5.42 & 5.0 & 3.2 & 3.7 & -46.3 & 41 & 0.03 & 0.03 & 1 \\
4213 & KOI-3782 & 19 40 20.9 & +49 10 12 & 4918 & 4.44 & 0.04 & 0.50 & -4.52 & 4.6 & 4.0 & 1.7 & -11.4 & 56 & 0.02 & 0.03 & 1 \\
4214 & KOI-2639 & 19 01 27.6 & +49 12 06 & 5720 & 4.27 & 0.03 & 0.11 & -5.56 & 3.8 & 1.8 & 3.3 & -37.9 & 32 & 0.04 & 0.05 & 1 \\
4215 & KOI-3015 & 19 28 43.2 & +49 12 09 & 5770 & 4.11 & -0.07 & 0.10 & -5.88 & 4.1 & 2.1 & 3.5 & -4.7 & 49 & 0.02 & 0.02 & 1 \\
4216 & KOI-1428 & 19 23 49.8 & +49 12 14 & 4734 & 4.50 & -0.15 & 0.25 & -4.94 & 1.7 & 0.2 & 1.6 & 7.8 & 32 & 0.04 & 0.04 & 1 \\
4217 & KOI-4036 & 19 49 08.4 & +49 12 45 & 4776 & 4.48 & -0.04 & 0.76 & -4.39 & 2.7 & 2.1 & 1.6 & -21.4 & 49 & 0.03 & 0.03 & 1 \\
4218 & KOI-1436 & 18 55 55.9 & +49 13 59 & 5609 & 4.47 & 0.11 & 0.19 & -4.88 & 3.5 & 1.9 & 2.9 & -13.6 & 35 & 0.03 & 0.04 & 1 \\
4219 & Kepler-301 & 18 55 55.9 & +49 13 59 & 5625 & 4.53 & 0.06 & 0.00 & 0.00 & 3.8 & 2.3 & 2.9 & -11.8 & 57 & 0.03 & 0.07 & 1 \\
4220 & KOI-2143 & 19 28 20.3 & +49 14 15 & 5385 & 4.39 & 0.11 & 0.39 & -4.48 & 3.2 & 2.2 & 2.3 & -28.4 & 51 & 0.03 & 0.07 & 1 \\
4221 & KOI-2195 & 19 25 01.5 & +49 15 32 & 6032 & 4.07 & -0.13 & 0.11 & -5.74 & 6.7 & 4.4 & 4.9 & -29.1 & 31 & 0.08 & 0.05 & 1 \\
4222 & KOI-349 & 19 07 24.6 & +49 15 42 & 5694 & 4.29 & 0.26 & 0.12 & -5.41 & 5.2 & 4.0 & 3.2 & 2.0 & 50 & 0.02 & 0.03 & 1 \\
4223 & KOI-350 & 19 11 26.7 & +49 15 52 & 5790 & 4.49 & 0.02 & 0.11 & -5.46 & 3.6 & 0.4 & 3.6 & -30.1 & 49 & 0.02 & 0.02 & 1 \\
4224 & KOI-1623 & 19 03 37.5 & +49 17 15 & 5732 & 4.16 & 0.02 & 0.13 & -5.23 & 4.1 & 2.0 & 3.3 & 6.1 & 49 & 0.02 & 0.02 & 2 \\
4225 & KOI-351 & 18 57 44.0 & +49 18 19 & 6020 & 4.31 & 0.12 & 0.13 & nan & 5.8 & 3.1 & 4.8 & -19.9 & 67 & 0.02 & 0.02 & 2 \\
4226 & KOI-1992 & 19 16 47.9 & +49 18 21 & 5851 & 4.23 & -0.10 & 0.24 & -4.65 & 3.3 & 0.1 & 3.8 & -67.6 & 32 & 0.04 & 0.05 & 1 \\
4227 & KOI-2047 & 19 32 46.9 & +49 19 00 & 6103 & 4.32 & -0.04 & 0.10 & -5.91 & 7.0 & 4.2 & 5.4 & -44.7 & 47 & 0.02 & 0.03 & 1 \\
4228 & KOI-2771 & 19 29 59.5 & +49 19 44 & 6211 & 4.40 & -0.01 & 0.21 & -4.72 & 6.3 & 0.4 & 6.3 & -16.3 & 50 & 0.02 & 0.03 & 1 \\
4229 & KOI-2110 & 19 37 52.5 & +49 19 52 & 6165 & 4.06 & 0.11 & 0.09 & nan & 19.7 & 16.2 & 5.9 & -33.4 & 47 & 0.03 & 0.03 & 1 \\
4230 & KOI-5900 & 19 24 34.9 & +49 21 55 & 6249 & 4.15 & -0.10 & 0.11 & -5.59 & 15.4 & 12.2 & 6.7 & 0.4 & 47 & 0.02 & 0.07 & 1 \\
4231 & KOI-2399 & 19 39 33.5 & +49 22 47 & 4983 & 4.40 & -0.11 & 0.19 & -4.98 & 2.3 & 1.2 & 1.8 & -18.5 & 52 & 0.02 & 0.08 & 1 \\
4232 & KOI-352 & 19 52 16.3 & +49 24 45 & 5835 & 4.27 & -0.06 & 0.11 & -5.51 & 3.8 & 0.4 & 3.8 & -34.2 & 49 & 0.02 & 0.08 & 1 \\
4233 & KOI-2109 & 19 09 31.7 & +49 27 09 & 6035 & 4.09 & 0.02 & 0.14 & -5.10 & 8.7 & 6.6 & 4.9 & -42.9 & 42 & 0.03 & 0.03 & 1 \\
4234 & KOI-3419 & 19 48 09.5 & +49 28 09 & 6521 & 4.19 & -0.25 & 0.15 & -5.05 & 7.6 & 0.1 & 10.4 & -55.7 & 48 & 0.03 & 0.06 & 1 \\
4235 & KOI-168 & 19 36 52.5 & +49 28 45 & 5827 & 4.04 & -0.10 & 0.12 & -5.37 & 4.1 & 1.5 & 3.7 & -27.4 & 53 & 0.02 & 0.03 & 2 \\
4236 & KOI-1856 & 19 48 18.9 & +49 30 07 & 5198 & 4.50 & -0.05 & 0.30 & -4.68 & 3.0 & 2.1 & 2.0 & -23.8 & 49 & 0.02 & 0.03 & 1 \\
4237 & KOI-1655 & 18 58 55.6 & +49 32 00 & 5553 & 4.50 & -0.14 & 0.15 & -5.10 & 2.8 & 0.1 & 2.7 & 20.6 & 48 & 0.02 & 0.02 & 1 \\
4238 & KOI-354 & 19 45 40.5 & +49 32 24 & 5940 & 4.51 & 0.04 & 0.16 & -4.96 & 4.2 & 0.1 & 4.3 & -36.0 & 49 & 0.02 & 0.03 & 1 \\
4239 & KOI-2365 & 19 31 14.1 & +49 34 46 & 5913 & 4.19 & 0.19 & 0.10 & -6.12 & 5.3 & 3.1 & 4.2 & -28.6 & 49 & 0.02 & 0.03 & 1 \\
4240 & KOI-2837 & 19 40 36.5 & +49 35 15 & 6539 & 4.09 & -0.08 & 0.14 & -5.14 & 24.8 & 19.3 & 10.7 & -9.0 & 46 & 0.03 & 0.03 & 1 \\
4241 & KOI-3109 & 19 50 34.1 & +49 35 42 & 6162 & 3.90 & 0.06 & 0.14 & -5.17 & 20.8 & 16.9 & 6.7 & 3.8 & 48 & 0.03 & 0.03 & 1 \\
4242 & KOI-295 & 18 58 57.4 & +49 35 54 & 5957 & 4.45 & -0.15 & 0.15 & -5.07 & 4.5 & 0.4 & 4.4 & -30.9 & 47 & 0.02 & 0.03 & 1 \\
4243 & KOI-4792 & 19 42 17.2 & +49 36 27 & 5925 & 4.47 & 0.07 & 0.15 & -5.07 & 4.6 & 1.7 & 4.2 & -22.2 & 48 & 0.02 & 0.02 & 1 \\
4244 & KOI-356 & 19 50 56.7 & +49 38 14 & 5405 & 4.43 & -0.05 & 0.11 & -5.42 & 3.3 & 2.1 & 2.4 & -15.0 & 51 & 0.02 & 0.02 & 1 \\
4245 & KOI-1831 & 19 05 53.2 & +49 38 56 & 5148 & 4.45 & 0.11 & 0.20 & -4.91 & 3.0 & 2.1 & 2.0 & -71.0 & 51 & 0.02 & 0.03 & 1 \\
4246 & KOI-4304 & 19 30 42.7 & +49 39 50 & 5912 & 4.20 & 0.13 & 0.19 & -4.84 & 5.1 & 2.9 & 4.2 & -37.5 & 49 & 0.03 & 0.03 & 1 \\
4247 & KOI-355 & 19 46 16.0 & +49 41 47 & 6040 & 4.24 & 0.18 & 0.31 & -4.45 & 6.5 & 4.1 & 4.9 & 8.6 & 47 & 0.02 & 0.03 & 1 \\
4248 & KOI-3363 & 19 02 50.9 & +49 42 24 & 5809 & 4.43 & -0.02 & 0.17 & -4.93 & 3.4 & 0.1 & 3.6 & -100.2 & 49 & 0.03 & 0.04 & 1 \\
4249 & KOI-167 & 19 37 51.3 & +49 45 54 & 6193 & 4.10 & 0.10 & 0.12 & -5.39 & 4.8 & 0.1 & 6.2 & -22.7 & 47 & 0.03 & 0.03 & 1 \\
4250 & KOI-1945 & 19 16 07.1 & +49 46 11 & 5258 & 4.42 & 0.16 & 0.34 & -4.59 & 2.7 & 1.6 & 2.1 & -5.6 & 37 & 0.03 & 0.03 & 1 \\
4251 & KOI-1894 & 19 49 26.2 & +49 47 51 & 4922 & 3.43 & 0.14 & 0.10 & -5.40 & 3.3 & 0.1 & 3.4 & -42.1 & 55 & 0.02 & 0.04 & 1 \\
4252 & KOI-1832 & 19 19 20.5 & +49 49 32 & 5466 & 4.78 & -0.09 & 0.24 & -4.72 & 4.1 & 3.1 & 2.5 & -20.1 & 28 & 0.06 & 0.05 & 1 \\
4253 & KOI-1841 & 19 20 39.7 & +49 55 26 & 5124 & 4.53 & -0.02 & 0.22 & -4.86 & 2.8 & 1.9 & 1.9 & -23.4 & 50 & 0.02 & 0.03 & 1 \\
4254 & KOI-2582 & 19 43 23.2 & +49 56 10 & 5851 & 4.28 & 0.29 & 0.11 & -5.51 & 4.9 & 2.9 & 3.8 & -32.9 & 50 & 0.02 & 0.02 & 1 \\
4255 & KOI-620 & 19 45 55.1 & +49 56 16 & 5574 & 4.60 & -0.11 & 0.14 & -5.18 & 6.4 & 5.4 & 2.8 & -5.4 & 33 & 0.04 & 0.04 & 1 \\
4256 & KOI-3403 & 19 06 35.1 & +49 56 16 & 5752 & 3.94 & 0.09 & 0.11 & -5.55 & 5.3 & 2.9 & 4.4 & -10.6 & 49 & 0.03 & 0.02 & 1 \\
4257 & KOI-1883 & 19 16 56.0 & +49 56 20 & 6031 & 4.16 & 0.06 & 0.14 & -5.12 & 8.1 & 6.0 & 4.9 & -31.9 & 50 & 0.03 & 0.05 & 1 \\
4258 & KOI-3892 & 19 22 14.3 & +49 56 35 & 5545 & 4.24 & 0.22 & 0.15 & -5.09 & 4.2 & 3.1 & 2.7 & -20.6 & 51 & 0.24 & 0.05 & 1 \\
4259 & KOI-1980 & 19 40 43.6 & +49 56 45 & 5425 & 4.52 & 0.09 & 0.20 & -4.86 & 3.6 & 2.6 & 2.4 & -41.8 & 47 & 0.03 & 0.03 & 1 \\
4260 & KOI-2173 & 19 49 10.2 & +49 58 54 & 4725 & 4.51 & 0.06 & 0.93 & -4.32 & 2.9 & 2.4 & 1.6 & -24.4 & 55 & 0.02 & 0.03 & 1 \\
4261 & KOI-2492 & 19 01 37.2 & +49 59 41 & 5832 & 4.64 & -0.29 & 0.16 & -4.99 & 3.0 & 0.1 & 3.7 & -62.9 & 48 & 0.02 & 0.03 & 1 \\
4262 & KOI-2260 & 19 20 56.6 & +50 01 48 & 6116 & 4.16 & -0.01 & 0.09 & nan & 9.7 & 7.3 & 5.5 & -45.6 & 48 & 0.02 & 0.03 & 1 \\
4263 & KOI-296 & 19 00 10.0 & +50 04 31 & 5818 & 4.42 & -0.15 & 0.15 & -5.09 & 3.6 & 0.1 & 3.7 & -11.4 & 48 & 0.02 & 0.03 & 1 \\
4264 & KOI-2581 & 19 37 24.2 & +50 04 52 & 5401 & 4.45 & 0.19 & 0.12 & -5.28 & 3.6 & 2.6 & 2.4 & -0.9 & 50 & 0.02 & 0.02 & 1 \\
4265 & KOI-543 & 19 44 36.3 & +50 05 45 & 5102 & 4.49 & -0.08 & 0.20 & -4.94 & 2.6 & 1.6 & 1.9 & -43.6 & 37 & 0.03 & 0.04 & 1 \\
4266 & KOI-4062 & 19 15 38.1 & +50 09 46 & 6006 & 4.15 & 0.02 & 0.07 & nan & 6.0 & 3.5 & 4.7 & -10.8 & 40 & 0.03 & 0.03 & 1 \\
4267 & KOI-3875 & 19 20 35.8 & +50 14 21 & 6200 & 4.61 & -0.60 & 0.22 & -4.66 & 11.1 & 7.9 & 6.2 & 10.5 & 49 & 0.04 & 0.06 & 1 \\
4268 & KOI-72 & 19 02 43.1 & +50 14 29 & 5646 & 4.33 & -0.15 & 0.17 & -4.94 & 3.6 & 1.8 & 3.0 & -98.8 & 47 & 0.03 & 0.03 & 1 \\
4269 & KOI-297 & 19 04 59.3 & +50 14 33 & 6087 & 4.20 & 0.13 & 0.14 & -5.16 & 8.9 & 6.5 & 5.3 & -13.6 & 42 & 0.03 & 0.03 & 1 \\
4270 & KOI-2026 & 19 44 55.2 & +50 16 31 & 6041 & 4.51 & -0.07 & 0.18 & -4.85 & 6.1 & 3.3 & 4.9 & -8.0 & 48 & 0.02 & 0.03 & 1 \\
4271 & KOI-2433 & 19 37 21.2 & +50 20 12 & 5864 & 4.23 & -0.00 & 0.08 & nan & 4.4 & 2.0 & 3.9 & -2.8 & 25 & 0.05 & 0.05 & 1 \\
4272 & KOI-4011 & 19 40 12.8 & +50 20 52 & 5914 & 4.32 & 0.16 & 0.11 & -5.62 & 5.4 & 3.3 & 4.2 & -22.6 & 50 & 0.04 & 0.10 & 1 \\
4273 & KOI-4129 & 19 42 07.1 & +50 22 13 & 5039 & 4.51 & 0.12 & 0.23 & -4.87 & 2.3 & 1.1 & 1.8 & -49.4 & 53 & 0.02 & 0.03 & 1 \\
4274 & KOI-4021 & 19 36 08.2 & +50 22 18 & 6336 & 4.29 & 0.01 & 0.10 & -5.82 & 23.6 & 19.1 & 7.7 & -7.2 & 47 & 0.03 & 0.03 & 1 \\
4275 & KOI-2590 & 19 34 01.7 & +50 27 00 & 6068 & 3.77 & -0.00 & 0.11 & -5.68 & 12.3 & 9.6 & 5.9 & -2.6 & 47 & 0.03 & 0.03 & 1 \\
4276 & KOI-2729 & 19 16 15.6 & +50 27 40 & 5798 & 4.58 & -0.25 & 0.11 & -5.59 & 3.3 & 0.1 & 3.6 & -3.2 & 49 & 0.03 & 0.03 & 1 \\
4277 & KOI-3194 & 19 06 30.9 & +50 28 17 & 6247 & 4.06 & 0.21 & 0.13 & -5.20 & 8.7 & 5.2 & 6.7 & -45.0 & 47 & 0.02 & 0.03 & 1 \\
4278 & Kepler-197 & 19 40 54.4 & +50 33 32 & 6059 & 4.33 & -0.38 & 0.13 & -5.24 & 4.6 & 0.1 & 5.1 & 0.7 & 108 & 0.02 & 0.02 & 1 \\
4279 & KOI-623 & 19 40 54.4 & +50 33 32 & 6068 & 4.37 & -0.37 & 0.12 & -5.38 & 3.8 & 0.1 & 5.1 & -0.2 & 48 & 0.02 & 0.03 & 1 \\
4280 & KOI-3017 & 19 47 26.2 & +50 33 37 & 5566 & 4.49 & -0.22 & 0.14 & -5.12 & 3.1 & 1.0 & 2.8 & -44.4 & 50 & 0.02 & 0.02 & 1 \\
4281 & KOI-546 & 19 19 19.2 & +50 35 10 & 5908 & 4.25 & 0.12 & 0.14 & -5.17 & 5.1 & 2.9 & 4.1 & -47.5 & 28 & 0.05 & 0.05 & 1 \\
4282 & KOI-2072 & 19 17 26.1 & +50 35 55 & 5866 & 4.22 & -0.12 & 0.12 & -5.39 & 4.1 & 0.8 & 3.9 & -25.3 & 45 & 0.03 & 0.03 & 3 \\
4283 & KOI-2407 & 19 45 30.5 & +50 37 17 & 5895 & 4.12 & 0.15 & 0.12 & -5.34 & 6.6 & 4.9 & 4.1 & -3.2 & 49 & 0.02 & 0.03 & 1 \\
4284 & KOI-2396 & 19 35 53.5 & +50 38 43 & 5168 & 4.54 & 0.02 & 0.24 & -4.82 & 2.4 & 1.2 & 2.0 & -9.9 & 37 & 0.03 & 0.03 & 1 \\
4285 & KOI-4457 & 19 22 03.0 & +50 38 57 & 6096 & 4.08 & -0.16 & 0.11 & -5.51 & 9.4 & 7.0 & 5.3 & -31.0 & 48 & 0.02 & 0.03 & 1 \\
4286 & KOI-360 & 19 16 51.6 & +50 39 03 & 5992 & 4.33 & -0.11 & 0.13 & -5.23 & 4.8 & 1.3 & 4.6 & -23.7 & 47 & 0.02 & 0.03 & 1 \\
4287 & KOI-141 & 19 12 09.2 & +50 39 06 & 5230 & 4.37 & 0.22 & 0.13 & -5.19 & 3.6 & 2.9 & 2.1 & -20.4 & 51 & 0.02 & 0.03 & 1 \\
4288 & KOI-2597 & 19 45 12.5 & +50 40 20 & 5924 & 4.53 & -0.26 & 0.14 & -5.17 & 4.3 & 0.6 & 4.2 & -7.1 & 29 & 0.05 & 0.05 & 1 \\
4289 & KOI-2004 & 19 14 35.1 & +50 47 20 & 5614 & 4.29 & 0.22 & 0.15 & -5.06 & 5.6 & 4.6 & 2.9 & -37.0 & 49 & 0.02 & 0.02 & 1 \\
4290 & KOI-2714 & 19 20 19.9 & +50 51 49 & 5959 & 4.03 & -0.04 & 0.13 & -5.29 & 7.2 & 5.3 & 4.4 & -15.9 & 46 & 0.03 & 0.03 & 1 \\
4291 & Kepler-401 & 19 20 19.9 & +50 51 49 & 5994 & 4.02 & -0.02 & 0.00 & 0.00 & 7.2 & 5.1 & 4.6 & -13.2 & 85 & 0.02 & 0.02 & 1 \\
4292 & KOI-1947 & 19 14 32.4 & +50 54 44 & 5865 & 3.93 & 0.18 & 0.09 & nan & 4.8 & 0.3 & 4.8 & -61.3 & 49 & 0.02 & 0.03 & 1 \\
4293 & KOI-2372 & 19 17 56.6 & +50 56 39 & 5905 & 4.04 & -0.11 & 0.14 & -5.12 & 5.6 & 3.7 & 4.1 & -55.8 & 48 & 0.02 & 0.03 & 1 \\
4294 & KOI-3310 & 19 15 13.1 & +50 59 26 & 5370 & 4.48 & 0.12 & 0.18 & -4.93 & 2.5 & 0.7 & 2.3 & -15.1 & 51 & 0.02 & 0.02 & 1 \\
4295 & KOI-3167 & 19 18 59.2 & +50 59 37 & 5491 & 4.56 & -0.09 & 0.38 & -4.46 & 4.5 & 3.5 & 2.6 & 3.7 & 52 & 0.02 & 0.02 & 1 \\
4296 & KOI-279 & 19 41 56.8 & +51 00 49 & 6141 & 3.98 & 0.15 & 0.13 & -5.23 & 15.8 & 12.5 & 6.5 & -20.3 & 48 & 0.02 & 0.03 & 1 \\
4297 & WASP-92 & 16 26 46.1 & +51 02 28 & 6033 & 4.32 & 0.07 & 0.00 & 0.00 & 6.3 & 3.8 & 4.9 & -30.5 & 111 & 0.01 & 0.02 & 1 \\
4298 & KOI-2541 & 19 22 29.2 & +51 03 26 & 4976 & 3.62 & 0.09 & 0.12 & -5.26 & 3.4 & 0.1 & 3.4 & 17.1 & 53 & 0.02 & 0.02 & 1 \\
4299 & KOI-2059 & 19 10 21.6 & +51 03 38 & 4886 & 4.39 & -0.06 & 0.20 & -4.98 & 4.9 & 4.4 & 1.7 & -33.0 & 54 & 0.02 & 0.03 & 1 \\
4300 & KOI-375 & 19 24 48.3 & +51 08 39 & 5732 & 4.02 & 0.15 & 0.13 & -5.21 & 4.2 & 2.5 & 3.3 & -20.8 & 49 & 0.02 & 0.02 & 1 \\
4301 & KOI-1474 & 19 41 40.3 & +51 11 05 & 6350 & 4.12 & 0.18 & 0.13 & -5.28 & 16.4 & 12.6 & 7.8 & -26.3 & 98 & 0.02 & 0.02 & 2 \\
4302 & KOI-3122 & 19 42 09.2 & +51 12 11 & 6067 & 3.92 & 0.20 & 0.12 & -5.30 & 12.0 & 9.4 & 5.9 & -28.2 & 47 & 0.03 & 0.03 & 1 \\
4303 & KOI-3009 & 19 20 20.3 & +51 12 31 & 5031 & 4.50 & 0.11 & 0.32 & -4.70 & 3.7 & 3.2 & 1.8 & -17.1 & 26 & 0.05 & 0.06 & 1 \\
4304 & KOI-4829 & 19 10 48.5 & +51 13 47 & 6003 & 4.21 & -0.06 & 0.11 & -5.58 & 4.9 & 1.3 & 4.7 & -36.1 & 48 & 0.02 & 0.02 & 1 \\
4305 & KOI-2331 & 19 12 34.7 & +51 16 32 & 5813 & 4.16 & 0.06 & 0.10 & -5.68 & 5.2 & 3.5 & 3.7 & -15.2 & 48 & 0.03 & 0.02 & 1 \\
4306 & KOI-361 & 19 19 31.4 & +51 16 37 & 5641 & 4.40 & 0.05 & 0.11 & -5.47 & 3.0 & 0.1 & 3.0 & -15.7 & 49 & 0.02 & 0.02 & 1 \\
4307 & KOI-2463 & 19 12 14.2 & +51 21 16 & 6070 & 4.34 & 0.19 & 0.10 & -5.85 & 7.1 & 4.6 & 5.1 & 2.9 & 48 & 0.02 & 0.03 & 1 \\
4308 & KOI-439 & 19 45 37.6 & +51 21 29 & 5342 & 4.32 & 0.25 & 0.34 & -4.57 & 3.2 & 2.2 & 2.3 & -80.0 & 51 & 0.02 & 0.02 & 1 \\
4309 & KOI-4329 & 19 16 02.8 & +51 22 34 & 6148 & 4.15 & 0.12 & 0.14 & -5.07 & 9.9 & 7.3 & 5.8 & -36.5 & 50 & 0.02 & 0.03 & 1 \\
4310 & KOI-4605 & 19 21 41.5 & +51 23 19 & 5962 & 3.77 & -0.00 & 0.12 & -5.30 & 5.9 & 2.5 & 5.3 & -54.9 & 44 & 0.03 & 0.05 & 1 \\
4311 & KOI-4190 & 19 14 17.7 & +51 28 22 & 5547 & 4.00 & 0.20 & 0.12 & -5.32 & 4.3 & 1.7 & 3.9 & -40.1 & 42 & 0.03 & 0.07 & 1 \\
4312 & KOI-548 & 19 18 00.2 & +51 41 09 & 5974 & 4.23 & -0.07 & 0.13 & -5.25 & 4.9 & 1.7 & 4.5 & -34.9 & 47 & 0.03 & 0.03 & 1 \\
4313 & KOI-3663 & 19 19 03.3 & +51 57 45 & 5717 & 4.57 & -0.07 & 0.22 & -4.76 & 3.9 & 1.9 & 3.3 & -22.3 & 48 & 0.02 & 0.03 & 1 \\
4314 & KOI-4245 & 19 21 55.2 & +51 57 54 & 5968 & 3.95 & 0.20 & 0.11 & -5.49 & 7.3 & 4.8 & 5.3 & -23.9 & 44 & 0.03 & 0.03 & 1 \\
4315 & BD+52_277A & 01 12 39.8 & +53 10 57 & 6748 & 4.13 & 0.11 & 0.00 & 0.00 & 15.4 & 4.0 & 15.2 & -2.0 & 216 & 0.01 & 0.02 & 1 \\
4316 & HD 239643 & 21 22 18.4 & +57 32 33 & 6091 & 4.26 & 0.03 & 0.00 & 0.00 & 6.6 & 3.7 & 5.3 & -51.6 & 244 & 0.01 & 0.01 & 1 \\
4317 & HD 203802 & 21 22 20.5 & +57 33 55 & 6140 & 4.18 & 0.11 & 0.00 & 0.00 & 9.2 & 6.7 & 5.7 & -52.2 & 244 & 0.01 & 0.01 & 1 \\
4318 & HD 240051 & 22 46 08.8 & +58 04 06 & 5940 & 4.51 & 0.14 & 0.00 & 0.00 & 5.8 & 3.8 & 4.3 & 5.3 & 251 & 0.01 & 0.01 & 1 \\
4319 & HD 215714 & 22 46 05.3 & +58 04 20 & 6409 & 4.26 & 0.12 & 0.00 & 0.00 & 17.8 & 13.6 & 8.6 & 2.4 & 243 & 0.01 & 0.01 & 1 \\
\enddata
\end{deluxetable*}


==> table_04.tex <==
\begin{deluxetable*}{llrrrrrrrrrrrrrrr}
\tablecaption{Spectroscopically determined stellar elemental abundances.
\label{table:stellar_abunds}
}
\tablehead{\colhead{ID} & \colhead{NAME} & \colhead{[C/H]} & \colhead{[N/H]} & \colhead{[O/H]} & \colhead{[Na/H]} & \colhead{[Mg/H]} & \colhead{[Al/H]} & \colhead{[Si/H]} & \colhead{[Ca/H]} & \colhead{[Ti/H]} & \colhead{[V/H]} & \colhead{[Cr/H]} & \colhead{[Mn/H]} & \colhead{[Fe/H]} & \colhead{[Ni/H]} & \colhead{[Y/H]} \\
\colhead{(1)} & \colhead{(2)} & \colhead{(18)} & \colhead{(19)} & \colhead{(20)} & \colhead{(21)} & \colhead{(22)} & \colhead{(23)} & \colhead{(24)} & \colhead{(25)} & \colhead{(26)} & \colhead{(27)} & \colhead{(28)} & \colhead{(29)} & \colhead{(30)} & \colhead{(31)} & \colhead{(32)}}
\startdata
2281 & KOI-3248 & -0.06 & -0.04 & -0.05 & -0.17 & -0.07 & 0.03 & -0.04 & -0.06 & -0.06 & -0.16 & -0.06 & -0.12 & -0.08 & -0.11 & -0.15 \\
2361 & KOI-4273 & 0.07 & -0.02 & 0.18 & 0.14 & 0.11 & 0.13 & 0.08 & 0.24 & 0.25 & -0.06 & 0.18 & 0.01 & 0.17 & 0.10 & 0.34 \\
2393 & KOI-3605 & 0.01 & 0.08 & -0.03 & 0.17 & 0.05 & 0.09 & 0.09 & 0.09 & 0.09 & 0.10 & 0.10 & 0.03 & 0.07 & 0.09 & -0.12 \\
2405 & KOI-3197 & -0.03 & -0.04 & -0.02 & -0.08 & -0.01 & -0.21 & -0.04 & 0.03 & 0.00 & 0.03 & 0.03 & -0.20 & 0.00 & -0.09 & 0.15 \\
2430 & KOI-1353 & -0.04 & 0.03 & -0.00 & -0.14 & -0.06 & -0.01 & -0.04 & 0.08 & -0.01 & -0.15 & 0.01 & -0.10 & 0.03 & -0.08 & 0.04 \\
2435 & KOI-4323 & 0.03 & 0.62 & 0.05 & -0.05 & -0.04 & -0.02 & -0.07 & 0.02 & 0.10 & -0.58 & 0.03 & -0.17 & -0.01 & -0.09 & -0.01 \\
2445 & KOI-3384 & 0.01 & 0.16 & 0.04 & 0.08 & 0.06 & 0.08 & 0.07 & 0.12 & 0.05 & -0.03 & 0.07 & -0.01 & 0.08 & 0.08 & 0.05 \\
2460 & KOI-4409 & 0.16 & 0.36 & 0.23 & 0.31 & 0.18 & 0.20 & 0.26 & 0.21 & 0.21 & 0.28 & 0.19 & 0.29 & 0.23 & 0.23 & 0.18 \\
2464 & KOI-4226 & 0.32 & 0.43 & 0.43 & 0.55 & 0.32 & 0.41 & 0.31 & 0.31 & 0.37 & 0.29 & 0.40 & 0.53 & 0.37 & 0.43 & 0.47 \\
2485 & K2-58 & 0.17 & 0.09 & 0.14 & 0.21 & 0.16 & 0.20 & 0.23 & 0.24 & 0.21 & 0.22 & 0.24 & 0.27 & 0.25 & 0.22 & 0.17 \\
2914 & XO-1 & -0.09 & -0.31 & -0.04 & -0.22 & -0.05 & -0.06 & -0.08 & -0.05 & -0.04 & -0.02 & -0.08 & -0.19 & -0.08 & -0.10 & 0.03 \\
2962 & TRES-4 & 0.15 & 0.42 & 0.44 & 0.28 & 0.19 & 0.23 & 0.25 & 0.31 & 0.33 & 0.13 & 0.29 & 0.23 & 0.31 & 0.28 & 0.40 \\
2980 & KOI-104 & 0.19 & 0.46 & 0.10 & 0.70 & 0.30 & 0.51 & 0.36 & 0.39 & 0.36 & 0.30 & 0.31 & 0.43 & 0.38 & 0.41 & 0.17 \\
2981 & KOI-263 & -0.14 & -0.19 & -0.09 & -0.14 & -0.14 & -0.11 & -0.20 & -0.09 & -0.05 & -0.17 & -0.15 & -0.15 & -0.13 & -0.13 & -0.14 \\
2982 & KOI-10 & -0.05 & 0.06 & 0.17 & -0.15 & -0.11 & -0.29 & 0.01 & 0.03 & 0.01 & -0.07 & -0.03 & -0.31 & -0.02 & -0.12 & 0.05 \\
2983 & KOI-82 & 0.22 & -0.16 & 0.21 & 0.12 & 0.11 & 0.10 & 0.10 & 0.14 & 0.11 & 0.10 & 0.10 & 0.06 & 0.13 & 0.11 & -0.02 \\
2986 & KOI-274 & -0.05 & -0.10 & 0.13 & -0.01 & -0.02 & 0.07 & -0.04 & 0.02 & 0.10 & -0.08 & 0.07 & -0.16 & 0.02 & -0.02 & 0.06 \\
2987 & KOI-22 & 0.10 & 0.03 & 0.14 & 0.21 & 0.15 & 0.18 & 0.17 & 0.17 & 0.16 & 0.11 & 0.18 & 0.19 & 0.17 & 0.22 & 0.17 \\
2988 & KOI-42 & 0.07 & -0.17 & 0.19 & -0.01 & -0.01 & -0.05 & 0.06 & 0.09 & 0.08 & -0.12 & 0.07 & -0.11 & 0.05 & -0.02 & 0.11 \\
2989 & KOI-701 & -0.34 & -0.60 & -0.34 & -0.41 & -0.28 & -0.29 & -0.30 & -0.29 & -0.27 & -0.29 & -0.37 & -0.50 & -0.36 & -0.37 & -1.03 \\
2997 & KOI-245 & -0.29 & -0.21 & -0.10 & -0.36 & -0.25 & -0.23 & -0.29 & -0.25 & -0.24 & -0.24 & -0.29 & -0.37 & -0.30 & -0.32 & -0.27 \\
2998 & KOI-180 & -0.09 & -0.09 & -0.03 & -0.13 & -0.05 & -0.07 & -0.04 & 0.02 & -0.01 & -0.06 & 0.02 & -0.08 & -0.00 & -0.08 & 0.12 \\
2999 & KOI-367 & 0.04 & -0.09 & 0.09 & 0.03 & 0.09 & 0.12 & 0.09 & 0.08 & 0.11 & 0.10 & 0.13 & 0.08 & 0.11 & 0.11 & 0.17 \\
3000 & KOI-122 & 0.27 & 0.33 & 0.32 & 0.28 & 0.24 & 0.26 & 0.24 & 0.25 & 0.27 & 0.23 & 0.22 & 0.25 & 0.24 & 0.26 & 0.20 \\
3001 & KOI-1612 & -0.10 & 0.19 & 0.05 & -0.20 & -0.12 & -0.11 & -0.12 & -0.03 & -0.02 & 0.06 & -0.09 & -0.38 & -0.10 & -0.20 & -0.04 \\
3003 & KOI-2169 & 0.01 & 0.05 & 0.03 & 0.10 & 0.06 & 0.09 & 0.08 & 0.11 & 0.11 & 0.08 & 0.10 & 0.11 & 0.10 & 0.10 & 0.05 \\
3006 & KOI-7 & 0.07 & 0.06 & 0.19 & 0.12 & 0.11 & 0.18 & 0.14 & 0.22 & 0.19 & 0.22 & 0.12 & 0.09 & 0.16 & 0.13 & 0.11 \\
3007 & KOI-299 & 0.06 & -0.02 & 0.06 & 0.07 & 0.09 & 0.07 & 0.11 & 0.13 & 0.14 & 0.13 & 0.13 & 0.12 & 0.13 & 0.10 & 0.12 \\
3011 & KOI-1442 & 0.32 & 0.45 & 0.24 & 0.50 & 0.33 & 0.45 & 0.34 & 0.33 & 0.35 & 0.33 & 0.34 & 0.50 & 0.35 & 0.40 & 0.13 \\
3017 & KOI-244 & 0.01 & 0.09 & 0.14 & -0.08 & -0.09 & -0.64 & -0.01 & 0.04 & 0.01 & -0.03 & -0.01 & -0.23 & -0.02 & -0.14 & 0.06 \\
3018 & KOI-1 & -0.00 & 0.05 & -0.03 & -0.11 & -0.04 & -0.12 & 0.00 & 0.03 & 0.00 & -0.03 & -0.02 & -0.07 & -0.01 & -0.08 & 0.10 \\
3020 & KOI-1431 & 0.20 & 0.18 & 0.11 & 0.29 & 0.20 & 0.22 & 0.20 & 0.19 & 0.19 & 0.17 & 0.20 & 0.22 & 0.20 & 0.20 & 0.15 \\
3022 & KOI-292 & -0.14 & -0.35 & -0.06 & -0.22 & -0.19 & -0.16 & -0.17 & -0.16 & -0.15 & -0.21 & -0.19 & -0.37 & -0.21 & -0.25 & -0.04 \\
3024 & Kepler-174 & -0.23 & -0.33 & -0.16 & -0.46 & -0.37 & -0.26 & -0.26 & -0.41 & -0.33 & -0.42 & -0.66 & -0.80 & -0.63 & -0.48 & -1.38 \\
3025 & KOI-273 & 0.17 & 0.35 & 0.18 & 0.30 & 0.21 & 0.26 & 0.21 & 0.19 & 0.17 & 0.20 & 0.18 & 0.29 & 0.22 & 0.25 & 0.11 \\
3026 & KOI-111 & -0.29 & -0.01 & -0.19 & -0.37 & -0.36 & -0.42 & -0.32 & -0.34 & -0.33 & -0.50 & -0.44 & -0.58 & -0.40 & -0.45 & -0.51 \\
3027 & KOI-1781 & 0.15 & -0.15 & 0.06 & 0.21 & 0.08 & 0.14 & 0.23 & 0.27 & 0.17 & 0.15 & 0.16 & 0.24 & 0.23 & 0.17 & 0.04 \\
3031 & KOI-70 & 0.00 & 0.06 & 0.10 & -0.01 & 0.04 & -0.02 & 0.09 & 0.07 & 0.04 & 0.07 & 0.03 & -0.02 & 0.04 & 0.02 & 0.08 \\
3032 & KOI-98 & -0.03 & 0.14 & 0.25 & -0.03 & 0.08 & -0.08 & 0.10 & 0.15 & 0.17 & 0.08 & 0.15 & -0.07 & 0.11 & -0.03 & 0.23 \\
3034 & KOI-153 & 0.79 & 0.28 & 0.87 & 0.26 & 0.19 & 0.23 & 0.25 & 0.19 & 0.19 & 0.15 & 0.11 & 0.15 & 0.16 & 0.18 & -0.03 \\
3036 & KOI-262 & -0.09 & -0.03 & 0.16 & 0.03 & -0.04 & -0.13 & 0.02 & 0.11 & 0.03 & -0.11 & -0.02 & -0.19 & -0.02 & -0.11 & -0.16 \\
3040 & KOI-283 & 0.09 & 0.08 & 0.09 & 0.06 & 0.12 & 0.06 & 0.11 & 0.13 & 0.12 & 0.08 & 0.15 & 0.11 & 0.15 & 0.12 & 0.14 \\
3041 & KOI-97 & 0.14 & 0.40 & 0.37 & 0.14 & 0.17 & 0.15 & 0.21 & 0.25 & 0.30 & 0.22 & 0.27 & 0.20 & 0.27 & 0.22 & 0.31 \\
3042 & KOI-85 & 0.05 & -0.11 & 0.33 & 0.17 & 0.11 & 0.07 & 0.19 & 0.22 & 0.22 & 0.08 & 0.22 & 0.16 & 0.19 & 0.17 & 0.17 \\
3043 & KOI-108 & 0.07 & -0.03 & 0.08 & 0.16 & 0.11 & 0.06 & 0.07 & 0.13 & 0.10 & 0.14 & 0.15 & 0.17 & 0.13 & 0.14 & 0.14 \\
3045 & KOI-87 & -0.21 & -0.10 & -0.12 & -0.29 & -0.23 & -0.23 & -0.17 & -0.25 & -0.20 & -0.19 & -0.26 & -0.41 & -0.26 & -0.30 & -0.30 \\
3046 & KOI-63 & -0.02 & -0.12 & -0.09 & -0.03 & 0.03 & 0.05 & 0.10 & 0.24 & 0.11 & 0.13 & 0.16 & 0.07 & 0.16 & 0.05 & 0.31 \\
3048 & KOI-260 & -0.06 & 0.14 & -0.09 & -0.46 & -0.12 & -0.29 & -0.12 & -0.13 & 0.08 & 0.12 & -0.07 & -0.22 & -0.08 & -0.14 & -0.25 \\
3054 & KOI-5 & 0.06 & 0.44 & 0.29 & 0.20 & 0.08 & 0.19 & 0.06 & 0.24 & 0.17 & 0.03 & 0.13 & 0.09 & 0.15 & 0.13 & 0.06 \\
3055 & KOI-3158 & -0.15 & -0.70 & 0.13 & -0.43 & -0.29 & -0.31 & -0.36 & -0.37 & -0.25 & -0.35 & -0.55 & -0.69 & -0.52 & -0.43 & -0.62 \\
3058 & KOI-123 & 0.00 & 0.30 & 0.08 & -0.01 & -0.06 & -0.11 & -0.04 & -0.01 & -0.04 & -0.06 & -0.02 & -0.09 & -0.01 & -0.03 & -0.01 \\
3059 & KOI-84 & -0.11 & -0.10 & -0.05 & -0.17 & -0.05 & -0.12 & -0.07 & -0.07 & -0.04 & -0.09 & -0.10 & -0.15 & -0.08 & -0.10 & -0.07 \\
3064 & KOI-277 & -0.14 & 0.35 & 0.08 & -0.24 & -0.17 & -0.13 & -0.17 & -0.16 & -0.07 & -0.06 & -0.13 & -0.41 & -0.17 & -0.22 & -0.17 \\
3065 & KOI-41 & 0.01 & 0.17 & 0.12 & 0.17 & 0.07 & 0.16 & 0.09 & 0.11 & 0.10 & 0.12 & 0.12 & 0.00 & 0.10 & 0.11 & 0.05 \\
3067 & KOI-69 & -0.20 & -0.07 & -0.14 & -0.21 & -0.11 & -0.15 & -0.17 & -0.15 & -0.10 & -0.12 & -0.16 & -0.23 & -0.16 & -0.18 & -0.24 \\
3068 & KOI-75 & -0.10 & -0.53 & 0.03 & -0.21 & -0.14 & -0.22 & -0.14 & 0.03 & -0.00 & -0.31 & -0.07 & -0.30 & -0.05 & -0.16 & 0.07 \\
3072 & KOI-103 & -0.06 & -0.12 & -0.04 & -0.17 & -0.06 & -0.13 & -0.03 & -0.08 & -0.10 & -0.11 & -0.06 & -0.10 & -0.06 & -0.10 & 0.09 \\
3074 & KOI-321 & 0.18 & 0.14 & 0.25 & 0.21 & 0.22 & 0.16 & 0.22 & 0.19 & 0.23 & 0.27 & 0.22 & 0.23 & 0.23 & 0.25 & 0.24 \\
3078 & KOI-2687 & -0.04 & -0.17 & -0.04 & -0.17 & -0.02 & 0.01 & -0.00 & 0.00 & 0.00 & 0.01 & 0.01 & -0.09 & 0.02 & -0.05 & 0.16 \\
3084 & KOI-1925 & 0.01 & 0.05 & 0.02 & 0.08 & 0.04 & 0.09 & 0.04 & 0.04 & 0.08 & 0.08 & 0.04 & 0.04 & 0.05 & 0.05 & -0.06 \\
3091 & KOI-1924 & 0.23 & 0.46 & 0.29 & 0.54 & 0.22 & 0.31 & 0.26 & 0.34 & 0.31 & 0.22 & 0.31 & 0.43 & 0.35 & 0.37 & 0.62 \\
3100 & KOI-99 & 0.00 & -0.29 & 0.21 & -0.22 & -0.12 & -0.07 & -0.14 & -0.17 & -0.09 & -0.13 & -0.31 & -0.48 & -0.28 & -0.23 & -0.59 \\
3101 & KOI-2720 & -0.08 & -0.26 & 0.03 & -0.18 & -0.16 & -0.25 & -0.13 & -0.07 & -0.06 & -0.17 & -0.12 & -0.30 & -0.13 & -0.17 & -0.15 \\
3103 & KOI-364 & 0.21 & 0.25 & 0.27 & 0.26 & 0.21 & 0.25 & 0.24 & 0.22 & 0.18 & 0.19 & 0.23 & 0.26 & 0.24 & 0.25 & 0.24 \\
3105 & KOI-64 & -0.10 & 0.08 & -0.07 & -0.06 & -0.04 & -0.04 & -0.06 & 0.03 & 0.01 & -0.04 & 0.01 & -0.01 & 0.04 & -0.00 & 0.12 \\
3110 & KOI-174 & -0.32 & -0.50 & -0.32 & -0.06 & -0.12 & 0.04 & -0.09 & -0.11 & -0.07 & -0.13 & -0.35 & -0.31 & -0.22 & -0.21 & -0.44 \\
3111 & KOI-17 & 0.30 & 0.28 & 0.23 & 0.41 & 0.28 & 0.30 & 0.28 & 0.29 & 0.31 & 0.27 & 0.29 & 0.34 & 0.30 & 0.32 & 0.25 \\
3113 & KOI-265 & 0.11 & 0.11 & 0.21 & 0.18 & 0.17 & 0.04 & 0.16 & 0.16 & 0.18 & 0.31 & 0.22 & 0.17 & 0.19 & 0.18 & 0.18 \\
3114 & KOI-261 & -0.00 & 0.02 & -0.02 & -0.08 & 0.03 & 0.00 & 0.03 & 0.07 & 0.09 & 0.07 & 0.05 & -0.04 & 0.07 & 0.01 & 0.05 \\
3117 & KOI-305 & 0.14 & 0.15 & 0.04 & 0.41 & 0.28 & 0.28 & 0.18 & 0.33 & 0.28 & 0.25 & 0.25 & 0.29 & 0.27 & 0.31 & 0.07 \\
3118 & KOI-365 & -0.18 & -0.25 & -0.07 & -0.20 & -0.15 & -0.17 & -0.16 & -0.16 & -0.14 & -0.18 & -0.16 & -0.27 & -0.17 & -0.20 & -0.17 \\
3123 & KOI-137 & 0.17 & 0.27 & 0.17 & 0.31 & 0.18 & 0.19 & 0.17 & 0.18 & 0.18 & 0.18 & 0.21 & 0.25 & 0.19 & 0.23 & 0.04 \\
3130 & KOI-148 & 0.19 & 0.21 & 0.21 & 0.34 & 0.19 & 0.25 & 0.21 & 0.23 & 0.20 & 0.20 & 0.22 & 0.23 & 0.21 & 0.22 & 0.13 \\
3131 & KOI-18 & -0.05 & 0.33 & 0.23 & 0.07 & 0.05 & -0.06 & 0.03 & 0.19 & 0.18 & -0.00 & 0.15 & -0.12 & 0.10 & 0.04 & 0.31 \\
3133 & KOI-116 & -0.03 & -0.02 & -0.08 & -0.09 & -0.07 & -0.08 & -0.08 & -0.03 & -0.05 & 0.08 & -0.10 & -0.25 & -0.07 & -0.10 & -0.16 \\
3239 & HD 240429 & 0.00 & -0.06 & 0.01 & -0.04 & 0.01 & -0.00 & 0.01 & 0.03 & 0.03 & 0.02 & 0.00 & -0.03 & 0.01 & -0.01 & 0.02 \\
3240 & HD 240430 & 0.08 & 0.01 & 0.08 & -0.04 & 0.18 & 0.21 & 0.16 & 0.23 & 0.21 & 0.21 & 0.18 & -0.00 & 0.20 & 0.21 & 0.26 \\
3248 & WASP-57 & 0.02 & 0.02 & 0.07 & -0.04 & 0.06 & 0.07 & 0.06 & 0.08 & 0.08 & 0.06 & 0.05 & 0.01 & 0.06 & 0.06 & 0.09 \\
3249 & WASP-74 & 0.31 & 0.48 & 0.38 & 0.51 & 0.34 & 0.43 & 0.40 & 0.41 & 0.38 & 0.33 & 0.39 & 0.52 & 0.40 & 0.47 & 0.41 \\
3250 & WASP-37 & -0.17 & -0.23 & -0.09 & -0.20 & -0.20 & -0.17 & -0.61 & -0.21 & -0.19 & -0.24 & -0.23 & -0.33 & -0.24 & -0.23 & -0.26 \\
3251 & HAT-P-41 & -0.08 & 0.44 & 0.37 & 0.17 & 0.13 & 0.07 & 0.22 & 0.26 & 0.22 & 0.09 & 0.24 & 0.10 & 0.24 & 0.16 & 0.40 \\
3252 & COROT-28 & 0.15 & 0.28 & 0.09 & 0.26 & 0.20 & 0.16 & 0.17 & 0.27 & 0.22 & 0.18 & 0.24 & 0.30 & 0.27 & 0.31 & 0.23 \\
3253 & HAT-P-27 & 0.22 & 0.36 & 0.20 & 0.45 & 0.23 & 0.33 & 0.28 & 0.31 & 0.27 & 0.28 & 0.28 & 0.36 & 0.30 & 0.32 & 0.12 \\
3254 & WASP-103 & 0.16 & 0.45 & 0.30 & 0.33 & 0.17 & 0.20 & 0.13 & 0.33 & 0.31 & 0.35 & 0.22 & 0.26 & 0.22 & 0.21 & 0.15 \\
3255 & WASP-52 & 0.17 & 0.26 & 0.18 & 0.44 & 0.16 & 0.29 & 0.26 & 0.34 & 0.26 & 0.25 & 0.30 & 0.37 & 0.31 & 0.28 & 0.16 \\
3256 & WASP-114 & 0.25 & 0.45 & 0.32 & 0.47 & 0.26 & 0.36 & 0.32 & 0.30 & 0.30 & 0.27 & 0.31 & 0.42 & 0.30 & 0.37 & 0.22 \\
3257 & BD+1290 & -0.04 & -0.13 & -0.01 & -0.02 & -0.05 & -0.05 & -0.04 & 0.00 & -0.02 & -0.06 & -0.04 & -0.09 & -0.08 & -0.02 & -0.08 \\
3258 & HD 4552 & -0.00 & 0.06 & 0.05 & 0.04 & -0.01 & -0.01 & 0.03 & 0.04 & 0.09 & 0.05 & 0.03 & -0.10 & 0.03 & -0.01 & -0.07 \\
3259 & HD 209622 & 0.24 & 0.42 & 0.44 & 0.46 & 0.20 & 0.31 & 0.29 & 0.35 & 0.32 & 0.30 & 0.34 & 0.42 & 0.34 & 0.34 & 0.24 \\
3260 & BD+15_4556 & -0.16 & 0.28 & -0.03 & 0.13 & -0.04 & 0.04 & -0.09 & 0.15 & 0.11 & 0.01 & 0.16 & 0.28 & 0.22 & 0.21 & 0.58 \\
3261 & HAT-P-23 & 0.15 & 0.16 & 0.19 & 0.15 & 0.16 & 0.18 & 0.18 & 0.26 & 0.26 & 0.32 & 0.25 & 0.19 & 0.23 & 0.19 & 0.24 \\
3262 & HAT-P-55 & -0.03 & -0.15 & 0.05 & -0.06 & -0.05 & 0.02 & -0.02 & -0.03 & -0.03 & -0.06 & -0.06 & -0.08 & -0.05 & -0.07 & -0.01 \\
3263 & HAT-P-31 & 0.05 & 0.21 & 0.18 & 0.06 & 0.08 & 0.05 & 0.08 & 0.15 & 0.11 & 0.07 & 0.10 & 0.06 & 0.10 & 0.09 & 0.43 \\
3264 & BD+28_4543S & -0.20 & 0.24 & -0.08 & 0.10 & -0.04 & -0.02 & -0.15 & 0.03 & 0.02 & -0.07 & 0.00 & 0.09 & 0.07 & 0.06 & 0.29 \\
3265 & WASP-135 & 0.28 & 0.40 & 0.20 & 0.63 & 0.33 & 0.46 & 0.40 & 0.44 & 0.39 & 0.36 & 0.38 & 0.49 & 0.42 & 0.45 & 0.17 \\
3266 & WASP-10 & 0.30 & -0.12 & 0.22 & 0.33 & 0.16 & 0.26 & 0.27 & 0.32 & 0.22 & 0.16 & 0.20 & 0.25 & 0.26 & 0.24 & -0.03 \\
3267 & KELT-16 & -0.15 & 0.19 & 0.17 & -0.04 & -0.06 & -0.16 & -0.00 & 0.11 & 0.07 & -0.07 & 0.02 & -0.16 & 0.03 & -0.07 & 0.11 \\
3268 & HAT-P-18 & 0.39 & 0.08 & 0.38 & 0.26 & 0.15 & 0.22 & 0.23 & 0.25 & 0.18 & 0.17 & 0.16 & 0.20 & 0.19 & 0.19 & 0.07 \\
3269 & HAT-P-4 & 0.17 & 0.30 & 0.31 & 0.20 & 0.24 & 0.33 & 0.25 & 0.30 & 0.28 & 0.26 & 0.29 & 0.27 & 0.29 & 0.30 & 0.39 \\
3270 & KELT-12 & 0.16 & 0.53 & 0.49 & 0.40 & 0.21 & 0.24 & 0.31 & 0.38 & 0.37 & 0.24 & 0.34 & 0.29 & 0.35 & 0.34 & 0.38 \\
3271 & KOI-958 & -0.15 & -0.45 & -0.22 & -0.07 & -0.06 & 0.01 & 0.04 & 0.04 & 0.02 & 0.01 & -0.03 & -0.05 & 0.02 & -0.05 & -0.19 \\
3272 & KOI-1010 & -0.01 & -0.06 & 0.08 & 0.06 & -0.05 & -0.04 & -0.02 & 0.04 & 0.08 & -0.04 & -0.00 & -0.16 & 0.01 & -0.05 & -0.03 \\
3273 & KOI-984 & 0.06 & -0.06 & 0.03 & 0.17 & 0.10 & 0.13 & 0.10 & 0.28 & 0.22 & 0.19 & 0.28 & 0.21 & 0.26 & 0.16 & 0.32 \\
3274 & KOI-4212 & 0.00 & 0.12 & 0.31 & 0.11 & 0.09 & 0.05 & 0.19 & 0.18 & 0.11 & 0.12 & 0.17 & 0.03 & 0.16 & 0.11 & 0.18 \\
3275 & KOI-1002 & 0.07 & 0.02 & 0.14 & 0.16 & 0.02 & 0.10 & 0.10 & 0.14 & 0.10 & 0.12 & 0.04 & 0.07 & 0.05 & 0.03 & 0.01 \\
3276 & KOI-2538 & -0.18 & -0.36 & -0.04 & -0.20 & -0.20 & -0.16 & -0.23 & -0.18 & -0.19 & -0.19 & -0.23 & -0.28 & -0.24 & -0.27 & -0.36 \\
3277 & KOI-2534 & 0.01 & -0.33 & 0.04 & -0.11 & -0.00 & -0.05 & 0.01 & 0.05 & 0.04 & -0.01 & 0.04 & -0.11 & 0.04 & -0.00 & 0.12 \\
3278 & KOI-3233 & -0.06 & -0.05 & -0.05 & -0.01 & -0.04 & -0.07 & -0.06 & -0.00 & -0.05 & -0.12 & -0.06 & -0.07 & -0.04 & -0.06 & -0.07 \\
3279 & KOI-2403 & 0.11 & -0.06 & 0.14 & 0.20 & 0.12 & 0.10 & 0.13 & 0.21 & 0.15 & 0.03 & 0.13 & 0.25 & 0.17 & 0.16 & 0.06 \\
3280 & KOI-2201 & 0.11 & -0.06 & 0.19 & 0.21 & 0.13 & 0.01 & 0.19 & 0.26 & 0.23 & 0.14 & 0.20 & 0.19 & 0.22 & 0.19 & 0.27 \\
3281 & KOI-988 & 0.05 & 0.02 & 0.13 & 0.01 & -0.00 & 0.02 & 0.05 & 0.13 & 0.03 & 0.04 & 0.09 & 0.02 & 0.10 & 0.01 & -0.01 \\
3282 & KOI-151 & -0.04 & 0.38 & 0.08 & -0.06 & -0.09 & -0.19 & -0.06 & 0.08 & 0.00 & 0.16 & -0.03 & -0.29 & -0.00 & -0.15 & 0.06 \\
3283 & KOI-113 & 0.27 & 0.41 & 0.28 & 0.41 & 0.27 & 0.42 & 0.29 & 0.32 & 0.30 & 0.30 & 0.32 & 0.38 & 0.33 & 0.35 & 0.32 \\
3284 & KOI-3201 & -0.34 & -0.22 & -0.28 & -0.49 & -0.38 & -0.49 & -0.34 & -0.39 & -0.32 & -0.54 & -0.46 & -0.76 & -0.47 & -0.47 & -0.52 \\
3285 & KOI-2053 & 0.02 & -0.26 & 0.16 & 0.05 & -0.02 & -0.05 & 0.05 & 0.08 & 0.04 & -0.33 & 0.04 & -0.04 & 0.07 & -0.02 & 0.12 \\
3286 & KOI-2033 & -0.03 & -0.18 & 0.07 & -0.23 & -0.09 & -0.06 & -0.10 & -0.07 & -0.07 & -0.12 & -0.18 & -0.24 & -0.14 & -0.15 & -0.38 \\
3287 & KOI-1944 & -0.11 & -0.57 & -0.10 & -0.11 & -0.03 & -0.14 & -0.03 & 0.07 & -0.01 & 0.01 & 0.05 & -0.08 & 0.01 & -0.01 & 0.11 \\
3288 & KOI-2603 & -0.21 & -0.32 & 0.19 & -0.04 & -0.09 & -0.44 & -0.09 & 0.05 & 0.07 & -0.15 & -0.02 & -0.29 & -0.00 & -0.11 & 0.05 \\
3289 & KOI-440 & 0.13 & 0.49 & 0.10 & 0.18 & 0.14 & 0.15 & 0.18 & 0.16 & 0.20 & 0.18 & 0.16 & 0.16 & 0.15 & 0.33 & -0.01 \\
3290 & KOI-166 & -0.28 & -0.28 & -0.20 & -0.28 & -0.22 & -0.24 & -0.27 & -0.24 & -0.22 & -0.23 & -0.28 & -0.37 & -0.29 & -0.30 & -0.40 \\
3291 & KOI-379 & -0.02 & 0.38 & 0.41 & 0.14 & 0.10 & 0.10 & 0.16 & 0.29 & 0.24 & -0.06 & 0.20 & -0.01 & 0.21 & 0.14 & 0.30 \\
3292 & KOI-2009 & -0.14 & -0.53 & -0.04 & -0.37 & -0.11 & -0.08 & -0.18 & -0.21 & -0.03 & -0.14 & -0.23 & -0.49 & -0.27 & -0.23 & -0.28 \\
3293 & KOI-4581 & 0.03 & -0.03 & 0.02 & 0.06 & 0.08 & 0.08 & 0.05 & 0.11 & 0.08 & 0.09 & 0.06 & 0.03 & 0.07 & 0.08 & 0.05 \\
3294 & KOI-3835 & 0.02 & -0.16 & 0.05 & -0.05 & -0.09 & -0.05 & 0.04 & 0.10 & 0.00 & -0.03 & 0.03 & -0.01 & 0.05 & -0.05 & -0.02 \\
3295 & KOI-3681 & 0.13 & 0.49 & 0.17 & 0.14 & 0.14 & 0.05 & 0.16 & 0.17 & 0.21 & 0.16 & 0.20 & 0.12 & 0.18 & 0.20 & 0.13 \\
3296 & KOI-3853 & -0.04 & 0.05 & 0.14 & -0.04 & 0.01 & 0.14 & -0.07 & -0.03 & 0.04 & -0.03 & -0.11 & -0.16 & -0.08 & -0.04 & -0.17 \\
3297 & KOI-2979 & -0.10 & 0.12 & -0.12 & -0.24 & -0.14 & -0.16 & -0.19 & -0.12 & -0.14 & -0.28 & -0.17 & -0.25 & -0.13 & -0.20 & -0.15 \\
3298 & KOI-986 & 0.15 & 0.16 & 0.18 & 0.25 & 0.13 & 0.19 & 0.17 & 0.21 & 0.21 & 0.16 & 0.23 & 0.27 & 0.22 & 0.20 & 0.11 \\
3299 & KOI-2896 & -0.01 & 0.16 & 0.21 & 0.10 & -0.02 & 0.09 & 0.00 & 0.17 & 0.14 & -0.27 & 0.08 & -0.12 & 0.05 & 0.01 & 0.02 \\
3300 & KOI-4659 & -0.11 & -0.12 & -0.15 & -0.16 & -0.11 & -0.06 & -0.05 & -0.05 & -0.05 & -0.04 & -0.02 & -0.18 & -0.06 & -0.10 & 0.08 \\
3301 & KOI-1118 & -0.06 & -0.05 & -0.00 & -0.09 & -0.05 & -0.06 & -0.09 & -0.06 & 0.04 & -0.44 & -0.07 & -0.09 & -0.05 & -0.09 & -0.04 \\
3302 & KOI-4298 & -0.30 & -0.40 & -0.09 & -0.50 & -0.32 & -0.92 & -0.37 & -0.24 & -0.14 & -0.12 & -0.31 & -0.70 & -0.36 & -0.39 & -0.37 \\
3303 & KOI-1113 & 0.05 & -0.16 & 0.11 & -0.02 & 0.06 & -0.06 & 0.04 & 0.08 & 0.13 & -0.12 & 0.07 & -0.01 & 0.07 & 0.03 & 0.10 \\
3304 & KOI-1116 & 0.05 & -0.07 & 0.09 & 0.02 & 0.02 & -0.00 & 0.01 & 0.02 & 0.03 & 0.05 & -0.02 & -0.03 & 0.01 & 0.01 & -0.01 \\
3305 & KOI-2081 & -0.00 & 0.30 & 0.11 & 0.16 & 0.07 & 0.07 & -0.05 & 0.15 & 0.12 & 0.04 & 0.17 & 0.26 & 0.16 & 0.13 & 0.20 \\
3306 & KOI-4400 & 0.01 & 0.08 & 0.06 & -0.10 & -0.02 & 0.08 & 0.04 & 0.06 & 0.09 & 0.09 & -0.01 & -0.10 & 0.01 & 0.04 & 0.08 \\
3307 & KOI-1824 & -0.18 & -0.24 & -0.15 & -0.20 & -0.18 & -0.13 & -0.19 & -0.12 & -0.16 & -0.09 & -0.17 & -0.39 & -0.19 & -0.24 & -0.19 \\
3308 & KOI-2807 & 0.09 & 0.45 & 0.36 & 0.30 & 0.11 & 0.10 & 0.18 & 0.30 & 0.13 & -1.24 & 0.19 & 0.22 & 0.21 & 0.05 & 0.17 \\
3309 & KOI-2335 & -0.01 & -0.22 & 0.01 & -0.10 & -0.06 & -0.03 & -0.07 & -0.09 & -0.03 & -0.11 & -0.06 & -0.12 & -0.07 & -0.08 & -0.03 \\
3310 & KOI-197 & -0.18 & 0.55 & 0.19 & -0.03 & 0.04 & -0.15 & -0.11 & 0.00 & 0.03 & 0.03 & 0.05 & -0.06 & -0.01 & 0.05 & -0.21 \\
3311 & KOI-4144 & -0.12 & 0.14 & 0.13 & -0.14 & -0.10 & -0.19 & -0.07 & -0.12 & -0.07 & -0.04 & -0.10 & -0.29 & -0.11 & -0.16 & -0.09 \\
3312 & KOI-1115 & -0.02 & -0.08 & 0.01 & -0.09 & 0.02 & 0.04 & -0.04 & 0.06 & 0.03 & -0.03 & 0.07 & 0.04 & 0.06 & 0.03 & 0.08 \\
3313 & HAT-P-14 & -0.25 & 0.14 & 0.27 & -0.09 & -0.03 & -0.19 & 0.06 & 0.14 & 0.15 & 0.02 & 0.06 & -0.24 & 0.07 & -0.10 & 0.19 \\
3314 & KOI-1878 & 0.18 & 0.47 & 0.28 & 0.15 & 0.18 & 0.13 & 0.17 & 0.25 & 0.21 & 0.11 & 0.18 & 0.11 & 0.19 & 0.15 & 0.22 \\
3315 & KOI-3277 & -0.07 & -0.10 & 0.13 & -0.07 & -0.06 & -0.13 & -0.10 & 0.03 & 0.02 & -0.10 & -0.03 & -0.15 & -0.02 & -0.11 & 0.06 \\
3316 & KOI-3203 & -0.59 & 0.63 & 0.25 & -0.29 & -0.20 & -0.34 & -0.09 & -0.05 & -0.14 & -0.28 & -0.17 & -0.52 & -0.12 & -0.47 & -0.01 \\
3317 & KOI-3225 & 0.03 & 0.07 & 0.07 & 0.04 & 0.07 & 0.10 & 0.14 & 0.12 & 0.12 & 0.12 & 0.10 & 0.11 & 0.10 & 0.09 & -0.01 \\
3318 & Kepler-24 & 0.02 & 0.01 & -0.12 & -0.05 & -0.05 & -0.19 & -0.05 & 0.06 & 0.07 & -0.25 & 0.01 & -0.11 & -0.02 & -0.05 & 0.07 \\
3319 & KOI-490 & -0.04 & 0.14 & -0.07 & 0.09 & 0.03 & 0.14 & 0.10 & 0.08 & 0.09 & 0.04 & -0.02 & 0.02 & 0.06 & 0.08 & -0.32 \\
3320 & KOI-1089 & 0.07 & 0.11 & 0.03 & 0.15 & 0.08 & 0.12 & 0.09 & 0.10 & 0.10 & -0.09 & 0.09 & 0.06 & 0.08 & 0.06 & 0.07 \\
3321 & KOI-2863 & -0.18 & -0.11 & 0.02 & -0.31 & -0.16 & -0.07 & -0.17 & -0.19 & -0.04 & -0.03 & -0.29 & -0.50 & -0.29 & -0.26 & -0.33 \\
3322 & KOI-3515 & -0.26 & 0.21 & -0.19 & -0.54 & -0.16 & -0.56 & -0.15 & -0.34 & 0.09 & -0.41 & -0.23 & -0.40 & -0.23 & -0.24 & -0.17 \\
3323 & KOI-401 & 0.25 & 0.29 & 0.28 & 0.34 & 0.23 & 0.29 & 0.27 & 0.25 & 0.24 & 0.25 & 0.26 & 0.32 & 0.27 & 0.28 & 0.20 \\
3324 & KOI-2278 & -0.10 & -0.17 & 0.00 & -0.20 & -0.12 & -0.08 & -0.15 & -0.15 & -0.06 & -0.25 & -0.16 & -0.30 & -0.15 & -0.17 & -0.25 \\
3325 & KOI-3172 & -0.06 & 0.30 & 0.08 & -0.02 & -0.07 & -0.04 & -0.02 & 0.04 & 0.06 & -0.04 & 0.04 & -0.26 & 0.02 & -0.05 & 0.15 \\
3326 & KOI-2974 & -0.21 & 0.26 & 0.60 & -0.03 & 0.02 & 0.06 & 0.08 & 0.13 & 0.28 & 0.21 & 0.15 & -0.12 & 0.22 & 0.01 & 0.15 \\
3327 & KOI-384 & -0.08 & 0.28 & 0.32 & 0.02 & -0.01 & -0.15 & 0.07 & 0.12 & 0.10 & -0.22 & 0.06 & -0.16 & 0.07 & -0.02 & 0.16 \\
3328 & KOI-2740 & -0.08 & 0.23 & -0.10 & -0.20 & -0.18 & -0.45 & -0.16 & -0.15 & -0.04 & -0.06 & -0.20 & -0.38 & -0.19 & -0.27 & -0.36 \\
3329 & KOI-1196 & -0.11 & -0.12 & 0.21 & -0.14 & -0.09 & -0.03 & -0.10 & -0.13 & -0.06 & -0.06 & -0.25 & -0.44 & -0.24 & -0.24 & -0.34 \\
3330 & KOI-1845 & 0.65 & 0.71 & 0.73 & 0.67 & 0.37 & 0.47 & 0.37 & 0.42 & 0.35 & 0.32 & 0.36 & 0.49 & 0.37 & 0.44 & 0.19 \\
3331 & KOI-3075 & -0.34 & -0.24 & 0.03 & -0.47 & -0.31 & -0.24 & -0.38 & -0.37 & -0.29 & -0.43 & -0.57 & -0.79 & -0.53 & -0.49 & -0.48 \\
3332 & KOI-268 & -0.10 & 0.26 & 0.25 & 0.03 & 0.03 & 0.01 & 0.08 & 0.07 & 0.15 & 0.18 & 0.07 & -0.19 & 0.07 & -0.05 & -0.22 \\
3333 & KOI-2043 & -0.06 & -0.30 & -0.00 & -0.00 & 0.01 & 0.05 & -0.01 & 0.02 & 0.05 & 0.04 & -0.03 & -0.03 & -0.00 & 0.01 & -0.05 \\
3334 & KOI-3876 & -0.01 & 0.04 & -0.07 & -0.10 & -0.01 & -0.20 & 0.05 & 0.13 & 0.11 & 0.16 & 0.07 & 0.02 & 0.12 & -0.04 & 0.01 \\
3335 & KOI-1218 & -0.05 & -0.14 & -0.02 & -0.13 & -0.06 & -0.02 & -0.04 & -0.07 & -0.02 & -0.04 & -0.06 & -0.21 & -0.06 & -0.06 & -0.06 \\
3336 & KOI-385 & 0.04 & 0.13 & 0.17 & 0.07 & 0.06 & 0.04 & 0.04 & 0.07 & 0.08 & 0.07 & 0.07 & 0.05 & 0.07 & 0.07 & -0.04 \\
3337 & KOI-3415 & -0.36 & -0.57 & -0.30 & 0.23 & -0.55 & 0.61 & 0.41 & -0.74 & -0.91 & -0.40 & -1.16 & -0.84 & -0.55 & -0.49 & -0.96 \\
3338 & KOI-3340 & -0.05 & 0.53 & -0.05 & -0.20 & -0.08 & -0.13 & 0.00 & -0.00 & -0.02 & 0.09 & -0.08 & -0.22 & -0.04 & -0.12 & -0.12 \\
3339 & KOI-3641 & -0.06 & 0.47 & 0.04 & -0.09 & -0.12 & -0.11 & -0.04 & 0.06 & 0.01 & -0.08 & -0.05 & -0.15 & -0.06 & -0.16 & -0.02 \\
3340 & KOI-118 & 0.03 & -0.12 & 0.12 & -0.00 & 0.03 & 0.06 & 0.01 & 0.07 & 0.04 & 0.01 & 0.04 & -0.05 & 0.04 & -0.01 & -0.06 \\
3341 & KOI-2755 & -0.16 & -0.03 & -0.08 & -0.20 & -0.16 & -0.12 & -0.14 & -0.15 & -0.12 & -0.13 & -0.17 & -0.30 & -0.17 & -0.19 & -0.26 \\
3342 & KOI-2194 & -0.17 & 0.03 & 0.03 & -0.18 & -0.12 & -0.05 & -0.08 & -0.13 & 0.04 & 0.01 & -0.28 & -0.50 & -0.23 & -0.18 & -0.32 \\
3343 & KOI-6102 & -0.23 & 0.33 & 0.55 & 0.20 & 0.03 & -0.65 & 0.14 & 0.46 & 0.26 & -0.11 & 0.21 & -0.08 & 0.24 & -0.13 & 0.68 \\
3344 & KOI-624 & -0.04 & -0.13 & -0.08 & -0.07 & -0.03 & -0.01 & 0.02 & 0.09 & 0.02 & -0.01 & 0.06 & -0.05 & 0.06 & -0.05 & 0.07 \\
3345 & KOI-1221 & 0.28 & 0.33 & 0.27 & 0.42 & 0.26 & 0.34 & 0.16 & 0.30 & 0.27 & 0.21 & 0.31 & 0.45 & 0.34 & 0.36 & 0.29 \\
3346 & KOI-386 & 0.05 & 0.06 & 0.03 & -0.06 & 0.05 & 0.00 & 0.02 & 0.10 & 0.09 & -0.03 & 0.04 & 0.02 & 0.07 & 0.04 & 0.14 \\
3347 & KOI-975 & -0.02 & -0.35 & 0.17 & -0.13 & -0.03 & -0.12 & 0.03 & 0.04 & 0.10 & 0.07 & 0.04 & -0.17 & 0.03 & -0.06 & 0.07 \\
3348 & KOI-2279 & 0.06 & 0.01 & 0.10 & -0.04 & 0.03 & 0.04 & 0.05 & 0.01 & 0.07 & 0.03 & 0.07 & 0.01 & 0.05 & 0.03 & 0.07 \\
3349 & KOI-302 & -0.14 & 0.53 & 0.18 & -0.10 & 0.09 & -0.71 & 0.05 & 0.30 & 0.17 & 0.10 & 0.23 & -0.05 & 0.25 & 0.07 & 0.44 \\
3350 & KOI-1901 & 0.14 & 0.37 & 0.17 & 0.22 & 0.16 & 0.16 & 0.19 & 0.20 & 0.20 & 0.28 & 0.17 & 0.21 & 0.20 & 0.21 & 0.21 \\
3351 & KOI-1861 & -0.04 & -0.13 & -0.05 & -0.07 & 0.01 & -0.16 & -0.02 & 0.12 & 0.11 & 0.08 & 0.14 & -0.08 & 0.05 & -0.03 & 0.20 \\
3352 & KOI-3308 & 0.02 & 0.08 & 0.08 & -0.05 & 0.03 & 0.03 & 0.02 & 0.07 & 0.05 & -0.02 & 0.04 & -0.11 & 0.02 & 0.01 & 0.00 \\
3353 & KOI-301 & 0.02 & 0.12 & 0.05 & -0.13 & -0.09 & 0.07 & -0.07 & -0.02 & -0.00 & -0.02 & -0.01 & -0.23 & -0.03 & -0.16 & 0.01 \\
3354 & KOI-2808 & -0.34 & -0.06 & 0.19 & -0.09 & 0.09 & -0.11 & 0.15 & -0.54 & 0.35 & 0.55 & 0.11 & -0.26 & 0.07 & -0.10 & -0.04 \\
3355 & KOI-442 & -0.05 & -0.23 & -0.04 & -0.08 & -0.07 & -0.11 & -0.05 & -0.01 & -0.08 & -0.04 & -0.06 & -0.14 & -0.05 & -0.06 & -0.17 \\
3356 & KOI-2261 & -0.07 & -0.32 & -0.10 & -0.14 & -0.04 & -0.02 & 0.02 & 0.07 & 0.03 & 0.01 & 0.02 & -0.06 & 0.04 & -0.06 & 0.07 \\
3357 & KOI-1206 & 0.01 & -0.06 & 0.22 & -0.09 & -0.08 & -0.02 & -0.02 & 0.09 & 0.02 & 0.01 & 0.08 & -0.12 & 0.07 & -0.02 & 0.36 \\
3358 & KOI-3002 & -0.15 & -0.60 & 0.02 & -0.22 & -0.25 & -0.16 & -0.18 & -0.10 & -0.02 & 0.04 & -0.13 & -0.26 & -0.13 & -0.32 & -0.09 \\
3359 & KOI-388 & 0.07 & 0.28 & 0.13 & 0.11 & 0.08 & 0.06 & 0.09 & 0.11 & 0.13 & 0.06 & 0.08 & 0.08 & 0.13 & 0.10 & 0.09 \\
3360 & KOI-444 & -0.13 & -0.23 & -0.07 & -0.13 & -0.14 & -0.14 & -0.14 & -0.14 & -0.14 & -0.17 & -0.16 & -0.20 & -0.16 & -0.18 & -0.13 \\
3361 & KOI-149 & -0.05 & -0.40 & 0.09 & -0.05 & 0.05 & -0.08 & -0.05 & 0.17 & 0.12 & -0.16 & 0.03 & -0.19 & 0.04 & -0.03 & -0.18 \\
3362 & KOI-2289 & 0.18 & -0.83 & 0.11 & -0.04 & 0.12 & -0.07 & 0.07 & 0.10 & 0.24 & 0.32 & 0.31 & 0.17 & 0.19 & 0.06 & 0.71 \\
3363 & KOI-4423 & -0.21 & 0.07 & 0.22 & -0.09 & -0.10 & -0.22 & -0.02 & -0.06 & 0.03 & -0.27 & -0.10 & -0.22 & -0.04 & -0.16 & -0.21 \\
3364 & KOI-1216 & -0.03 & 0.09 & 0.05 & -0.05 & -0.04 & 0.01 & -0.05 & -0.02 & 0.03 & 0.09 & 0.01 & -0.22 & -0.03 & -0.08 & -0.08 \\
3365 & KOI-1208 & -0.15 & 0.21 & 0.26 & -0.09 & -0.08 & -0.44 & -0.05 & 0.07 & 0.11 & 0.20 & -0.01 & -0.26 & -0.01 & -0.13 & 0.05 \\
3366 & KOI-2904 & 0.18 & 0.32 & 0.45 & 0.42 & 0.20 & 0.19 & 0.29 & 0.41 & 0.40 & 0.31 & 0.36 & 0.37 & 0.36 & 0.35 & 0.43 \\
3367 & KOI-393 & -0.26 & -0.13 & 0.08 & -0.10 & -0.15 & -0.40 & -0.12 & -0.10 & -0.03 & 0.06 & -0.12 & -0.31 & -0.13 & -0.24 & -0.23 \\
3368 & KOI-3180 & 0.05 & -0.04 & 0.35 & 0.04 & -0.02 & 0.02 & 0.08 & 0.15 & 0.14 & -0.01 & 0.16 & -0.03 & 0.15 & 0.06 & 0.40 \\
3369 & KOI-392 & 0.17 & 0.21 & 0.20 & 0.19 & 0.17 & 0.23 & 0.11 & 0.14 & 0.11 & 0.15 & 0.15 & 0.20 & 0.17 & 0.18 & 0.15 \\
3370 & KOI-1336 & 0.00 & -0.04 & 0.01 & -0.05 & 0.09 & -0.28 & -0.04 & 0.01 & 0.06 & -0.15 & 0.04 & -0.01 & 0.01 & 0.03 & -0.14 \\
3371 & KOI-4887 & -0.03 & -0.23 & 0.04 & -0.04 & -0.05 & -0.09 & -0.03 & 0.06 & 0.02 & -0.09 & -0.01 & -0.12 & 0.02 & 0.00 & 0.11 \\
3372 & KOI-1222 & -0.02 & 0.02 & 0.12 & 0.01 & -0.00 & 0.04 & -0.06 & 0.03 & 0.02 & -0.04 & 0.05 & 0.12 & 0.07 & 0.06 & 0.33 \\
3373 & KOI-280 & -0.25 & 0.21 & -0.22 & -0.26 & -0.28 & -0.33 & -0.27 & -0.27 & -0.24 & -0.12 & -0.30 & -0.50 & -0.28 & -0.37 & -0.37 \\
3374 & KOI-1335 & 0.07 & 0.44 & 0.49 & 0.13 & 0.13 & -0.54 & 0.27 & 0.26 & 0.20 & 0.21 & 0.19 & 0.08 & 0.24 & 0.13 & 0.19 \\
3375 & KOI-2202 & 0.26 & 0.36 & 0.25 & 0.47 & 0.24 & 0.27 & 0.26 & 0.29 & 0.27 & 0.28 & 0.31 & 0.34 & 0.26 & 0.30 & 0.14 \\
3376 & KOI-1344 & -0.23 & -0.15 & -0.19 & -0.36 & -0.28 & -0.26 & -0.29 & -0.26 & -0.21 & -0.07 & -0.29 & -0.55 & -0.32 & -0.40 & -0.37 \\
3377 & KOI-281 & -0.34 & -0.26 & 0.06 & -0.31 & -0.29 & -0.15 & -0.23 & -0.27 & -0.12 & -0.19 & -0.42 & -0.90 & -0.41 & -0.39 & -0.24 \\
3378 & KOI-2866 & 0.10 & 0.08 & 0.21 & 0.20 & 0.14 & 0.15 & 0.13 & 0.21 & 0.31 & 0.31 & 0.21 & 0.01 & 0.18 & 0.14 & 0.11 \\
3379 & KOI-144 & 0.52 & 0.31 & 0.54 & 0.40 & 0.25 & 0.34 & 0.26 & 0.30 & 0.26 & 0.23 & 0.25 & 0.29 & 0.29 & 0.28 & 0.02 \\
3380 & KOI-3864 & 0.01 & -0.17 & -0.03 & 0.01 & -0.00 & 0.00 & 0.06 & 0.14 & 0.07 & 0.08 & 0.05 & 0.07 & 0.10 & 0.01 & 0.01 \\
3381 & KOI-3880 & -0.02 & 0.06 & 0.29 & -0.06 & 0.01 & -0.18 & 0.10 & 0.10 & 0.09 & 0.10 & 0.10 & 0.02 & 0.12 & -0.01 & 0.36 \\
3382 & KOI-1864 & -0.01 & 0.05 & 0.01 & -0.07 & 0.06 & 0.06 & 0.02 & 0.03 & 0.06 & 0.03 & 0.04 & -0.03 & 0.10 & 0.04 & 0.01 \\
3383 & KOI-3678 & 0.09 & 0.06 & 0.13 & 0.08 & 0.07 & 0.09 & 0.13 & 0.09 & 0.09 & 0.07 & 0.10 & 0.11 & 0.08 & 0.10 & 0.11 \\
3384 & KOI-551 & 0.08 & 0.12 & 0.07 & 0.25 & 0.10 & 0.02 & 0.11 & 0.19 & 0.07 & 0.10 & 0.06 & 0.13 & 0.09 & 0.13 & 0.08 \\
3385 & KOI-3202 & -0.13 & 0.12 & -0.10 & -0.11 & -0.07 & -0.12 & -0.14 & -0.03 & -0.01 & -0.11 & -0.03 & -0.07 & -0.02 & -0.05 & 0.12 \\
3386 & KOI-2311 & 0.03 & 0.21 & -0.01 & -0.01 & 0.08 & 0.06 & 0.12 & 0.19 & 0.20 & 0.08 & 0.16 & 0.10 & 0.13 & 0.13 & 0.07 \\
3387 & KOI-1619 & -0.20 & -0.37 & -0.18 & -0.29 & -0.26 & -0.25 & -0.21 & -0.23 & -0.24 & -0.25 & -0.27 & -0.35 & -0.29 & -0.31 & -0.47 \\
3388 & KOI-5048 & -0.15 & 0.14 & -0.09 & 0.02 & 0.02 & 0.07 & -0.10 & 0.04 & 0.04 & -0.03 & 0.06 & 0.17 & 0.08 & 0.12 & 0.16 \\
3389 & KOI-3358 & -0.15 & -0.29 & 0.00 & -0.27 & -0.16 & -0.15 & -0.15 & -0.16 & -0.12 & -0.17 & -0.20 & -0.31 & -0.18 & -0.19 & -0.29 \\
3390 & KOI-3928 & -0.04 & -0.91 & 0.10 & -0.14 & -0.05 & -0.07 & -0.05 & -0.03 & 0.02 & -0.12 & 0.00 & -0.13 & -0.01 & -0.10 & -0.06 \\
3391 & KOI-3528 & -0.43 & 0.38 & -0.04 & -0.11 & -0.17 & -0.23 & -0.07 & -0.13 & -0.00 & 0.01 & -0.14 & -0.31 & -0.15 & 0.01 & 0.22 \\
3392 & KOI-1615 & 0.10 & 0.24 & 0.29 & 0.24 & 0.17 & 0.25 & 0.19 & 0.36 & 0.33 & 0.43 & 0.31 & 0.26 & 0.29 & 0.22 & 0.23 \\
3393 & KOI-403 & 0.02 & 0.96 & 0.34 & 0.45 & 0.17 & -0.12 & 0.50 & 0.21 & 0.46 & 0.37 & 0.20 & -0.03 & 0.27 & 0.09 & 0.12 \\
3394 & KOI-4774 & -0.13 & -0.23 & -0.12 & -0.10 & -0.03 & -0.05 & -0.05 & -0.04 & 0.00 & -0.02 & -0.02 & -0.09 & -0.02 & -0.04 & 0.01 \\
3395 & KOI-5057 & -0.15 & 0.18 & -0.00 & -0.08 & -0.01 & -0.11 & -0.21 & -0.00 & -0.01 & -0.08 & -0.01 & 0.07 & 0.04 & 0.03 & 0.22 \\
3396 & KOI-2787 & -0.26 & -0.07 & -0.12 & -0.30 & -0.20 & -0.38 & -0.15 & -0.08 & 0.02 & -0.71 & -0.12 & -0.36 & -0.16 & -0.27 & -0.25 \\
3397 & KOI-1738 & 0.15 & 0.20 & 0.16 & 0.28 & 0.14 & 0.18 & 0.18 & 0.17 & 0.18 & 0.16 & 0.18 & 0.24 & 0.19 & 0.18 & 0.09 \\
3398 & KOI-3378 & -0.34 & -0.49 & -0.20 & -0.46 & -0.37 & -0.38 & -0.33 & -0.41 & -0.31 & -0.27 & -0.41 & -0.59 & -0.43 & -0.46 & -0.45 \\
3399 & KOI-1803 & -0.04 & -0.24 & -0.14 & 0.04 & -0.01 & 0.01 & 0.03 & 0.12 & 0.05 & 0.04 & 0.05 & -0.01 & 0.05 & -0.01 & 0.01 \\
3400 & KOI-4452 & -0.22 & -0.05 & -0.06 & -0.32 & -0.28 & -0.25 & -0.22 & -0.25 & -0.14 & -0.30 & -0.32 & -0.61 & -0.32 & -0.36 & -0.39 \\
3401 & KOI-3168 & -0.16 & -0.28 & -0.03 & -0.33 & -0.19 & -0.21 & -0.20 & -0.12 & -0.12 & -0.19 & -0.21 & -0.40 & -0.17 & -0.25 & -0.27 \\
3402 & KOI-626 & -0.19 & 0.04 & -0.02 & -0.14 & -0.17 & -0.44 & -0.18 & -0.15 & -0.08 & -0.20 & -0.16 & -0.37 & -0.16 & -0.21 & -0.15 \\
3403 & KOI-1338 & -0.12 & 0.00 & -0.05 & -0.27 & -0.16 & -0.20 & -0.16 & -0.12 & -0.09 & -0.23 & -0.20 & -0.37 & -0.21 & -0.19 & -0.27 \\
3404 & KOI-1332 & -0.24 & -0.92 & -0.16 & -0.34 & -0.22 & -0.12 & -0.25 & -0.23 & -0.19 & -0.31 & -0.28 & -0.39 & -0.27 & -0.29 & -0.28 \\
3405 & KOI-2547 & -0.09 & 0.22 & -0.13 & -0.13 & -0.07 & -0.10 & -0.11 & -0.05 & -0.04 & -0.03 & -0.09 & -0.25 & -0.09 & -0.14 & -0.01 \\
3406 & KOI-4288 & 0.06 & -0.07 & 0.17 & 0.05 & 0.06 & -0.01 & 0.07 & 0.10 & 0.10 & 0.04 & 0.07 & 0.03 & 0.09 & 0.09 & 0.11 \\
3407 & KOI-3181 & 0.02 & 0.27 & 0.12 & 0.16 & 0.08 & 0.08 & 0.08 & 0.14 & 0.17 & 0.12 & 0.08 & 0.09 & 0.14 & 0.14 & 0.03 \\
3408 & KOI-627 & 0.09 & 0.13 & 0.18 & 0.20 & 0.16 & -0.27 & 0.17 & 0.19 & 0.15 & 0.14 & 0.16 & 0.20 & 0.18 & 0.18 & 0.10 \\
3409 & KOI-4157 & 0.03 & 0.33 & 0.22 & -0.15 & -0.06 & -0.08 & 0.06 & 0.13 & 0.06 & 0.19 & 0.05 & -0.16 & 0.05 & -0.05 & 0.18 \\
3410 & KOI-2025 & -0.26 & -0.34 & 0.19 & -0.26 & -0.02 & 0.21 & 0.05 & 0.07 & -0.09 & -0.13 & -0.00 & -0.00 & 0.08 & -0.04 & -0.02 \\
3411 & Kepler-350 & -0.04 & 0.07 & -0.01 & -0.19 & -0.05 & -0.94 & -0.01 & 0.08 & 0.01 & 0.18 & 0.14 & -0.08 & 0.07 & -0.09 & 0.08 \\
3412 & KOI-628 & -0.30 & -0.09 & -0.21 & -0.48 & -0.27 & -0.27 & -0.29 & -0.35 & -0.29 & -0.28 & -0.37 & -0.61 & -0.40 & -0.42 & -0.33 \\
3413 & KOI-3811 & -0.02 & 0.52 & 0.16 & 0.12 & -0.05 & -0.02 & 0.10 & 0.02 & 0.15 & 0.16 & -0.03 & -0.08 & -0.05 & -0.09 & -0.08 \\
3414 & KOI-629 & -0.18 & 0.07 & -0.15 & -0.30 & -0.23 & -0.27 & -0.28 & -0.28 & -0.13 & -0.24 & -0.28 & -0.53 & -0.27 & -0.29 & -0.43 \\
3415 & KOI-1805 & -0.08 & -0.14 & 0.07 & -0.15 & -0.09 & -0.13 & -0.05 & -0.02 & -0.04 & -0.07 & -0.02 & -0.18 & -0.03 & -0.13 & 0.09 \\
3416 & KOI-2393 & -0.17 & 0.13 & -0.18 & -0.05 & -0.04 & -0.09 & 0.01 & 0.01 & -0.06 & -0.04 & -0.06 & -0.06 & -0.04 & -0.12 & 0.14 \\
3417 & KOI-1534 & 0.06 & 0.00 & 0.16 & -0.01 & 0.07 & -0.01 & 0.04 & 0.04 & 0.18 & 0.17 & 0.14 & -0.09 & 0.10 & 0.01 & 0.13 \\
3418 & KOI-3184 & 0.23 & 0.23 & 0.27 & 0.23 & 0.23 & 0.25 & 0.18 & 0.25 & 0.21 & 0.21 & 0.22 & 0.24 & 0.23 & 0.23 & 0.24 \\
3419 & KOI-4367 & -0.02 & 0.15 & 0.23 & 0.05 & -0.04 & -0.15 & 0.03 & 0.02 & 0.08 & 0.17 & 0.03 & -0.17 & 0.00 & -0.10 & 0.03 \\
3420 & KOI-4004 & -0.13 & 0.16 & -0.10 & -0.23 & -0.14 & -0.20 & -0.06 & -0.01 & 0.02 & -0.03 & -0.02 & -0.16 & -0.03 & -0.20 & 0.01 \\
3421 & KOI-2120 & -0.13 & -0.36 & -0.15 & -0.11 & -0.12 & -0.14 & -0.08 & 0.01 & -0.08 & -0.12 & -0.08 & -0.16 & -0.09 & -0.14 & -0.14 \\
3422 & KOI-4639 & -0.11 & 0.31 & 0.76 & 0.19 & 0.14 & 0.05 & 0.25 & 0.38 & 0.36 & -0.04 & 0.31 & 0.07 & 0.34 & 0.13 & 0.38 \\
3423 & KOI-633 & -0.13 & -0.10 & -0.03 & -0.21 & -0.10 & -0.11 & -0.11 & -0.08 & -0.05 & -0.03 & -0.20 & -0.37 & -0.15 & -0.21 & -0.31 \\
3424 & KOI-632 & -0.01 & -0.17 & 0.08 & -0.03 & -0.01 & 0.05 & 0.03 & 0.07 & 0.02 & 0.04 & 0.02 & -0.04 & 0.05 & 0.00 & 0.02 \\
3425 & KOI-232 & 0.09 & -0.26 & 0.11 & -0.05 & -0.03 & -0.02 & -0.10 & -0.08 & -0.01 & -0.29 & -0.05 & -0.07 & -0.06 & -0.09 & -0.01 \\
3426 & Kepler-122 & -0.05 & 0.79 & 0.09 & -0.13 & -0.05 & -0.06 & -0.01 & -0.04 & 0.02 & -0.04 & -0.04 & -0.17 & -0.03 & -0.11 & 0.01 \\
3427 & KOI-3823 & -0.03 & -0.07 & 0.03 & -0.10 & -0.01 & 0.00 & -0.00 & 0.07 & 0.04 & 0.02 & 0.05 & -0.02 & 0.02 & -0.03 & 0.21 \\
3428 & KOI-3936 & 0.09 & -0.08 & 0.07 & 0.10 & 0.05 & 0.09 & 0.19 & 0.23 & 0.11 & 0.09 & 0.14 & 0.16 & 0.19 & 0.08 & 0.01 \\
3429 & KOI-1665 & 0.25 & 0.53 & 0.27 & 0.42 & 0.29 & 0.34 & 0.36 & 0.32 & 0.27 & 0.28 & 0.31 & 0.42 & 0.34 & 0.37 & 0.32 \\
3430 & KOI-4018 & -0.18 & -0.18 & -0.13 & -0.22 & -0.16 & -0.15 & -0.13 & -0.10 & -0.05 & -0.10 & -0.05 & -0.17 & -0.09 & -0.14 & -0.01 \\
3431 & KOI-2635 & -0.17 & -0.52 & 0.04 & -0.24 & -0.14 & -0.21 & -0.14 & -0.08 & -0.06 & -0.20 & -0.16 & -0.33 & -0.12 & -0.16 & -0.18 \\
3432 & KOI-5107 & -0.25 & 0.04 & -0.13 & -0.16 & -0.11 & -0.09 & -0.23 & -0.08 & -0.05 & -0.14 & -0.11 & -0.06 & -0.02 & -0.05 & 0.19 \\
3433 & KOI-3770 & -0.09 & 0.06 & 0.15 & -0.07 & -0.03 & -0.11 & -0.02 & 0.05 & 0.12 & 0.03 & -0.00 & -0.27 & 0.02 & -0.07 & 0.19 \\
3434 & KOI-5119 & -0.09 & 0.19 & 0.18 & -0.02 & -0.03 & -0.03 & -0.12 & 0.08 & 0.03 & -0.03 & 0.10 & 0.14 & 0.13 & 0.09 & 0.34 \\
3435 & KOI-4546 & 0.07 & -0.19 & 0.09 & 0.02 & 0.07 & -0.01 & 0.06 & 0.01 & 0.14 & 0.11 & 0.06 & 0.02 & 0.07 & 0.08 & 0.14 \\
3436 & KOI-2951 & -0.20 & -0.12 & -0.11 & -0.22 & -0.21 & -0.21 & -0.19 & -0.14 & -0.13 & 0.05 & -0.20 & -0.36 & -0.23 & -0.32 & -0.03 \\
3437 & KOI-3421 & -0.03 & 0.35 & 0.32 & 0.01 & 0.06 & -0.06 & 0.10 & 0.12 & 0.19 & 0.14 & 0.11 & -0.03 & 0.13 & 0.08 & 0.10 \\
3438 & KOI-1666 & -0.03 & 0.90 & 0.36 & 0.23 & 0.11 & -0.04 & 0.09 & 0.19 & 0.33 & 0.19 & 0.13 & 0.01 & 0.17 & 0.06 & 0.13 \\
3439 & KOI-635 & 0.05 & 0.34 & 0.08 & -0.05 & 0.04 & 0.15 & 0.05 & 0.13 & 0.09 & -0.13 & 0.11 & 0.04 & 0.10 & 0.08 & 0.13 \\
3440 & KOI-161 & 0.35 & 0.27 & 0.28 & 0.50 & 0.31 & 0.37 & 0.32 & 0.35 & 0.32 & 0.31 & 0.32 & 0.38 & 0.37 & 0.35 & 0.17 \\
3441 & KOI-639 & -0.00 & 0.42 & 0.25 & 0.03 & 0.06 & -0.02 & 0.04 & 0.11 & 0.12 & -0.11 & 0.09 & -0.03 & 0.10 & 0.06 & 0.10 \\
3442 & KOI-3093 & -0.02 & 0.11 & 0.00 & -0.04 & 0.01 & 0.08 & 0.03 & 0.17 & 0.11 & 0.21 & 0.10 & -0.06 & 0.06 & -0.01 & 0.20 \\
3443 & Kepler-130 & -0.06 & -0.44 & -0.13 & -0.17 & -0.06 & -0.06 & -0.12 & -0.11 & -0.01 & -0.08 & -0.10 & -0.25 & -0.12 & -0.12 & -0.15 \\
3444 & KOI-282 & -0.15 & 0.08 & -0.10 & -0.25 & -0.12 & -0.22 & -0.14 & -0.11 & -0.09 & -0.18 & -0.16 & -0.29 & -0.16 & -0.19 & -0.23 \\
3445 & KOI-4331 & -0.01 & -0.04 & 0.16 & -0.04 & 0.05 & -0.03 & 0.06 & 0.11 & 0.13 & 0.07 & 0.12 & -0.04 & 0.10 & 0.04 & 0.06 \\
3446 & KOI-1822 & -0.12 & 0.60 & -0.11 & -0.31 & -0.17 & -0.19 & -0.15 & -0.16 & -0.16 & -0.22 & -0.15 & -0.35 & -0.19 & -0.26 & -0.14 \\
3447 & KOI-640 & -0.00 & -0.07 & 0.02 & 0.05 & 0.07 & 0.15 & 0.09 & 0.10 & 0.10 & 0.12 & 0.10 & 0.07 & 0.10 & 0.10 & 0.04 \\
3448 & KOI-2698 & 0.08 & 0.17 & 0.14 & 0.07 & 0.07 & 0.10 & 0.09 & 0.10 & 0.06 & 0.07 & 0.12 & 0.00 & 0.09 & 0.09 & 0.25 \\
3449 & KOI-1563 & 0.05 & 0.19 & 0.10 & 0.09 & 0.03 & 0.12 & 0.03 & 0.12 & 0.04 & 0.05 & 0.08 & 0.10 & 0.07 & 0.01 & -0.05 \\
3450 & KOI-3474 & -0.11 & -0.41 & -0.06 & -0.09 & -0.09 & -0.22 & -0.13 & -0.05 & 0.01 & -0.05 & -0.08 & -0.28 & -0.12 & -0.14 & 0.31 \\
3451 & KOI-2158 & -0.02 & -0.03 & 0.16 & -0.06 & 0.03 & 0.10 & -0.02 & -0.01 & 0.07 & 0.01 & -0.09 & -0.19 & -0.09 & -0.05 & -0.18 \\
3452 & KOI-2563 & 0.06 & -0.30 & 0.31 & 0.12 & 0.05 & 0.18 & 0.07 & 0.18 & 0.17 & 0.19 & 0.20 & -0.02 & 0.16 & 0.10 & 0.34 \\
3453 & KOI-4246 & 0.06 & 0.01 & 0.15 & 0.13 & 0.09 & 0.06 & 0.16 & 0.23 & 0.18 & 0.20 & 0.21 & 0.17 & 0.21 & 0.16 & 0.26 \\
3454 & KOI-1576 & 0.08 & 0.21 & 0.10 & 0.21 & 0.12 & 0.12 & 0.12 & 0.14 & 0.10 & 0.11 & 0.15 & 0.15 & 0.14 & 0.14 & 0.17 \\
3455 & KOI-825 & 0.10 & 0.13 & -0.02 & 0.31 & 0.22 & 0.25 & 0.22 & 0.24 & 0.19 & 0.19 & 0.18 & 0.17 & 0.19 & 0.24 & -0.14 \\
3456 & KOI-4713 & 0.11 & -11.62 & 0.24 & 0.18 & 0.07 & -0.07 & 0.24 & 0.07 & 0.40 & 0.48 & 0.21 & -0.00 & 0.15 & 0.16 & 1.16 \\
3457 & KOI-4411 & -0.10 & -0.02 & -0.04 & -0.24 & -0.16 & -0.31 & -0.18 & -0.12 & -0.15 & -0.34 & -0.17 & -0.37 & -0.16 & -0.26 & -0.07 \\
3458 & KOI-3239 & -0.04 & -0.18 & 0.10 & -0.15 & -0.09 & -0.14 & -0.05 & 0.04 & 0.01 & 0.01 & 0.04 & -0.18 & 0.01 & -0.10 & 0.11 \\
3459 & KOI-2711 & 0.07 & 0.05 & 0.06 & -0.07 & 0.02 & 0.01 & 0.00 & 0.05 & 0.04 & -0.06 & 0.09 & -0.03 & 0.08 & 0.02 & 0.11 \\
3460 & KOI-1589 & -0.17 & -0.58 & 0.06 & -0.00 & -0.09 & -0.26 & 0.02 & -0.04 & 0.03 & -0.03 & -0.08 & -0.23 & -0.06 & -0.11 & -0.02 \\
3461 & KOI-408 & 0.04 & 0.88 & -0.53 & 0.20 & 0.29 & -0.01 & 0.15 & 0.84 & 0.34 & 0.33 & 0.25 & -0.43 & 0.26 & 0.87 & 0.11 \\
3462 & KOI-644 & -0.11 & 0.18 & 0.13 & -0.12 & -0.08 & -0.05 & -0.07 & -0.06 & 0.06 & -0.14 & -0.14 & -0.25 & -0.11 & -0.11 & -0.18 \\
3463 & KOI-2370 & -0.27 & 0.89 & 0.04 & -0.52 & -0.13 & -0.40 & -0.07 & -0.02 & -0.13 & -0.82 & -0.13 & -0.40 & -0.09 & -0.29 & 0.08 \\
3464 & KOI-2555 & -0.07 & 0.20 & 0.08 & -0.31 & -0.08 & -0.13 & -0.02 & -0.06 & -0.03 & -0.08 & -0.05 & -0.25 & -0.05 & -0.09 & -0.04 \\
3465 & KOI-2011 & -0.22 & -0.21 & 0.21 & -0.04 & -0.09 & -0.37 & 0.01 & 0.10 & 0.04 & -0.94 & -0.02 & -0.24 & -0.01 & -0.17 & 0.04 \\
3466 & KOI-2219 & 0.18 & 0.20 & 0.25 & 0.21 & 0.10 & 0.15 & 0.16 & 0.14 & 0.11 & 0.12 & 0.09 & 0.12 & 0.14 & 0.15 & -0.07 \\
3467 & KOI-1825 & -0.01 & -0.04 & 0.10 & -0.06 & -0.03 & -0.05 & -0.06 & 0.13 & 0.04 & -0.03 & 0.08 & 0.02 & 0.06 & -0.03 & 0.26 \\
3468 & KOI-2440 & 0.24 & 0.33 & 0.26 & 0.39 & 0.24 & 0.27 & 0.25 & 0.26 & 0.25 & 0.23 & 0.26 & 0.35 & 0.26 & 0.30 & 0.20 \\
3469 & KOI-1557 & -0.18 & -0.25 & -0.19 & -0.07 & -0.04 & -0.13 & -0.00 & 0.06 & 0.00 & 0.01 & -0.05 & -0.04 & -0.00 & -0.05 & -0.15 \\
3470 & KOI-829 & 0.01 & -0.11 & 0.17 & 0.02 & 0.05 & 0.06 & 0.00 & 0.05 & 0.04 & 0.00 & 0.03 & 0.00 & 0.02 & -0.00 & 0.01 \\
3471 & KOI-2556 & -0.18 & -0.33 & -0.20 & -0.30 & -0.17 & -0.14 & -0.17 & -0.23 & -0.15 & -0.14 & -0.24 & -0.36 & -0.24 & -0.23 & -0.27 \\
3472 & KOI-2690 & -0.05 & -0.02 & 0.02 & -0.07 & -0.04 & -0.08 & 0.03 & 0.08 & 0.03 & -0.03 & 0.06 & -0.03 & 0.05 & -0.04 & 0.14 \\
3473 & KOI-645 & -0.24 & -0.26 & -0.19 & -0.24 & -0.24 & -0.20 & -0.28 & -0.23 & -0.15 & -0.26 & -0.25 & -0.25 & -0.24 & -0.24 & -0.24 \\
3474 & KOI-3039 & -0.23 & -0.11 & 0.02 & -0.29 & -0.21 & -0.22 & -0.23 & -0.22 & -0.08 & -0.21 & -0.28 & -0.57 & -0.30 & -0.26 & 0.20 \\
3475 & KOI-1567 & 0.04 & -0.10 & 0.09 & -0.07 & -0.02 & 0.00 & -0.13 & -0.04 & 0.00 & -0.05 & -0.16 & -0.27 & -0.12 & -0.11 & -0.43 \\
3476 & KOI-4907 & 0.03 & -0.10 & 0.16 & 0.06 & 0.06 & 0.01 & 0.06 & 0.09 & 0.08 & 0.08 & 0.09 & 0.07 & 0.08 & 0.06 & 0.05 \\
3477 & KOI-834 & 0.21 & 0.34 & 0.25 & 0.34 & 0.26 & 0.37 & 0.24 & 0.29 & 0.23 & 0.21 & 0.30 & 0.28 & 0.28 & 0.35 & 0.12 \\
3478 & KOI-3791 & 0.12 & 0.32 & 0.30 & 0.11 & 0.13 & 0.23 & 0.17 & 0.10 & 0.26 & 0.08 & 0.10 & -0.07 & 0.10 & 0.07 & 0.06 \\
3479 & KOI-1601 & -0.10 & -0.14 & 0.10 & -0.12 & -0.06 & 0.06 & -0.06 & -0.08 & 0.03 & -0.06 & -0.14 & -0.32 & -0.16 & -0.13 & -0.25 \\
3480 & KOI-2970 & -0.04 & 0.43 & 0.04 & -0.15 & -0.05 & -0.11 & -0.06 & 0.05 & -0.00 & -0.14 & -0.07 & -0.33 & -0.07 & -0.11 & 0.07 \\
3481 & KOI-142 & 0.17 & 0.30 & 0.21 & 0.27 & 0.15 & 0.20 & 0.17 & 0.17 & 0.18 & 0.17 & 0.21 & 0.28 & 0.20 & 0.20 & 0.11 \\
3482 & KOI-2707 & -0.11 & -0.11 & -0.08 & -0.17 & -0.09 & -0.20 & -0.18 & -0.10 & -0.10 & -0.15 & -0.12 & -0.15 & -0.14 & -0.18 & -0.03 \\
3483 & Kepler-399 & -0.15 & -0.27 & -0.16 & -0.21 & -0.18 & -0.13 & -0.13 & -0.13 & -0.09 & -0.09 & -0.18 & -0.20 & -0.17 & -0.20 & -0.09 \\
3484 & KOI-4368 & -0.01 & 0.07 & 0.23 & -0.05 & -0.06 & -0.03 & 0.02 & 0.05 & 0.03 & -0.11 & 0.05 & -0.08 & 0.06 & -0.01 & 0.21 \\
3485 & KOI-409 & 0.11 & 0.18 & 0.12 & 0.12 & 0.15 & 0.20 & 0.14 & 0.14 & 0.19 & 0.14 & 0.16 & 0.18 & 0.16 & 0.18 & 0.24 \\
3486 & KOI-647 & -0.27 & 0.16 & -0.20 & -0.30 & -0.30 & -0.34 & -0.26 & -0.14 & -0.20 & -0.25 & -0.42 & -0.80 & -0.41 & -0.49 & -0.41 \\
3487 & KOI-2741 & -0.00 & -0.01 & 0.05 & -0.04 & 0.04 & 0.06 & -0.02 & 0.08 & 0.04 & 0.02 & 0.04 & -0.06 & 0.05 & 0.01 & 0.05 \\
3488 & KOI-257 & 0.13 & 0.33 & 0.10 & 0.05 & 0.12 & 0.04 & 0.14 & 0.15 & 0.21 & 0.12 & 0.18 & 0.14 & 0.17 & 0.15 & 0.18 \\
3489 & KOI-1590 & 0.01 & -0.43 & -0.14 & 0.04 & -0.03 & 0.02 & 0.25 & -0.00 & 0.04 & -0.02 & -0.13 & -0.02 & 0.02 & 0.01 & -0.29 \\
3490 & KOI-2854 E & 0.14 & 0.47 & 0.14 & 0.04 & 0.07 & 0.04 & 0.03 & 0.13 & 0.12 & 0.15 & 0.14 & -0.06 & 0.10 & 0.06 & 0.18 \\
3491 & KOI-2854 W & 0.09 & 0.20 & 0.03 & 0.04 & 0.07 & 0.11 & 0.07 & 0.10 & 0.09 & 0.01 & 0.07 & 0.10 & 0.08 & 0.05 & 0.21 \\
3492 & KOI-2668 & -0.20 & -0.33 & -0.15 & -0.11 & -0.10 & -0.10 & -0.09 & -0.04 & -0.06 & -0.14 & -0.08 & -0.24 & -0.10 & -0.15 & 0.08 \\
3493 & KOI-837 & 0.76 & 0.66 & 0.82 & 0.83 & 0.36 & 0.49 & 0.41 & 0.43 & 0.39 & 0.35 & 0.40 & 0.47 & 0.44 & 0.50 & 0.21 \\
3494 & KOI-1621 & -0.06 & 0.14 & 0.27 & 0.07 & 0.00 & -0.01 & 0.10 & 0.12 & 0.16 & -0.04 & 0.08 & -0.08 & 0.09 & 0.03 & 0.15 \\
3495 & KOI-4067 & 0.02 & 0.24 & 0.09 & -0.01 & 0.04 & 0.07 & 0.10 & 0.12 & 0.05 & 0.04 & 0.07 & -0.01 & 0.09 & 0.04 & 0.05 \\
3496 & Kepler-338 & -0.04 & 0.00 & 0.09 & -0.10 & -0.08 & -0.07 & -0.05 & -0.00 & 0.03 & -0.07 & -0.02 & -0.08 & -0.00 & -0.06 & 0.02 \\
3497 & KOI-1930 & -0.08 & -0.43 & 0.05 & -0.13 & -0.10 & -0.21 & -0.09 & 0.00 & -0.02 & -0.10 & -0.09 & -0.16 & -0.04 & -0.09 & -0.10 \\
3498 & KOI-2332 & -0.03 & -0.07 & 0.20 & -0.12 & -0.02 & 0.07 & -0.09 & -0.08 & -0.01 & -0.07 & -0.14 & -0.25 & -0.11 & -0.08 & -0.14 \\
3499 & KOI-1962 & -0.08 & -0.26 & 0.12 & -0.06 & -0.06 & -0.03 & -0.05 & -0.03 & -0.04 & -0.09 & -0.06 & -0.16 & -0.06 & -0.08 & -0.18 \\
3500 & KOI-649 & 0.08 & 0.13 & 0.42 & 0.34 & 0.14 & 0.08 & 0.21 & 0.33 & 0.24 & 0.08 & 0.25 & 0.23 & 0.26 & 0.22 & 0.26 \\
3501 & KOI-2915 & -0.10 & -0.02 & -0.03 & -0.11 & -0.05 & -0.02 & -0.04 & -0.09 & -0.03 & -0.07 & -0.09 & -0.11 & -0.08 & -0.05 & -0.08 \\
3502 & KOI-2790 & 0.09 & -0.24 & 0.33 & -0.13 & -0.11 & 0.00 & -0.03 & -0.13 & -0.04 & -0.11 & -0.29 & -0.37 & -0.28 & -0.21 & -0.39 \\
3503 & KOI-371 & -0.08 & 0.24 & -0.05 & -0.05 & 0.01 & -0.05 & -0.10 & 0.04 & 0.03 & -0.04 & 0.06 & 0.02 & 0.07 & 0.03 & 0.23 \\
3504 & KOI-2369 & 0.06 & 0.04 & 0.18 & 0.11 & 0.04 & 0.10 & 0.07 & 0.08 & 0.03 & 0.08 & 0.08 & 0.04 & 0.09 & 0.05 & 0.00 \\
3505 & KOI-2676 & -0.09 & 0.32 & 0.30 & -0.03 & -0.06 & -0.13 & -0.03 & 0.10 & -0.00 & -0.08 & 0.05 & -0.36 & 0.01 & -0.12 & 0.18 \\
3506 & KOI-2010 & -0.18 & -0.11 & 0.26 & 0.05 & -0.01 & -0.42 & 0.00 & 0.12 & 0.09 & 0.22 & 0.07 & -0.19 & 0.09 & -0.06 & 0.05 \\
3507 & KOI-2752 & 0.05 & 0.52 & 0.35 & 0.13 & 0.13 & 0.03 & 0.16 & 0.19 & 0.25 & 0.23 & 0.18 & 0.14 & 0.20 & 0.19 & 0.15 \\
3508 & KOI-2183 & 0.00 & -0.04 & -0.01 & -0.06 & 0.05 & -0.05 & 0.02 & 0.06 & 0.05 & 0.01 & 0.06 & 0.03 & 0.06 & 0.03 & -0.10 \\
3509 & KOI-505 & 0.20 & 0.07 & 0.17 & 0.18 & 0.10 & 0.14 & 0.12 & 0.11 & 0.15 & 0.13 & 0.16 & 0.17 & 0.17 & 0.13 & 0.07 \\
3510 & Kepler-169 & 0.04 & 0.06 & 0.05 & 0.19 & 0.02 & 0.19 & 0.07 & 0.17 & 0.07 & 0.07 & 0.14 & 0.17 & 0.10 & 0.09 & -0.03 \\
3511 & KOI-555 & -0.03 & -0.07 & -0.00 & -0.00 & 0.02 & 0.07 & 0.00 & 0.01 & 0.05 & 0.03 & 0.03 & -0.02 & 0.02 & 0.03 & -0.02 \\
3512 & KOI-4744 & 0.23 & 0.19 & 0.38 & 0.28 & 0.19 & 0.23 & 0.20 & 0.21 & 0.20 & 0.17 & 0.22 & 0.29 & 0.23 & 0.24 & 0.29 \\
3513 & KOI-2358 & -0.05 & 0.61 & 0.47 & 0.18 & 0.07 & -0.10 & 0.17 & 0.22 & 0.19 & 0.12 & 0.20 & 0.06 & 0.24 & 0.12 & 0.12 \\
3514 & KOI-1897 & -0.08 & -0.11 & -0.03 & -0.12 & -0.11 & -0.01 & -0.09 & -0.08 & -0.09 & -0.22 & -0.12 & -0.19 & -0.11 & -0.15 & -0.16 \\
3515 & KOI-2675 & -0.05 & -0.13 & -0.05 & -0.09 & -0.05 & -0.08 & -0.03 & 0.09 & 0.04 & 0.01 & 0.08 & -0.05 & 0.06 & -0.08 & 0.12 \\
3516 & KOI-3288 & -0.05 & -0.18 & -0.08 & -0.13 & -0.03 & -0.14 & -0.00 & 0.02 & -0.01 & -0.03 & 0.02 & -0.05 & 0.01 & -0.05 & 0.05 \\
3517 & KOI-650 & 0.02 & -0.09 & 0.02 & 0.09 & 0.06 & 0.01 & 0.05 & 0.05 & 0.07 & 0.08 & 0.02 & 0.01 & 0.04 & 0.03 & -0.10 \\
3518 & KOI-1928 & 0.07 & 0.06 & 0.10 & 0.11 & 0.15 & 0.15 & 0.16 & 0.23 & 0.16 & 0.12 & 0.18 & 0.16 & 0.18 & 0.18 & 0.22 \\
3519 & KOI-4686 & 0.18 & 0.33 & 0.28 & 0.34 & 0.23 & 0.28 & 0.24 & 0.32 & 0.25 & 0.19 & 0.26 & 0.40 & 0.29 & 0.33 & 0.15 \\
3520 & KOI-4002 & 0.03 & 0.12 & 0.06 & 0.09 & 0.11 & 0.18 & 0.06 & 0.15 & 0.17 & 0.16 & 0.18 & 0.08 & 0.16 & 0.15 & 0.08 \\
3521 & KOI-652 & -0.03 & -0.16 & -0.04 & -0.05 & 0.03 & 0.02 & 0.17 & 0.17 & 0.06 & 0.09 & 0.12 & -0.00 & 0.07 & 0.04 & -0.09 \\
3522 & KOI-4913 & -0.08 & 0.04 & 0.15 & -0.18 & 0.05 & -0.18 & 0.08 & 0.14 & 0.11 & -0.51 & 0.13 & 0.09 & 0.13 & 0.02 & 0.13 \\
3523 & KOI-3422 & 0.06 & 0.15 & 0.09 & -0.01 & 0.03 & 0.00 & 0.05 & 0.14 & 0.09 & 0.09 & 0.15 & 0.08 & 0.12 & 0.04 & 0.20 \\
3524 & KOI-4156 & 0.17 & 0.26 & 0.27 & 0.14 & 0.21 & 0.33 & 0.24 & 0.28 & 0.27 & 0.21 & 0.23 & 0.20 & 0.23 & 0.26 & 0.36 \\
3525 & KOI-1060 & -0.07 & -8.50 & -0.11 & -0.29 & -0.20 & -0.10 & -0.19 & -0.27 & -0.26 & -1.07 & -0.30 & -0.31 & -0.23 & -0.32 & -0.19 \\
3526 & Kepler-758 & -0.59 & 0.05 & 0.04 & -0.25 & -0.20 & 0.00 & 0.02 & -0.16 & 0.00 & -0.02 & -0.21 & -0.47 & -0.17 & -0.33 & -0.42 \\
3527 & KOI-2801 & -0.05 & 0.03 & 0.10 & -0.09 & 0.03 & 0.00 & -0.00 & 0.11 & 0.13 & -0.06 & 0.03 & -0.18 & 0.05 & 0.02 & 0.06 \\
3528 & KOI-1839 & -0.06 & -0.44 & -0.17 & -0.05 & -0.00 & 0.03 & 0.04 & 0.13 & 0.15 & 0.13 & 0.03 & 0.04 & 0.08 & -0.01 & -0.04 \\
3529 & KOI-2498 & -0.06 & -2.57 & 0.10 & -0.21 & -0.06 & -0.10 & -0.10 & -0.11 & -0.02 & -0.08 & -0.15 & -0.25 & -0.14 & -0.13 & -0.27 \\
3530 & KOI-4633 & 0.06 & -0.00 & 0.15 & 0.05 & 0.05 & -0.00 & 0.07 & 0.06 & 0.09 & 0.07 & 0.13 & 0.07 & 0.11 & 0.09 & 0.17 \\
3531 & KOI-654 & -0.07 & -0.14 & -0.08 & -0.19 & -0.06 & -0.07 & -0.07 & -0.01 & -0.06 & -0.00 & -0.02 & -0.09 & -0.03 & -0.08 & -0.05 \\
3532 & KOI-1052 & -0.17 & 0.59 & -0.12 & -0.08 & -0.07 & -0.00 & -0.08 & -0.04 & -0.07 & -0.25 & -0.05 & -0.32 & -0.07 & -0.15 & -0.33 \\
3533 & KOI-3190 & -0.09 & -0.09 & -0.07 & -0.16 & -0.10 & -0.27 & -0.16 & -0.09 & -0.03 & -0.08 & -0.10 & -0.29 & -0.11 & -0.14 & -0.11 \\
3534 & KOI-655 & -0.02 & 0.07 & 0.16 & -0.04 & -0.05 & -0.10 & -0.02 & 0.01 & 0.01 & -0.06 & -0.00 & -0.15 & -0.00 & -0.07 & 0.03 \\
3535 & KOI-2479 & -0.10 & -0.05 & -0.07 & -0.06 & -0.03 & -0.02 & -0.07 & -0.03 & -0.03 & -0.07 & -0.02 & -0.04 & 0.01 & -0.03 & 0.08 \\
3536 & KOI-2250 & -0.09 & -0.26 & -0.20 & 0.15 & 0.03 & 0.13 & 0.08 & 0.21 & 0.09 & 0.10 & 0.08 & 0.10 & 0.13 & 0.09 & -0.23 \\
3537 & KOI-303 & -0.17 & -0.15 & 0.00 & -0.18 & -0.07 & 0.02 & -0.11 & -0.14 & -0.03 & -0.15 & -0.22 & -0.41 & -0.22 & -0.20 & -0.36 \\
3538 & KOI-2733 & -0.14 & -0.45 & -0.26 & -0.07 & -0.10 & -0.00 & -0.01 & 0.08 & -0.04 & -0.06 & -0.03 & -0.01 & 0.00 & -0.07 & -0.06 \\
3539 & KOI-2148 & 0.29 & 0.36 & 0.25 & 0.44 & 0.30 & 0.36 & 0.31 & 0.35 & 0.33 & 0.29 & 0.36 & 0.48 & 0.39 & 0.42 & 0.32 \\
3540 & Kepler-363 & 0.28 & 0.30 & 0.26 & 0.47 & 0.32 & 0.37 & 0.29 & 0.38 & 0.31 & 0.28 & 0.36 & 0.42 & 0.36 & 0.41 & 0.27 \\
3541 & KOI-1054 & -0.77 & 0.26 & -0.06 & -1.05 & -0.74 & -1.07 & -0.65 & -0.46 & -0.28 & -0.66 & -0.61 & -1.53 & -0.62 & -0.77 & -0.05 \\
3542 & KOI-2167 & 0.01 & 0.03 & 0.05 & -0.03 & 0.03 & 0.01 & -0.02 & 0.15 & 0.07 & 0.12 & 0.12 & 0.03 & 0.09 & 0.03 & 0.16 \\
3543 & KOI-2071 & 0.09 & -0.04 & 0.06 & 0.15 & 0.11 & 0.12 & 0.13 & 0.11 & 0.12 & 0.11 & 0.12 & 0.13 & 0.12 & 0.14 & -0.04 \\
3544 & KOI-1684 & -1.00 & -0.05 & 0.21 & 0.05 & -0.03 & -0.35 & -0.14 & -0.39 & -0.30 & 0.38 & -0.16 & -0.40 & -0.05 & -0.23 & -0.25 \\
3545 & KOI-1916 & 0.14 & 0.33 & 0.14 & 0.31 & 0.13 & 0.22 & 0.18 & 0.29 & 0.25 & 0.32 & 0.24 & 0.29 & 0.23 & 0.19 & 0.16 \\
3546 & Kepler-336 & 0.12 & 0.27 & 0.07 & 0.26 & 0.11 & 0.27 & 0.20 & 0.28 & 0.31 & 0.39 & 0.22 & 0.28 & 0.22 & 0.15 & 0.21 \\
3547 & KOI-2949 & 0.01 & -0.00 & 0.04 & -0.06 & 0.03 & -0.00 & 0.01 & 0.08 & 0.01 & -0.01 & 0.04 & -0.06 & 0.06 & 0.06 & 0.03 \\
3548 & KOI-3500 & 0.09 & 0.08 & 0.36 & 0.25 & 0.07 & 0.20 & 0.11 & 0.24 & 0.17 & 0.07 & 0.18 & 0.23 & 0.19 & 0.16 & 0.26 \\
3549 & Kepler-132 & -0.15 & -0.09 & -0.07 & -0.21 & -0.19 & -0.32 & -0.17 & -0.19 & -0.16 & -0.14 & -0.23 & -0.37 & -0.21 & -0.25 & -0.29 \\
3550 & KOI-284 & -0.16 & -0.17 & -0.06 & -0.13 & -0.12 & -0.10 & -0.09 & -0.11 & -0.02 & -0.20 & -0.17 & -0.36 & -0.16 & -0.16 & -0.24 \\
3551 & KOI-4276 & -0.01 & 0.13 & 0.36 & 0.06 & 0.01 & 0.01 & 0.10 & 0.19 & 0.24 & 0.09 & 0.17 & 0.01 & 0.18 & 0.08 & 0.30 \\
3552 & KOI-304 & -0.15 & -0.24 & -0.17 & -0.25 & -0.20 & -0.26 & -0.18 & -0.12 & -0.14 & -0.34 & -0.19 & -0.29 & -0.19 & -0.25 & -0.14 \\
3553 & KOI-2001 & -0.02 & -0.27 & -0.06 & -0.04 & -0.03 & -0.06 & 0.06 & 0.07 & 0.01 & -0.03 & 0.07 & -0.03 & 0.05 & -0.01 & 0.16 \\
3554 & KOI-306 & -0.03 & -0.19 & -0.03 & -0.03 & 0.02 & 0.05 & 0.07 & 0.14 & 0.08 & 0.06 & 0.10 & 0.03 & 0.12 & 0.03 & 0.21 \\
3555 & Kepler-203 & 0.01 & -0.17 & 0.08 & -0.00 & 0.06 & 0.05 & 0.03 & 0.09 & 0.05 & 0.10 & 0.10 & 0.01 & 0.07 & 0.03 & 0.15 \\
3556 & KOI-659 & 0.02 & 0.36 & 0.12 & -0.01 & -0.05 & -0.21 & 0.01 & 0.07 & 0.03 & -0.10 & 0.03 & -0.18 & 0.03 & -0.05 & 0.05 \\
3557 & KOI-2098 & -0.21 & 0.91 & -0.13 & -0.16 & -0.12 & 0.08 & -0.17 & -0.02 & -0.03 & -0.49 & -0.13 & -0.27 & -0.08 & -0.23 & -0.22 \\
3558 & KOI-3179 & -0.04 & -0.31 & -0.03 & -0.08 & -0.01 & -0.06 & 0.01 & 0.06 & 0.04 & 0.06 & 0.04 & -0.08 & 0.02 & -0.03 & 0.08 \\
3559 & KOI-4123 & 0.05 & 0.03 & 0.33 & 0.12 & 0.04 & 0.02 & 0.13 & 0.25 & 0.19 & -0.11 & 0.18 & 0.06 & 0.16 & 0.10 & 0.29 \\
3560 & KOI-2398 & -0.14 & 0.34 & -0.22 & -0.23 & -0.27 & -0.14 & -0.30 & -0.16 & -0.17 & -0.32 & -0.24 & -0.47 & -0.25 & -0.37 & -0.34 \\
3561 & KOI-2829 & -0.01 & 0.21 & 0.01 & -0.01 & -0.01 & -0.07 & 0.01 & 0.01 & 0.01 & -0.04 & 0.00 & -0.09 & -0.00 & -0.00 & -0.03 \\
3562 & Kepler-92 & 0.14 & 0.55 & 0.25 & 0.23 & 0.14 & 0.23 & 0.17 & 0.21 & 0.21 & 0.12 & 0.19 & 0.24 & 0.20 & 0.20 & 0.25 \\
3563 & KOI-285 & 0.12 & 0.31 & 0.17 & 0.26 & 0.14 & 0.22 & 0.14 & 0.20 & 0.21 & 0.09 & 0.19 & 0.17 & 0.20 & 0.21 & 0.31 \\
3564 & KOI-2252 & 0.08 & 0.48 & 0.42 & 0.16 & 0.07 & 0.10 & 0.17 & 0.22 & 0.29 & 0.18 & 0.18 & 0.06 & 0.18 & 0.13 & 0.24 \\
3565 & KOI-3240 & 0.21 & 0.25 & 0.31 & 0.31 & 0.16 & 0.24 & 0.23 & 0.31 & 0.29 & 0.18 & 0.08 & 0.31 & 0.31 & 0.27 & 0.26 \\
3566 & KOI-2636 & 0.04 & -0.16 & -0.01 & -0.09 & 0.02 & -0.02 & 0.01 & 0.07 & 0.03 & 0.09 & 0.07 & 0.02 & 0.06 & 0.02 & 0.08 \\
3567 & KOI-1812 & 0.01 & 0.25 & 0.03 & 0.04 & 0.00 & -0.21 & 0.02 & 0.06 & 0.03 & 0.10 & -0.05 & -0.12 & -0.00 & 0.01 & 0.02 \\
3568 & KOI-308 & -0.05 & 0.33 & 0.34 & 0.08 & -0.04 & -0.14 & 0.03 & 0.18 & 0.05 & 0.07 & 0.07 & -0.10 & 0.09 & -0.08 & 0.01 \\
3569 & KOI-2608 & -0.23 & -0.03 & 0.20 & -0.28 & -0.09 & -0.41 & -0.00 & 0.21 & 0.07 & -0.11 & 0.03 & -0.17 & 0.08 & -0.12 & 0.08 \\
3570 & KOI-415 & -0.13 & -0.41 & 0.08 & -0.26 & -0.08 & -0.07 & -0.07 & -0.16 & 0.02 & -0.06 & -0.23 & -0.49 & -0.23 & -0.17 & -0.22 \\
3571 & KOI-4302 & -0.09 & 0.30 & 0.08 & -0.11 & -0.08 & -0.24 & -0.11 & -0.02 & 0.04 & 0.02 & -0.09 & -0.35 & -0.07 & -0.11 & -0.12 \\
3572 & KOI-1688 & 0.08 & -18.51 & 0.16 & 0.14 & 0.13 & 0.46 & 0.15 & 0.26 & 0.20 & 0.16 & 0.22 & 0.12 & 0.19 & 0.19 & 0.43 \\
3573 & KOI-660 & -0.18 & -0.25 & -0.05 & -0.22 & -0.11 & -0.08 & -0.19 & -0.11 & -0.09 & -0.15 & -0.16 & -0.24 & -0.13 & -0.14 & -0.13 \\
3574 & KOI-307 & -0.13 & -0.80 & -0.11 & -0.36 & -0.10 & -0.28 & -0.14 & -0.11 & -0.04 & -0.15 & -0.12 & -0.28 & -0.11 & -0.16 & -0.06 \\
3575 & KOI-1613 & -0.42 & -1.31 & -0.11 & -0.36 & -0.31 & -0.46 & -0.31 & -0.24 & -0.13 & -0.12 & -0.27 & -0.61 & -0.31 & -0.33 & -0.32 \\
3576 & KOI-3436 & 0.10 & 0.11 & 0.08 & 0.18 & 0.10 & 0.16 & 0.17 & 0.22 & 0.15 & 0.18 & 0.20 & 0.22 & 0.21 & 0.17 & 0.06 \\
3577 & KOI-219 & -0.01 & 0.23 & 0.27 & 0.18 & 0.09 & -0.00 & 0.15 & 0.25 & 0.19 & 0.00 & 0.13 & 0.09 & 0.18 & 0.14 & -0.06 \\
3578 & KOI-611 & 0.08 & -0.83 & 0.21 & -0.01 & 0.06 & -0.00 & 0.13 & 0.13 & 0.10 & -0.04 & 0.14 & 0.06 & 0.12 & 0.09 & -0.01 \\
3579 & KOI-2753 & 0.12 & 0.31 & 0.20 & 0.22 & 0.16 & 0.19 & 0.17 & 0.15 & 0.15 & 0.11 & 0.16 & 0.23 & 0.18 & 0.20 & 0.16 \\
3580 & KOI-1128 & -0.07 & -0.09 & -0.01 & -0.13 & -0.05 & -0.05 & -0.05 & -0.07 & -0.04 & -0.03 & -0.10 & -0.11 & -0.10 & -0.10 & -0.19 \\
3581 & KOI-662 & 0.02 & 0.06 & 0.04 & -0.15 & 0.01 & 0.06 & -0.04 & 0.02 & 0.11 & -0.02 & 0.00 & -0.20 & 0.04 & -0.01 & 0.03 \\
3582 & KOI-3503 & -0.31 & -0.00 & -0.21 & -0.46 & -0.42 & -0.73 & -0.39 & -0.39 & -0.33 & -0.28 & -0.49 & -0.71 & -0.44 & -0.51 & -0.62 \\
3583 & KOI-661 & 0.00 & 0.14 & 0.11 & -0.07 & -0.01 & -0.02 & 0.02 & 0.00 & 0.02 & 0.12 & 0.04 & -0.04 & 0.04 & -0.04 & 0.12 \\
3584 & KOI-1121 & 0.07 & 0.09 & 0.04 & 0.09 & 0.05 & 0.12 & 0.05 & 0.07 & 0.09 & 0.09 & 0.12 & 0.02 & 0.06 & 0.04 & 0.05 \\
3585 & KOI-1127 & 0.25 & 0.26 & 0.25 & 0.39 & 0.19 & 0.36 & 0.25 & 0.33 & 0.35 & 0.26 & 0.39 & 0.30 & 0.32 & 0.35 & 0.21 \\
3586 & KOI-2857 & 0.15 & 0.13 & 0.25 & 0.20 & 0.21 & 0.24 & 0.22 & 0.29 & 0.32 & 0.35 & 0.30 & 0.23 & 0.29 & 0.27 & 0.33 \\
3587 & KOI-2948 & 0.35 & 0.42 & 0.26 & 0.54 & 0.38 & 0.48 & 0.40 & 0.41 & 0.41 & 0.40 & 0.44 & 0.48 & 0.44 & 0.47 & 0.34 \\
3588 & KOI-3456 & -0.25 & -0.88 & -0.23 & -0.37 & -0.26 & -0.30 & -0.31 & -0.29 & -0.21 & -0.23 & -0.31 & -0.45 & -0.30 & -0.33 & -0.44 \\
3589 & KOI-1230 & -0.28 & 0.12 & -0.06 & -0.15 & -0.13 & -0.19 & -0.24 & -0.00 & -0.08 & -0.16 & -0.03 & -0.05 & 0.01 & -0.07 & 0.26 \\
3590 & KOI-2840 & 0.01 & -0.79 & 0.11 & -0.08 & 0.02 & 0.10 & -0.01 & -0.04 & 0.08 & 0.05 & -0.06 & -0.16 & -0.06 & -0.04 & -0.04 \\
3591 & Kepler-172 & 0.25 & 0.28 & 0.24 & 0.41 & 0.26 & 0.36 & 0.32 & 0.30 & 0.32 & 0.33 & 0.32 & 0.41 & 0.30 & 0.35 & 0.15 \\
3592 & KOI-664 & 0.01 & 0.05 & 0.10 & -0.03 & 0.02 & 0.02 & 0.05 & 0.01 & 0.03 & 0.07 & 0.01 & -0.03 & 0.02 & 0.02 & -0.06 \\
3593 & Kepler-206 & 0.05 & -0.10 & -0.03 & -0.01 & 0.04 & 0.11 & 0.01 & 0.04 & 0.06 & 0.04 & 0.03 & 0.05 & 0.02 & 0.04 & -0.03 \\
3594 & KOI-372 & -0.10 & -0.10 & -0.09 & -0.24 & -0.10 & -0.11 & -0.10 & -0.01 & -0.05 & -0.07 & -0.04 & -0.24 & -0.08 & -0.16 & 0.05 \\
3595 & KOI-1241 & 0.24 & 0.59 & 0.28 & 0.55 & 0.33 & 0.46 & 0.24 & 0.37 & 0.34 & 0.28 & 0.39 & 0.56 & 0.42 & 0.47 & 0.25 \\
3596 & KOI-2408 & -0.19 & -0.16 & -0.24 & -0.25 & -0.11 & -0.10 & -0.12 & -0.13 & -0.09 & -0.10 & -0.16 & -0.27 & -0.15 & -0.18 & -0.19 \\
3597 & KOI-511 & 0.19 & 0.68 & 0.09 & -0.06 & 0.07 & 0.06 & 0.11 & 0.06 & 0.08 & -0.17 & 0.09 & -0.10 & 0.05 & 0.01 & 0.14 \\
3598 & KOI-176 & -0.12 & -1.53 & 0.03 & -0.29 & -0.21 & -0.08 & -0.20 & -0.15 & 0.04 & 0.16 & -0.11 & -0.39 & -0.15 & -0.34 & -0.29 \\
3599 & KOI-94 & 0.07 & 0.34 & 0.22 & 0.13 & 0.06 & 0.01 & 0.14 & 0.15 & 0.16 & 0.13 & 0.14 & 0.09 & 0.14 & 0.08 & 0.11 \\
3600 & KOI-270 & -0.08 & -0.14 & 0.21 & -0.07 & -0.02 & 0.04 & -0.02 & -0.10 & 0.09 & -0.07 & -0.18 & -0.40 & -0.18 & -0.14 & -0.14 \\
3601 & KOI-3117 & 0.00 & 0.03 & -0.04 & 0.01 & -0.02 & 0.05 & 0.02 & 0.08 & 0.01 & 0.03 & 0.07 & 0.02 & 0.04 & -0.02 & 0.10 \\
3602 & KOI-4657 & -0.09 & -0.20 & 0.04 & -0.22 & -0.10 & -0.10 & -0.08 & -0.12 & -0.07 & -0.11 & -0.07 & -0.16 & -0.08 & -0.12 & -0.12 \\
3603 & KOI-3438 & -0.09 & -0.32 & 0.01 & -0.18 & -0.17 & -0.30 & -0.18 & -0.13 & -0.14 & -0.27 & -0.16 & -0.32 & -0.15 & -0.22 & -0.04 \\
3604 & KOI-1239 & -0.13 & 0.22 & -0.07 & -0.11 & -0.11 & -0.24 & -0.07 & -0.14 & -0.10 & -0.07 & -0.14 & -0.23 & -0.10 & -0.15 & -0.23 \\
3605 & KOI-3287 & -0.09 & -0.24 & -0.01 & -0.11 & -0.12 & -0.18 & -0.11 & -0.06 & -0.12 & -0.10 & -0.17 & -0.21 & -0.12 & -0.15 & -0.17 \\
3606 & KOI-857 & 0.14 & 0.07 & 0.07 & 0.19 & 0.16 & 0.18 & 0.13 & 0.23 & 0.22 & 0.23 & 0.23 & 0.21 & 0.22 & 0.22 & 0.12 \\
3607 & KOI-1242 & -0.05 & 0.17 & 0.09 & -0.08 & -0.01 & -0.08 & -0.03 & 0.01 & 0.04 & 0.03 & -0.04 & -0.12 & 0.00 & -0.01 & -0.04 \\
3608 & KOI-2559 & 0.02 & -0.04 & 0.04 & 0.08 & 0.10 & 0.16 & 0.07 & 0.07 & 0.07 & 0.10 & 0.11 & 0.08 & 0.10 & 0.12 & 0.05 \\
3609 & KOI-3237 & 0.05 & -0.39 & 0.05 & 0.04 & 0.06 & 0.03 & 0.13 & 0.20 & 0.13 & 0.16 & 0.15 & 0.10 & 0.14 & 0.09 & 0.21 \\
3610 & KOI-2838 & 0.01 & 0.08 & 0.13 & -0.07 & 0.04 & 0.07 & 0.03 & 0.10 & 0.10 & 0.01 & 0.07 & 0.03 & 0.09 & 0.04 & 0.04 \\
3611 & KOI-1227 & 0.22 & 0.51 & -0.65 & -0.07 & -0.42 & 0.27 & -0.23 & -0.38 & -0.50 & 0.69 & 0.14 & 0.01 & -0.39 & -0.32 & -0.17 \\
3612 & KOI-2737 & 0.23 & 0.35 & 0.31 & 0.34 & 0.23 & 0.31 & 0.25 & 0.31 & 0.27 & 0.24 & 0.28 & 0.32 & 0.30 & 0.31 & 0.21 \\
3613 & KOI-4159 & 0.12 & -0.10 & 0.26 & 0.03 & 0.09 & 0.18 & 0.04 & 0.11 & 0.15 & 0.09 & 0.08 & 0.02 & 0.07 & 0.04 & 0.03 \\
3614 & KOI-1692 & 0.23 & 0.31 & 0.25 & 0.39 & 0.21 & 0.28 & 0.31 & 0.29 & 0.26 & 0.25 & 0.29 & 0.39 & 0.30 & 0.32 & 0.23 \\
3615 & KOI-612 & 0.02 & -0.18 & 0.06 & -0.06 & -0.04 & -0.04 & -0.07 & -0.01 & -0.02 & -0.00 & -0.01 & -0.07 & -0.03 & -0.08 & -0.16 \\
3616 & KOI-666 & 0.03 & 0.01 & 0.04 & 0.02 & 0.05 & 0.04 & 0.02 & 0.02 & 0.06 & 0.09 & 0.07 & 0.10 & 0.07 & 0.02 & 0.04 \\
3617 & KOI-4651 & -0.05 & 0.29 & -0.01 & -0.19 & -0.05 & -0.18 & -0.11 & 0.01 & -0.08 & -0.05 & -0.12 & -0.14 & -0.06 & -0.11 & -0.05 \\
3618 & KOI-665 & 0.20 & 0.30 & 0.23 & 0.36 & 0.19 & 0.25 & 0.25 & 0.27 & 0.24 & 0.21 & 0.28 & 0.37 & 0.28 & 0.29 & 0.28 \\
3619 & Kepler-207 & 0.17 & 0.21 & 0.30 & 0.39 & 0.22 & 0.29 & 0.22 & 0.27 & 0.27 & 0.22 & 0.27 & 0.38 & 0.27 & 0.29 & 0.20 \\
3620 & KOI-561 & 0.06 & -0.19 & 0.20 & -0.21 & -0.09 & -0.05 & -0.09 & -0.13 & -0.08 & -0.10 & -0.17 & -0.26 & -0.17 & -0.21 & -0.24 \\
3621 & KOI-1240 & -0.01 & 0.12 & 0.00 & 0.15 & 0.07 & 0.06 & 0.08 & 0.03 & 0.08 & 0.07 & 0.06 & 0.03 & 0.06 & 0.05 & 0.02 \\
3622 & KOI-2092 & -0.32 & -0.32 & -0.26 & -0.37 & -0.31 & -0.33 & -0.37 & -0.39 & -0.25 & -0.39 & -0.36 & -0.47 & -0.36 & -0.42 & -0.14 \\
3623 & KOI-5324 & -0.20 & -0.04 & -0.08 & -0.20 & -0.08 & -0.11 & -0.22 & -0.16 & -0.10 & -0.16 & -0.13 & -0.20 & -0.08 & -0.08 & -0.10 \\
3624 & KOI-4072 & 0.08 & 0.13 & 0.22 & 0.10 & 0.11 & 0.11 & 0.14 & 0.10 & 0.11 & 0.12 & 0.11 & 0.14 & 0.12 & 0.12 & 0.19 \\
3625 & KOI-2678 & -0.08 & -0.18 & -0.07 & -0.16 & -0.07 & -0.06 & -0.02 & 0.07 & 0.00 & 0.04 & 0.04 & -0.03 & 0.03 & -0.11 & -0.03 \\
3626 & KOI-177 & -0.04 & -0.06 & -0.03 & -0.06 & -0.05 & -0.02 & -0.04 & 0.01 & -0.04 & -0.12 & -0.05 & -0.12 & -0.04 & -0.06 & 0.01 \\
3627 & KOI-1695 & 0.12 & 0.21 & 0.25 & 0.22 & 0.15 & 0.04 & 0.14 & 0.14 & 0.17 & 0.00 & 0.15 & 0.19 & 0.15 & 0.16 & 0.17 \\
3628 & KOI-3980 & 0.07 & 0.17 & 0.22 & 0.16 & 0.09 & 0.10 & 0.15 & 0.16 & 0.12 & 0.08 & 0.06 & 0.09 & 0.10 & 0.12 & 0.01 \\
3629 & KOI-1375 & -0.28 & -0.26 & 0.11 & -0.07 & -0.15 & -0.50 & -0.09 & -0.10 & -0.05 & -0.05 & -0.11 & -0.46 & -0.13 & -0.23 & -0.29 \\
3630 & KOI-4850 & 0.00 & -0.28 & 0.04 & -0.04 & 0.01 & -0.06 & 0.00 & -0.02 & 0.05 & -0.01 & -0.03 & -0.08 & -0.01 & -0.02 & 0.05 \\
3631 & KOI-2086 & -0.09 & -0.09 & 0.07 & -0.05 & -0.03 & -0.02 & -0.06 & 0.01 & 0.02 & -0.04 & -0.08 & -0.20 & -0.03 & -0.05 & -0.13 \\
3632 & Kepler-60 & -0.02 & -0.12 & 0.02 & -0.09 & -0.10 & -0.07 & -0.06 & -0.03 & -0.01 & -0.16 & -0.32 & -0.15 & -0.07 & -0.09 & -0.07 \\
3633 & KOI-4871 & -0.10 & -0.08 & 0.07 & -0.04 & -0.03 & -0.08 & -0.04 & 0.01 & 0.05 & -0.19 & -0.06 & -0.24 & -0.07 & -0.09 & -0.00 \\
3634 & KOI-4184 & 0.07 & -0.26 & 0.08 & 0.04 & -0.07 & 0.04 & -0.03 & 0.02 & 0.00 & -0.02 & -0.03 & -0.06 & -0.03 & -0.05 & -0.23 \\
3635 & KOI-864 & -0.01 & 0.07 & 0.14 & -0.06 & -0.02 & -0.02 & -0.00 & -0.04 & -0.09 & -0.10 & 0.01 & -0.07 & -0.04 & -0.04 & 0.05 \\
3636 & KOI-3244 & -0.27 & 0.05 & -0.13 & -0.12 & -0.10 & -0.10 & -0.25 & -0.04 & -0.02 & -0.12 & -0.04 & -0.01 & 0.01 & -0.03 & 0.29 \\
3637 & KOI-4188 & 0.08 & 0.48 & -0.08 & 0.16 & 0.27 & 0.34 & 0.16 & 0.23 & 0.34 & 0.24 & 0.34 & 0.11 & 0.32 & 0.29 & 0.31 \\
3638 & KOI-4674 & 0.07 & -0.05 & 0.16 & -0.03 & 0.09 & 0.09 & 0.09 & 0.13 & 0.11 & 0.06 & 0.14 & 0.06 & 0.14 & 0.09 & 0.02 \\
3639 & KOI-201 & 0.26 & 0.37 & 0.25 & 0.41 & 0.31 & 0.34 & 0.24 & 0.24 & 0.27 & 0.27 & 0.38 & 0.21 & 0.34 & 0.40 & 0.48 \\
3640 & KOI-2571 & 0.15 & 0.11 & 0.14 & 0.33 & 0.16 & 0.27 & 0.17 & 0.36 & 0.26 & 0.20 & 0.23 & 0.24 & 0.23 & 0.21 & 0.08 \\
3641 & KOI-163 & -0.32 & -0.69 & -0.21 & -0.42 & -0.31 & -0.36 & -0.29 & -0.33 & -0.30 & -0.28 & -0.42 & -0.57 & -0.41 & -0.41 & -0.82 \\
3642 & KOI-2220 & 0.08 & 0.18 & 0.02 & 0.11 & 0.17 & 0.21 & 0.11 & 0.15 & 0.19 & 0.15 & 0.14 & 0.11 & 0.13 & 0.18 & 0.15 \\
3643 & KOI-1366 & 0.00 & -0.05 & 0.00 & -0.01 & -0.00 & -0.01 & -0.04 & 0.01 & 0.01 & 0.03 & -0.01 & -0.06 & 0.02 & -0.02 & 0.02 \\
3644 & KOI-2925 & 0.05 & 0.11 & 0.08 & 0.08 & 0.08 & 0.07 & 0.08 & 0.06 & 0.09 & 0.09 & 0.12 & 0.11 & 0.10 & 0.09 & 0.04 \\
3645 & KOI-1363 & 0.11 & -0.56 & 0.21 & 0.10 & 0.17 & 0.10 & 0.17 & 0.07 & 0.13 & 0.12 & 0.16 & 0.19 & 0.16 & 0.19 & 0.24 \\
3646 & KOI-2087 & 0.00 & -0.26 & -0.03 & -0.10 & 0.02 & -0.06 & 0.01 & 0.03 & 0.06 & 0.01 & 0.01 & -0.01 & 0.02 & -0.04 & 0.12 \\
3647 & KOI-1628 & 0.14 & -0.13 & 0.10 & 0.14 & 0.10 & -0.06 & 0.12 & 0.23 & 0.23 & 0.29 & 0.23 & 0.22 & 0.25 & 0.20 & 0.09 \\
3648 & KOI-1367 & -0.22 & -0.53 & -0.27 & -0.19 & -0.14 & -0.13 & -0.12 & -0.09 & -0.06 & -0.11 & -0.12 & -0.18 & -0.13 & -0.14 & -0.22 \\
3649 & KOI-4382 & -0.05 & 0.36 & 0.07 & -0.19 & -0.05 & -0.17 & -0.03 & 0.04 & 0.08 & 0.07 & -0.10 & -0.31 & -0.04 & -0.10 & 0.03 \\
3650 & KOI-2879 & -0.10 & -0.33 & -0.05 & -0.14 & -0.13 & -0.09 & -0.08 & -0.06 & -0.09 & -0.08 & -0.07 & -0.19 & -0.09 & -0.15 & -0.01 \\
3651 & KOI-670 & 0.07 & 0.10 & 0.22 & 0.07 & 0.09 & 0.16 & 0.11 & 0.07 & 0.12 & 0.12 & 0.11 & 0.06 & 0.12 & 0.09 & 0.13 \\
3652 & KOI-671 & 0.01 & 0.09 & 0.06 & 0.06 & -0.03 & -0.10 & 0.04 & 0.01 & -0.01 & -0.22 & -0.01 & 0.00 & 0.01 & 0.01 & -0.06 \\
3653 & KOI-2215 & -0.24 & -0.23 & -0.16 & -0.88 & 0.01 & -0.12 & 0.02 & -0.22 & 0.18 & 0.12 & 0.09 & -0.23 & -0.05 & -0.09 & 0.15 \\
3654 & KOI-3689 & -0.02 & 0.33 & -0.03 & -0.03 & 0.03 & 0.00 & -0.05 & 0.05 & 0.10 & -0.07 & 0.05 & -0.11 & 0.04 & -0.01 & 0.07 \\
3655 & KOI-312 & 0.01 & 0.55 & 0.29 & 0.06 & 0.05 & -0.02 & 0.11 & 0.13 & 0.21 & 0.13 & 0.09 & 0.03 & 0.12 & 0.03 & 0.02 \\
3656 & KOI-872 & 0.31 & 0.18 & 0.43 & 0.17 & 0.09 & 0.09 & 0.13 & 0.15 & 0.13 & 0.14 & 0.11 & 0.14 & 0.14 & 0.10 & 0.07 \\
3657 & KOI-673 & -0.03 & -0.48 & 0.11 & -0.16 & -0.03 & -0.03 & -0.01 & 0.06 & 0.09 & 0.07 & 0.11 & -0.05 & 0.09 & -0.13 & 0.10 \\
3658 & KOI-672 & 0.03 & 0.06 & 0.13 & 0.08 & 0.04 & 0.10 & 0.08 & 0.05 & 0.05 & 0.03 & 0.07 & 0.09 & 0.05 & 0.03 & -0.02 \\
3659 & KOI-2083 & -0.04 & -0.03 & 0.04 & -0.13 & -0.10 & 0.03 & -0.05 & 0.08 & 0.06 & 0.12 & -0.03 & -0.17 & -0.03 & -0.16 & -0.09 \\
3660 & KOI-3907 & -0.18 & 0.26 & 0.07 & -0.46 & -0.16 & -0.91 & -0.03 & -0.05 & -0.11 & -0.23 & -0.10 & -0.28 & -0.08 & -0.23 & 0.22 \\
3661 & Kepler-1542 & 0.04 & 0.01 & 0.16 & -0.03 & 0.08 & 0.16 & 0.07 & 0.06 & 0.14 & 0.10 & 0.00 & -0.08 & 0.01 & 0.03 & -0.06 \\
3662 & KOI-4032 & 0.08 & -0.09 & 0.12 & -0.01 & 0.09 & 0.13 & 0.07 & 0.07 & 0.13 & 0.09 & 0.04 & -0.05 & 0.03 & 0.02 & -0.01 \\
3663 & KOI-3012 & -0.34 & -0.07 & 0.03 & -0.45 & -0.36 & -0.25 & -0.31 & -0.35 & -0.15 & -0.22 & -0.52 & -0.90 & -0.51 & -0.46 & -0.31 \\
3664 & KOI-4473 & -0.02 & 0.06 & 0.19 & 0.03 & -0.05 & -0.15 & -0.00 & 0.08 & 0.05 & -0.10 & -0.03 & -0.09 & 0.03 & 0.03 & 0.09 \\
3665 & KOI-3083 & 0.25 & 0.39 & 0.31 & 0.35 & 0.27 & 0.25 & 0.29 & 0.25 & 0.27 & 0.27 & 0.29 & 0.32 & 0.28 & 0.34 & 0.23 \\
3666 & KOI-3100 & 0.20 & 0.53 & 0.34 & 0.41 & 0.22 & 0.23 & 0.26 & 0.31 & 0.27 & 0.26 & 0.28 & 0.40 & 0.28 & 0.33 & 0.13 \\
3667 & KOI-1379 & -0.08 & -0.17 & 0.02 & -0.09 & -0.10 & -0.11 & -0.07 & -0.12 & -0.12 & -0.15 & -0.12 & -0.16 & -0.13 & -0.15 & -0.11 \\
3668 & KOI-1618 & 0.12 & 0.40 & 0.18 & -0.03 & 0.11 & 0.10 & 0.13 & 0.21 & 0.20 & 0.11 & 0.16 & 0.02 & 0.16 & 0.16 & 0.22 \\
3669 & KOI-5375 & -0.28 & 0.12 & 0.04 & -0.19 & -0.22 & -0.06 & -0.00 & -0.12 & -0.14 & -0.13 & -0.17 & -0.23 & -0.10 & -0.14 & 0.14 \\
3670 & KOI-369 & -0.12 & -0.14 & -0.01 & -0.24 & -0.13 & -0.46 & -0.08 & -0.07 & 0.01 & 0.16 & -0.09 & -0.41 & -0.08 & -0.19 & -0.03 \\
3671 & KOI-238 & -0.13 & 0.05 & -0.04 & -0.01 & -0.07 & -0.15 & -0.02 & -0.04 & -0.08 & -0.02 & -0.07 & -0.21 & -0.04 & -0.10 & -0.05 \\
3672 & KOI-987 & -0.03 & -0.13 & -0.03 & -0.07 & 0.03 & -0.02 & 0.05 & 0.07 & 0.07 & 0.05 & 0.05 & -0.03 & 0.05 & -0.02 & 0.13 \\
3673 & KOI-4136 & 0.06 & 0.07 & 0.12 & 0.10 & 0.06 & 0.07 & 0.09 & 0.14 & 0.11 & 0.04 & 0.07 & 0.07 & 0.10 & 0.10 & 0.15 \\
3674 & KOI-2051 & -0.08 & -0.01 & 0.10 & -0.16 & -0.09 & -0.08 & -0.10 & -0.05 & -0.06 & -0.08 & -0.09 & -0.24 & -0.08 & -0.11 & -0.22 \\
3675 & KOI-1961 & -0.05 & -0.13 & 0.11 & -0.13 & -0.08 & -0.14 & -0.00 & -0.02 & -0.06 & -0.08 & -0.05 & -0.11 & -0.06 & -0.10 & 0.03 \\
3676 & KOI-2916 & -0.14 & 0.01 & -0.12 & -0.02 & -0.01 & -0.01 & 0.01 & 0.01 & 0.04 & 0.00 & -0.03 & -0.02 & 0.01 & 0.00 & 0.01 \\
3677 & KOI-2561 & 0.07 & -0.04 & 0.17 & 0.08 & 0.04 & 0.02 & 0.09 & 0.11 & 0.14 & 0.09 & 0.06 & -0.05 & 0.06 & 0.07 & 0.12 \\
3678 & KOI-2516 & 0.10 & 0.25 & 0.12 & 0.16 & 0.17 & 0.22 & 0.10 & 0.23 & 0.23 & 0.15 & 0.20 & 0.27 & 0.24 & 0.25 & 0.14 \\
3679 & KOI-456 & 0.10 & 0.06 & 0.13 & 0.03 & 0.18 & 0.15 & 0.09 & 0.10 & 0.15 & 0.15 & 0.11 & 0.19 & 0.15 & 0.15 & 0.09 \\
3680 & KOI-1979 & 0.06 & 0.02 & 0.07 & 0.11 & 0.16 & 0.22 & 0.10 & 0.21 & 0.19 & 0.16 & 0.13 & 0.09 & 0.15 & 0.15 & 0.16 \\
3681 & KOI-5379 & -0.13 & 0.19 & 0.03 & -0.04 & -0.01 & -0.08 & -0.14 & 0.06 & -0.02 & -0.07 & 0.00 & 0.00 & 0.03 & 0.03 & 0.66 \\
3682 & KOI-1862 & 0.17 & 0.19 & 0.15 & 0.23 & 0.17 & 0.15 & 0.17 & 0.15 & 0.17 & 0.15 & 0.17 & 0.23 & 0.17 & 0.21 & 0.12 \\
3683 & KOI-674 & 0.35 & 0.21 & 0.43 & 0.24 & 0.24 & 0.36 & 0.14 & 0.18 & 0.25 & 0.17 & 0.20 & 0.28 & 0.22 & 0.26 & 0.10 \\
3684 & KOI-373 & -0.25 & -0.33 & -0.16 & -0.36 & -0.31 & -0.53 & -0.27 & -0.30 & -0.27 & -0.32 & -0.35 & -0.53 & -0.35 & -0.38 & -0.35 \\
3685 & KOI-1378 & -0.18 & -0.28 & -0.12 & -0.31 & -0.17 & -0.09 & -0.24 & -0.21 & -0.08 & -0.11 & -0.31 & -0.55 & -0.29 & -0.28 & -0.32 \\
3686 & KOI-4864 & -0.21 & -0.50 & -0.13 & -0.34 & -0.28 & -0.34 & -0.26 & -0.23 & -0.15 & -0.49 & -0.24 & -0.53 & -0.26 & -0.30 & -0.23 \\
3687 & KOI-4665 & 0.04 & 0.12 & 0.15 & 0.04 & 0.07 & 0.10 & 0.04 & 0.04 & 0.14 & 0.07 & -0.03 & -0.08 & -0.01 & 0.01 & -0.02 \\
3688 & KOI-266 & -0.03 & -1.42 & 0.02 & -0.08 & -0.04 & -0.18 & -0.06 & -0.02 & 0.03 & -0.06 & -0.02 & -0.20 & -0.02 & -0.11 & -0.01 \\
3689 & KOI-3096 & -0.07 & -0.54 & 0.16 & -0.08 & 0.03 & 0.17 & -0.02 & 0.00 & 0.13 & 0.02 & -0.11 & -0.36 & -0.12 & -0.07 & -0.10 \\
3690 & KOI-313 & 0.01 & -0.07 & 0.07 & -0.09 & 0.01 & 0.02 & 0.05 & -0.00 & 0.03 & 0.03 & 0.03 & -0.01 & 0.03 & -0.02 & -0.08 \\
3691 & KOI-884 & 0.12 & 0.33 & 0.08 & 0.39 & 0.21 & 0.26 & 0.12 & 0.23 & 0.23 & 0.21 & 0.24 & 0.32 & 0.22 & 0.24 & 0.10 \\
3692 & KOI-1848 & -0.07 & -0.13 & -0.00 & -0.08 & -0.12 & -0.13 & -0.12 & 0.03 & -0.01 & 0.22 & -0.02 & -0.31 & -0.07 & -0.21 & -0.02 \\
3693 & KOI-2357 & 0.11 & -0.95 & 0.26 & -0.07 & 0.05 & 0.06 & -0.01 & -0.06 & 0.12 & 0.10 & -0.03 & -0.07 & -0.04 & -0.00 & -0.01 \\
3694 & KOI-5393 & -0.12 & 0.06 & 0.01 & -0.07 & 0.02 & 0.05 & -0.14 & -0.01 & 0.06 & -0.02 & -0.06 & 0.01 & 0.04 & 0.07 & 0.09 \\
3695 & KOI-3193 & -0.12 & 0.41 & -0.09 & 0.13 & 0.07 & 0.01 & -0.11 & 0.06 & 0.04 & -0.05 & 0.04 & 0.22 & 0.12 & 0.08 & 0.44 \\
3696 & KOI-1890 & 0.00 & 0.20 & 0.28 & 0.06 & 0.08 & 0.19 & 0.08 & 0.13 & 0.25 & 0.31 & 0.13 & -0.00 & 0.15 & 0.08 & 0.19 \\
3697 & KOI-457 & 0.08 & 0.09 & 0.02 & 0.32 & 0.16 & 0.18 & 0.14 & 0.22 & 0.21 & 0.19 & 0.17 & 0.21 & 0.22 & 0.21 & 0.04 \\
3698 & KOI-679 & 0.14 & 0.32 & 0.32 & 0.26 & 0.15 & 0.15 & 0.20 & 0.16 & 0.17 & 0.08 & 0.19 & 0.23 & 0.19 & 0.20 & 0.22 \\
3699 & KOI-678 & 0.02 & -0.01 & 0.04 & 0.10 & 0.06 & 0.13 & 0.06 & 0.17 & 0.11 & 0.09 & 0.14 & 0.13 & 0.14 & 0.10 & 0.13 \\
3700 & KOI-4663 & 0.13 & 0.34 & 0.10 & 0.27 & 0.17 & 0.23 & 0.21 & 0.23 & 0.28 & 0.17 & 0.21 & 0.30 & 0.25 & 0.27 & 0.22 \\
3701 & Kepler-435 & -0.02 & 0.10 & 0.26 & 0.06 & -0.03 & -0.06 & 0.05 & 0.19 & 0.10 & -0.09 & 0.10 & -0.14 & 0.09 & 0.00 & 0.20 \\
3702 & KOI-150 & -0.36 & -0.28 & -0.13 & -0.40 & -0.34 & -0.32 & -0.34 & -0.41 & -0.26 & -0.25 & -0.52 & -0.75 & -0.49 & -0.49 & -0.46 \\
3703 & KOI-4160 & 0.12 & 0.10 & 0.14 & 0.16 & 0.12 & 0.12 & 0.16 & 0.22 & 0.17 & 0.19 & 0.21 & 0.24 & 0.20 & 0.16 & 0.16 \\
3704 & KOI-3128 & -0.08 & -0.05 & 0.07 & -0.07 & -0.09 & -0.12 & -0.10 & 0.04 & 0.04 & -0.06 & -0.03 & -0.33 & -0.04 & -0.15 & 0.16 \\
3705 & Kepler-431 & -0.09 & -0.45 & 0.14 & -0.08 & -0.08 & -0.09 & -0.02 & 0.01 & 0.01 & -0.11 & -0.06 & -0.26 & -0.05 & -0.10 & -0.10 \\
3706 & KOI-3097 & -0.07 & 0.23 & 0.02 & -0.07 & -0.04 & -0.10 & 0.01 & 0.08 & 0.04 & -0.08 & -0.03 & -0.18 & -0.01 & -0.07 & -0.11 \\
3707 & KOI-2631 & -0.31 & -0.26 & -0.12 & -0.58 & -0.33 & -0.36 & -0.34 & -0.34 & -0.17 & -0.39 & -0.46 & -0.78 & -0.44 & -0.47 & -0.48 \\
3708 & KOI-683 & 0.16 & 0.10 & 0.18 & 0.12 & 0.12 & 0.03 & 0.14 & 0.14 & 0.11 & 0.04 & 0.19 & 0.12 & 0.13 & 0.15 & 0.15 \\
3709 & KOI-1706 & 0.01 & 0.09 & 0.06 & 0.08 & 0.03 & 0.10 & 0.04 & 0.05 & 0.06 & 0.08 & 0.10 & 0.05 & 0.08 & 0.05 & -0.03 \\
3710 & KOI-568 & -0.09 & -0.22 & -0.00 & -0.08 & -0.05 & 0.04 & -0.03 & -0.04 & 0.02 & -0.01 & -0.00 & -0.01 & -0.03 & -0.04 & -0.05 \\
3711 & KOI-4614 & 0.07 & 0.14 & 0.21 & 0.05 & 0.04 & 0.04 & 0.11 & 0.16 & 0.04 & 0.04 & 0.06 & 0.04 & 0.11 & 0.10 & 0.15 \\
3712 & KOI-1898 & -0.06 & -0.43 & 0.07 & -0.17 & -0.04 & -0.04 & -0.00 & -0.00 & 0.02 & 0.06 & -0.05 & -0.14 & -0.03 & -0.07 & -0.03 \\
3713 & KOI-3943 & -0.14 & 0.44 & 0.08 & -0.03 & -0.02 & -0.19 & -0.06 & 0.05 & 0.08 & 0.02 & -0.02 & -0.18 & -0.01 & -0.04 & -0.05 \\
3714 & KOI-315 & -0.23 & -0.38 & -0.24 & -0.23 & -0.23 & -0.22 & -0.20 & -0.17 & -0.21 & -0.19 & -0.25 & -0.31 & -0.25 & -0.28 & -0.47 \\
3715 & KOI-1528 & 0.00 & 0.00 & 0.06 & -0.03 & -0.04 & -0.02 & -0.02 & -0.03 & -0.04 & -0.38 & -0.00 & -0.06 & -0.01 & -0.14 & -0.05 \\
3716 & KOI-2722 & -0.02 & -0.23 & -0.04 & -0.24 & -0.04 & -0.12 & -0.11 & -0.03 & 0.02 & -0.28 & -0.02 & -0.22 & -0.04 & -0.10 & -0.06 \\
3717 & Kepler-402 & -0.05 & 0.32 & 0.02 & -0.19 & -0.07 & -0.17 & -0.05 & -0.04 & 0.02 & -0.00 & -0.03 & -0.23 & -0.06 & -0.14 & -0.02 \\
3718 & KOI-892 & -0.22 & -0.07 & -0.35 & -0.15 & -0.06 & -0.17 & -0.37 & -0.13 & -0.08 & -0.17 & -0.17 & -0.12 & -0.13 & -0.09 & -0.13 \\
3719 & KOI-2585 & -0.23 & -1.00 & -0.20 & -0.51 & -0.36 & -0.22 & -0.34 & -0.32 & -0.26 & -0.10 & -0.40 & -0.61 & -0.36 & -0.44 & -0.61 \\
3720 & KOI-269 & -0.10 & -0.23 & 0.07 & -0.14 & -0.05 & -0.17 & 0.03 & 0.07 & 0.12 & 0.24 & -0.01 & -0.22 & 0.02 & -0.12 & 0.01 \\
3721 & KOI-684 & -0.07 & 0.10 & 0.08 & 0.04 & 0.02 & 0.13 & -0.03 & 0.03 & 0.04 & -0.02 & 0.05 & -0.00 & 0.06 & 0.05 & 0.01 \\
3722 & KOI-4561 & -0.11 & -0.02 & 0.16 & -0.12 & -0.06 & -0.17 & -0.02 & 0.06 & 0.01 & -0.12 & -0.02 & -0.26 & 0.01 & -0.05 & 0.08 \\
3723 & KOI-1921 & -0.09 & 0.52 & 0.32 & -0.02 & 0.02 & -0.12 & 0.04 & 0.13 & 0.07 & -0.30 & 0.01 & 0.06 & 0.10 & -0.10 & 0.04 \\
3724 & KOI-4482 & -0.09 & -0.97 & 0.13 & -0.10 & -0.05 & -0.23 & -0.01 & 0.01 & 0.04 & 0.09 & -0.01 & -0.27 & 0.01 & -0.11 & 0.07 \\
3725 & KOI-3721 & -0.97 & 0.03 & -0.20 & -0.23 & -0.17 & -0.21 & -0.04 & -0.36 & 0.08 & -0.07 & -0.28 & -0.45 & -0.20 & -0.06 & -0.19 \\
3726 & KOI-4022 & -0.06 & 0.13 & 0.13 & -0.14 & -0.11 & -0.20 & -0.11 & 0.02 & 0.04 & -0.08 & -0.10 & -0.16 & -0.05 & -0.09 & -0.21 \\
3727 & KOI-1808 & 0.03 & 0.43 & 0.15 & -0.09 & 0.02 & -0.03 & 0.06 & 0.11 & 0.06 & -0.10 & 0.04 & -0.06 & 0.05 & -0.01 & 0.22 \\
3728 & KOI-685 & -0.38 & 0.40 & 0.24 & -0.34 & -0.09 & -0.38 & -0.03 & 0.02 & 0.00 & -0.01 & -0.08 & -0.19 & -0.01 & -0.20 & -0.35 \\
3729 & KOI-3023 & 0.08 & -0.23 & 0.24 & -0.09 & 0.03 & 0.03 & 0.02 & -0.00 & 0.07 & 0.21 & 0.03 & -0.25 & -0.04 & -0.11 & -0.08 \\
3730 & KOI-4725 & -0.12 & -0.39 & -0.20 & 0.03 & -0.02 & -0.00 & -0.08 & 0.07 & 0.03 & -0.03 & -0.05 & -0.13 & -0.04 & -0.03 & -0.72 \\
3731 & KOI-2848 & 0.19 & 0.23 & 0.16 & 0.23 & 0.20 & 0.25 & 0.21 & 0.23 & 0.20 & 0.19 & 0.24 & 0.26 & 0.26 & 0.25 & 0.15 \\
3732 & KOI-3787 & 0.06 & -0.01 & -0.01 & -0.01 & 0.04 & 0.08 & 0.06 & 0.09 & 0.07 & 0.04 & 0.08 & 0.09 & 0.08 & 0.06 & 0.06 \\
3733 & KOI-171 & 0.01 & 0.02 & 0.25 & 0.09 & 0.12 & 0.01 & 0.08 & 0.16 & 0.18 & 0.06 & 0.10 & -0.00 & 0.14 & 0.11 & 0.08 \\
3734 & KOI-1533 & -0.16 & -0.23 & -0.10 & -0.30 & -0.22 & -0.26 & -0.21 & -0.24 & -0.18 & -0.29 & -0.29 & -0.42 & -0.25 & -0.30 & -0.23 \\
3735 & KOI-4582 & -0.18 & -0.34 & -0.11 & -0.25 & -0.19 & -0.21 & -0.18 & -0.18 & -0.16 & -0.14 & -0.23 & -0.35 & -0.23 & -0.27 & -0.28 \\
3736 & KOI-1964 & -0.01 & -0.05 & 0.05 & -0.01 & -0.03 & -0.06 & 0.04 & 0.04 & 0.03 & 0.04 & -0.02 & -0.05 & -0.02 & -0.07 & 0.09 \\
3737 & KOI-2984 & 0.04 & 0.03 & 0.21 & 0.12 & 0.04 & 0.13 & 0.10 & 0.12 & 0.11 & 0.09 & 0.13 & 0.02 & 0.13 & 0.06 & 0.14 \\
3738 & KOI-1818 & -0.09 & -0.25 & 0.01 & -0.13 & -0.08 & -0.18 & -0.05 & 0.02 & 0.01 & -0.05 & -0.00 & -0.09 & -0.01 & -0.11 & 0.06 \\
3739 & KOI-4257 & -0.09 & -0.17 & -0.05 & -0.06 & -0.03 & -0.10 & -0.12 & -0.03 & -0.02 & -0.05 & -0.01 & -0.06 & 0.01 & -0.05 & 0.18 \\
3740 & KOI-686 & -0.01 & 0.08 & 0.11 & -0.07 & 0.02 & 0.02 & 0.00 & -0.01 & 0.05 & 0.03 & -0.04 & -0.20 & -0.05 & -0.06 & -0.05 \\
3741 & KOI-3236 & -0.10 & 0.34 & 0.31 & -0.11 & 0.11 & -0.20 & 0.10 & 0.14 & 0.26 & -0.15 & 0.12 & 0.01 & 0.17 & 0.13 & -0.02 \\
3742 & KOI-4109 & 0.26 & 0.25 & 0.23 & 0.27 & 0.25 & 0.31 & 0.24 & 0.24 & 0.26 & 0.25 & 0.24 & 0.20 & 0.26 & 0.27 & -0.01 \\
3743 & KOI-4773 & -0.32 & 0.21 & 0.18 & -0.22 & -0.19 & -0.26 & -0.20 & -0.13 & -0.05 & -0.11 & -0.21 & -0.51 & -0.17 & -0.28 & -0.20 \\
3744 & KOI-687 & 0.05 & -0.06 & 0.06 & 0.01 & 0.01 & 0.08 & -0.01 & 0.17 & 0.14 & 0.25 & 0.13 & 0.02 & 0.09 & -0.01 & 0.18 \\
3745 & KOI-459 & 0.07 & -0.20 & 0.05 & 0.03 & 0.05 & 0.05 & 0.03 & -0.00 & 0.10 & 0.14 & 0.08 & 0.02 & 0.05 & 0.06 & 0.13 \\
3746 & KOI-92 & 0.08 & -0.56 & 0.19 & 0.04 & 0.05 & 0.14 & 0.04 & 0.05 & 0.05 & 0.13 & 0.08 & 0.04 & 0.09 & 0.00 & 0.19 \\
3747 & KOI-3214 & -0.14 & -0.19 & 0.06 & -0.17 & -0.13 & -0.19 & -0.11 & -0.01 & -0.00 & -0.13 & -0.07 & -0.29 & -0.07 & -0.15 & -0.01 \\
3748 & KOI-2674 & -0.02 & -0.07 & 0.13 & -0.07 & 0.00 & 0.01 & 0.01 & 0.05 & 0.07 & -0.01 & 0.04 & -0.04 & 0.05 & -0.01 & 0.00 \\
3749 & KOI-2352 & -0.17 & -0.07 & -0.04 & -0.18 & -0.12 & -0.57 & -0.09 & -0.04 & 0.10 & 0.07 & -0.07 & -0.35 & -0.08 & -0.17 & -0.16 \\
3750 & KOI-237 & 0.25 & 0.13 & 0.20 & 0.29 & 0.24 & 0.26 & 0.21 & 0.17 & 0.24 & 0.26 & 0.27 & 0.35 & 0.21 & 0.29 & 0.21 \\
3751 & KOI-520 & -0.04 & 0.05 & -0.01 & 0.09 & 0.07 & 0.13 & 0.05 & 0.11 & 0.12 & 0.13 & 0.06 & 0.11 & 0.10 & 0.10 & -0.09 \\
3752 & KOI-517 & 0.16 & 0.15 & 0.20 & 0.11 & 0.14 & 0.05 & 0.15 & 0.16 & 0.13 & 0.12 & 0.20 & 0.10 & 0.16 & 0.14 & 0.29 \\
3753 & KOI-519 & 0.02 & -0.07 & 0.01 & 0.11 & 0.04 & 0.08 & 0.03 & 0.15 & 0.12 & -0.02 & -0.01 & -0.04 & 0.07 & 0.02 & -0.03 \\
3754 & KOI-155 & -0.14 & -0.62 & -0.02 & -0.23 & -0.06 & -0.02 & -0.11 & -0.08 & 0.04 & -0.09 & -0.19 & -0.37 & -0.19 & -0.20 & -0.27 \\
3755 & KOI-316 & 0.24 & 0.36 & 0.23 & 0.43 & 0.23 & 0.28 & 0.25 & 0.27 & 0.25 & 0.20 & 0.29 & 0.36 & 0.27 & 0.30 & 0.17 \\
3756 & KOI-569 & -0.24 & -0.62 & -0.28 & -0.18 & -0.17 & -0.20 & -0.19 & -0.12 & -0.15 & -0.15 & -0.23 & -0.31 & -0.19 & -0.20 & -0.45 \\
3757 & KOI-2743 & -0.12 & -0.31 & -0.07 & -0.20 & -0.07 & -0.09 & -0.09 & -0.05 & -0.07 & -0.07 & -0.09 & -0.23 & -0.10 & -0.12 & -0.11 \\
3758 & KOI-3245 & -0.06 & -1.68 & -0.00 & -0.15 & -0.09 & -0.10 & -0.03 & -0.03 & -0.02 & 0.03 & -0.09 & -0.21 & -0.08 & -0.13 & -0.10 \\
3759 & KOI-2486 & 0.05 & 0.02 & 0.20 & 0.01 & 0.09 & -0.02 & 0.10 & 0.19 & 0.18 & 0.05 & 0.12 & -0.09 & 0.14 & 0.10 & 0.18 \\
3760 & KOI-2426 & 0.10 & 0.03 & 0.26 & 0.02 & 0.06 & 0.10 & 0.04 & -0.00 & 0.07 & 0.04 & -0.02 & -0.09 & -0.02 & 0.02 & -0.06 \\
3761 & KOI-4343 & -0.34 & -0.22 & -0.19 & -0.51 & -0.43 & -0.38 & -0.34 & -0.34 & -0.25 & -0.32 & -0.45 & -0.78 & -0.41 & -0.48 & -0.49 \\
3762 & KOI-1951 & -0.09 & -0.61 & -0.04 & -0.33 & -0.16 & -0.08 & -0.16 & -0.14 & 0.01 & -0.04 & -0.12 & -0.34 & -0.17 & -0.22 & -0.21 \\
3763 & KOI-162 & 0.05 & 0.08 & 0.10 & 0.16 & 0.18 & 0.21 & 0.15 & 0.22 & 0.19 & 0.17 & 0.18 & 0.15 & 0.20 & 0.23 & 0.15 \\
3764 & KOI-4656 & -0.09 & 0.09 & 0.41 & 0.11 & 0.08 & 0.03 & 0.10 & 0.19 & 0.28 & 0.16 & 0.18 & -0.12 & 0.20 & 0.03 & 0.30 \\
3765 & KOI-4881 & -0.03 & -0.18 & 0.19 & 0.05 & -0.01 & -0.05 & -0.03 & 0.12 & 0.09 & -0.12 & -0.00 & -0.03 & 0.04 & -0.03 & 0.25 \\
3766 & KOI-317 & -0.11 & -0.77 & 0.36 & -0.10 & 0.01 & -0.40 & 0.14 & 0.25 & 0.08 & -0.73 & 0.13 & -0.15 & 0.11 & -0.12 & 0.33 \\
3767 & KOI-2073 & -0.08 & -0.16 & -0.14 & 0.02 & 0.01 & 0.03 & 0.02 & 0.03 & 0.03 & 0.04 & 0.04 & -0.03 & 0.01 & 0.02 & -0.13 \\
3768 & KOI-1019 & -0.07 & 0.20 & -0.04 & 0.08 & 0.09 & 0.13 & -0.03 & 0.12 & 0.11 & 0.03 & 0.12 & 0.24 & 0.16 & 0.18 & 0.12 \\
3769 & KOI-688 & 0.02 & 0.48 & -0.03 & -0.29 & 0.09 & 0.08 & -0.15 & 0.13 & 0.26 & 0.24 & -0.02 & -0.48 & 0.04 & -0.02 & 0.07 \\
3770 & KOI-4634 & 0.08 & 0.16 & 0.23 & 0.12 & 0.14 & 0.02 & 0.16 & 0.20 & 0.24 & 0.23 & 0.20 & 0.14 & 0.19 & 0.15 & 0.19 \\
3771 & KOI-3046 & 0.18 & 0.17 & 0.16 & 0.24 & 0.20 & 0.18 & 0.18 & 0.19 & 0.19 & 0.16 & 0.19 & 0.25 & 0.20 & 0.21 & 0.13 \\
3772 & KOI-318 & 0.20 & 0.79 & 0.54 & 0.35 & 0.31 & 0.35 & 0.41 & 0.31 & 0.41 & 0.31 & 0.35 & 0.34 & 0.35 & 0.32 & 0.23 \\
3773 & KOI-2781 & -0.39 & -0.36 & -0.08 & -0.43 & -0.39 & -0.31 & -0.37 & -0.34 & -0.23 & -0.36 & -0.52 & -0.83 & -0.48 & -0.52 & -0.53 \\
3774 & KOI-2105 & -0.04 & 0.00 & -0.03 & -0.09 & -0.02 & -0.03 & -0.08 & 0.01 & 0.05 & 0.07 & -0.04 & -0.12 & -0.03 & -0.07 & 0.01 \\
3775 & KOI-1985 & 0.02 & -0.38 & 0.04 & -0.07 & -0.02 & -0.04 & -0.06 & 0.02 & 0.01 & 0.01 & -0.04 & -0.10 & -0.03 & -0.07 & -0.32 \\
3776 & KOI-572 & -0.03 & -0.25 & 0.06 & -0.08 & -0.05 & -0.13 & -0.05 & 0.01 & -0.05 & -0.17 & -0.06 & -0.11 & -0.04 & -0.10 & -0.09 \\
3777 & KOI-907 & 0.01 & 0.09 & 0.17 & -0.22 & -0.11 & -0.14 & -0.17 & -0.14 & -0.03 & -0.23 & -0.12 & -0.21 & -0.12 & -0.15 & -0.12 \\
3778 & KOI-1809 & 0.05 & -0.10 & 0.02 & 0.05 & 0.01 & -0.08 & 0.06 & 0.11 & 0.00 & 0.07 & 0.06 & 0.06 & 0.05 & 0.03 & 0.01 \\
3779 & KOI-1726 & 0.59 & -0.05 & 0.61 & 0.21 & 0.15 & 0.21 & 0.11 & 0.20 & 0.15 & 0.12 & 0.06 & 0.12 & 0.14 & 0.13 & -0.31 \\
3780 & KOI-2593 & 0.03 & 0.49 & 0.25 & 0.09 & 0.15 & 0.14 & 0.19 & 0.25 & 0.23 & 0.18 & 0.21 & 0.11 & 0.22 & 0.17 & 0.27 \\
3781 & KOI-4037 & 0.01 & 0.50 & 0.13 & 0.06 & -0.03 & -0.05 & 0.04 & 0.06 & 0.18 & 0.17 & 0.08 & -0.13 & 0.06 & 0.01 & 0.17 \\
3782 & KOI-4426 & -0.03 & 0.19 & 0.27 & -0.01 & -0.01 & -0.08 & 0.03 & 0.14 & 0.14 & -0.14 & 0.08 & -0.16 & 0.11 & 0.04 & 0.17 \\
3783 & KOI-4098 & -0.02 & -0.16 & 0.09 & -0.10 & -0.14 & -0.09 & -0.03 & 0.01 & -0.05 & -0.06 & -0.09 & -0.19 & -0.07 & -0.14 & -0.07 \\
3784 & KOI-1069 & 0.22 & 0.16 & 0.21 & 0.27 & 0.21 & 0.39 & 0.17 & 0.20 & 0.24 & 0.23 & 0.27 & 0.22 & 0.24 & 0.22 & -0.10 \\
3785 & KOI-3338 & -0.20 & 0.31 & -0.02 & -0.29 & -0.21 & -0.35 & 0.07 & -0.17 & -0.03 & 0.26 & -0.20 & -0.44 & -0.11 & -0.32 & -0.26 \\
3786 & KOI-4834 & 0.28 & 0.46 & 0.25 & 0.47 & 0.33 & 0.44 & 0.23 & 0.35 & 0.35 & 0.29 & 0.41 & 0.49 & 0.40 & 0.44 & 0.29 \\
3787 & KOI-4567 & -0.21 & -0.09 & 0.24 & -0.04 & -0.04 & -0.18 & 0.02 & 0.00 & 0.04 & -0.03 & 0.06 & -0.21 & 0.01 & -0.10 & 0.01 \\
3788 & KOI-4435 & 0.13 & 0.24 & 0.35 & 0.08 & 0.06 & 0.02 & 0.12 & 0.22 & 0.17 & -0.06 & 0.19 & 0.13 & 0.17 & 0.12 & 0.27 \\
3789 & KOI-1137 & -0.23 & -0.26 & -0.28 & -0.23 & -0.24 & -0.20 & -0.20 & -0.14 & -0.18 & -0.27 & -0.20 & -0.35 & -0.26 & -0.24 & -0.18 \\
3790 & KOI-3301 & 0.15 & 0.28 & 0.23 & 0.30 & 0.19 & 0.25 & 0.20 & 0.23 & 0.23 & 0.19 & 0.21 & 0.30 & 0.23 & 0.28 & 0.26 \\
3791 & Kepler-271 & -0.24 & 0.07 & -0.24 & -0.23 & -0.15 & -0.19 & -0.05 & -0.19 & -0.14 & -0.06 & -0.28 & -0.38 & -0.24 & -0.27 & -0.24 \\
3792 & KOI-1150 & -0.01 & 0.09 & 0.10 & 0.11 & 0.06 & 0.08 & 0.03 & 0.10 & 0.17 & 0.21 & 0.08 & 0.01 & 0.07 & 0.07 & 0.11 \\
3793 & KOI-1820 & -0.05 & -0.12 & 0.06 & -0.07 & -0.07 & -0.00 & 0.05 & 0.04 & -0.05 & 0.02 & 0.07 & -0.03 & 0.03 & -0.05 & 0.12 \\
3794 & KOI-4399 & -0.21 & -0.55 & -0.28 & -0.29 & -0.19 & -0.21 & -0.09 & -0.14 & -0.12 & -0.15 & -0.12 & -0.27 & -0.15 & -0.20 & -0.04 \\
3795 & KOI-574 & -0.12 & -0.21 & -0.06 & -0.09 & -0.06 & -0.09 & -0.08 & -0.04 & -0.06 & -0.04 & -0.09 & -0.14 & -0.08 & -0.11 & -0.45 \\
3796 & KOI-4763 & 0.07 & 0.11 & 0.21 & 0.13 & 0.12 & 0.16 & 0.08 & 0.15 & 0.15 & 0.11 & 0.12 & 0.12 & 0.14 & 0.15 & 0.22 \\
3797 & KOI-573 & 0.02 & -0.17 & 0.03 & 0.02 & 0.09 & 0.09 & 0.05 & 0.03 & 0.12 & 0.06 & 0.03 & 0.04 & 0.07 & 0.08 & 0.02 \\
3798 & KOI-127 & 0.21 & 0.26 & 0.17 & 0.37 & 0.25 & 0.26 & 0.27 & 0.28 & 0.24 & 0.28 & 0.25 & 0.35 & 0.26 & 0.31 & 0.20 \\
3799 & KOI-4407 & -0.22 & -0.03 & 0.05 & -0.05 & -0.09 & -0.19 & -0.03 & 0.01 & -0.01 & -0.04 & -0.06 & -0.30 & -0.07 & -0.21 & -0.10 \\
3800 & Kepler-79 & -0.03 & 0.87 & 0.04 & -0.08 & -0.09 & 0.07 & 0.08 & 0.07 & 0.14 & 0.23 & -0.04 & -0.14 & 0.07 & -0.09 & 0.15 \\
3801 & KOI-152 & 0.06 & 0.15 & 0.33 & 0.08 & 0.04 & 0.05 & 0.15 & 0.13 & 0.07 & 0.07 & 0.16 & -0.13 & 0.14 & 0.03 & 0.18 \\
3802 & KOI-689 & -0.43 & -0.65 & -0.18 & -0.57 & -0.38 & -0.37 & -0.43 & -0.47 & -0.39 & -0.44 & -0.57 & -0.81 & -0.55 & -0.54 & -0.47 \\
3803 & KOI-2730 & -0.01 & -0.00 & 0.28 & -0.07 & 0.04 & 0.14 & 0.03 & -0.03 & 0.11 & 0.02 & -0.07 & -0.19 & -0.09 & -0.06 & -0.01 \\
3804 & KOI-4693 & -0.15 & -0.46 & 0.12 & -0.28 & -0.15 & -0.12 & -0.11 & -0.15 & -0.05 & -0.05 & -0.31 & -0.59 & -0.30 & -0.26 & -0.29 \\
3805 & KOI-1148 & 0.10 & 0.30 & 0.18 & 0.07 & 0.13 & 0.15 & 0.12 & 0.16 & 0.13 & 0.20 & 0.19 & 0.09 & 0.16 & 0.16 & 0.13 \\
3806 & KOI-102 & 0.13 & 0.13 & 0.09 & 0.20 & 0.17 & 0.18 & 0.19 & 0.18 & 0.16 & 0.17 & 0.16 & 0.21 & 0.17 & 0.20 & 0.15 \\
3807 & KOI-4603 & 0.04 & 0.50 & 0.26 & 0.06 & 0.13 & 0.16 & 0.19 & 0.22 & 0.17 & 0.01 & 0.24 & 0.06 & 0.19 & 0.17 & 0.21 \\
3808 & TYC 2810-1660-1 & -0.03 & -0.42 & -0.02 & -0.11 & -0.08 & -0.14 & -0.06 & 0.03 & 0.01 & 0.05 & 0.02 & -0.09 & -0.04 & -0.07 & 0.06 \\
3809 & BD+43183 & 0.05 & 0.22 & 0.13 & -0.05 & -0.01 & -0.19 & 0.06 & 0.13 & 0.13 & 0.17 & 0.09 & -0.08 & 0.10 & -0.04 & 0.07 \\
3810 & KOI-3497 & 0.44 & 0.01 & 0.46 & 0.25 & 0.06 & 0.10 & 0.22 & 0.24 & 0.10 & 0.08 & 0.08 & 0.19 & 0.19 & 0.14 & 0.07 \\
3811 & KOI-3251 & 0.05 & -0.00 & 0.08 & 0.14 & 0.08 & -0.01 & -0.09 & 0.06 & 0.01 & 0.03 & 0.06 & 0.11 & 0.06 & 0.10 & 0.01 \\
3812 & KOI-370 & -0.14 & 0.30 & 0.26 & -0.04 & -0.09 & -0.14 & 0.02 & 0.02 & 0.01 & 0.01 & -0.01 & -0.02 & -0.02 & -0.03 & 0.03 \\
3813 & KOI-2389 & -0.11 & -0.09 & 0.02 & -0.14 & -0.11 & -0.24 & -0.09 & -0.04 & -0.08 & -0.07 & -0.10 & -0.27 & -0.08 & -0.12 & -0.14 \\
3814 & KOI-4505 & -0.02 & -0.47 & 0.09 & -0.20 & -0.09 & -0.28 & -0.07 & -0.01 & -0.08 & -0.03 & -0.07 & -0.20 & -0.06 & -0.11 & -0.10 \\
3815 & KOI-2016 & 0.42 & 0.90 & 0.31 & 0.50 & 0.36 & 0.35 & 0.42 & 0.33 & 0.37 & 0.24 & 0.37 & 0.48 & 0.40 & 0.56 & 0.29 \\
3816 & KOI-691 & -0.20 & -1.94 & -0.15 & -0.37 & -0.27 & -0.49 & -0.29 & -0.25 & -0.16 & -0.21 & -0.30 & -0.55 & -0.29 & -0.33 & -0.41 \\
3817 & KOI-3315 & -0.37 & -0.60 & -0.13 & -0.41 & -0.34 & -0.27 & -0.34 & -0.39 & -0.25 & -0.34 & -0.55 & -0.74 & -0.51 & -0.45 & -0.52 \\
3818 & KOI-2022 & 0.04 & 0.08 & 0.12 & 0.05 & 0.03 & -0.19 & 0.09 & 0.14 & 0.06 & 0.11 & 0.18 & 0.01 & 0.12 & 0.03 & 0.17 \\
3819 & KOI-3111 & -0.07 & -0.14 & -0.01 & -0.10 & -0.09 & -0.23 & -0.05 & -0.01 & -0.06 & 0.00 & -0.04 & -0.21 & -0.07 & -0.13 & 0.12 \\
3820 & KOI-1792 & 0.03 & 0.06 & 0.07 & 0.03 & -0.10 & 0.31 & 0.12 & -0.02 & -0.04 & 0.01 & -0.07 & 0.02 & -0.04 & -0.06 & -0.22 \\
3821 & KOI-3890 & -0.07 & -0.03 & 0.16 & -0.11 & -0.02 & 0.05 & -0.18 & -0.08 & 0.07 & -0.07 & -0.15 & -0.13 & -0.11 & -0.03 & -0.08 \\
3822 & KOI-692 & -0.16 & 0.21 & 0.06 & 0.12 & 0.08 & 0.09 & 0.12 & 0.08 & 0.09 & 0.10 & 0.10 & 0.07 & 0.09 & 0.11 & -0.06 \\
3823 & KOI-1270 & 0.03 & -0.00 & 0.11 & 0.03 & -0.00 & -0.03 & 0.02 & 0.05 & 0.03 & 0.03 & 0.06 & 0.02 & 0.05 & 0.00 & 0.04 \\
3824 & KOI-2969 & 0.02 & 0.75 & 0.37 & 0.16 & 0.06 & 0.13 & 0.38 & 0.17 & 0.40 & 0.40 & 0.13 & 0.12 & 0.24 & 0.06 & 0.26 \\
3825 & KOI-2488 & -0.03 & -0.10 & 0.02 & -0.16 & -0.06 & -0.19 & -0.07 & -0.00 & 0.00 & 0.00 & -0.05 & -0.17 & -0.03 & -0.09 & 0.02 \\
3826 & KOI-139 & 0.16 & 0.29 & 0.24 & 0.22 & 0.16 & 0.14 & 0.20 & 0.17 & 0.21 & 0.24 & 0.22 & 0.25 & 0.20 & 0.20 & 0.18 \\
3827 & KOI-1275 & -0.02 & -0.24 & 0.07 & -0.05 & 0.02 & -0.05 & 0.00 & -0.02 & -0.03 & -0.06 & -0.01 & -0.03 & 0.00 & -0.00 & -0.06 \\
3828 & KOI-981 & -0.40 & -0.11 & -0.25 & -0.23 & -0.20 & -0.17 & -0.36 & -0.13 & -0.16 & -0.27 & -0.22 & -0.20 & -0.15 & -0.17 & 0.04 \\
3829 & KOI-3946 & -0.20 & 0.08 & 0.06 & -0.21 & -0.15 & -0.39 & -0.15 & -0.11 & 0.03 & -0.31 & -0.15 & -0.38 & -0.13 & -0.19 & -0.20 \\
3830 & KOI-4580 & -0.22 & -0.33 & -0.10 & -0.23 & -0.22 & -0.24 & -0.22 & -0.19 & -0.15 & -0.35 & -0.25 & -0.52 & -0.23 & -0.27 & -0.31 \\
3831 & KOI-579 & -0.15 & -0.09 & -0.25 & 0.01 & 0.02 & -0.02 & 0.06 & 0.07 & 0.06 & 0.03 & 0.04 & 0.02 & 0.05 & 0.00 & -0.05 \\
3832 & KOI-2503 & 0.05 & -0.21 & -0.05 & 0.14 & 0.13 & 0.25 & 0.18 & 0.16 & 0.17 & 0.15 & 0.13 & 0.13 & 0.16 & 0.15 & -0.14 \\
3833 & KOI-1754 & -0.01 & 0.14 & 0.08 & -0.14 & -0.01 & -0.25 & -0.02 & 0.03 & 0.03 & 0.07 & 0.06 & -0.12 & 0.03 & -0.05 & 0.11 \\
3834 & KOI-2111 & 0.01 & -1.86 & 0.04 & -0.05 & 0.02 & -0.00 & -0.00 & 0.09 & 0.05 & 0.08 & 0.09 & 0.03 & 0.09 & 0.01 & 0.11 \\
3835 & KOI-4775 & 0.31 & 0.54 & 0.31 & 0.53 & 0.35 & 0.46 & 0.28 & 0.41 & 0.37 & 0.32 & 0.41 & 0.55 & 0.45 & 0.48 & 0.38 \\
3836 & KOI-2414 & -0.24 & -0.11 & 0.09 & -0.27 & -0.22 & -0.18 & -0.22 & -0.24 & -0.13 & -0.20 & -0.37 & -0.67 & -0.36 & -0.35 & -0.34 \\
3837 & KOI-1279 & -0.06 & -0.02 & -0.01 & -0.18 & -0.06 & -0.05 & -0.07 & -0.04 & -0.05 & -0.09 & -0.06 & -0.15 & -0.08 & -0.09 & -0.13 \\
3838 & KOI-1271 & -0.26 & 0.07 & -0.05 & -0.23 & -0.20 & -0.44 & -0.22 & -0.16 & -0.06 & -0.05 & -0.22 & -0.49 & -0.20 & -0.31 & -0.20 \\
3839 & KOI-1278 & -0.10 & -1.79 & 0.09 & -0.11 & -0.14 & -0.05 & -0.06 & -0.12 & -0.00 & -0.29 & -0.19 & -0.39 & -0.27 & -0.17 & -0.14 \\
3840 & Kepler-282 & -0.12 & 0.06 & -0.05 & -0.24 & -0.13 & -0.02 & -0.11 & -0.19 & -0.02 & -0.30 & -0.16 & -0.47 & -0.29 & -0.20 & -0.04 \\
3841 & KOI-1891 & 0.03 & -0.02 & -0.04 & 0.15 & 0.10 & 0.18 & 0.10 & 0.13 & 0.13 & 0.12 & 0.13 & 0.18 & 0.12 & 0.14 & 0.07 \\
3842 & KOI-4066 & -0.02 & 0.21 & 0.37 & 0.13 & 0.06 & -0.02 & 0.14 & 0.18 & 0.11 & -0.10 & 0.10 & -0.04 & 0.11 & 0.03 & 0.23 \\
3843 & KOI-2758 & 0.20 & 0.41 & 0.33 & 0.25 & 0.22 & 0.27 & 0.14 & 0.30 & 0.27 & 0.21 & 0.29 & 0.31 & 0.33 & 0.29 & 0.24 \\
3844 & KOI-1283 & -0.20 & -0.05 & -0.04 & -0.36 & -0.20 & -0.19 & -0.18 & -0.21 & -0.07 & -0.17 & -0.25 & -0.46 & -0.24 & -0.28 & -0.24 \\
3845 & KOI-105 & -0.26 & -0.61 & -0.05 & -0.42 & -0.22 & -0.16 & -0.18 & -0.28 & -0.09 & -0.26 & -0.40 & -0.69 & -0.41 & -0.35 & -0.39 \\
3846 & KOI-921 & 0.00 & -0.01 & 0.00 & 0.01 & 0.09 & 0.16 & 0.04 & 0.14 & 0.12 & 0.12 & 0.12 & 0.06 & 0.11 & 0.10 & -0.02 \\
3847 & KOI-172 & -0.11 & -0.08 & 0.12 & -0.19 & -0.08 & 0.06 & -0.08 & -0.12 & 0.01 & -0.14 & -0.34 & -0.45 & -0.25 & -0.20 & -0.30 \\
3848 & KOI-319 & 0.05 & 0.31 & 0.12 & 0.11 & 0.06 & 0.14 & 0.07 & 0.17 & 0.15 & -0.01 & 0.14 & 0.15 & 0.16 & 0.13 & 0.22 \\
3849 & KOI-374 & -0.10 & 0.10 & -0.05 & -0.23 & -0.14 & -0.10 & -0.12 & -0.13 & -0.03 & -0.08 & -0.18 & -0.42 & -0.18 & -0.22 & -0.32 \\
3850 & KOI-1629 & 0.18 & 0.33 & 0.10 & 0.31 & 0.22 & 0.24 & 0.22 & 0.24 & 0.24 & 0.18 & 0.24 & 0.35 & 0.25 & 0.29 & 0.17 \\
3851 & KOI-2749 & -0.24 & -0.37 & 0.22 & -0.10 & -0.06 & -0.34 & -0.05 & 0.15 & 0.12 & -0.16 & -0.02 & -0.28 & 0.06 & -0.06 & 0.07 \\
3852 & KOI-2473 & 0.27 & -0.24 & 0.27 & -0.21 & -0.07 & -0.15 & -0.10 & -0.14 & -0.12 & -0.10 & -0.10 & -0.22 & -0.13 & -0.13 & -0.18 \\
3853 & KOI-3891 & -0.03 & -0.10 & 0.12 & -0.17 & -0.08 & -0.06 & 0.11 & -0.08 & -0.03 & -0.02 & -0.09 & -0.16 & -0.01 & -0.07 & 0.03 \\
3854 & KOI-4301 & -0.17 & 0.11 & -0.08 & -0.25 & -0.26 & -0.38 & -0.20 & -0.19 & -0.20 & -0.11 & -0.23 & -0.44 & -0.19 & -0.35 & -0.27 \\
3855 & KOI-1257 & 0.17 & 0.24 & 0.33 & 0.24 & 0.14 & 0.26 & 0.21 & 0.28 & 0.15 & 0.15 & 0.18 & 0.26 & 0.16 & 0.18 & 0.24 \\
3856 & KOI-2017 & -0.08 & -0.35 & 0.03 & -0.13 & -0.13 & -0.16 & -0.02 & 0.03 & -0.05 & -0.03 & -0.00 & -0.08 & -0.01 & -0.13 & 0.08 \\
3857 & KOI-1904 & 0.05 & -0.28 & 0.16 & -0.12 & -0.04 & -0.07 & -0.02 & 0.02 & -0.01 & -0.02 & -0.03 & -0.06 & -0.00 & -0.04 & 0.00 \\
3858 & KOI-4251 & -0.06 & -0.20 & -0.05 & -0.10 & -0.07 & -0.10 & -0.05 & -0.02 & -0.02 & -0.04 & 0.02 & -0.08 & -0.01 & -0.09 & 0.12 \\
3859 & KOI-2159 & 0.01 & -0.24 & -0.01 & -0.04 & 0.03 & 0.08 & 0.01 & 0.08 & 0.03 & 0.00 & 0.09 & -0.01 & 0.06 & 0.04 & 0.05 \\
3860 & KOI-694 & 0.10 & 0.14 & 0.10 & 0.12 & 0.11 & 0.09 & 0.15 & 0.16 & 0.12 & 0.06 & 0.13 & 0.20 & 0.15 & 0.14 & 0.07 \\
3861 & KOI-2039 & 0.07 & 0.06 & 0.09 & 0.11 & 0.15 & 0.14 & 0.10 & 0.17 & 0.19 & 0.16 & 0.19 & 0.14 & 0.18 & 0.13 & 0.21 \\
3862 & KOI-1850 & -0.01 & -0.30 & 0.10 & -0.01 & 0.01 & 0.00 & -0.01 & 0.03 & 0.03 & 0.03 & 0.03 & -0.08 & 0.02 & -0.02 & 0.05 \\
3863 & KOI-1276 & 0.04 & -0.19 & -0.10 & -0.01 & 0.11 & 0.02 & 0.06 & 0.08 & 0.18 & 0.12 & 0.12 & 0.09 & 0.06 & 0.05 & -0.20 \\
3864 & KOI-695 & -0.33 & -0.62 & -0.10 & -0.46 & -0.35 & -0.34 & -0.37 & -0.42 & -0.34 & -0.33 & -0.45 & -0.61 & -0.42 & -0.44 & -0.56 \\
3865 & KOI-3052 & -0.26 & -0.55 & -0.18 & -0.30 & -0.20 & -0.19 & -0.23 & -0.20 & -0.19 & -0.23 & -0.21 & -0.33 & -0.22 & -0.27 & -0.18 \\
3866 & KOI-2956 & -0.23 & 0.23 & 0.28 & 0.15 & -0.02 & -0.08 & 0.06 & 0.20 & 0.14 & -0.17 & 0.09 & -0.14 & 0.09 & -0.03 & 0.17 \\
3867 & KOI-3886 & 0.24 & 0.48 & 0.28 & 0.57 & 0.20 & 0.67 & 0.54 & 0.31 & 0.26 & 0.20 & 0.30 & 0.48 & 0.38 & 0.44 & 0.39 \\
3868 & KOI-1274 & -0.25 & -0.44 & -0.16 & -0.38 & -0.20 & -0.24 & -0.21 & -0.21 & -0.18 & -0.21 & -0.26 & -0.40 & -0.26 & -0.27 & -0.21 \\
3869 & KOI-4811 & -0.03 & 0.50 & 0.04 & -0.07 & 0.00 & 0.95 & -0.08 & 0.02 & 0.05 & -0.08 & 0.00 & -0.05 & 0.01 & 0.03 & 0.20 \\
3870 & KOI-2659 & 0.06 & 0.35 & 0.10 & 0.28 & 0.15 & 0.18 & 0.05 & 0.18 & 0.17 & 0.11 & 0.18 & 0.31 & 0.22 & 0.23 & 0.23 \\
3871 & KOI-464 & 0.11 & 0.21 & 0.18 & 0.15 & 0.12 & 0.16 & 0.14 & 0.17 & 0.18 & 0.12 & 0.24 & 0.16 & 0.18 & 0.17 & 0.21 \\
3872 & KOI-3541 & -0.15 & -0.14 & -0.01 & -0.33 & -0.24 & -0.51 & -0.17 & -0.13 & -0.13 & -0.25 & -0.17 & -0.50 & -0.19 & -0.32 & -0.08 \\
3873 & KOI-2641 & -0.01 & -0.08 & 0.12 & -0.06 & -0.02 & 0.00 & 0.01 & -0.00 & 0.06 & 0.12 & 0.04 & -0.12 & -0.01 & -0.03 & -0.11 \\
3874 & KOI-465 & 0.01 & 0.29 & 0.20 & 0.13 & 0.03 & -0.11 & 0.06 & 0.11 & 0.20 & 0.15 & 0.07 & -0.06 & 0.08 & 0.03 & 0.20 \\
3875 & KOI-697 & 0.00 & 0.20 & 0.10 & 0.03 & 0.09 & 0.07 & 0.12 & 0.10 & 0.11 & 0.10 & 0.07 & -0.01 & 0.10 & 0.11 & 0.02 \\
3876 & KOI-4269 & -0.13 & 0.03 & -0.13 & 0.01 & 0.03 & 0.09 & -0.04 & 0.07 & 0.08 & 0.01 & 0.07 & 0.13 & 0.10 & 0.08 & 0.06 \\
3877 & WASP-58 & -0.15 & -0.21 & -0.12 & -0.30 & -0.19 & -0.26 & -0.18 & -0.19 & -0.15 & -0.22 & -0.25 & -0.40 & -0.23 & -0.26 & -0.28 \\
3878 & KOI-3473 & -0.05 & -0.36 & -0.04 & -0.16 & -0.11 & -0.11 & -0.07 & 0.02 & -0.06 & -0.04 & 0.01 & -0.07 & 0.00 & -0.12 & -0.04 \\
3879 & KOI-698 & -0.06 & 0.03 & 0.09 & -0.26 & 0.02 & -0.04 & 0.05 & 0.01 & 0.16 & 0.04 & 0.08 & -0.06 & 0.08 & -0.04 & 0.02 \\
3880 & KOI-2595 & -0.07 & 0.20 & 0.13 & -0.10 & -0.03 & -0.25 & -0.01 & 0.14 & 0.21 & 0.13 & 0.11 & 0.08 & 0.09 & 0.00 & 0.06 \\
3881 & KOI-2517 & -0.17 & -0.35 & -0.03 & -0.31 & -0.20 & -0.29 & -0.07 & -0.16 & -0.15 & -0.19 & -0.14 & -0.35 & -0.20 & -0.25 & -0.09 \\
3882 & KOI-700 & -0.39 & 0.04 & -0.28 & -0.50 & -0.40 & -0.27 & -0.36 & -0.40 & -0.34 & -0.24 & -0.54 & -0.75 & -0.49 & -0.54 & -0.60 \\
3883 & Kepler-215 & -0.36 & -1.37 & -0.19 & -0.52 & -0.43 & -0.52 & -0.38 & -0.47 & -0.37 & -0.48 & -0.52 & -0.74 & -0.52 & -0.54 & -0.53 \\
3884 & KOI-1412 & 0.10 & 0.25 & 0.21 & 0.14 & 0.12 & 0.04 & 0.09 & 0.16 & 0.13 & 0.08 & 0.12 & 0.15 & 0.15 & 0.16 & 0.09 \\
3885 & KOI-159 & -0.01 & -0.13 & 0.05 & -0.13 & -0.04 & -0.09 & -0.04 & -0.02 & -0.02 & 0.13 & -0.02 & -0.15 & -0.02 & -0.07 & 0.08 \\
3886 & KOI-2038 & -0.01 & 0.09 & 0.08 & -0.05 & 0.01 & -0.03 & 0.02 & -0.00 & 0.02 & 0.00 & 0.05 & 0.01 & 0.05 & -0.00 & 0.06 \\
3887 & KOI-3227 & -0.01 & 0.04 & 0.05 & -0.02 & 0.01 & 0.06 & 0.03 & 0.03 & 0.05 & -0.05 & 0.00 & 0.01 & 0.02 & 0.03 & -0.07 \\
3888 & KOI-4585 & -0.17 & -0.20 & 0.11 & -0.21 & -0.12 & -0.05 & -0.13 & -0.06 & -0.00 & -0.25 & -0.09 & -0.47 & -0.10 & -0.21 & -0.03 \\
3889 & KOI-582 & -0.01 & 0.00 & 0.03 & 0.02 & -0.00 & -0.00 & 0.06 & 0.09 & 0.03 & 0.06 & 0.08 & 0.04 & 0.09 & 0.04 & 0.00 \\
3890 & KOI-2319 & -0.04 & -0.20 & 0.07 & -0.09 & -0.06 & -0.04 & -0.02 & -0.04 & 0.04 & 0.04 & -0.04 & -0.18 & -0.03 & -0.09 & 0.02 \\
3891 & KOI-3196 & -0.03 & 0.02 & 0.11 & -0.09 & -0.03 & -0.08 & 0.03 & 0.03 & 0.01 & -0.04 & -0.00 & -0.16 & 0.02 & -0.04 & 0.02 \\
3892 & KOI-2530 & 0.04 & 0.08 & 0.16 & 0.10 & 0.04 & 0.08 & 0.08 & 0.10 & 0.10 & 0.02 & 0.10 & 0.10 & 0.12 & 0.08 & 0.15 \\
3893 & KOI-2768 & -0.14 & -0.38 & -0.07 & -0.17 & -0.16 & -0.20 & -0.16 & -0.12 & -0.14 & -0.17 & -0.09 & -0.18 & -0.14 & -0.18 & 0.09 \\
3894 & KOI-4014 & 0.10 & -0.05 & -0.02 & 0.04 & 0.06 & 0.14 & 0.03 & 0.09 & 0.04 & 0.03 & 0.08 & 0.03 & 0.07 & 0.04 & 0.10 \\
3895 & KOI-134 & 0.27 & 0.65 & 0.44 & 0.48 & 0.27 & 0.11 & 0.37 & 0.42 & 0.33 & 0.16 & 0.37 & 0.47 & 0.36 & 0.37 & 0.40 \\
3896 & KOI-1413 & -0.14 & -0.02 & -0.04 & -0.09 & -0.07 & -0.08 & -0.12 & -0.01 & -0.02 & -0.03 & -0.03 & -0.05 & -0.01 & -0.03 & 0.01 \\
3897 & KOI-1616 & 0.13 & 0.08 & 0.14 & 0.09 & 0.14 & 0.22 & 0.18 & 0.19 & 0.20 & 0.16 & 0.21 & 0.24 & 0.19 & 0.19 & 0.19 \\
3898 & KOI-2564 & -0.21 & -0.73 & 0.10 & -0.16 & -0.09 & -0.23 & -0.10 & -0.07 & 0.04 & -0.50 & -0.05 & -0.34 & -0.08 & -0.16 & -0.01 \\
3899 & KOI-2175 & -0.03 & 0.02 & -0.08 & 0.04 & 0.03 & 0.07 & 0.01 & 0.05 & 0.07 & 0.03 & 0.04 & 0.11 & 0.07 & 0.03 & 0.13 \\
3900 & KOI-2833 & -0.17 & -0.02 & -0.06 & -0.22 & -0.19 & -0.56 & -0.17 & -0.18 & -0.07 & -0.39 & -0.19 & -0.40 & -0.18 & -0.27 & -0.17 \\
3901 & KOI-2367 & 0.10 & 0.33 & 0.30 & 0.27 & 0.15 & 0.13 & 0.23 & 0.20 & 0.24 & 0.18 & 0.19 & 0.22 & 0.23 & 0.24 & 0.16 \\
3902 & KOI-2470 & 0.23 & 0.24 & 0.19 & 0.33 & 0.25 & 0.32 & 0.23 & 0.24 & 0.20 & 0.12 & 0.26 & 0.37 & 0.25 & 0.31 & 0.20 \\
3903 & KOI-3008 & -0.07 & -0.51 & 0.03 & -0.06 & -0.10 & -0.21 & -0.06 & -0.02 & -0.02 & -0.11 & -0.02 & -0.23 & -0.06 & -0.10 & -0.02 \\
3904 & KOI-2640 & -0.32 & -0.08 & -0.18 & -0.19 & -0.18 & -0.14 & -0.31 & -0.14 & -0.12 & -0.22 & -0.20 & -0.07 & -0.10 & -0.11 & 0.08 \\
3905 & KOI-4060 & 0.10 & 0.07 & 0.10 & 0.20 & 0.12 & 0.20 & 0.06 & 0.12 & 0.18 & -0.01 & 0.15 & 0.16 & 0.14 & 0.15 & 0.07 \\
3906 & KOI-3249 & 0.08 & 0.05 & 0.11 & 0.02 & 0.03 & -0.00 & 0.09 & 0.03 & 0.10 & 0.07 & 0.07 & 0.03 & 0.06 & 0.04 & 0.00 \\
3907 & HAT-P-40 & 0.08 & 0.46 & 0.35 & 0.18 & 0.11 & 0.16 & 0.16 & 0.25 & 0.20 & 0.05 & 0.23 & 0.15 & 0.23 & 0.18 & 0.32 \\
3908 & KOI-4839 & -0.05 & -0.10 & 0.09 & -0.10 & -0.09 & -0.28 & -0.05 & -0.06 & -0.02 & -0.17 & -0.05 & -0.17 & -0.04 & -0.11 & -0.06 \\
3909 & KOI-4198 & -0.46 & -37.41 & -0.10 & -0.56 & -0.35 & -0.63 & -0.28 & -0.25 & -0.17 & -0.98 & -0.35 & -0.63 & -0.33 & -0.44 & -0.35 \\
3910 & KOI-3087 & 0.22 & 0.25 & 0.27 & 0.23 & 0.16 & 0.21 & 0.20 & 0.23 & 0.19 & 0.21 & 0.24 & 0.24 & 0.22 & 0.22 & 0.22 \\
3911 & KOI-3425 & -0.02 & 0.15 & 0.24 & -0.09 & -0.05 & -0.13 & -0.01 & 0.13 & 0.02 & -0.17 & 0.01 & -0.13 & 0.03 & -0.05 & 0.05 \\
3912 & KOI-2874 & -0.06 & -0.31 & -0.04 & -0.15 & -0.10 & -0.11 & -0.07 & -0.11 & -0.07 & -0.12 & -0.09 & -0.20 & -0.11 & -0.12 & -0.21 \\
3913 & KOI-323 & -0.05 & -0.15 & 0.02 & -0.15 & -0.10 & -0.09 & 0.02 & 0.04 & -0.00 & -0.01 & -0.01 & -0.05 & 0.01 & -0.10 & 0.11 \\
3914 & KOI-703 & 0.08 & 0.67 & 0.45 & 0.27 & 0.18 & 0.07 & 0.27 & 0.35 & 0.35 & 0.29 & 0.36 & 0.20 & 0.34 & 0.27 & 0.41 \\
3915 & KOI-2522 & 0.15 & 0.05 & 0.08 & 0.39 & 0.20 & 0.26 & 0.22 & 0.23 & 0.23 & 0.20 & 0.20 & 0.25 & 0.23 & 0.22 & -0.01 \\
3916 & KOI-584 & 0.17 & 0.27 & 0.16 & 0.30 & 0.18 & 0.18 & 0.21 & 0.20 & 0.19 & 0.19 & 0.23 & 0.29 & 0.23 & 0.25 & 0.09 \\
3917 & Kepler-192 & 0.18 & 0.23 & 0.23 & 0.29 & 0.18 & 0.40 & 0.24 & 0.19 & 0.21 & 0.21 & 0.20 & 0.29 & 0.21 & 0.25 & 0.14 \\
3918 & KOI-4222 & -0.12 & -0.30 & -0.03 & -0.20 & -0.13 & -0.26 & -0.11 & -0.07 & -0.08 & -0.44 & -0.10 & -0.17 & -0.08 & -0.15 & -0.04 \\
3919 & KOI-2443 & -0.13 & -0.47 & -0.16 & -0.34 & -0.24 & -0.34 & -0.29 & -0.28 & -0.26 & -0.09 & -0.30 & -0.44 & -0.30 & -0.31 & -0.49 \\
3920 & KOI-2281 & 0.06 & 0.03 & 0.05 & 0.15 & 0.11 & 0.18 & 0.09 & 0.14 & 0.14 & 0.13 & 0.11 & 0.15 & 0.14 & 0.15 & 0.09 \\
3921 & KOI-2162 & -0.39 & -0.42 & -0.35 & -0.41 & -0.40 & -0.39 & -0.46 & -0.42 & -0.32 & -0.42 & -0.42 & -0.41 & -0.40 & -0.41 & -0.41 \\
3922 & KOI-4318 & -0.12 & 0.69 & 0.15 & -0.02 & -0.09 & -0.12 & 0.08 & 0.09 & 0.08 & -0.02 & 0.02 & -0.30 & 0.04 & -0.15 & 0.24 \\
3923 & KOI-704 & -0.18 & -0.25 & -0.07 & -0.23 & -0.17 & -0.19 & -0.18 & -0.10 & -0.12 & -0.19 & -0.12 & -0.26 & -0.14 & -0.22 & -0.11 \\
3924 & KOI-2657 & -0.21 & -0.39 & -0.05 & -0.32 & -0.16 & -0.14 & -0.20 & -0.22 & -0.15 & -0.19 & -0.25 & -0.39 & -0.25 & -0.26 & -0.36 \\
3925 & KOI-3114 & 0.11 & 0.40 & 0.48 & 0.24 & 0.14 & 0.10 & 0.17 & 0.32 & 0.26 & 0.09 & 0.22 & 0.10 & 0.23 & 0.23 & 0.36 \\
3926 & KOI-3867 & 0.06 & 0.02 & -0.01 & 0.04 & 0.07 & 0.02 & 0.05 & 0.05 & 0.04 & 0.03 & 0.03 & 0.07 & 0.06 & 0.07 & -0.07 \\
3927 & KOI-4215 & -0.24 & -0.21 & 0.08 & -0.27 & -0.15 & -0.13 & -0.21 & -0.25 & -0.07 & -0.19 & -0.31 & -0.66 & -0.33 & -0.27 & -0.24 \\
3928 & KOI-2137 & -0.14 & -0.41 & 0.02 & -0.25 & -0.16 & -0.21 & -0.17 & -0.17 & -0.14 & -0.21 & -0.24 & -0.30 & -0.20 & -0.23 & -0.24 \\
3929 & KOI-1411 & 0.25 & 0.27 & 0.25 & 0.30 & 0.23 & 0.33 & 0.24 & 0.23 & 0.26 & 0.22 & 0.25 & 0.27 & 0.26 & 0.29 & 0.16 \\
3930 & KOI-4640 & -0.09 & -0.97 & 0.46 & 0.09 & -0.02 & -0.31 & 0.08 & 0.07 & 0.12 & 0.13 & 0.08 & -0.25 & 0.05 & -0.12 & 0.11 \\
3931 & KOI-1922 & -0.08 & 0.29 & -0.23 & -0.03 & -0.04 & -0.11 & -0.00 & 0.01 & 0.02 & 0.04 & -0.04 & -0.13 & -0.01 & -0.09 & -0.11 \\
3932 & KOI-974 & -0.08 & 0.08 & 0.14 & -0.07 & -0.07 & -0.04 & -0.03 & 0.03 & 0.05 & -0.01 & 0.03 & -0.19 & 0.02 & -0.13 & 0.05 \\
3933 & KOI-1835 & 0.05 & -0.11 & 0.02 & 0.06 & 0.06 & 0.04 & 0.12 & 0.20 & 0.15 & 0.14 & 0.15 & 0.14 & 0.17 & 0.09 & 0.14 \\
3934 & KOI-707 & 0.05 & 0.22 & 0.16 & 0.02 & 0.05 & 0.07 & 0.06 & 0.09 & 0.07 & -0.07 & 0.08 & 0.06 & 0.10 & 0.09 & 0.16 \\
3935 & Kepler-33 & 0.00 & 0.28 & 0.17 & 0.10 & 0.08 & 0.04 & 0.12 & 0.12 & 0.10 & 0.03 & 0.11 & 0.08 & 0.12 & 0.10 & 0.16 \\
3936 & KOI-2079 & 0.23 & 0.32 & 0.18 & 0.37 & 0.25 & 0.34 & 0.26 & 0.31 & 0.26 & 0.28 & 0.30 & 0.33 & 0.30 & 0.31 & 0.14 \\
3937 & KOI-2786 & -0.16 & -0.10 & 0.05 & -0.15 & -0.09 & -0.23 & -0.13 & -0.04 & 0.04 & -0.06 & -0.07 & -0.30 & -0.08 & -0.13 & -0.08 \\
3938 & KOI-941 & 0.25 & 0.48 & 0.27 & 0.50 & 0.29 & 0.41 & 0.31 & 0.43 & 0.33 & 0.33 & 0.43 & 0.38 & 0.38 & 0.35 & 0.38 \\
3939 & Kepler-127 & 0.21 & 0.43 & 0.33 & 0.34 & 0.20 & 0.27 & 0.28 & 0.30 & 0.28 & 0.23 & 0.29 & 0.36 & 0.29 & 0.31 & 0.21 \\
3940 & KOI-271 & 0.19 & 0.17 & 0.31 & 0.36 & 0.22 & 0.34 & 0.26 & 0.30 & 0.30 & 0.27 & 0.31 & 0.30 & 0.30 & 0.27 & 0.26 \\
3941 & KOI-4637 & -0.33 & 0.29 & 0.10 & -0.14 & -0.15 & -0.08 & -0.11 & -0.04 & -0.02 & -0.27 & -0.14 & -0.46 & -0.10 & -0.23 & -0.10 \\
3942 & KOI-2029 & -0.19 & -0.26 & -0.16 & -0.28 & -0.21 & -0.24 & -0.17 & -0.10 & -0.20 & -0.16 & -0.15 & -0.28 & -0.16 & -0.27 & -0.11 \\
3943 & KOI-2694 & 0.12 & 0.44 & 0.04 & 0.54 & 0.27 & 0.22 & 0.23 & 0.24 & 0.27 & 0.21 & 0.23 & 0.35 & 0.27 & 0.29 & 0.08 \\
3944 & KOI-2246 & -0.18 & -0.72 & -0.17 & -0.30 & -0.21 & -0.26 & -0.21 & -0.25 & -0.15 & -0.20 & -0.24 & -0.33 & -0.25 & -0.25 & -0.21 \\
3945 & KOI-119 & 0.24 & 0.46 & 0.27 & 0.45 & 0.22 & 0.32 & 0.25 & 0.34 & 0.27 & 0.21 & 0.29 & 0.40 & 0.30 & 0.38 & 0.24 \\
3946 & KOI-110 & -0.22 & 0.32 & 0.07 & -0.21 & -0.12 & -0.29 & -0.08 & -0.10 & -0.03 & 0.04 & -0.11 & -0.38 & -0.12 & -0.19 & -0.19 \\
3947 & KOI-1813 & -0.04 & -0.07 & 0.09 & -0.13 & -0.06 & -0.10 & -0.04 & -0.00 & -0.01 & -0.09 & -0.01 & -0.08 & -0.02 & -0.09 & 0.05 \\
3948 & KOI-2082 & 0.25 & 0.30 & 0.37 & 0.41 & 0.26 & 0.26 & 0.30 & 0.32 & 0.26 & 0.21 & 0.33 & 0.39 & 0.34 & 0.38 & 0.29 \\
3949 & KOI-939 & 0.19 & 0.26 & 0.08 & 0.27 & 0.13 & 0.13 & 0.19 & 0.19 & 0.12 & 0.06 & 0.14 & 0.22 & 0.15 & 0.19 & 0.09 \\
3950 & KOI-2717 & 0.03 & 0.18 & 0.05 & -0.02 & 0.03 & -0.09 & 0.03 & 0.06 & 0.06 & 0.07 & 0.07 & -0.04 & 0.03 & -0.00 & 0.13 \\
3951 & KOI-1978 & 0.06 & -0.08 & 0.02 & -0.03 & 0.07 & 0.07 & 0.03 & 0.06 & 0.09 & 0.05 & 0.09 & 0.07 & 0.07 & 0.07 & 0.23 \\
3952 & KOI-708 & -0.13 & 0.23 & 0.09 & -0.09 & -0.10 & -0.22 & -0.06 & -0.04 & 0.01 & -0.09 & -0.04 & -0.23 & -0.05 & -0.15 & -0.13 \\
3953 & KOI-3132 & 0.21 & 0.72 & 0.72 & 0.49 & 0.28 & 0.44 & 0.38 & 0.45 & 0.37 & 0.22 & 0.42 & 0.52 & 0.44 & 0.45 & 0.33 \\
3954 & KOI-49 & -0.05 & -0.04 & 0.14 & -0.02 & -0.06 & 0.08 & -0.01 & -0.01 & 0.09 & 0.17 & -0.05 & -0.20 & -0.05 & -0.12 & -0.24 \\
3955 & KOI-1806 & -0.03 & -0.10 & 0.03 & -0.19 & -0.03 & -0.01 & -0.01 & 0.06 & 0.12 & 0.05 & -0.01 & -0.34 & -0.02 & -0.06 & 0.06 \\
3956 & KOI-165 & -0.16 & -0.44 & -0.01 & -0.25 & -0.26 & -0.16 & -0.23 & -0.16 & -0.19 & -0.19 & -0.25 & -0.30 & -0.29 & -0.29 & -0.34 \\
3957 & KOI-1886 & -0.01 & 0.22 & 0.21 & 0.01 & -0.02 & -0.33 & 0.01 & 0.06 & 0.16 & 0.20 & 0.11 & -0.10 & 0.09 & 0.02 & 0.16 \\
3958 & KOI-709 & -0.19 & -0.39 & -0.01 & -0.34 & -0.18 & -0.15 & -0.24 & -0.22 & -0.17 & -0.22 & -0.23 & -0.34 & -0.21 & -0.25 & -0.38 \\
3959 & KOI-3165 & -0.28 & 0.14 & 0.01 & -0.23 & -0.14 & -0.28 & -0.14 & -0.11 & -0.01 & -0.11 & -0.16 & -0.41 & -0.12 & -0.21 & 0.32 \\
3960 & KOI-3232 & -0.00 & -0.16 & 0.03 & -0.01 & -0.05 & 0.01 & 0.05 & 0.05 & 0.02 & 0.05 & 0.06 & 0.00 & 0.04 & 0.01 & 0.11 \\
3961 & KOI-288 & 0.17 & 0.04 & 0.38 & 0.23 & 0.12 & 0.19 & 0.20 & 0.27 & 0.24 & 0.16 & 0.26 & 0.20 & 0.27 & 0.23 & 0.40 \\
3962 & KOI-1819 & -0.15 & -0.13 & -0.03 & -0.18 & -0.11 & -0.08 & -0.06 & 0.01 & -0.03 & -0.04 & -0.01 & -0.16 & -0.03 & -0.15 & 0.00 \\
3963 & KOI-3229 & -0.30 & -0.47 & -0.13 & -0.40 & -0.30 & -0.20 & -0.29 & -0.34 & -0.22 & -0.18 & -0.40 & -0.63 & -0.41 & -0.39 & -0.48 \\
3964 & KOI-711 & 0.25 & 0.36 & 0.27 & 0.39 & 0.26 & 0.33 & 0.26 & 0.27 & 0.25 & 0.24 & 0.30 & 0.34 & 0.30 & 0.31 & 0.18 \\
3965 & KOI-115 & -0.07 & -0.15 & -0.06 & -0.17 & -0.09 & -0.10 & -0.06 & -0.08 & -0.06 & -0.06 & -0.09 & -0.25 & -0.11 & -0.16 & -0.04 \\
3966 & KOI-710 & -0.35 & 0.22 & 0.11 & -0.12 & -0.15 & -0.31 & -0.12 & 0.08 & -0.08 & -0.24 & -0.02 & -0.30 & -0.03 & -0.27 & -0.04 \\
3967 & Kepler-217 & -0.23 & 0.03 & 0.14 & -0.01 & -0.11 & -0.03 & -0.01 & 0.08 & 0.06 & -0.17 & 0.01 & -0.17 & 0.00 & -0.19 & -0.03 \\
3968 & KOI-2612 & 0.18 & 0.17 & 0.07 & 0.29 & 0.21 & 0.22 & 0.22 & 0.23 & 0.22 & 0.12 & 0.23 & 0.25 & 0.22 & 0.24 & 0.17 \\
3969 & KOI-2884 & -0.11 & -0.12 & -0.01 & -0.11 & -0.10 & -0.05 & -0.10 & 0.03 & -0.01 & -0.06 & -0.02 & -0.09 & -0.03 & -0.06 & -0.03 \\
3970 & KOI-1970 & 0.01 & 0.01 & -0.05 & 0.06 & 0.05 & 0.07 & -0.04 & 0.04 & 0.07 & 0.06 & -0.00 & 0.11 & 0.02 & 0.00 & -0.02 \\
3971 & KOI-4430 & -0.00 & -0.12 & 0.02 & 0.09 & -0.02 & 0.01 & 0.07 & 0.10 & 0.06 & 0.04 & 0.09 & 0.06 & 0.09 & 0.03 & 0.11 \\
3972 & KOI-179 & 0.16 & 0.48 & 0.39 & 0.19 & 0.15 & 0.05 & 0.22 & 0.25 & 0.21 & 0.05 & 0.30 & 0.20 & 0.28 & 0.19 & 0.60 \\
3973 & KOI-2049 & 0.02 & 0.35 & 0.13 & -0.02 & 0.02 & 0.07 & 0.06 & 0.14 & 0.01 & 0.02 & 0.03 & -0.00 & 0.06 & 0.07 & 0.16 \\
3974 & KOI-712 & -0.09 & -0.09 & 0.01 & -0.14 & -0.09 & -0.03 & -0.01 & -0.03 & -0.08 & -0.06 & -0.08 & -0.18 & -0.07 & -0.12 & -0.02 \\
3975 & KOI-1938 & -0.24 & -0.44 & -0.21 & -0.30 & -0.22 & -0.20 & -0.28 & -0.25 & -0.23 & -0.25 & -0.24 & -0.33 & -0.26 & -0.27 & -0.25 \\
3976 & KOI-2815 & -0.04 & -0.27 & -0.07 & -0.12 & -0.06 & -0.04 & -0.06 & -0.09 & -0.09 & -0.02 & -0.04 & -0.14 & -0.06 & -0.09 & -0.09 \\
3977 & Kepler-423 & 0.02 & -0.15 & 0.06 & 0.05 & 0.04 & 0.16 & 0.10 & 0.04 & 0.08 & 0.15 & 0.03 & -0.10 & 0.04 & 0.04 & 0.09 \\
3978 & KOI-1854 & -0.10 & 0.04 & -0.02 & -0.09 & -0.03 & 0.01 & -0.00 & -0.00 & -0.04 & -0.02 & -0.02 & -0.06 & -0.03 & -0.04 & -0.02 \\
3979 & KOI-4822 & -0.03 & -0.05 & 0.03 & -0.04 & -0.03 & 0.00 & -0.05 & 0.01 & 0.02 & -0.05 & -0.01 & -0.15 & -0.02 & -0.05 & -0.02 \\
3980 & KOI-4617 & -0.09 & -0.63 & -0.04 & -0.20 & -0.10 & -0.16 & -0.11 & -0.07 & -0.03 & -0.04 & -0.11 & -0.33 & -0.12 & -0.15 & -0.14 \\
3981 & KOI-2831 & -0.12 & -0.15 & 0.04 & -0.07 & -0.11 & -0.09 & -0.10 & -0.02 & -0.02 & -0.18 & -0.07 & -0.17 & -0.05 & -0.09 & 0.03 \\
3982 & KOI-2706 & -0.10 & 0.30 & 0.35 & 0.17 & 0.06 & 0.01 & 0.13 & 0.24 & 0.21 & 0.13 & 0.15 & 0.01 & 0.19 & 0.11 & 0.21 \\
3983 & KOI-2769 & -0.14 & 0.08 & -0.04 & -0.09 & -0.11 & -0.15 & -0.15 & -0.01 & -0.06 & -0.19 & -0.08 & -0.16 & -0.06 & -0.12 & -0.03 \\
3984 & KOI-2545 & 0.07 & 0.43 & 0.36 & 0.12 & 0.07 & 0.07 & 0.13 & 0.23 & 0.27 & 0.22 & 0.19 & 0.07 & 0.19 & 0.15 & 0.37 \\
3985 & KOI-1751 & -0.18 & -0.35 & -0.23 & -0.13 & -0.09 & -0.06 & -0.08 & -0.02 & -0.04 & -0.07 & -0.03 & -0.15 & -0.06 & -0.09 & 0.05 \\
3986 & KOI-1913 & 0.07 & 0.12 & 0.04 & 0.13 & 0.10 & 0.08 & 0.14 & 0.15 & 0.15 & 0.12 & 0.11 & 0.17 & 0.16 & 0.12 & 0.09 \\
3987 & KOI-714 & -0.05 & -0.13 & -0.01 & -0.04 & 0.05 & 0.07 & 0.05 & 0.08 & 0.09 & 0.06 & 0.06 & -0.02 & 0.07 & 0.05 & 0.07 \\
3988 & KOI-2913 & 0.23 & 0.40 & 0.30 & 0.40 & 0.25 & 0.33 & 0.28 & 0.27 & 0.25 & 0.21 & 0.29 & 0.37 & 0.26 & 0.32 & 0.25 \\
3989 & KOI-2273 & 0.12 & 0.16 & 0.23 & 0.29 & 0.20 & 0.19 & 0.21 & 0.30 & 0.25 & 0.20 & 0.25 & 0.27 & 0.24 & 0.25 & 0.32 \\
3990 & KOI-2035 & -0.09 & -0.30 & -0.04 & -0.15 & -0.05 & -0.15 & -0.01 & 0.07 & 0.05 & 0.01 & 0.04 & -0.09 & 0.04 & -0.08 & 0.18 \\
3991 & KOI-2457 & -0.30 & 0.09 & 0.14 & -0.11 & -0.05 & -0.34 & 0.09 & 0.07 & 0.12 & -0.16 & 0.01 & -0.35 & 0.03 & -0.12 & 0.12 \\
3992 & KOI-3871 & -0.01 & -0.24 & 0.00 & -0.08 & 0.02 & -0.02 & 0.05 & 0.08 & 0.05 & 0.05 & 0.06 & 0.02 & 0.06 & 0.02 & 0.09 \\
3993 & KOI-3162 & 0.06 & 0.24 & 0.23 & -0.15 & -0.07 & -0.25 & 0.09 & 0.09 & 0.10 & 0.02 & 0.10 & -0.04 & 0.09 & -0.04 & 0.15 \\
3994 & KOI-3465 & -0.04 & 0.02 & 0.01 & -0.08 & -0.07 & 0.01 & -0.02 & 0.03 & -0.02 & -0.04 & 0.01 & -0.06 & 0.00 & -0.07 & 0.25 \\
3995 & KOI-3837 & -0.17 & 0.04 & 0.00 & -0.41 & -0.07 & -0.57 & -0.04 & -0.15 & 0.17 & 0.34 & -0.07 & -0.32 & -0.06 & -0.15 & -0.09 \\
3996 & KOI-1852 & -0.34 & -0.40 & -0.07 & -0.25 & -0.08 & -0.20 & -0.11 & -0.08 & 0.03 & -0.12 & -0.11 & -0.34 & -0.10 & -0.20 & 0.05 \\
3997 & KOI-1529 & -0.14 & -2.63 & 0.04 & -0.40 & -0.26 & -0.22 & -0.19 & -0.25 & -0.13 & -0.32 & -0.20 & -0.42 & -0.23 & -0.29 & -0.29 \\
3998 & KOI-2943 & 0.26 & 0.42 & 0.28 & 0.48 & 0.26 & 0.29 & 0.29 & 0.29 & 0.26 & 0.22 & 0.31 & 0.37 & 0.28 & 0.37 & 0.24 \\
3999 & KOI-135 & 0.22 & 0.53 & 0.31 & 0.49 & 0.28 & 0.34 & 0.35 & 0.37 & 0.31 & 0.31 & 0.35 & 0.48 & 0.35 & 0.39 & 0.28 \\
4000 & KOI-4421 & 0.04 & -0.24 & 0.06 & -0.09 & 0.01 & 0.03 & -0.00 & 0.06 & 0.04 & 0.05 & 0.04 & -0.06 & 0.06 & 0.00 & 0.17 \\
4001 & KOI-1715 & -0.14 & -0.20 & -0.06 & -0.27 & -0.23 & -0.14 & -0.19 & -0.23 & -0.21 & -0.20 & -0.29 & -0.38 & -0.25 & -0.34 & -0.29 \\
4002 & KOI-1958 & -0.11 & 0.10 & -0.13 & -0.09 & -0.04 & -0.05 & -0.04 & 0.03 & 0.06 & 0.02 & 0.08 & -0.14 & 0.05 & -0.07 & 0.08 \\
4003 & KOI-716 & 0.05 & 0.24 & 0.22 & 0.21 & 0.14 & 0.10 & 0.11 & 0.22 & 0.18 & 0.10 & 0.18 & 0.11 & 0.17 & 0.17 & 0.17 \\
4004 & KOI-1606 & 0.04 & 0.07 & 0.07 & 0.10 & 0.02 & -0.01 & 0.03 & 0.06 & 0.05 & 0.04 & 0.06 & 0.06 & 0.04 & 0.04 & 0.10 \\
4005 & KOI-717 & 0.23 & 0.22 & 0.21 & 0.24 & 0.25 & 0.31 & 0.24 & 0.21 & 0.26 & 0.24 & 0.24 & 0.30 & 0.26 & 0.28 & 0.14 \\
4006 & KOI-4230 & -0.23 & -0.37 & -0.10 & -0.43 & -0.33 & -0.32 & -0.31 & -0.32 & -0.22 & -0.30 & -0.34 & -0.65 & -0.33 & -0.43 & -0.36 \\
4007 & KOI-3246 & 0.27 & -0.01 & 0.26 & 0.21 & 0.02 & 0.10 & 0.13 & 0.21 & 0.10 & 0.08 & 0.05 & 0.14 & 0.14 & 0.10 & -0.08 \\
4008 & KOI-1955 & 0.03 & 0.60 & 0.30 & 0.09 & 0.05 & 0.07 & 0.13 & 0.16 & 0.18 & 0.16 & 0.18 & 0.06 & 0.15 & 0.03 & 0.31 \\
4009 & Kepler-342 & 0.07 & 0.34 & 0.20 & 0.06 & 0.06 & 0.04 & 0.11 & 0.18 & 0.21 & 0.19 & 0.12 & 0.06 & 0.15 & 0.10 & 0.13 \\
4010 & KOI-2135 & 0.06 & 0.38 & 0.20 & -0.01 & 0.01 & -0.11 & 0.04 & 0.06 & 0.12 & -0.18 & 0.06 & -0.05 & 0.05 & 0.03 & 0.21 \\
4011 & KOI-2732 & 0.05 & -0.06 & 0.10 & -0.01 & 0.03 & -0.03 & 0.04 & 0.10 & 0.14 & -0.05 & 0.04 & 0.01 & 0.10 & 0.05 & 0.08 \\
4012 & Kepler-403 & 0.06 & 0.10 & 0.26 & 0.08 & 0.01 & 0.03 & 0.07 & 0.15 & 0.10 & 0.07 & 0.09 & 0.02 & 0.09 & 0.02 & 0.12 \\
4013 & KOI-4575 & -0.09 & 0.07 & 0.33 & 0.01 & -0.02 & 0.01 & 0.06 & 0.14 & 0.09 & -0.10 & 0.08 & -0.24 & 0.07 & -0.06 & 0.21 \\
4014 & KOI-718 & 0.28 & 0.40 & 0.28 & 0.39 & 0.32 & 0.27 & 0.37 & 0.36 & 0.31 & 0.33 & 0.34 & 0.38 & 0.33 & 0.38 & 0.31 \\
4015 & Kepler-219 & 0.28 & 0.29 & 0.30 & 0.46 & 0.29 & 0.45 & 0.37 & 0.33 & 0.36 & 0.36 & 0.37 & 0.44 & 0.35 & 0.40 & 0.34 \\
4016 & KOI-327 & -0.02 & -0.02 & 0.05 & -0.09 & -0.02 & -0.14 & -0.05 & -0.01 & -0.04 & -0.07 & -0.01 & -0.12 & -0.00 & -0.07 & -0.03 \\
4017 & KOI-4383 & 0.01 & -0.25 & 0.05 & -0.13 & 0.02 & -0.03 & -0.03 & 0.02 & 0.00 & 0.01 & 0.05 & -0.02 & 0.02 & -0.03 & 0.18 \\
4018 & KOI-1537 & -0.19 & 0.12 & 0.00 & -0.24 & -0.15 & -0.20 & -0.15 & -0.04 & -0.09 & -0.21 & -0.13 & -0.42 & -0.10 & -0.25 & -0.10 \\
4019 & KOI-2803 & 0.10 & 0.16 & 0.15 & 0.14 & 0.09 & 0.10 & 0.06 & 0.10 & 0.08 & 0.09 & 0.12 & 0.13 & 0.08 & 0.12 & 0.08 \\
4020 & KOI-1779 & 0.14 & -0.06 & 0.13 & 0.15 & 0.16 & -0.00 & 0.23 & 0.26 & 0.21 & 0.28 & 0.26 & 0.26 & 0.29 & 0.19 & 0.26 \\
4021 & KOI-721 & 0.03 & 0.22 & 0.10 & 0.13 & 0.06 & 0.11 & 0.06 & 0.15 & 0.08 & 0.08 & 0.10 & 0.15 & 0.12 & 0.10 & 0.15 \\
4022 & KOI-720 & -0.12 & -0.23 & -0.04 & -0.21 & -0.13 & -0.18 & -0.07 & -0.01 & -0.05 & -0.05 & -0.01 & -0.07 & -0.02 & -0.12 & 0.02 \\
4023 & KOI-722 & 0.12 & 0.66 & -0.30 & 0.03 & 0.22 & 0.08 & 0.02 & 0.12 & 0.21 & 0.49 & 0.14 & -0.07 & 0.15 & 0.03 & 0.09 \\
4024 & KOI-4431 & -0.10 & 0.01 & 0.15 & -0.25 & -0.21 & -0.36 & -0.17 & -0.10 & -0.08 & -0.38 & -0.12 & -0.38 & -0.10 & -0.24 & -0.14 \\
4025 & KOI-1875 & -0.11 & -0.36 & 0.01 & -0.28 & -0.06 & -0.08 & -0.08 & -0.15 & -0.03 & -0.05 & -0.15 & -0.37 & -0.16 & -0.17 & -0.17 \\
4026 & KOI-4647 & -0.01 & 0.12 & -0.01 & 0.16 & 0.11 & 0.17 & 0.05 & 0.16 & 0.16 & 0.12 & 0.19 & 0.28 & 0.20 & 0.21 & 0.28 \\
4027 & KOI-528 & -0.17 & -0.54 & -0.33 & -0.20 & -0.02 & 0.01 & -0.04 & -0.12 & -0.02 & -0.11 & -0.13 & -0.14 & -0.10 & -0.12 & -0.15 \\
4028 & KOI-2748 & -0.15 & -0.26 & 0.06 & -0.19 & -0.09 & -0.02 & -0.13 & -0.06 & -0.03 & -0.11 & -0.19 & -0.30 & -0.14 & -0.16 & -0.11 \\
4029 & KOI-2832 & 0.03 & 0.05 & -0.01 & 0.15 & 0.05 & 0.07 & 0.09 & 0.08 & 0.10 & 0.08 & 0.10 & 0.09 & 0.09 & 0.08 & -0.02 \\
4030 & KOI-2312 & -0.50 & -0.07 & -0.12 & -0.11 & -0.23 & -1.21 & -0.14 & -0.02 & 0.00 & -0.35 & -0.21 & -0.43 & -0.17 & -0.29 & -0.20 \\
4031 & KOI-4146 & 0.10 & 0.01 & 0.07 & 0.15 & 0.10 & 0.19 & 0.17 & 0.28 & 0.19 & 0.18 & 0.24 & 0.21 & 0.24 & 0.17 & 0.14 \\
4032 & KOI-4706 & -0.22 & -0.02 & -0.10 & -0.34 & -0.24 & -0.30 & -0.16 & -0.18 & -0.10 & -0.05 & -0.25 & -0.50 & -0.22 & -0.31 & -0.28 \\
4033 & KOI-3382 & 0.04 & 0.06 & 0.04 & 0.08 & 0.13 & 0.13 & 0.07 & 0.11 & 0.18 & 0.10 & 0.13 & 0.15 & 0.12 & 0.11 & -0.09 \\
4034 & KOI-723 & 0.13 & 0.03 & 0.11 & 0.24 & 0.16 & 0.30 & 0.25 & 0.29 & 0.26 & 0.24 & 0.27 & 0.29 & 0.27 & 0.26 & 0.20 \\
4035 & KOI-1796 & -0.04 & -0.10 & 0.03 & -0.13 & -0.04 & -0.11 & -0.04 & -0.00 & -0.03 & -0.00 & -0.00 & -0.12 & -0.02 & -0.11 & 0.00 \\
4036 & KOI-2785 & -0.01 & 0.02 & 0.06 & -0.00 & -0.01 & 0.01 & 0.02 & -0.00 & 0.02 & -0.02 & -0.04 & -0.02 & -0.01 & 0.01 & -0.05 \\
4037 & KOI-4469 & -0.03 & -0.31 & -0.12 & 0.16 & 0.02 & 0.06 & 0.07 & 0.07 & 0.07 & 0.07 & 0.07 & -0.00 & 0.06 & 0.07 & -0.20 \\
4038 & WASP-113 & 0.20 & 0.32 & 0.27 & 0.33 & 0.23 & 0.26 & 0.26 & 0.29 & 0.27 & 0.20 & 0.28 & 0.35 & 0.29 & 0.32 & 0.31 \\
4039 & KOI-1598 & -0.20 & -0.72 & -0.04 & -0.25 & -0.17 & -0.19 & -0.18 & -0.19 & -0.12 & -0.21 & -0.16 & -0.34 & -0.21 & -0.22 & -0.05 \\
4040 & Kepler-310 & -0.22 & -0.40 & -0.25 & -0.24 & -0.19 & -0.20 & -0.14 & -0.17 & -0.17 & -0.16 & -0.22 & -0.31 & -0.24 & -0.24 & -0.27 \\
4041 & KOI-1783 & 0.09 & 0.14 & 0.09 & 0.09 & 0.12 & 0.05 & 0.10 & 0.12 & 0.09 & 0.04 & 0.12 & 0.11 & 0.11 & 0.12 & 0.16 \\
4042 & KOI-2002 & 0.01 & 0.11 & -0.03 & -0.04 & 0.00 & 0.07 & 0.03 & 0.13 & 0.09 & 0.22 & 0.07 & -0.02 & 0.03 & -0.05 & 0.08 \\
4043 & KOI-1984 & 0.04 & 0.15 & 0.15 & 0.10 & 0.07 & 0.07 & 0.11 & 0.17 & 0.12 & 0.03 & 0.15 & 0.11 & 0.14 & 0.09 & 0.09 \\
4044 & HAT-P-44 & 0.32 & 0.41 & 0.33 & 0.51 & 0.28 & 0.41 & 0.35 & 0.30 & 0.31 & 0.31 & 0.31 & 0.43 & 0.33 & 0.38 & 0.17 \\
4045 & KOI-4292 & 0.06 & 0.02 & 0.24 & 0.01 & 0.06 & 0.18 & 0.07 & -0.02 & 0.12 & 0.03 & -0.06 & -0.14 & -0.05 & -0.03 & -0.14 \\
4046 & KOI-2891 & 0.06 & -0.06 & 0.21 & 0.03 & 0.03 & -0.04 & 0.06 & 0.19 & 0.16 & 0.01 & 0.13 & -0.00 & 0.15 & 0.08 & 0.25 \\
4047 & KOI-1917 & -0.08 & -0.18 & -0.05 & -0.11 & -0.11 & -0.11 & -0.09 & -0.08 & -0.07 & -0.03 & -0.08 & -0.25 & -0.09 & -0.15 & -0.06 \\
4048 & KOI-2964 & -0.25 & 0.14 & 0.02 & -0.53 & -0.36 & -0.42 & -0.30 & -0.28 & -0.27 & -0.39 & -0.35 & -0.61 & -0.35 & -0.43 & -0.59 \\
4049 & KOI-1608 & -0.03 & -0.17 & -0.09 & -0.10 & -0.02 & -0.08 & -0.09 & -0.06 & 0.02 & -0.17 & -0.03 & -0.11 & -0.03 & -0.06 & -0.08 \\
4050 & KOI-1888 & -0.10 & 0.20 & 0.32 & -0.00 & 0.07 & -1.12 & 0.12 & 0.18 & 0.23 & 0.07 & 0.13 & 0.14 & 0.19 & 0.07 & 0.27 \\
4051 & KOI-1909 & -0.04 & -0.14 & -0.03 & -0.12 & -0.02 & -0.06 & -0.02 & 0.03 & -0.01 & -0.12 & -0.01 & -0.08 & -0.00 & -0.04 & -0.01 \\
4052 & Kepler-334 & 0.01 & -0.25 & -0.00 & -0.04 & 0.00 & -0.05 & 0.02 & 0.03 & 0.02 & -0.01 & 0.02 & -0.08 & 0.02 & -0.04 & 0.05 \\
4053 & KOI-1929 & -0.05 & -0.01 & 0.00 & -0.11 & -0.03 & 0.08 & -0.04 & 0.04 & 0.05 & -0.05 & -0.00 & -0.10 & 0.02 & -0.02 & -0.04 \\
4054 & KOI-3195 & -0.29 & -1.79 & -0.00 & -0.40 & -0.36 & -0.42 & -0.33 & -0.25 & -0.16 & -0.45 & -0.29 & -0.68 & -0.33 & -0.44 & -0.31 \\
4055 & KOI-1784 & 0.03 & 0.30 & 0.11 & -0.07 & -0.01 & 0.10 & 0.05 & -0.00 & 0.04 & 0.05 & 0.09 & -0.04 & 0.04 & 0.05 & 0.30 \\
4056 & KOI-3208 & -0.07 & -0.45 & -0.14 & -0.15 & -0.08 & -0.25 & -0.12 & -0.08 & -0.05 & -0.08 & -0.10 & -0.20 & -0.13 & -0.15 & -0.08 \\
4057 & KOI-991 & -0.27 & -0.57 & -0.16 & -0.29 & -0.23 & -0.25 & -0.22 & -0.22 & -0.18 & -0.23 & -0.23 & -0.35 & -0.25 & -0.27 & -0.23 \\
4058 & KOI-4613 & -0.19 & -0.40 & -0.13 & -0.34 & -0.13 & -0.12 & -0.20 & -0.14 & -0.13 & -0.08 & -0.21 & -0.32 & -0.18 & -0.19 & -0.11 \\
4059 & KOI-3218 & 0.05 & 0.01 & -0.10 & -0.07 & 0.03 & -0.03 & 0.05 & 0.06 & 0.06 & 0.06 & 0.09 & 0.02 & 0.06 & 0.02 & 0.09 \\
4060 & KOI-4070 & -0.10 & -0.05 & -0.12 & 0.02 & 0.06 & 0.04 & 0.01 & 0.03 & 0.08 & 0.03 & 0.06 & 0.03 & 0.04 & 0.08 & 0.03 \\
4061 & KOI-2342 & -0.30 & -0.13 & -0.20 & -0.50 & -0.32 & -0.42 & -0.34 & -0.30 & -0.16 & -0.02 & -0.40 & -0.67 & -0.39 & -0.46 & -0.58 \\
4062 & KOI-427 & -0.05 & -0.08 & -0.14 & 0.00 & 0.06 & 0.02 & 0.02 & 0.03 & 0.11 & 0.03 & 0.03 & 0.04 & 0.07 & 0.05 & 0.17 \\
4063 & KOI-3130 & -0.30 & -0.23 & -0.23 & -0.48 & -0.41 & -0.47 & -0.35 & -0.42 & -0.41 & -0.41 & -0.51 & -0.60 & -0.48 & -0.46 & -0.93 \\
4064 & KOI-5782 & -0.16 & 0.15 & -0.07 & -0.01 & 0.06 & 0.10 & -0.07 & 0.13 & 0.14 & 0.04 & 0.13 & 0.23 & 0.14 & 0.14 & 0.23 \\
4065 & KOI-331 & -0.03 & 0.01 & 0.01 & -0.03 & 0.01 & 0.08 & -0.07 & 0.01 & 0.05 & 0.01 & 0.01 & 0.03 & 0.05 & 0.03 & 0.09 \\
4066 & KOI-2390 & -0.04 & 0.13 & 0.19 & -0.00 & -0.03 & 0.05 & 0.04 & 0.13 & 0.09 & -0.16 & 0.07 & -0.09 & 0.08 & 0.03 & 0.33 \\
4067 & KOI-732 & 0.19 & 0.28 & 0.19 & 0.34 & 0.22 & 0.27 & 0.22 & 0.21 & 0.21 & 0.21 & 0.23 & 0.22 & 0.24 & 0.26 & 0.06 \\
4068 & KOI-4557 & 0.01 & -0.00 & 0.08 & 0.04 & 0.01 & 0.03 & -0.00 & 0.09 & 0.02 & -0.01 & -0.00 & -0.03 & 0.04 & 0.03 & -0.03 \\
4069 & KOI-3608 & -0.11 & 0.01 & -0.11 & -0.12 & -0.08 & -0.02 & -0.12 & -0.05 & -0.06 & 0.06 & -0.07 & -0.17 & -0.09 & -0.13 & -0.11 \\
4070 & KOI-332 & 0.24 & 0.24 & 0.26 & 0.40 & 0.26 & 0.34 & 0.30 & 0.28 & 0.25 & 0.25 & 0.30 & 0.39 & 0.32 & 0.35 & 0.22 \\
4071 & KOI-2153 & -0.04 & -0.42 & 0.05 & -0.08 & -0.06 & -0.19 & -0.08 & 0.03 & 0.01 & -0.11 & -0.02 & -0.14 & -0.00 & -0.08 & 0.04 \\
4072 & KOI-333 & -0.06 & 0.49 & 0.16 & -0.07 & 0.09 & -0.02 & 0.04 & 0.19 & 0.20 & 0.16 & 0.15 & -0.10 & 0.15 & 0.04 & 0.16 \\
4073 & KOI-1905 & -0.20 & -0.49 & -0.22 & -0.25 & -0.16 & -0.13 & -0.12 & -0.10 & -0.14 & -0.13 & -0.15 & -0.23 & -0.15 & -0.19 & -0.23 \\
4074 & KOI-3216 & 0.09 & 0.09 & 0.14 & 0.11 & -0.03 & 0.06 & -0.06 & 0.18 & 0.25 & 0.16 & 0.10 & 0.05 & 0.07 & -0.04 & -0.44 \\
4075 & KOI-3908 & -0.05 & -0.73 & -0.12 & -0.12 & -0.03 & 0.01 & -0.04 & 0.04 & 0.04 & -0.07 & -0.03 & -0.08 & 0.01 & 0.00 & 0.11 \\
4076 & KOI-1175 & -0.08 & -0.06 & -0.02 & -0.09 & -0.02 & -0.07 & -0.06 & 0.06 & -0.01 & -0.14 & 0.02 & -0.03 & 0.03 & -0.02 & 0.13 \\
4077 & KOI-1169 & 0.04 & -0.03 & 0.06 & 0.09 & 0.08 & 0.14 & 0.08 & 0.07 & 0.09 & 0.11 & 0.06 & 0.02 & 0.07 & 0.08 & 0.02 \\
4078 & KOI-1165 & -0.13 & -0.10 & -0.10 & -0.12 & -0.12 & -0.06 & -0.10 & -0.10 & -0.07 & -0.14 & -0.10 & -0.13 & -0.11 & -0.12 & -0.09 \\
4079 & KOI-3991 & -0.17 & 0.01 & -0.11 & -0.20 & -0.17 & -0.28 & -0.11 & -0.04 & -0.10 & -0.04 & -0.06 & -0.23 & -0.09 & -0.20 & 0.00 \\
4080 & KOI-4446 & -0.22 & -0.41 & 0.03 & -0.31 & -0.16 & -0.09 & -0.27 & -0.23 & -0.09 & -0.19 & -0.38 & -0.54 & -0.34 & -0.29 & -0.31 \\
4081 & KOI-2147 & -0.19 & -0.01 & -0.12 & -0.21 & -0.15 & -0.04 & -0.18 & -0.08 & -0.03 & 0.09 & -0.18 & -0.29 & -0.20 & -0.25 & -0.25 \\
4082 & KOI-2859 & -0.11 & -0.14 & -0.01 & -0.20 & -0.10 & -0.12 & -0.08 & -0.11 & -0.09 & -0.13 & -0.15 & -0.14 & -0.15 & -0.14 & -0.24 \\
4083 & KOI-4556 & -0.21 & -0.04 & -0.08 & -0.22 & -0.15 & -0.16 & -0.15 & -0.11 & -0.10 & -0.17 & -0.13 & -0.30 & -0.14 & -0.15 & 0.03 \\
4084 & KOI-289 & -0.23 & -0.75 & -0.18 & -0.21 & -0.23 & -0.15 & -0.15 & -0.14 & 0.09 & -0.24 & -0.27 & -0.29 & -0.26 & -0.25 & -0.29 \\
4085 & KOI-3224 & -0.05 & -0.17 & 0.01 & -0.05 & -0.05 & -0.02 & -0.01 & 0.00 & -0.01 & 0.01 & 0.03 & -0.06 & -0.01 & -0.04 & -0.02 \\
4086 & KOI-2583 & -0.04 & -0.09 & -0.06 & -0.00 & 0.01 & 0.03 & 0.04 & 0.04 & 0.05 & 0.08 & 0.02 & 0.05 & 0.04 & 0.05 & 0.04 \\
4087 & KOI-1161 & 0.02 & -0.38 & 0.25 & -0.04 & -0.11 & 0.07 & -0.06 & -0.03 & -0.02 & -0.01 & -0.01 & -0.11 & -0.08 & -0.10 & -0.09 \\
4088 & KOI-1168 & 0.09 & 0.37 & 0.39 & 0.06 & -0.00 & 0.07 & 0.06 & 0.20 & 0.18 & 0.07 & 0.09 & -0.00 & 0.11 & 0.01 & 0.09 \\
4089 & KOI-2040 & -0.08 & -0.08 & -0.05 & -0.05 & -0.03 & -0.03 & -0.02 & -0.03 & -0.01 & -0.05 & -0.06 & -0.08 & -0.06 & -0.04 & -0.17 \\
4090 & KOI-474 & -0.02 & -0.32 & 0.07 & -0.08 & -0.04 & -0.17 & -0.00 & -0.04 & -0.01 & -0.15 & 0.00 & -0.05 & -0.01 & -0.10 & 0.06 \\
4091 & Kepler-164 & 0.06 & 0.58 & 0.04 & 0.02 & 0.05 & 0.10 & 0.05 & 0.06 & 0.08 & 0.01 & 0.06 & 0.02 & 0.03 & -0.01 & 0.14 \\
4092 & KOI-2484 & -0.26 & 0.04 & 0.03 & -0.29 & -0.23 & -0.22 & -0.21 & -0.25 & -0.09 & -0.02 & -0.36 & -0.70 & -0.36 & -0.34 & -0.37 \\
4093 & KOI-3231 & -0.08 & 0.10 & 0.04 & 0.12 & 0.08 & -0.00 & 0.01 & 0.03 & 0.10 & 0.05 & 0.12 & -0.10 & 0.04 & 0.09 & 0.35 \\
4094 & KOI-4480 & 0.20 & 0.26 & 0.19 & 0.30 & 0.16 & 0.25 & 0.23 & 0.26 & 0.18 & 0.24 & 0.25 & 0.24 & 0.21 & 0.23 & 0.22 \\
4095 & KOI-2961 & 0.06 & 0.38 & 0.14 & 0.05 & 0.06 & 0.03 & 0.28 & 0.11 & 0.21 & 0.19 & 0.08 & -0.01 & 0.14 & 0.04 & 0.13 \\
4096 & KOI-1163 & -0.31 & -0.85 & -0.23 & -0.28 & -0.30 & -0.22 & -0.29 & -0.28 & -0.26 & -0.35 & -0.27 & -0.44 & -0.34 & -0.35 & -0.19 \\
4097 & KOI-2208 & 0.06 & 0.06 & 0.04 & 0.07 & 0.09 & 0.16 & 0.03 & 0.08 & 0.09 & 0.11 & 0.09 & 0.09 & 0.07 & 0.12 & 0.06 \\
4098 & KOI-338 & 0.30 & 0.38 & 0.25 & 0.53 & 0.29 & 0.33 & 0.33 & 0.36 & 0.30 & 0.31 & 0.35 & 0.41 & 0.36 & 0.37 & 0.09 \\
4099 & KOI-4345 & -0.10 & 0.02 & -0.01 & -0.09 & -0.07 & 0.06 & -0.05 & 0.04 & -0.00 & -0.01 & -0.05 & -0.16 & -0.08 & -0.12 & -0.12 \\
4100 & KOI-337 & 0.05 & 0.00 & 0.09 & -0.02 & 0.05 & 0.02 & 0.08 & 0.03 & 0.10 & 0.11 & 0.04 & -0.03 & 0.06 & 0.03 & -0.05 \\
4101 & KOI-263 B & -0.10 & -0.24 & -0.02 & -0.20 & -0.08 & -0.16 & -0.10 & -0.09 & -0.00 & -0.06 & -0.13 & -0.25 & -0.12 & -0.14 & -0.18 \\
4102 & KOI-340 & 0.20 & 0.49 & 0.32 & 0.40 & 0.19 & 0.27 & 0.22 & 0.33 & 0.27 & 0.24 & 0.29 & 0.35 & 0.33 & 0.31 & 0.25 \\
4103 & KOI-2300 & -0.12 & -0.30 & -0.05 & -0.24 & -0.14 & -0.23 & -0.12 & -0.14 & -0.12 & -0.13 & -0.17 & -0.22 & -0.15 & -0.21 & -0.14 \\
4104 & KOI-203 & 0.17 & 0.16 & 0.22 & 0.28 & 0.15 & 0.15 & 0.22 & 0.28 & 0.21 & 0.09 & 0.26 & 0.25 & 0.26 & 0.24 & 0.18 \\
4105 & KOI-4765 & 0.10 & -0.20 & 0.27 & 0.07 & 0.12 & -0.03 & 0.14 & 0.20 & 0.17 & 0.09 & 0.17 & 0.01 & 0.14 & 0.15 & 0.11 \\
4106 & KOI-1308 & -0.02 & -0.22 & 0.06 & -0.05 & 0.05 & 0.12 & 0.03 & 0.02 & 0.12 & 0.05 & -0.05 & -0.21 & -0.06 & -0.02 & -0.12 \\
4107 & KOI-275 & 0.16 & 0.39 & 0.30 & 0.33 & 0.17 & 0.20 & 0.19 & 0.21 & 0.20 & 0.14 & 0.20 & 0.31 & 0.23 & 0.25 & 0.15 \\
4108 & KOI-4892 & -0.37 & 0.15 & -0.06 & -0.27 & -0.38 & -0.46 & -0.31 & -0.31 & -0.28 & -0.35 & -0.44 & -0.68 & -0.37 & -0.45 & -0.27 \\
4109 & KOI-3032 & 0.41 & 0.57 & 0.61 & 0.48 & 0.28 & 0.40 & 0.28 & 0.29 & 0.30 & 0.35 & 0.29 & 0.39 & 0.34 & 0.37 & 0.13 \\
4110 & KOI-4204 & 0.13 & 0.15 & 0.08 & 0.21 & 0.15 & 0.13 & 0.14 & 0.17 & 0.13 & 0.14 & 0.16 & 0.19 & 0.17 & 0.18 & 0.12 \\
4111 & KOI-339 & -0.11 & -0.06 & -0.10 & -0.21 & -0.16 & -0.32 & -0.17 & -0.07 & -0.05 & -0.07 & -0.11 & -0.25 & -0.14 & -0.19 & -0.14 \\
4112 & KOI-749 & 0.07 & -0.02 & 0.16 & -0.02 & 0.01 & 0.07 & 0.01 & 0.05 & 0.01 & -0.03 & 0.09 & -0.07 & 0.02 & -0.03 & -0.09 \\
4113 & KOI-2149 & 0.11 & -0.25 & 0.24 & 0.22 & 0.14 & -0.01 & 0.21 & 0.24 & 0.27 & 0.24 & 0.25 & 0.26 & 0.25 & 0.20 & 0.16 \\
4114 & KOI-4833 & -0.07 & -0.66 & 0.02 & -0.26 & -0.02 & -0.03 & -0.07 & 0.04 & 0.05 & -0.03 & -0.03 & -0.27 & -0.01 & -0.06 & 0.00 \\
4115 & KOI-1837 & -0.02 & -0.18 & -0.01 & -0.02 & 0.02 & 0.10 & 0.05 & 0.12 & 0.09 & 0.07 & 0.11 & 0.10 & 0.11 & 0.05 & 0.10 \\
4116 & KOI-1797 & 0.10 & -0.04 & 0.07 & 0.12 & -0.00 & 0.12 & 0.18 & 0.20 & 0.09 & 0.09 & 0.16 & 0.15 & 0.16 & 0.11 & 0.10 \\
4117 & KOI-598 & -0.14 & -0.26 & -0.17 & -0.11 & -0.05 & 0.00 & -0.06 & 0.03 & -0.00 & -0.06 & 0.01 & -0.01 & 0.01 & -0.02 & 0.07 \\
4118 & KOI-2 & 0.01 & 0.29 & 0.35 & 0.02 & 0.10 & 0.13 & 0.19 & 0.35 & 0.28 & 0.07 & 0.24 & -0.11 & 0.24 & 0.13 & 0.51 \\
4119 & KOI-4366 & -0.15 & -0.01 & 0.02 & -0.13 & -0.15 & -0.13 & -0.21 & -0.11 & -0.15 & -0.16 & -0.13 & -0.33 & -0.16 & -0.22 & -0.29 \\
4120 & KOI-211 & -0.01 & -0.23 & 0.00 & -0.02 & -0.02 & -0.07 & -0.03 & -0.03 & 0.09 & 0.00 & 0.00 & -0.15 & -0.01 & -0.05 & -0.07 \\
4121 & KOI-2046 & 0.15 & 0.13 & 0.34 & 0.11 & 0.20 & 0.28 & 0.19 & 0.21 & 0.23 & 0.18 & 0.13 & 0.10 & 0.15 & 0.17 & 0.19 \\
4122 & KOI-4312 & -0.11 & -0.42 & 0.06 & -0.23 & -0.10 & 0.06 & -0.11 & -0.12 & 0.04 & -0.05 & -0.25 & -0.49 & -0.23 & -0.18 & -0.27 \\
4123 & KOI-4335 & -0.25 & -0.29 & -0.20 & -0.33 & -0.26 & -0.21 & -0.26 & -0.28 & -0.19 & -0.18 & -0.30 & -0.42 & -0.28 & -0.32 & -0.42 \\
4124 & KOI-4024 & 0.05 & -0.08 & 0.22 & -0.16 & -0.07 & -0.04 & -0.04 & -0.01 & -0.04 & -0.04 & -0.11 & -0.18 & -0.07 & -0.12 & -0.25 \\
4125 & KOI-209 & 0.01 & 0.06 & 0.15 & 0.10 & -0.00 & 0.00 & 0.03 & 0.09 & 0.15 & -0.16 & 0.08 & -0.04 & 0.07 & 0.01 & 0.02 \\
4126 & KOI-1305 & 0.00 & 0.01 & 0.01 & 0.06 & 0.08 & 0.09 & 0.10 & 0.09 & 0.12 & 0.12 & 0.15 & 0.07 & 0.12 & 0.07 & 0.04 \\
4127 & KOI-3 & 0.14 & 0.40 & 0.11 & 0.55 & 0.29 & 0.42 & 0.29 & 0.40 & 0.31 & 0.27 & 0.28 & 0.35 & 0.35 & 0.37 & 0.11 \\
4128 & KOI-3889 & 0.14 & 0.24 & 0.17 & 0.20 & 0.16 & 0.19 & 0.16 & 0.17 & 0.19 & 0.17 & 0.18 & 0.16 & 0.17 & 0.20 & 0.08 \\
4129 & KOI-1311 & 0.06 & 1.14 & 0.56 & 0.03 & 0.09 & 0.14 & -0.03 & -0.06 & 0.19 & 0.14 & 0.04 & 0.01 & 0.03 & 0.04 & 0.04 \\
4130 & KOI-1639 & 0.08 & 0.39 & 0.37 & 0.21 & 0.06 & -0.03 & 0.12 & 0.23 & 0.11 & -0.01 & 0.13 & 0.01 & 0.17 & 0.05 & 1.05 \\
4131 & KOI-2236 & -0.19 & -0.39 & -0.15 & -0.20 & -0.07 & -0.11 & -0.10 & -0.09 & -0.01 & -0.02 & -0.04 & -0.18 & -0.08 & -0.11 & -0.18 \\
4132 & KOI-1316 & 0.17 & 0.37 & 0.27 & 0.37 & 0.21 & 0.38 & 0.23 & 0.30 & 0.27 & 0.19 & 0.26 & 0.29 & 0.27 & 0.33 & 0.39 \\
4133 & KOI-1989 & -0.03 & -0.03 & -0.04 & -0.04 & -0.02 & -0.02 & 0.01 & 0.04 & -0.02 & -0.07 & -0.03 & -0.02 & -0.00 & -0.02 & 0.05 \\
4134 & KOI-752 & -0.00 & -0.02 & 0.08 & -0.04 & 0.03 & 0.01 & -0.01 & 0.04 & 0.04 & 0.02 & 0.06 & 0.04 & 0.03 & 0.01 & 0.09 \\
4135 & KOI-3451 & -0.03 & -0.22 & 0.04 & -0.16 & -0.03 & -0.18 & -0.01 & 0.06 & 0.03 & 0.03 & 0.02 & -0.12 & 0.01 & -0.04 & 0.07 \\
4136 & KOI-3925 & -0.10 & -0.47 & -0.12 & -0.07 & -0.04 & -0.05 & -0.02 & 0.01 & 0.02 & -0.05 & 0.01 & -0.05 & 0.01 & -0.05 & 0.13 \\
4137 & KOI-3683 & -0.15 & 0.24 & 0.17 & -0.05 & -0.04 & 0.01 & 0.02 & 0.04 & 0.05 & 0.05 & 0.01 & -0.20 & 0.04 & -0.08 & 0.00 \\
4138 & KOI-4235 & -0.05 & 0.49 & 0.33 & 0.02 & 0.01 & -0.25 & 0.13 & 0.15 & 0.09 & 0.08 & 0.09 & -0.13 & 0.10 & 0.01 & 0.06 \\
4139 & KOI-2228 & -0.61 & 0.01 & 0.41 & -0.08 & -0.08 & -2.36 & -0.04 & 0.06 & 0.15 & -0.19 & -0.04 & -0.39 & -0.01 & -0.29 & 0.22 \\
4140 & KOI-117 & 0.22 & 0.37 & 0.20 & 0.37 & 0.24 & 0.32 & 0.24 & 0.27 & 0.24 & 0.15 & 0.26 & 0.33 & 0.27 & 0.34 & 0.32 \\
4141 & Kepler-107 & 0.20 & 0.50 & 0.26 & 0.42 & 0.22 & 0.28 & 0.29 & 0.28 & 0.25 & 0.21 & 0.26 & 0.36 & 0.27 & 0.34 & 0.23 \\
4142 & KOI-3602 & -0.13 & -0.23 & -0.27 & -0.20 & -0.04 & -0.07 & -0.06 & -0.25 & 0.01 & 0.12 & -0.17 & -0.30 & -0.20 & -0.20 & -0.52 \\
4143 & KOI-756 & 0.08 & -0.24 & 0.09 & 0.01 & 0.07 & 0.12 & 0.12 & 0.15 & 0.15 & 0.07 & 0.17 & -0.04 & 0.12 & 0.07 & 0.09 \\
4144 & KOI-2960 & 0.08 & -0.13 & 0.11 & 0.08 & 0.06 & 0.05 & 0.06 & 0.08 & 0.08 & 0.14 & 0.09 & 0.10 & 0.09 & 0.09 & 0.09 \\
4145 & KOI-341 & 0.06 & 0.00 & 0.08 & 0.06 & 0.03 & 0.09 & 0.10 & 0.11 & 0.09 & 0.13 & 0.12 & 0.08 & 0.12 & 0.05 & 0.14 \\
4146 & KOI-2075 & 0.01 & 0.16 & 0.04 & -0.04 & -0.05 & -0.08 & -0.03 & 0.04 & 0.06 & -0.19 & 0.03 & -0.18 & 0.00 & -0.09 & -0.03 \\
4147 & KOI-431 & -0.25 & -0.51 & -0.15 & -0.44 & -0.24 & -0.25 & -0.25 & -0.29 & -0.24 & -0.29 & -0.31 & -0.47 & -0.33 & -0.28 & -0.14 \\
4148 & KOI-1299 & -0.16 & 0.13 & -0.09 & -0.03 & 0.00 & 0.05 & -0.12 & 0.03 & 0.04 & -0.02 & 0.05 & 0.15 & 0.09 & 0.06 & 0.15 \\
4149 & KOI-1306 & -0.24 & -2.31 & -0.21 & -0.27 & -0.26 & -0.44 & -0.27 & -0.24 & -0.23 & -0.37 & -0.35 & -0.31 & -0.31 & -0.33 & -0.04 \\
4150 & KOI-3146 & 0.12 & 0.12 & 0.19 & 0.15 & 0.11 & 0.13 & 0.11 & 0.18 & 0.12 & 0.10 & 0.15 & 0.16 & 0.16 & 0.15 & 0.08 \\
4151 & KOI-291 & 0.20 & 0.21 & 0.26 & 0.25 & 0.21 & 0.24 & 0.21 & 0.25 & 0.25 & 0.22 & 0.23 & 0.27 & 0.24 & 0.24 & 0.27 \\
4152 & KOI-2623 & 0.02 & -0.81 & 0.30 & 0.15 & 0.09 & 0.05 & 0.09 & 0.20 & 0.21 & 0.07 & 0.19 & 0.08 & 0.18 & 0.12 & 0.35 \\
4153 & KOI-46 & 0.19 & 0.27 & 0.20 & 0.21 & 0.28 & 0.35 & 0.28 & 0.32 & 0.32 & 0.28 & 0.29 & 0.29 & 0.34 & 0.36 & 0.27 \\
4154 & KOI-1963 & 0.30 & 0.41 & 0.10 & 0.02 & 0.15 & 0.02 & 0.12 & 0.21 & 0.44 & 0.04 & 0.15 & 0.46 & 0.19 & 0.29 & 0.32 \\
4155 & KOI-2754 & -0.09 & -0.08 & 0.01 & -0.11 & -0.14 & -0.13 & -0.12 & -0.03 & -0.07 & 0.11 & -0.13 & -0.23 & -0.13 & -0.18 & -0.15 \\
4156 & KOI-757 & 0.32 & -0.44 & 0.48 & -0.03 & -0.04 & -0.07 & 0.01 & 0.06 & 0.09 & -0.01 & 0.11 & 0.04 & 0.04 & -0.03 & 0.38 \\
4157 & KOI-601 & -0.04 & -0.67 & 0.10 & -0.17 & 0.04 & -0.18 & 0.03 & 0.02 & 0.14 & 0.13 & 0.06 & -0.06 & 0.05 & -0.01 & 0.29 \\
4158 & KOI-1307 & -0.00 & 0.00 & 0.17 & 0.04 & -0.00 & 0.04 & 0.06 & 0.03 & 0.08 & 0.05 & 0.05 & -0.05 & 0.06 & 0.04 & 0.05 \\
4159 & KOI-4374 & -0.04 & -0.12 & 0.05 & -0.06 & -0.02 & -0.00 & 0.02 & 0.02 & 0.05 & 0.04 & -0.02 & -0.06 & -0.02 & -0.03 & -0.09 \\
4160 & KOI-1931 & -0.17 & -0.19 & -0.05 & -0.21 & -0.12 & -0.23 & -0.07 & -0.07 & -0.07 & -0.10 & -0.03 & -0.19 & -0.06 & -0.15 & -0.02 \\
4161 & KOI-343 & -0.01 & -0.15 & -0.09 & -0.00 & 0.01 & 0.07 & -0.02 & 0.01 & 0.04 & 0.08 & 0.02 & -0.02 & 0.03 & 0.02 & -0.02 \\
4162 & Kepler-142 & -0.05 & -0.05 & 0.04 & 0.01 & 0.02 & -0.01 & -0.04 & 0.06 & -0.02 & -0.04 & -0.03 & -0.05 & -0.05 & -0.02 & -0.15 \\
4163 & KOI-112 & -0.03 & -0.07 & 0.00 & -0.01 & -0.05 & 0.06 & -0.10 & 0.03 & 0.09 & 0.16 & 0.03 & -0.07 & -0.03 & -0.09 & 0.04 \\
4164 & KOI-759 & -0.25 & -0.49 & -0.11 & -0.30 & -0.24 & -0.27 & -0.22 & -0.24 & -0.23 & -0.25 & -0.26 & -0.40 & -0.28 & -0.30 & -0.33 \\
4165 & KOI-3060 & -0.06 & 0.55 & 0.16 & -0.13 & -0.07 & -0.06 & -0.03 & 0.04 & 0.14 & 0.02 & 0.04 & -0.14 & 0.01 & -0.08 & 0.09 \\
4166 & KOI-344 & -0.23 & -0.46 & -0.06 & -0.31 & -0.25 & -0.26 & -0.22 & -0.23 & -0.26 & -0.25 & -0.26 & -0.40 & -0.27 & -0.31 & -0.19 \\
4167 & KOI-479 & -0.15 & -0.20 & -0.11 & -0.21 & -0.15 & -0.05 & -0.17 & -0.15 & -0.09 & -0.13 & -0.34 & -0.23 & -0.16 & -0.17 & -0.19 \\
4168 & KOI-1645 & -0.39 & -0.60 & -0.17 & -0.43 & -0.12 & -0.12 & 0.16 & -0.36 & 0.06 & -0.02 & -0.32 & -0.43 & -0.29 & -0.14 & -0.31 \\
4169 & KOI-1800 & -0.12 & 0.02 & -0.08 & -0.15 & -0.09 & -0.17 & -0.03 & 0.08 & -0.01 & -0.03 & 0.01 & -0.10 & 0.03 & -0.12 & 0.10 \\
4170 & KOI-1444 & -0.00 & -0.81 & 0.40 & 0.08 & 0.06 & -0.05 & 0.03 & 0.18 & 0.20 & 0.06 & 0.15 & -0.12 & 0.14 & -0.01 & 0.26 \\
4171 & Kepler-299 & 0.02 & 0.15 & 0.07 & 0.05 & 0.04 & 0.05 & 0.06 & 0.05 & 0.07 & 0.14 & 0.01 & 0.01 & 0.02 & 0.01 & -0.05 \\
4172 & KOI-124 & -0.11 & -0.02 & -0.04 & -0.17 & -0.09 & -0.21 & -0.11 & -0.09 & -0.03 & -0.06 & -0.11 & -0.27 & -0.09 & -0.11 & -0.19 \\
4173 & KOI-1889 & 0.00 & -0.44 & 0.08 & -0.13 & -0.13 & -0.11 & -0.05 & 0.00 & 0.01 & -0.11 & -0.01 & -0.08 & -0.05 & -0.12 & 0.27 \\
4174 & KOI-2007 & 0.11 & 0.03 & 0.13 & 0.06 & 0.06 & 0.11 & 0.10 & 0.09 & 0.09 & 0.04 & 0.12 & 0.14 & 0.13 & 0.10 & 0.17 \\
4175 & KOI-2977 & -0.06 & 0.24 & 0.01 & -0.12 & -0.11 & -0.07 & -0.09 & -0.01 & -0.05 & -0.21 & -0.10 & -0.19 & -0.08 & -0.08 & -0.17 \\
4176 & KOI-2885 & -0.37 & -0.14 & -0.25 & -0.46 & -0.38 & -0.33 & -0.35 & -0.37 & -0.26 & -0.32 & -0.42 & -0.65 & -0.38 & -0.44 & -0.40 \\
4177 & KOI-2533 & -0.11 & -0.05 & 0.01 & -0.07 & -0.01 & 0.02 & -0.12 & 0.01 & 0.03 & -0.06 & 0.01 & 0.03 & 0.03 & 0.01 & -0.03 \\
4178 & KOI-4287 & -0.10 & 0.38 & 0.19 & -0.09 & -0.04 & -0.34 & 0.00 & 0.03 & 0.06 & 0.04 & 0.00 & -0.18 & 0.05 & -0.05 & -0.05 \\
4179 & KOI-2442 & -0.03 & -0.04 & -0.09 & 0.04 & 0.01 & 0.00 & 0.06 & 0.02 & 0.02 & 0.07 & 0.05 & -0.00 & 0.03 & 0.06 & 0.12 \\
4180 & KOI-2712 & 0.05 & 0.26 & 0.43 & 0.26 & 0.16 & 0.20 & 0.29 & 0.32 & 0.24 & 0.10 & 0.24 & 0.29 & 0.29 & 0.26 & 0.17 \\
4181 & KOI-2805 & -0.19 & -0.12 & -0.11 & -0.31 & -0.23 & -0.22 & -0.25 & -0.20 & -0.17 & -0.27 & -0.25 & -0.37 & -0.24 & -0.28 & -0.33 \\
4182 & KOI-276 & -0.04 & 0.03 & 0.04 & -0.09 & -0.05 & -0.15 & -0.05 & -0.02 & -0.03 & 0.00 & -0.04 & -0.04 & -0.02 & -0.05 & -0.04 \\
4183 & KOI-1863 & 0.51 & -0.40 & 0.83 & -0.16 & 0.30 & -0.08 & 0.39 & -0.28 & -0.09 & -0.07 & -0.17 & -0.24 & -0.02 & 0.21 & 0.07 \\
4184 & KOI-3371 & -0.17 & -0.05 & -0.02 & -0.15 & -0.18 & -0.02 & -0.08 & 0.08 & -0.05 & 0.01 & -0.05 & -0.18 & -0.07 & -0.19 & 0.03 \\
4185 & KOI-2792 & 0.10 & 0.23 & 0.11 & 0.13 & 0.15 & 0.18 & 0.14 & 0.16 & 0.15 & 0.11 & 0.17 & 0.15 & 0.18 & 0.19 & 0.22 \\
4186 & KOI-2333 & -0.04 & 0.09 & -0.02 & -0.14 & -0.12 & -0.30 & -0.07 & -0.08 & -0.04 & 0.00 & -0.13 & -0.27 & -0.12 & -0.17 & -0.13 \\
4187 & KOI-1647 & 0.17 & 0.15 & 0.20 & 0.25 & 0.19 & 0.13 & 0.17 & 0.21 & 0.21 & 0.20 & 0.21 & 0.30 & 0.23 & 0.23 & 0.12 \\
4188 & KOI-1426 & -0.10 & -0.47 & -0.17 & -0.30 & -0.16 & -0.20 & -0.15 & -0.16 & -0.16 & -0.17 & -0.18 & -0.25 & -0.19 & -0.24 & -0.07 \\
4189 & KOI-1438 & 0.03 & -0.04 & 0.08 & 0.01 & 0.06 & 0.09 & 0.08 & 0.11 & 0.11 & 0.03 & 0.14 & 0.11 & 0.15 & 0.15 & 0.18 \\
4190 & KOI-2813 & -0.51 & -0.20 & -0.40 & -0.34 & -0.39 & 0.20 & 0.04 & -0.30 & -0.28 & -0.27 & -0.46 & -0.24 & -0.33 & -0.33 & -0.51 \\
4191 & KOI-481 & -0.04 & -0.17 & 0.09 & -0.15 & -0.11 & -0.15 & -0.18 & -0.12 & -0.08 & -0.12 & -0.10 & -0.19 & -0.13 & -0.16 & -0.14 \\
4192 & KOI-2765 & -0.03 & 0.20 & 0.25 & 0.03 & 0.06 & 0.00 & 0.09 & 0.16 & 0.16 & 0.11 & 0.11 & -0.07 & 0.14 & 0.05 & 0.16 \\
4193 & KOI-4653 & -0.05 & -0.07 & 0.11 & 0.01 & -0.01 & -0.11 & 0.02 & 0.07 & 0.03 & -0.14 & 0.05 & -0.08 & 0.05 & -0.03 & 0.11 \\
4194 & KOI-294 & 0.01 & -0.03 & 0.08 & 0.05 & 0.08 & 0.01 & 0.07 & 0.10 & 0.11 & 0.14 & 0.10 & 0.07 & 0.09 & 0.05 & 0.14 \\
4195 & KOI-2796 & -0.05 & 0.11 & -0.11 & -0.14 & -0.03 & -0.03 & -0.08 & -0.04 & 0.05 & -0.08 & -0.06 & -0.05 & -0.04 & -0.03 & -0.09 \\
4196 & KOI-3103 & 0.20 & 0.26 & 0.25 & 0.36 & 0.23 & 0.21 & 0.27 & 0.31 & 0.24 & 0.22 & 0.25 & 0.38 & 0.25 & 0.29 & 0.24 \\
4197 & KOI-2672 & 0.04 & 0.01 & 0.08 & 0.03 & 0.03 & -0.00 & 0.06 & 0.11 & 0.05 & 0.04 & 0.10 & 0.07 & 0.09 & 0.06 & 0.12 \\
4198 & KOI-107 & 0.17 & 0.14 & 0.37 & 0.30 & 0.16 & 0.29 & 0.23 & 0.25 & 0.21 & 0.20 & 0.24 & 0.23 & 0.24 & 0.26 & 0.29 \\
4199 & KOI-3346 & -0.05 & 0.02 & 0.02 & -0.11 & -0.04 & -0.11 & -0.02 & -0.02 & 0.01 & -0.06 & -0.02 & -0.15 & -0.02 & -0.05 & -0.03 \\
4200 & KOI-1857 & -0.04 & 0.03 & -0.04 & -0.11 & -0.12 & -0.08 & -0.09 & 0.03 & 0.00 & 0.19 & -0.05 & -0.13 & -0.07 & -0.17 & -0.09 \\
4201 & KOI-4716 & 0.04 & 0.12 & 0.17 & 0.00 & -0.03 & -0.07 & 0.02 & 0.05 & 0.05 & 0.09 & 0.03 & 0.03 & 0.05 & -0.01 & 0.06 \\
4202 & KOI-246 & 0.10 & 0.03 & 0.03 & 0.10 & 0.15 & 0.17 & 0.10 & 0.18 & 0.19 & 0.11 & 0.13 & 0.14 & 0.13 & 0.16 & 0.15 \\
4203 & KOI-1802 & 0.03 & -0.02 & 0.01 & -0.05 & -0.03 & -0.01 & 0.02 & 0.04 & -0.02 & -0.15 & 0.06 & 0.00 & 0.01 & -0.05 & 0.16 \\
4204 & KOI-241 & -0.02 & -0.44 & 0.21 & -0.41 & -0.24 & -0.29 & -0.22 & -0.34 & -0.23 & -0.27 & -0.53 & -0.70 & -0.48 & -0.37 & -0.95 \\
4205 & Kepler-124 & -0.16 & -1.42 & 0.01 & -0.45 & -0.28 & -0.21 & -0.29 & -0.35 & -0.26 & -0.30 & -0.59 & -0.68 & -0.52 & -0.40 & -0.92 \\
4206 & KOI-2168 & -0.05 & -0.14 & -0.10 & -0.14 & -0.11 & -0.17 & -0.18 & -0.03 & -0.13 & -0.25 & -0.06 & -0.28 & -0.10 & -0.14 & 0.15 \\
4207 & KOI-2422 & -0.14 & -0.21 & -0.11 & -0.09 & -0.06 & -0.11 & -0.04 & -0.06 & -0.01 & -0.03 & -0.09 & -0.19 & -0.06 & -0.08 & -0.02 \\
4208 & KOI-2632 & -0.15 & -0.20 & 0.22 & -0.10 & -0.08 & -0.32 & -0.12 & 0.05 & 0.06 & -0.29 & 0.02 & -0.25 & 0.00 & -0.13 & 0.14 \\
4209 & Kepler-15 & 0.19 & 0.25 & 0.18 & 0.15 & 0.19 & 0.21 & 0.22 & 0.21 & 0.23 & 0.16 & 0.19 & 0.21 & 0.21 & 0.20 & 0.18 \\
4210 & KOI-128 & 0.19 & 0.25 & 0.31 & 0.18 & 0.19 & 0.21 & 0.20 & 0.24 & 0.20 & 0.17 & 0.21 & 0.23 & 0.21 & 0.21 & 0.19 \\
4211 & KOI-2366 & -0.04 & 0.15 & 0.09 & 0.05 & 0.01 & 0.02 & 0.00 & 0.09 & 0.05 & -0.05 & 0.05 & -0.13 & 0.05 & -0.02 & 0.01 \\
4212 & KOI-330 & -0.07 & 0.25 & 0.12 & -0.09 & -0.03 & 0.01 & -0.01 & -0.02 & 0.06 & 0.01 & -0.01 & -0.03 & 0.01 & -0.03 & -0.05 \\
4213 & KOI-3782 & 0.12 & -0.01 & 0.08 & 0.25 & 0.05 & 0.13 & 0.07 & 0.21 & 0.06 & 0.08 & 0.07 & 0.14 & 0.09 & 0.09 & -0.01 \\
4214 & KOI-2639 & -0.04 & -0.38 & 0.05 & -0.15 & 0.07 & 0.25 & 0.06 & 0.02 & 0.21 & 0.13 & -0.01 & -0.24 & 0.02 & -0.00 & 0.06 \\
4215 & KOI-3015 & -0.09 & -0.26 & 0.08 & -0.23 & -0.06 & -0.07 & -0.04 & 0.02 & -0.01 & -0.03 & -0.06 & -0.26 & -0.06 & -0.15 & -0.11 \\
4216 & KOI-1428 & -0.34 & -0.23 & -0.33 & -0.13 & -0.16 & -0.13 & -0.15 & -0.15 & -0.11 & -0.10 & -0.21 & -0.17 & -0.16 & -0.18 & -0.28 \\
4217 & KOI-4036 & -0.13 & -0.50 & -0.21 & -0.04 & -0.06 & -0.05 & 0.02 & 0.05 & 0.00 & -0.00 & 0.00 & -0.02 & 0.01 & -0.01 & -0.08 \\
4218 & KOI-1436 & 0.10 & 0.10 & 0.27 & 0.08 & 0.09 & 0.04 & 0.10 & 0.11 & 0.13 & 0.14 & 0.13 & 0.12 & 0.13 & 0.13 & 0.14 \\
4219 & Kepler-301 & 0.07 & -0.08 & 0.10 & 0.06 & 0.04 & 0.03 & 0.09 & 0.06 & 0.11 & 0.07 & 0.11 & 0.09 & 0.09 & 0.09 & 0.16 \\
4220 & KOI-2143 & 0.05 & 0.08 & -0.09 & 0.16 & 0.10 & 0.18 & 0.08 & 0.18 & 0.15 & 0.18 & 0.20 & 0.20 & 0.11 & 0.13 & 0.02 \\
4221 & KOI-2195 & -0.02 & 0.55 & -0.16 & -0.43 & -0.14 & -0.68 & -0.17 & -0.22 & -0.04 & -0.03 & -0.09 & -0.34 & -0.11 & -0.20 & -0.23 \\
4222 & KOI-349 & 0.24 & 0.39 & 0.21 & 0.38 & 0.22 & 0.30 & 0.28 & 0.27 & 0.18 & 0.22 & 0.26 & 0.42 & 0.27 & 0.30 & 0.14 \\
4223 & KOI-350 & 0.02 & -0.17 & 0.05 & 0.02 & 0.02 & -0.01 & 0.01 & 0.06 & 0.03 & 0.07 & 0.05 & 0.02 & 0.04 & -0.03 & 0.09 \\
4224 & KOI-1623 & 0.04 & 0.04 & 0.14 & -0.01 & 0.06 & 0.05 & 0.03 & 0.05 & 0.12 & -0.01 & -0.01 & -0.13 & -0.01 & -0.01 & -0.01 \\
4225 & KOI-351 & 0.07 & 0.18 & 0.15 & 0.10 & 0.10 & 0.08 & 0.13 & 0.15 & 0.14 & 0.10 & 0.14 & 0.13 & 0.14 & 0.12 & 0.13 \\
4226 & KOI-1992 & -0.12 & 0.07 & -0.04 & -0.12 & -0.08 & 0.00 & -0.08 & -0.16 & -0.01 & -0.44 & -0.14 & -0.29 & -0.12 & -0.16 & -0.19 \\
4227 & KOI-2047 & -0.05 & -0.13 & 0.16 & -0.03 & -0.04 & -0.13 & 0.00 & -0.03 & -0.03 & 0.08 & 0.01 & -0.24 & -0.04 & -0.10 & -0.01 \\
4228 & KOI-2771 & 0.05 & 0.33 & 0.09 & -0.05 & -0.05 & -0.24 & -0.03 & 0.04 & -0.01 & -0.02 & 0.04 & -0.09 & 0.02 & -0.09 & 0.10 \\
4229 & KOI-2110 & -0.19 & 0.41 & 0.49 & -0.01 & 0.04 & 0.05 & 0.18 & 0.23 & 0.11 & 0.01 & 0.12 & -0.10 & 0.19 & 0.11 & 0.10 \\
4230 & KOI-5900 & -0.05 & 0.24 & 0.11 & -0.12 & -0.13 & -0.72 & -0.07 & -0.04 & -0.01 & -0.30 & -0.04 & -0.29 & -0.06 & -0.18 & -0.14 \\
4231 & KOI-2399 & -0.18 & -0.23 & -0.16 & -0.14 & -0.10 & -0.12 & -0.20 & -0.02 & -0.11 & -0.11 & -0.10 & -0.17 & -0.17 & -0.16 & 0.02 \\
4232 & KOI-352 & -0.04 & -0.25 & -0.01 & -0.11 & -0.05 & -0.05 & -0.03 & -0.04 & -0.01 & -0.00 & -0.28 & -0.31 & -0.03 & -0.07 & -0.10 \\
4233 & KOI-2109 & -0.07 & -0.07 & 0.14 & 0.08 & -0.03 & -0.19 & 0.05 & 0.09 & 0.10 & -0.10 & 0.05 & -0.15 & 0.07 & 0.00 & 0.08 \\
4234 & KOI-3419 & -0.50 & -0.17 & -0.32 & -0.31 & -0.15 & -0.41 & -0.18 & -0.30 & 0.08 & -0.38 & -0.42 & -0.28 & -0.30 & 0.03 & 0.11 \\
4235 & KOI-168 & -0.09 & -0.18 & 0.04 & -0.14 & -0.12 & -0.13 & -0.14 & -0.07 & -0.08 & -0.16 & -0.12 & -0.25 & -0.11 & -0.14 & -0.17 \\
4236 & KOI-1856 & -0.10 & -0.13 & -0.08 & -0.08 & -0.05 & -0.06 & -0.06 & 0.01 & -0.03 & -0.04 & -0.03 & -0.15 & -0.04 & -0.07 & -0.02 \\
4237 & KOI-1655 & -0.16 & -0.20 & -0.12 & -0.17 & -0.10 & -0.12 & -0.16 & -0.13 & -0.15 & -0.19 & -0.18 & -0.24 & -0.17 & -0.19 & -0.13 \\
4238 & KOI-354 & -0.04 & 0.01 & -0.03 & -0.10 & 0.05 & 0.01 & -0.00 & 0.09 & 0.07 & -0.06 & 0.04 & -0.09 & 0.05 & 0.01 & 0.13 \\
4239 & KOI-2365 & 0.15 & 0.31 & 0.22 & 0.24 & 0.16 & 0.21 & 0.20 & 0.24 & 0.17 & 0.14 & 0.18 & 0.28 & 0.21 & 0.22 & 0.19 \\
4240 & KOI-2837 & -0.44 & 0.09 & 0.18 & -0.17 & -0.08 & 0.11 & 0.02 & 0.10 & -0.04 & -0.37 & -0.01 & -0.31 & -0.03 & -0.19 & 0.06 \\
4241 & KOI-3109 & -0.16 & 0.57 & 0.39 & 0.04 & 0.01 & -0.18 & 0.10 & 0.10 & 0.06 & -0.63 & 0.09 & -0.13 & 0.13 & -0.07 & 0.34 \\
4242 & KOI-295 & -0.12 & -0.02 & -0.02 & -0.29 & -0.16 & -0.24 & -0.18 & -0.16 & -0.13 & -0.13 & -0.17 & -0.32 & -0.16 & -0.25 & -0.12 \\
4243 & KOI-4792 & 0.07 & 0.25 & 0.14 & 0.04 & 0.07 & 0.00 & 0.08 & 0.11 & 0.04 & 0.02 & 0.06 & 0.02 & 0.08 & 0.05 & 0.14 \\
4244 & KOI-356 & -0.10 & -0.22 & -0.08 & -0.08 & -0.04 & -0.06 & -0.04 & -0.04 & -0.01 & 0.02 & -0.05 & -0.12 & -0.05 & -0.08 & -0.02 \\
4245 & KOI-1831 & 0.09 & 0.07 & 0.07 & 0.09 & 0.11 & 0.18 & 0.10 & 0.04 & 0.10 & 0.12 & 0.12 & 0.11 & 0.13 & 0.13 & -0.00 \\
4246 & KOI-4304 & 0.12 & 0.13 & 0.15 & 0.15 & 0.13 & 0.10 & 0.07 & 0.17 & 0.14 & 0.11 & 0.15 & 0.10 & 0.13 & 0.14 & 0.10 \\
4247 & KOI-355 & 0.09 & 0.12 & 0.17 & 0.18 & 0.15 & 0.16 & 0.19 & 0.26 & 0.15 & 0.12 & 0.21 & 0.11 & 0.21 & 0.19 & 0.17 \\
4248 & KOI-3363 & -0.04 & -0.07 & 0.04 & -0.09 & 0.01 & 0.03 & -0.01 & -0.03 & 0.09 & 0.06 & -0.06 & -0.19 & -0.05 & -0.06 & -0.14 \\
4249 & KOI-167 & 0.08 & 0.18 & 0.16 & 0.05 & 0.05 & -0.06 & 0.05 & 0.14 & 0.15 & 0.12 & 0.10 & -0.03 & 0.12 & 0.04 & 0.14 \\
4250 & KOI-1945 & 0.06 & 0.26 & 0.09 & 0.23 & 0.16 & 0.19 & 0.11 & 0.16 & 0.17 & 0.16 & 0.16 & 0.16 & 0.16 & 0.16 & -0.18 \\
4251 & KOI-1894 & -0.10 & 0.17 & -0.12 & 0.15 & 0.08 & 0.10 & -0.04 & 0.12 & 0.12 & 0.08 & 0.17 & 0.25 & 0.17 & 0.17 & 0.16 \\
4252 & KOI-1832 & -0.06 & -0.50 & -0.02 & -0.16 & -0.04 & -0.15 & -0.08 & -0.09 & -0.02 & -0.10 & -0.08 & -0.22 & -0.10 & -0.11 & 0.00 \\
4253 & KOI-1841 & -0.08 & -0.20 & -0.07 & -0.11 & -0.02 & 0.02 & -0.01 & 0.04 & 0.04 & -0.03 & -0.00 & -0.06 & 0.00 & -0.02 & 0.01 \\
4254 & KOI-2582 & 0.22 & 0.31 & 0.24 & 0.41 & 0.28 & 0.34 & 0.29 & 0.26 & 0.29 & 0.22 & 0.27 & 0.37 & 0.28 & 0.36 & 0.26 \\
4255 & KOI-620 & -0.07 & -0.35 & 0.01 & -0.32 & -0.14 & -0.27 & -0.09 & -0.08 & -0.07 & -0.10 & -0.12 & -0.20 & -0.07 & -0.18 & -0.04 \\
4256 & KOI-3403 & 0.00 & 0.08 & 0.12 & 0.10 & 0.06 & 0.01 & 0.06 & 0.12 & 0.12 & 0.01 & 0.09 & 0.05 & 0.10 & 0.08 & 0.13 \\
4257 & KOI-1883 & 0.04 & 0.27 & -0.02 & 0.04 & 0.02 & 0.03 & 0.05 & 0.04 & 0.06 & 0.08 & 0.09 & -0.02 & 0.10 & 0.04 & 0.18 \\
4258 & KOI-3892 & 0.19 & 0.50 & 0.16 & 0.31 & 0.19 & 0.18 & 0.24 & 0.21 & 0.23 & 0.34 & 0.17 & 0.30 & 0.22 & 0.22 & 0.10 \\
4259 & KOI-1980 & 0.03 & -0.04 & -0.01 & 0.08 & 0.05 & 0.11 & 0.06 & 0.12 & 0.11 & 0.14 & 0.13 & 0.11 & 0.13 & 0.08 & 0.06 \\
4260 & KOI-2173 & 0.01 & -0.24 & -0.11 & 0.12 & 0.04 & 0.09 & 0.17 & 0.17 & 0.10 & 0.09 & 0.07 & 0.17 & 0.15 & 0.09 & 0.14 \\
4261 & KOI-2492 & -0.21 & -0.44 & 0.02 & -0.37 & -0.21 & -0.07 & -0.17 & -0.24 & -0.03 & -0.16 & -0.39 & -0.62 & -0.38 & -0.32 & -0.25 \\
4262 & KOI-2260 & -0.07 & -0.05 & 0.21 & 0.01 & -0.05 & -0.05 & -0.00 & 0.09 & 0.00 & -0.26 & 0.04 & -0.17 & 0.02 & -0.05 & 0.18 \\
4263 & KOI-296 & -0.11 & -0.32 & 0.01 & -0.17 & -0.13 & -0.06 & -0.15 & -0.13 & -0.08 & -0.26 & -0.18 & -0.27 & -0.16 & -0.18 & -0.33 \\
4264 & KOI-2581 & 0.14 & 0.28 & 0.13 & 0.23 & 0.16 & 0.18 & 0.19 & 0.19 & 0.20 & 0.19 & 0.21 & 0.22 & 0.20 & 0.21 & 0.17 \\
4265 & KOI-543 & -0.05 & -0.27 & 0.01 & -0.14 & -0.04 & -0.05 & -0.19 & -0.02 & -0.06 & -0.03 & -0.10 & -0.16 & -0.12 & -0.12 & -0.28 \\
4266 & KOI-4062 & 0.03 & 0.02 & 0.14 & -0.02 & -0.00 & 0.03 & 0.01 & 0.04 & 0.05 & -0.07 & 0.06 & -0.07 & 0.04 & -0.02 & 0.06 \\
4267 & KOI-3875 & -0.58 & -1.59 & -0.59 & -0.51 & -0.58 & -0.49 & -0.33 & -0.69 & -0.74 & -1.83 & -0.64 & -0.54 & -0.61 & -0.58 & -0.78 \\
4268 & KOI-72 & -0.15 & -0.32 & 0.02 & -0.18 & -0.11 & 0.03 & -0.12 & -0.10 & -0.08 & -0.12 & -0.18 & -0.38 & -0.19 & -0.20 & -0.20 \\
4269 & KOI-297 & 0.06 & 0.36 & 0.26 & 0.11 & 0.10 & -0.07 & 0.16 & 0.24 & 0.24 & 0.24 & 0.18 & 0.03 & 0.16 & 0.13 & 0.21 \\
4270 & KOI-2026 & -0.06 & 0.19 & -0.07 & -0.15 & -0.09 & -0.06 & -0.06 & 0.01 & 0.00 & 0.00 & -0.06 & -0.24 & -0.06 & -0.17 & 0.08 \\
4271 & KOI-2433 & -0.04 & 0.38 & 0.10 & 0.12 & -0.02 & -0.15 & -0.01 & 0.07 & -0.02 & -0.03 & -0.03 & -0.00 & 0.01 & -0.07 & -0.11 \\
4272 & KOI-4011 & 0.12 & 0.02 & 0.05 & 0.20 & 0.13 & 0.25 & 0.17 & 0.18 & 0.21 & 0.16 & 0.20 & 0.20 & 0.18 & 0.21 & 0.26 \\
4273 & KOI-4129 & 0.09 & 0.07 & 0.10 & 0.13 & 0.12 & 0.16 & 0.08 & 0.14 & 0.13 & 0.16 & 0.10 & 0.12 & 0.14 & 0.13 & 0.08 \\
4274 & KOI-4021 & -0.11 & 0.13 & 0.34 & 0.16 & -0.01 & -0.21 & 0.12 & 0.18 & 0.08 & -0.17 & 0.08 & -0.05 & 0.05 & -0.03 & 0.02 \\
4275 & KOI-2590 & -0.00 & -0.73 & 0.26 & -0.11 & -0.06 & -0.22 & -0.02 & 0.04 & 0.01 & -0.34 & 0.04 & -0.19 & 0.06 & -0.09 & 0.29 \\
4276 & KOI-2729 & -0.24 & -0.48 & 0.01 & -0.36 & -0.18 & -0.10 & -0.15 & -0.26 & -0.04 & -0.04 & -0.34 & -0.52 & -0.32 & -0.27 & -0.31 \\
4277 & KOI-3194 & 0.08 & 0.42 & 0.51 & 0.29 & 0.16 & 0.11 & 0.23 & 0.24 & 0.25 & 0.16 & 0.24 & 0.20 & 0.25 & 0.20 & 0.25 \\
4278 & Kepler-197 & -0.28 & 0.03 & -0.19 & -0.40 & -0.36 & -0.48 & -0.32 & -0.35 & -0.24 & -0.16 & -0.40 & -0.64 & -0.39 & -0.45 & -0.50 \\
4279 & KOI-623 & -0.24 & 0.16 & -0.20 & -0.40 & -0.34 & -0.50 & -0.27 & -0.33 & -0.23 & -0.24 & -0.41 & -0.57 & -0.38 & -0.45 & -0.47 \\
4280 & KOI-3017 & -0.24 & -0.18 & -0.25 & -0.34 & -0.19 & -0.23 & -0.21 & -0.20 & -0.19 & -0.25 & -0.24 & -0.34 & -0.23 & -0.29 & -0.16 \\
4281 & KOI-546 & 0.12 & 0.07 & 0.06 & 0.11 & 0.12 & 0.22 & -0.04 & 0.09 & 0.18 & 0.13 & 0.15 & 0.13 & 0.11 & 0.12 & 0.14 \\
4282 & KOI-2072 & -0.11 & -0.26 & 0.07 & -0.20 & -0.11 & -0.16 & -0.11 & -0.09 & -0.04 & -0.16 & -0.14 & -0.35 & -0.15 & -0.17 & -0.13 \\
4283 & KOI-2407 & 0.08 & 0.12 & 0.15 & 0.18 & 0.11 & 0.09 & 0.15 & 0.24 & 0.18 & 0.12 & 0.18 & 0.15 & 0.17 & 0.16 & 0.24 \\
4284 & KOI-2396 & -0.01 & -0.17 & 0.01 & -0.01 & 0.01 & -0.02 & 0.02 & 0.05 & 0.05 & 0.01 & 0.06 & 0.04 & 0.04 & 0.03 & 0.05 \\
4285 & KOI-4457 & -0.22 & 0.29 & -0.02 & -0.24 & -0.19 & -0.29 & -0.18 & -0.09 & -0.03 & -0.19 & -0.14 & -0.42 & -0.13 & -0.22 & -0.23 \\
4286 & KOI-360 & -0.09 & -0.27 & -0.01 & -0.17 & -0.11 & -0.04 & -0.12 & -0.12 & -0.07 & 0.00 & -0.12 & -0.25 & -0.11 & -0.15 & -0.13 \\
4287 & KOI-141 & 0.19 & 0.38 & 0.18 & 0.48 & 0.17 & 0.36 & 0.22 & 0.28 & 0.28 & 0.30 & 0.21 & 0.30 & 0.25 & 0.23 & 0.09 \\
4288 & KOI-2597 & -0.13 & -0.48 & -0.09 & -0.23 & -0.22 & -0.71 & -0.15 & -0.26 & -0.16 & -0.02 & -0.33 & -0.51 & -0.28 & -0.31 & -0.32 \\
4289 & KOI-2004 & 0.22 & 0.24 & 0.25 & 0.29 & 0.22 & 0.26 & 0.24 & 0.21 & 0.21 & 0.18 & 0.20 & 0.25 & 0.21 & 0.27 & 0.08 \\
4290 & KOI-2714 & -0.03 & -0.38 & 0.11 & 0.05 & -0.10 & -0.09 & -0.03 & 0.04 & 0.07 & -0.24 & -0.00 & -0.21 & -0.02 & -0.07 & 0.08 \\
4291 & Kepler-401 & 0.01 & 0.16 & 0.07 & -0.07 & -0.04 & -0.00 & -0.03 & 0.02 & 0.04 & 0.06 & -0.02 & -0.13 & -0.00 & -0.05 & -0.06 \\
4292 & KOI-1947 & 0.10 & 0.28 & 0.21 & 0.19 & 0.14 & 0.16 & 0.15 & 0.19 & 0.19 & 0.09 & 0.18 & 0.19 & 0.21 & 0.21 & 0.42 \\
4293 & KOI-2372 & -0.07 & -0.03 & 0.07 & -0.16 & -0.12 & -0.29 & -0.16 & -0.08 & -0.07 & -0.19 & -0.09 & -0.29 & -0.09 & -0.16 & -0.18 \\
4294 & KOI-3310 & 0.09 & 0.07 & 0.15 & 0.12 & 0.12 & 0.11 & 0.14 & 0.16 & 0.15 & 0.10 & 0.17 & 0.15 & 0.13 & 0.16 & 0.14 \\
4295 & KOI-3167 & -0.06 & -0.14 & 0.00 & -0.19 & -0.11 & -0.18 & -0.08 & -0.00 & -0.03 & -0.12 & -0.04 & -0.16 & -0.06 & -0.16 & 0.13 \\
4296 & KOI-279 & 0.10 & 0.41 & 0.49 & 0.21 & 0.08 & 0.03 & 0.17 & 0.30 & 0.18 & 0.08 & 0.17 & 0.18 & 0.20 & 0.11 & 0.26 \\
4297 & WASP-92 & 0.08 & 0.05 & 0.14 & 0.03 & 0.06 & 0.10 & 0.09 & 0.10 & 0.10 & 0.06 & 0.09 & 0.07 & 0.10 & 0.07 & 0.16 \\
4298 & KOI-2541 & -0.02 & 0.07 & 0.04 & 0.01 & 0.06 & 0.14 & -0.03 & 0.05 & 0.09 & 0.03 & 0.09 & 0.13 & 0.11 & 0.09 & 0.13 \\
4299 & KOI-2059 & 0.06 & -0.07 & 0.09 & 0.19 & -0.08 & 0.05 & 0.04 & 0.12 & 0.01 & 0.03 & -0.04 & 0.01 & -0.02 & -0.05 & -0.17 \\
4300 & KOI-375 & 0.09 & 0.22 & 0.27 & 0.15 & 0.13 & 0.19 & 0.11 & 0.18 & 0.14 & 0.08 & 0.15 & 0.14 & 0.16 & 0.18 & 0.14 \\
4301 & KOI-1474 & 0.05 & 0.45 & 0.37 & 0.25 & 0.14 & 0.15 & 0.22 & 0.29 & 0.29 & 0.05 & 0.23 & 0.13 & 0.24 & 0.18 & 0.23 \\
4302 & KOI-3122 & 0.16 & 0.08 & 0.32 & 0.16 & 0.13 & 0.03 & 0.16 & 0.28 & 0.25 & 0.07 & 0.28 & 0.11 & 0.26 & 0.17 & 0.62 \\
4303 & KOI-3009 & 0.12 & 0.08 & 0.11 & 0.17 & 0.09 & 0.16 & 0.13 & 0.19 & 0.16 & 0.05 & 0.15 & 0.18 & 0.17 & 0.08 & 0.18 \\
4304 & KOI-4829 & -0.04 & 0.33 & 0.08 & -0.13 & -0.07 & -0.21 & -0.07 & 0.00 & -0.05 & -0.06 & -0.06 & -0.22 & -0.06 & -0.08 & -0.05 \\
4305 & KOI-2331 & 0.05 & 0.11 & 0.11 & 0.12 & 0.05 & 0.11 & 0.07 & 0.09 & 0.03 & 0.06 & 0.06 & 0.08 & 0.07 & 0.07 & 0.04 \\
4306 & KOI-361 & 0.04 & 0.12 & 0.08 & 0.01 & 0.03 & 0.06 & 0.10 & 0.05 & 0.01 & 0.06 & 0.09 & 0.06 & 0.07 & 0.05 & 0.14 \\
4307 & KOI-2463 & 0.18 & 0.43 & 0.21 & 0.13 & 0.14 & 0.22 & 0.22 & 0.15 & 0.24 & 0.31 & 0.23 & 0.20 & 0.22 & 0.21 & 0.23 \\
4308 & KOI-439 & 0.29 & 0.27 & 0.32 & 0.37 & 0.23 & 0.31 & 0.26 & 0.24 & 0.26 & 0.25 & 0.27 & 0.31 & 0.27 & 0.25 & 0.13 \\
4309 & KOI-4329 & -0.04 & 0.37 & 0.08 & 0.01 & 0.12 & 0.19 & 0.08 & 0.17 & 0.19 & 0.25 & 0.15 & 0.02 & 0.14 & 0.09 & 0.08 \\
4310 & KOI-4605 & -0.06 & 0.14 & 0.15 & -0.10 & -0.04 & -0.09 & -0.03 & 0.09 & 0.03 & -0.08 & 0.02 & -0.13 & 0.03 & -0.03 & 0.08 \\
4311 & KOI-4190 & 0.13 & 0.15 & 0.01 & 0.28 & 0.19 & 0.22 & 0.17 & 0.25 & 0.22 & 0.19 & 0.20 & 0.23 & 0.22 & 0.16 & 0.23 \\
4312 & KOI-548 & -0.03 & -0.10 & -0.01 & -0.20 & -0.05 & -0.18 & -0.09 & -0.03 & -0.01 & -0.09 & -0.06 & -0.31 & -0.06 & -0.10 & -0.13 \\
4313 & KOI-3663 & -0.07 & -0.17 & -0.06 & -0.16 & -0.06 & -0.07 & -0.08 & -0.07 & -0.03 & -0.12 & -0.03 & -0.09 & -0.08 & -0.09 & 0.00 \\
4314 & KOI-4245 & 0.07 & 0.56 & 0.32 & 0.17 & 0.14 & 0.21 & 0.19 & 0.23 & 0.20 & 0.11 & 0.23 & 0.24 & 0.25 & 0.20 & 0.32 \\
4315 & BD+52_277A & -0.30 & 0.19 & 0.50 & 0.04 & 0.09 & -0.25 & 0.16 & 0.21 & 0.20 & 0.05 & 0.14 & -0.10 & 0.19 & -0.00 & 0.23 \\
4316 & HD 239643 & 0.03 & 0.07 & 0.15 & 0.01 & -0.00 & -0.02 & 0.03 & 0.06 & 0.02 & 0.05 & 0.04 & -0.04 & 0.05 & 0.00 & 0.04 \\
4317 & HD 203802 & -0.01 & 0.27 & 0.19 & 0.01 & 0.08 & 0.09 & 0.11 & 0.13 & 0.18 & 0.24 & 0.13 & 0.01 & 0.14 & 0.13 & 0.16 \\
4318 & HD 240051 & 0.10 & 0.03 & 0.11 & 0.03 & 0.11 & 0.09 & 0.13 & 0.19 & 0.17 & 0.18 & 0.19 & 0.13 & 0.18 & 0.12 & 0.29 \\
4319 & HD 215714 & -0.06 & 0.36 & 0.34 & 0.06 & 0.09 & -0.27 & 0.20 & 0.19 & 0.19 & 0.02 & 0.17 & 0.06 & 0.18 & 0.09 & 0.18 \\
\enddata
\end{deluxetable*}


==> table_05.tex <==
\begin{deluxetable*}{llDDrrrrrr}
\tablecaption{Derived Stellar Properties.
    \label{table:derived_stellar_props}
    }
\tablehead{\colhead{ID} & \colhead{Name} & \twocolhead{Plx} & \twocolhead{$\sigma$ Plx} & \colhead{R} & \colhead{$\Delta$ R} & \colhead{M} & \colhead{$\Delta$ M} & \colhead{Age} & \colhead{$\Delta$ Age} \\
 \colhead{} & \colhead{} & \twocolhead{(mas)} & \twocolhead{(mas)} & \colhead{(R$_{\odot}$)} & \colhead{(R$_{\odot}$)} & \colhead{(M$_{\odot}$)} & \colhead{(M$_{\odot}$)} & \colhead{(Gyrs)} & \colhead{(Gyrs)} \\
 \colhead{(1)} & \colhead{(2)} & \twocolhead{(33)} & \twocolhead{(34)} & \colhead{(35)} & \colhead{(36)} & \colhead{(37)} & \colhead{(38)} & \colhead{(39)} & \colhead{(40)}}
\decimals
\startdata
2281 & KOI-3248 & 2.7 & 0.023 & 1.14 & 1.12 -  1.16 & 0.96 & 0.95 -  0.97 & 8.40 & 8.01 -  8.73 \\
2361 & KOI-4273 & -1.31 & 0.5 & 1.81 & 1.69 -  1.95 & 1.34 & 1.29 -  1.39 & 3.48 & 3.29 -  3.76 \\
2393 & KOI-3605 & 1.78 & 0.018 & 0.98 & 0.97 -  0.99 & 0.86 & 0.85 -  0.86 & 14.77 & 14.40 - 14.94 \\
2405 & KOI-3197 & 3.54 & 0.035 & 1.12 & 1.10 -  1.13 & 1.16 & 1.15 -  1.18 & 1.08 & 0.61 -  1.60 \\
2430 & KOI-1353 & 1.39 & 0.018 & 1.03 & 1.01 -  1.05 & 1.07 & 1.06 -  1.09 & 2.22 & 1.40 -  3.03 \\
2435 & KOI-4323 & 0.93 & 0.015 & 1.74 & 1.70 -  1.78 & 1.33 & 1.32 -  1.35 & 3.06 & 2.96 -  3.14 \\
2445 & KOI-3384 & 1.6 & 0.017 & 1.29 & 1.27 -  1.32 & 1.11 & 1.10 -  1.12 & 5.20 & 4.89 -  5.54 \\
2460 & KOI-4409 & 2.2 & 0.028 & 1.28 & 1.25 -  1.30 & 1.12 & 1.10 -  1.13 & 5.36 & 4.96 -  5.76 \\
2464 & KOI-4226 & 1.34 & 0.031 & 1.98 & 1.93 -  2.04 & 1.39 & 1.37 -  1.40 & 3.62 & 3.48 -  3.80 \\
2485 & K2-58 & 5.47 & 0.043 &  &  &  &  &  &  \\
2914 & XO-1 & 6.09 & 0.023 & 0.95 & 0.94 -  0.96 & 0.96 & 0.95 -  0.97 & 4.65 & 3.76 -  5.58 \\
2962 & TRES-4 & 1.91 & 0.026 & 1.73 & 1.61 -  1.87 & 1.38 & 1.34 -  1.43 & 2.75 & 2.64 -  2.89 \\
2980 & KOI-104 & 5.18 & 0.022 & 0.78 & 0.76 -  0.78 & 0.81 & 0.79 -  0.82 & 7.89 & 4.73 - 10.84 \\
2981 & KOI-263 & 3.67 & 0.024 & 1.95 & 1.92 -  1.98 & 1.16 & 1.14 -  1.20 & 4.77 & 4.23 -  5.20 \\
2982 & KOI-10 & 0.95 & 0.014 & 1.63 & 1.60 -  1.67 & 1.22 & 1.19 -  1.26 & 4.16 & 3.59 -  4.54 \\
2983 & KOI-82 & 9.25 & 0.019 & 0.76 & 0.75 -  0.77 & 0.79 & 0.77 -  0.80 & 7.77 & 4.20 - 11.27 \\
2986 & KOI-274 & 2.49 & 0.025 & 1.72 & 1.68 -  1.75 & 1.27 & 1.20 -  1.29 & 3.81 & 3.64 -  4.80 \\
2987 & KOI-22 & 1.35 & 0.013 & 1.33 & 1.31 -  1.35 & 1.08 & 1.07 -  1.10 & 6.78 & 6.19 -  7.39 \\
2988 & KOI-42 & 6.75 & 0.022 & 1.53 & 1.51 -  1.56 & 1.28 & 1.27 -  1.29 & 3.07 & 2.94 -  3.20 \\
2989 & KOI-701 & 3.29 & 0.013 & 0.70 & 0.70 -  0.71 & 0.68 & 0.68 -  0.69 & 14.41 & 13.46 - 14.84 \\
2997 & KOI-245 & 15.6 & 0.029 & 0.80 & 0.79 -  0.81 & 0.80 & 0.78 -  0.81 & 7.87 & 6.10 -  9.61 \\
2998 & KOI-180 & 2.59 & 0.019 & 0.91 & 0.90 -  0.93 & 0.96 & 0.95 -  0.97 & 3.88 & 2.60 -  5.15 \\
2999 & KOI-367 & 5.35 & 0.024 & 1.03 & 1.02 -  1.05 & 0.99 & 0.98 -  1.00 & 6.55 & 5.69 -  7.32 \\
3000 & KOI-122 & 2.22 & 0.029 & 1.46 & 1.43 -  1.49 & 1.06 & 1.04 -  1.07 & 8.96 & 8.48 -  9.47 \\
3001 & KOI-1612 & 11.2 & 0.033 & 1.28 & 1.26 -  1.30 & 1.07 & 1.06 -  1.08 & 5.30 & 5.01 -  5.58 \\
3003 & KOI-2169 & 3.98 & 0.029 & 0.90 & 0.88 -  0.91 & 0.88 & 0.87 -  0.89 & 9.33 & 7.74 - 10.95 \\
3006 & KOI-7 & 2.02 & 0.024 & 1.58 & 1.55 -  1.62 & 1.10 & 1.09 -  1.11 & 7.41 & 7.10 -  7.77 \\
3007 & KOI-299 & 2.83 & 0.024 & 0.95 & 0.93 -  0.96 & 0.94 & 0.92 -  0.95 & 7.11 & 5.80 -  8.40 \\
3011 & KOI-1442 & 2.93 & 0.022 & 1.08 & 1.06 -  1.10 & 0.99 & 0.98 -  1.00 & 8.06 & 7.27 -  8.92 \\
3017 & KOI-244 & 4.08 & 0.024 & 1.40 & 1.38 -  1.42 & 1.16 & 1.15 -  1.18 & 4.26 & 3.88 -  4.65 \\
3018 & KOI-1 & 4.62 & 0.022 & 1.07 & 1.05 -  1.09 & 1.01 & 1.00 -  1.02 & 5.69 & 4.97 -  6.37 \\
3020 & KOI-1431 & 2.09 & 0.015 & 0.99 & 0.97 -  1.01 & 0.93 & 0.92 -  0.94 & 9.18 & 8.01 - 10.35 \\
3022 & KOI-292 & 2.47 & 0.022 & 1.00 & 0.99 -  1.02 & 0.92 & 0.91 -  0.93 & 7.20 & 6.43 -  7.88 \\
3024 & Kepler-174 & 2.57 & 0.018 & 0.65 & 0.65 -  0.66 & 0.64 & 0.64 -  0.64 & 14.81 & 14.49 - 14.95 \\
3025 & KOI-273 & 4.3 & 0.024 & 1.12 & 1.10 -  1.14 & 0.99 & 0.97 -  1.00 & 8.86 & 8.11 -  9.63 \\
3026 & KOI-111 & 2.47 & 0.027 & 1.06 & 1.04 -  1.08 & 0.88 & 0.87 -  0.89 & 9.37 & 8.66 - 10.10 \\
3027 & KOI-1781 & 6.48 & 0.019 & 0.78 & 0.77 -  0.79 & 0.80 & 0.78 -  0.81 & 9.92 & 6.56 - 12.86 \\
3031 & KOI-70 & 3.51 & 0.022 & 0.91 & 0.90 -  0.93 & 0.92 & 0.90 -  0.93 & 6.92 & 5.46 -  8.33 \\
3032 & KOI-98 &  &  & 2.02 & 1.87 -  2.18 & 1.46 & 1.41 -  1.52 & 2.52 & 2.33 -  2.70 \\
3034 & KOI-153 & 3.78 & 0.016 & 0.76 & 0.76 -  0.77 & 0.76 & 0.75 -  0.77 & 13.53 & 11.48 - 14.62 \\
3036 & KOI-262 & 3.97 & 0.029 & 1.63 & 1.60 -  1.65 & 1.25 & 1.20 -  1.27 & 3.67 & 3.36 -  4.50 \\
3040 & KOI-283 & 4.34 & 0.027 & 1.03 & 1.01 -  1.05 & 1.02 & 1.01 -  1.03 & 4.78 & 3.92 -  5.63 \\
3041 & KOI-97 & 1.06 & 0.024 & 2.10 & 2.04 -  2.15 & 1.46 & 1.44 -  1.48 & 3.02 & 2.87 -  3.13 \\
3042 & KOI-85 & 3.26 & 0.029 & 1.51 & 1.48 -  1.53 & 1.25 & 1.24 -  1.26 & 3.73 & 3.60 -  3.87 \\
3043 & KOI-108 & 1.99 & 0.024 & 1.54 & 1.51 -  1.57 & 1.12 & 1.11 -  1.13 & 6.64 & 6.25 -  6.96 \\
3045 & KOI-87 & 5.11 & 0.024 & 0.86 & 0.85 -  0.87 & 0.87 & 0.85 -  0.88 & 5.71 & 4.47 -  6.97 \\
3046 & KOI-63 & 5.12 & 0.025 & 0.94 & 0.92 -  0.95 & 0.94 & 0.92 -  0.95 & 6.85 & 5.48 -  8.13 \\
3048 & KOI-260 & 4.18 & 0.029 & 1.43 & 1.41 -  1.45 & 1.18 & 1.17 -  1.19 & 3.68 & 3.54 -  3.86 \\
3054 & KOI-5 & 1.81 & 0.081 & 2.13 & 2.06 -  2.21 & 1.36 & 1.34 -  1.40 & 3.77 & 3.49 -  3.94 \\
3055 & KOI-3158 & 27.4 & 0.029 & 0.76 & 0.75 -  0.76 & 0.71 & 0.71 -  0.71 & 14.89 & 14.70 - 14.97 \\
3058 & KOI-123 & 2.08 & 0.023 & 1.38 & 1.36 -  1.41 & 1.08 & 1.07 -  1.10 & 6.35 & 5.89 -  6.85 \\
3059 & KOI-84 & 4.55 & 0.02 & 0.90 & 0.89 -  0.91 & 0.90 & 0.89 -  0.92 & 6.23 & 4.96 -  7.46 \\
3064 & KOI-277 & 1.87 & 0.021 & 1.70 & 1.67 -  1.73 & 1.14 & 1.12 -  1.16 & 4.77 & 4.31 -  5.14 \\
3065 & KOI-41 & 3.25 & 0.019 & 1.57 & 1.55 -  1.60 & 1.11 & 1.10 -  1.12 & 6.94 & 6.67 -  7.24 \\
3067 & KOI-69 & 10.4 & 0.024 & 0.96 & 0.94 -  0.97 & 0.90 & 0.89 -  0.91 & 7.88 & 7.01 -  8.71 \\
3068 & KOI-75 & 2.33 & 0.022 & 2.62 & 2.58 -  2.67 & 1.28 & 1.23 -  1.31 & 3.83 & 3.48 -  4.45 \\
3072 & KOI-103 & 3.25 & 0.025 & 0.90 & 0.88 -  0.91 & 0.92 & 0.91 -  0.94 & 5.20 & 3.81 -  6.54 \\
3074 & KOI-321 & 2.72 & 0.025 & 1.11 & 1.10 -  1.13 & 0.98 & 0.97 -  0.99 & 9.22 & 8.39 - 10.02 \\
3078 & KOI-2687 & 8.82 & 0.023 & 0.96 & 0.95 -  0.98 & 1.00 & 0.99 -  1.01 & 3.43 & 2.47 -  4.40 \\
3084 & KOI-1925 & 14.6 & 0.021 & 0.92 & 0.91 -  0.94 & 0.88 & 0.87 -  0.89 & 9.78 & 8.39 - 11.17 \\
3091 & KOI-1924 & 8.71 & 0.27 & 2.59 & 2.50 -  2.65 & 1.56 & 1.52 -  1.61 & 2.58 & 2.30 -  2.87 \\
3100 & KOI-99 & 3.99 & 0.019 & 0.77 & 0.77 -  0.78 & 0.73 & 0.73 -  0.73 & 14.79 & 14.47 - 14.94 \\
3101 & KOI-2720 & 4.65 & 0.027 & 1.59 & 1.56 -  1.61 & 1.13 & 1.10 -  1.13 & 5.05 & 4.84 -  5.54 \\
3103 & KOI-364 & 5.99 & 0.026 & 1.45 & 1.43 -  1.47 & 1.09 & 1.08 -  1.12 & 7.40 & 6.64 -  7.82 \\
3105 & KOI-64 & 1.08 & 0.014 & 2.58 & 2.53 -  2.63 & 1.28 & 1.24 -  1.33 & 4.57 & 4.05 -  5.02 \\
3110 & KOI-174 & 3.17 & 0.023 & 0.74 & 0.74 -  0.75 & 0.71 & 0.71 -  0.72 & 14.81 & 14.49 - 14.95 \\
3111 & KOI-17 & 1.67 & 0.015 & 1.32 & 1.30 -  1.34 & 1.06 & 1.04 -  1.09 & 8.20 & 6.89 -  8.87 \\
3113 & KOI-265 & 2.52 & 0.021 & 1.31 & 1.29 -  1.34 & 1.17 & 1.16 -  1.18 & 4.02 & 3.72 -  4.30 \\
3114 & KOI-261 & 8.11 & 0.026 & 0.96 & 0.95 -  0.98 & 1.01 & 1.00 -  1.03 & 2.99 & 2.01 -  3.95 \\
3117 & KOI-305 & 4.77 & 0.024 & 0.77 & 0.76 -  0.78 & 0.81 & 0.80 -  0.83 & 6.57 & 3.39 - 10.09 \\
3118 & KOI-365 & 6.38 & 0.029 & 0.88 & 0.87 -  0.89 & 0.86 & 0.84 -  0.87 & 8.22 & 6.95 -  9.47 \\
3123 & KOI-137 & 2.28 & 0.017 & 0.95 & 0.94 -  0.97 & 0.89 & 0.88 -  0.91 & 10.89 & 9.52 - 12.27 \\
3130 & KOI-148 & 3.23 & 0.019 & 0.88 & 0.86 -  0.89 & 0.86 & 0.85 -  0.87 & 10.59 & 8.54 - 12.57 \\
3131 & KOI-18 & 1.08 & 0.02 & 1.79 & 1.75 -  1.83 & 1.37 & 1.36 -  1.39 & 2.88 & 2.80 -  2.97 \\
3133 & KOI-116 & 2.22 & 0.03 & 1.06 & 1.04 -  1.08 & 1.02 & 1.01 -  1.03 & 4.46 & 3.72 -  5.18 \\
3239 & HD 240429 & 9.7 & 0.025 & 1.05 & 1.04 -  1.07 & 1.04 & 1.03 -  1.05 & 4.20 & 3.58 -  4.81 \\
3240 & HD 240430 & 9.69 & 0.026 & 1.14 & 1.13 -  1.16 & 1.06 & 1.05 -  1.07 & 5.70 & 5.17 -  6.21 \\
3248 & WASP-57 & 2.48 & 0.036 & 1.05 & 1.03 -  1.07 & 1.02 & 1.01 -  1.03 & 5.20 & 4.34 -  6.02 \\
3249 & WASP-74 & 6.67 & 0.051 & 1.56 & 1.53 -  1.59 & 1.27 & 1.26 -  1.28 & 3.86 & 3.74 -  3.99 \\
3250 & WASP-37 & 2.52 & 0.049 & 1.07 & 1.05 -  1.09 & 0.94 & 0.93 -  0.95 & 7.16 & 6.59 -  7.72 \\
3251 & HAT-P-41 & 2.84 & 0.037 & 1.73 & 1.69 -  1.77 & 1.41 & 1.40 -  1.43 & 2.34 & 2.25 -  2.43 \\
3252 & COROT-28 & 1.28 & 0.024 & 2.39 & 2.34 -  2.44 & 1.25 & 1.20 -  1.28 & 5.50 & 5.12 -  6.20 \\
3253 & HAT-P-27 & 4.99 & 0.036 & 0.94 & 0.92 -  0.96 & 0.90 & 0.89 -  0.91 & 10.58 & 9.06 - 12.09 \\
3254 & WASP-103 & 1.14 & 0.17 & 1.78 & 1.68 -  1.88 & 1.32 & 1.29 -  1.36 & 3.72 & 3.48 -  3.93 \\
3255 & WASP-52 & 5.69 & 0.043 & 0.90 & 0.87 -  0.92 & 0.86 & 0.85 -  0.88 & 12.61 & 9.30 - 14.34 \\
3256 & WASP-114 & 1.88 & 0.061 & 1.34 & 1.25 -  1.43 & 1.19 & 1.17 -  1.22 & 3.80 & 3.33 -  4.07 \\
3257 & BD+1290 & 9.2 & 0.058 & 1.43 & 1.40 -  1.45 & 1.07 & 1.07 -  1.07 & 6.12 & 5.87 -  6.38 \\
3258 & HD 4552 & 9.12 & 0.056 & 1.50 & 1.47 -  1.52 & 1.19 & 1.17 -  1.22 & 4.33 & 3.99 -  4.91 \\
3259 & HD 209622 &  &  & 1.60 & 1.49 -  1.72 & 1.30 & 1.27 -  1.34 & 3.41 & 3.24 -  3.55 \\
3260 & BD+15_4556 & 2.28 & 0.051 & 11.79 & 11.54 - 12.09 & 2.64 & 2.61 -  2.70 & 0.61 & 0.57 -  0.64 \\
3261 & HAT-P-23 & 2.71 & 0.035 & 1.14 & 1.12 -  1.16 & 1.16 & 1.15 -  1.17 & 1.96 & 1.41 -  2.53 \\
3262 & HAT-P-55 & 1.93 & 0.014 & 1.13 & 1.11 -  1.15 & 0.98 & 0.97 -  0.99 & 7.64 & 7.22 -  8.02 \\
3263 & HAT-P-31 & 2.88 & 0.024 & 1.53 & 1.50 -  1.56 & 1.15 & 1.13 -  1.17 & 5.66 & 5.29 -  6.08 \\
3264 & BD+28_4543S & 1.48 & 0.04 &  &  &  &  &  &  \\
3265 & WASP-135 & 3.32 & 0.016 & 0.97 & 0.93 -  0.99 & 0.88 & 0.87 -  0.88 & 13.72 & 11.85 - 14.66 \\
3266 & WASP-10 & 7.06 & 0.037 & 0.76 & 0.75 -  0.77 & 0.80 & 0.79 -  0.82 & 6.01 & 3.07 -  9.10 \\
3267 & KELT-16 & 2.22 & 0.028 & 1.72 & 1.61 -  1.84 & 1.32 & 1.28 -  1.36 & 3.18 & 3.08 -  3.30 \\
3268 & HAT-P-18 & 6.17 & 0.023 & 0.76 & 0.75 -  0.77 & 0.78 & 0.77 -  0.80 & 9.53 & 6.07 - 12.53 \\
3269 & HAT-P-4 & 3.09 & 0.027 & 1.55 & 1.44 -  1.67 & 1.24 & 1.21 -  1.28 & 4.26 & 4.09 -  4.45 \\
3270 & KELT-12 & 2.69 & 0.023 & 2.20 & 2.17 -  2.24 & 1.56 & 1.55 -  1.57 & 2.21 & 2.14 -  2.28 \\
3271 & KOI-958 & 5.86 & 0.022 & 0.74 & 0.73 -  0.75 & 0.78 & 0.76 -  0.80 & 6.04 & 2.72 -  9.42 \\
3272 & KOI-1010 & 0.986 & 0.016 & 1.64 & 1.60 -  1.68 & 1.24 & 1.19 -  1.27 & 3.99 & 3.67 -  4.80 \\
3273 & KOI-984 & 4.27 & 0.024 & 1.10 & 1.09 -  1.12 & 0.90 & 0.90 -  0.91 & 14.78 & 14.45 - 14.94 \\
3274 & KOI-4212 & 1.03 & 0.018 & 1.32 & 1.30 -  1.36 & 1.19 & 1.17 -  1.20 & 3.64 & 3.32 -  3.89 \\
3275 & KOI-1002 & 1.29 & 0.52 & 0.97 & 0.94 -  1.00 & 0.86 & 0.85 -  0.87 & 13.97 & 12.30 - 14.72 \\
3276 & KOI-2538 & 1.84 & 0.093 & 0.76 & 0.75 -  0.77 & 0.73 & 0.72 -  0.73 & 14.54 & 13.78 - 14.88 \\
3277 & KOI-2534 & 1.17 & 0.027 & 1.21 & 1.17 -  1.24 & 1.12 & 1.11 -  1.13 & 3.72 & 3.18 -  4.20 \\
3278 & KOI-3233 & 3.05 & 0.028 & 1.00 & 0.98 -  1.02 & 0.98 & 0.96 -  0.99 & 5.57 & 4.60 -  6.43 \\
3279 & KOI-2403 & 1.76 & 0.026 & 1.24 & 1.21 -  1.27 & 1.16 & 1.14 -  1.17 & 3.46 & 3.04 -  3.83 \\
3280 & KOI-2201 & 0.796 & 0.017 & 1.88 & 1.83 -  1.92 & 1.35 & 1.33 -  1.37 & 3.65 & 3.52 -  3.80 \\
3281 & KOI-988 & 3.12 & 0.017 & 0.79 & 0.77 -  0.80 & 0.82 & 0.80 -  0.84 & 7.20 & 4.15 - 10.10 \\
3282 & KOI-151 & 0.998 & 0.047 & 1.40 & 1.34 -  1.46 & 1.18 & 1.16 -  1.21 & 3.84 & 3.58 -  4.28 \\
3283 & KOI-113 & -1.62 & 0.63 & 1.77 & 1.64 -  1.90 & 1.13 & 1.08 -  1.19 & 7.71 & 6.24 -  9.03 \\
3284 & KOI-3201 & 4.13 & 0.021 & 0.95 & 0.93 -  0.96 & 0.82 & 0.81 -  0.83 & 10.77 & 9.76 - 11.78 \\
3285 & KOI-2053 & 1.38 & 0.021 & 1.49 & 1.46 -  1.53 & 1.17 & 1.15 -  1.19 & 4.95 & 4.54 -  5.35 \\
3286 & KOI-2033 &  &  & 0.77 & 0.75 -  0.78 & 0.75 & 0.74 -  0.77 & 12.30 & 8.48 - 14.26 \\
3287 & KOI-1944 & 1.59 & 0.016 & 0.92 & 0.90 -  0.93 & 0.99 & 0.98 -  1.01 & 2.04 & 0.99 -  3.30 \\
3288 & KOI-2603 & 1.31 & 0.025 & 1.81 & 1.77 -  1.85 & 1.32 & 1.26 -  1.34 & 3.32 & 3.20 -  4.04 \\
3289 & KOI-440 & 2.23 & 0.018 & 0.83 & 0.81 -  0.84 & 0.82 & 0.81 -  0.84 & 10.70 & 8.15 - 13.09 \\
3290 & KOI-166 & 2.87 & 0.016 & 0.78 & 0.77 -  0.79 & 0.74 & 0.73 -  0.75 & 13.21 & 11.45 - 14.39 \\
3291 & KOI-379 & 0.801 & 0.017 & 2.75 & 2.67 -  2.81 & 1.58 & 1.55 -  1.66 & 2.35 & 2.06 -  2.65 \\
3292 & KOI-2009 & 1.48 & 0.018 & 1.09 & 1.07 -  1.11 & 0.89 & 0.88 -  0.90 & 9.71 & 9.17 - 10.28 \\
3293 & KOI-4581 & 1.44 & 0.014 & 1.21 & 1.19 -  1.24 & 1.06 & 1.04 -  1.07 & 6.26 & 5.80 -  6.78 \\
3294 & KOI-3835 & 4.8 & 0.026 & 0.75 & 0.74 -  0.76 & 0.80 & 0.78 -  0.82 & 4.63 & 1.76 -  7.80 \\
3295 & KOI-3681 & 2.49 & 0.026 & 1.31 & 1.28 -  1.33 & 1.20 & 1.19 -  1.21 & 3.16 & 2.88 -  3.46 \\
3296 & KOI-3853 & 3.22 & 0.025 & 3.12 & 3.08 -  3.18 & 0.98 & 0.94 -  1.03 & 11.77 & 9.79 - 13.56 \\
3297 & KOI-2979 & 1.45 & 0.016 & 1.29 & 1.27 -  1.32 & 1.05 & 1.04 -  1.07 & 5.79 & 5.47 -  6.07 \\
3298 & KOI-986 & 1.57 & 0.018 & 0.97 & 0.95 -  0.99 & 0.93 & 0.92 -  0.94 & 8.85 & 7.35 - 10.18 \\
3299 & KOI-2896 & 2.71 & 0.93 & 1.18 & 1.12 -  1.24 & 1.17 & 1.16 -  1.18 & 2.07 & 1.03 -  2.93 \\
3300 & KOI-4659 & 1.89 & 0.017 & 0.94 & 0.93 -  0.96 & 0.92 & 0.91 -  0.94 & 6.70 & 5.50 -  7.78 \\
3301 & KOI-1118 & 1.06 & 0.018 & 1.20 & 1.13 -  1.27 & 1.07 & 1.05 -  1.08 & 5.06 & 4.29 -  5.52 \\
3302 & KOI-4298 & 1.08 & 0.015 & 1.54 & 1.51 -  1.57 & 1.03 & 1.02 -  1.05 & 6.28 & 5.94 -  6.55 \\
3303 & KOI-1113 & 1.15 & 0.016 & 1.32 & 1.29 -  1.35 & 1.14 & 1.13 -  1.15 & 4.47 & 4.16 -  4.79 \\
3304 & KOI-1116 & 1.8 & 0.014 & 1.08 & 1.06 -  1.10 & 0.99 & 0.98 -  1.00 & 6.85 & 6.13 -  7.57 \\
3305 & KOI-2081 & 0.763 & 0.015 & 3.56 & 3.49 -  3.64 & 1.23 & 1.20 -  1.35 & 5.79 & 4.17 -  6.24 \\
3306 & KOI-4400 & 1.52 & 0.015 & 1.08 & 1.06 -  1.10 & 1.02 & 1.01 -  1.03 & 5.32 & 4.62 -  6.03 \\
3307 & KOI-1824 & 2.17 & 0.031 & 1.13 & 1.11 -  1.16 & 0.98 & 0.96 -  0.99 & 6.87 & 6.36 -  7.34 \\
3308 & KOI-2807 & 0.923 & 0.018 & 1.50 & 1.46 -  1.54 & 1.29 & 1.27 -  1.30 & 2.94 & 2.75 -  3.11 \\
3309 & KOI-2335 & 0.836 & 0.14 & 1.04 & 0.99 -  1.10 & 0.91 & 0.90 -  0.92 & 9.90 & 9.02 - 10.47 \\
3310 & KOI-197 & 2.68 & 0.017 & 0.77 & 0.76 -  0.78 & 0.76 & 0.75 -  0.77 & 13.28 & 11.01 - 14.53 \\
3311 & KOI-4144 & 1.16 & 0.02 & 1.01 & 0.99 -  1.03 & 1.02 & 1.01 -  1.04 & 3.17 & 2.16 -  4.07 \\
3312 & KOI-1115 & 0.856 & 0.019 & 1.91 & 1.86 -  1.96 & 1.14 & 1.11 -  1.18 & 6.77 & 5.91 -  7.40 \\
3313 & HAT-P-14 & 4.46 & 0.025 & 1.65 & 1.62 -  1.68 & 1.37 & 1.36 -  1.38 & 2.35 & 2.27 -  2.44 \\
3314 & KOI-1878 & 1.44 & 0.021 & 1.42 & 1.39 -  1.45 & 1.22 & 1.21 -  1.23 & 3.72 & 3.53 -  3.88 \\
3315 & KOI-3277 & 0.975 & 0.016 & 2.25 & 2.20 -  2.30 & 1.21 & 1.18 -  1.26 & 4.83 & 4.39 -  5.04 \\
3316 & KOI-3203 & 1.69 & 0.028 & 1.81 & 1.78 -  1.84 & 1.32 & 1.31 -  1.33 & 2.86 & 2.78 -  2.92 \\
3317 & KOI-3225 & 4.37 & 0.025 & 0.89 & 0.87 -  0.90 & 0.88 & 0.87 -  0.89 & 8.73 & 6.95 - 10.48 \\
3318 & Kepler-24 & 0.836 & 0.024 & 1.13 & 1.10 -  1.17 & 1.10 & 1.09 -  1.12 & 3.05 & 2.28 -  3.74 \\
3319 & KOI-490 & 2.9 & 0.017 & 0.76 & 0.75 -  0.77 & 0.76 & 0.75 -  0.77 & 12.95 & 10.42 - 14.41 \\
3320 & KOI-1089 & 0.969 & 0.02 & 1.11 & 1.09 -  1.15 & 1.04 & 1.03 -  1.06 & 5.30 & 4.47 -  6.05 \\
3321 & KOI-2863 & 1.44 & 0.015 & 1.13 & 1.12 -  1.16 & 0.90 & 0.89 -  0.91 & 9.91 & 9.40 - 10.42 \\
3322 & KOI-3515 & 1.42 & 0.023 & 1.96 & 1.91 -  2.01 & 1.29 & 1.26 -  1.34 & 2.99 & 2.68 -  3.32 \\
3323 & KOI-401 & 1.72 & 0.017 & 1.03 & 1.01 -  1.05 & 0.91 & 0.90 -  0.92 & 12.61 & 11.47 - 13.71 \\
3324 & KOI-2278 & 1.05 & 0.019 & 1.48 & 1.45 -  1.51 & 1.07 & 1.06 -  1.09 & 5.94 & 5.40 -  6.22 \\
3325 & KOI-3172 &  &  & 1.81 & 1.68 -  1.95 & 1.21 & 1.18 -  1.28 & 4.83 & 4.14 -  5.30 \\
3326 & KOI-2974 & 0.319 & 0.02 & 3.31 & 3.23 -  3.65 & 1.85 & 1.84 -  1.92 & 1.48 & 1.27 -  1.50 \\
3327 & KOI-384 & 0.914 & 0.015 & 2.21 & 2.17 -  2.26 & 1.39 & 1.38 -  1.44 & 3.35 & 3.06 -  3.53 \\
3328 & KOI-2740 & 0.804 & 0.021 & 1.99 & 1.96 -  2.02 & 1.30 & 1.30 -  1.31 & 2.95 & 2.87 -  3.05 \\
3329 & KOI-1196 & 0.722 & 0.024 & 1.28 & 1.24 -  1.32 & 0.92 & 0.90 -  0.93 & 9.96 & 9.44 - 10.52 \\
3330 & KOI-1845 & 2.32 & 0.019 & 0.81 & 0.80 -  0.82 & 0.80 & 0.80 -  0.82 & 12.48 & 9.90 - 14.19 \\
3331 & KOI-3075 & 2.74 & 0.014 & 0.83 & 0.82 -  0.83 & 0.74 & 0.73 -  0.74 & 14.77 & 14.41 - 14.94 \\
3332 & KOI-268 & 3.86 & 0.035 & 1.31 & 1.23 -  1.39 & 1.25 & 1.23 -  1.26 & 1.98 & 1.16 -  2.54 \\
3333 & KOI-2043 & 1.13 & 0.018 & 1.20 & 1.17 -  1.23 & 1.03 & 1.02 -  1.04 & 6.80 & 6.30 -  7.32 \\
3334 & KOI-3876 & 3.04 & 0.023 & 0.93 & 0.92 -  0.95 & 0.99 & 0.98 -  1.01 & 3.08 & 1.86 -  4.25 \\
3335 & KOI-1218 & 2.0 & 0.019 & 1.06 & 1.04 -  1.08 & 0.93 & 0.92 -  0.94 & 9.39 & 8.84 -  9.88 \\
3336 & KOI-385 & 2.26 & 0.017 & 0.93 & 0.91 -  0.94 & 0.91 & 0.90 -  0.92 & 7.92 & 6.52 -  9.26 \\
3337 & KOI-3415 & 1.9 & 0.055 & 1.56 & 1.53 -  1.59 & 0.83 & 0.83 -  0.83 & 14.91 & 14.82 - 14.97 \\
3338 & KOI-3340 & 0.741 & 0.066 & 1.63 & 1.55 -  1.71 & 1.19 & 1.17 -  1.24 & 4.26 & 3.78 -  4.59 \\
3339 & KOI-3641 & 0.798 & 0.048 & 1.70 & 1.64 -  1.78 & 1.27 & 1.21 -  1.28 & 3.37 & 3.19 -  4.15 \\
3340 & KOI-118 & 2.12 & 0.023 & 1.44 & 1.42 -  1.47 & 1.04 & 1.03 -  1.05 & 8.81 & 8.40 -  9.18 \\
3341 & KOI-2755 & 3.37 & 0.02 & 0.99 & 0.97 -  1.00 & 0.94 & 0.93 -  0.96 & 5.98 & 5.18 -  6.73 \\
3342 & KOI-2194 & 1.2 & 0.019 & 1.24 & 1.22 -  1.27 & 0.97 & 0.96 -  0.98 & 7.85 & 7.44 -  8.17 \\
3343 & KOI-6102 & 1.56 & 0.024 & 2.98 & 2.92 -  3.04 & 1.83 & 1.81 -  1.85 & 1.42 & 1.40 -  1.47 \\
3344 & KOI-624 & 1.99 & 0.017 & 0.93 & 0.92 -  0.95 & 0.95 & 0.94 -  0.96 & 5.29 & 3.98 -  6.53 \\
3345 & KOI-1221 & 2.23 & 0.032 & 2.96 & 2.90 -  3.01 & 1.17 & 1.13 -  1.20 & 7.30 & 6.61 -  8.27 \\
3346 & KOI-386 & 1.37 & 0.018 & 1.07 & 1.05 -  1.09 & 1.09 & 1.08 -  1.10 & 2.67 & 1.94 -  3.32 \\
3347 & KOI-975 & 9.19 & 0.032 & 1.97 & 1.94 -  2.01 & 1.38 & 1.37 -  1.39 & 3.19 & 3.11 -  3.30 \\
3348 & KOI-2279 & 1.19 & 0.018 & 1.24 & 1.22 -  1.27 & 1.07 & 1.06 -  1.08 & 6.05 & 5.60 -  6.57 \\
3349 & KOI-302 & 1.43 & 0.029 & 1.91 & 1.86 -  1.95 & 1.52 & 1.50 -  1.54 & 1.86 & 1.78 -  1.94 \\
3350 & KOI-1901 & 1.49 & 0.014 & 1.20 & 1.17 -  1.22 & 1.14 & 1.13 -  1.16 & 3.21 & 2.70 -  3.68 \\
3351 & KOI-1861 & 1.33 & 0.017 & 1.06 & 1.04 -  1.08 & 1.10 & 1.09 -  1.11 & 1.99 & 1.26 -  2.67 \\
3352 & KOI-3308 & 0.84 & 0.016 & 1.70 & 1.66 -  1.75 & 1.13 & 1.11 -  1.14 & 6.57 & 6.24 -  6.88 \\
3353 & KOI-301 & 1.58 & 0.028 & 1.50 & 1.47 -  1.53 & 1.13 & 1.11 -  1.14 & 5.40 & 5.11 -  5.85 \\
3354 & KOI-2808 & 0.375 & 0.076 & 1.60 & 1.52 -  1.69 & 1.38 & 1.36 -  1.41 & 1.99 & 1.80 -  2.12 \\
3355 & KOI-442 & 1.26 & 0.017 & 1.10 & 1.08 -  1.13 & 1.00 & 0.99 -  1.01 & 6.43 & 5.81 -  6.99 \\
3356 & KOI-2261 & 2.29 & 0.017 & 0.79 & 0.78 -  0.81 & 0.85 & 0.83 -  0.86 & 4.93 & 2.37 -  7.58 \\
3357 & KOI-1206 & 0.609 & 0.018 & 2.95 & 2.88 -  3.03 & 1.52 & 1.39 -  1.55 & 2.66 & 2.44 -  3.63 \\
3358 & KOI-3002 & 0.804 & 0.16 & 1.17 & 1.12 -  1.24 & 0.98 & 0.97 -  0.99 & 7.38 & 6.93 -  7.76 \\
3359 & KOI-388 & 1.08 & 0.013 & 1.91 & 1.88 -  1.94 & 1.25 & 1.20 -  1.27 & 4.88 & 4.49 -  5.54 \\
3360 & KOI-444 & 1.45 & 0.02 & 0.93 & 0.92 -  0.95 & 0.91 & 0.90 -  0.93 & 6.28 & 5.19 -  7.35 \\
3361 & KOI-149 & 1.07 & 0.015 & 2.07 & 2.03 -  2.10 & 1.14 & 1.13 -  1.15 & 6.71 & 6.55 -  7.13 \\
3362 & KOI-2289 & 1.34 & 0.013 & 1.38 & 1.35 -  1.40 & 1.13 & 1.10 -  1.15 & 5.63 & 5.13 -  6.44 \\
3363 & KOI-4423 & 0.952 & 0.019 & 1.93 & 1.88 -  1.98 & 1.37 & 1.36 -  1.38 & 2.81 & 2.69 -  2.92 \\
3364 & KOI-1216 & 1.05 & 0.017 & 1.70 & 1.66 -  1.74 & 1.15 & 1.15 -  1.17 & 5.23 & 4.78 -  5.55 \\
3365 & KOI-1208 & 0.468 & 0.071 & 2.49 & 2.35 -  2.63 & 1.52 & 1.48 -  1.57 & 2.37 & 2.19 -  2.54 \\
3366 & KOI-2904 & 1.33 & 0.053 & 1.89 & 1.82 -  1.97 & 1.41 & 1.38 -  1.43 & 3.04 & 2.93 -  3.15 \\
3367 & KOI-393 & 1.01 & 0.015 & 1.53 & 1.50 -  1.57 & 1.16 & 1.14 -  1.18 & 4.04 & 3.97 -  4.58 \\
3368 & KOI-3180 & 1.85 & 0.055 & 2.84 & 2.75 -  2.91 & 1.61 & 1.58 -  1.67 & 2.20 & 1.92 -  2.35 \\
3369 & KOI-392 & 0.931 & 0.024 & 1.62 & 1.57 -  1.67 & 1.20 & 1.16 -  1.24 & 5.06 & 4.55 -  5.91 \\
3370 & KOI-1336 & 1.0 & 0.025 & 0.99 & 0.97 -  1.02 & 1.00 & 0.99 -  1.02 & 4.36 & 2.97 -  5.67 \\
3371 & KOI-4887 & 0.966 & 0.022 & 2.33 & 2.26 -  2.39 & 1.35 & 1.31 -  1.40 & 3.80 & 3.35 -  4.02 \\
3372 & KOI-1222 & 1.24 & 0.024 & 3.68 & 3.61 -  3.76 & 1.33 & 1.28 -  1.38 & 4.30 & 3.84 -  4.83 \\
3373 & KOI-280 & 4.66 & 0.021 & 1.07 & 1.06 -  1.09 & 0.97 & 0.95 -  0.98 & 5.93 & 5.38 -  6.48 \\
3374 & KOI-1335 & 0.692 & 0.019 & 1.97 & 1.91 -  2.03 & 1.47 & 1.45 -  1.49 & 2.51 & 2.37 -  2.65 \\
3375 & KOI-2202 & 1.99 & 0.02 & 0.85 & 0.84 -  0.87 & 0.91 & 0.89 -  0.93 & 4.58 & 2.30 -  6.80 \\
3376 & KOI-1344 & 1.25 & 0.015 & 1.43 & 1.40 -  1.46 & 1.00 & 0.99 -  1.01 & 7.01 & 6.74 -  7.40 \\
3377 & KOI-281 & 2.56 & 0.025 & 1.45 & 1.43 -  1.48 & 0.90 & 0.89 -  0.91 & 10.75 & 10.23 - 11.23 \\
3378 & KOI-2866 & 0.56 & 0.042 & 1.74 & 1.66 -  1.83 & 1.37 & 1.34 -  1.40 & 2.87 & 2.77 -  2.97 \\
3379 & KOI-144 & 3.23 & 0.02 & 0.81 & 0.80 -  0.82 & 0.80 & 0.80 -  0.81 & 12.89 & 10.57 - 14.40 \\
3380 & KOI-3864 & 4.47 & 0.024 & 0.76 & 0.76 -  0.77 & 0.83 & 0.82 -  0.85 & 2.59 & 0.93 -  4.83 \\
3381 & KOI-3880 & 4.41 & 0.024 & 1.25 & 1.23 -  1.28 & 1.17 & 1.15 -  1.18 & 3.20 & 2.84 -  3.58 \\
3382 & KOI-1864 & 1.12 & 0.016 & 1.93 & 1.89 -  1.96 & 1.14 & 1.11 -  1.16 & 6.91 & 6.27 -  7.59 \\
3383 & KOI-3678 & 2.83 & 0.021 & 0.92 & 0.91 -  0.94 & 0.91 & 0.89 -  0.92 & 8.30 & 6.81 -  9.67 \\
3384 & KOI-551 & 0.924 & 0.025 & 1.07 & 1.04 -  1.10 & 0.99 & 0.98 -  1.00 & 6.94 & 5.89 -  7.87 \\
3385 & KOI-3202 & 2.08 & 0.024 & 2.39 & 2.36 -  2.44 & 1.07 & 1.02 -  1.12 & 8.65 & 7.36 - 10.03 \\
3386 & KOI-2311 & 2.15 & 0.023 & 1.35 & 1.33 -  1.37 & 1.00 & 0.99 -  1.01 & 10.34 & 9.87 - 10.80 \\
3387 & KOI-1619 & 8.37 & 0.027 & 0.72 & 0.71 -  0.72 & 0.69 & 0.69 -  0.70 & 14.60 & 13.96 - 14.89 \\
3388 & KOI-5048 & 0.627 & 0.015 & 4.69 & 4.59 -  4.81 & 1.33 & 1.26 -  1.41 & 4.35 & 3.62 -  5.18 \\
3389 & KOI-3358 & 1.92 & 0.018 & 0.87 & 0.85 -  0.88 & 0.81 & 0.80 -  0.82 & 11.22 & 9.69 - 12.66 \\
3390 & KOI-3928 & 1.47 & 0.012 & 1.34 & 1.32 -  1.37 & 1.15 & 1.13 -  1.16 & 4.32 & 3.89 -  4.63 \\
3391 & KOI-3528 & 0.99 & 0.021 & 3.08 & 2.99 -  3.15 & 1.52 & 1.51 -  1.57 & 2.02 & 1.87 -  2.15 \\
3392 & KOI-1615 & 3.41 & 0.022 & 1.33 & 1.31 -  1.35 & 1.20 & 1.19 -  1.21 & 3.50 & 3.24 -  3.77 \\
3393 & KOI-403 & 0.911 & 0.017 & 1.47 & 1.44 -  1.51 & 1.32 & 1.31 -  1.34 & 2.23 & 2.01 -  2.44 \\
3394 & KOI-4774 & 2.3 & 0.015 & 0.83 & 0.82 -  0.85 & 0.84 & 0.83 -  0.86 & 8.08 & 5.82 - 10.26 \\
3395 & KOI-5057 & 0.837 & 0.02 & 5.09 & 4.97 -  5.22 & 1.36 & 1.31 -  1.45 & 3.98 & 3.27 -  4.46 \\
3396 & KOI-2787 & 0.677 & 0.017 & 2.54 & 2.50 -  2.67 & 1.51 & 1.50 -  1.51 & 2.01 & 1.89 -  2.12 \\
3397 & KOI-1738 & 2.77 & 0.017 & 0.89 & 0.88 -  0.90 & 0.86 & 0.84 -  0.87 & 11.68 & 9.85 - 13.36 \\
3398 & KOI-3378 & 1.89 & 0.015 & 0.92 & 0.90 -  0.94 & 0.80 & 0.79 -  0.82 & 11.55 & 10.40 - 12.72 \\
3399 & KOI-1803 & 4.09 & 0.014 & 0.75 & 0.74 -  0.76 & 0.78 & 0.76 -  0.80 & 8.02 & 4.48 - 11.38 \\
3400 & KOI-4452 & 1.07 & 0.017 & 1.53 & 1.50 -  1.56 & 0.97 & 0.96 -  0.98 & 8.29 & 7.83 -  8.65 \\
3401 & KOI-3168 & 4.43 & 0.023 & 1.64 & 1.62 -  1.67 & 1.10 & 1.10 -  1.10 & 5.53 & 5.33 -  5.78 \\
3402 & KOI-626 & 1.31 & 0.021 & 1.25 & 1.22 -  1.28 & 1.04 & 1.03 -  1.05 & 5.70 & 5.39 -  6.04 \\
3403 & KOI-1338 & 1.13 & 0.018 & 1.00 & 0.97 -  1.02 & 0.90 & 0.89 -  0.91 & 8.18 & 7.26 -  9.06 \\
3404 & KOI-1332 & 0.809 & 0.023 & 1.04 & 1.01 -  1.08 & 0.90 & 0.89 -  0.91 & 8.97 & 8.16 -  9.68 \\
3405 & KOI-2547 & 1.14 & 0.023 & 1.16 & 1.14 -  1.19 & 1.05 & 1.04 -  1.06 & 5.03 & 4.51 -  5.52 \\
3406 & KOI-4288 & 2.0 & 0.024 & 1.43 & 1.40 -  1.46 & 1.10 & 1.09 -  1.12 & 6.48 & 6.05 -  6.89 \\
3407 & KOI-3181 & 2.65 & 0.033 & 2.54 & 2.49 -  2.59 & 1.28 & 1.23 -  1.35 & 4.81 & 4.09 -  5.50 \\
3408 & KOI-627 & 1.29 & 0.017 & 1.48 & 1.45 -  1.51 & 1.19 & 1.14 -  1.20 & 4.82 & 4.55 -  5.82 \\
3409 & KOI-4157 & 1.76 & 0.023 & 1.28 & 1.25 -  1.30 & 1.18 & 1.17 -  1.19 & 3.09 & 2.74 -  3.46 \\
3410 & KOI-2025 & 1.02 & 0.021 & 1.42 & 1.38 -  1.46 & 1.27 & 1.26 -  1.29 & 2.44 & 2.24 -  2.64 \\
3411 & Kepler-350 & 1.02 & 0.021 & 1.43 & 1.39 -  1.47 & 1.25 & 1.24 -  1.27 & 2.85 & 2.66 -  3.00 \\
3412 & KOI-628 & 1.54 & 0.016 & 0.98 & 0.97 -  1.00 & 0.85 & 0.84 -  0.86 & 9.98 & 9.08 - 10.89 \\
3413 & KOI-3811 & 1.13 & 0.017 & 1.43 & 1.41 -  1.46 & 1.10 & 1.10 -  1.11 & 5.56 & 5.31 -  5.81 \\
3414 & KOI-629 & 0.987 & 0.017 & 1.36 & 1.33 -  1.39 & 1.02 & 1.00 -  1.03 & 6.58 & 6.30 -  6.95 \\
3415 & KOI-1805 & 1.96 & 0.019 & 0.88 & 0.86 -  0.89 & 0.92 & 0.91 -  0.94 & 4.34 & 2.73 -  5.90 \\
3416 & KOI-2393 & 1.97 & 0.033 & 0.74 & 0.73 -  0.75 & 0.73 & 0.73 -  0.75 & 13.01 & 10.27 - 14.41 \\
3417 & KOI-1534 & 1.1 & 0.016 & 1.45 & 1.42 -  1.48 & 1.21 & 1.20 -  1.23 & 3.83 & 3.65 -  4.10 \\
3418 & KOI-3184 & 3.45 & 0.025 & 1.48 & 1.45 -  1.50 & 1.12 & 1.10 -  1.17 & 6.54 & 5.48 -  7.12 \\
3419 & KOI-4367 & 0.831 & 0.018 & 1.58 & 1.54 -  1.62 & 1.24 & 1.20 -  1.27 & 3.62 & 3.38 -  4.47 \\
3420 & KOI-4004 & 3.02 & 0.02 & 0.92 & 0.91 -  0.94 & 0.98 & 0.97 -  1.00 & 2.86 & 1.74 -  4.03 \\
3421 & KOI-2120 & 3.19 & 0.016 & 0.74 & 0.73 -  0.75 & 0.78 & 0.76 -  0.80 & 6.11 & 2.86 -  9.21 \\
3422 & KOI-4639 & 0.898 & 0.035 & 3.29 & 3.20 -  3.37 & 1.95 & 1.90 -  1.97 & 1.22 & 1.19 -  1.29 \\
3423 & KOI-633 & 1.16 & 0.017 & 1.37 & 1.34 -  1.40 & 1.02 & 1.00 -  1.04 & 6.99 & 6.64 -  7.42 \\
3424 & KOI-632 & 2.66 & 0.014 & 0.86 & 0.84 -  0.87 & 0.88 & 0.87 -  0.89 & 6.88 & 4.86 -  8.80 \\
3425 & KOI-232 & 0.945 & 0.018 & 1.28 & 1.25 -  1.31 & 1.08 & 1.06 -  1.09 & 5.43 & 5.10 -  5.79 \\
3426 & Kepler-122 & 0.945 & 0.018 & 1.34 & 1.30 -  1.37 & 1.07 & 1.06 -  1.09 & 6.09 & 5.74 -  6.41 \\
3427 & KOI-3823 & 1.68 & 0.015 & 0.93 & 0.92 -  0.95 & 0.95 & 0.94 -  0.97 & 5.03 & 3.66 -  6.31 \\
3428 & KOI-3936 & 3.6 & 0.015 & 0.79 & 0.78 -  0.80 & 0.82 & 0.80 -  0.83 & 8.46 & 5.53 - 11.11 \\
3429 & KOI-1665 & 0.971 & 0.02 & 1.38 & 1.34 -  1.41 & 1.21 & 1.20 -  1.23 & 3.68 & 3.46 -  3.90 \\
3430 & KOI-4018 & 1.34 & 0.025 & 0.86 & 0.84 -  0.88 & 0.88 & 0.87 -  0.90 & 5.80 & 3.68 -  7.84 \\
3431 & KOI-2635 & 1.26 & 0.024 & 1.90 & 1.87 -  1.94 & 1.27 & 1.20 -  1.28 & 3.34 & 3.22 -  4.45 \\
3432 & KOI-5107 & 0.336 & 0.015 & 7.25 & 7.02 -  7.50 & 1.49 & 1.45 -  1.52 & 2.91 & 2.66 -  3.16 \\
3433 & KOI-3770 & 0.345 & 0.039 & 2.27 & 2.17 -  2.39 & 1.44 & 1.40 -  1.47 & 3.01 & 2.77 -  3.24 \\
3434 & KOI-5119 & 0.606 & 0.033 & 6.52 & 6.28 -  6.76 & 1.46 & 1.45 -  1.53 & 3.34 & 2.85 -  3.39 \\
3435 & KOI-4546 & 1.32 & 0.021 & 1.34 & 1.31 -  1.37 & 1.11 & 1.10 -  1.12 & 5.53 & 5.20 -  5.88 \\
3436 & KOI-2951 & 1.57 & 0.19 & 0.97 & 0.92 -  1.02 & 0.87 & 0.86 -  0.89 & 9.27 & 7.49 - 10.57 \\
3437 & KOI-3421 & 0.732 & 0.017 & 1.78 & 1.73 -  1.83 & 1.35 & 1.34 -  1.37 & 3.15 & 3.06 -  3.24 \\
3438 & KOI-1666 & 0.694 & 0.021 & 1.34 & 1.30 -  1.38 & 1.30 & 1.28 -  1.31 & 1.53 & 1.10 -  1.90 \\
3439 & KOI-635 & 1.76 & 0.017 & 1.14 & 1.12 -  1.16 & 1.14 & 1.13 -  1.15 & 2.19 & 1.61 -  2.73 \\
3440 & KOI-161 & 3.54 & 0.015 & 0.82 & 0.81 -  0.83 & 0.83 & 0.82 -  0.85 & 9.79 & 6.96 - 12.25 \\
3441 & KOI-639 & 1.28 & 0.018 & 1.26 & 1.23 -  1.29 & 1.17 & 1.16 -  1.18 & 3.18 & 2.79 -  3.60 \\
3442 & KOI-3093 & 1.21 & 0.11 & 1.18 & 1.13 -  1.24 & 1.05 & 1.04 -  1.07 & 5.84 & 5.08 -  6.52 \\
3443 & Kepler-130 & 3.13 & 0.023 & 1.14 & 1.12 -  1.15 & 1.04 & 1.03 -  1.05 & 4.72 & 4.29 -  5.14 \\
3444 & KOI-282 & 3.13 & 0.023 & 1.15 & 1.14 -  1.18 & 0.99 & 0.98 -  1.00 & 6.66 & 6.21 -  7.07 \\
3445 & KOI-4331 &  &  & 1.62 & 1.50 -  1.76 & 1.32 & 1.29 -  1.37 & 2.83 & 2.70 -  2.94 \\
3446 & KOI-1822 & 2.53 & 0.029 & 1.08 & 1.06 -  1.10 & 1.03 & 1.02 -  1.04 & 4.05 & 3.45 -  4.63 \\
3447 & KOI-640 &  &  & 0.88 & 0.85 -  0.91 & 0.85 & 0.84 -  0.87 & 11.28 & 7.35 - 13.82 \\
3448 & KOI-2698 & 1.22 & 0.015 & 1.23 & 1.20 -  1.25 & 1.07 & 1.06 -  1.08 & 6.01 & 5.56 -  6.52 \\
3449 & KOI-1563 & 1.12 & 0.034 & 0.81 & 0.80 -  0.83 & 0.80 & 0.79 -  0.81 & 12.87 & 10.03 - 14.39 \\
3450 & KOI-3474 & -3.02 & 0.53 & 1.31 & 1.22 -  1.40 & 1.04 & 1.02 -  1.06 & 6.18 & 5.73 -  6.58 \\
3451 & KOI-2158 & 2.82 & 0.017 & 0.95 & 0.94 -  0.97 & 0.82 & 0.82 -  0.83 & 14.05 & 13.26 - 14.63 \\
3452 & KOI-2563 & 0.64 & 0.016 & 2.09 & 2.04 -  2.14 & 1.41 & 1.39 -  1.43 & 3.32 & 3.17 -  3.45 \\
3453 & KOI-4246 & 2.14 & 0.013 & 0.96 & 0.94 -  0.98 & 1.00 & 0.98 -  1.01 & 4.05 & 2.83 -  5.22 \\
3454 & KOI-1576 & 1.71 & 0.016 & 0.97 & 0.95 -  0.99 & 0.91 & 0.90 -  0.93 & 9.54 & 8.27 - 10.75 \\
3455 & KOI-825 & 1.49 & 0.024 & 0.79 & 0.78 -  0.80 & 0.79 & 0.78 -  0.80 & 12.41 & 9.32 - 14.27 \\
3456 & KOI-4713 & 0.923 & 0.025 & 1.00 & 0.98 -  1.03 & 1.09 & 1.07 -  1.10 & 0.90 & 0.42 -  1.85 \\
3457 & KOI-4411 & 1.56 & 0.014 & 1.13 & 1.11 -  1.15 & 1.02 & 1.01 -  1.03 & 5.28 & 4.77 -  5.76 \\
3458 & KOI-3239 & 3.72 & 0.022 & 0.90 & 0.89 -  0.92 & 0.95 & 0.93 -  0.96 & 4.12 & 2.68 -  5.46 \\
3459 & KOI-2711 &  &  & 1.03 & 0.99 -  1.08 & 1.07 & 1.05 -  1.08 & 2.61 & 1.13 -  4.14 \\
3460 & KOI-1589 & 0.693 & 0.7 & 1.02 & 0.99 -  1.05 & 1.08 & 1.07 -  1.10 & 1.15 & 0.50 -  2.28 \\
3461 & KOI-408 & 1.09 & 0.021 & 0.96 & 0.95 -  0.98 & 1.08 & 1.06 -  1.09 & 0.43 & 0.30 -  0.71 \\
3462 & KOI-644 & 1.42 & 0.019 & 1.38 & 1.35 -  1.40 & 1.03 & 1.02 -  1.05 & 6.84 & 6.39 -  7.18 \\
3463 & KOI-2370 & 1.4 & 0.022 & 1.36 & 1.34 -  1.39 & 1.19 & 1.18 -  1.21 & 3.13 & 2.89 -  3.34 \\
3464 & KOI-2555 & 1.83 & 0.024 & 1.16 & 1.14 -  1.19 & 1.09 & 1.08 -  1.11 & 3.67 & 3.19 -  4.14 \\
3465 & KOI-2011 & 1.72 & 0.024 & 1.35 & 1.33 -  1.38 & 1.22 & 1.20 -  1.23 & 2.86 & 2.61 -  3.08 \\
3466 & KOI-2219 & 2.41 & 0.02 & 0.79 & 0.77 -  0.80 & 0.79 & 0.78 -  0.81 & 11.39 & 6.75 - 13.97 \\
3467 & KOI-1825 & 2.17 & 0.022 & 0.84 & 0.83 -  0.86 & 0.88 & 0.87 -  0.90 & 5.50 & 3.29 -  7.73 \\
3468 & KOI-2440 & 1.13 & 0.018 & 1.39 & 1.36 -  1.43 & 1.04 & 1.03 -  1.06 & 9.21 & 8.67 -  9.73 \\
3469 & KOI-1557 & 2.27 & 0.028 & 0.71 & 0.70 -  0.72 & 0.76 & 0.74 -  0.78 & 3.30 & 1.04 -  6.78 \\
3470 & KOI-829 & 0.704 & 0.033 & 1.06 & 1.02 -  1.11 & 1.03 & 1.01 -  1.04 & 4.83 & 3.50 -  5.94 \\
3471 & KOI-2556 & 1.77 & 0.018 & 0.87 & 0.86 -  0.89 & 0.84 & 0.82 -  0.85 & 9.01 & 7.62 - 10.38 \\
3472 & KOI-2690 & 2.43 & 0.016 & 0.88 & 0.87 -  0.90 & 0.90 & 0.89 -  0.91 & 6.86 & 5.16 -  8.57 \\
3473 & KOI-645 & 1.04 & 0.016 & 1.75 & 1.71 -  1.81 & 1.10 & 1.09 -  1.13 & 5.37 & 4.92 -  5.60 \\
3474 & KOI-3039 & 0.98 & 0.017 & 1.58 & 1.55 -  1.61 & 1.00 & 0.98 -  1.00 & 7.53 & 7.22 -  8.03 \\
3475 & KOI-1567 & 1.26 & 0.03 & 0.76 & 0.75 -  0.77 & 0.74 & 0.73 -  0.75 & 13.77 & 11.89 - 14.69 \\
3476 & KOI-4907 & 1.18 & 0.017 & 1.28 & 1.25 -  1.31 & 1.10 & 1.09 -  1.11 & 5.30 & 4.96 -  5.65 \\
3477 & KOI-834 & 0.527 & 0.022 & 1.75 & 1.68 -  1.82 & 1.19 & 1.15 -  1.27 & 6.02 & 4.95 -  6.79 \\
3478 & KOI-3791 & 0.756 & 0.017 & 1.90 & 1.85 -  1.95 & 1.37 & 1.36 -  1.39 & 3.21 & 3.11 -  3.31 \\
3479 & KOI-1601 & 0.702 & 0.02 & 1.65 & 1.61 -  1.70 & 1.03 & 1.01 -  1.05 & 7.14 & 6.67 -  7.62 \\
3480 & KOI-2970 & 1.86 & 0.024 & 1.17 & 1.15 -  1.20 & 1.10 & 1.09 -  1.11 & 3.64 & 3.17 -  4.06 \\
3481 & KOI-142 & 2.62 & 0.014 & 0.95 & 0.93 -  0.96 & 0.91 & 0.90 -  0.92 & 9.27 & 7.91 - 10.62 \\
3482 & KOI-2707 & 0.734 & 0.11 & 1.05 & 1.00 -  1.11 & 0.91 & 0.89 -  0.92 & 9.63 & 8.67 - 10.27 \\
3483 & Kepler-399 & 0.734 & 0.11 & 1.05 & 1.00 -  1.10 & 0.88 & 0.87 -  0.89 & 11.01 & 10.23 - 11.62 \\
3484 & KOI-4368 & 0.929 & 0.014 & 2.44 & 2.38 -  2.49 & 1.39 & 1.35 -  1.44 & 3.47 & 3.09 -  3.77 \\
3485 & KOI-409 & 1.19 & 0.018 & 1.10 & 1.08 -  1.13 & 1.05 & 1.04 -  1.07 & 4.94 & 4.20 -  5.65 \\
3486 & KOI-647 & 1.1 & 0.015 & 1.50 & 1.47 -  1.53 & 0.99 & 0.98 -  1.01 & 7.23 & 6.87 -  7.53 \\
3487 & KOI-2741 & 2.12 & 0.019 & 1.05 & 1.03 -  1.07 & 1.03 & 1.02 -  1.05 & 4.26 & 3.49 -  5.02 \\
3488 & KOI-257 & 4.35 & 0.026 & 1.23 & 1.21 -  1.25 & 1.19 & 1.18 -  1.20 & 2.30 & 1.96 -  2.65 \\
3489 & KOI-1590 & 1.37 & 0.16 & 0.75 & 0.74 -  0.77 & 0.77 & 0.75 -  0.79 & 9.99 & 4.52 - 13.55 \\
3490 & KOI-2854 E & 0.871 & 0.018 &  &  &  &  &  &  \\
3491 & KOI-2854 W & 0.792 & 0.027 &  &  &  &  &  &  \\
3492 & KOI-2668 & 1.73 & 0.021 & 0.89 & 0.88 -  0.91 & 0.87 & 0.86 -  0.88 & 8.15 & 6.68 -  9.51 \\
3493 & KOI-837 & 1.31 & 0.035 & 0.82 & 0.80 -  0.84 & 0.82 & 0.81 -  0.84 & 10.53 & 6.60 - 13.45 \\
3494 & KOI-1621 & 1.77 & 0.026 & 2.00 & 1.97 -  2.05 & 1.37 & 1.34 -  1.38 & 3.52 & 3.40 -  3.73 \\
3495 & KOI-4067 & 1.08 & 0.019 & 1.17 & 1.14 -  1.19 & 1.08 & 1.07 -  1.09 & 4.62 & 4.07 -  5.12 \\
3496 & Kepler-338 & 1.78 & 0.022 & 1.82 & 1.78 -  1.85 & 1.15 & 1.13 -  1.17 & 6.00 & 5.71 -  6.34 \\
3497 & KOI-1930 & 1.78 & 0.022 & 1.84 & 1.81 -  1.88 & 1.11 & 1.10 -  1.12 & 6.33 & 6.04 -  6.70 \\
3498 & KOI-2332 & 1.43 & 0.017 & 2.01 & 1.98 -  2.05 & 0.89 & 0.88 -  0.90 & 12.86 & 12.39 - 13.96 \\
3499 & KOI-1962 & 0.908 & 0.33 & 2.07 & 1.92 -  2.22 & 1.26 & 1.15 -  1.28 & 3.75 & 3.63 -  5.24 \\
3500 & KOI-649 & 0.848 & 0.018 & 2.20 & 2.15 -  2.26 & 1.50 & 1.48 -  1.52 & 2.69 & 2.60 -  2.84 \\
3501 & KOI-2915 & 2.03 & 0.016 & 0.94 & 0.93 -  0.96 & 0.91 & 0.90 -  0.93 & 7.20 & 6.07 -  8.22 \\
3502 & KOI-2790 &  &  & 0.77 & 0.75 -  0.78 & 0.74 & 0.73 -  0.75 & 13.19 & 10.43 - 14.50 \\
3503 & KOI-371 & 1.34 & 0.029 & 3.41 & 3.34 -  3.49 & 1.32 & 1.28 -  1.37 & 4.32 & 3.85 -  4.75 \\
3504 & KOI-2369 & 0.518 & 0.036 & 1.26 & 1.20 -  1.33 & 1.02 & 1.00 -  1.04 & 8.40 & 7.70 -  9.05 \\
3505 & KOI-2676 & 0.709 & 0.02 & 2.55 & 2.48 -  2.62 & 1.57 & 1.53 -  1.58 & 2.25 & 2.21 -  2.45 \\
3506 & KOI-2010 & 1.18 & 0.015 & 1.50 & 1.47 -  1.53 & 1.27 & 1.26 -  1.29 & 3.00 & 2.87 -  3.15 \\
3507 & KOI-2752 & 2.54 & 0.26 & 1.43 & 1.35 -  1.52 & 1.21 & 1.19 -  1.24 & 4.01 & 3.80 -  4.20 \\
3508 & KOI-2183 & 0.828 & 0.026 & 1.07 & 1.04 -  1.11 & 0.94 & 0.93 -  0.96 & 9.78 & 8.65 - 10.84 \\
3509 & KOI-505 & 2.43 & 0.018 & 0.77 & 0.76 -  0.78 & 0.83 & 0.82 -  0.85 & 4.59 & 1.94 -  7.59 \\
3510 & Kepler-169 & 2.43 & 0.018 & 0.79 & 0.78 -  0.79 & 0.78 & 0.77 -  0.79 & 12.73 & 10.11 - 14.31 \\
3511 & KOI-555 & 1.44 & 0.023 & 0.88 & 0.86 -  0.90 & 0.83 & 0.82 -  0.84 & 12.96 & 10.97 - 14.34 \\
3512 & KOI-4744 & 1.06 & 0.016 & 1.52 & 1.49 -  1.55 & 1.09 & 1.08 -  1.11 & 7.66 & 7.19 -  8.09 \\
3513 & KOI-2358 & 0.918 & 0.017 & 1.76 & 1.72 -  1.81 & 1.33 & 1.32 -  1.35 & 3.54 & 3.40 -  3.70 \\
3514 & KOI-1897 & 1.2 & 0.018 & 1.20 & 1.17 -  1.22 & 1.01 & 1.00 -  1.02 & 6.78 & 6.38 -  7.15 \\
3515 & KOI-2675 & 3.31 & 0.025 & 0.93 & 0.91 -  0.94 & 1.00 & 0.98 -  1.01 & 2.52 & 1.39 -  3.66 \\
3516 & KOI-3288 & 1.81 & 0.016 & 0.85 & 0.83 -  0.86 & 0.89 & 0.87 -  0.91 & 5.14 & 3.06 -  7.19 \\
3517 & KOI-650 & 2.95 & 0.014 & 0.82 & 0.81 -  0.83 & 0.79 & 0.79 -  0.81 & 13.12 & 11.21 - 14.41 \\
3518 & KOI-1928 & 1.51 & 0.014 & 1.14 & 1.12 -  1.16 & 1.04 & 1.03 -  1.05 & 6.28 & 5.66 -  6.87 \\
3519 & KOI-4686 & 1.7 & 0.024 & 2.01 & 1.98 -  2.06 & 1.30 & 1.24 -  1.32 & 4.89 & 4.49 -  5.50 \\
3520 & KOI-4002 & 1.37 & 0.025 & 0.85 & 0.83 -  0.87 & 0.85 & 0.83 -  0.86 & 10.06 & 7.02 - 12.65 \\
3521 & KOI-652 & 1.98 & 0.029 & 1.13 & 1.08 -  1.15 & 0.86 & 0.85 -  0.88 & 14.72 & 14.38 - 14.93 \\
3522 & KOI-4913 & 1.13 & 0.014 & 1.45 & 1.42 -  1.48 & 1.28 & 1.26 -  1.29 & 2.71 & 2.54 -  2.89 \\
3523 & KOI-3422 & 1.98 & 0.019 & 1.07 & 1.06 -  1.09 & 1.04 & 1.03 -  1.05 & 4.90 & 4.18 -  5.62 \\
3524 & KOI-4156 & 0.967 & 0.017 & 1.69 & 1.65 -  1.73 & 1.20 & 1.15 -  1.25 & 5.53 & 4.94 -  6.59 \\
3525 & KOI-1060 & 0.637 & 0.019 & 1.55 & 1.50 -  1.60 & 1.22 & 1.20 -  1.24 & 3.30 & 3.08 -  3.47 \\
3526 & Kepler-758 & 0.637 & 0.019 & 1.57 & 1.48 -  1.66 & 1.22 & 1.20 -  1.25 & 3.42 & 3.21 -  3.55 \\
3527 & KOI-2801 & 3.82 & 0.026 & 1.53 & 1.50 -  1.55 & 1.14 & 1.12 -  1.15 & 5.90 & 5.49 -  6.25 \\
3528 & KOI-1839 & 2.93 & 0.057 & 0.86 & 0.84 -  0.87 & 0.94 & 0.93 -  0.95 & 2.24 & 0.91 -  4.05 \\
3529 & KOI-2498 & 2.27 & 0.019 & 0.83 & 0.82 -  0.84 & 0.77 & 0.77 -  0.78 & 13.86 & 12.46 - 14.68 \\
3530 & KOI-4633 & 0.929 & 0.015 & 1.68 & 1.65 -  1.72 & 1.20 & 1.16 -  1.22 & 5.07 & 4.77 -  5.91 \\
3531 & KOI-654 & 1.47 & 0.016 & 1.01 & 0.99 -  1.02 & 1.01 & 0.99 -  1.02 & 4.29 & 3.36 -  5.17 \\
3532 & KOI-1052 & 0.753 & 0.028 & 1.03 & 1.00 -  1.07 & 1.02 & 1.00 -  1.04 & 4.10 & 2.73 -  5.20 \\
3533 & KOI-3190 & 2.42 & 0.026 & 1.19 & 1.17 -  1.21 & 1.06 & 1.05 -  1.07 & 4.78 & 4.37 -  5.17 \\
3534 & KOI-655 & 1.54 & 0.024 & 1.31 & 1.29 -  1.34 & 1.14 & 1.13 -  1.16 & 4.26 & 3.87 -  4.58 \\
3535 & KOI-2479 & 1.25 & 0.023 & 2.32 & 2.27 -  2.37 & 1.13 & 1.09 -  1.21 & 7.07 & 5.40 -  8.16 \\
3536 & KOI-2250 & 1.35 & 0.028 & 0.79 & 0.77 -  0.80 & 0.78 & 0.77 -  0.79 & 12.98 & 10.29 - 14.41 \\
3537 & KOI-303 & 3.42 & 0.024 & 1.02 & 1.00 -  1.03 & 0.87 & 0.86 -  0.88 & 10.27 & 9.58 - 10.96 \\
3538 & KOI-2733 & 1.76 & 0.36 & 0.74 & 0.73 -  0.75 & 0.74 & 0.73 -  0.75 & 13.55 & 11.24 - 14.63 \\
3539 & KOI-2148 & 1.28 & 0.012 & 1.71 & 1.67 -  1.74 & 1.13 & 1.12 -  1.15 & 7.35 & 7.02 -  7.69 \\
3540 & Kepler-363 & 1.28 & 0.012 & 1.72 & 1.69 -  1.75 & 1.13 & 1.11 -  1.14 & 7.60 & 7.26 -  7.96 \\
3541 & KOI-1054 & 0.552 & 0.02 & 7.33 & 7.13 -  7.53 & 1.50 & 1.45 -  1.51 & 1.87 & 1.85 -  2.09 \\
3542 & KOI-2167 & 0.817 & 0.03 & 0.97 & 0.94 -  1.00 & 1.01 & 0.99 -  1.02 & 3.49 & 1.82 -  5.16 \\
3543 & KOI-2071 & 2.35 & 0.016 & 0.87 & 0.85 -  0.88 & 0.85 & 0.84 -  0.87 & 10.49 & 8.44 - 12.43 \\
3544 & KOI-1684 & 1.09 & 0.025 & 1.77 & 1.73 -  1.81 & 1.38 & 1.36 -  1.39 & 2.50 & 2.40 -  2.58 \\
3545 & KOI-1916 & 0.429 & 0.38 & 1.15 & 1.08 -  1.22 & 1.10 & 1.08 -  1.12 & 4.20 & 2.87 -  5.05 \\
3546 & Kepler-336 & 0.429 & 0.38 & 1.16 & 1.09 -  1.23 & 1.06 & 1.05 -  1.08 & 5.75 & 4.62 -  6.54 \\
3547 & KOI-2949 & 1.33 & 0.014 & 1.43 & 1.40 -  1.46 & 1.08 & 1.06 -  1.09 & 7.30 & 6.89 -  7.67 \\
3548 & KOI-3500 & 0.888 & 0.02 & 2.19 & 2.13 -  2.25 & 1.41 & 1.39 -  1.44 & 3.47 & 3.24 -  3.59 \\
3549 & Kepler-132 & 3.62 & 0.29 & 1.06 & 1.01 -  1.11 & 0.97 & 0.96 -  0.98 & 5.92 & 4.76 -  6.77 \\
3550 & KOI-284 & 3.62 & 0.29 & 1.06 & 1.01 -  1.11 & 1.00 & 0.99 -  1.01 & 4.97 & 3.69 -  5.93 \\
3551 & KOI-4276 & 0.97 & 0.024 & 2.55 & 2.47 -  2.62 & 1.57 & 1.54 -  1.60 & 2.40 & 2.24 -  2.64 \\
3552 & KOI-304 & 2.93 & 0.025 & 0.94 & 0.92 -  0.95 & 0.96 & 0.95 -  0.97 & 3.75 & 2.78 -  4.69 \\
3553 & KOI-2001 & 3.76 & 0.017 & 0.80 & 0.79 -  0.81 & 0.82 & 0.80 -  0.83 & 8.91 & 5.99 - 11.56 \\
3554 & KOI-306 & 4.03 & 0.024 & 0.86 & 0.85 -  0.87 & 0.86 & 0.85 -  0.88 & 9.06 & 6.92 - 11.04 \\
3555 & Kepler-203 & 1.39 & 0.019 & 1.07 & 1.04 -  1.09 & 1.05 & 1.04 -  1.06 & 4.06 & 3.26 -  4.83 \\
3556 & KOI-659 & 1.24 & 0.015 & 1.30 & 1.27 -  1.32 & 1.21 & 1.20 -  1.22 & 2.56 & 2.26 -  2.83 \\
3557 & KOI-2098 & 0.903 & 0.018 & 1.52 & 1.49 -  1.56 & 1.23 & 1.22 -  1.24 & 3.45 & 3.27 -  3.59 \\
3558 & KOI-3179 & 3.68 & 0.027 & 0.95 & 0.93 -  0.96 & 0.99 & 0.97 -  1.00 & 3.80 & 2.69 -  4.92 \\
3559 & KOI-4123 & 0.693 & 0.02 & 2.48 & 2.41 -  2.54 & 1.54 & 1.50 -  1.55 & 2.67 & 2.44 -  2.76 \\
3560 & KOI-2398 & 0.941 & 0.014 & 1.66 & 1.63 -  1.70 & 1.13 & 1.12 -  1.16 & 4.68 & 4.27 -  4.86 \\
3561 & KOI-2829 & 1.57 & 0.022 & 1.51 & 1.48 -  1.54 & 1.08 & 1.07 -  1.09 & 7.15 & 6.74 -  7.50 \\
3562 & Kepler-92 & 2.06 & 0.023 & 1.84 & 1.80 -  1.87 & 1.31 & 1.30 -  1.32 & 4.10 & 3.96 -  4.23 \\
3563 & KOI-285 & 2.06 & 0.023 & 1.84 & 1.80 -  1.87 & 1.30 & 1.28 -  1.32 & 4.23 & 4.07 -  4.43 \\
3564 & KOI-2252 & 0.645 & 0.017 & 2.37 & 2.31 -  2.43 & 1.52 & 1.50 -  1.54 & 2.67 & 2.61 -  2.72 \\
3565 & KOI-3240 & 1.3 & 0.027 & 2.67 & 2.61 -  2.71 & 1.64 & 1.63 -  1.65 & 2.22 & 2.16 -  2.25 \\
3566 & KOI-2636 & 3.32 & 0.021 & 1.02 & 1.01 -  1.04 & 1.04 & 1.02 -  1.05 & 3.60 & 2.81 -  4.37 \\
3567 & KOI-1812 & 1.18 & 0.015 & 1.31 & 1.28 -  1.34 & 1.10 & 1.09 -  1.11 & 5.43 & 5.13 -  5.75 \\
3568 & KOI-308 & 1.89 & 0.057 & 1.51 & 1.47 -  1.55 & 1.21 & 1.19 -  1.23 & 4.24 & 3.92 -  4.55 \\
3569 & KOI-2608 & 1.4 & 0.091 & 1.73 & 1.64 -  1.81 & 1.27 & 1.24 -  1.32 & 3.92 & 3.48 -  4.21 \\
3570 & KOI-415 & 1.04 & 0.016 & 1.26 & 1.23 -  1.29 & 0.95 & 0.94 -  0.96 & 8.53 & 8.19 -  8.93 \\
3571 & KOI-4302 & 0.993 & 0.018 & 1.55 & 1.51 -  1.58 & 1.17 & 1.15 -  1.18 & 4.37 & 4.18 -  4.62 \\
3572 & KOI-1688 & 0.734 & 0.02 & 1.66 & 1.61 -  1.70 & 1.24 & 1.19 -  1.27 & 4.53 & 4.32 -  5.33 \\
3573 & KOI-660 & 0.98 & 0.016 & 2.23 & 2.19 -  2.28 & 0.96 & 0.96 -  0.97 & 9.44 & 9.29 -  9.86 \\
3574 & KOI-307 & 1.34 & 0.12 & 1.28 & 1.23 -  1.35 & 1.05 & 1.04 -  1.08 & 5.72 & 5.37 -  6.04 \\
3575 & KOI-1613 & 4.6 & 0.95 & 1.10 & 1.04 -  1.17 & 1.01 & 0.99 -  1.02 & 4.76 & 3.57 -  5.61 \\
3576 & KOI-3436 & 3.2 & 0.016 & 0.82 & 0.80 -  0.83 & 0.81 & 0.80 -  0.83 & 11.61 & 8.96 - 13.76 \\
3577 & KOI-219 & 0.549 & 0.27 & 1.60 & 1.48 -  1.72 & 1.23 & 1.19 -  1.27 & 4.37 & 4.13 -  4.65 \\
3578 & KOI-611 & 0.929 & 0.016 & 1.37 & 1.33 -  1.40 & 1.23 & 1.22 -  1.24 & 2.94 & 2.67 -  3.14 \\
3579 & KOI-2753 & 1.3 & 0.019 & 1.34 & 1.31 -  1.37 & 1.07 & 1.05 -  1.09 & 7.47 & 6.71 -  7.98 \\
3580 & KOI-1128 & 2.48 & 0.013 & 0.86 & 0.85 -  0.88 & 0.85 & 0.83 -  0.86 & 8.88 & 7.18 - 10.39 \\
3581 & KOI-662 & 1.15 & 0.015 & 1.66 & 1.63 -  1.70 & 1.13 & 1.12 -  1.14 & 6.51 & 6.23 -  6.81 \\
3582 & KOI-3503 & 1.1 & 0.016 & 1.29 & 1.27 -  1.32 & 0.93 & 0.92 -  0.94 & 8.60 & 8.22 -  8.97 \\
3583 & KOI-661 & 1.43 & 0.015 & 1.03 & 1.01 -  1.05 & 1.04 & 1.03 -  1.05 & 3.48 & 2.63 -  4.34 \\
3584 & KOI-1121 & 1.57 & 0.021 & 1.56 & 1.53 -  1.59 & 1.09 & 1.08 -  1.10 & 7.37 & 7.07 -  7.67 \\
3585 & KOI-1127 & 0.413 & 0.034 & 1.71 & 1.61 -  1.81 & 1.14 & 1.10 -  1.21 & 7.24 & 5.80 -  8.11 \\
3586 & KOI-2857 & 0.967 & 0.016 & 1.58 & 1.54 -  1.61 & 1.30 & 1.29 -  1.32 & 3.33 & 3.17 -  3.48 \\
3587 & KOI-2948 & 2.45 & 0.028 & 1.68 & 1.65 -  1.71 & 1.12 & 1.11 -  1.14 & 7.49 & 7.15 -  7.86 \\
3588 & KOI-3456 & 1.99 & 0.033 & 1.18 & 1.16 -  1.20 & 0.87 & 0.86 -  0.88 & 11.96 & 11.47 - 12.52 \\
3589 & KOI-1230 & 0.733 & 0.025 & 6.72 & 6.53 -  6.91 & 1.56 & 1.49 -  1.62 & 2.46 & 2.22 -  2.95 \\
3590 & KOI-2840 & 1.04 & 0.017 & 1.56 & 1.53 -  1.59 & 1.02 & 1.02 -  1.04 & 7.64 & 7.21 -  8.17 \\
3591 & Kepler-172 & 1.18 & 0.026 & 1.09 & 1.06 -  1.12 & 1.00 & 0.99 -  1.01 & 7.77 & 6.77 -  8.66 \\
3592 & KOI-664 & 1.65 & 0.014 & 1.12 & 1.10 -  1.14 & 0.97 & 0.96 -  0.98 & 8.65 & 7.97 -  9.33 \\
3593 & Kepler-206 & 1.65 & 0.014 & 1.11 & 1.09 -  1.13 & 0.99 & 0.98 -  1.00 & 7.62 & 6.96 -  8.26 \\
3594 & KOI-372 & 3.23 & 0.037 & 0.94 & 0.92 -  0.96 & 0.98 & 0.97 -  0.99 & 3.15 & 2.13 -  4.18 \\
3595 & KOI-1241 & 1.07 & 0.028 & 4.42 & 4.32 -  4.54 & 1.33 & 1.25 -  1.38 & 4.87 & 4.21 -  5.85 \\
3596 & KOI-2408 & 1.57 & 0.016 & 0.95 & 0.93 -  0.96 & 0.85 & 0.84 -  0.86 & 11.09 & 10.10 - 12.08 \\
3597 & KOI-511 & 1.17 & 0.021 & 1.14 & 1.11 -  1.17 & 1.04 & 1.03 -  1.06 & 5.65 & 4.97 -  6.29 \\
3598 & KOI-176 & 1.13 & 0.014 & 1.41 & 1.38 -  1.44 & 1.14 & 1.13 -  1.16 & 4.09 & 3.70 -  4.32 \\
3599 & KOI-94 & 2.07 & 0.022 & 1.42 & 1.39 -  1.45 & 1.21 & 1.20 -  1.22 & 3.79 & 3.63 -  3.95 \\
3600 & KOI-270 &  &  & 1.04 & 0.98 -  1.10 & 0.91 & 0.90 -  0.92 & 8.83 & 7.48 -  9.57 \\
3601 & KOI-3117 & 2.49 & 0.015 & 0.95 & 0.94 -  0.97 & 0.91 & 0.90 -  0.92 & 8.69 & 7.47 -  9.93 \\
3602 & KOI-4657 & 2.69 & 0.02 & 0.93 & 0.92 -  0.95 & 0.82 & 0.81 -  0.83 & 14.04 & 13.19 - 14.65 \\
3603 & KOI-3438 & 1.31 & 0.013 & 1.18 & 1.15 -  1.20 & 1.01 & 1.00 -  1.03 & 5.99 & 5.58 -  6.42 \\
3604 & KOI-1239 & 0.969 & 0.033 & 0.96 & 0.93 -  0.99 & 0.95 & 0.94 -  0.97 & 5.06 & 3.33 -  6.57 \\
3605 & KOI-3287 & 1.09 & 0.015 & 1.29 & 1.26 -  1.32 & 1.01 & 1.01 -  1.03 & 6.91 & 6.50 -  7.21 \\
3606 & KOI-857 & 1.41 & 0.02 & 0.86 & 0.85 -  0.87 & 0.84 & 0.83 -  0.85 & 12.25 & 9.91 - 13.99 \\
3607 & KOI-1242 & 1.07 & 0.019 & 1.34 & 1.31 -  1.38 & 1.14 & 1.13 -  1.16 & 4.43 & 4.01 -  4.75 \\
3608 & KOI-2559 & 1.34 & 0.014 & 1.16 & 1.14 -  1.19 & 1.05 & 1.03 -  1.06 & 6.12 & 5.55 -  6.68 \\
3609 & KOI-3237 & 3.1 & 0.021 & 1.02 & 1.01 -  1.04 & 1.03 & 1.02 -  1.04 & 4.25 & 3.43 -  5.09 \\
3610 & KOI-2838 & 1.16 & 0.017 & 1.73 & 1.70 -  1.77 & 1.09 & 1.07 -  1.11 & 7.95 & 7.42 -  8.41 \\
3611 & KOI-1227 & 1.12 & 0.021 & 1.30 & 1.27 -  1.33 & 0.97 & 0.95 -  0.98 & 7.51 & 7.14 -  7.87 \\
3612 & KOI-2737 & 1.91 & 0.02 & 1.66 & 1.63 -  1.69 & 1.11 & 1.10 -  1.12 & 7.96 & 7.63 -  8.35 \\
3613 & KOI-4159 & 1.6 & 0.025 & 0.89 & 0.88 -  0.90 & 0.83 & 0.82 -  0.83 & 14.34 & 13.34 - 14.82 \\
3614 & KOI-1692 & 3.69 & 0.024 & 0.93 & 0.92 -  0.95 & 0.92 & 0.91 -  0.94 & 8.25 & 6.69 -  9.74 \\
3615 & KOI-612 & 2.19 & 0.015 & 0.82 & 0.80 -  0.83 & 0.80 & 0.79 -  0.81 & 11.97 & 9.54 - 13.87 \\
3616 & KOI-666 & 1.76 & 0.015 & 1.01 & 0.99 -  1.03 & 0.93 & 0.92 -  0.94 & 9.10 & 8.08 - 10.08 \\
3617 & KOI-4651 & 1.78 & 0.02 & 1.00 & 0.98 -  1.02 & 0.90 & 0.89 -  0.91 & 10.02 & 9.15 - 10.75 \\
3618 & KOI-665 & 1.11 & 0.013 & 1.79 & 1.76 -  1.83 & 1.32 & 1.30 -  1.33 & 4.07 & 3.90 -  4.22 \\
3619 & Kepler-207 & 1.11 & 0.013 & 1.80 & 1.76 -  1.83 & 1.31 & 1.30 -  1.33 & 4.09 & 3.94 -  4.23 \\
3620 & KOI-561 & 2.38 & 0.014 & 0.78 & 0.77 -  0.79 & 0.75 & 0.74 -  0.75 & 13.86 & 12.46 - 14.69 \\
3621 & KOI-1240 & 1.25 & 0.018 & 1.03 & 1.00 -  1.05 & 0.90 & 0.89 -  0.92 & 11.64 & 10.49 - 12.79 \\
3622 & KOI-2092 & 0.666 & 0.036 & 0.82 & 0.79 -  0.86 & 0.85 & 0.83 -  0.87 & 4.57 & 1.91 -  7.32 \\
3623 & KOI-5324 & 0.548 & 0.016 & 4.35 & 4.23 -  4.47 & 1.27 & 1.08 -  1.32 & 4.49 & 4.09 -  7.82 \\
3624 & KOI-4072 & 1.45 & 0.013 & 1.26 & 1.24 -  1.28 & 1.07 & 1.05 -  1.08 & 6.58 & 6.08 -  7.14 \\
3625 & KOI-2678 & 5.71 & 0.023 & 0.83 & 0.81 -  0.84 & 0.88 & 0.87 -  0.90 & 4.60 & 2.54 -  6.58 \\
3626 & KOI-177 &  &  & 0.98 & 0.94 -  1.04 & 0.98 & 0.97 -  1.00 & 5.03 & 2.78 -  6.83 \\
3627 & KOI-1695 & 1.15 & 0.016 & 1.39 & 1.37 -  1.42 & 1.13 & 1.11 -  1.15 & 5.60 & 5.22 -  6.25 \\
3628 & KOI-3980 & 0.797 & 0.026 & 1.33 & 1.29 -  1.38 & 1.03 & 1.01 -  1.04 & 8.77 & 8.25 -  9.32 \\
3629 & KOI-1375 & 0.992 & 0.018 & 1.59 & 1.55 -  1.62 & 1.21 & 1.19 -  1.22 & 3.92 & 3.80 -  3.97 \\
3630 & KOI-4850 & 1.51 & 0.017 & 0.96 & 0.95 -  0.98 & 0.93 & 0.92 -  0.94 & 7.69 & 6.48 -  8.83 \\
3631 & KOI-2086 & 0.947 & 0.018 & 1.50 & 1.47 -  1.53 & 1.09 & 1.08 -  1.10 & 6.20 & 5.79 -  6.72 \\
3632 & Kepler-60 & 0.947 & 0.018 & 1.51 & 1.48 -  1.54 & 1.10 & 1.08 -  1.11 & 5.75 & 5.46 -  6.12 \\
3633 & KOI-4871 & 1.33 & 0.037 & 1.40 & 1.36 -  1.44 & 1.21 & 1.20 -  1.22 & 3.17 & 2.96 -  3.35 \\
3634 & KOI-4184 &  &  & 0.75 & 0.74 -  0.77 & 0.75 & 0.74 -  0.77 & 11.79 & 7.27 - 14.14 \\
3635 & KOI-864 & 0.937 & 0.032 & 0.91 & 0.88 -  0.94 & 0.87 & 0.85 -  0.88 & 9.97 & 7.63 - 11.91 \\
3636 & KOI-3244 & 0.635 & 0.021 & 7.09 & 6.91 -  7.29 & 1.46 & 1.42 -  1.49 & 3.18 & 2.95 -  3.44 \\
3637 & KOI-4188 & 2.1 & 0.021 & 1.11 & 1.10 -  1.12 & 1.20 & 1.19 -  1.21 & 0.35 & 0.28 -  0.54 \\
3638 & KOI-4674 & 1.49 & 0.014 & 1.24 & 1.22 -  1.26 & 0.99 & 0.98 -  1.00 & 10.12 & 9.54 - 10.71 \\
3639 & KOI-201 & 1.56 & 0.016 & 1.06 & 1.04 -  1.08 & 0.95 & 0.94 -  0.97 & 10.05 & 8.96 - 11.09 \\
3640 & KOI-2571 & 1.11 & 0.031 & 1.41 & 1.37 -  1.44 & 0.94 & 0.94 -  0.94 & 14.80 & 14.60 - 14.93 \\
3641 & KOI-163 & 1.73 & 0.086 & 0.77 & 0.77 -  0.79 & 0.72 & 0.72 -  0.73 & 14.82 & 14.52 - 14.95 \\
3642 & KOI-2220 & 0.762 & 0.022 & 1.38 & 1.34 -  1.43 & 1.05 & 1.03 -  1.06 & 8.32 & 7.86 -  8.81 \\
3643 & KOI-1366 & 0.998 & 0.024 & 0.90 & 0.87 -  0.92 & 0.89 & 0.87 -  0.90 & 8.25 & 5.90 - 10.57 \\
3644 & KOI-2925 & 2.46 & 0.015 & 0.89 & 0.88 -  0.90 & 0.89 & 0.88 -  0.91 & 7.83 & 6.12 -  9.39 \\
3645 & KOI-1363 & 0.531 & 0.033 & 1.14 & 1.09 -  1.19 & 0.98 & 0.97 -  1.00 & 9.22 & 8.16 - 10.15 \\
3646 & KOI-2087 & 3.53 & 0.02 & 1.03 & 1.02 -  1.05 & 1.07 & 1.06 -  1.09 & 2.35 & 1.65 -  3.04 \\
3647 & KOI-1628 & 1.23 & 0.022 & 1.66 & 1.63 -  1.69 & 1.35 & 1.33 -  1.36 & 2.88 & 2.74 -  3.02 \\
3648 & KOI-1367 & 1.71 & 0.019 & 0.75 & 0.73 -  0.76 & 0.74 & 0.73 -  0.76 & 11.69 & 8.53 - 13.80 \\
3649 & KOI-4382 & 0.79 & 0.016 & 1.46 & 1.42 -  1.49 & 1.20 & 1.19 -  1.22 & 3.68 & 3.53 -  3.86 \\
3650 & KOI-2879 &  &  & 0.89 & 0.84 -  0.93 & 0.86 & 0.84 -  0.87 & 9.36 & 5.78 - 11.84 \\
3651 & KOI-670 & 1.0 & 0.017 & 1.73 & 1.69 -  1.77 & 1.08 & 1.06 -  1.10 & 8.39 & 7.81 -  8.87 \\
3652 & KOI-671 & 1.26 & 0.015 & 1.31 & 1.28 -  1.33 & 1.11 & 1.10 -  1.12 & 5.23 & 4.92 -  5.54 \\
3653 & KOI-2215 & 0.652 & 0.019 & 2.01 & 1.97 -  2.11 & 1.45 & 1.44 -  1.50 & 2.19 & 2.05 -  2.32 \\
3654 & KOI-3689 & 0.981 & 0.017 & 1.38 & 1.35 -  1.41 & 1.10 & 1.09 -  1.12 & 5.96 & 5.62 -  6.37 \\
3655 & KOI-312 & 2.35 & 0.024 & 1.51 & 1.48 -  1.53 & 1.24 & 1.23 -  1.25 & 3.66 & 3.52 -  3.80 \\
3656 & KOI-872 & 1.26 & 0.028 & 0.85 & 0.83 -  0.86 & 0.83 & 0.82 -  0.84 & 11.81 & 8.85 - 13.88 \\
3657 & KOI-673 & 1.25 & 0.014 & 1.37 & 1.34 -  1.39 & 1.20 & 1.19 -  1.21 & 3.50 & 3.26 -  3.77 \\
3658 & KOI-672 & 1.7 & 0.017 & 0.94 & 0.92 -  0.96 & 0.93 & 0.91 -  0.94 & 7.37 & 5.98 -  8.72 \\
3659 & KOI-2083 & 0.987 & 0.16 & 1.41 & 1.34 -  1.50 & 1.10 & 1.09 -  1.12 & 5.62 & 5.32 -  5.94 \\
3660 & KOI-3907 & 1.7 & 0.025 & 1.46 & 1.43 -  1.49 & 1.25 & 1.23 -  1.26 & 2.82 & 2.56 -  3.00 \\
3661 & Kepler-1542 & 2.48 & 0.024 &  &  &  &  &  &  \\
3662 & KOI-4032 & 2.48 & 0.024 & 1.19 & 1.17 -  1.21 & 0.94 & 0.93 -  0.96 & 11.51 & 10.79 - 12.19 \\
3663 & KOI-3012 & 1.43 & 0.021 & 1.78 & 1.75 -  1.81 & 0.92 & 0.90 -  0.93 & 10.23 & 9.71 - 10.89 \\
3664 & KOI-4473 & 0.749 & 0.023 & 2.17 & 2.12 -  2.25 & 1.31 & 1.28 -  1.36 & 3.98 & 3.64 -  4.23 \\
3665 & KOI-3083 & 2.06 & 0.021 & 1.18 & 1.16 -  1.20 & 1.09 & 1.08 -  1.10 & 5.13 & 4.61 -  5.60 \\
3666 & KOI-3100 & 0.988 & 0.013 & 1.80 & 1.76 -  1.83 & 1.33 & 1.32 -  1.35 & 3.80 & 3.65 -  3.95 \\
3667 & KOI-1379 & 1.66 & 0.015 & 1.04 & 1.02 -  1.06 & 0.93 & 0.92 -  0.94 & 8.28 & 7.60 -  8.89 \\
3668 & KOI-1618 & 2.47 & 0.03 & 1.57 & 1.55 -  1.60 & 1.26 & 1.25 -  1.27 & 3.78 & 3.64 -  3.96 \\
3669 & KOI-5375 & 0.362 & 0.018 & 6.47 & 6.23 -  6.70 & 1.30 & 1.19 -  1.34 & 4.04 & 3.76 -  5.24 \\
3670 & KOI-369 & 2.57 & 0.022 & 1.22 & 1.20 -  1.24 & 1.10 & 1.08 -  1.11 & 4.12 & 3.79 -  4.45 \\
3671 & KOI-238 & 0.95 & 0.021 & 1.39 & 1.35 -  1.42 & 1.14 & 1.12 -  1.15 & 4.63 & 4.21 -  4.87 \\
3672 & KOI-987 & 3.56 & 0.026 & 0.93 & 0.92 -  0.95 & 0.91 & 0.89 -  0.92 & 8.59 & 7.29 -  9.85 \\
3673 & KOI-4136 & 0.769 & 0.018 & 2.02 & 1.98 -  2.06 & 1.25 & 1.19 -  1.27 & 4.91 & 4.45 -  5.69 \\
3674 & KOI-2051 & 0.669 & 0.023 & 1.24 & 1.19 -  1.28 & 1.00 & 0.98 -  1.02 & 7.52 & 7.09 -  7.97 \\
3675 & KOI-1961 & 2.44 & 0.03 & 1.16 & 1.14 -  1.17 & 0.86 & 0.85 -  0.87 & 13.85 & 13.27 - 14.39 \\
3676 & KOI-2916 & 2.11 & 0.017 & 0.79 & 0.78 -  0.80 & 0.77 & 0.77 -  0.79 & 13.06 & 10.82 - 14.41 \\
3677 & KOI-2561 & 1.1 & 0.02 & 1.44 & 1.41 -  1.47 & 1.14 & 1.13 -  1.16 & 5.35 & 5.04 -  5.71 \\
3678 & KOI-2516 & 1.11 & 0.015 & 2.10 & 2.07 -  2.14 & 1.21 & 1.16 -  1.24 & 5.98 & 5.48 -  6.85 \\
3679 & KOI-456 & 1.04 & 0.018 & 1.11 & 1.08 -  1.13 & 0.95 & 0.94 -  0.96 & 10.35 & 9.48 - 11.24 \\
3680 & KOI-1979 & 1.75 & 0.062 & 1.31 & 1.27 -  1.35 & 1.03 & 1.02 -  1.04 & 8.78 & 8.26 -  9.31 \\
3681 & KOI-5379 & 0.893 & 0.021 & 4.50 & 4.40 -  4.60 & 1.34 & 1.29 -  1.37 & 4.19 & 3.87 -  4.71 \\
3682 & KOI-1862 & 1.79 & 0.019 & 1.00 & 0.98 -  1.02 & 0.96 & 0.95 -  0.98 & 7.15 & 6.05 -  8.24 \\
3683 & KOI-674 & 0.911 & 0.015 & 2.72 & 2.67 -  2.78 & 1.03 & 1.00 -  1.05 & 11.44 & 10.38 - 12.70 \\
3684 & KOI-373 & 2.63 & 0.021 & 0.95 & 0.94 -  0.97 & 0.89 & 0.88 -  0.90 & 7.00 & 6.17 -  7.89 \\
3685 & KOI-1378 & 1.17 & 0.016 & 1.80 & 1.77 -  1.83 & 1.07 & 1.07 -  1.10 & 5.91 & 5.43 -  6.12 \\
3686 & KOI-4864 & 0.886 & 0.014 & 2.44 & 2.39 -  2.50 & 1.21 & 1.17 -  1.28 & 4.21 & 3.27 -  4.46 \\
3687 & KOI-4665 & 1.13 & 0.023 & 1.50 & 1.46 -  1.54 & 1.03 & 1.02 -  1.04 & 8.79 & 8.07 -  9.31 \\
3688 & KOI-266 & 3.05 & 0.024 & 1.24 & 1.22 -  1.26 & 1.12 & 1.11 -  1.13 & 4.08 & 3.70 -  4.40 \\
3689 & KOI-3096 & 1.13 & 0.015 & 1.70 & 1.68 -  1.73 & 1.00 & 0.98 -  1.00 & 8.29 & 7.88 -  8.71 \\
3690 & KOI-313 & 3.27 & 0.02 & 0.88 & 0.86 -  0.89 & 0.83 & 0.82 -  0.84 & 12.90 & 11.24 - 14.23 \\
3691 & KOI-884 & 1.48 & 0.031 & 0.83 & 0.82 -  0.84 & 0.82 & 0.81 -  0.83 & 12.66 & 10.08 - 14.33 \\
3692 & KOI-1848 & 0.961 & 0.24 & 1.28 & 1.21 -  1.38 & 1.06 & 1.04 -  1.09 & 5.81 & 5.40 -  6.17 \\
3693 & KOI-2357 & 0.584 & 0.037 & 1.13 & 1.07 -  1.19 & 0.96 & 0.94 -  0.97 & 8.91 & 8.32 -  9.50 \\
3694 & KOI-5393 & 0.562 & 0.017 & 5.56 & 5.41 -  5.71 & 1.38 & 1.32 -  1.39 & 3.83 & 3.80 -  4.38 \\
3695 & KOI-3193 &  &  & 2.82 & 2.69 -  2.95 & 0.95 & 0.95 -  0.97 & 14.33 & 13.60 - 14.72 \\
3696 & KOI-1890 & 0.698 & 0.49 & 1.80 & 1.68 -  1.94 & 1.30 & 1.26 -  1.35 & 3.94 & 3.59 -  4.26 \\
3697 & KOI-457 & 2.27 & 0.016 & 0.80 & 0.79 -  0.81 & 0.85 & 0.84 -  0.87 & 4.76 & 2.20 -  7.43 \\
3698 & KOI-679 & 1.43 & 0.018 & 1.53 & 1.50 -  1.56 & 1.11 & 1.10 -  1.14 & 6.93 & 6.34 -  7.28 \\
3699 & KOI-678 & 3.2 & 0.018 & 0.81 & 0.79 -  0.82 & 0.85 & 0.84 -  0.87 & 5.59 & 3.05 -  8.20 \\
3700 & KOI-4663 & 1.39 & 0.02 & 2.11 & 2.06 -  2.14 & 1.24 & 1.20 -  1.27 & 5.47 & 5.16 -  6.10 \\
3701 & Kepler-435 & 0.676 & 0.017 & 2.29 & 2.24 -  2.35 & 1.48 & 1.45 -  1.50 & 2.78 & 2.72 -  3.06 \\
3702 & KOI-150 & 1.92 & 0.016 & 0.89 & 0.88 -  0.90 & 0.76 & 0.76 -  0.77 & 14.42 & 13.67 - 14.83 \\
3703 & KOI-4160 & 1.96 & 0.017 & 1.00 & 0.98 -  1.02 & 1.03 & 1.02 -  1.05 & 3.35 & 2.34 -  4.35 \\
3704 & KOI-3128 & 0.855 & 0.016 & 2.18 & 2.13 -  2.23 & 1.34 & 1.27 -  1.38 & 3.27 & 3.15 -  3.98 \\
3705 & Kepler-431 & 2.03 & 0.02 & 1.61 & 1.51 -  1.72 & 1.11 & 1.09 -  1.12 & 5.77 & 5.47 -  6.08 \\
3706 & KOI-3097 & 2.03 & 0.02 & 1.68 & 1.65 -  1.70 & 1.13 & 1.12 -  1.14 & 6.12 & 5.79 -  6.39 \\
3707 & KOI-2631 & 1.13 & 0.015 & 1.58 & 1.55 -  1.61 & 0.93 & 0.92 -  0.95 & 9.34 & 8.83 -  9.81 \\
3708 & KOI-683 & 1.45 & 0.016 & 1.13 & 1.10 -  1.15 & 1.05 & 1.04 -  1.07 & 5.26 & 4.59 -  5.87 \\
3709 & KOI-1706 & 2.12 & 0.019 & 0.85 & 0.84 -  0.87 & 0.82 & 0.81 -  0.84 & 12.49 & 10.35 - 14.08 \\
3710 & KOI-568 & 1.77 & 0.017 & 0.90 & 0.89 -  0.92 & 0.83 & 0.82 -  0.84 & 13.08 & 11.64 - 14.20 \\
3711 & KOI-4614 & 1.02 & 0.015 & 1.44 & 1.41 -  1.47 & 1.16 & 1.14 -  1.17 & 5.13 & 4.76 -  5.61 \\
3712 & KOI-1898 & 1.73 & 0.013 & 1.21 & 1.19 -  1.23 & 0.99 & 0.98 -  1.00 & 8.16 & 7.72 -  8.74 \\
3713 & KOI-3943 & 1.58 & 0.023 & 1.52 & 1.50 -  1.55 & 1.21 & 1.18 -  1.23 & 4.05 & 3.75 -  4.49 \\
3714 & KOI-315 & 5.09 & 0.025 & 0.70 & 0.69 -  0.70 & 0.68 & 0.68 -  0.69 & 13.86 & 12.17 - 14.68 \\
3715 & KOI-1528 & 1.95 & 0.016 & 0.88 & 0.87 -  0.89 & 0.82 & 0.81 -  0.83 & 14.01 & 12.86 - 14.73 \\
3716 & KOI-2722 & 1.57 & 0.018 & 1.14 & 1.12 -  1.16 & 1.11 & 1.09 -  1.12 & 3.01 & 2.45 -  3.50 \\
3717 & Kepler-402 & 1.57 & 0.018 & 1.15 & 1.13 -  1.17 & 1.09 & 1.08 -  1.10 & 3.52 & 3.06 -  3.95 \\
3718 & KOI-892 & 1.55 & 0.022 & 0.76 & 0.74 -  0.77 & 0.77 & 0.75 -  0.80 & 8.44 & 4.43 - 11.85 \\
3719 & KOI-2585 & 1.44 & 0.016 & 1.19 & 1.17 -  1.21 & 0.92 & 0.91 -  0.93 & 8.66 & 8.23 -  9.06 \\
3720 & KOI-269 & 3.36 & 0.025 & 1.47 & 1.44 -  1.49 & 1.25 & 1.24 -  1.26 & 3.06 & 2.90 -  3.21 \\
3721 & KOI-684 & 0.881 & 0.013 & 2.22 & 2.18 -  2.26 & 1.10 & 1.06 -  1.14 & 8.11 & 7.00 -  9.27 \\
3722 & KOI-4561 & 0.634 & 0.027 & 2.08 & 1.99 -  2.15 & 1.25 & 1.20 -  1.31 & 4.55 & 3.93 -  5.04 \\
3723 & KOI-1921 & 1.32 & 0.026 & 1.55 & 1.51 -  1.58 & 1.30 & 1.29 -  1.32 & 2.75 & 2.63 -  2.87 \\
3724 & KOI-4482 & 1.89 & 0.022 & 1.29 & 1.26 -  1.31 & 1.15 & 1.14 -  1.16 & 3.78 & 3.43 -  4.14 \\
3725 & KOI-3721 & 0.321 & 0.021 & 2.91 & 2.86 -  3.21 & 1.65 & 1.65 -  1.76 & 1.40 & 1.34 -  1.50 \\
3726 & KOI-4022 & 0.919 & 0.013 & 2.11 & 2.06 -  2.15 & 1.19 & 1.17 -  1.22 & 4.89 & 4.64 -  5.09 \\
3727 & KOI-1808 & 2.25 & 0.023 & 1.18 & 1.11 -  1.26 & 1.14 & 1.12 -  1.15 & 3.06 & 1.86 -  3.92 \\
3728 & KOI-685 & 0.73 & 0.021 & 1.91 & 1.85 -  1.97 & 1.39 & 1.37 -  1.41 & 2.79 & 2.69 -  2.89 \\
3729 & KOI-3023 & 1.46 & 0.025 & 1.26 & 1.23 -  1.28 & 1.18 & 1.17 -  1.19 & 2.56 & 2.22 -  2.93 \\
3730 & KOI-4725 & 3.99 & 0.014 & 0.75 & 0.74 -  0.75 & 0.73 & 0.73 -  0.74 & 13.82 & 12.13 - 14.69 \\
3731 & KOI-2848 & 2.23 & 0.021 & 1.39 & 1.36 -  1.42 & 1.04 & 1.03 -  1.06 & 9.26 & 8.73 -  9.80 \\
3732 & KOI-3787 & 1.62 & 0.02 & 0.97 & 0.95 -  0.99 & 0.99 & 0.98 -  1.00 & 4.55 & 3.38 -  5.59 \\
3733 & KOI-171 & 1.02 & 0.017 & 1.47 & 1.44 -  1.50 & 1.23 & 1.21 -  1.24 & 3.82 & 3.67 -  3.98 \\
3734 & KOI-1533 & 1.38 & 0.014 & 1.02 & 1.00 -  1.04 & 0.93 & 0.92 -  0.94 & 6.71 & 5.98 -  7.36 \\
3735 & KOI-4582 & 4.42 & 0.027 & 0.95 & 0.94 -  0.97 & 0.89 & 0.88 -  0.90 & 7.66 & 6.81 -  8.52 \\
3736 & KOI-1964 & 7.35 & 0.1 & 1.03 & 1.02 -  1.05 & 0.90 & 0.89 -  0.91 & 11.47 & 10.80 - 12.31 \\
3737 & KOI-2984 & 1.2 & 0.014 & 1.78 & 1.75 -  1.82 & 1.28 & 1.26 -  1.31 & 4.08 & 3.84 -  4.27 \\
3738 & KOI-1818 & 1.71 & 0.017 & 0.88 & 0.87 -  0.90 & 0.92 & 0.91 -  0.94 & 4.87 & 3.16 -  6.54 \\
3739 & KOI-4257 & 0.839 & 0.015 & 2.60 & 2.56 -  2.64 & 1.37 & 1.31 -  1.40 & 3.64 & 3.41 -  4.10 \\
3740 & KOI-686 & 1.87 & 0.017 & 1.06 & 1.04 -  1.07 & 0.94 & 0.93 -  0.95 & 8.89 & 8.27 -  9.45 \\
3741 & KOI-3236 & 1.8 & 0.029 & 1.50 & 1.47 -  1.53 & 1.29 & 1.28 -  1.30 & 2.87 & 2.71 -  3.02 \\
3742 & KOI-4109 & 2.18 & 0.023 & 0.80 & 0.79 -  0.82 & 0.82 & 0.80 -  0.84 & 9.44 & 6.00 - 12.47 \\
3743 & KOI-4773 & 0.804 & 0.015 & 2.17 & 2.11 -  2.25 & 1.35 & 1.32 -  1.40 & 2.66 & 2.57 -  2.96 \\
3744 & KOI-687 & 3.03 & 0.25 & 1.01 & 0.98 -  1.06 & 1.06 & 1.05 -  1.07 & 2.22 & 0.95 -  3.77 \\
3745 & KOI-459 & 1.14 & 0.02 & 1.19 & 1.16 -  1.22 & 1.03 & 1.01 -  1.04 & 7.17 & 6.55 -  7.82 \\
3746 & KOI-92 & 3.62 & 0.025 & 1.10 & 1.08 -  1.12 & 1.06 & 1.05 -  1.07 & 4.28 & 3.66 -  4.90 \\
3747 & KOI-3214 &  &  & 1.70 & 1.59 -  1.81 & 1.12 & 1.11 -  1.14 & 5.57 & 5.24 -  5.86 \\
3748 & KOI-2674 & 1.13 & 0.018 & 1.78 & 1.74 -  1.82 & 1.12 & 1.11 -  1.13 & 7.07 & 6.67 -  7.45 \\
3749 & KOI-2352 & 3.71 & 0.024 & 1.48 & 1.46 -  1.50 & 1.23 & 1.22 -  1.25 & 3.18 & 3.01 -  3.34 \\
3750 & KOI-237 & 1.21 & 0.018 & 1.15 & 1.13 -  1.18 & 1.04 & 1.03 -  1.06 & 6.50 & 5.81 -  7.19 \\
3751 & KOI-520 & 1.87 & 0.021 & 0.82 & 0.81 -  0.83 & 0.81 & 0.80 -  0.82 & 12.04 & 9.26 - 13.97 \\
3752 & KOI-517 & 1.68 & 0.016 & 0.95 & 0.93 -  0.96 & 0.90 & 0.89 -  0.92 & 9.56 & 8.15 - 11.03 \\
3753 & KOI-519 & 0.734 & 0.025 & 1.25 & 1.21 -  1.30 & 1.02 & 1.01 -  1.04 & 8.16 & 7.51 -  8.80 \\
3754 & KOI-155 & 1.16 & 0.015 & 1.62 & 1.59 -  1.65 & 1.10 & 1.07 -  1.10 & 5.52 & 5.29 -  5.99 \\
3755 & KOI-316 & 2.53 & 0.027 & 1.11 & 1.09 -  1.13 & 0.98 & 0.97 -  1.00 & 9.08 & 8.24 -  9.89 \\
3756 & KOI-569 & 2.11 & 0.021 & 0.75 & 0.74 -  0.76 & 0.73 & 0.73 -  0.75 & 12.59 & 10.09 - 14.26 \\
3757 & KOI-2743 & 1.86 & 0.015 & 0.95 & 0.94 -  0.97 & 0.88 & 0.87 -  0.90 & 9.36 & 8.34 - 10.32 \\
3758 & KOI-3245 & 1.95 & 0.026 & 1.38 & 1.35 -  1.41 & 1.11 & 1.09 -  1.12 & 5.08 & 4.91 -  5.32 \\
3759 & KOI-2486 & 2.09 & 0.51 & 1.53 & 1.42 -  1.64 & 1.19 & 1.16 -  1.23 & 4.71 & 4.41 -  5.19 \\
3760 & KOI-2426 & 1.82 & 0.015 & 0.96 & 0.94 -  0.98 & 0.84 & 0.84 -  0.85 & 14.13 & 13.45 - 14.68 \\
3761 & KOI-4343 & 1.75 & 0.37 & 1.73 & 1.60 -  1.85 & 1.00 & 0.96 -  1.04 & 7.56 & 6.56 -  8.55 \\
3762 & KOI-1951 & 1.22 & 0.038 & 1.34 & 1.30 -  1.38 & 1.05 & 1.03 -  1.06 & 5.99 & 5.72 -  6.27 \\
3763 & KOI-162 &  &  & 1.18 & 1.11 -  1.26 & 1.06 & 1.05 -  1.08 & 6.06 & 5.15 -  6.80 \\
3764 & KOI-4656 & 0.701 & 0.018 & 2.02 & 1.97 -  2.08 & 1.53 & 1.51 -  1.55 & 2.02 & 1.95 -  2.08 \\
3765 & KOI-4881 & 0.991 & 0.014 & 1.50 & 1.46 -  1.54 & 1.24 & 1.20 -  1.25 & 3.61 & 3.46 -  4.23 \\
3766 & KOI-317 & 1.18 & 0.02 & 1.78 & 1.74 -  1.82 & 1.38 & 1.36 -  1.39 & 2.82 & 2.73 -  2.90 \\
3767 & KOI-2073 & 1.42 & 0.03 & 0.76 & 0.74 -  0.77 & 0.77 & 0.75 -  0.78 & 10.99 & 6.74 - 13.65 \\
3768 & KOI-1019 & 3.3 & 0.022 & 3.53 & 3.47 -  3.59 & 1.18 & 1.15 -  1.21 & 6.71 & 5.93 -  7.29 \\
3769 & KOI-688 & 0.823 & 0.015 & 1.62 & 1.58 -  1.66 & 1.27 & 1.25 -  1.29 & 3.50 & 3.37 -  3.84 \\
3770 & KOI-4634 &  &  & 1.25 & 1.18 -  1.34 & 1.16 & 1.15 -  1.19 & 3.51 & 2.67 -  4.00 \\
3771 & KOI-3046 & 1.71 & 0.013 & 1.21 & 1.20 -  1.24 & 0.99 & 0.98 -  1.00 & 9.92 & 9.23 - 10.59 \\
3772 & KOI-318 & 1.54 & 0.025 & 1.74 & 1.71 -  1.78 & 1.43 & 1.42 -  1.45 & 2.20 & 2.10 -  2.31 \\
3773 & KOI-2781 & 1.7 & 0.029 & 1.59 & 1.56 -  1.63 & 0.91 & 0.90 -  0.93 & 10.20 & 9.66 - 10.77 \\
3774 & KOI-2105 & 1.41 & 0.017 & 1.04 & 1.02 -  1.06 & 1.04 & 1.02 -  1.05 & 3.73 & 2.87 -  4.52 \\
3775 & KOI-1985 & 3.24 & 0.015 & 0.76 & 0.75 -  0.77 & 0.76 & 0.75 -  0.77 & 12.05 & 9.44 - 14.03 \\
3776 & KOI-572 & 0.847 & 0.025 & 1.62 & 1.57 -  1.66 & 1.15 & 1.14 -  1.16 & 5.15 & 4.63 -  5.42 \\
3777 & KOI-907 & 1.05 & 0.031 & 0.85 & 0.83 -  0.88 & 0.91 & 0.89 -  0.93 & 3.31 & 1.43 -  5.42 \\
3778 & KOI-1809 & 2.57 & 0.023 & 1.02 & 1.00 -  1.04 & 0.99 & 0.98 -  1.00 & 5.96 & 5.11 -  6.82 \\
3779 & KOI-1726 & 4.59 & 0.014 & 0.76 & 0.76 -  0.77 & 0.75 & 0.75 -  0.76 & 13.88 & 12.22 - 14.72 \\
3780 & KOI-2593 & 2.34 & 0.019 & 1.55 & 1.52 -  1.57 & 1.26 & 1.25 -  1.27 & 3.89 & 3.74 -  4.03 \\
3781 & KOI-4037 & 1.66 & 0.025 & 1.25 & 1.22 -  1.28 & 1.19 & 1.18 -  1.20 & 2.39 & 2.04 -  2.75 \\
3782 & KOI-4426 & 0.806 & 0.015 & 2.00 & 1.96 -  2.04 & 1.35 & 1.33 -  1.37 & 3.59 & 3.50 -  3.79 \\
3783 & KOI-4098 & 2.81 & 0.3 & 0.77 & 0.75 -  0.78 & 0.76 & 0.75 -  0.77 & 12.13 & 8.09 - 14.25 \\
3784 & KOI-1069 & 1.23 & 0.025 & 0.89 & 0.88 -  0.91 & 0.85 & 0.84 -  0.86 & 12.82 & 10.68 - 14.31 \\
3785 & KOI-3338 & 1.37 & 0.014 & 1.23 & 1.20 -  1.25 & 1.07 & 1.06 -  1.08 & 4.97 & 4.62 -  5.31 \\
3786 & KOI-4834 & 1.24 & 0.015 & 2.66 & 2.62 -  2.71 & 1.17 & 1.14 -  1.21 & 7.17 & 6.40 -  7.84 \\
3787 & KOI-4567 & 0.818 & 0.063 & 1.56 & 1.48 -  1.65 & 1.32 & 1.29 -  1.34 & 2.57 & 2.42 -  2.69 \\
3788 & KOI-4435 & 0.797 & 0.012 & 2.04 & 1.99 -  2.08 & 1.41 & 1.39 -  1.42 & 3.27 & 3.18 -  3.40 \\
3789 & KOI-1137 & -1.41 & 0.38 & 0.84 & 0.80 -  0.88 & 0.86 & 0.84 -  0.88 & 5.41 & 2.40 -  8.50 \\
3790 & KOI-3301 & 0.75 & 0.022 & 1.92 & 1.88 -  1.99 & 1.23 & 1.20 -  1.28 & 5.42 & 4.88 -  5.88 \\
3791 & Kepler-271 & 2.44 & 0.023 & 0.87 & 0.86 -  0.89 & 0.84 & 0.83 -  0.85 & 8.80 & 7.40 - 10.08 \\
3792 & KOI-1150 & 0.681 & 0.33 & 1.19 & 1.12 -  1.26 & 1.01 & 1.00 -  1.02 & 8.08 & 7.24 -  8.79 \\
3793 & KOI-1820 & 2.47 & 0.016 & 0.86 & 0.84 -  0.87 & 0.86 & 0.84 -  0.87 & 8.75 & 6.63 - 10.77 \\
3794 & KOI-4399 & 4.71 & 0.018 & 0.86 & 0.85 -  0.88 & 0.86 & 0.84 -  0.87 & 7.69 & 6.34 -  9.05 \\
3795 & KOI-574 & 1.66 & 0.02 & 0.79 & 0.77 -  0.80 & 0.77 & 0.76 -  0.79 & 12.19 & 9.46 - 14.06 \\
3796 & KOI-4763 & 0.742 & 0.017 & 1.97 & 1.93 -  2.02 & 1.27 & 1.21 -  1.30 & 4.66 & 4.35 -  5.55 \\
3797 & KOI-573 & 1.0 & 0.023 & 1.09 & 1.06 -  1.12 & 0.96 & 0.95 -  0.97 & 9.13 & 8.17 - 10.06 \\
3798 & KOI-127 & 1.54 & 0.017 & 1.05 & 1.03 -  1.07 & 0.96 & 0.95 -  0.97 & 9.30 & 8.23 - 10.29 \\
3799 & KOI-4407 & 3.16 & 0.023 & 1.52 & 1.49 -  1.54 & 1.28 & 1.27 -  1.29 & 2.63 & 2.49 -  2.81 \\
3800 & Kepler-79 & 0.951 & 0.016 & 1.43 & 1.39 -  1.46 & 1.21 & 1.19 -  1.22 & 3.77 & 3.58 -  4.04 \\
3801 & KOI-152 & 0.951 & 0.016 & 1.40 & 1.36 -  1.43 & 1.25 & 1.24 -  1.26 & 2.75 & 2.52 -  2.95 \\
3802 & KOI-689 & 2.18 & 0.015 & 0.81 & 0.80 -  0.81 & 0.73 & 0.72 -  0.73 & 14.73 & 14.34 - 14.93 \\
3803 & KOI-2730 & 1.2 & 0.016 & 1.34 & 1.31 -  1.37 & 0.99 & 0.98 -  0.99 & 8.23 & 7.84 -  8.70 \\
3804 & KOI-4693 & 1.33 & 0.015 & 1.45 & 1.42 -  1.47 & 0.96 & 0.95 -  0.97 & 8.51 & 8.20 -  8.98 \\
3805 & KOI-1148 & 1.03 & 0.014 & 1.31 & 1.29 -  1.34 & 1.16 & 1.15 -  1.17 & 4.16 & 3.90 -  4.46 \\
3806 & KOI-102 & 2.52 & 0.027 & 1.13 & 1.11 -  1.16 & 1.02 & 1.00 -  1.03 & 7.30 & 6.63 -  7.95 \\
3807 & KOI-4603 & 0.966 & 0.017 & 1.59 & 1.55 -  1.63 & 1.26 & 1.24 -  1.27 & 4.04 & 3.88 -  4.20 \\
3808 & TYC 2810-1660-1 & 11.1 & 0.06 & 0.91 & 0.90 -  0.92 & 1.00 & 0.99 -  1.01 & 1.03 & 0.48 -  1.83 \\
3809 & BD+43183 & 11.1 & 0.051 & 1.17 & 1.15 -  1.19 & 1.17 & 1.16 -  1.18 & 2.03 & 1.59 -  2.44 \\
3810 & KOI-3497 & 3.17 & 0.24 & 0.78 & 0.77 -  0.79 & 0.77 & 0.76 -  0.77 & 14.34 & 13.26 - 14.83 \\
3811 & KOI-3251 & 2.11 & 0.027 & 1.31 & 1.28 -  1.33 & 1.08 & 1.06 -  1.09 & 6.39 & 5.96 -  6.92 \\
3812 & KOI-370 & 1.74 & 0.025 & 1.97 & 1.93 -  2.01 & 1.19 & 1.17 -  1.22 & 5.00 & 4.76 -  5.24 \\
3813 & KOI-2389 & 1.16 & 0.018 & 1.48 & 1.45 -  1.50 & 1.07 & 1.06 -  1.08 & 6.16 & 5.85 -  6.41 \\
3814 & KOI-4505 & 1.15 & 0.015 & 1.33 & 1.30 -  1.35 & 1.11 & 1.10 -  1.12 & 4.91 & 4.69 -  5.14 \\
3815 & KOI-2016 & 0.888 & 0.019 & 1.47 & 1.44 -  1.51 & 1.24 & 1.23 -  1.26 & 3.81 & 3.64 -  3.99 \\
3816 & KOI-691 & 0.89 & 0.016 & 1.52 & 1.49 -  1.55 & 1.02 & 1.01 -  1.04 & 6.80 & 6.35 -  7.09 \\
3817 & KOI-3315 & 1.55 & 0.015 & 0.96 & 0.95 -  0.98 & 0.78 & 0.78 -  0.79 & 13.88 & 12.98 - 14.58 \\
3818 & KOI-2022 & 1.03 & 0.021 & 1.02 & 0.99 -  1.05 & 1.01 & 1.00 -  1.02 & 4.96 & 3.81 -  6.05 \\
3819 & KOI-3111 & 2.21 & 0.022 & 1.11 & 1.10 -  1.13 & 1.01 & 1.00 -  1.02 & 5.88 & 5.33 -  6.41 \\
3820 & KOI-1792 & 0.89 & 0.34 & 1.71 & 1.63 -  1.81 & 0.96 & 0.95 -  0.98 & 10.74 & 9.70 - 11.79 \\
3821 & KOI-3890 & 0.535 & 0.014 & 6.24 & 6.09 -  6.39 & 1.30 & 1.26 -  1.33 & 4.12 & 3.87 -  4.48 \\
3822 & KOI-692 & 1.55 & 0.018 & 1.15 & 1.13 -  1.17 & 0.96 & 0.94 -  0.97 & 10.59 & 9.88 - 11.30 \\
3823 & KOI-1270 & 1.52 & 0.021 & 0.85 & 0.84 -  0.87 & 0.82 & 0.81 -  0.83 & 13.01 & 11.01 - 14.37 \\
3824 & KOI-2969 & 1.34 & 0.72 & 1.99 & 1.88 -  2.09 & 1.36 & 1.32 -  1.39 & 3.90 & 3.69 -  4.19 \\
3825 & KOI-2488 & 1.09 & 0.016 & 1.49 & 1.46 -  1.52 & 1.11 & 1.09 -  1.11 & 5.84 & 5.49 -  6.34 \\
3826 & KOI-139 & 1.49 & 0.014 & 1.17 & 1.15 -  1.19 & 1.08 & 1.07 -  1.09 & 5.14 & 4.61 -  5.65 \\
3827 & KOI-1275 & 1.53 & 0.016 & 1.20 & 1.18 -  1.22 & 1.02 & 1.01 -  1.03 & 7.29 & 6.82 -  7.83 \\
3828 & KOI-981 & 1.7 & 0.024 & 5.33 & 5.23 -  5.43 & 1.02 & 1.00 -  1.06 & 8.65 & 7.71 -  9.33 \\
3829 & KOI-3946 & 1.01 & 0.019 & 1.76 & 1.73 -  1.81 & 1.29 & 1.28 -  1.32 & 3.05 & 2.89 -  3.13 \\
3830 & KOI-4580 & 1.35 & 0.02 & 1.76 & 1.71 -  1.79 & 1.13 & 1.09 -  1.15 & 5.02 & 4.52 -  5.41 \\
3831 & KOI-579 & 2.28 & 0.015 & 0.79 & 0.78 -  0.80 & 0.84 & 0.83 -  0.86 & 4.62 & 2.18 -  7.29 \\
3832 & KOI-2503 & 2.64 & 0.017 & 0.78 & 0.78 -  0.79 & 0.77 & 0.77 -  0.78 & 13.84 & 12.25 - 14.68 \\
3833 & KOI-1754 & 1.55 & 0.015 & 1.18 & 1.16 -  1.20 & 1.16 & 1.14 -  1.17 & 2.38 & 1.89 -  2.87 \\
3834 & KOI-2111 & 1.11 & 0.02 & 0.95 & 0.93 -  0.97 & 0.93 & 0.92 -  0.95 & 7.30 & 5.75 -  8.74 \\
3835 & KOI-4775 & 1.35 & 0.018 & 2.28 & 2.24 -  2.33 & 1.16 & 1.14 -  1.20 & 7.18 & 6.27 -  7.75 \\
3836 & KOI-2414 & 1.09 & 0.013 & 1.67 & 1.64 -  1.70 & 0.97 & 0.95 -  0.97 & 8.59 & 8.23 -  9.09 \\
3837 & KOI-1279 & 1.51 & 0.015 & 1.08 & 1.06 -  1.11 & 0.95 & 0.94 -  0.96 & 8.15 & 7.62 -  8.65 \\
3838 & KOI-1271 & 0.907 & 0.014 & 1.65 & 1.61 -  1.68 & 1.20 & 1.19 -  1.22 & 3.89 & 3.78 -  3.93 \\
3839 & KOI-1278 & 0.719 & 0.024 & 1.10 & 1.06 -  1.13 & 0.92 & 0.91 -  0.93 & 8.50 & 7.77 -  9.20 \\
3840 & Kepler-282 & 0.719 & 0.024 & 1.09 & 1.06 -  1.13 & 0.89 & 0.88 -  0.90 & 9.83 & 9.16 - 10.49 \\
3841 & KOI-1891 & 1.37 & 0.027 & 0.81 & 0.80 -  0.82 & 0.79 & 0.79 -  0.80 & 13.24 & 10.94 - 14.48 \\
3842 & KOI-4066 & 1.12 & 0.015 & 1.45 & 1.42 -  1.48 & 1.23 & 1.22 -  1.25 & 3.48 & 3.32 -  3.63 \\
3843 & KOI-2758 & 1.43 & 0.024 & 3.71 & 3.64 -  3.78 & 1.49 & 1.36 -  1.57 & 3.18 & 2.70 -  4.38 \\
3844 & KOI-1283 & 2.73 & 0.022 & 1.57 & 1.55 -  1.59 & 1.04 & 1.04 -  1.07 & 6.41 & 5.86 -  6.64 \\
3845 & KOI-105 & 2.5 & 0.022 & 1.04 & 1.02 -  1.05 & 0.83 & 0.82 -  0.84 & 12.18 & 11.43 - 13.01 \\
3846 & KOI-921 & 1.16 & 0.028 & 0.82 & 0.81 -  0.84 & 0.81 & 0.80 -  0.82 & 12.76 & 10.00 - 14.35 \\
3847 & KOI-172 & 1.34 & 0.014 & 1.20 & 1.18 -  1.22 & 0.92 & 0.92 -  0.93 & 9.28 & 8.87 -  9.63 \\
3848 & KOI-319 & 1.49 & 0.022 & 2.16 & 2.12 -  2.20 & 1.40 & 1.35 -  1.40 & 3.50 & 3.39 -  3.88 \\
3849 & KOI-374 & 2.53 & 0.026 & 1.22 & 1.21 -  1.24 & 0.99 & 0.98 -  1.00 & 7.09 & 6.74 -  7.49 \\
3850 & KOI-1629 & 1.3 & 0.016 & 1.34 & 1.31 -  1.36 & 1.11 & 1.08 -  1.13 & 6.21 & 5.55 -  7.15 \\
3851 & KOI-2749 & 1.79 & 0.03 & 2.48 & 2.43 -  2.54 & 1.46 & 1.46 -  1.51 & 2.88 & 2.60 -  3.01 \\
3852 & KOI-2473 & 1.2 & 0.032 & 0.74 & 0.72 -  0.75 & 0.78 & 0.76 -  0.80 & 5.43 & 1.95 -  9.63 \\
3853 & KOI-3891 & 0.974 & 0.018 & 2.36 & 2.31 -  2.43 & 1.03 & 0.99 -  1.08 & 10.25 & 8.60 - 11.71 \\
3854 & KOI-4301 & 1.78 & 0.015 & 1.21 & 1.18 -  1.23 & 1.00 & 0.99 -  1.01 & 6.49 & 6.06 -  6.90 \\
3855 & KOI-1257 & -0.336 & 0.25 & 1.59 & 1.50 -  1.71 & 0.97 & 0.94 -  1.00 & 12.98 & 11.50 - 14.11 \\
3856 & KOI-2017 & 2.54 & 0.016 & 0.90 & 0.89 -  0.91 & 0.96 & 0.95 -  0.98 & 2.81 & 1.59 -  4.09 \\
3857 & KOI-1904 & 3.51 & 0.016 & 0.77 & 0.76 -  0.78 & 0.81 & 0.79 -  0.83 & 5.79 & 2.80 -  8.74 \\
3858 & KOI-4251 & 1.9 & 0.015 & 0.93 & 0.92 -  0.95 & 0.91 & 0.89 -  0.92 & 8.19 & 6.94 -  9.40 \\
3859 & KOI-2159 & 1.82 & 0.015 & 1.03 & 1.01 -  1.05 & 0.99 & 0.97 -  1.00 & 6.24 & 5.35 -  7.14 \\
3860 & KOI-694 & 1.54 & 0.019 & 0.99 & 0.97 -  1.01 & 0.98 & 0.97 -  1.00 & 5.72 & 4.56 -  6.82 \\
3861 & KOI-2039 & 1.47 & 0.018 & 0.94 & 0.92 -  0.96 & 0.94 & 0.93 -  0.96 & 6.64 & 5.10 -  8.16 \\
3862 & KOI-1850 & 1.01 & 0.018 & 1.33 & 1.30 -  1.36 & 1.05 & 1.04 -  1.06 & 7.49 & 7.00 -  7.95 \\
3863 & KOI-1276 & 1.14 & 0.019 & 0.99 & 0.97 -  1.02 & 0.92 & 0.91 -  0.93 & 9.46 & 8.14 - 10.71 \\
3864 & KOI-695 & 1.92 & 0.017 & 0.94 & 0.92 -  0.95 & 0.85 & 0.84 -  0.86 & 8.59 & 7.60 -  9.51 \\
3865 & KOI-3052 & 1.85 & 0.014 & 1.15 & 1.13 -  1.16 & 0.83 & 0.82 -  0.83 & 14.70 & 14.31 - 14.92 \\
3866 & KOI-2956 & 1.53 & 0.02 & 2.09 & 2.05 -  2.13 & 1.48 & 1.47 -  1.50 & 2.45 & 2.38 -  2.54 \\
3867 & KOI-3886 &  &  & 11.45 & 11.04 - 12.00 & 2.56 & 2.54 -  2.62 & 0.66 & 0.64 -  0.66 \\
3868 & KOI-1274 & 2.84 & 0.017 & 0.84 & 0.83 -  0.84 & 0.76 & 0.76 -  0.77 & 14.38 & 13.54 - 14.83 \\
3869 & KOI-4811 & 0.817 & 0.018 & 2.12 & 2.08 -  2.18 & 1.21 & 1.16 -  1.24 & 5.35 & 4.86 -  6.16 \\
3870 & KOI-2659 & 0.906 & 0.019 & 3.70 & 3.62 -  3.78 & 1.26 & 1.20 -  1.33 & 5.41 & 4.52 -  6.34 \\
3871 & KOI-464 & 1.58 & 0.024 & 0.93 & 0.91 -  0.95 & 0.90 & 0.89 -  0.92 & 9.23 & 7.35 - 10.95 \\
3872 & KOI-3541 & 0.818 & 0.012 & 1.88 & 1.85 -  1.92 & 1.22 & 1.21 -  1.24 & 4.03 & 3.59 -  4.13 \\
3873 & KOI-2641 & 0.986 & 0.018 & 1.60 & 1.57 -  1.64 & 1.07 & 1.06 -  1.09 & 7.52 & 7.06 -  7.93 \\
3874 & KOI-465 & 0.836 & 0.02 & 1.46 & 1.42 -  1.51 & 1.17 & 1.15 -  1.19 & 4.91 & 4.46 -  5.32 \\
3875 & KOI-697 &  &  & 1.36 & 1.27 -  1.46 & 1.05 & 1.03 -  1.07 & 8.03 & 7.56 -  8.51 \\
3876 & KOI-4269 & 0.94 & 0.017 & 3.19 & 3.13 -  3.25 & 1.13 & 1.09 -  1.19 & 7.56 & 6.25 -  8.62 \\
3877 & WASP-58 & 3.41 & 0.021 & 1.17 & 1.16 -  1.19 & 0.95 & 0.94 -  0.96 & 7.96 & 7.62 -  8.31 \\
3878 & KOI-3473 & 2.88 & 0.02 & 0.77 & 0.76 -  0.78 & 0.83 & 0.81 -  0.85 & 3.66 & 1.46 -  6.16 \\
3879 & KOI-698 & 0.698 & 0.024 & 1.64 & 1.59 -  1.70 & 1.28 & 1.26 -  1.30 & 3.50 & 3.37 -  3.74 \\
3880 & KOI-2595 & 1.11 & 0.018 & 1.58 & 1.54 -  1.61 & 1.29 & 1.28 -  1.30 & 3.14 & 3.03 -  3.26 \\
3881 & KOI-2517 & 1.22 & 0.039 & 0.96 & 0.93 -  0.99 & 0.86 & 0.85 -  0.87 & 10.19 & 8.90 - 11.36 \\
3882 & KOI-700 & 2.03 & 0.015 & 0.90 & 0.89 -  0.92 & 0.81 & 0.79 -  0.82 & 10.53 & 9.41 - 11.68 \\
3883 & Kepler-215 & 2.03 & 0.015 & 0.90 & 0.89 -  0.92 & 0.79 & 0.78 -  0.80 & 11.51 & 10.44 - 12.58 \\
3884 & KOI-1412 & 1.03 & 0.015 & 1.57 & 1.54 -  1.61 & 1.16 & 1.13 -  1.20 & 5.79 & 5.00 -  6.26 \\
3885 & KOI-159 & 1.57 & 0.018 & 1.16 & 1.14 -  1.18 & 1.06 & 1.05 -  1.08 & 4.86 & 4.34 -  5.34 \\
3886 & KOI-2038 & 1.28 & 0.023 & 0.90 & 0.88 -  0.92 & 0.90 & 0.89 -  0.92 & 7.29 & 5.24 -  9.25 \\
3887 & KOI-3227 & 2.68 & 0.031 & 1.19 & 1.17 -  1.21 & 1.07 & 1.05 -  1.08 & 5.40 & 4.92 -  5.88 \\
3888 & KOI-4585 & 0.85 & 0.013 & 1.90 & 1.86 -  1.95 & 1.27 & 1.20 -  1.28 & 3.40 & 3.22 -  4.48 \\
3889 & KOI-582 & 1.65 & 0.022 & 0.81 & 0.79 -  0.83 & 0.83 & 0.81 -  0.85 & 8.88 & 5.44 - 11.99 \\
3890 & KOI-2319 & 1.35 & 0.016 & 1.29 & 1.26 -  1.31 & 1.09 & 1.08 -  1.11 & 5.18 & 4.90 -  5.48 \\
3891 & KOI-3196 & 3.05 & 0.021 & 1.30 & 1.28 -  1.32 & 1.13 & 1.12 -  1.14 & 4.56 & 4.27 -  4.83 \\
3892 & KOI-2530 & 0.883 & 0.017 & 1.87 & 1.83 -  1.91 & 1.24 & 1.20 -  1.27 & 4.86 & 4.41 -  5.42 \\
3893 & KOI-2768 & 1.2 & 0.022 & 0.82 & 0.80 -  0.84 & 0.81 & 0.80 -  0.83 & 9.29 & 6.56 - 11.71 \\
3894 & KOI-4014 & 1.36 & 0.017 & 1.13 & 1.11 -  1.15 & 1.07 & 1.06 -  1.08 & 4.46 & 3.84 -  5.05 \\
3895 & KOI-134 & 0.834 & 0.012 & 1.85 & 1.81 -  1.89 & 1.42 & 1.41 -  1.43 & 2.76 & 2.67 -  2.86 \\
3896 & KOI-1413 & 0.559 & 0.024 & 2.42 & 2.33 -  2.51 & 1.14 & 1.06 -  1.26 & 6.77 & 4.67 -  8.68 \\
3897 & KOI-1616 & 3.2 & 0.022 & 1.24 & 1.22 -  1.26 & 1.15 & 1.14 -  1.16 & 3.65 & 3.28 -  4.03 \\
3898 & KOI-2564 & 0.644 & 0.016 & 2.04 & 1.99 -  2.10 & 1.33 & 1.30 -  1.35 & 3.08 & 2.93 -  3.18 \\
3899 & KOI-2175 & 1.27 & 0.023 & 2.21 & 2.17 -  2.26 & 1.26 & 1.21 -  1.28 & 4.74 & 4.45 -  5.51 \\
3900 & KOI-2833 & 2.08 & 0.026 & 1.28 & 1.25 -  1.30 & 1.07 & 1.06 -  1.08 & 4.90 & 4.60 -  5.18 \\
3901 & KOI-2367 & 1.66 & 0.021 & 1.51 & 1.48 -  1.54 & 1.24 & 1.23 -  1.26 & 3.92 & 3.76 -  4.07 \\
3902 & KOI-2470 & 1.38 & 0.025 & 1.29 & 1.26 -  1.31 & 1.10 & 1.08 -  1.12 & 5.95 & 5.51 -  6.72 \\
3903 & KOI-3008 & 1.84 & 0.022 & 1.78 & 1.75 -  1.81 & 1.18 & 1.17 -  1.23 & 4.56 & 3.98 -  4.72 \\
3904 & KOI-2640 & 0.419 & 0.015 & 7.42 & 7.20 -  7.64 & 1.35 & 1.34 -  1.40 & 3.73 & 3.34 -  3.82 \\
3905 & KOI-4060 & 1.05 & 0.018 & 1.52 & 1.49 -  1.55 & 1.09 & 1.08 -  1.10 & 7.53 & 7.19 -  7.90 \\
3906 & KOI-3249 & 2.1 & 0.024 & 1.28 & 1.26 -  1.30 & 1.12 & 1.11 -  1.13 & 4.80 & 4.48 -  5.11 \\
3907 & HAT-P-40 & 2.12 & 0.03 & 2.13 & 2.09 -  2.17 & 1.45 & 1.43 -  1.47 & 3.14 & 3.00 -  3.23 \\
3908 & KOI-4839 & 1.2 & 0.018 & 1.47 & 1.44 -  1.50 & 1.17 & 1.15 -  1.19 & 4.29 & 4.03 -  4.63 \\
3909 & KOI-4198 & 1.21 & 0.023 & 2.01 & 1.96 -  2.05 & 1.19 & 1.16 -  1.20 & 4.06 & 4.00 -  4.34 \\
3910 & KOI-3087 & 3.6 & 0.023 & 0.88 & 0.86 -  0.89 & 0.88 & 0.86 -  0.89 & 8.99 & 6.90 - 10.90 \\
3911 & KOI-3425 & 1.05 & 0.017 & 2.17 & 2.12 -  2.23 & 1.34 & 1.30 -  1.37 & 3.76 & 3.42 -  4.02 \\
3912 & KOI-2874 & 1.36 & 0.022 & 0.83 & 0.81 -  0.85 & 0.81 & 0.80 -  0.83 & 10.17 & 7.80 - 12.37 \\
3913 & KOI-323 & 3.92 & 0.025 & 0.84 & 0.83 -  0.86 & 0.91 & 0.90 -  0.92 & 3.38 & 1.69 -  5.16 \\
3914 & KOI-703 & 0.845 & 0.014 & 2.18 & 2.13 -  2.23 & 1.55 & 1.54 -  1.57 & 2.23 & 2.16 -  2.31 \\
3915 & KOI-2522 & 3.2 & 0.016 & 0.80 & 0.79 -  0.81 & 0.79 & 0.78 -  0.81 & 12.27 & 9.55 - 14.16 \\
3916 & KOI-584 & 1.51 & 0.016 & 1.05 & 1.03 -  1.07 & 0.92 & 0.91 -  0.93 & 11.80 & 10.71 - 12.84 \\
3917 & Kepler-192 & 1.51 & 0.016 & 1.04 & 1.02 -  1.06 & 0.92 & 0.91 -  0.94 & 11.31 & 10.23 - 12.30 \\
3918 & KOI-4222 & 1.45 & 0.017 & 1.23 & 1.20 -  1.25 & 0.96 & 0.95 -  0.97 & 9.00 & 8.61 -  9.46 \\
3919 & KOI-2443 & 1.22 & 0.017 & 1.16 & 1.13 -  1.18 & 0.92 & 0.91 -  0.93 & 8.82 & 8.38 -  9.25 \\
3920 & KOI-2281 & 2.62 & 0.017 & 0.81 & 0.80 -  0.82 & 0.81 & 0.80 -  0.83 & 10.31 & 7.46 - 12.92 \\
3921 & KOI-2162 & 1.54 & 0.017 & 0.91 & 0.89 -  0.93 & 0.86 & 0.85 -  0.88 & 7.17 & 6.02 -  8.31 \\
3922 & KOI-4318 & 1.67 & 0.019 & 1.35 & 1.32 -  1.37 & 1.24 & 1.23 -  1.25 & 2.48 & 2.24 -  2.71 \\
3923 & KOI-704 & 2.53 & 0.013 & 0.79 & 0.78 -  0.80 & 0.82 & 0.80 -  0.83 & 6.62 & 4.31 -  8.82 \\
3924 & KOI-2657 &  &  & 0.83 & 0.79 -  0.87 & 0.83 & 0.81 -  0.85 & 7.56 & 3.96 - 10.77 \\
3925 & KOI-3114 & 1.12 & 0.025 & 2.50 & 2.45 -  2.57 & 1.57 & 1.55 -  1.60 & 2.49 & 2.27 -  2.64 \\
3926 & KOI-3867 & 1.13 & 0.024 & 0.96 & 0.94 -  0.98 & 0.93 & 0.91 -  0.94 & 8.06 & 6.41 -  9.63 \\
3927 & KOI-4215 & 1.06 & 0.017 & 1.77 & 1.73 -  1.80 & 0.97 & 0.96 -  0.99 & 8.39 & 7.91 -  8.94 \\
3928 & KOI-2137 & 2.36 & 0.016 & 0.84 & 0.83 -  0.85 & 0.78 & 0.77 -  0.79 & 13.05 & 11.51 - 14.28 \\
3929 & KOI-1411 & 1.81 & 0.016 & 1.21 & 1.18 -  1.23 & 1.00 & 0.99 -  1.01 & 9.65 & 8.91 - 10.41 \\
3930 & KOI-4640 & 0.785 & 0.018 & 1.77 & 1.72 -  1.82 & 1.38 & 1.36 -  1.39 & 2.70 & 2.62 -  2.78 \\
3931 & KOI-1922 & 0.685 & 0.03 & 1.16 & 1.12 -  1.21 & 0.98 & 0.97 -  0.99 & 8.54 & 7.86 -  9.36 \\
3932 & KOI-974 & 4.67 & 0.028 & 2.00 & 1.97 -  2.03 & 1.39 & 1.33 -  1.40 & 3.18 & 3.08 -  3.62 \\
3933 & KOI-1835 & 2.02 & 0.045 & 0.95 & 0.94 -  0.97 & 0.85 & 0.85 -  0.86 & 14.85 & 14.60 - 14.96 \\
3934 & KOI-707 & 0.798 & 0.015 & 1.74 & 1.70 -  1.79 & 1.17 & 1.16 -  1.22 & 5.73 & 4.90 -  6.08 \\
3935 & Kepler-33 & 0.798 & 0.015 & 1.74 & 1.70 -  1.78 & 1.21 & 1.16 -  1.23 & 5.05 & 4.76 -  5.94 \\
3936 & KOI-2079 & 2.73 & 0.026 & 1.02 & 1.00 -  1.04 & 0.93 & 0.92 -  0.94 & 11.06 & 9.85 - 12.22 \\
3937 & KOI-2786 & 0.709 & 0.013 & 1.82 & 1.79 -  1.92 & 1.33 & 1.32 -  1.39 & 2.79 & 2.57 -  2.93 \\
3938 & KOI-941 & 1.25 & 0.028 & 0.87 & 0.83 -  0.90 & 0.88 & 0.86 -  0.90 & 8.59 & 3.85 - 12.48 \\
3939 & Kepler-127 & 2.81 & 0.021 & 1.44 & 1.42 -  1.47 & 1.26 & 1.25 -  1.27 & 3.36 & 3.21 -  3.52 \\
3940 & KOI-271 & 2.81 & 0.021 & 1.44 & 1.42 -  1.47 & 1.26 & 1.25 -  1.27 & 3.35 & 3.17 -  3.53 \\
3941 & KOI-4637 & 3.29 & 0.026 & 1.92 & 1.89 -  1.94 & 1.35 & 1.34 -  1.35 & 2.69 & 2.61 -  2.92 \\
3942 & KOI-2029 & 3.93 & 0.022 & 0.76 & 0.75 -  0.77 & 0.80 & 0.79 -  0.82 & 4.90 & 2.21 -  7.33 \\
3943 & KOI-2694 & 2.05 & 0.025 & 0.76 & 0.74 -  0.77 & 0.80 & 0.78 -  0.81 & 6.68 & 2.89 - 10.79 \\
3944 & KOI-2246 & 1.42 & 0.015 & 0.96 & 0.94 -  0.98 & 0.89 & 0.88 -  0.90 & 7.61 & 6.67 -  8.51 \\
3945 & KOI-119 & 0.775 & 0.088 & 2.72 & 2.60 -  2.88 & 1.52 & 1.46 -  1.61 & 2.95 & 2.40 -  3.43 \\
3946 & KOI-110 & 1.78 & 0.022 & 1.28 & 1.26 -  1.31 & 1.11 & 1.10 -  1.12 & 4.24 & 3.97 -  4.50 \\
3947 & KOI-1813 & 2.19 & 0.014 & 0.86 & 0.85 -  0.88 & 0.86 & 0.85 -  0.88 & 8.22 & 6.42 -  9.99 \\
3948 & KOI-2082 & 0.906 & 0.019 & 1.46 & 1.42 -  1.50 & 1.23 & 1.22 -  1.25 & 3.94 & 3.77 -  4.11 \\
3949 & KOI-939 & 0.946 & 0.022 & 1.05 & 1.02 -  1.08 & 0.94 & 0.92 -  0.95 & 10.30 & 8.97 - 11.48 \\
3950 & KOI-2717 & 2.12 & 0.022 & 1.27 & 1.25 -  1.30 & 1.12 & 1.11 -  1.13 & 4.65 & 4.34 -  4.98 \\
3951 & KOI-1978 & 0.988 & 0.027 & 0.91 & 0.89 -  0.94 & 0.92 & 0.91 -  0.94 & 6.38 & 4.14 -  8.38 \\
3952 & KOI-708 & 0.813 & 0.015 & 1.64 & 1.61 -  1.68 & 1.20 & 1.18 -  1.24 & 4.27 & 3.86 -  4.49 \\
3953 & KOI-3132 & 0.981 & 0.025 & 2.52 & 2.46 -  2.59 & 1.63 & 1.61 -  1.65 & 2.13 & 2.04 -  2.20 \\
3954 & KOI-49 & 1.42 & 0.014 & 1.33 & 1.31 -  1.35 & 1.05 & 1.04 -  1.05 & 6.62 & 6.34 -  6.93 \\
3955 & KOI-1806 & 1.18 & 0.015 & 1.32 & 1.29 -  1.35 & 1.13 & 1.11 -  1.14 & 4.58 & 4.27 -  4.84 \\
3956 & KOI-165 & 1.49 & 0.35 & 0.77 & 0.75 -  0.78 & 0.73 & 0.73 -  0.74 & 13.83 & 11.93 - 14.70 \\
3957 & KOI-1886 & 1.81 & 0.027 & 1.64 & 1.60 -  1.67 & 1.25 & 1.22 -  1.28 & 4.03 & 3.69 -  4.41 \\
3958 & KOI-709 & 1.93 & 0.013 & 0.88 & 0.86 -  0.89 & 0.79 & 0.78 -  0.80 & 13.27 & 12.00 - 14.29 \\
3959 & KOI-3165 & 3.45 & 0.021 & 1.89 & 1.84 -  1.92 & 1.32 & 1.30 -  1.35 & 2.84 & 2.66 -  2.97 \\
3960 & KOI-3232 & 3.34 & 0.02 & 0.95 & 0.94 -  0.97 & 1.04 & 1.02 -  1.05 & 1.46 & 0.74 -  2.32 \\
3961 & KOI-288 & 2.41 & 0.025 & 2.15 & 2.11 -  2.19 & 1.47 & 1.46 -  1.49 & 2.92 & 2.76 -  3.05 \\
3962 & KOI-1819 & 2.4 & 0.013 & 0.84 & 0.82 -  0.85 & 0.89 & 0.87 -  0.90 & 4.36 & 2.52 -  6.23 \\
3963 & KOI-3229 & 3.15 & 0.024 &  &  &  &  &  &  \\
3964 & KOI-711 & 1.49 & 0.015 & 1.11 & 1.09 -  1.13 & 0.98 & 0.97 -  0.99 & 9.31 & 8.53 - 10.18 \\
3965 & KOI-115 & 2.15 & 0.026 & 1.06 & 1.04 -  1.08 & 1.01 & 1.00 -  1.03 & 4.64 & 4.00 -  5.24 \\
3966 & KOI-710 & 0.876 & 0.013 & 1.93 & 1.90 -  1.97 & 1.40 & 1.38 -  1.41 & 2.64 & 2.53 -  2.72 \\
3967 & Kepler-217 & 0.876 & 0.013 & 1.86 & 1.82 -  1.91 & 1.43 & 1.41 -  1.44 & 2.37 & 2.30 -  2.44 \\
3968 & KOI-2612 & 4.1 & 0.025 & 1.07 & 1.05 -  1.09 & 0.94 & 0.92 -  0.95 & 11.18 & 10.17 - 12.21 \\
3969 & KOI-2884 & 0.392 & 0.031 & 2.86 & 2.75 -  2.98 & 1.40 & 1.31 -  1.47 & 3.29 & 2.83 -  3.82 \\
3970 & KOI-1970 & 0.969 & 0.029 & 0.90 & 0.87 -  0.93 & 0.91 & 0.90 -  0.93 & 6.37 & 3.91 -  8.73 \\
3971 & KOI-4430 & 1.12 & 0.027 & 0.82 & 0.81 -  0.83 & 0.80 & 0.79 -  0.81 & 12.96 & 10.33 - 14.44 \\
3972 & KOI-179 & 0.599 & 0.017 & 2.34 & 2.27 -  2.41 & 1.53 & 1.52 -  1.56 & 2.65 & 2.49 -  2.73 \\
3973 & KOI-2049 & 0.989 & 0.015 & 1.44 & 1.41 -  1.47 & 1.09 & 1.08 -  1.11 & 6.69 & 6.30 -  7.06 \\
3974 & KOI-712 &  &  & 0.88 & 0.84 -  0.92 & 0.86 & 0.84 -  0.88 & 9.07 & 5.31 - 11.83 \\
3975 & KOI-1938 & 2.38 & 0.024 & 0.77 & 0.76 -  0.78 & 0.74 & 0.73 -  0.75 & 13.35 & 11.38 - 14.50 \\
3976 & KOI-2815 & 1.47 & 0.018 & 1.22 & 1.20 -  1.24 & 1.03 & 1.02 -  1.04 & 6.47 & 6.17 -  6.79 \\
3977 & Kepler-423 & 1.29 & 0.022 & 1.01 & 0.98 -  1.03 & 0.96 & 0.95 -  0.97 & 7.33 & 6.18 -  8.37 \\
3978 & KOI-1854 & 2.14 & 0.015 & 0.95 & 0.93 -  0.96 & 0.92 & 0.91 -  0.93 & 7.50 & 6.40 -  8.57 \\
3979 & KOI-4822 & 1.04 & 0.014 & 1.73 & 1.70 -  1.76 & 1.09 & 1.08 -  1.11 & 6.88 & 6.51 -  7.25 \\
3980 & KOI-4617 & 1.08 & 0.016 & 1.44 & 1.42 -  1.47 & 1.06 & 1.06 -  1.10 & 5.96 & 5.41 -  6.24 \\
3981 & KOI-2831 & 1.24 & 0.019 & 2.31 & 2.26 -  2.35 & 1.13 & 1.11 -  1.15 & 6.12 & 5.73 -  6.43 \\
3982 & KOI-2706 & 3.33 & 0.027 & 2.00 & 1.97 -  2.04 & 1.44 & 1.43 -  1.45 & 2.85 & 2.77 -  2.94 \\
3983 & KOI-2769 & 0.835 & 0.013 & 2.05 & 2.01 -  2.10 & 1.11 & 1.10 -  1.12 & 6.22 & 5.73 -  6.59 \\
3984 & KOI-2545 & 1.6 & 0.029 & 2.26 & 2.22 -  2.32 & 1.47 & 1.45 -  1.50 & 2.96 & 2.76 -  3.17 \\
3985 & KOI-1751 & 2.03 & 0.023 & 0.78 & 0.77 -  0.79 & 0.80 & 0.78 -  0.82 & 8.18 & 5.00 - 11.17 \\
3986 & KOI-1913 & 2.4 & 0.014 & 0.92 & 0.91 -  0.94 & 0.92 & 0.91 -  0.94 & 7.28 & 5.93 -  8.70 \\
3987 & KOI-714 & 2.51 & 0.014 & 0.87 & 0.86 -  0.89 & 0.87 & 0.86 -  0.88 & 8.79 & 7.01 - 10.59 \\
3988 & KOI-2913 & 1.42 & 0.033 & 1.69 & 1.66 -  1.73 & 1.21 & 1.14 -  1.25 & 5.56 & 5.02 -  6.90 \\
3989 & KOI-2273 & 1.88 & 0.018 & 1.26 & 1.24 -  1.29 & 1.16 & 1.14 -  1.17 & 3.81 & 3.42 -  4.19 \\
3990 & KOI-2035 & 2.88 & 0.021 & 0.88 & 0.87 -  0.90 & 0.94 & 0.92 -  0.95 & 3.93 & 2.42 -  5.46 \\
3991 & KOI-2457 & 0.901 & 0.022 & 2.59 & 2.54 -  2.64 & 1.62 & 1.60 -  1.64 & 1.97 & 1.92 -  2.04 \\
3992 & KOI-3871 & 5.15 & 0.26 & 0.83 & 0.81 -  0.86 & 0.83 & 0.82 -  0.85 & 9.75 & 5.83 - 12.94 \\
3993 & KOI-3162 & 5.12 & 0.022 & 1.54 & 1.52 -  1.56 & 1.18 & 1.17 -  1.19 & 4.98 & 4.79 -  5.23 \\
3994 & KOI-3465 & 3.09 & 0.014 & 0.84 & 0.83 -  0.86 & 0.85 & 0.83 -  0.86 & 8.79 & 6.73 - 10.71 \\
3995 & KOI-3837 & 0.827 & 0.025 & 1.36 & 1.33 -  1.40 & 1.22 & 1.20 -  1.23 & 2.80 & 2.53 -  3.05 \\
3996 & KOI-1852 & 1.22 & 0.023 & 1.46 & 1.43 -  1.50 & 1.23 & 1.22 -  1.24 & 3.08 & 2.91 -  3.24 \\
3997 & KOI-1529 & 0.831 & 0.016 & 1.43 & 1.39 -  1.46 & 1.00 & 0.99 -  1.02 & 7.27 & 6.83 -  7.66 \\
3998 & KOI-2943 & 0.934 & 0.016 & 1.66 & 1.62 -  1.70 & 1.22 & 1.16 -  1.25 & 5.26 & 4.84 -  6.44 \\
3999 & KOI-135 & 0.965 & 0.014 & 1.46 & 1.42 -  1.49 & 1.23 & 1.22 -  1.25 & 3.92 & 3.74 -  4.09 \\
4000 & KOI-4421 & 1.67 & 0.027 & 1.43 & 1.41 -  1.47 & 1.10 & 1.09 -  1.12 & 6.44 & 6.04 -  6.82 \\
4001 & KOI-1715 & 1.97 & 0.019 & 1.18 & 1.16 -  1.21 & 0.93 & 0.92 -  0.94 & 8.94 & 8.50 -  9.30 \\
4002 & KOI-1958 & 0.803 & 0.026 & 1.05 & 1.02 -  1.09 & 1.01 & 1.00 -  1.03 & 5.44 & 4.21 -  6.55 \\
4003 & KOI-716 & 0.907 & 0.016 & 1.77 & 1.74 -  1.81 & 1.31 & 1.29 -  1.32 & 3.82 & 3.68 -  3.98 \\
4004 & KOI-1606 & 1.86 & 0.014 & 0.92 & 0.90 -  0.93 & 0.87 & 0.86 -  0.88 & 11.21 & 9.65 - 12.71 \\
4005 & KOI-717 & 1.65 & 0.013 & 1.26 & 1.24 -  1.28 & 0.99 & 0.98 -  1.01 & 10.67 & 10.00 - 11.37 \\
4006 & KOI-4230 & 1.03 & 0.014 & 1.50 & 1.47 -  1.52 & 0.98 & 0.96 -  0.99 & 7.94 & 7.63 -  8.40 \\
4007 & KOI-3246 & 6.55 & 0.029 & 0.74 & 0.73 -  0.75 & 0.76 & 0.75 -  0.78 & 9.27 & 5.46 - 12.36 \\
4008 & KOI-1955 & 1.25 & 0.016 & 1.45 & 1.42 -  1.48 & 1.24 & 1.23 -  1.25 & 3.53 & 3.36 -  3.68 \\
4009 & Kepler-342 & 1.25 & 0.016 & 1.46 & 1.43 -  1.49 & 1.24 & 1.22 -  1.25 & 3.61 & 3.47 -  3.75 \\
4010 & KOI-2135 & 1.05 & 0.018 & 1.55 & 1.52 -  1.58 & 1.20 & 1.18 -  1.23 & 4.46 & 4.01 -  4.89 \\
4011 & KOI-2732 & 1.16 & 0.023 & 1.92 & 1.88 -  1.96 & 1.30 & 1.27 -  1.31 & 4.06 & 3.88 -  4.26 \\
4012 & Kepler-403 & 1.16 & 0.023 & 1.93 & 1.89 -  1.97 & 1.28 & 1.26 -  1.31 & 4.16 & 3.92 -  4.34 \\
4013 & KOI-4575 & 0.85 & 0.014 & 2.28 & 2.23 -  2.33 & 1.47 & 1.45 -  1.49 & 2.79 & 2.72 -  3.03 \\
4014 & KOI-718 & 1.24 & 0.017 & 1.23 & 1.21 -  1.26 & 1.14 & 1.13 -  1.15 & 4.11 & 3.68 -  4.53 \\
4015 & Kepler-219 & 1.24 & 0.017 & 1.22 & 1.19 -  1.24 & 1.15 & 1.14 -  1.17 & 3.41 & 2.97 -  3.84 \\
4016 & KOI-327 & 1.68 & 0.02 & 1.23 & 1.20 -  1.25 & 1.10 & 1.08 -  1.11 & 4.70 & 4.34 -  5.05 \\
4017 & KOI-4383 & 1.58 & 0.019 & 0.95 & 0.94 -  0.97 & 1.01 & 0.99 -  1.02 & 2.70 & 1.61 -  3.86 \\
4018 & KOI-1537 & 1.9 & 0.022 & 1.86 & 1.83 -  1.88 & 1.30 & 1.30 -  1.31 & 3.05 & 2.97 -  3.14 \\
4019 & KOI-2803 & 3.48 & 0.023 & 1.01 & 0.99 -  1.03 & 0.94 & 0.93 -  0.95 & 8.56 & 7.61 -  9.58 \\
4020 & KOI-1779 & 2.02 & 0.013 & 1.02 & 1.00 -  1.04 & 1.08 & 1.07 -  1.10 & 1.93 & 1.10 -  2.84 \\
4021 & KOI-721 & 0.998 & 0.016 & 1.71 & 1.67 -  1.74 & 1.14 & 1.12 -  1.17 & 6.55 & 5.79 -  6.93 \\
4022 & KOI-720 & 2.57 & 0.019 & 0.81 & 0.80 -  0.82 & 0.83 & 0.81 -  0.85 & 7.81 & 5.23 - 10.20 \\
4023 & KOI-722 & 1.3 & 0.016 & 1.24 & 1.23 -  1.25 & 1.30 & 1.29 -  1.31 & 0.34 & 0.27 -  0.47 \\
4024 & KOI-4431 & 1.35 & 0.021 & 1.88 & 1.85 -  1.91 & 1.31 & 1.30 -  1.31 & 3.03 & 2.94 -  3.12 \\
4025 & KOI-1875 & 1.22 & 0.019 & 0.87 & 0.84 -  0.91 & 0.91 & 0.89 -  0.93 & 3.69 & 1.45 -  6.33 \\
4026 & KOI-4647 & 0.806 & 0.013 & 2.75 & 2.70 -  2.80 & 1.17 & 1.13 -  1.25 & 6.81 & 5.45 -  7.81 \\
4027 & KOI-528 & 1.37 & 0.02 & 0.91 & 0.90 -  0.93 & 0.84 & 0.82 -  0.85 & 11.74 & 10.29 - 13.07 \\
4028 & KOI-2748 & 0.859 & 0.018 & 1.82 & 1.79 -  1.87 & 0.98 & 0.97 -  1.00 & 8.42 & 7.95 -  8.84 \\
4029 & KOI-2832 & 2.54 & 0.014 & 0.80 & 0.79 -  0.81 & 0.80 & 0.79 -  0.82 & 10.96 & 8.02 - 13.33 \\
4030 & KOI-2312 & 0.992 & 0.024 & 2.33 & 2.28 -  2.37 & 1.44 & 1.44 -  1.50 & 2.20 & 1.91 -  2.39 \\
4031 & KOI-4146 & 3.04 & 0.014 & 0.79 & 0.78 -  0.80 & 0.86 & 0.84 -  0.87 & 3.42 & 1.44 -  5.78 \\
4032 & KOI-4706 &  &  & 1.28 & 1.20 -  1.36 & 0.99 & 0.98 -  1.01 & 7.01 & 6.57 -  7.44 \\
4033 & KOI-3382 & 1.81 & 0.02 & 1.01 & 0.99 -  1.03 & 0.88 & 0.87 -  0.89 & 13.74 & 12.66 - 14.55 \\
4034 & KOI-723 & 1.29 & 0.025 & 0.87 & 0.85 -  0.89 & 0.91 & 0.89 -  0.93 & 5.68 & 3.01 -  8.33 \\
4035 & KOI-1796 & 2.49 & 0.027 & 1.10 & 1.08 -  1.12 & 1.06 & 1.05 -  1.08 & 3.91 & 3.30 -  4.50 \\
4036 & KOI-2785 & 1.14 & 0.018 & 1.18 & 1.15 -  1.20 & 1.04 & 1.02 -  1.05 & 6.32 & 5.84 -  6.76 \\
4037 & KOI-4469 & 2.46 & 0.017 & 0.77 & 0.76 -  0.77 & 0.77 & 0.76 -  0.78 & 12.04 & 9.01 - 14.07 \\
4038 & WASP-113 & 2.27 & 0.023 & 1.66 & 1.53 -  1.79 & 1.28 & 1.24 -  1.33 & 4.10 & 3.87 -  4.28 \\
4039 & KOI-1598 & 1.63 & 0.019 & 0.87 & 0.85 -  0.89 & 0.82 & 0.81 -  0.84 & 9.99 & 8.46 - 11.54 \\
4040 & Kepler-310 & 1.63 & 0.019 & 0.87 & 0.86 -  0.89 & 0.81 & 0.80 -  0.82 & 10.91 & 9.47 - 12.26 \\
4041 & KOI-1783 & 1.13 & 0.018 & 1.21 & 1.18 -  1.23 & 1.09 & 1.08 -  1.10 & 5.08 & 4.63 -  5.54 \\
4042 & KOI-2002 & 1.79 & 0.092 & 1.09 & 1.05 -  1.13 & 1.08 & 1.07 -  1.10 & 3.10 & 2.02 -  4.06 \\
4043 & KOI-1984 & 1.33 & 0.016 & 1.20 & 1.17 -  1.22 & 1.10 & 1.09 -  1.11 & 4.52 & 4.08 -  4.96 \\
4044 & HAT-P-44 & 2.85 & 0.018 & 0.96 & 0.95 -  0.98 & 0.91 & 0.90 -  0.92 & 10.34 & 9.04 - 11.61 \\
4045 & KOI-4292 & 2.45 & 0.018 & 1.06 & 1.05 -  1.08 & 0.91 & 0.90 -  0.92 & 10.36 & 9.89 - 10.77 \\
4046 & KOI-2891 & 0.91 & 0.32 & 2.05 & 1.93 -  2.16 & 1.38 & 1.33 -  1.41 & 3.58 & 3.37 -  3.81 \\
4047 & KOI-1917 & 1.42 & 0.014 & 1.14 & 1.12 -  1.16 & 1.01 & 1.00 -  1.02 & 6.10 & 5.60 -  6.58 \\
4048 & KOI-2964 & 0.806 & 0.017 & 1.82 & 1.78 -  1.87 & 1.09 & 1.08 -  1.10 & 5.45 & 5.12 -  5.59 \\
4049 & KOI-1608 & 1.26 & 0.015 & 1.19 & 1.16 -  1.21 & 1.04 & 1.03 -  1.05 & 5.96 & 5.56 -  6.36 \\
4050 & KOI-1888 & 0.868 & 0.013 & 1.92 & 1.88 -  1.96 & 1.44 & 1.42 -  1.45 & 2.64 & 2.54 -  2.73 \\
4051 & KOI-1909 & 2.32 & 0.024 & 1.04 & 1.02 -  1.06 & 1.03 & 1.02 -  1.05 & 3.97 & 3.14 -  4.74 \\
4052 & Kepler-334 & 2.32 & 0.024 & 1.03 & 1.01 -  1.05 & 1.06 & 1.04 -  1.07 & 2.83 & 2.10 -  3.57 \\
4053 & KOI-1929 & 1.45 & 0.02 & 1.89 & 1.86 -  1.93 & 1.12 & 1.09 -  1.14 & 7.08 & 6.67 -  7.71 \\
4054 & KOI-3195 & 1.88 & 0.025 & 2.23 & 2.20 -  2.28 & 1.22 & 1.20 -  1.27 & 3.85 & 3.18 -  4.13 \\
4055 & KOI-1784 &  &  & 1.03 & 1.01 -  1.06 & 1.11 & 1.09 -  1.12 & 0.96 & 0.45 -  1.92 \\
4056 & KOI-3208 & 3.32 & 0.022 & 1.00 & 0.99 -  1.02 & 1.00 & 0.99 -  1.02 & 3.89 & 3.17 -  4.60 \\
4057 & KOI-991 & 2.19 & 0.023 & 0.90 & 0.88 -  0.91 & 0.82 & 0.81 -  0.83 & 10.88 & 9.59 - 12.13 \\
4058 & KOI-4613 & 2.0 & 0.013 & 0.84 & 0.83 -  0.86 & 0.86 & 0.85 -  0.87 & 5.97 & 4.37 -  7.50 \\
4059 & KOI-3218 & 3.0 & 0.019 & 1.09 & 1.07 -  1.10 & 1.09 & 1.08 -  1.11 & 2.76 & 2.16 -  3.34 \\
4060 & KOI-4070 & 2.15 & 0.017 & 0.77 & 0.77 -  0.78 & 0.76 & 0.76 -  0.77 & 13.31 & 11.16 - 14.51 \\
4061 & KOI-2342 & 1.72 & 0.1 & 1.26 & 1.20 -  1.32 & 0.90 & 0.89 -  0.92 & 9.83 & 9.37 - 10.32 \\
4062 & KOI-427 & 1.55 & 0.017 & 0.85 & 0.83 -  0.87 & 0.87 & 0.86 -  0.89 & 7.07 & 4.63 -  9.48 \\
4063 & KOI-3130 & 3.39 & 0.015 & 0.67 & 0.66 -  0.67 & 0.66 & 0.65 -  0.66 & 13.93 & 12.39 - 14.71 \\
4064 & KOI-5782 & 1.78 & 0.025 & 3.75 & 3.69 -  3.82 & 1.33 & 1.23 -  1.38 & 4.33 & 3.89 -  5.63 \\
4065 & KOI-331 & 0.979 & 0.016 & 2.14 & 2.10 -  2.17 & 1.21 & 1.16 -  1.25 & 5.43 & 4.75 -  6.38 \\
4066 & KOI-2390 & 1.11 & 0.023 & 2.80 & 2.72 -  2.88 & 1.55 & 1.50 -  1.55 & 2.50 & 2.36 -  2.82 \\
4067 & KOI-732 & 1.09 & 0.026 & 0.90 & 0.88 -  0.92 & 0.85 & 0.84 -  0.87 & 12.92 & 10.79 - 14.33 \\
4068 & KOI-4557 & 0.973 & 0.016 & 1.64 & 1.60 -  1.68 & 1.13 & 1.12 -  1.15 & 6.37 & 6.07 -  6.65 \\
4069 & KOI-3608 & 1.42 & 0.015 & 1.25 & 1.22 -  1.27 & 1.01 & 1.01 -  1.03 & 6.86 & 6.44 -  7.15 \\
4070 & KOI-332 & 1.47 & 0.018 & 1.60 & 1.57 -  1.63 & 1.19 & 1.14 -  1.22 & 5.69 & 5.17 -  6.85 \\
4071 & KOI-2153 & 1.09 & 0.012 & 1.39 & 1.36 -  1.41 & 1.12 & 1.11 -  1.13 & 5.35 & 5.09 -  5.65 \\
4072 & KOI-333 & 1.3 & 0.013 & 1.29 & 1.27 -  1.32 & 1.18 & 1.17 -  1.19 & 3.33 & 3.02 -  3.66 \\
4073 & KOI-1905 & 2.88 & 0.015 & 0.73 & 0.71 -  0.74 & 0.73 & 0.72 -  0.75 & 10.06 & 6.61 - 12.87 \\
4074 & KOI-3216 &  &  & 0.97 & 0.93 -  1.02 & 0.98 & 0.97 -  1.00 & 4.73 & 2.28 -  6.97 \\
4075 & KOI-3908 & 1.94 & 0.021 & 1.95 & 1.91 -  1.99 & 1.16 & 1.11 -  1.18 & 6.11 & 5.65 -  6.95 \\
4076 & KOI-1175 & 0.738 & 0.012 & 3.02 & 2.97 -  3.08 & 1.44 & 1.38 -  1.48 & 3.12 & 2.88 -  3.63 \\
4077 & KOI-1169 & 1.96 & 0.012 & 1.08 & 1.07 -  1.10 & 0.96 & 0.95 -  0.97 & 9.14 & 8.47 -  9.85 \\
4078 & KOI-1165 & 1.91 & 0.018 & 0.89 & 0.87 -  0.90 & 0.82 & 0.81 -  0.83 & 12.03 & 10.62 - 13.36 \\
4079 & KOI-3991 & 3.06 & 0.11 & 0.85 & 0.84 -  0.87 & 0.93 & 0.91 -  0.94 & 2.36 & 0.96 -  4.23 \\
4080 & KOI-4446 & 1.8 & 0.022 & 2.07 & 2.04 -  2.11 & 0.84 & 0.84 -  0.86 & 14.37 & 13.25 - 14.74 \\
4081 & KOI-2147 & 0.89 & 0.045 & 1.29 & 1.24 -  1.34 & 0.93 & 0.92 -  0.95 & 9.55 & 8.88 - 10.17 \\
4082 & KOI-2859 & 1.91 & 0.021 & 0.96 & 0.95 -  0.99 & 0.81 & 0.81 -  0.82 & 14.82 & 14.68 - 14.94 \\
4083 & KOI-4556 & 1.81 & 0.023 & 2.19 & 2.17 -  2.20 & 0.99 & 0.99 -  0.99 & 8.56 & 8.35 -  8.75 \\
4084 & KOI-289 & 1.51 & 0.024 & 1.68 & 1.64 -  1.71 & 1.12 & 1.09 -  1.14 & 4.91 & 4.70 -  5.31 \\
4085 & KOI-3224 & 4.65 & 0.021 & 0.85 & 0.83 -  0.86 & 0.87 & 0.86 -  0.88 & 6.74 & 4.90 -  8.52 \\
4086 & KOI-2583 & 2.9 & 0.021 & 0.99 & 0.97 -  1.01 & 0.93 & 0.92 -  0.94 & 8.44 & 7.37 -  9.51 \\
4087 & KOI-1161 & 1.1 & 0.017 & 1.25 & 1.22 -  1.27 & 0.87 & 0.86 -  0.88 & 13.19 & 12.61 - 13.77 \\
4088 & KOI-1168 & 0.552 & 0.015 & 2.40 & 2.35 -  2.46 & 1.47 & 1.43 -  1.50 & 2.85 & 2.75 -  3.19 \\
4089 & KOI-2040 & 1.31 & 0.019 & 1.04 & 1.02 -  1.06 & 0.94 & 0.92 -  0.95 & 8.49 & 7.77 -  9.15 \\
4090 & KOI-474 & 1.09 & 0.017 & 1.08 & 1.06 -  1.11 & 1.04 & 1.03 -  1.06 & 4.54 & 3.76 -  5.28 \\
4091 & Kepler-164 & 1.09 & 0.017 & 1.06 & 1.04 -  1.08 & 1.10 & 1.09 -  1.11 & 2.06 & 1.37 -  2.72 \\
4092 & KOI-2484 & 1.91 & 0.021 & 1.48 & 1.46 -  1.50 & 0.95 & 0.94 -  0.96 & 8.80 & 8.37 -  9.12 \\
4093 & KOI-3231 & 1.77 & 0.032 & 1.77 & 1.74 -  1.81 & 1.33 & 1.32 -  1.34 & 3.31 & 3.22 -  3.41 \\
4094 & KOI-4480 & 1.34 & 0.019 & 1.16 & 1.14 -  1.19 & 0.97 & 0.96 -  0.98 & 10.71 & 9.86 - 11.53 \\
4095 & KOI-2961 & 2.0 & 0.029 & 1.26 & 1.23 -  1.28 & 1.12 & 1.11 -  1.14 & 4.52 & 4.14 -  4.89 \\
4096 & KOI-1163 & 1.37 & 0.022 & 0.79 & 0.78 -  0.81 & 0.75 & 0.74 -  0.76 & 12.71 & 10.60 - 14.21 \\
4097 & KOI-2208 & 2.51 & 0.024 & 1.17 & 1.15 -  1.19 & 1.04 & 1.03 -  1.06 & 6.19 & 5.66 -  6.72 \\
4098 & KOI-338 & 3.29 & 0.014 & 0.82 & 0.81 -  0.84 & 0.84 & 0.83 -  0.85 & 9.17 & 6.42 - 11.69 \\
4099 & KOI-4345 & 0.0135 & 0.33 & 1.25 & 1.16 -  1.33 & 0.99 & 0.96 -  1.01 & 8.00 & 7.52 -  8.59 \\
4100 & KOI-337 & 1.25 & 0.016 & 1.22 & 1.20 -  1.24 & 1.01 & 0.99 -  1.02 & 8.54 & 7.95 -  9.14 \\
4101 & KOI-263 B &  &  &  &  &  &  &  &  \\
4102 & KOI-340 & 1.3 & 0.014 & 1.87 & 1.84 -  1.91 & 1.21 & 1.18 -  1.25 & 5.99 & 5.25 -  6.36 \\
4103 & KOI-2300 & 2.38 & 0.015 & 0.77 & 0.75 -  0.78 & 0.77 & 0.76 -  0.79 & 9.12 & 6.42 - 11.64 \\
4104 & KOI-203 & 1.36 & 0.02 & 1.05 & 1.03 -  1.07 & 1.01 & 0.99 -  1.02 & 6.36 & 5.32 -  7.36 \\
4105 & KOI-4765 & 1.23 & 0.014 & 1.39 & 1.36 -  1.42 & 1.20 & 1.19 -  1.21 & 3.93 & 3.71 -  4.11 \\
4106 & KOI-1308 & 0.986 & 0.017 & 1.50 & 1.47 -  1.54 & 1.01 & 1.00 -  1.02 & 7.92 & 7.50 -  8.36 \\
4107 & KOI-275 & 2.42 & 0.026 & 1.71 & 1.68 -  1.75 & 1.16 & 1.14 -  1.22 & 6.40 & 5.27 -  6.78 \\
4108 & KOI-4892 & 0.534 & 0.014 & 2.63 & 2.57 -  2.71 & 1.31 & 1.27 -  1.31 & 3.05 & 2.93 -  3.26 \\
4109 & KOI-3032 & 0.93 & 0.036 & 0.89 & 0.86 -  0.91 & 0.87 & 0.86 -  0.89 & 10.18 & 6.50 - 13.03 \\
4110 & KOI-4204 & 1.06 & 0.017 & 1.29 & 1.26 -  1.32 & 1.11 & 1.09 -  1.12 & 5.64 & 5.28 -  6.11 \\
4111 & KOI-339 & 0.552 & 0.31 & 1.11 & 1.05 -  1.18 & 1.03 & 1.02 -  1.04 & 4.85 & 3.69 -  5.61 \\
4112 & KOI-749 & 0.992 & 0.027 & 0.91 & 0.89 -  0.92 & 0.84 & 0.83 -  0.85 & 13.67 & 11.94 - 14.62 \\
4113 & KOI-2149 & 2.05 & 0.019 & 1.53 & 1.50 -  1.56 & 1.27 & 1.26 -  1.29 & 3.48 & 3.31 -  3.64 \\
4114 & KOI-4833 & 1.12 & 0.015 & 1.58 & 1.55 -  1.61 & 1.04 & 1.02 -  1.05 & 8.61 & 7.94 -  9.08 \\
4115 & KOI-1837 & 2.53 & 0.017 & 0.82 & 0.81 -  0.83 & 0.86 & 0.84 -  0.87 & 6.33 & 3.90 -  8.70 \\
4116 & KOI-1797 & 4.6 & 0.024 & 0.77 & 0.76 -  0.78 & 0.80 & 0.78 -  0.81 & 8.39 & 5.10 - 11.43 \\
4117 & KOI-598 & 1.5 & 0.021 & 0.84 & 0.82 -  0.86 & 0.83 & 0.81 -  0.85 & 10.44 & 7.99 - 12.85 \\
4118 & KOI-2 & 2.9 & 0.021 & 2.09 & 2.06 -  2.13 & 1.49 & 1.47 -  1.50 & 2.58 & 2.49 -  2.70 \\
4119 & KOI-4366 & 1.05 & 0.029 & 0.83 & 0.81 -  0.86 & 0.81 & 0.79 -  0.82 & 10.59 & 7.70 - 13.08 \\
4120 & KOI-211 & 0.547 & 0.02 & 1.53 & 1.48 -  1.59 & 1.10 & 1.09 -  1.12 & 6.57 & 6.12 -  6.95 \\
4121 & KOI-2046 & 1.41 & 0.013 & 1.65 & 1.62 -  1.68 & 1.06 & 1.05 -  1.08 & 8.98 & 8.56 -  9.40 \\
4122 & KOI-4312 & 1.05 & 0.018 & 1.41 & 1.37 -  1.44 & 0.99 & 0.98 -  1.00 & 7.59 & 7.24 -  8.02 \\
4123 & KOI-4335 & 1.27 & 0.018 & 1.04 & 1.02 -  1.07 & 0.91 & 0.90 -  0.92 & 8.21 & 7.54 -  8.88 \\
4124 & KOI-4024 & 2.37 & 0.015 & 0.85 & 0.84 -  0.87 & 0.81 & 0.80 -  0.82 & 12.54 & 10.99 - 13.99 \\
4125 & KOI-209 & 0.658 & 0.018 & 1.70 & 1.65 -  1.75 & 1.22 & 1.20 -  1.25 & 4.62 & 4.30 -  5.02 \\
4126 & KOI-1305 & 1.18 & 0.023 & 0.88 & 0.86 -  0.90 & 0.86 & 0.84 -  0.87 & 10.77 & 8.23 - 12.97 \\
4127 & KOI-3 & 26.5 & 0.023 & 0.79 & 0.78 -  0.80 & 0.81 & 0.79 -  0.82 & 9.44 & 5.96 - 12.24 \\
4128 & KOI-3889 & 1.38 & 0.014 & 1.27 & 1.25 -  1.29 & 1.04 & 1.03 -  1.05 & 7.85 & 7.30 -  8.40 \\
4129 & KOI-1311 & 1.57 & 0.015 & 1.11 & 1.11 -  1.12 & 1.20 & 1.19 -  1.20 & 0.30 & 0.26 -  0.38 \\
4130 & KOI-1639 & 0.635 & 0.014 & 2.52 & 2.46 -  2.59 & 1.55 & 1.50 -  1.56 & 2.53 & 2.43 -  2.76 \\
4131 & KOI-2236 & 0.779 & 0.034 & 0.92 & 0.89 -  0.95 & 0.89 & 0.87 -  0.90 & 8.28 & 6.11 - 10.07 \\
4132 & KOI-1316 & 1.83 & 0.021 & 1.95 & 1.91 -  1.98 & 1.33 & 1.30 -  1.35 & 4.36 & 4.13 -  4.64 \\
4133 & KOI-1989 & 2.05 & 0.014 & 1.00 & 0.99 -  1.02 & 0.96 & 0.95 -  0.97 & 7.00 & 6.11 -  7.91 \\
4134 & KOI-752 & 0.895 & 0.025 & 0.97 & 0.94 -  1.00 & 0.92 & 0.90 -  0.93 & 8.94 & 7.06 - 10.58 \\
4135 & KOI-3451 & 1.14 & 0.015 & 1.14 & 1.12 -  1.17 & 1.06 & 1.05 -  1.07 & 4.90 & 4.28 -  5.48 \\
4136 & KOI-3925 & 2.01 & 0.016 & 0.84 & 0.83 -  0.86 & 0.87 & 0.85 -  0.88 & 6.74 & 4.52 -  8.98 \\
4137 & KOI-3683 & 1.83 & 0.022 & 1.62 & 1.58 -  1.65 & 1.30 & 1.29 -  1.31 & 3.09 & 2.99 -  3.19 \\
4138 & KOI-4235 & 1.15 & 0.016 & 1.51 & 1.48 -  1.54 & 1.26 & 1.24 -  1.27 & 3.44 & 3.30 -  3.58 \\
4139 & KOI-2228 & 0.864 & 0.029 & 2.29 & 2.21 -  2.37 & 1.55 & 1.52 -  1.58 & 2.02 & 1.94 -  2.11 \\
4140 & KOI-117 & 1.87 & 0.02 & 1.52 & 1.49 -  1.55 & 1.16 & 1.13 -  1.21 & 5.87 & 5.05 -  6.76 \\
4141 & Kepler-107 & 1.87 & 0.02 & 1.52 & 1.49 -  1.55 & 1.17 & 1.13 -  1.21 & 5.78 & 5.04 -  6.57 \\
4142 & KOI-3602 & 1.08 & 0.021 & 1.32 & 1.29 -  1.35 & 1.07 & 1.06 -  1.08 & 5.06 & 4.83 -  5.34 \\
4143 & KOI-756 & 0.58 & 0.028 & 1.23 & 1.18 -  1.29 & 0.95 & 0.94 -  0.97 & 11.77 & 10.96 - 12.60 \\
4144 & KOI-2960 & 1.6 & 0.012 & 1.23 & 1.21 -  1.25 & 1.08 & 1.07 -  1.09 & 5.41 & 5.00 -  5.84 \\
4145 & KOI-341 & 2.39 & 0.017 & 0.91 & 0.90 -  0.93 & 0.94 & 0.93 -  0.95 & 5.30 & 3.82 -  6.76 \\
4146 & KOI-2075 & 2.44 & 0.034 & 1.24 & 1.21 -  1.26 & 1.13 & 1.12 -  1.15 & 3.66 & 3.24 -  4.06 \\
4147 & KOI-431 & 2.15 & 0.016 & 0.75 & 0.74 -  0.76 & 0.74 & 0.73 -  0.76 & 10.15 & 7.47 - 12.61 \\
4148 & KOI-1299 & 1.15 & 0.028 & 4.17 & 4.09 -  4.28 & 1.29 & 1.20 -  1.36 & 4.83 & 4.07 -  6.06 \\
4149 & KOI-1306 & 0.789 & 0.07 & 0.86 & 0.83 -  0.91 & 0.87 & 0.85 -  0.89 & 5.80 & 3.11 -  8.28 \\
4150 & KOI-3146 & 0.868 & 0.019 & 1.67 & 1.63 -  1.72 & 1.09 & 1.07 -  1.10 & 8.15 & 7.66 -  8.63 \\
4151 & KOI-291 & 1.5 & 0.044 & 1.66 & 1.61 -  1.71 & 1.12 & 1.10 -  1.13 & 7.53 & 7.10 -  8.01 \\
4152 & KOI-2623 & 0.944 & 0.014 & 1.83 & 1.79 -  1.86 & 1.35 & 1.33 -  1.36 & 3.42 & 3.31 -  3.55 \\
4153 & KOI-46 & 1.05 & 0.017 & 1.80 & 1.76 -  1.84 & 1.16 & 1.14 -  1.22 & 6.83 & 5.71 -  7.31 \\
4154 & KOI-1963 & 0.552 & 0.077 & 1.64 & 1.54 -  1.75 & 1.24 & 1.19 -  1.28 & 4.52 & 4.19 -  5.17 \\
4155 & KOI-2754 & 2.67 & 0.057 & 1.26 & 1.24 -  1.30 & 1.00 & 0.99 -  1.01 & 7.28 & 6.88 -  7.62 \\
4156 & KOI-757 & 1.18 & 0.034 & 0.76 & 0.75 -  0.78 & 0.80 & 0.78 -  0.83 & 5.87 & 2.06 - 10.25 \\
4157 & KOI-601 & 1.08 & 0.02 & 0.94 & 0.93 -  0.96 & 1.03 & 1.02 -  1.04 & 1.24 & 0.55 -  2.31 \\
4158 & KOI-1307 & 1.17 & 0.021 & 0.96 & 0.94 -  0.98 & 0.92 & 0.90 -  0.93 & 8.51 & 6.91 - 10.07 \\
4159 & KOI-4374 & 1.7 & 0.019 & 0.91 & 0.90 -  0.93 & 0.86 & 0.85 -  0.88 & 10.69 & 9.19 - 12.08 \\
4160 & KOI-1931 & 1.59 & 0.024 & 0.82 & 0.81 -  0.84 & 0.88 & 0.86 -  0.90 & 3.85 & 1.84 -  6.13 \\
4161 & KOI-343 & 1.79 & 0.013 & 1.15 & 1.13 -  1.17 & 1.00 & 0.99 -  1.01 & 7.89 & 7.30 -  8.51 \\
4162 & Kepler-142 & 1.79 & 0.013 & 1.17 & 1.15 -  1.19 & 0.97 & 0.96 -  0.98 & 8.50 & 8.14 -  8.82 \\
4163 & KOI-112 & 2.61 & 0.2 & 1.02 & 0.98 -  1.07 & 1.03 & 1.01 -  1.04 & 3.85 & 2.27 -  5.21 \\
4164 & KOI-759 & 1.32 & 0.025 & 0.80 & 0.78 -  0.81 & 0.75 & 0.74 -  0.76 & 13.50 & 11.72 - 14.60 \\
4165 & KOI-3060 & 1.25 & 0.021 & 1.75 & 1.71 -  1.79 & 1.28 & 1.24 -  1.32 & 3.81 & 3.35 -  4.24 \\
4166 & KOI-344 & 2.16 & 0.015 & 0.91 & 0.89 -  0.92 & 0.85 & 0.84 -  0.87 & 8.46 & 7.37 -  9.56 \\
4167 & KOI-479 & 1.54 & 0.017 & 0.96 & 0.95 -  0.98 & 0.87 & 0.86 -  0.88 & 10.18 & 9.24 - 11.06 \\
4168 & KOI-1645 & 2.23 & 0.018 & 1.05 & 1.03 -  1.06 & 0.81 & 0.81 -  0.81 & 14.80 & 14.52 - 14.94 \\
4169 & KOI-1800 & 3.7 & 0.025 & 0.89 & 0.88 -  0.90 & 0.93 & 0.92 -  0.95 & 4.62 & 3.13 -  6.07 \\
4170 & KOI-1444 & 0.589 & 0.019 & 2.34 & 2.27 -  2.42 & 1.46 & 1.42 -  1.49 & 3.00 & 2.79 -  3.35 \\
4171 & Kepler-299 & 0.922 & 0.023 & 1.04 & 1.01 -  1.07 & 0.95 & 0.94 -  0.96 & 8.63 & 7.49 -  9.67 \\
4172 & KOI-124 & 1.68 & 0.023 & 1.28 & 1.26 -  1.31 & 1.05 & 1.04 -  1.06 & 6.04 & 5.80 -  6.35 \\
4173 & KOI-1889 & 1.05 & 0.027 & 0.84 & 0.82 -  0.86 & 0.89 & 0.88 -  0.91 & 4.15 & 1.81 -  6.63 \\
4174 & KOI-2007 & 2.01 & 0.014 & 1.03 & 1.02 -  1.05 & 1.06 & 1.05 -  1.08 & 2.92 & 2.17 -  3.71 \\
4175 & KOI-2977 & 1.14 & 0.015 & 1.36 & 1.34 -  1.39 & 1.06 & 1.06 -  1.07 & 6.06 & 5.84 -  6.34 \\
4176 & KOI-2885 & 0.875 & 0.015 & 2.04 & 2.00 -  2.09 & 1.07 & 1.04 -  1.10 & 5.96 & 5.48 -  6.49 \\
4177 & KOI-2533 & 0.884 & 0.012 & 3.23 & 3.17 -  3.30 & 1.11 & 1.06 -  1.17 & 8.00 & 6.51 -  9.39 \\
4178 & KOI-4287 & 4.59 & 0.51 & 1.48 & 1.37 -  1.59 & 1.22 & 1.19 -  1.26 & 3.61 & 3.41 -  3.97 \\
4179 & KOI-2442 & 1.11 & 0.036 & 0.81 & 0.80 -  0.82 & 0.79 & 0.78 -  0.80 & 13.47 & 11.24 - 14.56 \\
4180 & KOI-2712 & 2.39 & 0.03 & 1.91 & 1.87 -  1.95 & 1.44 & 1.42 -  1.45 & 2.79 & 2.71 -  2.89 \\
4181 & KOI-2805 & 1.46 & 0.012 & 1.29 & 1.27 -  1.32 & 0.96 & 0.95 -  0.97 & 8.28 & 7.90 -  8.63 \\
4182 & KOI-276 & 2.98 & 0.034 & 1.22 & 1.20 -  1.25 & 1.06 & 1.05 -  1.07 & 5.76 & 5.36 -  6.13 \\
4183 & KOI-1863 & 1.35 & 0.013 & 1.14 & 1.12 -  1.16 & 0.92 & 0.91 -  0.93 & 10.91 & 10.32 - 11.85 \\
4184 & KOI-3371 & 1.73 & 0.035 & 1.09 & 1.07 -  1.12 & 0.86 & 0.85 -  0.87 & 13.32 & 12.80 - 13.84 \\
4185 & KOI-2792 & 3.59 & 0.025 & 1.42 & 1.40 -  1.45 & 1.14 & 1.11 -  1.16 & 5.67 & 5.24 -  6.54 \\
4186 & KOI-2333 & 1.2 & 0.021 & 1.29 & 1.26 -  1.32 & 1.07 & 1.06 -  1.08 & 5.28 & 4.98 -  5.55 \\
4187 & KOI-1647 & 0.926 & 0.076 & 1.41 & 1.34 -  1.49 & 1.05 & 1.03 -  1.07 & 8.94 & 8.37 -  9.53 \\
4188 & KOI-1426 & 1.42 & 0.017 & 0.91 & 0.90 -  0.93 & 0.91 & 0.90 -  0.93 & 5.32 & 4.03 -  6.47 \\
4189 & KOI-1438 & 0.697 & 0.015 & 2.19 & 2.14 -  2.24 & 1.31 & 1.27 -  1.34 & 4.28 & 4.01 -  4.80 \\
4190 & KOI-2813 & 0.911 & 0.31 & 7.66 & 7.37 -  7.86 & 0.98 & 0.96 -  0.99 & 9.23 & 8.62 - 10.06 \\
4191 & KOI-481 & 1.63 & 0.02 & 0.80 & 0.78 -  0.81 & 0.80 & 0.78 -  0.81 & 9.40 & 6.65 - 11.84 \\
4192 & KOI-2765 & 0.709 & 0.013 & 2.05 & 2.01 -  2.11 & 1.41 & 1.39 -  1.43 & 3.22 & 3.09 -  3.35 \\
4193 & KOI-4653 & 1.06 & 0.014 & 1.52 & 1.49 -  1.55 & 1.18 & 1.17 -  1.22 & 4.76 & 4.14 -  5.11 \\
4194 & KOI-294 & 2.11 & 0.022 & 1.16 & 1.14 -  1.19 & 1.12 & 1.11 -  1.13 & 3.17 & 2.64 -  3.68 \\
4195 & KOI-2796 & 0.884 & 0.019 & 1.08 & 1.05 -  1.11 & 0.97 & 0.96 -  0.98 & 7.68 & 6.90 -  8.30 \\
4196 & KOI-3103 & 2.22 & 0.39 & 1.25 & 1.17 -  1.34 & 1.12 & 1.10 -  1.15 & 4.95 & 4.34 -  5.44 \\
4197 & KOI-2672 & 4.44 & 0.036 & 0.93 & 0.92 -  0.95 & 0.96 & 0.94 -  0.97 & 5.15 & 3.88 -  6.36 \\
4198 & KOI-107 & 1.47 & 0.021 & 1.69 & 1.66 -  1.73 & 1.24 & 1.18 -  1.27 & 4.91 & 4.54 -  5.89 \\
4199 & KOI-3346 & 1.5 & 0.015 & 1.20 & 1.18 -  1.22 & 1.05 & 1.03 -  1.06 & 6.13 & 5.71 -  6.53 \\
4200 & KOI-1857 & 0.963 & 0.22 & 1.13 & 1.06 -  1.20 & 0.96 & 0.95 -  0.98 & 8.15 & 7.58 -  8.63 \\
4201 & KOI-4716 & 2.0 & 0.023 & 1.46 & 1.43 -  1.48 & 1.11 & 1.10 -  1.12 & 6.36 & 6.03 -  6.70 \\
4202 & KOI-246 & 6.91 & 0.021 & 1.28 & 1.26 -  1.30 & 1.05 & 1.04 -  1.07 & 7.21 & 6.54 -  7.73 \\
4203 & KOI-1802 & 1.81 & 0.014 & 1.03 & 1.01 -  1.04 & 1.05 & 1.03 -  1.06 & 3.17 & 2.34 -  3.96 \\
4204 & KOI-241 & 2.35 & 0.017 & 0.71 & 0.70 -  0.72 & 0.68 & 0.68 -  0.69 & 14.61 & 13.99 - 14.90 \\
4205 & Kepler-124 & 2.35 & 0.017 & 0.70 & 0.69 -  0.70 & 0.67 & 0.67 -  0.68 & 14.69 & 14.22 - 14.92 \\
4206 & KOI-2168 & 0.51 & 0.029 & 1.71 & 1.64 -  1.78 & 1.13 & 1.11 -  1.14 & 5.31 & 4.93 -  5.74 \\
4207 & KOI-2422 & 1.55 & 0.019 & 0.81 & 0.79 -  0.83 & 0.83 & 0.81 -  0.85 & 7.61 & 5.02 - 10.24 \\
4208 & KOI-2632 & 1.81 & 0.023 & 2.32 & 2.28 -  2.37 & 1.42 & 1.38 -  1.45 & 3.01 & 2.90 -  3.19 \\
4209 & Kepler-15 & 1.32 & 0.02 & 1.28 & 1.25 -  1.31 & 0.99 & 0.98 -  1.01 & 10.49 & 9.94 - 11.06 \\
4210 & KOI-128 & 1.32 & 0.02 & 1.29 & 1.26 -  1.32 & 1.00 & 0.98 -  1.01 & 10.46 & 9.80 - 11.05 \\
4211 & KOI-2366 & 1.95 & 0.03 & 1.30 & 1.27 -  1.33 & 1.16 & 1.14 -  1.17 & 3.92 & 3.53 -  4.26 \\
4212 & KOI-330 & 0.916 & 0.013 & 1.67 & 1.64 -  1.71 & 1.10 & 1.08 -  1.12 & 7.16 & 6.82 -  7.49 \\
4213 & KOI-3782 & 2.62 & 0.025 & 0.91 & 0.90 -  0.92 & 0.83 & 0.83 -  0.84 & 14.91 & 14.77 - 14.98 \\
4214 & KOI-2639 & 0.366 & 0.027 & 1.60 & 1.52 -  1.69 & 1.06 & 1.03 -  1.09 & 8.38 & 7.68 -  9.04 \\
4215 & KOI-3015 & 1.29 & 0.015 & 1.58 & 1.55 -  1.61 & 1.06 & 1.04 -  1.06 & 6.83 & 6.47 -  7.35 \\
4216 & KOI-1428 & 2.29 & 0.018 & 0.71 & 0.70 -  0.72 & 0.71 & 0.70 -  0.72 & 12.71 & 9.81 - 14.37 \\
4217 & KOI-4036 & 2.96 & 0.015 & 0.74 & 0.73 -  0.75 & 0.75 & 0.74 -  0.77 & 9.92 & 6.27 - 13.04 \\
4218 & KOI-1436 & 1.36 & 0.02 & 0.99 & 0.97 -  1.01 & 0.97 & 0.95 -  0.98 & 6.62 & 5.41 -  7.76 \\
4219 & Kepler-301 & 1.36 & 0.02 & 0.98 & 0.96 -  1.00 & 0.97 & 0.96 -  0.98 & 6.07 & 4.87 -  7.16 \\
4220 & KOI-2143 & 1.73 & 0.018 & 0.91 & 0.89 -  0.93 & 0.90 & 0.88 -  0.91 & 8.50 & 6.71 - 10.11 \\
4221 & KOI-2195 & 0.64 & 0.022 & 1.40 & 1.36 -  1.47 & 1.08 & 1.07 -  1.11 & 5.48 & 5.16 -  5.82 \\
4222 & KOI-349 &  &  & 1.22 & 1.15 -  1.30 & 1.05 & 1.04 -  1.08 & 7.07 & 6.26 -  7.99 \\
4223 & KOI-350 & 1.87 & 0.014 & 1.02 & 1.00 -  1.03 & 1.01 & 1.00 -  1.03 & 4.52 & 3.64 -  5.36 \\
4224 & KOI-1623 & 2.22 & 0.031 & 1.66 & 1.62 -  1.69 & 1.06 & 1.04 -  1.08 & 8.07 & 7.57 -  8.51 \\
4225 & KOI-351 & 1.15 & 0.015 & 1.25 & 1.23 -  1.28 & 1.13 & 1.12 -  1.14 & 4.33 & 3.98 -  4.68 \\
4226 & KOI-1992 & 0.741 & 0.017 & 1.51 & 1.47 -  1.55 & 1.10 & 1.07 -  1.10 & 5.75 & 5.38 -  6.18 \\
4227 & KOI-2047 & 1.04 & 0.013 & 1.26 & 1.23 -  1.28 & 1.10 & 1.09 -  1.11 & 4.53 & 4.21 -  4.85 \\
4228 & KOI-2771 & 3.2 & 0.024 & 1.12 & 1.10 -  1.14 & 1.16 & 1.15 -  1.18 & 1.20 & 0.72 -  1.71 \\
4229 & KOI-2110 & 1.86 & 0.044 & 1.57 & 1.53 -  1.62 & 1.27 & 1.26 -  1.29 & 3.62 & 3.48 -  3.76 \\
4230 & KOI-5900 & 1.23 & 0.017 & 1.47 & 1.44 -  1.51 & 1.20 & 1.18 -  1.21 & 3.76 & 3.62 -  3.90 \\
4231 & KOI-2399 & 2.38 & 0.018 & 0.77 & 0.76 -  0.78 & 0.74 & 0.73 -  0.75 & 14.02 & 12.67 - 14.74 \\
4232 & KOI-352 & 1.21 & 0.017 & 1.36 & 1.33 -  1.39 & 1.05 & 1.04 -  1.06 & 6.82 & 6.44 -  7.32 \\
4233 & KOI-2109 & 0.722 & 0.013 & 1.77 & 1.73 -  1.81 & 1.23 & 1.20 -  1.25 & 4.60 & 4.35 -  5.09 \\
4234 & KOI-3419 & 0.997 & 0.015 & 1.92 & 1.89 -  1.96 & 1.28 & 1.26 -  1.32 & 3.03 & 2.77 -  3.20 \\
4235 & KOI-168 & 1.17 & 0.016 & 1.59 & 1.56 -  1.62 & 1.10 & 1.08 -  1.10 & 5.77 & 5.45 -  6.16 \\
4236 & KOI-1856 & 2.15 & 0.015 & 0.81 & 0.80 -  0.82 & 0.83 & 0.82 -  0.85 & 7.12 & 4.51 -  9.43 \\
4237 & KOI-1655 & 1.84 & 0.013 & 0.94 & 0.92 -  0.96 & 0.86 & 0.85 -  0.88 & 9.57 & 8.53 - 10.56 \\
4238 & KOI-354 & 1.72 & 0.035 & 1.16 & 1.13 -  1.19 & 1.07 & 1.06 -  1.08 & 4.88 & 4.28 -  5.43 \\
4239 & KOI-2365 & 1.06 & 0.019 & 1.44 & 1.41 -  1.48 & 1.17 & 1.13 -  1.19 & 5.13 & 4.75 -  5.92 \\
4240 & KOI-2837 &  &  & 1.70 & 1.59 -  1.82 & 1.36 & 1.33 -  1.40 & 2.48 & 2.37 -  2.56 \\
4241 & KOI-3109 & 0.625 & 0.016 & 2.65 & 2.59 -  2.72 & 1.59 & 1.54 -  1.61 & 2.28 & 2.16 -  2.59 \\
4242 & KOI-295 & 2.96 & 0.021 & 0.99 & 0.98 -  1.01 & 1.00 & 0.98 -  1.01 & 3.69 & 2.89 -  4.44 \\
4243 & KOI-4792 & 1.2 & 0.015 & 1.03 & 1.01 -  1.06 & 1.08 & 1.06 -  1.09 & 2.23 & 1.35 -  3.14 \\
4244 & KOI-356 & 2.14 & 0.07 & 0.94 & 0.91 -  0.96 & 0.86 & 0.85 -  0.87 & 11.64 & 10.06 - 12.76 \\
4245 & KOI-1831 & 1.96 & 0.014 & 0.88 & 0.86 -  0.89 & 0.83 & 0.82 -  0.84 & 13.17 & 11.36 - 14.41 \\
4246 & KOI-4304 & 0.946 & 0.017 & 1.43 & 1.40 -  1.47 & 1.12 & 1.10 -  1.15 & 6.22 & 5.50 -  6.69 \\
4247 & KOI-355 & 1.43 & 0.013 & 1.35 & 1.33 -  1.38 & 1.19 & 1.17 -  1.20 & 3.99 & 3.73 -  4.23 \\
4248 & KOI-3363 & 1.34 & 0.017 & 1.19 & 1.16 -  1.22 & 1.00 & 0.99 -  1.01 & 7.39 & 6.99 -  7.69 \\
4249 & KOI-167 & 1.15 & 0.016 & 1.51 & 1.48 -  1.54 & 1.25 & 1.24 -  1.26 & 3.58 & 3.44 -  3.72 \\
4250 & KOI-1945 & 1.41 & 0.025 & 0.95 & 0.93 -  0.97 & 0.86 & 0.85 -  0.87 & 14.00 & 12.80 - 14.72 \\
4251 & KOI-1894 & 0.839 & 0.027 & 3.67 & 3.58 -  3.78 & 1.20 & 1.16 -  1.23 & 6.31 & 5.81 -  7.18 \\
4252 & KOI-1832 & 1.19 & 0.021 & 0.83 & 0.82 -  0.85 & 0.90 & 0.89 -  0.92 & 2.58 & 1.06 -  4.51 \\
4253 & KOI-1841 & 3.02 & 0.043 & 0.86 & 0.85 -  0.87 & 0.81 & 0.80 -  0.82 & 14.31 & 13.31 - 14.82 \\
4254 & KOI-2582 & 1.18 & 0.018 & 1.39 & 1.36 -  1.42 & 1.17 & 1.16 -  1.19 & 4.82 & 4.57 -  5.13 \\
4255 & KOI-620 & 1.25 & 0.022 & 0.87 & 0.85 -  0.88 & 0.94 & 0.92 -  0.95 & 2.52 & 1.04 -  4.18 \\
4256 & KOI-3403 & 1.08 & 0.014 & 2.03 & 1.99 -  2.07 & 1.27 & 1.22 -  1.29 & 4.53 & 4.20 -  5.31 \\
4257 & KOI-1883 & 2.11 & 0.026 & 1.62 & 1.58 -  1.65 & 1.20 & 1.18 -  1.22 & 4.84 & 4.63 -  5.21 \\
4258 & KOI-3892 & 2.58 & 0.021 & 1.08 & 1.06 -  1.10 & 0.96 & 0.95 -  0.97 & 9.83 & 8.90 - 10.73 \\
4259 & KOI-1980 & 2.01 & 0.016 & 0.90 & 0.88 -  0.91 & 0.93 & 0.91 -  0.94 & 5.53 & 3.84 -  7.14 \\
4260 & KOI-2173 & 5.29 & 0.024 & 0.74 & 0.73 -  0.74 & 0.78 & 0.76 -  0.79 & 6.25 & 2.97 -  9.74 \\
4261 & KOI-2492 & 1.36 & 0.017 & 1.09 & 1.07 -  1.11 & 0.87 & 0.86 -  0.88 & 10.33 & 9.69 - 11.00 \\
4262 & KOI-2260 & 2.06 & 0.02 & 1.40 & 1.38 -  1.43 & 1.15 & 1.14 -  1.17 & 4.76 & 4.24 -  5.08 \\
4263 & KOI-296 & 2.11 & 0.02 & 1.10 & 1.09 -  1.12 & 0.94 & 0.93 -  0.95 & 8.07 & 7.55 -  8.57 \\
4264 & KOI-2581 & 2.25 & 0.013 & 0.93 & 0.92 -  0.95 & 0.92 & 0.91 -  0.93 & 8.09 & 6.62 -  9.49 \\
4265 & KOI-543 & 1.61 & 0.021 & 0.81 & 0.80 -  0.83 & 0.77 & 0.77 -  0.79 & 13.20 & 11.16 - 14.43 \\
4266 & KOI-4062 & 0.884 & 0.017 & 1.45 & 1.41 -  1.49 & 1.13 & 1.11 -  1.14 & 5.78 & 5.41 -  6.14 \\
4267 & KOI-3875 & 1.06 & 0.013 & 1.64 & 1.61 -  1.66 & 1.02 & 0.99 -  1.02 & 5.94 & 5.73 -  6.51 \\
4268 & KOI-72 & 5.36 & 0.023 & 1.10 & 1.09 -  1.12 & 0.89 & 0.88 -  0.90 & 10.85 & 10.36 - 11.35 \\
4269 & KOI-297 & 2.17 & 0.024 & 1.39 & 1.37 -  1.42 & 1.19 & 1.18 -  1.20 & 4.06 & 3.87 -  4.26 \\
4270 & KOI-2026 & 1.81 & 0.015 & 1.02 & 1.00 -  1.04 & 1.08 & 1.06 -  1.09 & 1.62 & 0.93 -  2.36 \\
4271 & KOI-2433 & 0.669 & 0.022 & 1.21 & 1.16 -  1.26 & 1.03 & 1.02 -  1.05 & 6.90 & 6.27 -  7.56 \\
4272 & KOI-4011 & 2.01 & 0.023 & 1.34 & 1.32 -  1.37 & 1.13 & 1.12 -  1.14 & 5.35 & 5.00 -  5.80 \\
4273 & KOI-4129 & 3.0 & 0.021 & 0.81 & 0.80 -  0.83 & 0.83 & 0.81 -  0.84 & 9.16 & 6.36 - 11.69 \\
4274 & KOI-4021 & 0.797 & 0.42 & 1.36 & 1.27 -  1.45 & 1.24 & 1.22 -  1.26 & 2.65 & 2.05 -  2.94 \\
4275 & KOI-2590 & 1.65 & 0.027 & 2.30 & 2.25 -  2.34 & 1.39 & 1.38 -  1.43 & 3.46 & 3.13 -  3.56 \\
4276 & KOI-2729 & 1.45 & 0.012 & 0.85 & 0.83 -  0.88 & 0.91 & 0.90 -  0.92 & 2.22 & 0.85 -  4.20 \\
4277 & KOI-3194 & 2.12 & 0.022 & 1.79 & 1.75 -  1.82 & 1.39 & 1.38 -  1.41 & 2.86 & 2.74 -  2.98 \\
4278 & Kepler-197 & 3.0 & 0.021 & 1.17 & 1.15 -  1.19 & 0.93 & 0.92 -  0.94 & 8.11 & 7.76 -  8.50 \\
4279 & KOI-623 & 3.0 & 0.021 & 1.17 & 1.15 -  1.19 & 0.94 & 0.93 -  0.95 & 7.84 & 7.40 -  8.25 \\
4280 & KOI-3017 & 2.31 & 0.013 & 0.91 & 0.90 -  0.93 & 0.85 & 0.84 -  0.86 & 9.42 & 8.38 - 10.47 \\
4281 & KOI-546 & 0.617 & 0.021 & 1.43 & 1.38 -  1.48 & 1.11 & 1.09 -  1.14 & 6.29 & 5.56 -  6.84 \\
4282 & KOI-2072 & 1.32 & 0.014 & 1.40 & 1.37 -  1.42 & 1.04 & 1.02 -  1.04 & 6.58 & 6.30 -  7.01 \\
4283 & KOI-2407 & 0.86 & 0.03 & 1.57 & 1.52 -  1.63 & 1.16 & 1.13 -  1.20 & 5.84 & 5.00 -  6.48 \\
4284 & KOI-2396 & 1.59 & 0.022 & 0.84 & 0.82 -  0.85 & 0.84 & 0.82 -  0.85 & 9.42 & 6.68 - 11.97 \\
4285 & KOI-4457 & 1.14 & 0.05 & 1.36 & 1.31 -  1.41 & 1.08 & 1.07 -  1.10 & 5.39 & 5.08 -  5.63 \\
4286 & KOI-360 & 1.81 & 0.019 & 1.21 & 1.18 -  1.23 & 1.03 & 1.02 -  1.04 & 5.95 & 5.58 -  6.35 \\
4287 & KOI-141 & 1.84 & 0.19 & 0.97 & 0.94 -  1.00 & 0.88 & 0.87 -  0.89 & 13.79 & 12.03 - 14.66 \\
4288 & KOI-2597 & 0.916 & 0.021 & 1.01 & 0.99 -  1.04 & 0.94 & 0.92 -  0.95 & 6.27 & 5.31 -  7.16 \\
4289 & KOI-2004 & 1.19 & 0.015 & 1.68 & 1.65 -  1.71 & 1.09 & 1.08 -  1.11 & 8.10 & 7.69 -  8.48 \\
4290 & KOI-2714 & 1.01 & 0.018 & 1.82 & 1.78 -  1.86 & 1.16 & 1.14 -  1.18 & 5.55 & 5.22 -  5.83 \\
4291 & Kepler-401 & 1.01 & 0.018 & 1.81 & 1.77 -  1.85 & 1.18 & 1.16 -  1.19 & 5.32 & 5.10 -  5.54 \\
4292 & KOI-1947 & 2.3 & 0.024 & 1.34 & 1.32 -  1.37 & 1.09 & 1.07 -  1.12 & 6.74 & 5.95 -  7.19 \\
4293 & KOI-2372 & 1.21 & 0.013 & 1.53 & 1.50 -  1.56 & 1.10 & 1.10 -  1.11 & 5.61 & 5.33 -  5.83 \\
4294 & KOI-3310 & 2.22 & 0.017 & 0.93 & 0.91 -  0.94 & 0.89 & 0.88 -  0.91 & 9.64 & 8.05 - 11.16 \\
4295 & KOI-3167 & 9.43 & 0.024 & 0.89 & 0.87 -  0.90 & 0.90 & 0.89 -  0.91 & 6.29 & 4.86 -  7.67 \\
4296 & KOI-279 & 2.16 & 0.025 & 1.72 & 1.69 -  1.75 & 1.32 & 1.30 -  1.33 & 3.57 & 3.43 -  3.71 \\
4297 & WASP-92 & 1.71 & 0.019 & 1.31 & 1.29 -  1.34 & 1.13 & 1.12 -  1.14 & 4.69 & 4.39 -  4.98 \\
4298 & KOI-2541 & 1.12 & 0.017 & 2.88 & 2.83 -  2.94 & 1.11 & 1.05 -  1.17 & 8.17 & 6.71 - 10.00 \\
4299 & KOI-2059 &  &  & 0.77 & 0.76 -  0.78 & 0.76 & 0.75 -  0.77 & 13.44 & 10.95 - 14.60 \\
4300 & KOI-375 & 1.17 & 0.013 & 1.75 & 1.71 -  1.79 & 1.14 & 1.13 -  1.18 & 6.69 & 5.86 -  7.03 \\
4301 & KOI-1474 & 0.96 & 0.024 & 1.91 & 1.86 -  1.96 & 1.46 & 1.44 -  1.48 & 2.49 & 2.37 -  2.59 \\
4302 & KOI-3122 & 1.26 & 0.024 & 2.43 & 2.38 -  2.47 & 1.55 & 1.54 -  1.57 & 2.58 & 2.46 -  2.71 \\
4303 & KOI-3009 & 1.41 & 0.02 & 0.81 & 0.79 -  0.82 & 0.83 & 0.81 -  0.85 & 8.05 & 4.51 - 11.34 \\
4304 & KOI-4829 & 0.943 & 0.019 & 1.32 & 1.29 -  1.36 & 1.08 & 1.07 -  1.09 & 5.51 & 5.28 -  5.79 \\
4305 & KOI-2331 & 1.22 & 0.016 & 1.46 & 1.43 -  1.49 & 1.06 & 1.05 -  1.07 & 7.96 & 7.61 -  8.36 \\
4306 & KOI-361 & 2.25 & 0.012 & 1.00 & 0.98 -  1.01 & 0.96 & 0.95 -  0.97 & 6.73 & 5.73 -  7.75 \\
4307 & KOI-2463 &  &  & 1.21 & 1.15 -  1.29 & 1.17 & 1.16 -  1.19 & 2.82 & 1.81 -  3.50 \\
4308 & KOI-439 & 1.42 & 0.018 & 1.03 & 1.01 -  1.05 & 0.91 & 0.90 -  0.92 & 12.65 & 11.44 - 13.79 \\
4309 & KOI-4329 & 1.52 & 0.019 & 2.00 & 1.97 -  2.04 & 1.40 & 1.39 -  1.42 & 3.19 & 3.10 -  3.29 \\
4310 & KOI-4605 & 0.765 & 0.014 & 2.29 & 2.23 -  2.34 & 1.35 & 1.33 -  1.39 & 3.75 & 3.45 -  3.83 \\
4311 & KOI-4190 & 0.589 & 0.29 & 1.77 & 1.64 -  1.91 & 1.11 & 1.06 -  1.16 & 7.84 & 6.60 -  9.16 \\
4312 & KOI-548 & 0.948 & 0.022 & 1.37 & 1.33 -  1.40 & 1.09 & 1.06 -  1.10 & 5.53 & 5.31 -  5.92 \\
4313 & KOI-3663 & 2.88 & 0.03 & 0.96 & 0.94 -  0.97 & 0.96 & 0.94 -  0.97 & 5.14 & 3.99 -  6.18 \\
4314 & KOI-4245 & 0.742 & 0.018 & 2.22 & 2.17 -  2.28 & 1.45 & 1.43 -  1.48 & 3.25 & 3.04 -  3.35 \\
4315 & BD+52_277A & 3.6 & 0.041 & 1.78 & 1.74 -  1.81 & 1.50 & 1.49 -  1.51 & 1.61 & 1.54 -  1.67 \\
4316 & HD 239643 & 11.9 & 0.029 & 1.29 & 1.27 -  1.31 & 1.13 & 1.12 -  1.14 & 4.39 & 4.10 -  4.66 \\
4317 & HD 203802 & 11.9 & 0.038 & 1.77 & 1.75 -  1.80 & 1.32 & 1.31 -  1.34 & 3.51 & 3.41 -  3.67 \\
4318 & HD 240051 & 15.8 & 0.033 & 1.06 & 1.05 -  1.08 & 1.10 & 1.09 -  1.12 & 2.07 & 1.47 -  2.71 \\
4319 & HD 215714 & 15.9 & 0.033 & 1.39 & 1.37 -  1.42 & 1.29 & 1.28 -  1.30 & 2.05 & 1.85 -  2.25 \\
\enddata
\end{deluxetable*}


==> table_06.tex <==
\begin{deluxetable*}{llrrrrrrrrrrrrrrrrrrr}
\tablecaption{Uncertainties for spectroscopically determined stellar properties and abundances.
\label{table:uncertainties}
}
\tablehead{\colhead{ID} & \colhead{Name} & \colhead{$T_{\mathrm{{eff}}}$} & \colhead{$ \log g$} & \colhead{{{[M/H]}}} & \colhead{$v\sin{i}$} & \colhead{{[C/H]}} & \colhead{{[N/H]}} & \colhead{{[O/H]}} & \colhead{{[Na/H]}} & \colhead{{[Mg/H]}} & \colhead{{[Al/H]}} & \colhead{{[Si/H]}} & \colhead{{[Ca/H]}} & \colhead{{[Ti/H]}} & \colhead{{[V/H]}} & \colhead{{[Cr/H]}} & \colhead{{[Mn/H]}} & \colhead{{[Fe/H]}} & \colhead{{[Ni/H]}} & \colhead{{[Y/H]}} \\
\colhead{(1)} & \colhead{(2)} & \colhead{(3)} & \colhead{(4)} & \colhead{(5)} & \colhead{(6)} & \colhead{(7)} & \colhead{(8)} & \colhead{(9)} & \colhead{(10)} & \colhead{(11)} & \colhead{(12)} & \colhead{(13)} & \colhead{(14)} & \colhead{(15)} & \colhead{(16)} & \colhead{(17)} & \colhead{(18)} & \colhead{(19)} & \colhead{(20)} & \colhead{(21)}}
\startdata
2281 & KOI-3248 & 27 & 0.05 & 0.01 & 0.5 & 0.03 & 0.08 & 0.06 & 0.03 & 0.02 & 0.04 & 0.02 & 0.02 & 0.02 & 0.04 & 0.02 & 0.03 & 0.02 & 0.02 & 0.04 \\
2361 & KOI-4273 & 28 & 0.05 & 0.01 & 0.5 & 0.04 & 0.08 & 0.06 & 0.03 & 0.02 & 0.04 & 0.02 & 0.03 & 0.02 & 0.04 & 0.02 & 0.03 & 0.02 & 0.02 & 0.04 \\
2393 & KOI-3605 & 27 & 0.05 & 0.01 & 0.5 & 0.03 & 0.07 & 0.06 & 0.03 & 0.02 & 0.04 & 0.02 & 0.02 & 0.02 & 0.04 & 0.02 & 0.03 & 0.02 & 0.02 & 0.04 \\
2405 & KOI-3197 & 27 & 0.05 & 0.01 & 0.5 & 0.03 & 0.08 & 0.06 & 0.03 & 0.02 & 0.04 & 0.02 & 0.03 & 0.02 & 0.04 & 0.02 & 0.03 & 0.02 & 0.02 & 0.04 \\
2430 & KOI-1353 & 28 & 0.05 & 0.01 & 0.5 & 0.03 & 0.08 & 0.06 & 0.03 & 0.02 & 0.04 & 0.02 & 0.03 & 0.02 & 0.04 & 0.02 & 0.03 & 0.02 & 0.02 & 0.04 \\
2435 & KOI-4323 & 28 & 0.06 & 0.02 & 0.5 & 0.04 & 0.09 & 0.07 & 0.03 & 0.02 & 0.05 & 0.02 & 0.03 & 0.02 & 0.05 & 0.02 & 0.03 & 0.02 & 0.02 & 0.04 \\
2445 & KOI-3384 & 27 & 0.05 & 0.01 & 0.5 & 0.03 & 0.08 & 0.06 & 0.03 & 0.02 & 0.04 & 0.02 & 0.02 & 0.02 & 0.04 & 0.02 & 0.03 & 0.02 & 0.02 & 0.04 \\
2460 & KOI-4409 & 27 & 0.05 & 0.01 & 0.5 & 0.03 & 0.07 & 0.06 & 0.03 & 0.02 & 0.04 & 0.02 & 0.02 & 0.02 & 0.04 & 0.02 & 0.03 & 0.02 & 0.02 & 0.04 \\
2464 & KOI-4226 & 28 & 0.06 & 0.02 & 0.5 & 0.04 & 0.09 & 0.06 & 0.03 & 0.02 & 0.05 & 0.02 & 0.03 & 0.02 & 0.05 & 0.02 & 0.03 & 0.02 & 0.02 & 0.04 \\
2485 & K2-58 & 25 & 0.05 & 0.01 & 0.5 & 0.03 & 0.05 & 0.04 & 0.02 & 0.01 & 0.03 & 0.01 & 0.02 & 0.01 & 0.04 & 0.02 & 0.02 & 0.01 & 0.01 & 0.03 \\
2914 & XO-1 & 25 & 0.05 & 0.01 & 0.5 & 0.03 & 0.04 & 0.04 & 0.01 & 0.01 & 0.03 & 0.01 & 0.01 & 0.01 & 0.03 & 0.01 & 0.02 & 0.01 & 0.01 & 0.03 \\
2962 & TRES-4 & 26 & 0.05 & 0.01 & 0.5 & 0.03 & 0.06 & 0.05 & 0.02 & 0.02 & 0.03 & 0.01 & 0.02 & 0.02 & 0.04 & 0.02 & 0.02 & 0.01 & 0.02 & 0.04 \\
2980 & KOI-104 & 27 & 0.05 & 0.01 & 0.5 & 0.03 & 0.07 & 0.05 & 0.03 & 0.02 & 0.04 & 0.02 & 0.02 & 0.02 & 0.04 & 0.02 & 0.03 & 0.01 & 0.02 & 0.04 \\
2981 & KOI-263 & 28 & 0.06 & 0.02 & 0.5 & 0.04 & 0.09 & 0.07 & 0.03 & 0.02 & 0.05 & 0.02 & 0.03 & 0.02 & 0.05 & 0.02 & 0.03 & 0.02 & 0.02 & 0.04 \\
2982 & KOI-10 & 27 & 0.05 & 0.01 & 0.5 & 0.03 & 0.08 & 0.06 & 0.03 & 0.02 & 0.04 & 0.02 & 0.02 & 0.02 & 0.04 & 0.02 & 0.03 & 0.02 & 0.02 & 0.04 \\
2983 & KOI-82 & 27 & 0.05 & 0.01 & 0.5 & 0.03 & 0.07 & 0.06 & 0.03 & 0.02 & 0.04 & 0.02 & 0.02 & 0.02 & 0.04 & 0.02 & 0.03 & 0.01 & 0.02 & 0.04 \\
2986 & KOI-274 & 27 & 0.05 & 0.01 & 0.5 & 0.03 & 0.08 & 0.06 & 0.03 & 0.02 & 0.04 & 0.02 & 0.03 & 0.02 & 0.04 & 0.02 & 0.03 & 0.02 & 0.02 & 0.04 \\
2987 & KOI-22 & 27 & 0.05 & 0.01 & 0.5 & 0.03 & 0.08 & 0.06 & 0.03 & 0.02 & 0.04 & 0.02 & 0.02 & 0.02 & 0.04 & 0.02 & 0.03 & 0.02 & 0.02 & 0.04 \\
2988 & KOI-42 & 27 & 0.05 & 0.01 & 0.5 & 0.03 & 0.08 & 0.06 & 0.03 & 0.02 & 0.04 & 0.02 & 0.02 & 0.02 & 0.04 & 0.02 & 0.03 & 0.02 & 0.02 & 0.04 \\
2989 & KOI-701 & 27 & 0.05 & 0.01 & 0.5 & 0.03 & 0.07 & 0.06 & 0.03 & 0.02 & 0.04 & 0.02 & 0.02 & 0.02 & 0.04 & 0.02 & 0.03 & 0.02 & 0.02 & 0.04 \\
2997 & KOI-245 & 27 & 0.05 & 0.01 & 0.5 & 0.03 & 0.08 & 0.06 & 0.03 & 0.02 & 0.04 & 0.02 & 0.02 & 0.02 & 0.04 & 0.02 & 0.03 & 0.02 & 0.02 & 0.04 \\
2998 & KOI-180 & 27 & 0.05 & 0.01 & 0.5 & 0.03 & 0.08 & 0.06 & 0.03 & 0.02 & 0.04 & 0.02 & 0.02 & 0.02 & 0.04 & 0.02 & 0.03 & 0.02 & 0.02 & 0.04 \\
2999 & KOI-367 & 25 & 0.05 & 0.01 & 0.5 & 0.03 & 0.06 & 0.04 & 0.02 & 0.02 & 0.03 & 0.01 & 0.02 & 0.02 & 0.04 & 0.02 & 0.02 & 0.01 & 0.01 & 0.03 \\
3000 & KOI-122 & 27 & 0.05 & 0.01 & 0.5 & 0.03 & 0.08 & 0.06 & 0.03 & 0.02 & 0.04 & 0.02 & 0.03 & 0.02 & 0.04 & 0.02 & 0.03 & 0.02 & 0.02 & 0.04 \\
3001 & KOI-1612 & 27 & 0.05 & 0.01 & 0.5 & 0.03 & 0.08 & 0.06 & 0.03 & 0.02 & 0.04 & 0.02 & 0.02 & 0.02 & 0.04 & 0.02 & 0.03 & 0.02 & 0.02 & 0.04 \\
3003 & KOI-2169 & 27 & 0.05 & 0.01 & 0.5 & 0.03 & 0.07 & 0.06 & 0.03 & 0.02 & 0.04 & 0.02 & 0.02 & 0.02 & 0.04 & 0.02 & 0.03 & 0.02 & 0.02 & 0.04 \\
3006 & KOI-7 & 28 & 0.05 & 0.01 & 0.5 & 0.04 & 0.08 & 0.06 & 0.03 & 0.02 & 0.04 & 0.02 & 0.03 & 0.02 & 0.04 & 0.02 & 0.03 & 0.02 & 0.02 & 0.04 \\
3007 & KOI-299 & 27 & 0.05 & 0.01 & 0.5 & 0.03 & 0.07 & 0.06 & 0.03 & 0.02 & 0.04 & 0.02 & 0.02 & 0.02 & 0.04 & 0.02 & 0.03 & 0.02 & 0.02 & 0.04 \\
3011 & KOI-1442 & 28 & 0.05 & 0.01 & 0.5 & 0.04 & 0.08 & 0.06 & 0.03 & 0.02 & 0.04 & 0.02 & 0.03 & 0.02 & 0.04 & 0.02 & 0.03 & 0.02 & 0.02 & 0.04 \\
3017 & KOI-244 & 28 & 0.05 & 0.01 & 0.5 & 0.03 & 0.08 & 0.06 & 0.03 & 0.02 & 0.04 & 0.02 & 0.03 & 0.02 & 0.04 & 0.02 & 0.03 & 0.02 & 0.02 & 0.04 \\
3018 & KOI-1 & 27 & 0.05 & 0.01 & 0.5 & 0.03 & 0.08 & 0.06 & 0.03 & 0.02 & 0.04 & 0.02 & 0.03 & 0.02 & 0.04 & 0.02 & 0.03 & 0.02 & 0.02 & 0.04 \\
3020 & KOI-1431 & 27 & 0.05 & 0.01 & 0.5 & 0.03 & 0.07 & 0.06 & 0.03 & 0.02 & 0.04 & 0.02 & 0.02 & 0.02 & 0.04 & 0.02 & 0.03 & 0.02 & 0.02 & 0.04 \\
3022 & KOI-292 & 27 & 0.05 & 0.01 & 0.5 & 0.03 & 0.08 & 0.06 & 0.03 & 0.02 & 0.04 & 0.02 & 0.02 & 0.02 & 0.04 & 0.02 & 0.03 & 0.02 & 0.02 & 0.04 \\
3024 & Kepler-174 & 26 & 0.05 & 0.01 & 0.5 & 0.03 & 0.07 & 0.05 & 0.03 & 0.02 & 0.04 & 0.02 & 0.02 & 0.02 & 0.04 & 0.02 & 0.03 & 0.01 & 0.02 & 0.04 \\
3025 & KOI-273 & 27 & 0.05 & 0.01 & 0.5 & 0.03 & 0.08 & 0.06 & 0.03 & 0.02 & 0.04 & 0.02 & 0.02 & 0.02 & 0.04 & 0.02 & 0.03 & 0.02 & 0.02 & 0.04 \\
3026 & KOI-111 & 29 & 0.06 & 0.02 & 0.6 & 0.04 & 0.09 & 0.07 & 0.04 & 0.02 & 0.05 & 0.02 & 0.03 & 0.02 & 0.05 & 0.02 & 0.03 & 0.02 & 0.02 & 0.05 \\
3027 & KOI-1781 & 27 & 0.05 & 0.01 & 0.5 & 0.03 & 0.07 & 0.05 & 0.03 & 0.02 & 0.04 & 0.02 & 0.02 & 0.02 & 0.04 & 0.02 & 0.03 & 0.01 & 0.02 & 0.04 \\
3031 & KOI-70 & 28 & 0.05 & 0.01 & 0.5 & 0.04 & 0.08 & 0.06 & 0.03 & 0.02 & 0.04 & 0.02 & 0.03 & 0.02 & 0.04 & 0.02 & 0.03 & 0.02 & 0.02 & 0.04 \\
3032 & KOI-98 & 28 & 0.05 & 0.01 & 0.5 & 0.04 & 0.08 & 0.06 & 0.03 & 0.02 & 0.05 & 0.02 & 0.03 & 0.02 & 0.04 & 0.02 & 0.03 & 0.02 & 0.02 & 0.04 \\
3034 & KOI-153 & 27 & 0.05 & 0.01 & 0.5 & 0.03 & 0.07 & 0.05 & 0.03 & 0.02 & 0.04 & 0.02 & 0.02 & 0.02 & 0.04 & 0.02 & 0.03 & 0.01 & 0.02 & 0.04 \\
3036 & KOI-262 & 27 & 0.05 & 0.01 & 0.5 & 0.03 & 0.08 & 0.06 & 0.03 & 0.02 & 0.04 & 0.02 & 0.02 & 0.02 & 0.04 & 0.02 & 0.03 & 0.02 & 0.02 & 0.04 \\
3040 & KOI-283 & 27 & 0.05 & 0.01 & 0.5 & 0.03 & 0.08 & 0.06 & 0.03 & 0.02 & 0.04 & 0.02 & 0.02 & 0.02 & 0.04 & 0.02 & 0.03 & 0.02 & 0.02 & 0.04 \\
3041 & KOI-97 & 27 & 0.05 & 0.01 & 0.5 & 0.03 & 0.08 & 0.06 & 0.03 & 0.02 & 0.04 & 0.02 & 0.02 & 0.02 & 0.04 & 0.02 & 0.03 & 0.02 & 0.02 & 0.04 \\
3042 & KOI-85 & 27 & 0.05 & 0.01 & 0.5 & 0.03 & 0.08 & 0.06 & 0.03 & 0.02 & 0.04 & 0.02 & 0.02 & 0.02 & 0.04 & 0.02 & 0.03 & 0.02 & 0.02 & 0.04 \\
3043 & KOI-108 & 28 & 0.05 & 0.01 & 0.5 & 0.03 & 0.08 & 0.06 & 0.03 & 0.02 & 0.04 & 0.02 & 0.03 & 0.02 & 0.04 & 0.02 & 0.03 & 0.02 & 0.02 & 0.04 \\
3045 & KOI-87 & 27 & 0.05 & 0.01 & 0.5 & 0.03 & 0.08 & 0.06 & 0.03 & 0.02 & 0.04 & 0.02 & 0.03 & 0.02 & 0.04 & 0.02 & 0.03 & 0.02 & 0.02 & 0.04 \\
3046 & KOI-63 & 26 & 0.05 & 0.01 & 0.5 & 0.03 & 0.06 & 0.05 & 0.02 & 0.02 & 0.04 & 0.01 & 0.02 & 0.02 & 0.04 & 0.02 & 0.02 & 0.01 & 0.02 & 0.04 \\
3048 & KOI-260 & 27 & 0.05 & 0.01 & 0.5 & 0.03 & 0.08 & 0.06 & 0.03 & 0.02 & 0.04 & 0.02 & 0.03 & 0.02 & 0.04 & 0.02 & 0.03 & 0.02 & 0.02 & 0.04 \\
3054 & KOI-5 & 27 & 0.05 & 0.01 & 0.5 & 0.03 & 0.08 & 0.06 & 0.03 & 0.02 & 0.04 & 0.02 & 0.03 & 0.02 & 0.04 & 0.02 & 0.03 & 0.02 & 0.02 & 0.04 \\
3055 & KOI-3158 & 27 & 0.05 & 0.01 & 0.5 & 0.03 & 0.07 & 0.06 & 0.03 & 0.02 & 0.04 & 0.02 & 0.02 & 0.02 & 0.04 & 0.02 & 0.03 & 0.01 & 0.02 & 0.04 \\
3058 & KOI-123 & 28 & 0.05 & 0.01 & 0.5 & 0.04 & 0.08 & 0.06 & 0.03 & 0.02 & 0.04 & 0.02 & 0.03 & 0.02 & 0.04 & 0.02 & 0.03 & 0.02 & 0.02 & 0.04 \\
3059 & KOI-84 & 27 & 0.05 & 0.01 & 0.5 & 0.03 & 0.08 & 0.06 & 0.03 & 0.02 & 0.04 & 0.02 & 0.03 & 0.02 & 0.04 & 0.02 & 0.03 & 0.02 & 0.02 & 0.04 \\
3064 & KOI-277 & 27 & 0.05 & 0.01 & 0.5 & 0.03 & 0.08 & 0.06 & 0.03 & 0.02 & 0.04 & 0.02 & 0.02 & 0.02 & 0.04 & 0.02 & 0.03 & 0.02 & 0.02 & 0.04 \\
3065 & KOI-41 & 27 & 0.05 & 0.01 & 0.5 & 0.03 & 0.08 & 0.06 & 0.03 & 0.02 & 0.04 & 0.02 & 0.02 & 0.02 & 0.04 & 0.02 & 0.03 & 0.02 & 0.02 & 0.04 \\
3067 & KOI-69 & 27 & 0.05 & 0.01 & 0.5 & 0.03 & 0.08 & 0.06 & 0.03 & 0.02 & 0.04 & 0.02 & 0.02 & 0.02 & 0.04 & 0.02 & 0.03 & 0.02 & 0.02 & 0.04 \\
3068 & KOI-75 & 27 & 0.05 & 0.01 & 0.5 & 0.03 & 0.08 & 0.06 & 0.03 & 0.02 & 0.04 & 0.02 & 0.02 & 0.02 & 0.04 & 0.02 & 0.03 & 0.02 & 0.02 & 0.04 \\
3072 & KOI-103 & 29 & 0.06 & 0.02 & 0.6 & 0.04 & 0.10 & 0.07 & 0.04 & 0.02 & 0.05 & 0.03 & 0.03 & 0.02 & 0.05 & 0.02 & 0.04 & 0.02 & 0.02 & 0.05 \\
3074 & KOI-321 & 28 & 0.05 & 0.01 & 0.5 & 0.04 & 0.08 & 0.06 & 0.03 & 0.02 & 0.04 & 0.02 & 0.03 & 0.02 & 0.04 & 0.02 & 0.03 & 0.02 & 0.02 & 0.04 \\
3078 & KOI-2687 & 27 & 0.05 & 0.01 & 0.5 & 0.03 & 0.08 & 0.06 & 0.03 & 0.02 & 0.04 & 0.02 & 0.02 & 0.02 & 0.04 & 0.02 & 0.03 & 0.02 & 0.02 & 0.04 \\
3084 & KOI-1925 & 25 & 0.05 & 0.01 & 0.5 & 0.03 & 0.04 & 0.04 & 0.01 & 0.01 & 0.03 & 0.01 & 0.01 & 0.01 & 0.03 & 0.01 & 0.02 & 0.01 & 0.01 & 0.03 \\
3091 & KOI-1924 & 27 & 0.05 & 0.01 & 0.5 & 0.03 & 0.08 & 0.06 & 0.03 & 0.02 & 0.04 & 0.02 & 0.02 & 0.02 & 0.04 & 0.02 & 0.03 & 0.02 & 0.02 & 0.04 \\
3100 & KOI-99 & 27 & 0.05 & 0.01 & 0.5 & 0.03 & 0.07 & 0.06 & 0.03 & 0.02 & 0.04 & 0.02 & 0.02 & 0.02 & 0.04 & 0.02 & 0.03 & 0.02 & 0.02 & 0.04 \\
3101 & KOI-2720 & 27 & 0.05 & 0.01 & 0.5 & 0.03 & 0.08 & 0.06 & 0.03 & 0.02 & 0.04 & 0.02 & 0.02 & 0.02 & 0.04 & 0.02 & 0.03 & 0.02 & 0.02 & 0.04 \\
3103 & KOI-364 & 27 & 0.05 & 0.01 & 0.5 & 0.03 & 0.08 & 0.06 & 0.03 & 0.02 & 0.04 & 0.02 & 0.02 & 0.02 & 0.04 & 0.02 & 0.03 & 0.02 & 0.02 & 0.04 \\
3105 & KOI-64 & 27 & 0.05 & 0.01 & 0.5 & 0.03 & 0.07 & 0.06 & 0.03 & 0.02 & 0.04 & 0.02 & 0.02 & 0.02 & 0.04 & 0.02 & 0.03 & 0.02 & 0.02 & 0.04 \\
3110 & KOI-174 & 27 & 0.05 & 0.01 & 0.5 & 0.03 & 0.08 & 0.06 & 0.03 & 0.02 & 0.04 & 0.02 & 0.02 & 0.02 & 0.04 & 0.02 & 0.03 & 0.02 & 0.02 & 0.04 \\
3111 & KOI-17 & 27 & 0.05 & 0.01 & 0.5 & 0.03 & 0.07 & 0.06 & 0.03 & 0.02 & 0.04 & 0.02 & 0.02 & 0.02 & 0.04 & 0.02 & 0.03 & 0.02 & 0.02 & 0.04 \\
3113 & KOI-265 & 28 & 0.05 & 0.01 & 0.5 & 0.03 & 0.08 & 0.06 & 0.03 & 0.02 & 0.04 & 0.02 & 0.03 & 0.02 & 0.04 & 0.02 & 0.03 & 0.02 & 0.02 & 0.04 \\
3114 & KOI-261 & 27 & 0.05 & 0.01 & 0.5 & 0.03 & 0.08 & 0.06 & 0.03 & 0.02 & 0.04 & 0.02 & 0.02 & 0.02 & 0.04 & 0.02 & 0.03 & 0.02 & 0.02 & 0.04 \\
3117 & KOI-305 & 27 & 0.05 & 0.01 & 0.5 & 0.03 & 0.07 & 0.05 & 0.03 & 0.02 & 0.04 & 0.02 & 0.02 & 0.02 & 0.04 & 0.02 & 0.03 & 0.01 & 0.02 & 0.04 \\
3118 & KOI-365 & 27 & 0.05 & 0.01 & 0.5 & 0.03 & 0.08 & 0.06 & 0.03 & 0.02 & 0.04 & 0.02 & 0.02 & 0.02 & 0.04 & 0.02 & 0.03 & 0.02 & 0.02 & 0.04 \\
3123 & KOI-137 & 28 & 0.05 & 0.01 & 0.5 & 0.03 & 0.08 & 0.06 & 0.03 & 0.02 & 0.04 & 0.02 & 0.03 & 0.02 & 0.04 & 0.02 & 0.03 & 0.02 & 0.02 & 0.04 \\
3130 & KOI-148 & 27 & 0.05 & 0.01 & 0.5 & 0.03 & 0.07 & 0.06 & 0.03 & 0.02 & 0.04 & 0.02 & 0.02 & 0.02 & 0.04 & 0.02 & 0.03 & 0.01 & 0.02 & 0.04 \\
3131 & KOI-18 & 27 & 0.05 & 0.01 & 0.5 & 0.03 & 0.08 & 0.06 & 0.03 & 0.02 & 0.04 & 0.02 & 0.02 & 0.02 & 0.04 & 0.02 & 0.03 & 0.02 & 0.02 & 0.04 \\
3133 & KOI-116 & 27 & 0.05 & 0.01 & 0.5 & 0.03 & 0.08 & 0.06 & 0.03 & 0.02 & 0.04 & 0.02 & 0.02 & 0.02 & 0.04 & 0.02 & 0.03 & 0.02 & 0.02 & 0.04 \\
3239 & HD 240429 & 25 & 0.05 & 0.01 & 0.5 & 0.03 & 0.04 & 0.04 & 0.01 & 0.01 & 0.03 & 0.01 & 0.01 & 0.01 & 0.03 & 0.01 & 0.02 & 0.01 & 0.01 & 0.03 \\
3240 & HD 240430 & 25 & 0.05 & 0.01 & 0.5 & 0.03 & 0.04 & 0.04 & 0.01 & 0.01 & 0.03 & 0.01 & 0.01 & 0.01 & 0.03 & 0.01 & 0.02 & 0.01 & 0.01 & 0.03 \\
3248 & WASP-57 & 26 & 0.05 & 0.01 & 0.5 & 0.03 & 0.06 & 0.05 & 0.02 & 0.02 & 0.03 & 0.01 & 0.02 & 0.02 & 0.04 & 0.02 & 0.02 & 0.01 & 0.01 & 0.03 \\
3249 & WASP-74 & 25 & 0.05 & 0.01 & 0.5 & 0.03 & 0.04 & 0.04 & 0.01 & 0.01 & 0.03 & 0.01 & 0.01 & 0.01 & 0.03 & 0.01 & 0.02 & 0.01 & 0.01 & 0.03 \\
3250 & WASP-37 & 26 & 0.05 & 0.01 & 0.5 & 0.03 & 0.06 & 0.05 & 0.02 & 0.02 & 0.03 & 0.01 & 0.02 & 0.02 & 0.04 & 0.02 & 0.02 & 0.01 & 0.01 & 0.03 \\
3251 & HAT-P-41 & 25 & 0.05 & 0.01 & 0.5 & 0.03 & 0.04 & 0.04 & 0.01 & 0.01 & 0.03 & 0.01 & 0.01 & 0.01 & 0.03 & 0.01 & 0.02 & 0.01 & 0.01 & 0.03 \\
3252 & COROT-28 & 26 & 0.05 & 0.01 & 0.5 & 0.03 & 0.06 & 0.05 & 0.02 & 0.02 & 0.04 & 0.01 & 0.02 & 0.02 & 0.04 & 0.02 & 0.02 & 0.01 & 0.02 & 0.04 \\
3253 & HAT-P-27 & 25 & 0.05 & 0.01 & 0.5 & 0.03 & 0.04 & 0.04 & 0.01 & 0.01 & 0.03 & 0.01 & 0.01 & 0.01 & 0.03 & 0.01 & 0.02 & 0.01 & 0.01 & 0.03 \\
3254 & WASP-103 & 25 & 0.05 & 0.01 & 0.5 & 0.03 & 0.04 & 0.04 & 0.01 & 0.01 & 0.03 & 0.01 & 0.01 & 0.01 & 0.03 & 0.01 & 0.02 & 0.01 & 0.01 & 0.03 \\
3255 & WASP-52 & 25 & 0.05 & 0.01 & 0.5 & 0.03 & 0.04 & 0.04 & 0.01 & 0.01 & 0.03 & 0.01 & 0.01 & 0.01 & 0.03 & 0.01 & 0.02 & 0.01 & 0.01 & 0.03 \\
3256 & WASP-114 & 25 & 0.05 & 0.01 & 0.5 & 0.03 & 0.05 & 0.04 & 0.02 & 0.01 & 0.03 & 0.01 & 0.02 & 0.01 & 0.04 & 0.02 & 0.02 & 0.01 & 0.01 & 0.03 \\
3257 & BD+1290 & 25 & 0.05 & 0.01 & 0.5 & 0.03 & 0.04 & 0.04 & 0.01 & 0.01 & 0.03 & 0.01 & 0.01 & 0.01 & 0.03 & 0.01 & 0.02 & 0.01 & 0.01 & 0.03 \\
3258 & HD 4552 & 25 & 0.05 & 0.01 & 0.5 & 0.03 & 0.04 & 0.04 & 0.01 & 0.01 & 0.03 & 0.01 & 0.01 & 0.01 & 0.03 & 0.01 & 0.02 & 0.01 & 0.01 & 0.03 \\
3259 & HD 209622 & 25 & 0.05 & 0.01 & 0.5 & 0.03 & 0.04 & 0.04 & 0.01 & 0.01 & 0.03 & 0.01 & 0.01 & 0.01 & 0.03 & 0.01 & 0.02 & 0.01 & 0.01 & 0.03 \\
3260 & BD+15_4556 & 25 & 0.05 & 0.01 & 0.5 & 0.03 & 0.04 & 0.04 & 0.01 & 0.01 & 0.03 & 0.01 & 0.01 & 0.01 & 0.03 & 0.01 & 0.02 & 0.01 & 0.01 & 0.03 \\
3261 & HAT-P-23 & 25 & 0.05 & 0.01 & 0.5 & 0.03 & 0.04 & 0.04 & 0.01 & 0.01 & 0.03 & 0.01 & 0.01 & 0.01 & 0.03 & 0.01 & 0.02 & 0.01 & 0.01 & 0.03 \\
3262 & HAT-P-55 & 25 & 0.05 & 0.01 & 0.5 & 0.03 & 0.05 & 0.04 & 0.02 & 0.01 & 0.03 & 0.01 & 0.02 & 0.01 & 0.04 & 0.02 & 0.02 & 0.01 & 0.01 & 0.03 \\
3263 & HAT-P-31 & 25 & 0.05 & 0.01 & 0.5 & 0.03 & 0.04 & 0.04 & 0.01 & 0.01 & 0.03 & 0.01 & 0.01 & 0.01 & 0.03 & 0.01 & 0.02 & 0.01 & 0.01 & 0.03 \\
3264 & BD+28_4543S & 25 & 0.05 & 0.01 & 0.5 & 0.03 & 0.04 & 0.04 & 0.01 & 0.01 & 0.03 & 0.01 & 0.01 & 0.01 & 0.03 & 0.01 & 0.02 & 0.01 & 0.01 & 0.03 \\
3265 & WASP-135 & 25 & 0.05 & 0.01 & 0.5 & 0.03 & 0.05 & 0.04 & 0.02 & 0.01 & 0.03 & 0.01 & 0.02 & 0.01 & 0.04 & 0.02 & 0.02 & 0.01 & 0.01 & 0.03 \\
3266 & WASP-10 & 25 & 0.05 & 0.01 & 0.5 & 0.03 & 0.04 & 0.04 & 0.01 & 0.01 & 0.03 & 0.01 & 0.01 & 0.01 & 0.03 & 0.01 & 0.02 & 0.01 & 0.01 & 0.03 \\
3267 & KELT-16 & 25 & 0.05 & 0.01 & 0.5 & 0.03 & 0.04 & 0.04 & 0.01 & 0.01 & 0.03 & 0.01 & 0.01 & 0.01 & 0.03 & 0.01 & 0.02 & 0.01 & 0.01 & 0.03 \\
3268 & HAT-P-18 & 25 & 0.05 & 0.01 & 0.5 & 0.03 & 0.04 & 0.04 & 0.01 & 0.01 & 0.03 & 0.01 & 0.01 & 0.01 & 0.03 & 0.01 & 0.02 & 0.01 & 0.01 & 0.03 \\
3269 & HAT-P-4 & 25 & 0.05 & 0.01 & 0.5 & 0.03 & 0.04 & 0.04 & 0.01 & 0.01 & 0.03 & 0.01 & 0.01 & 0.01 & 0.03 & 0.01 & 0.02 & 0.01 & 0.01 & 0.03 \\
3270 & KELT-12 & 25 & 0.05 & 0.01 & 0.5 & 0.03 & 0.04 & 0.04 & 0.01 & 0.01 & 0.03 & 0.01 & 0.01 & 0.01 & 0.03 & 0.01 & 0.02 & 0.01 & 0.01 & 0.03 \\
3271 & KOI-958 & 27 & 0.05 & 0.01 & 0.5 & 0.03 & 0.07 & 0.06 & 0.03 & 0.02 & 0.04 & 0.02 & 0.02 & 0.02 & 0.04 & 0.02 & 0.03 & 0.02 & 0.02 & 0.04 \\
3272 & KOI-1010 & 28 & 0.06 & 0.02 & 0.5 & 0.04 & 0.09 & 0.07 & 0.03 & 0.02 & 0.05 & 0.02 & 0.03 & 0.02 & 0.05 & 0.02 & 0.03 & 0.02 & 0.02 & 0.04 \\
3273 & KOI-984 & 27 & 0.05 & 0.01 & 0.5 & 0.03 & 0.08 & 0.06 & 0.03 & 0.02 & 0.04 & 0.02 & 0.02 & 0.02 & 0.04 & 0.02 & 0.03 & 0.02 & 0.02 & 0.04 \\
3274 & KOI-4212 & 27 & 0.05 & 0.01 & 0.5 & 0.03 & 0.08 & 0.06 & 0.03 & 0.02 & 0.04 & 0.02 & 0.02 & 0.02 & 0.04 & 0.02 & 0.03 & 0.02 & 0.02 & 0.04 \\
3275 & KOI-1002 & 27 & 0.05 & 0.01 & 0.5 & 0.03 & 0.08 & 0.06 & 0.03 & 0.02 & 0.04 & 0.02 & 0.02 & 0.02 & 0.04 & 0.02 & 0.03 & 0.02 & 0.02 & 0.04 \\
3276 & KOI-2538 & 28 & 0.05 & 0.01 & 0.5 & 0.03 & 0.08 & 0.06 & 0.03 & 0.02 & 0.04 & 0.02 & 0.03 & 0.02 & 0.04 & 0.02 & 0.03 & 0.02 & 0.02 & 0.04 \\
3277 & KOI-2534 & 28 & 0.05 & 0.01 & 0.5 & 0.04 & 0.08 & 0.06 & 0.03 & 0.02 & 0.04 & 0.02 & 0.03 & 0.02 & 0.04 & 0.02 & 0.03 & 0.02 & 0.02 & 0.04 \\
3278 & KOI-3233 & 27 & 0.05 & 0.01 & 0.5 & 0.03 & 0.08 & 0.06 & 0.03 & 0.02 & 0.04 & 0.02 & 0.02 & 0.02 & 0.04 & 0.02 & 0.03 & 0.02 & 0.02 & 0.04 \\
3279 & KOI-2403 & 28 & 0.05 & 0.01 & 0.5 & 0.03 & 0.08 & 0.06 & 0.03 & 0.02 & 0.04 & 0.02 & 0.03 & 0.02 & 0.04 & 0.02 & 0.03 & 0.02 & 0.02 & 0.04 \\
3280 & KOI-2201 & 27 & 0.05 & 0.01 & 0.5 & 0.03 & 0.08 & 0.06 & 0.03 & 0.02 & 0.04 & 0.02 & 0.02 & 0.02 & 0.04 & 0.02 & 0.03 & 0.02 & 0.02 & 0.04 \\
3281 & KOI-988 & 27 & 0.05 & 0.01 & 0.5 & 0.03 & 0.07 & 0.06 & 0.03 & 0.02 & 0.04 & 0.02 & 0.02 & 0.02 & 0.04 & 0.02 & 0.03 & 0.02 & 0.02 & 0.04 \\
3282 & KOI-151 & 27 & 0.05 & 0.01 & 0.5 & 0.03 & 0.08 & 0.06 & 0.03 & 0.02 & 0.04 & 0.02 & 0.02 & 0.02 & 0.04 & 0.02 & 0.03 & 0.02 & 0.02 & 0.04 \\
3283 & KOI-113 & 27 & 0.05 & 0.01 & 0.5 & 0.03 & 0.07 & 0.06 & 0.03 & 0.02 & 0.04 & 0.02 & 0.02 & 0.02 & 0.04 & 0.02 & 0.03 & 0.02 & 0.02 & 0.04 \\
3284 & KOI-3201 & 27 & 0.05 & 0.01 & 0.5 & 0.03 & 0.08 & 0.06 & 0.03 & 0.02 & 0.04 & 0.02 & 0.02 & 0.02 & 0.04 & 0.02 & 0.03 & 0.02 & 0.02 & 0.04 \\
3285 & KOI-2053 & 27 & 0.05 & 0.01 & 0.5 & 0.03 & 0.08 & 0.06 & 0.03 & 0.02 & 0.04 & 0.02 & 0.02 & 0.02 & 0.04 & 0.02 & 0.03 & 0.02 & 0.02 & 0.04 \\
3286 & KOI-2033 & 28 & 0.05 & 0.01 & 0.5 & 0.03 & 0.08 & 0.06 & 0.03 & 0.02 & 0.04 & 0.02 & 0.03 & 0.02 & 0.04 & 0.02 & 0.03 & 0.02 & 0.02 & 0.04 \\
3287 & KOI-1944 & 27 & 0.05 & 0.01 & 0.5 & 0.03 & 0.08 & 0.06 & 0.03 & 0.02 & 0.04 & 0.02 & 0.02 & 0.02 & 0.04 & 0.02 & 0.03 & 0.02 & 0.02 & 0.04 \\
3288 & KOI-2603 & 27 & 0.05 & 0.01 & 0.5 & 0.03 & 0.08 & 0.06 & 0.03 & 0.02 & 0.04 & 0.02 & 0.03 & 0.02 & 0.04 & 0.02 & 0.03 & 0.02 & 0.02 & 0.04 \\
3289 & KOI-440 & 27 & 0.05 & 0.01 & 0.5 & 0.03 & 0.07 & 0.06 & 0.03 & 0.02 & 0.04 & 0.02 & 0.02 & 0.02 & 0.04 & 0.02 & 0.03 & 0.02 & 0.02 & 0.04 \\
3290 & KOI-166 & 27 & 0.05 & 0.01 & 0.5 & 0.03 & 0.07 & 0.06 & 0.03 & 0.02 & 0.04 & 0.02 & 0.02 & 0.02 & 0.04 & 0.02 & 0.03 & 0.02 & 0.02 & 0.04 \\
3291 & KOI-379 & 27 & 0.05 & 0.01 & 0.5 & 0.03 & 0.08 & 0.06 & 0.03 & 0.02 & 0.04 & 0.02 & 0.02 & 0.02 & 0.04 & 0.02 & 0.03 & 0.02 & 0.02 & 0.04 \\
3292 & KOI-2009 & 27 & 0.05 & 0.01 & 0.5 & 0.03 & 0.08 & 0.06 & 0.03 & 0.02 & 0.04 & 0.02 & 0.02 & 0.02 & 0.04 & 0.02 & 0.03 & 0.02 & 0.02 & 0.04 \\
3293 & KOI-4581 & 27 & 0.05 & 0.01 & 0.5 & 0.03 & 0.08 & 0.06 & 0.03 & 0.02 & 0.04 & 0.02 & 0.02 & 0.02 & 0.04 & 0.02 & 0.03 & 0.02 & 0.02 & 0.04 \\
3294 & KOI-3835 & 27 & 0.05 & 0.01 & 0.5 & 0.03 & 0.07 & 0.06 & 0.03 & 0.02 & 0.04 & 0.02 & 0.02 & 0.02 & 0.04 & 0.02 & 0.03 & 0.01 & 0.02 & 0.04 \\
3295 & KOI-3681 & 27 & 0.05 & 0.01 & 0.5 & 0.03 & 0.08 & 0.06 & 0.03 & 0.02 & 0.04 & 0.02 & 0.03 & 0.02 & 0.04 & 0.02 & 0.03 & 0.02 & 0.02 & 0.04 \\
3296 & KOI-3853 & 27 & 0.05 & 0.01 & 0.5 & 0.03 & 0.07 & 0.05 & 0.03 & 0.02 & 0.04 & 0.02 & 0.02 & 0.02 & 0.04 & 0.02 & 0.03 & 0.01 & 0.02 & 0.04 \\
3297 & KOI-2979 & 27 & 0.05 & 0.01 & 0.5 & 0.03 & 0.08 & 0.06 & 0.03 & 0.02 & 0.04 & 0.02 & 0.02 & 0.02 & 0.04 & 0.02 & 0.03 & 0.02 & 0.02 & 0.04 \\
3298 & KOI-986 & 27 & 0.05 & 0.01 & 0.5 & 0.03 & 0.08 & 0.06 & 0.03 & 0.02 & 0.04 & 0.02 & 0.03 & 0.02 & 0.04 & 0.02 & 0.03 & 0.02 & 0.02 & 0.04 \\
3299 & KOI-2896 & 28 & 0.05 & 0.01 & 0.5 & 0.03 & 0.08 & 0.06 & 0.03 & 0.02 & 0.04 & 0.02 & 0.03 & 0.02 & 0.04 & 0.02 & 0.03 & 0.02 & 0.02 & 0.04 \\
3300 & KOI-4659 & 28 & 0.06 & 0.02 & 0.5 & 0.04 & 0.09 & 0.07 & 0.03 & 0.02 & 0.05 & 0.02 & 0.03 & 0.02 & 0.05 & 0.02 & 0.03 & 0.02 & 0.02 & 0.04 \\
3301 & KOI-1118 & 27 & 0.05 & 0.01 & 0.5 & 0.03 & 0.08 & 0.06 & 0.03 & 0.02 & 0.04 & 0.02 & 0.02 & 0.02 & 0.04 & 0.02 & 0.03 & 0.02 & 0.02 & 0.04 \\
3302 & KOI-4298 & 28 & 0.05 & 0.02 & 0.5 & 0.04 & 0.08 & 0.06 & 0.03 & 0.02 & 0.05 & 0.02 & 0.03 & 0.02 & 0.04 & 0.02 & 0.03 & 0.02 & 0.02 & 0.04 \\
3303 & KOI-1113 & 27 & 0.05 & 0.01 & 0.5 & 0.03 & 0.08 & 0.06 & 0.03 & 0.02 & 0.04 & 0.02 & 0.03 & 0.02 & 0.04 & 0.02 & 0.03 & 0.02 & 0.02 & 0.04 \\
3304 & KOI-1116 & 27 & 0.05 & 0.01 & 0.5 & 0.03 & 0.08 & 0.06 & 0.03 & 0.02 & 0.04 & 0.02 & 0.03 & 0.02 & 0.04 & 0.02 & 0.03 & 0.02 & 0.02 & 0.04 \\
3305 & KOI-2081 & 27 & 0.05 & 0.01 & 0.5 & 0.03 & 0.08 & 0.06 & 0.03 & 0.02 & 0.04 & 0.02 & 0.02 & 0.02 & 0.04 & 0.02 & 0.03 & 0.02 & 0.02 & 0.04 \\
3306 & KOI-4400 & 27 & 0.05 & 0.01 & 0.5 & 0.03 & 0.08 & 0.06 & 0.03 & 0.02 & 0.04 & 0.02 & 0.02 & 0.02 & 0.04 & 0.02 & 0.03 & 0.02 & 0.02 & 0.04 \\
3307 & KOI-1824 & 27 & 0.05 & 0.01 & 0.5 & 0.03 & 0.08 & 0.06 & 0.03 & 0.02 & 0.04 & 0.02 & 0.02 & 0.02 & 0.04 & 0.02 & 0.03 & 0.02 & 0.02 & 0.04 \\
3308 & KOI-2807 & 28 & 0.05 & 0.01 & 0.5 & 0.03 & 0.08 & 0.06 & 0.03 & 0.02 & 0.04 & 0.02 & 0.03 & 0.02 & 0.04 & 0.02 & 0.03 & 0.02 & 0.02 & 0.04 \\
3309 & KOI-2335 & 27 & 0.05 & 0.01 & 0.5 & 0.03 & 0.08 & 0.06 & 0.03 & 0.02 & 0.04 & 0.02 & 0.02 & 0.02 & 0.04 & 0.02 & 0.03 & 0.02 & 0.02 & 0.04 \\
3310 & KOI-197 & 30 & 0.06 & 0.02 & 0.6 & 0.04 & 0.10 & 0.07 & 0.04 & 0.03 & 0.05 & 0.03 & 0.03 & 0.03 & 0.05 & 0.02 & 0.04 & 0.02 & 0.02 & 0.05 \\
3311 & KOI-4144 & 30 & 0.06 & 0.02 & 0.6 & 0.04 & 0.10 & 0.07 & 0.04 & 0.03 & 0.05 & 0.03 & 0.03 & 0.03 & 0.05 & 0.02 & 0.04 & 0.02 & 0.02 & 0.05 \\
3312 & KOI-1115 & 27 & 0.05 & 0.01 & 0.5 & 0.03 & 0.08 & 0.06 & 0.03 & 0.02 & 0.04 & 0.02 & 0.02 & 0.02 & 0.04 & 0.02 & 0.03 & 0.02 & 0.02 & 0.04 \\
3313 & HAT-P-14 & 25 & 0.05 & 0.01 & 0.5 & 0.03 & 0.04 & 0.04 & 0.01 & 0.01 & 0.03 & 0.01 & 0.01 & 0.01 & 0.03 & 0.01 & 0.02 & 0.01 & 0.01 & 0.03 \\
3314 & KOI-1878 & 27 & 0.05 & 0.01 & 0.5 & 0.03 & 0.08 & 0.06 & 0.03 & 0.02 & 0.04 & 0.02 & 0.02 & 0.02 & 0.04 & 0.02 & 0.03 & 0.02 & 0.02 & 0.04 \\
3315 & KOI-3277 & 27 & 0.05 & 0.01 & 0.5 & 0.03 & 0.08 & 0.06 & 0.03 & 0.02 & 0.04 & 0.02 & 0.02 & 0.02 & 0.04 & 0.02 & 0.03 & 0.02 & 0.02 & 0.04 \\
3316 & KOI-3203 & 27 & 0.05 & 0.01 & 0.5 & 0.03 & 0.08 & 0.06 & 0.03 & 0.02 & 0.04 & 0.02 & 0.03 & 0.02 & 0.04 & 0.02 & 0.03 & 0.02 & 0.02 & 0.04 \\
3317 & KOI-3225 & 27 & 0.05 & 0.01 & 0.5 & 0.03 & 0.07 & 0.06 & 0.03 & 0.02 & 0.04 & 0.02 & 0.02 & 0.02 & 0.04 & 0.02 & 0.03 & 0.02 & 0.02 & 0.04 \\
3318 & Kepler-24 & 29 & 0.06 & 0.02 & 0.6 & 0.04 & 0.09 & 0.07 & 0.04 & 0.02 & 0.05 & 0.02 & 0.03 & 0.02 & 0.05 & 0.02 & 0.04 & 0.02 & 0.02 & 0.05 \\
3319 & KOI-490 & 27 & 0.05 & 0.01 & 0.5 & 0.03 & 0.07 & 0.06 & 0.03 & 0.02 & 0.04 & 0.02 & 0.02 & 0.02 & 0.04 & 0.02 & 0.03 & 0.02 & 0.02 & 0.04 \\
3320 & KOI-1089 & 32 & 0.06 & 0.02 & 0.6 & 0.05 & 0.12 & 0.09 & 0.05 & 0.03 & 0.06 & 0.03 & 0.04 & 0.03 & 0.06 & 0.03 & 0.04 & 0.02 & 0.03 & 0.06 \\
3321 & KOI-2863 & 28 & 0.05 & 0.01 & 0.5 & 0.04 & 0.08 & 0.06 & 0.03 & 0.02 & 0.04 & 0.02 & 0.03 & 0.02 & 0.04 & 0.02 & 0.03 & 0.02 & 0.02 & 0.04 \\
3322 & KOI-3515 & 28 & 0.05 & 0.01 & 0.5 & 0.03 & 0.08 & 0.06 & 0.03 & 0.02 & 0.04 & 0.02 & 0.03 & 0.02 & 0.04 & 0.02 & 0.03 & 0.02 & 0.02 & 0.04 \\
3323 & KOI-401 & 26 & 0.05 & 0.01 & 0.5 & 0.03 & 0.06 & 0.05 & 0.02 & 0.02 & 0.04 & 0.02 & 0.02 & 0.02 & 0.04 & 0.02 & 0.03 & 0.01 & 0.02 & 0.04 \\
3324 & KOI-2278 & 28 & 0.05 & 0.01 & 0.5 & 0.04 & 0.08 & 0.06 & 0.03 & 0.02 & 0.04 & 0.02 & 0.03 & 0.02 & 0.04 & 0.02 & 0.03 & 0.02 & 0.02 & 0.04 \\
3325 & KOI-3172 & 27 & 0.05 & 0.01 & 0.5 & 0.03 & 0.08 & 0.06 & 0.03 & 0.02 & 0.04 & 0.02 & 0.02 & 0.02 & 0.04 & 0.02 & 0.03 & 0.02 & 0.02 & 0.04 \\
3326 & KOI-2974 & 28 & 0.05 & 0.01 & 0.5 & 0.04 & 0.08 & 0.06 & 0.03 & 0.02 & 0.05 & 0.02 & 0.03 & 0.02 & 0.04 & 0.02 & 0.03 & 0.02 & 0.02 & 0.04 \\
3327 & KOI-384 & 27 & 0.05 & 0.01 & 0.5 & 0.03 & 0.08 & 0.06 & 0.03 & 0.02 & 0.04 & 0.02 & 0.02 & 0.02 & 0.04 & 0.02 & 0.03 & 0.02 & 0.02 & 0.04 \\
3328 & KOI-2740 & 27 & 0.05 & 0.01 & 0.5 & 0.03 & 0.08 & 0.06 & 0.03 & 0.02 & 0.04 & 0.02 & 0.02 & 0.02 & 0.04 & 0.02 & 0.03 & 0.02 & 0.02 & 0.04 \\
3329 & KOI-1196 & 29 & 0.06 & 0.02 & 0.6 & 0.04 & 0.10 & 0.07 & 0.04 & 0.02 & 0.05 & 0.03 & 0.03 & 0.02 & 0.05 & 0.02 & 0.04 & 0.02 & 0.02 & 0.05 \\
3330 & KOI-1845 & 29 & 0.06 & 0.02 & 0.6 & 0.04 & 0.09 & 0.07 & 0.04 & 0.02 & 0.05 & 0.03 & 0.03 & 0.02 & 0.05 & 0.02 & 0.04 & 0.02 & 0.02 & 0.05 \\
3331 & KOI-3075 & 27 & 0.05 & 0.01 & 0.5 & 0.03 & 0.08 & 0.06 & 0.03 & 0.02 & 0.04 & 0.02 & 0.02 & 0.02 & 0.04 & 0.02 & 0.03 & 0.02 & 0.02 & 0.04 \\
3332 & KOI-268 & 27 & 0.05 & 0.01 & 0.5 & 0.03 & 0.08 & 0.06 & 0.03 & 0.02 & 0.04 & 0.02 & 0.03 & 0.02 & 0.04 & 0.02 & 0.03 & 0.02 & 0.02 & 0.04 \\
3333 & KOI-2043 & 29 & 0.06 & 0.02 & 0.5 & 0.04 & 0.09 & 0.07 & 0.03 & 0.02 & 0.05 & 0.02 & 0.03 & 0.02 & 0.05 & 0.02 & 0.03 & 0.02 & 0.02 & 0.05 \\
3334 & KOI-3876 & 27 & 0.05 & 0.01 & 0.5 & 0.03 & 0.07 & 0.06 & 0.03 & 0.02 & 0.04 & 0.02 & 0.02 & 0.02 & 0.04 & 0.02 & 0.03 & 0.02 & 0.02 & 0.04 \\
3335 & KOI-1218 & 27 & 0.05 & 0.01 & 0.5 & 0.03 & 0.08 & 0.06 & 0.03 & 0.02 & 0.04 & 0.02 & 0.03 & 0.02 & 0.04 & 0.02 & 0.03 & 0.02 & 0.02 & 0.04 \\
3336 & KOI-385 & 27 & 0.05 & 0.01 & 0.5 & 0.03 & 0.08 & 0.06 & 0.03 & 0.02 & 0.04 & 0.02 & 0.02 & 0.02 & 0.04 & 0.02 & 0.03 & 0.02 & 0.02 & 0.04 \\
3337 & KOI-3415 & 27 & 0.05 & 0.01 & 0.5 & 0.03 & 0.08 & 0.06 & 0.03 & 0.02 & 0.04 & 0.02 & 0.02 & 0.02 & 0.04 & 0.02 & 0.03 & 0.02 & 0.02 & 0.04 \\
3338 & KOI-3340 & 27 & 0.05 & 0.01 & 0.5 & 0.03 & 0.08 & 0.06 & 0.03 & 0.02 & 0.04 & 0.02 & 0.02 & 0.02 & 0.04 & 0.02 & 0.03 & 0.02 & 0.02 & 0.04 \\
3339 & KOI-3641 & 27 & 0.05 & 0.01 & 0.5 & 0.03 & 0.08 & 0.06 & 0.03 & 0.02 & 0.04 & 0.02 & 0.02 & 0.02 & 0.04 & 0.02 & 0.03 & 0.02 & 0.02 & 0.04 \\
3340 & KOI-118 & 27 & 0.05 & 0.01 & 0.5 & 0.03 & 0.08 & 0.06 & 0.03 & 0.02 & 0.04 & 0.02 & 0.02 & 0.02 & 0.04 & 0.02 & 0.03 & 0.02 & 0.02 & 0.04 \\
3341 & KOI-2755 & 27 & 0.05 & 0.01 & 0.5 & 0.03 & 0.08 & 0.06 & 0.03 & 0.02 & 0.04 & 0.02 & 0.02 & 0.02 & 0.04 & 0.02 & 0.03 & 0.02 & 0.02 & 0.04 \\
3342 & KOI-2194 & 28 & 0.06 & 0.02 & 0.5 & 0.04 & 0.09 & 0.06 & 0.03 & 0.02 & 0.05 & 0.02 & 0.03 & 0.02 & 0.05 & 0.02 & 0.03 & 0.02 & 0.02 & 0.04 \\
3343 & KOI-6102 & 27 & 0.05 & 0.01 & 0.5 & 0.03 & 0.08 & 0.06 & 0.03 & 0.02 & 0.04 & 0.02 & 0.03 & 0.02 & 0.04 & 0.02 & 0.03 & 0.02 & 0.02 & 0.04 \\
3344 & KOI-624 & 27 & 0.05 & 0.01 & 0.5 & 0.03 & 0.08 & 0.06 & 0.03 & 0.02 & 0.04 & 0.02 & 0.02 & 0.02 & 0.04 & 0.02 & 0.03 & 0.02 & 0.02 & 0.04 \\
3345 & KOI-1221 & 26 & 0.05 & 0.01 & 0.5 & 0.03 & 0.06 & 0.05 & 0.02 & 0.02 & 0.04 & 0.02 & 0.02 & 0.02 & 0.04 & 0.02 & 0.03 & 0.01 & 0.02 & 0.04 \\
3346 & KOI-386 & 27 & 0.05 & 0.01 & 0.5 & 0.03 & 0.08 & 0.06 & 0.03 & 0.02 & 0.04 & 0.02 & 0.03 & 0.02 & 0.04 & 0.02 & 0.03 & 0.02 & 0.02 & 0.04 \\
3347 & KOI-975 & 27 & 0.05 & 0.01 & 0.5 & 0.03 & 0.07 & 0.06 & 0.03 & 0.02 & 0.04 & 0.02 & 0.02 & 0.02 & 0.04 & 0.02 & 0.03 & 0.02 & 0.02 & 0.04 \\
3348 & KOI-2279 & 28 & 0.05 & 0.01 & 0.5 & 0.04 & 0.08 & 0.06 & 0.03 & 0.02 & 0.04 & 0.02 & 0.03 & 0.02 & 0.04 & 0.02 & 0.03 & 0.02 & 0.02 & 0.04 \\
3349 & KOI-302 & 28 & 0.05 & 0.01 & 0.5 & 0.04 & 0.08 & 0.06 & 0.03 & 0.02 & 0.04 & 0.02 & 0.03 & 0.02 & 0.04 & 0.02 & 0.03 & 0.02 & 0.02 & 0.04 \\
3350 & KOI-1901 & 27 & 0.05 & 0.01 & 0.5 & 0.03 & 0.08 & 0.06 & 0.03 & 0.02 & 0.04 & 0.02 & 0.03 & 0.02 & 0.04 & 0.02 & 0.03 & 0.02 & 0.02 & 0.04 \\
3351 & KOI-1861 & 27 & 0.05 & 0.01 & 0.5 & 0.03 & 0.08 & 0.06 & 0.03 & 0.02 & 0.04 & 0.02 & 0.03 & 0.02 & 0.04 & 0.02 & 0.03 & 0.02 & 0.02 & 0.04 \\
3352 & KOI-3308 & 27 & 0.05 & 0.01 & 0.5 & 0.03 & 0.08 & 0.06 & 0.03 & 0.02 & 0.04 & 0.02 & 0.02 & 0.02 & 0.04 & 0.02 & 0.03 & 0.02 & 0.02 & 0.04 \\
3353 & KOI-301 & 27 & 0.05 & 0.01 & 0.5 & 0.03 & 0.08 & 0.06 & 0.03 & 0.02 & 0.04 & 0.02 & 0.02 & 0.02 & 0.04 & 0.02 & 0.03 & 0.02 & 0.02 & 0.04 \\
3354 & KOI-2808 & 27 & 0.05 & 0.01 & 0.5 & 0.03 & 0.08 & 0.06 & 0.03 & 0.02 & 0.04 & 0.02 & 0.02 & 0.02 & 0.04 & 0.02 & 0.03 & 0.02 & 0.02 & 0.04 \\
3355 & KOI-442 & 27 & 0.05 & 0.01 & 0.5 & 0.03 & 0.08 & 0.06 & 0.03 & 0.02 & 0.04 & 0.02 & 0.02 & 0.02 & 0.04 & 0.02 & 0.03 & 0.02 & 0.02 & 0.04 \\
3356 & KOI-2261 & 28 & 0.05 & 0.01 & 0.5 & 0.04 & 0.08 & 0.06 & 0.03 & 0.02 & 0.05 & 0.02 & 0.03 & 0.02 & 0.04 & 0.02 & 0.03 & 0.02 & 0.02 & 0.04 \\
3357 & KOI-1206 & 27 & 0.05 & 0.01 & 0.5 & 0.03 & 0.08 & 0.06 & 0.03 & 0.02 & 0.04 & 0.02 & 0.02 & 0.02 & 0.04 & 0.02 & 0.03 & 0.02 & 0.02 & 0.04 \\
3358 & KOI-3002 & 27 & 0.05 & 0.01 & 0.5 & 0.03 & 0.08 & 0.06 & 0.03 & 0.02 & 0.04 & 0.02 & 0.02 & 0.02 & 0.04 & 0.02 & 0.03 & 0.02 & 0.02 & 0.04 \\
3359 & KOI-388 & 27 & 0.05 & 0.01 & 0.5 & 0.03 & 0.08 & 0.06 & 0.03 & 0.02 & 0.04 & 0.02 & 0.02 & 0.02 & 0.04 & 0.02 & 0.03 & 0.02 & 0.02 & 0.04 \\
3360 & KOI-444 & 27 & 0.05 & 0.01 & 0.5 & 0.03 & 0.08 & 0.06 & 0.03 & 0.02 & 0.04 & 0.02 & 0.03 & 0.02 & 0.04 & 0.02 & 0.03 & 0.02 & 0.02 & 0.04 \\
3361 & KOI-149 & 27 & 0.05 & 0.01 & 0.5 & 0.03 & 0.08 & 0.06 & 0.03 & 0.02 & 0.04 & 0.02 & 0.02 & 0.02 & 0.04 & 0.02 & 0.03 & 0.02 & 0.02 & 0.04 \\
3362 & KOI-2289 & 27 & 0.05 & 0.01 & 0.5 & 0.03 & 0.08 & 0.06 & 0.03 & 0.02 & 0.04 & 0.02 & 0.02 & 0.02 & 0.04 & 0.02 & 0.03 & 0.02 & 0.02 & 0.04 \\
3363 & KOI-4423 & 27 & 0.05 & 0.01 & 0.5 & 0.03 & 0.08 & 0.06 & 0.03 & 0.02 & 0.04 & 0.02 & 0.02 & 0.02 & 0.04 & 0.02 & 0.03 & 0.02 & 0.02 & 0.04 \\
3364 & KOI-1216 & 27 & 0.05 & 0.01 & 0.5 & 0.03 & 0.08 & 0.06 & 0.03 & 0.02 & 0.04 & 0.02 & 0.02 & 0.02 & 0.04 & 0.02 & 0.03 & 0.02 & 0.02 & 0.04 \\
3365 & KOI-1208 & 27 & 0.05 & 0.01 & 0.5 & 0.03 & 0.08 & 0.06 & 0.03 & 0.02 & 0.04 & 0.02 & 0.03 & 0.02 & 0.04 & 0.02 & 0.03 & 0.02 & 0.02 & 0.04 \\
3366 & KOI-2904 & 27 & 0.05 & 0.01 & 0.5 & 0.03 & 0.08 & 0.06 & 0.03 & 0.02 & 0.04 & 0.02 & 0.02 & 0.02 & 0.04 & 0.02 & 0.03 & 0.02 & 0.02 & 0.04 \\
3367 & KOI-393 & 28 & 0.05 & 0.01 & 0.5 & 0.03 & 0.08 & 0.06 & 0.03 & 0.02 & 0.04 & 0.02 & 0.03 & 0.02 & 0.04 & 0.02 & 0.03 & 0.02 & 0.02 & 0.04 \\
3368 & KOI-3180 & 27 & 0.05 & 0.01 & 0.5 & 0.03 & 0.08 & 0.06 & 0.03 & 0.02 & 0.04 & 0.02 & 0.02 & 0.02 & 0.04 & 0.02 & 0.03 & 0.02 & 0.02 & 0.04 \\
3369 & KOI-392 & 27 & 0.05 & 0.01 & 0.5 & 0.03 & 0.08 & 0.06 & 0.03 & 0.02 & 0.04 & 0.02 & 0.02 & 0.02 & 0.04 & 0.02 & 0.03 & 0.02 & 0.02 & 0.04 \\
3370 & KOI-1336 & 32 & 0.06 & 0.02 & 0.6 & 0.05 & 0.12 & 0.09 & 0.05 & 0.03 & 0.06 & 0.03 & 0.04 & 0.03 & 0.06 & 0.03 & 0.04 & 0.02 & 0.03 & 0.06 \\
3371 & KOI-4887 & 27 & 0.05 & 0.01 & 0.5 & 0.03 & 0.08 & 0.06 & 0.03 & 0.02 & 0.04 & 0.02 & 0.02 & 0.02 & 0.04 & 0.02 & 0.03 & 0.02 & 0.02 & 0.04 \\
3372 & KOI-1222 & 29 & 0.06 & 0.02 & 0.6 & 0.04 & 0.09 & 0.07 & 0.04 & 0.02 & 0.05 & 0.03 & 0.03 & 0.02 & 0.05 & 0.02 & 0.04 & 0.02 & 0.02 & 0.05 \\
3373 & KOI-280 & 27 & 0.05 & 0.01 & 0.5 & 0.03 & 0.08 & 0.06 & 0.03 & 0.02 & 0.04 & 0.02 & 0.02 & 0.02 & 0.04 & 0.02 & 0.03 & 0.02 & 0.02 & 0.04 \\
3374 & KOI-1335 & 27 & 0.05 & 0.01 & 0.5 & 0.03 & 0.08 & 0.06 & 0.03 & 0.02 & 0.04 & 0.02 & 0.02 & 0.02 & 0.04 & 0.02 & 0.03 & 0.02 & 0.02 & 0.04 \\
3375 & KOI-2202 & 28 & 0.05 & 0.01 & 0.5 & 0.03 & 0.08 & 0.06 & 0.03 & 0.02 & 0.04 & 0.02 & 0.03 & 0.02 & 0.04 & 0.02 & 0.03 & 0.02 & 0.02 & 0.04 \\
3376 & KOI-1344 & 27 & 0.05 & 0.01 & 0.5 & 0.03 & 0.08 & 0.06 & 0.03 & 0.02 & 0.04 & 0.02 & 0.02 & 0.02 & 0.04 & 0.02 & 0.03 & 0.02 & 0.02 & 0.04 \\
3377 & KOI-281 & 27 & 0.05 & 0.01 & 0.5 & 0.03 & 0.08 & 0.06 & 0.03 & 0.02 & 0.04 & 0.02 & 0.02 & 0.02 & 0.04 & 0.02 & 0.03 & 0.02 & 0.02 & 0.04 \\
3378 & KOI-2866 & 27 & 0.05 & 0.01 & 0.5 & 0.03 & 0.08 & 0.06 & 0.03 & 0.02 & 0.04 & 0.02 & 0.02 & 0.02 & 0.04 & 0.02 & 0.03 & 0.02 & 0.02 & 0.04 \\
3379 & KOI-144 & 27 & 0.05 & 0.01 & 0.5 & 0.03 & 0.07 & 0.05 & 0.03 & 0.02 & 0.04 & 0.02 & 0.02 & 0.02 & 0.04 & 0.02 & 0.03 & 0.01 & 0.02 & 0.04 \\
3380 & KOI-3864 & 27 & 0.05 & 0.01 & 0.5 & 0.03 & 0.07 & 0.06 & 0.03 & 0.02 & 0.04 & 0.02 & 0.02 & 0.02 & 0.04 & 0.02 & 0.03 & 0.01 & 0.02 & 0.04 \\
3381 & KOI-3880 & 27 & 0.05 & 0.01 & 0.5 & 0.03 & 0.08 & 0.06 & 0.03 & 0.02 & 0.04 & 0.02 & 0.02 & 0.02 & 0.04 & 0.02 & 0.03 & 0.02 & 0.02 & 0.04 \\
3382 & KOI-1864 & 27 & 0.05 & 0.01 & 0.5 & 0.03 & 0.08 & 0.06 & 0.03 & 0.02 & 0.04 & 0.02 & 0.02 & 0.02 & 0.04 & 0.02 & 0.03 & 0.02 & 0.02 & 0.04 \\
3383 & KOI-3678 & 27 & 0.05 & 0.01 & 0.5 & 0.03 & 0.08 & 0.06 & 0.03 & 0.02 & 0.04 & 0.02 & 0.02 & 0.02 & 0.04 & 0.02 & 0.03 & 0.02 & 0.02 & 0.04 \\
3384 & KOI-551 & 29 & 0.06 & 0.02 & 0.5 & 0.04 & 0.09 & 0.07 & 0.04 & 0.02 & 0.05 & 0.02 & 0.03 & 0.02 & 0.05 & 0.02 & 0.03 & 0.02 & 0.02 & 0.05 \\
3385 & KOI-3202 & 27 & 0.05 & 0.01 & 0.5 & 0.03 & 0.08 & 0.06 & 0.03 & 0.02 & 0.04 & 0.02 & 0.02 & 0.02 & 0.04 & 0.02 & 0.03 & 0.02 & 0.02 & 0.04 \\
3386 & KOI-2311 & 27 & 0.05 & 0.01 & 0.5 & 0.03 & 0.07 & 0.06 & 0.03 & 0.02 & 0.04 & 0.02 & 0.02 & 0.02 & 0.04 & 0.02 & 0.03 & 0.02 & 0.02 & 0.04 \\
3387 & KOI-1619 & 27 & 0.05 & 0.01 & 0.5 & 0.03 & 0.07 & 0.05 & 0.03 & 0.02 & 0.04 & 0.02 & 0.02 & 0.02 & 0.04 & 0.02 & 0.03 & 0.01 & 0.02 & 0.04 \\
3388 & KOI-5048 & 29 & 0.06 & 0.02 & 0.5 & 0.04 & 0.09 & 0.07 & 0.04 & 0.02 & 0.05 & 0.02 & 0.03 & 0.02 & 0.05 & 0.02 & 0.03 & 0.02 & 0.02 & 0.05 \\
3389 & KOI-3358 & 28 & 0.05 & 0.02 & 0.5 & 0.04 & 0.08 & 0.06 & 0.03 & 0.02 & 0.05 & 0.02 & 0.03 & 0.02 & 0.05 & 0.02 & 0.03 & 0.02 & 0.02 & 0.04 \\
3390 & KOI-3928 & 28 & 0.05 & 0.01 & 0.5 & 0.03 & 0.08 & 0.06 & 0.03 & 0.02 & 0.04 & 0.02 & 0.03 & 0.02 & 0.04 & 0.02 & 0.03 & 0.02 & 0.02 & 0.04 \\
3391 & KOI-3528 & 27 & 0.05 & 0.01 & 0.5 & 0.03 & 0.08 & 0.06 & 0.03 & 0.02 & 0.04 & 0.02 & 0.02 & 0.02 & 0.04 & 0.02 & 0.03 & 0.02 & 0.02 & 0.04 \\
3392 & KOI-1615 & 27 & 0.05 & 0.01 & 0.5 & 0.03 & 0.07 & 0.06 & 0.03 & 0.02 & 0.04 & 0.02 & 0.02 & 0.02 & 0.04 & 0.02 & 0.03 & 0.02 & 0.02 & 0.04 \\
3393 & KOI-403 & 28 & 0.05 & 0.01 & 0.5 & 0.04 & 0.08 & 0.06 & 0.03 & 0.02 & 0.04 & 0.02 & 0.03 & 0.02 & 0.04 & 0.02 & 0.03 & 0.02 & 0.02 & 0.04 \\
3394 & KOI-4774 & 27 & 0.05 & 0.01 & 0.5 & 0.03 & 0.07 & 0.06 & 0.03 & 0.02 & 0.04 & 0.02 & 0.02 & 0.02 & 0.04 & 0.02 & 0.03 & 0.02 & 0.02 & 0.04 \\
3395 & KOI-5057 & 29 & 0.06 & 0.02 & 0.6 & 0.04 & 0.09 & 0.07 & 0.04 & 0.02 & 0.05 & 0.03 & 0.03 & 0.02 & 0.05 & 0.02 & 0.04 & 0.02 & 0.02 & 0.05 \\
3396 & KOI-2787 & 27 & 0.05 & 0.01 & 0.5 & 0.03 & 0.08 & 0.06 & 0.03 & 0.02 & 0.04 & 0.02 & 0.02 & 0.02 & 0.04 & 0.02 & 0.03 & 0.02 & 0.02 & 0.04 \\
3397 & KOI-1738 & 27 & 0.05 & 0.01 & 0.5 & 0.03 & 0.07 & 0.06 & 0.03 & 0.02 & 0.04 & 0.02 & 0.02 & 0.02 & 0.04 & 0.02 & 0.03 & 0.02 & 0.02 & 0.04 \\
3398 & KOI-3378 & 28 & 0.05 & 0.01 & 0.5 & 0.03 & 0.08 & 0.06 & 0.03 & 0.02 & 0.04 & 0.02 & 0.03 & 0.02 & 0.04 & 0.02 & 0.03 & 0.02 & 0.02 & 0.04 \\
3399 & KOI-1803 & 27 & 0.05 & 0.01 & 0.5 & 0.03 & 0.07 & 0.05 & 0.03 & 0.02 & 0.04 & 0.02 & 0.02 & 0.02 & 0.04 & 0.02 & 0.03 & 0.01 & 0.02 & 0.04 \\
3400 & KOI-4452 & 27 & 0.05 & 0.01 & 0.5 & 0.03 & 0.08 & 0.06 & 0.03 & 0.02 & 0.04 & 0.02 & 0.02 & 0.02 & 0.04 & 0.02 & 0.03 & 0.02 & 0.02 & 0.04 \\
3401 & KOI-3168 & 25 & 0.05 & 0.01 & 0.5 & 0.03 & 0.04 & 0.04 & 0.01 & 0.01 & 0.03 & 0.01 & 0.01 & 0.01 & 0.03 & 0.01 & 0.02 & 0.01 & 0.01 & 0.03 \\
3402 & KOI-626 & 28 & 0.05 & 0.01 & 0.5 & 0.03 & 0.08 & 0.06 & 0.03 & 0.02 & 0.04 & 0.02 & 0.03 & 0.02 & 0.04 & 0.02 & 0.03 & 0.02 & 0.02 & 0.04 \\
3403 & KOI-1338 & 30 & 0.06 & 0.02 & 0.6 & 0.04 & 0.10 & 0.07 & 0.04 & 0.03 & 0.05 & 0.03 & 0.03 & 0.03 & 0.05 & 0.02 & 0.04 & 0.02 & 0.02 & 0.05 \\
3404 & KOI-1332 & 28 & 0.06 & 0.02 & 0.5 & 0.04 & 0.09 & 0.07 & 0.03 & 0.02 & 0.05 & 0.02 & 0.03 & 0.02 & 0.05 & 0.02 & 0.03 & 0.02 & 0.02 & 0.05 \\
3405 & KOI-2547 & 28 & 0.06 & 0.02 & 0.5 & 0.04 & 0.08 & 0.06 & 0.03 & 0.02 & 0.05 & 0.02 & 0.03 & 0.02 & 0.05 & 0.02 & 0.03 & 0.02 & 0.02 & 0.04 \\
3406 & KOI-4288 & 27 & 0.05 & 0.01 & 0.5 & 0.03 & 0.08 & 0.06 & 0.03 & 0.02 & 0.04 & 0.02 & 0.02 & 0.02 & 0.04 & 0.02 & 0.03 & 0.02 & 0.02 & 0.04 \\
3407 & KOI-3181 & 27 & 0.05 & 0.01 & 0.5 & 0.03 & 0.07 & 0.06 & 0.03 & 0.02 & 0.04 & 0.02 & 0.02 & 0.02 & 0.04 & 0.02 & 0.03 & 0.02 & 0.02 & 0.04 \\
3408 & KOI-627 & 27 & 0.05 & 0.01 & 0.5 & 0.03 & 0.08 & 0.06 & 0.03 & 0.02 & 0.04 & 0.02 & 0.02 & 0.02 & 0.04 & 0.02 & 0.03 & 0.02 & 0.02 & 0.04 \\
3409 & KOI-4157 & 27 & 0.05 & 0.01 & 0.5 & 0.03 & 0.08 & 0.06 & 0.03 & 0.02 & 0.04 & 0.02 & 0.02 & 0.02 & 0.04 & 0.02 & 0.03 & 0.02 & 0.02 & 0.04 \\
3410 & KOI-2025 & 28 & 0.05 & 0.01 & 0.5 & 0.04 & 0.08 & 0.06 & 0.03 & 0.02 & 0.04 & 0.02 & 0.03 & 0.02 & 0.04 & 0.02 & 0.03 & 0.02 & 0.02 & 0.04 \\
3411 & Kepler-350 & 26 & 0.05 & 0.01 & 0.5 & 0.03 & 0.06 & 0.05 & 0.02 & 0.02 & 0.04 & 0.02 & 0.02 & 0.02 & 0.04 & 0.02 & 0.03 & 0.01 & 0.02 & 0.04 \\
3412 & KOI-628 & 28 & 0.05 & 0.02 & 0.5 & 0.04 & 0.08 & 0.06 & 0.03 & 0.02 & 0.05 & 0.02 & 0.03 & 0.02 & 0.05 & 0.02 & 0.03 & 0.02 & 0.02 & 0.04 \\
3413 & KOI-3811 & 27 & 0.05 & 0.01 & 0.5 & 0.03 & 0.08 & 0.06 & 0.03 & 0.02 & 0.04 & 0.02 & 0.02 & 0.02 & 0.04 & 0.02 & 0.03 & 0.02 & 0.02 & 0.04 \\
3414 & KOI-629 & 28 & 0.06 & 0.02 & 0.5 & 0.04 & 0.08 & 0.06 & 0.03 & 0.02 & 0.05 & 0.02 & 0.03 & 0.02 & 0.05 & 0.02 & 0.03 & 0.02 & 0.02 & 0.04 \\
3415 & KOI-1805 & 27 & 0.05 & 0.01 & 0.5 & 0.03 & 0.08 & 0.06 & 0.03 & 0.02 & 0.04 & 0.02 & 0.02 & 0.02 & 0.04 & 0.02 & 0.03 & 0.02 & 0.02 & 0.04 \\
3416 & KOI-2393 & 30 & 0.06 & 0.02 & 0.6 & 0.04 & 0.10 & 0.08 & 0.04 & 0.03 & 0.06 & 0.03 & 0.03 & 0.03 & 0.05 & 0.02 & 0.04 & 0.02 & 0.02 & 0.05 \\
3417 & KOI-1534 & 28 & 0.06 & 0.02 & 0.5 & 0.04 & 0.08 & 0.06 & 0.03 & 0.02 & 0.05 & 0.02 & 0.03 & 0.02 & 0.05 & 0.02 & 0.03 & 0.02 & 0.02 & 0.04 \\
3418 & KOI-3184 & 27 & 0.05 & 0.01 & 0.5 & 0.03 & 0.08 & 0.06 & 0.03 & 0.02 & 0.04 & 0.02 & 0.02 & 0.02 & 0.04 & 0.02 & 0.03 & 0.02 & 0.02 & 0.04 \\
3419 & KOI-4367 & 27 & 0.05 & 0.01 & 0.5 & 0.03 & 0.08 & 0.06 & 0.03 & 0.02 & 0.04 & 0.02 & 0.02 & 0.02 & 0.04 & 0.02 & 0.03 & 0.02 & 0.02 & 0.04 \\
3420 & KOI-4004 & 27 & 0.05 & 0.01 & 0.5 & 0.03 & 0.07 & 0.06 & 0.03 & 0.02 & 0.04 & 0.02 & 0.02 & 0.02 & 0.04 & 0.02 & 0.03 & 0.02 & 0.02 & 0.04 \\
3421 & KOI-2120 & 27 & 0.05 & 0.01 & 0.5 & 0.03 & 0.08 & 0.06 & 0.03 & 0.02 & 0.04 & 0.02 & 0.02 & 0.02 & 0.04 & 0.02 & 0.03 & 0.02 & 0.02 & 0.04 \\
3422 & KOI-4639 & 27 & 0.05 & 0.01 & 0.5 & 0.03 & 0.08 & 0.06 & 0.03 & 0.02 & 0.04 & 0.02 & 0.03 & 0.02 & 0.04 & 0.02 & 0.03 & 0.02 & 0.02 & 0.04 \\
3423 & KOI-633 & 27 & 0.05 & 0.01 & 0.5 & 0.03 & 0.08 & 0.06 & 0.03 & 0.02 & 0.04 & 0.02 & 0.03 & 0.02 & 0.04 & 0.02 & 0.03 & 0.02 & 0.02 & 0.04 \\
3424 & KOI-632 & 27 & 0.05 & 0.01 & 0.5 & 0.03 & 0.08 & 0.06 & 0.03 & 0.02 & 0.04 & 0.02 & 0.02 & 0.02 & 0.04 & 0.02 & 0.03 & 0.02 & 0.02 & 0.04 \\
3425 & KOI-232 & 35 & 0.07 & 0.02 & 0.6 & 0.05 & 0.14 & 0.10 & 0.06 & 0.04 & 0.07 & 0.04 & 0.04 & 0.04 & 0.06 & 0.03 & 0.05 & 0.03 & 0.03 & 0.07 \\
3426 & Kepler-122 & 27 & 0.05 & 0.01 & 0.5 & 0.03 & 0.07 & 0.06 & 0.03 & 0.02 & 0.04 & 0.02 & 0.02 & 0.02 & 0.04 & 0.02 & 0.03 & 0.01 & 0.02 & 0.04 \\
3427 & KOI-3823 & 28 & 0.05 & 0.01 & 0.5 & 0.04 & 0.08 & 0.06 & 0.03 & 0.02 & 0.04 & 0.02 & 0.03 & 0.02 & 0.04 & 0.02 & 0.03 & 0.02 & 0.02 & 0.04 \\
3428 & KOI-3936 & 27 & 0.05 & 0.01 & 0.5 & 0.03 & 0.07 & 0.06 & 0.03 & 0.02 & 0.04 & 0.02 & 0.02 & 0.02 & 0.04 & 0.02 & 0.03 & 0.01 & 0.02 & 0.04 \\
3429 & KOI-1665 & 27 & 0.05 & 0.01 & 0.5 & 0.03 & 0.08 & 0.06 & 0.03 & 0.02 & 0.04 & 0.02 & 0.02 & 0.02 & 0.04 & 0.02 & 0.03 & 0.02 & 0.02 & 0.04 \\
3430 & KOI-4018 & 30 & 0.06 & 0.02 & 0.6 & 0.04 & 0.10 & 0.07 & 0.04 & 0.03 & 0.05 & 0.03 & 0.03 & 0.03 & 0.05 & 0.02 & 0.04 & 0.02 & 0.02 & 0.05 \\
3431 & KOI-2635 & 28 & 0.05 & 0.01 & 0.5 & 0.04 & 0.08 & 0.06 & 0.03 & 0.02 & 0.04 & 0.02 & 0.03 & 0.02 & 0.04 & 0.02 & 0.03 & 0.02 & 0.02 & 0.04 \\
3432 & KOI-5107 & 29 & 0.06 & 0.02 & 0.6 & 0.04 & 0.10 & 0.07 & 0.04 & 0.02 & 0.05 & 0.03 & 0.03 & 0.02 & 0.05 & 0.02 & 0.04 & 0.02 & 0.02 & 0.05 \\
3433 & KOI-3770 & 28 & 0.05 & 0.01 & 0.5 & 0.04 & 0.08 & 0.06 & 0.03 & 0.02 & 0.05 & 0.02 & 0.03 & 0.02 & 0.04 & 0.02 & 0.03 & 0.02 & 0.02 & 0.04 \\
3434 & KOI-5119 & 29 & 0.06 & 0.02 & 0.5 & 0.04 & 0.09 & 0.07 & 0.04 & 0.02 & 0.05 & 0.02 & 0.03 & 0.02 & 0.05 & 0.02 & 0.03 & 0.02 & 0.02 & 0.05 \\
3435 & KOI-4546 & 28 & 0.06 & 0.02 & 0.5 & 0.04 & 0.08 & 0.06 & 0.03 & 0.02 & 0.05 & 0.02 & 0.03 & 0.02 & 0.05 & 0.02 & 0.03 & 0.02 & 0.02 & 0.04 \\
3436 & KOI-2951 & 27 & 0.05 & 0.01 & 0.5 & 0.03 & 0.08 & 0.06 & 0.03 & 0.02 & 0.04 & 0.02 & 0.02 & 0.02 & 0.04 & 0.02 & 0.03 & 0.02 & 0.02 & 0.04 \\
3437 & KOI-3421 & 27 & 0.05 & 0.01 & 0.5 & 0.03 & 0.08 & 0.06 & 0.03 & 0.02 & 0.04 & 0.02 & 0.02 & 0.02 & 0.04 & 0.02 & 0.03 & 0.02 & 0.02 & 0.04 \\
3438 & KOI-1666 & 30 & 0.06 & 0.02 & 0.6 & 0.04 & 0.10 & 0.07 & 0.04 & 0.03 & 0.05 & 0.03 & 0.03 & 0.03 & 0.05 & 0.02 & 0.04 & 0.02 & 0.02 & 0.05 \\
3439 & KOI-635 & 27 & 0.05 & 0.01 & 0.5 & 0.03 & 0.08 & 0.06 & 0.03 & 0.02 & 0.04 & 0.02 & 0.02 & 0.02 & 0.04 & 0.02 & 0.03 & 0.02 & 0.02 & 0.04 \\
3440 & KOI-161 & 27 & 0.05 & 0.01 & 0.5 & 0.03 & 0.07 & 0.06 & 0.03 & 0.02 & 0.04 & 0.02 & 0.02 & 0.02 & 0.04 & 0.02 & 0.03 & 0.01 & 0.02 & 0.04 \\
3441 & KOI-639 & 27 & 0.05 & 0.01 & 0.5 & 0.03 & 0.08 & 0.06 & 0.03 & 0.02 & 0.04 & 0.02 & 0.02 & 0.02 & 0.04 & 0.02 & 0.03 & 0.02 & 0.02 & 0.04 \\
3442 & KOI-3093 & 27 & 0.05 & 0.01 & 0.5 & 0.03 & 0.08 & 0.06 & 0.03 & 0.02 & 0.04 & 0.02 & 0.02 & 0.02 & 0.04 & 0.02 & 0.03 & 0.02 & 0.02 & 0.04 \\
3443 & Kepler-130 & 25 & 0.05 & 0.01 & 0.5 & 0.03 & 0.04 & 0.04 & 0.01 & 0.01 & 0.03 & 0.01 & 0.01 & 0.01 & 0.03 & 0.01 & 0.02 & 0.01 & 0.01 & 0.03 \\
3444 & KOI-282 & 27 & 0.05 & 0.01 & 0.5 & 0.03 & 0.08 & 0.06 & 0.03 & 0.02 & 0.04 & 0.02 & 0.02 & 0.02 & 0.04 & 0.02 & 0.03 & 0.02 & 0.02 & 0.04 \\
3445 & KOI-4331 & 27 & 0.05 & 0.01 & 0.5 & 0.03 & 0.08 & 0.06 & 0.03 & 0.02 & 0.04 & 0.02 & 0.02 & 0.02 & 0.04 & 0.02 & 0.03 & 0.02 & 0.02 & 0.04 \\
3446 & KOI-1822 & 27 & 0.05 & 0.01 & 0.5 & 0.03 & 0.08 & 0.06 & 0.03 & 0.02 & 0.04 & 0.02 & 0.02 & 0.02 & 0.04 & 0.02 & 0.03 & 0.02 & 0.02 & 0.04 \\
3447 & KOI-640 & 27 & 0.05 & 0.01 & 0.5 & 0.03 & 0.07 & 0.06 & 0.03 & 0.02 & 0.04 & 0.02 & 0.02 & 0.02 & 0.04 & 0.02 & 0.03 & 0.02 & 0.02 & 0.04 \\
3448 & KOI-2698 & 27 & 0.05 & 0.01 & 0.5 & 0.03 & 0.08 & 0.06 & 0.03 & 0.02 & 0.04 & 0.02 & 0.02 & 0.02 & 0.04 & 0.02 & 0.03 & 0.02 & 0.02 & 0.04 \\
3449 & KOI-1563 & 33 & 0.06 & 0.02 & 0.6 & 0.05 & 0.13 & 0.09 & 0.05 & 0.03 & 0.07 & 0.04 & 0.04 & 0.03 & 0.06 & 0.03 & 0.05 & 0.02 & 0.03 & 0.06 \\
3450 & KOI-3474 & 27 & 0.05 & 0.01 & 0.5 & 0.03 & 0.08 & 0.06 & 0.03 & 0.02 & 0.04 & 0.02 & 0.03 & 0.02 & 0.04 & 0.02 & 0.03 & 0.02 & 0.02 & 0.04 \\
3451 & KOI-2158 & 27 & 0.05 & 0.01 & 0.5 & 0.03 & 0.08 & 0.06 & 0.03 & 0.02 & 0.04 & 0.02 & 0.02 & 0.02 & 0.04 & 0.02 & 0.03 & 0.02 & 0.02 & 0.04 \\
3452 & KOI-2563 & 27 & 0.05 & 0.01 & 0.5 & 0.03 & 0.08 & 0.06 & 0.03 & 0.02 & 0.04 & 0.02 & 0.02 & 0.02 & 0.04 & 0.02 & 0.03 & 0.02 & 0.02 & 0.04 \\
3453 & KOI-4246 & 27 & 0.05 & 0.01 & 0.5 & 0.03 & 0.08 & 0.06 & 0.03 & 0.02 & 0.04 & 0.02 & 0.02 & 0.02 & 0.04 & 0.02 & 0.03 & 0.02 & 0.02 & 0.04 \\
3454 & KOI-1576 & 27 & 0.05 & 0.01 & 0.5 & 0.03 & 0.08 & 0.06 & 0.03 & 0.02 & 0.04 & 0.02 & 0.02 & 0.02 & 0.04 & 0.02 & 0.03 & 0.02 & 0.02 & 0.04 \\
3455 & KOI-825 & 31 & 0.06 & 0.02 & 0.6 & 0.04 & 0.11 & 0.08 & 0.04 & 0.03 & 0.06 & 0.03 & 0.03 & 0.03 & 0.05 & 0.02 & 0.04 & 0.02 & 0.02 & 0.05 \\
3456 & KOI-4713 & 42 & 0.08 & 0.03 & 0.7 & 0.07 & 0.19 & 0.14 & 0.08 & 0.05 & 0.10 & 0.05 & 0.06 & 0.05 & 0.08 & 0.04 & 0.07 & 0.04 & 0.04 & 0.09 \\
3457 & KOI-4411 & 27 & 0.05 & 0.01 & 0.5 & 0.03 & 0.08 & 0.06 & 0.03 & 0.02 & 0.04 & 0.02 & 0.02 & 0.02 & 0.04 & 0.02 & 0.03 & 0.02 & 0.02 & 0.04 \\
3458 & KOI-3239 & 27 & 0.05 & 0.01 & 0.5 & 0.03 & 0.08 & 0.06 & 0.03 & 0.02 & 0.04 & 0.02 & 0.02 & 0.02 & 0.04 & 0.02 & 0.03 & 0.02 & 0.02 & 0.04 \\
3459 & KOI-2711 & 28 & 0.05 & 0.01 & 0.5 & 0.04 & 0.08 & 0.06 & 0.03 & 0.02 & 0.04 & 0.02 & 0.03 & 0.02 & 0.04 & 0.02 & 0.03 & 0.02 & 0.02 & 0.04 \\
3460 & KOI-1589 & 33 & 0.06 & 0.02 & 0.6 & 0.05 & 0.13 & 0.09 & 0.05 & 0.03 & 0.07 & 0.04 & 0.04 & 0.03 & 0.06 & 0.03 & 0.05 & 0.02 & 0.03 & 0.06 \\
3461 & KOI-408 & 32 & 0.06 & 0.02 & 0.6 & 0.05 & 0.12 & 0.09 & 0.05 & 0.03 & 0.06 & 0.03 & 0.04 & 0.03 & 0.06 & 0.03 & 0.04 & 0.02 & 0.03 & 0.06 \\
3462 & KOI-644 & 29 & 0.06 & 0.02 & 0.6 & 0.04 & 0.10 & 0.07 & 0.04 & 0.03 & 0.05 & 0.03 & 0.03 & 0.03 & 0.05 & 0.02 & 0.04 & 0.02 & 0.02 & 0.05 \\
3463 & KOI-2370 & 28 & 0.05 & 0.01 & 0.5 & 0.03 & 0.08 & 0.06 & 0.03 & 0.02 & 0.04 & 0.02 & 0.03 & 0.02 & 0.04 & 0.02 & 0.03 & 0.02 & 0.02 & 0.04 \\
3464 & KOI-2555 & 27 & 0.05 & 0.01 & 0.5 & 0.03 & 0.08 & 0.06 & 0.03 & 0.02 & 0.04 & 0.02 & 0.03 & 0.02 & 0.04 & 0.02 & 0.03 & 0.02 & 0.02 & 0.04 \\
3465 & KOI-2011 & 27 & 0.05 & 0.01 & 0.5 & 0.03 & 0.08 & 0.06 & 0.03 & 0.02 & 0.04 & 0.02 & 0.02 & 0.02 & 0.04 & 0.02 & 0.03 & 0.02 & 0.02 & 0.04 \\
3466 & KOI-2219 & 28 & 0.05 & 0.01 & 0.5 & 0.03 & 0.08 & 0.06 & 0.03 & 0.02 & 0.04 & 0.02 & 0.03 & 0.02 & 0.04 & 0.02 & 0.03 & 0.02 & 0.02 & 0.04 \\
3467 & KOI-1825 & 29 & 0.06 & 0.02 & 0.6 & 0.04 & 0.09 & 0.07 & 0.04 & 0.02 & 0.05 & 0.02 & 0.03 & 0.02 & 0.05 & 0.02 & 0.03 & 0.02 & 0.02 & 0.05 \\
3468 & KOI-2440 & 27 & 0.05 & 0.01 & 0.5 & 0.03 & 0.08 & 0.06 & 0.03 & 0.02 & 0.04 & 0.02 & 0.02 & 0.02 & 0.04 & 0.02 & 0.03 & 0.02 & 0.02 & 0.04 \\
3469 & KOI-1557 & 32 & 0.06 & 0.02 & 0.6 & 0.05 & 0.12 & 0.09 & 0.05 & 0.03 & 0.06 & 0.03 & 0.04 & 0.03 & 0.06 & 0.03 & 0.04 & 0.02 & 0.03 & 0.06 \\
3470 & KOI-829 & 32 & 0.06 & 0.02 & 0.6 & 0.05 & 0.12 & 0.09 & 0.05 & 0.03 & 0.06 & 0.03 & 0.04 & 0.03 & 0.06 & 0.02 & 0.04 & 0.02 & 0.03 & 0.06 \\
3471 & KOI-2556 & 28 & 0.06 & 0.02 & 0.5 & 0.04 & 0.09 & 0.06 & 0.03 & 0.02 & 0.05 & 0.02 & 0.03 & 0.02 & 0.05 & 0.02 & 0.03 & 0.02 & 0.02 & 0.04 \\
3472 & KOI-2690 & 27 & 0.05 & 0.01 & 0.5 & 0.03 & 0.07 & 0.06 & 0.03 & 0.02 & 0.04 & 0.02 & 0.02 & 0.02 & 0.04 & 0.02 & 0.03 & 0.02 & 0.02 & 0.04 \\
3473 & KOI-645 & 27 & 0.05 & 0.01 & 0.5 & 0.03 & 0.08 & 0.06 & 0.03 & 0.02 & 0.04 & 0.02 & 0.03 & 0.02 & 0.04 & 0.02 & 0.03 & 0.02 & 0.02 & 0.04 \\
3474 & KOI-3039 & 27 & 0.05 & 0.01 & 0.5 & 0.03 & 0.08 & 0.06 & 0.03 & 0.02 & 0.04 & 0.02 & 0.02 & 0.02 & 0.04 & 0.02 & 0.03 & 0.02 & 0.02 & 0.04 \\
3475 & KOI-1567 & 33 & 0.06 & 0.02 & 0.6 & 0.05 & 0.12 & 0.09 & 0.05 & 0.03 & 0.06 & 0.03 & 0.04 & 0.03 & 0.06 & 0.03 & 0.04 & 0.02 & 0.03 & 0.06 \\
3476 & KOI-4907 & 28 & 0.05 & 0.01 & 0.5 & 0.04 & 0.08 & 0.06 & 0.03 & 0.02 & 0.04 & 0.02 & 0.03 & 0.02 & 0.04 & 0.02 & 0.03 & 0.02 & 0.02 & 0.04 \\
3477 & KOI-834 & 33 & 0.06 & 0.02 & 0.6 & 0.05 & 0.13 & 0.10 & 0.05 & 0.03 & 0.07 & 0.04 & 0.04 & 0.03 & 0.06 & 0.03 & 0.05 & 0.03 & 0.03 & 0.06 \\
3478 & KOI-3791 & 27 & 0.05 & 0.01 & 0.5 & 0.03 & 0.08 & 0.06 & 0.03 & 0.02 & 0.04 & 0.02 & 0.02 & 0.02 & 0.04 & 0.02 & 0.03 & 0.02 & 0.02 & 0.04 \\
3479 & KOI-1601 & 29 & 0.06 & 0.02 & 0.6 & 0.04 & 0.10 & 0.07 & 0.04 & 0.02 & 0.05 & 0.03 & 0.03 & 0.02 & 0.05 & 0.02 & 0.04 & 0.02 & 0.02 & 0.05 \\
3480 & KOI-2970 & 27 & 0.05 & 0.01 & 0.5 & 0.03 & 0.08 & 0.06 & 0.03 & 0.02 & 0.04 & 0.02 & 0.03 & 0.02 & 0.04 & 0.02 & 0.03 & 0.02 & 0.02 & 0.04 \\
3481 & KOI-142 & 26 & 0.05 & 0.01 & 0.5 & 0.03 & 0.06 & 0.05 & 0.02 & 0.02 & 0.04 & 0.01 & 0.02 & 0.02 & 0.04 & 0.02 & 0.02 & 0.01 & 0.02 & 0.04 \\
3482 & KOI-2707 & 29 & 0.06 & 0.02 & 0.6 & 0.04 & 0.10 & 0.07 & 0.04 & 0.02 & 0.05 & 0.03 & 0.03 & 0.02 & 0.05 & 0.02 & 0.04 & 0.02 & 0.02 & 0.05 \\
3483 & Kepler-399 & 27 & 0.05 & 0.01 & 0.5 & 0.03 & 0.07 & 0.05 & 0.03 & 0.02 & 0.04 & 0.02 & 0.02 & 0.02 & 0.04 & 0.02 & 0.03 & 0.01 & 0.02 & 0.04 \\
3484 & KOI-4368 & 27 & 0.05 & 0.01 & 0.5 & 0.03 & 0.08 & 0.06 & 0.03 & 0.02 & 0.04 & 0.02 & 0.02 & 0.02 & 0.04 & 0.02 & 0.03 & 0.02 & 0.02 & 0.04 \\
3485 & KOI-409 & 28 & 0.05 & 0.02 & 0.5 & 0.04 & 0.08 & 0.06 & 0.03 & 0.02 & 0.05 & 0.02 & 0.03 & 0.02 & 0.04 & 0.02 & 0.03 & 0.02 & 0.02 & 0.04 \\
3486 & KOI-647 & 27 & 0.05 & 0.01 & 0.5 & 0.03 & 0.08 & 0.06 & 0.03 & 0.02 & 0.04 & 0.02 & 0.02 & 0.02 & 0.04 & 0.02 & 0.03 & 0.02 & 0.02 & 0.04 \\
3487 & KOI-2741 & 27 & 0.05 & 0.01 & 0.5 & 0.03 & 0.08 & 0.06 & 0.03 & 0.02 & 0.04 & 0.02 & 0.02 & 0.02 & 0.04 & 0.02 & 0.03 & 0.02 & 0.02 & 0.04 \\
3488 & KOI-257 & 27 & 0.05 & 0.01 & 0.5 & 0.03 & 0.08 & 0.06 & 0.03 & 0.02 & 0.04 & 0.02 & 0.02 & 0.02 & 0.04 & 0.02 & 0.03 & 0.02 & 0.02 & 0.04 \\
3489 & KOI-1590 & 35 & 0.06 & 0.02 & 0.6 & 0.05 & 0.14 & 0.10 & 0.05 & 0.03 & 0.07 & 0.04 & 0.04 & 0.03 & 0.06 & 0.03 & 0.05 & 0.03 & 0.03 & 0.06 \\
3490 & KOI-2854 E & 28 & 0.05 & 0.01 & 0.5 & 0.04 & 0.08 & 0.06 & 0.03 & 0.02 & 0.04 & 0.02 & 0.03 & 0.02 & 0.04 & 0.02 & 0.03 & 0.02 & 0.02 & 0.04 \\
3491 & KOI-2854 W & 27 & 0.05 & 0.01 & 0.5 & 0.03 & 0.07 & 0.06 & 0.03 & 0.02 & 0.04 & 0.02 & 0.02 & 0.02 & 0.04 & 0.02 & 0.03 & 0.01 & 0.02 & 0.04 \\
3492 & KOI-2668 & 27 & 0.05 & 0.01 & 0.5 & 0.03 & 0.08 & 0.06 & 0.03 & 0.02 & 0.04 & 0.02 & 0.02 & 0.02 & 0.04 & 0.02 & 0.03 & 0.02 & 0.02 & 0.04 \\
3493 & KOI-837 & 32 & 0.06 & 0.02 & 0.6 & 0.05 & 0.12 & 0.09 & 0.05 & 0.03 & 0.06 & 0.03 & 0.04 & 0.03 & 0.06 & 0.03 & 0.04 & 0.02 & 0.03 & 0.06 \\
3494 & KOI-1621 & 27 & 0.05 & 0.01 & 0.5 & 0.03 & 0.08 & 0.06 & 0.03 & 0.02 & 0.04 & 0.02 & 0.02 & 0.02 & 0.04 & 0.02 & 0.03 & 0.02 & 0.02 & 0.04 \\
3495 & KOI-4067 & 27 & 0.05 & 0.01 & 0.5 & 0.03 & 0.08 & 0.06 & 0.03 & 0.02 & 0.04 & 0.02 & 0.03 & 0.02 & 0.04 & 0.02 & 0.03 & 0.02 & 0.02 & 0.04 \\
3496 & Kepler-338 & 25 & 0.05 & 0.01 & 0.5 & 0.03 & 0.06 & 0.04 & 0.02 & 0.02 & 0.03 & 0.01 & 0.02 & 0.02 & 0.04 & 0.02 & 0.02 & 0.01 & 0.01 & 0.03 \\
3497 & KOI-1930 & 27 & 0.05 & 0.01 & 0.5 & 0.03 & 0.08 & 0.06 & 0.03 & 0.02 & 0.04 & 0.02 & 0.02 & 0.02 & 0.04 & 0.02 & 0.03 & 0.02 & 0.02 & 0.04 \\
3498 & KOI-2332 & 27 & 0.05 & 0.01 & 0.5 & 0.03 & 0.08 & 0.06 & 0.03 & 0.02 & 0.04 & 0.02 & 0.02 & 0.02 & 0.04 & 0.02 & 0.03 & 0.02 & 0.02 & 0.04 \\
3499 & KOI-1962 & 27 & 0.05 & 0.01 & 0.5 & 0.03 & 0.08 & 0.06 & 0.03 & 0.02 & 0.04 & 0.02 & 0.02 & 0.02 & 0.04 & 0.02 & 0.03 & 0.02 & 0.02 & 0.04 \\
3500 & KOI-649 & 27 & 0.05 & 0.01 & 0.5 & 0.03 & 0.08 & 0.06 & 0.03 & 0.02 & 0.04 & 0.02 & 0.02 & 0.02 & 0.04 & 0.02 & 0.03 & 0.02 & 0.02 & 0.04 \\
3501 & KOI-2915 & 27 & 0.05 & 0.01 & 0.5 & 0.03 & 0.08 & 0.06 & 0.03 & 0.02 & 0.04 & 0.02 & 0.02 & 0.02 & 0.04 & 0.02 & 0.03 & 0.02 & 0.02 & 0.04 \\
3502 & KOI-2790 & 27 & 0.05 & 0.01 & 0.5 & 0.03 & 0.07 & 0.06 & 0.03 & 0.02 & 0.04 & 0.02 & 0.02 & 0.02 & 0.04 & 0.02 & 0.03 & 0.02 & 0.02 & 0.04 \\
3503 & KOI-371 & 29 & 0.06 & 0.02 & 0.5 & 0.04 & 0.09 & 0.07 & 0.04 & 0.02 & 0.05 & 0.02 & 0.03 & 0.02 & 0.05 & 0.02 & 0.03 & 0.02 & 0.02 & 0.05 \\
3504 & KOI-2369 & 32 & 0.06 & 0.02 & 0.6 & 0.05 & 0.12 & 0.09 & 0.05 & 0.03 & 0.06 & 0.03 & 0.04 & 0.03 & 0.06 & 0.03 & 0.04 & 0.02 & 0.03 & 0.06 \\
3505 & KOI-2676 & 27 & 0.05 & 0.01 & 0.5 & 0.03 & 0.08 & 0.06 & 0.03 & 0.02 & 0.04 & 0.02 & 0.03 & 0.02 & 0.04 & 0.02 & 0.03 & 0.02 & 0.02 & 0.04 \\
3506 & KOI-2010 & 28 & 0.05 & 0.01 & 0.5 & 0.03 & 0.08 & 0.06 & 0.03 & 0.02 & 0.04 & 0.02 & 0.03 & 0.02 & 0.04 & 0.02 & 0.03 & 0.02 & 0.02 & 0.04 \\
3507 & KOI-2752 & 27 & 0.05 & 0.01 & 0.5 & 0.03 & 0.08 & 0.06 & 0.03 & 0.02 & 0.04 & 0.02 & 0.02 & 0.02 & 0.04 & 0.02 & 0.03 & 0.02 & 0.02 & 0.04 \\
3508 & KOI-2183 & 30 & 0.06 & 0.02 & 0.6 & 0.04 & 0.10 & 0.08 & 0.04 & 0.03 & 0.05 & 0.03 & 0.03 & 0.03 & 0.05 & 0.02 & 0.04 & 0.02 & 0.02 & 0.05 \\
3509 & KOI-505 & 28 & 0.05 & 0.01 & 0.5 & 0.04 & 0.08 & 0.06 & 0.03 & 0.02 & 0.04 & 0.02 & 0.03 & 0.02 & 0.04 & 0.02 & 0.03 & 0.02 & 0.02 & 0.04 \\
3510 & Kepler-169 & 27 & 0.05 & 0.01 & 0.5 & 0.03 & 0.07 & 0.06 & 0.03 & 0.02 & 0.04 & 0.02 & 0.02 & 0.02 & 0.04 & 0.02 & 0.03 & 0.02 & 0.02 & 0.04 \\
3511 & KOI-555 & 27 & 0.05 & 0.01 & 0.5 & 0.03 & 0.08 & 0.06 & 0.03 & 0.02 & 0.04 & 0.02 & 0.02 & 0.02 & 0.04 & 0.02 & 0.03 & 0.02 & 0.02 & 0.04 \\
3512 & KOI-4744 & 29 & 0.06 & 0.02 & 0.5 & 0.04 & 0.09 & 0.07 & 0.04 & 0.02 & 0.05 & 0.02 & 0.03 & 0.02 & 0.05 & 0.02 & 0.03 & 0.02 & 0.02 & 0.05 \\
3513 & KOI-2358 & 27 & 0.05 & 0.01 & 0.5 & 0.03 & 0.08 & 0.06 & 0.03 & 0.02 & 0.04 & 0.02 & 0.03 & 0.02 & 0.04 & 0.02 & 0.03 & 0.02 & 0.02 & 0.04 \\
3514 & KOI-1897 & 27 & 0.05 & 0.01 & 0.5 & 0.03 & 0.08 & 0.06 & 0.03 & 0.02 & 0.04 & 0.02 & 0.03 & 0.02 & 0.04 & 0.02 & 0.03 & 0.02 & 0.02 & 0.04 \\
3515 & KOI-2675 & 27 & 0.05 & 0.01 & 0.5 & 0.03 & 0.08 & 0.06 & 0.03 & 0.02 & 0.04 & 0.02 & 0.02 & 0.02 & 0.04 & 0.02 & 0.03 & 0.02 & 0.02 & 0.04 \\
3516 & KOI-3288 & 27 & 0.05 & 0.01 & 0.5 & 0.03 & 0.08 & 0.06 & 0.03 & 0.02 & 0.04 & 0.02 & 0.02 & 0.02 & 0.04 & 0.02 & 0.03 & 0.02 & 0.02 & 0.04 \\
3517 & KOI-650 & 27 & 0.05 & 0.01 & 0.5 & 0.03 & 0.07 & 0.06 & 0.03 & 0.02 & 0.04 & 0.02 & 0.02 & 0.02 & 0.04 & 0.02 & 0.03 & 0.02 & 0.02 & 0.04 \\
3518 & KOI-1928 & 27 & 0.05 & 0.01 & 0.5 & 0.03 & 0.08 & 0.06 & 0.03 & 0.02 & 0.04 & 0.02 & 0.02 & 0.02 & 0.04 & 0.02 & 0.03 & 0.02 & 0.02 & 0.04 \\
3519 & KOI-4686 & 27 & 0.05 & 0.01 & 0.5 & 0.03 & 0.07 & 0.06 & 0.03 & 0.02 & 0.04 & 0.02 & 0.02 & 0.02 & 0.04 & 0.02 & 0.03 & 0.02 & 0.02 & 0.04 \\
3520 & KOI-4002 & 31 & 0.06 & 0.02 & 0.6 & 0.04 & 0.11 & 0.08 & 0.04 & 0.03 & 0.06 & 0.03 & 0.03 & 0.03 & 0.05 & 0.02 & 0.04 & 0.02 & 0.03 & 0.05 \\
3521 & KOI-652 & 27 & 0.05 & 0.01 & 0.5 & 0.03 & 0.07 & 0.06 & 0.03 & 0.02 & 0.04 & 0.02 & 0.02 & 0.02 & 0.04 & 0.02 & 0.03 & 0.01 & 0.02 & 0.04 \\
3522 & KOI-4913 & 28 & 0.05 & 0.01 & 0.5 & 0.03 & 0.08 & 0.06 & 0.03 & 0.02 & 0.04 & 0.02 & 0.03 & 0.02 & 0.04 & 0.02 & 0.03 & 0.02 & 0.02 & 0.04 \\
3523 & KOI-3422 & 27 & 0.05 & 0.01 & 0.5 & 0.03 & 0.08 & 0.06 & 0.03 & 0.02 & 0.04 & 0.02 & 0.02 & 0.02 & 0.04 & 0.02 & 0.03 & 0.02 & 0.02 & 0.04 \\
3524 & KOI-4156 & 28 & 0.05 & 0.01 & 0.5 & 0.03 & 0.08 & 0.06 & 0.03 & 0.02 & 0.04 & 0.02 & 0.03 & 0.02 & 0.04 & 0.02 & 0.03 & 0.02 & 0.02 & 0.04 \\
3525 & KOI-1060 & 34 & 0.06 & 0.02 & 0.6 & 0.05 & 0.13 & 0.10 & 0.05 & 0.03 & 0.07 & 0.04 & 0.04 & 0.03 & 0.06 & 0.03 & 0.05 & 0.03 & 0.03 & 0.06 \\
3526 & Kepler-758 & 26 & 0.05 & 0.01 & 0.5 & 0.03 & 0.07 & 0.05 & 0.03 & 0.02 & 0.04 & 0.02 & 0.02 & 0.02 & 0.04 & 0.02 & 0.03 & 0.01 & 0.02 & 0.04 \\
3527 & KOI-2801 & 27 & 0.05 & 0.01 & 0.5 & 0.03 & 0.08 & 0.06 & 0.03 & 0.02 & 0.04 & 0.02 & 0.02 & 0.02 & 0.04 & 0.02 & 0.03 & 0.02 & 0.02 & 0.04 \\
3528 & KOI-1839 & 27 & 0.05 & 0.01 & 0.5 & 0.03 & 0.08 & 0.06 & 0.03 & 0.02 & 0.04 & 0.02 & 0.03 & 0.02 & 0.04 & 0.02 & 0.03 & 0.02 & 0.02 & 0.04 \\
3529 & KOI-2498 & 27 & 0.05 & 0.01 & 0.5 & 0.03 & 0.08 & 0.06 & 0.03 & 0.02 & 0.04 & 0.02 & 0.02 & 0.02 & 0.04 & 0.02 & 0.03 & 0.02 & 0.02 & 0.04 \\
3530 & KOI-4633 & 29 & 0.06 & 0.02 & 0.6 & 0.04 & 0.09 & 0.07 & 0.04 & 0.02 & 0.05 & 0.02 & 0.03 & 0.02 & 0.05 & 0.02 & 0.03 & 0.02 & 0.02 & 0.05 \\
3531 & KOI-654 & 27 & 0.05 & 0.01 & 0.5 & 0.03 & 0.08 & 0.06 & 0.03 & 0.02 & 0.04 & 0.02 & 0.02 & 0.02 & 0.04 & 0.02 & 0.03 & 0.02 & 0.02 & 0.04 \\
3532 & KOI-1052 & 33 & 0.06 & 0.02 & 0.6 & 0.05 & 0.13 & 0.09 & 0.05 & 0.03 & 0.07 & 0.03 & 0.04 & 0.03 & 0.06 & 0.03 & 0.05 & 0.02 & 0.03 & 0.06 \\
3533 & KOI-3190 & 28 & 0.05 & 0.01 & 0.5 & 0.03 & 0.08 & 0.06 & 0.03 & 0.02 & 0.04 & 0.02 & 0.03 & 0.02 & 0.04 & 0.02 & 0.03 & 0.02 & 0.02 & 0.04 \\
3534 & KOI-655 & 27 & 0.05 & 0.01 & 0.5 & 0.03 & 0.08 & 0.06 & 0.03 & 0.02 & 0.04 & 0.02 & 0.03 & 0.02 & 0.04 & 0.02 & 0.03 & 0.02 & 0.02 & 0.04 \\
3535 & KOI-2479 & 27 & 0.05 & 0.01 & 0.5 & 0.03 & 0.08 & 0.06 & 0.03 & 0.02 & 0.04 & 0.02 & 0.02 & 0.02 & 0.04 & 0.02 & 0.03 & 0.02 & 0.02 & 0.04 \\
3536 & KOI-2250 & 32 & 0.06 & 0.02 & 0.6 & 0.05 & 0.12 & 0.09 & 0.05 & 0.03 & 0.06 & 0.03 & 0.04 & 0.03 & 0.06 & 0.02 & 0.04 & 0.02 & 0.03 & 0.06 \\
3537 & KOI-303 & 27 & 0.05 & 0.01 & 0.5 & 0.03 & 0.08 & 0.06 & 0.03 & 0.02 & 0.04 & 0.02 & 0.02 & 0.02 & 0.04 & 0.02 & 0.03 & 0.02 & 0.02 & 0.04 \\
3538 & KOI-2733 & 27 & 0.05 & 0.01 & 0.5 & 0.03 & 0.08 & 0.06 & 0.03 & 0.02 & 0.04 & 0.02 & 0.03 & 0.02 & 0.04 & 0.02 & 0.03 & 0.02 & 0.02 & 0.04 \\
3539 & KOI-2148 & 27 & 0.05 & 0.01 & 0.5 & 0.03 & 0.08 & 0.06 & 0.03 & 0.02 & 0.04 & 0.02 & 0.02 & 0.02 & 0.04 & 0.02 & 0.03 & 0.02 & 0.02 & 0.04 \\
3540 & Kepler-363 & 25 & 0.05 & 0.01 & 0.5 & 0.03 & 0.06 & 0.04 & 0.02 & 0.02 & 0.03 & 0.01 & 0.02 & 0.02 & 0.04 & 0.02 & 0.02 & 0.01 & 0.01 & 0.03 \\
3541 & KOI-1054 & 27 & 0.05 & 0.01 & 0.5 & 0.03 & 0.08 & 0.06 & 0.03 & 0.02 & 0.04 & 0.02 & 0.02 & 0.02 & 0.04 & 0.02 & 0.03 & 0.02 & 0.02 & 0.04 \\
3542 & KOI-2167 & 30 & 0.06 & 0.02 & 0.6 & 0.04 & 0.10 & 0.08 & 0.04 & 0.03 & 0.05 & 0.03 & 0.03 & 0.03 & 0.05 & 0.02 & 0.04 & 0.02 & 0.02 & 0.05 \\
3543 & KOI-2071 & 28 & 0.05 & 0.01 & 0.5 & 0.04 & 0.08 & 0.06 & 0.03 & 0.02 & 0.04 & 0.02 & 0.03 & 0.02 & 0.04 & 0.02 & 0.03 & 0.02 & 0.02 & 0.04 \\
3544 & KOI-1684 & 27 & 0.05 & 0.01 & 0.5 & 0.03 & 0.08 & 0.06 & 0.03 & 0.02 & 0.04 & 0.02 & 0.02 & 0.02 & 0.04 & 0.02 & 0.03 & 0.02 & 0.02 & 0.04 \\
3545 & KOI-1916 & 27 & 0.05 & 0.01 & 0.5 & 0.03 & 0.08 & 0.06 & 0.03 & 0.02 & 0.04 & 0.02 & 0.02 & 0.02 & 0.04 & 0.02 & 0.03 & 0.02 & 0.02 & 0.04 \\
3546 & Kepler-336 & 26 & 0.05 & 0.01 & 0.5 & 0.03 & 0.06 & 0.05 & 0.02 & 0.02 & 0.04 & 0.02 & 0.02 & 0.02 & 0.04 & 0.02 & 0.03 & 0.01 & 0.02 & 0.04 \\
3547 & KOI-2949 & 27 & 0.05 & 0.01 & 0.5 & 0.03 & 0.08 & 0.06 & 0.03 & 0.02 & 0.04 & 0.02 & 0.02 & 0.02 & 0.04 & 0.02 & 0.03 & 0.02 & 0.02 & 0.04 \\
3548 & KOI-3500 & 27 & 0.05 & 0.01 & 0.5 & 0.03 & 0.08 & 0.06 & 0.03 & 0.02 & 0.04 & 0.02 & 0.02 & 0.02 & 0.04 & 0.02 & 0.03 & 0.02 & 0.02 & 0.04 \\
3549 & Kepler-132 & 25 & 0.05 & 0.01 & 0.5 & 0.03 & 0.06 & 0.05 & 0.02 & 0.02 & 0.03 & 0.01 & 0.02 & 0.02 & 0.04 & 0.02 & 0.02 & 0.01 & 0.01 & 0.03 \\
3550 & KOI-284 & 28 & 0.05 & 0.02 & 0.5 & 0.04 & 0.08 & 0.06 & 0.03 & 0.02 & 0.05 & 0.02 & 0.03 & 0.02 & 0.05 & 0.02 & 0.03 & 0.02 & 0.02 & 0.04 \\
3551 & KOI-4276 & 27 & 0.05 & 0.01 & 0.5 & 0.03 & 0.08 & 0.06 & 0.03 & 0.02 & 0.04 & 0.02 & 0.02 & 0.02 & 0.04 & 0.02 & 0.03 & 0.02 & 0.02 & 0.04 \\
3552 & KOI-304 & 27 & 0.05 & 0.01 & 0.5 & 0.03 & 0.08 & 0.06 & 0.03 & 0.02 & 0.04 & 0.02 & 0.02 & 0.02 & 0.04 & 0.02 & 0.03 & 0.02 & 0.02 & 0.04 \\
3553 & KOI-2001 & 27 & 0.05 & 0.01 & 0.5 & 0.03 & 0.08 & 0.06 & 0.03 & 0.02 & 0.04 & 0.02 & 0.02 & 0.02 & 0.04 & 0.02 & 0.03 & 0.02 & 0.02 & 0.04 \\
3554 & KOI-306 & 27 & 0.05 & 0.01 & 0.5 & 0.03 & 0.07 & 0.06 & 0.03 & 0.02 & 0.04 & 0.02 & 0.02 & 0.02 & 0.04 & 0.02 & 0.03 & 0.02 & 0.02 & 0.04 \\
3555 & Kepler-203 & 26 & 0.05 & 0.01 & 0.5 & 0.03 & 0.06 & 0.05 & 0.02 & 0.02 & 0.04 & 0.02 & 0.02 & 0.02 & 0.04 & 0.02 & 0.03 & 0.01 & 0.02 & 0.04 \\
3556 & KOI-659 & 28 & 0.05 & 0.01 & 0.5 & 0.03 & 0.08 & 0.06 & 0.03 & 0.02 & 0.04 & 0.02 & 0.03 & 0.02 & 0.04 & 0.02 & 0.03 & 0.02 & 0.02 & 0.04 \\
3557 & KOI-2098 & 28 & 0.06 & 0.02 & 0.5 & 0.04 & 0.09 & 0.07 & 0.03 & 0.02 & 0.05 & 0.02 & 0.03 & 0.02 & 0.05 & 0.02 & 0.03 & 0.02 & 0.02 & 0.05 \\
3558 & KOI-3179 & 27 & 0.05 & 0.01 & 0.5 & 0.03 & 0.08 & 0.06 & 0.03 & 0.02 & 0.04 & 0.02 & 0.02 & 0.02 & 0.04 & 0.02 & 0.03 & 0.02 & 0.02 & 0.04 \\
3559 & KOI-4123 & 28 & 0.05 & 0.01 & 0.5 & 0.04 & 0.08 & 0.06 & 0.03 & 0.02 & 0.04 & 0.02 & 0.03 & 0.02 & 0.04 & 0.02 & 0.03 & 0.02 & 0.02 & 0.04 \\
3560 & KOI-2398 & 27 & 0.05 & 0.01 & 0.5 & 0.03 & 0.08 & 0.06 & 0.03 & 0.02 & 0.04 & 0.02 & 0.03 & 0.02 & 0.04 & 0.02 & 0.03 & 0.02 & 0.02 & 0.04 \\
3561 & KOI-2829 & 27 & 0.05 & 0.01 & 0.5 & 0.03 & 0.08 & 0.06 & 0.03 & 0.02 & 0.04 & 0.02 & 0.02 & 0.02 & 0.04 & 0.02 & 0.03 & 0.02 & 0.02 & 0.04 \\
3562 & Kepler-92 & 25 & 0.05 & 0.01 & 0.5 & 0.03 & 0.04 & 0.04 & 0.01 & 0.01 & 0.03 & 0.01 & 0.01 & 0.01 & 0.03 & 0.01 & 0.02 & 0.01 & 0.01 & 0.03 \\
3563 & KOI-285 & 27 & 0.05 & 0.01 & 0.5 & 0.03 & 0.08 & 0.06 & 0.03 & 0.02 & 0.04 & 0.02 & 0.02 & 0.02 & 0.04 & 0.02 & 0.03 & 0.02 & 0.02 & 0.04 \\
3564 & KOI-2252 & 27 & 0.05 & 0.01 & 0.5 & 0.03 & 0.08 & 0.06 & 0.03 & 0.02 & 0.04 & 0.02 & 0.02 & 0.02 & 0.04 & 0.02 & 0.03 & 0.02 & 0.02 & 0.04 \\
3565 & KOI-3240 & 27 & 0.05 & 0.01 & 0.5 & 0.03 & 0.08 & 0.06 & 0.03 & 0.02 & 0.04 & 0.02 & 0.02 & 0.02 & 0.04 & 0.02 & 0.03 & 0.02 & 0.02 & 0.04 \\
3566 & KOI-2636 & 27 & 0.05 & 0.01 & 0.5 & 0.03 & 0.08 & 0.06 & 0.03 & 0.02 & 0.04 & 0.02 & 0.02 & 0.02 & 0.04 & 0.02 & 0.03 & 0.02 & 0.02 & 0.04 \\
3567 & KOI-1812 & 28 & 0.05 & 0.01 & 0.5 & 0.04 & 0.08 & 0.06 & 0.03 & 0.02 & 0.05 & 0.02 & 0.03 & 0.02 & 0.04 & 0.02 & 0.03 & 0.02 & 0.02 & 0.04 \\
3568 & KOI-308 & 27 & 0.05 & 0.01 & 0.5 & 0.03 & 0.08 & 0.06 & 0.03 & 0.02 & 0.04 & 0.02 & 0.03 & 0.02 & 0.04 & 0.02 & 0.03 & 0.02 & 0.02 & 0.04 \\
3569 & KOI-2608 & 27 & 0.05 & 0.01 & 0.5 & 0.03 & 0.08 & 0.06 & 0.03 & 0.02 & 0.04 & 0.02 & 0.02 & 0.02 & 0.04 & 0.02 & 0.03 & 0.02 & 0.02 & 0.04 \\
3570 & KOI-415 & 27 & 0.05 & 0.01 & 0.5 & 0.03 & 0.08 & 0.06 & 0.03 & 0.02 & 0.04 & 0.02 & 0.03 & 0.02 & 0.04 & 0.02 & 0.03 & 0.02 & 0.02 & 0.04 \\
3571 & KOI-4302 & 27 & 0.05 & 0.01 & 0.5 & 0.03 & 0.08 & 0.06 & 0.03 & 0.02 & 0.04 & 0.02 & 0.02 & 0.02 & 0.04 & 0.02 & 0.03 & 0.02 & 0.02 & 0.04 \\
3572 & KOI-1688 & 30 & 0.06 & 0.02 & 0.6 & 0.04 & 0.10 & 0.07 & 0.04 & 0.03 & 0.05 & 0.03 & 0.03 & 0.03 & 0.05 & 0.02 & 0.04 & 0.02 & 0.02 & 0.05 \\
3573 & KOI-660 & 27 & 0.05 & 0.01 & 0.5 & 0.03 & 0.08 & 0.06 & 0.03 & 0.02 & 0.04 & 0.02 & 0.02 & 0.02 & 0.04 & 0.02 & 0.03 & 0.02 & 0.02 & 0.04 \\
3574 & KOI-307 & 28 & 0.05 & 0.01 & 0.5 & 0.03 & 0.08 & 0.06 & 0.03 & 0.02 & 0.04 & 0.02 & 0.03 & 0.02 & 0.04 & 0.02 & 0.03 & 0.02 & 0.02 & 0.04 \\
3575 & KOI-1613 & 27 & 0.05 & 0.01 & 0.5 & 0.03 & 0.08 & 0.06 & 0.03 & 0.02 & 0.04 & 0.02 & 0.02 & 0.02 & 0.04 & 0.02 & 0.03 & 0.02 & 0.02 & 0.04 \\
3576 & KOI-3436 & 27 & 0.05 & 0.01 & 0.5 & 0.03 & 0.07 & 0.06 & 0.03 & 0.02 & 0.04 & 0.02 & 0.02 & 0.02 & 0.04 & 0.02 & 0.03 & 0.02 & 0.02 & 0.04 \\
3577 & KOI-219 & 27 & 0.05 & 0.01 & 0.5 & 0.03 & 0.08 & 0.06 & 0.03 & 0.02 & 0.04 & 0.02 & 0.02 & 0.02 & 0.04 & 0.02 & 0.03 & 0.02 & 0.02 & 0.04 \\
3578 & KOI-611 & 28 & 0.05 & 0.01 & 0.5 & 0.04 & 0.08 & 0.06 & 0.03 & 0.02 & 0.04 & 0.02 & 0.03 & 0.02 & 0.04 & 0.02 & 0.03 & 0.02 & 0.02 & 0.04 \\
3579 & KOI-2753 & 27 & 0.05 & 0.01 & 0.5 & 0.03 & 0.08 & 0.06 & 0.03 & 0.02 & 0.04 & 0.02 & 0.02 & 0.02 & 0.04 & 0.02 & 0.03 & 0.02 & 0.02 & 0.04 \\
3580 & KOI-1128 & 27 & 0.05 & 0.01 & 0.5 & 0.03 & 0.08 & 0.06 & 0.03 & 0.02 & 0.04 & 0.02 & 0.02 & 0.02 & 0.04 & 0.02 & 0.03 & 0.02 & 0.02 & 0.04 \\
3581 & KOI-662 & 27 & 0.05 & 0.01 & 0.5 & 0.03 & 0.08 & 0.06 & 0.03 & 0.02 & 0.04 & 0.02 & 0.02 & 0.02 & 0.04 & 0.02 & 0.03 & 0.02 & 0.02 & 0.04 \\
3582 & KOI-3503 & 28 & 0.05 & 0.01 & 0.5 & 0.03 & 0.08 & 0.06 & 0.03 & 0.02 & 0.04 & 0.02 & 0.03 & 0.02 & 0.04 & 0.02 & 0.03 & 0.02 & 0.02 & 0.04 \\
3583 & KOI-661 & 27 & 0.05 & 0.01 & 0.5 & 0.03 & 0.08 & 0.06 & 0.03 & 0.02 & 0.04 & 0.02 & 0.02 & 0.02 & 0.04 & 0.02 & 0.03 & 0.02 & 0.02 & 0.04 \\
3584 & KOI-1121 & 27 & 0.05 & 0.01 & 0.5 & 0.03 & 0.07 & 0.05 & 0.03 & 0.02 & 0.04 & 0.02 & 0.02 & 0.02 & 0.04 & 0.02 & 0.03 & 0.01 & 0.02 & 0.04 \\
3585 & KOI-1127 & 35 & 0.07 & 0.02 & 0.6 & 0.05 & 0.14 & 0.10 & 0.06 & 0.04 & 0.07 & 0.04 & 0.04 & 0.04 & 0.06 & 0.03 & 0.05 & 0.03 & 0.03 & 0.07 \\
3586 & KOI-2857 & 27 & 0.05 & 0.01 & 0.5 & 0.03 & 0.08 & 0.06 & 0.03 & 0.02 & 0.04 & 0.02 & 0.02 & 0.02 & 0.04 & 0.02 & 0.03 & 0.02 & 0.02 & 0.04 \\
3587 & KOI-2948 & 27 & 0.05 & 0.01 & 0.5 & 0.03 & 0.07 & 0.06 & 0.03 & 0.02 & 0.04 & 0.02 & 0.02 & 0.02 & 0.04 & 0.02 & 0.03 & 0.02 & 0.02 & 0.04 \\
3588 & KOI-3456 & 27 & 0.05 & 0.01 & 0.5 & 0.03 & 0.08 & 0.06 & 0.03 & 0.02 & 0.04 & 0.02 & 0.02 & 0.02 & 0.04 & 0.02 & 0.03 & 0.02 & 0.02 & 0.04 \\
3589 & KOI-1230 & 27 & 0.05 & 0.01 & 0.5 & 0.03 & 0.07 & 0.06 & 0.03 & 0.02 & 0.04 & 0.02 & 0.02 & 0.02 & 0.04 & 0.02 & 0.03 & 0.01 & 0.02 & 0.04 \\
3590 & KOI-2840 & 27 & 0.05 & 0.01 & 0.5 & 0.03 & 0.08 & 0.06 & 0.03 & 0.02 & 0.04 & 0.02 & 0.02 & 0.02 & 0.04 & 0.02 & 0.03 & 0.02 & 0.02 & 0.04 \\
3591 & Kepler-172 & 27 & 0.05 & 0.01 & 0.5 & 0.03 & 0.08 & 0.06 & 0.03 & 0.02 & 0.04 & 0.02 & 0.03 & 0.02 & 0.04 & 0.02 & 0.03 & 0.02 & 0.02 & 0.04 \\
3592 & KOI-664 & 27 & 0.05 & 0.01 & 0.5 & 0.03 & 0.08 & 0.06 & 0.03 & 0.02 & 0.04 & 0.02 & 0.02 & 0.02 & 0.04 & 0.02 & 0.03 & 0.02 & 0.02 & 0.04 \\
3593 & Kepler-206 & 26 & 0.05 & 0.01 & 0.5 & 0.03 & 0.06 & 0.05 & 0.02 & 0.02 & 0.04 & 0.01 & 0.02 & 0.02 & 0.04 & 0.02 & 0.02 & 0.01 & 0.02 & 0.04 \\
3594 & KOI-372 & 25 & 0.05 & 0.01 & 0.5 & 0.03 & 0.06 & 0.04 & 0.02 & 0.01 & 0.03 & 0.01 & 0.02 & 0.01 & 0.04 & 0.02 & 0.02 & 0.01 & 0.01 & 0.03 \\
3595 & KOI-1241 & 25 & 0.05 & 0.01 & 0.5 & 0.03 & 0.04 & 0.04 & 0.01 & 0.01 & 0.03 & 0.01 & 0.01 & 0.01 & 0.03 & 0.01 & 0.02 & 0.01 & 0.01 & 0.03 \\
3596 & KOI-2408 & 27 & 0.05 & 0.01 & 0.5 & 0.03 & 0.08 & 0.06 & 0.03 & 0.02 & 0.04 & 0.02 & 0.02 & 0.02 & 0.04 & 0.02 & 0.03 & 0.02 & 0.02 & 0.04 \\
3597 & KOI-511 & 29 & 0.06 & 0.02 & 0.6 & 0.04 & 0.10 & 0.07 & 0.04 & 0.02 & 0.05 & 0.03 & 0.03 & 0.02 & 0.05 & 0.02 & 0.04 & 0.02 & 0.02 & 0.05 \\
3598 & KOI-176 & 28 & 0.05 & 0.01 & 0.5 & 0.03 & 0.08 & 0.06 & 0.03 & 0.02 & 0.04 & 0.02 & 0.03 & 0.02 & 0.04 & 0.02 & 0.03 & 0.02 & 0.02 & 0.04 \\
3599 & KOI-94 & 26 & 0.05 & 0.01 & 0.5 & 0.03 & 0.07 & 0.05 & 0.02 & 0.02 & 0.04 & 0.02 & 0.02 & 0.02 & 0.04 & 0.02 & 0.03 & 0.01 & 0.02 & 0.04 \\
3600 & KOI-270 & 27 & 0.05 & 0.01 & 0.5 & 0.03 & 0.08 & 0.06 & 0.03 & 0.02 & 0.04 & 0.02 & 0.02 & 0.02 & 0.04 & 0.02 & 0.03 & 0.02 & 0.02 & 0.04 \\
3601 & KOI-3117 & 27 & 0.05 & 0.01 & 0.5 & 0.03 & 0.08 & 0.06 & 0.03 & 0.02 & 0.04 & 0.02 & 0.02 & 0.02 & 0.04 & 0.02 & 0.03 & 0.02 & 0.02 & 0.04 \\
3602 & KOI-4657 & 27 & 0.05 & 0.01 & 0.5 & 0.03 & 0.07 & 0.06 & 0.03 & 0.02 & 0.04 & 0.02 & 0.02 & 0.02 & 0.04 & 0.02 & 0.03 & 0.02 & 0.02 & 0.04 \\
3603 & KOI-3438 & 27 & 0.05 & 0.01 & 0.5 & 0.03 & 0.08 & 0.06 & 0.03 & 0.02 & 0.04 & 0.02 & 0.02 & 0.02 & 0.04 & 0.02 & 0.03 & 0.02 & 0.02 & 0.04 \\
3604 & KOI-1239 & 31 & 0.06 & 0.02 & 0.6 & 0.04 & 0.11 & 0.08 & 0.05 & 0.03 & 0.06 & 0.03 & 0.04 & 0.03 & 0.05 & 0.02 & 0.04 & 0.02 & 0.03 & 0.06 \\
3605 & KOI-3287 & 28 & 0.06 & 0.02 & 0.5 & 0.04 & 0.09 & 0.07 & 0.03 & 0.02 & 0.05 & 0.02 & 0.03 & 0.02 & 0.05 & 0.02 & 0.03 & 0.02 & 0.02 & 0.05 \\
3606 & KOI-857 & 29 & 0.06 & 0.02 & 0.6 & 0.04 & 0.10 & 0.07 & 0.04 & 0.02 & 0.05 & 0.03 & 0.03 & 0.02 & 0.05 & 0.02 & 0.04 & 0.02 & 0.02 & 0.05 \\
3607 & KOI-1242 & 28 & 0.05 & 0.01 & 0.5 & 0.03 & 0.08 & 0.06 & 0.03 & 0.02 & 0.04 & 0.02 & 0.03 & 0.02 & 0.04 & 0.02 & 0.03 & 0.02 & 0.02 & 0.04 \\
3608 & KOI-2559 & 28 & 0.05 & 0.01 & 0.5 & 0.04 & 0.08 & 0.06 & 0.03 & 0.02 & 0.05 & 0.02 & 0.03 & 0.02 & 0.04 & 0.02 & 0.03 & 0.02 & 0.02 & 0.04 \\
3609 & KOI-3237 & 27 & 0.05 & 0.01 & 0.5 & 0.03 & 0.08 & 0.06 & 0.03 & 0.02 & 0.04 & 0.02 & 0.02 & 0.02 & 0.04 & 0.02 & 0.03 & 0.02 & 0.02 & 0.04 \\
3610 & KOI-2838 & 27 & 0.05 & 0.01 & 0.5 & 0.03 & 0.08 & 0.06 & 0.03 & 0.02 & 0.04 & 0.02 & 0.02 & 0.02 & 0.04 & 0.02 & 0.03 & 0.02 & 0.02 & 0.04 \\
3611 & KOI-1227 & 27 & 0.05 & 0.01 & 0.5 & 0.03 & 0.08 & 0.06 & 0.03 & 0.02 & 0.04 & 0.02 & 0.03 & 0.02 & 0.04 & 0.02 & 0.03 & 0.02 & 0.02 & 0.04 \\
3612 & KOI-2737 & 27 & 0.05 & 0.01 & 0.5 & 0.03 & 0.08 & 0.06 & 0.03 & 0.02 & 0.04 & 0.02 & 0.02 & 0.02 & 0.04 & 0.02 & 0.03 & 0.02 & 0.02 & 0.04 \\
3613 & KOI-4159 & 30 & 0.06 & 0.02 & 0.6 & 0.04 & 0.10 & 0.07 & 0.04 & 0.03 & 0.05 & 0.03 & 0.03 & 0.03 & 0.05 & 0.02 & 0.04 & 0.02 & 0.02 & 0.05 \\
3614 & KOI-1692 & 27 & 0.05 & 0.01 & 0.5 & 0.03 & 0.07 & 0.06 & 0.03 & 0.02 & 0.04 & 0.02 & 0.02 & 0.02 & 0.04 & 0.02 & 0.03 & 0.01 & 0.02 & 0.04 \\
3615 & KOI-612 & 28 & 0.05 & 0.01 & 0.5 & 0.04 & 0.08 & 0.06 & 0.03 & 0.02 & 0.05 & 0.02 & 0.03 & 0.02 & 0.04 & 0.02 & 0.03 & 0.02 & 0.02 & 0.04 \\
3616 & KOI-666 & 27 & 0.05 & 0.01 & 0.5 & 0.03 & 0.08 & 0.06 & 0.03 & 0.02 & 0.04 & 0.02 & 0.02 & 0.02 & 0.04 & 0.02 & 0.03 & 0.02 & 0.02 & 0.04 \\
3617 & KOI-4651 & 30 & 0.06 & 0.02 & 0.6 & 0.04 & 0.10 & 0.07 & 0.04 & 0.03 & 0.05 & 0.03 & 0.03 & 0.03 & 0.05 & 0.02 & 0.04 & 0.02 & 0.02 & 0.05 \\
3618 & KOI-665 & 27 & 0.05 & 0.01 & 0.5 & 0.03 & 0.08 & 0.06 & 0.03 & 0.02 & 0.04 & 0.02 & 0.02 & 0.02 & 0.04 & 0.02 & 0.03 & 0.02 & 0.02 & 0.04 \\
3619 & Kepler-207 & 25 & 0.05 & 0.01 & 0.5 & 0.03 & 0.06 & 0.05 & 0.02 & 0.02 & 0.03 & 0.01 & 0.02 & 0.02 & 0.04 & 0.02 & 0.02 & 0.01 & 0.01 & 0.03 \\
3620 & KOI-561 & 27 & 0.05 & 0.01 & 0.5 & 0.03 & 0.07 & 0.06 & 0.03 & 0.02 & 0.04 & 0.02 & 0.02 & 0.02 & 0.04 & 0.02 & 0.03 & 0.02 & 0.02 & 0.04 \\
3621 & KOI-1240 & 30 & 0.06 & 0.02 & 0.6 & 0.04 & 0.10 & 0.07 & 0.04 & 0.03 & 0.05 & 0.03 & 0.03 & 0.03 & 0.05 & 0.02 & 0.04 & 0.02 & 0.02 & 0.05 \\
3622 & KOI-2092 & 32 & 0.06 & 0.02 & 0.6 & 0.05 & 0.12 & 0.09 & 0.05 & 0.03 & 0.06 & 0.03 & 0.04 & 0.03 & 0.06 & 0.03 & 0.04 & 0.02 & 0.03 & 0.06 \\
3623 & KOI-5324 & 30 & 0.06 & 0.02 & 0.6 & 0.04 & 0.10 & 0.07 & 0.04 & 0.03 & 0.05 & 0.03 & 0.03 & 0.03 & 0.05 & 0.02 & 0.04 & 0.02 & 0.02 & 0.05 \\
3624 & KOI-4072 & 27 & 0.05 & 0.01 & 0.5 & 0.03 & 0.08 & 0.06 & 0.03 & 0.02 & 0.04 & 0.02 & 0.03 & 0.02 & 0.04 & 0.02 & 0.03 & 0.02 & 0.02 & 0.04 \\
3625 & KOI-2678 & 28 & 0.05 & 0.01 & 0.5 & 0.04 & 0.08 & 0.06 & 0.03 & 0.02 & 0.05 & 0.02 & 0.03 & 0.02 & 0.04 & 0.02 & 0.03 & 0.02 & 0.02 & 0.04 \\
3626 & KOI-177 & 27 & 0.05 & 0.01 & 0.5 & 0.03 & 0.08 & 0.06 & 0.03 & 0.02 & 0.04 & 0.02 & 0.02 & 0.02 & 0.04 & 0.02 & 0.03 & 0.02 & 0.02 & 0.04 \\
3627 & KOI-1695 & 28 & 0.05 & 0.02 & 0.5 & 0.04 & 0.08 & 0.06 & 0.03 & 0.02 & 0.05 & 0.02 & 0.03 & 0.02 & 0.04 & 0.02 & 0.03 & 0.02 & 0.02 & 0.04 \\
3628 & KOI-3980 & 30 & 0.06 & 0.02 & 0.6 & 0.04 & 0.10 & 0.07 & 0.04 & 0.03 & 0.05 & 0.03 & 0.03 & 0.03 & 0.05 & 0.02 & 0.04 & 0.02 & 0.02 & 0.05 \\
3629 & KOI-1375 & 27 & 0.05 & 0.01 & 0.5 & 0.03 & 0.08 & 0.06 & 0.03 & 0.02 & 0.04 & 0.02 & 0.03 & 0.02 & 0.04 & 0.02 & 0.03 & 0.02 & 0.02 & 0.04 \\
3630 & KOI-4850 & 27 & 0.05 & 0.01 & 0.5 & 0.03 & 0.08 & 0.06 & 0.03 & 0.02 & 0.04 & 0.02 & 0.03 & 0.02 & 0.04 & 0.02 & 0.03 & 0.02 & 0.02 & 0.04 \\
3631 & KOI-2086 & 27 & 0.05 & 0.01 & 0.5 & 0.03 & 0.08 & 0.06 & 0.03 & 0.02 & 0.04 & 0.02 & 0.02 & 0.02 & 0.04 & 0.02 & 0.03 & 0.02 & 0.02 & 0.04 \\
3632 & Kepler-60 & 26 & 0.05 & 0.01 & 0.5 & 0.03 & 0.06 & 0.05 & 0.02 & 0.02 & 0.04 & 0.02 & 0.02 & 0.02 & 0.04 & 0.02 & 0.03 & 0.01 & 0.02 & 0.04 \\
3633 & KOI-4871 & 28 & 0.05 & 0.01 & 0.5 & 0.04 & 0.08 & 0.06 & 0.03 & 0.02 & 0.04 & 0.02 & 0.03 & 0.02 & 0.04 & 0.02 & 0.03 & 0.02 & 0.02 & 0.04 \\
3634 & KOI-4184 & 27 & 0.05 & 0.01 & 0.5 & 0.03 & 0.07 & 0.06 & 0.03 & 0.02 & 0.04 & 0.02 & 0.02 & 0.02 & 0.04 & 0.02 & 0.03 & 0.01 & 0.02 & 0.04 \\
3635 & KOI-864 & 32 & 0.06 & 0.02 & 0.6 & 0.05 & 0.12 & 0.09 & 0.05 & 0.03 & 0.06 & 0.03 & 0.04 & 0.03 & 0.06 & 0.02 & 0.04 & 0.02 & 0.03 & 0.06 \\
3636 & KOI-3244 & 27 & 0.05 & 0.01 & 0.5 & 0.03 & 0.07 & 0.06 & 0.03 & 0.02 & 0.04 & 0.02 & 0.02 & 0.02 & 0.04 & 0.02 & 0.03 & 0.01 & 0.02 & 0.04 \\
3637 & KOI-4188 & 30 & 0.06 & 0.02 & 0.6 & 0.04 & 0.10 & 0.08 & 0.04 & 0.03 & 0.05 & 0.03 & 0.03 & 0.03 & 0.05 & 0.02 & 0.04 & 0.02 & 0.02 & 0.05 \\
3638 & KOI-4674 & 28 & 0.05 & 0.01 & 0.5 & 0.03 & 0.08 & 0.06 & 0.03 & 0.02 & 0.04 & 0.02 & 0.03 & 0.02 & 0.04 & 0.02 & 0.03 & 0.02 & 0.02 & 0.04 \\
3639 & KOI-201 & 30 & 0.06 & 0.02 & 0.6 & 0.04 & 0.10 & 0.08 & 0.04 & 0.03 & 0.06 & 0.03 & 0.03 & 0.03 & 0.05 & 0.02 & 0.04 & 0.02 & 0.02 & 0.05 \\
3640 & KOI-2571 & 29 & 0.06 & 0.02 & 0.6 & 0.04 & 0.09 & 0.07 & 0.04 & 0.02 & 0.05 & 0.02 & 0.03 & 0.02 & 0.05 & 0.02 & 0.03 & 0.02 & 0.02 & 0.05 \\
3641 & KOI-163 & 27 & 0.05 & 0.01 & 0.5 & 0.03 & 0.07 & 0.06 & 0.03 & 0.02 & 0.04 & 0.02 & 0.02 & 0.02 & 0.04 & 0.02 & 0.03 & 0.02 & 0.02 & 0.04 \\
3642 & KOI-2220 & 30 & 0.06 & 0.02 & 0.6 & 0.04 & 0.10 & 0.07 & 0.04 & 0.03 & 0.05 & 0.03 & 0.03 & 0.03 & 0.05 & 0.02 & 0.04 & 0.02 & 0.02 & 0.05 \\
3643 & KOI-1366 & 30 & 0.06 & 0.02 & 0.6 & 0.04 & 0.10 & 0.08 & 0.04 & 0.03 & 0.05 & 0.03 & 0.03 & 0.03 & 0.05 & 0.02 & 0.04 & 0.02 & 0.02 & 0.05 \\
3644 & KOI-2925 & 27 & 0.05 & 0.01 & 0.5 & 0.03 & 0.07 & 0.06 & 0.03 & 0.02 & 0.04 & 0.02 & 0.02 & 0.02 & 0.04 & 0.02 & 0.03 & 0.02 & 0.02 & 0.04 \\
3645 & KOI-1363 & 33 & 0.06 & 0.02 & 0.6 & 0.05 & 0.12 & 0.09 & 0.05 & 0.03 & 0.06 & 0.03 & 0.04 & 0.03 & 0.06 & 0.03 & 0.04 & 0.02 & 0.03 & 0.06 \\
3646 & KOI-2087 & 27 & 0.05 & 0.01 & 0.5 & 0.03 & 0.08 & 0.06 & 0.03 & 0.02 & 0.04 & 0.02 & 0.03 & 0.02 & 0.04 & 0.02 & 0.03 & 0.02 & 0.02 & 0.04 \\
3647 & KOI-1628 & 27 & 0.05 & 0.01 & 0.5 & 0.03 & 0.08 & 0.06 & 0.03 & 0.02 & 0.04 & 0.02 & 0.02 & 0.02 & 0.04 & 0.02 & 0.03 & 0.02 & 0.02 & 0.04 \\
3648 & KOI-1367 & 29 & 0.06 & 0.02 & 0.6 & 0.04 & 0.09 & 0.07 & 0.04 & 0.02 & 0.05 & 0.02 & 0.03 & 0.02 & 0.05 & 0.02 & 0.03 & 0.02 & 0.02 & 0.05 \\
3649 & KOI-4382 & 28 & 0.05 & 0.01 & 0.5 & 0.03 & 0.08 & 0.06 & 0.03 & 0.02 & 0.04 & 0.02 & 0.03 & 0.02 & 0.04 & 0.02 & 0.03 & 0.02 & 0.02 & 0.04 \\
3650 & KOI-2879 & 27 & 0.05 & 0.01 & 0.5 & 0.03 & 0.08 & 0.06 & 0.03 & 0.02 & 0.04 & 0.02 & 0.02 & 0.02 & 0.04 & 0.02 & 0.03 & 0.02 & 0.02 & 0.04 \\
3651 & KOI-670 & 27 & 0.05 & 0.01 & 0.5 & 0.03 & 0.08 & 0.06 & 0.03 & 0.02 & 0.04 & 0.02 & 0.02 & 0.02 & 0.04 & 0.02 & 0.03 & 0.02 & 0.02 & 0.04 \\
3652 & KOI-671 & 27 & 0.05 & 0.01 & 0.5 & 0.03 & 0.07 & 0.06 & 0.03 & 0.02 & 0.04 & 0.02 & 0.02 & 0.02 & 0.04 & 0.02 & 0.03 & 0.01 & 0.02 & 0.04 \\
3653 & KOI-2215 & 27 & 0.05 & 0.01 & 0.5 & 0.03 & 0.08 & 0.06 & 0.03 & 0.02 & 0.04 & 0.02 & 0.02 & 0.02 & 0.04 & 0.02 & 0.03 & 0.02 & 0.02 & 0.04 \\
3654 & KOI-3689 & 28 & 0.06 & 0.02 & 0.5 & 0.04 & 0.09 & 0.07 & 0.03 & 0.02 & 0.05 & 0.02 & 0.03 & 0.02 & 0.05 & 0.02 & 0.03 & 0.02 & 0.02 & 0.04 \\
3655 & KOI-312 & 27 & 0.05 & 0.01 & 0.5 & 0.03 & 0.08 & 0.06 & 0.03 & 0.02 & 0.04 & 0.02 & 0.03 & 0.02 & 0.04 & 0.02 & 0.03 & 0.02 & 0.02 & 0.04 \\
3656 & KOI-872 & 31 & 0.06 & 0.02 & 0.6 & 0.04 & 0.11 & 0.08 & 0.04 & 0.03 & 0.06 & 0.03 & 0.03 & 0.03 & 0.05 & 0.02 & 0.04 & 0.02 & 0.02 & 0.05 \\
3657 & KOI-673 & 27 & 0.05 & 0.01 & 0.5 & 0.03 & 0.08 & 0.06 & 0.03 & 0.02 & 0.04 & 0.02 & 0.03 & 0.02 & 0.04 & 0.02 & 0.03 & 0.02 & 0.02 & 0.04 \\
3658 & KOI-672 & 27 & 0.05 & 0.01 & 0.5 & 0.03 & 0.08 & 0.06 & 0.03 & 0.02 & 0.04 & 0.02 & 0.02 & 0.02 & 0.04 & 0.02 & 0.03 & 0.02 & 0.02 & 0.04 \\
3659 & KOI-2083 & 27 & 0.05 & 0.01 & 0.5 & 0.03 & 0.08 & 0.06 & 0.03 & 0.02 & 0.04 & 0.02 & 0.02 & 0.02 & 0.04 & 0.02 & 0.03 & 0.02 & 0.02 & 0.04 \\
3660 & KOI-3907 & 27 & 0.05 & 0.01 & 0.5 & 0.03 & 0.08 & 0.06 & 0.03 & 0.02 & 0.04 & 0.02 & 0.02 & 0.02 & 0.04 & 0.02 & 0.03 & 0.02 & 0.02 & 0.04 \\
3661 & Kepler-1542 & 25 & 0.05 & 0.01 & 0.5 & 0.03 & 0.04 & 0.04 & 0.01 & 0.01 & 0.03 & 0.01 & 0.01 & 0.01 & 0.03 & 0.01 & 0.02 & 0.01 & 0.01 & 0.03 \\
3662 & KOI-4032 & 27 & 0.05 & 0.01 & 0.5 & 0.03 & 0.08 & 0.06 & 0.03 & 0.02 & 0.04 & 0.02 & 0.02 & 0.02 & 0.04 & 0.02 & 0.03 & 0.02 & 0.02 & 0.04 \\
3663 & KOI-3012 & 27 & 0.05 & 0.01 & 0.5 & 0.03 & 0.08 & 0.06 & 0.03 & 0.02 & 0.04 & 0.02 & 0.02 & 0.02 & 0.04 & 0.02 & 0.03 & 0.02 & 0.02 & 0.04 \\
3664 & KOI-4473 & 27 & 0.05 & 0.01 & 0.5 & 0.03 & 0.08 & 0.06 & 0.03 & 0.02 & 0.04 & 0.02 & 0.02 & 0.02 & 0.04 & 0.02 & 0.03 & 0.02 & 0.02 & 0.04 \\
3665 & KOI-3083 & 27 & 0.05 & 0.01 & 0.5 & 0.03 & 0.08 & 0.06 & 0.03 & 0.02 & 0.04 & 0.02 & 0.02 & 0.02 & 0.04 & 0.02 & 0.03 & 0.02 & 0.02 & 0.04 \\
3666 & KOI-3100 & 27 & 0.05 & 0.01 & 0.5 & 0.03 & 0.08 & 0.06 & 0.03 & 0.02 & 0.04 & 0.02 & 0.02 & 0.02 & 0.04 & 0.02 & 0.03 & 0.02 & 0.02 & 0.04 \\
3667 & KOI-1379 & 28 & 0.06 & 0.02 & 0.5 & 0.04 & 0.08 & 0.06 & 0.03 & 0.02 & 0.05 & 0.02 & 0.03 & 0.02 & 0.05 & 0.02 & 0.03 & 0.02 & 0.02 & 0.04 \\
3668 & KOI-1618 & 27 & 0.05 & 0.01 & 0.5 & 0.03 & 0.08 & 0.06 & 0.03 & 0.02 & 0.04 & 0.02 & 0.02 & 0.02 & 0.04 & 0.02 & 0.03 & 0.02 & 0.02 & 0.04 \\
3669 & KOI-5375 & 29 & 0.06 & 0.02 & 0.6 & 0.04 & 0.10 & 0.07 & 0.04 & 0.03 & 0.05 & 0.03 & 0.03 & 0.03 & 0.05 & 0.02 & 0.04 & 0.02 & 0.02 & 0.05 \\
3670 & KOI-369 & 27 & 0.05 & 0.01 & 0.5 & 0.03 & 0.08 & 0.06 & 0.03 & 0.02 & 0.04 & 0.02 & 0.03 & 0.02 & 0.04 & 0.02 & 0.03 & 0.02 & 0.02 & 0.04 \\
3671 & KOI-238 & 28 & 0.06 & 0.02 & 0.5 & 0.04 & 0.09 & 0.07 & 0.03 & 0.02 & 0.05 & 0.02 & 0.03 & 0.02 & 0.05 & 0.02 & 0.03 & 0.02 & 0.02 & 0.05 \\
3672 & KOI-987 & 27 & 0.05 & 0.01 & 0.5 & 0.03 & 0.08 & 0.06 & 0.03 & 0.02 & 0.04 & 0.02 & 0.02 & 0.02 & 0.04 & 0.02 & 0.03 & 0.02 & 0.02 & 0.04 \\
3673 & KOI-4136 & 27 & 0.05 & 0.01 & 0.5 & 0.03 & 0.08 & 0.06 & 0.03 & 0.02 & 0.04 & 0.02 & 0.02 & 0.02 & 0.04 & 0.02 & 0.03 & 0.02 & 0.02 & 0.04 \\
3674 & KOI-2051 & 30 & 0.06 & 0.02 & 0.6 & 0.04 & 0.10 & 0.08 & 0.04 & 0.03 & 0.05 & 0.03 & 0.03 & 0.03 & 0.05 & 0.02 & 0.04 & 0.02 & 0.02 & 0.05 \\
3675 & KOI-1961 & 27 & 0.05 & 0.01 & 0.5 & 0.03 & 0.08 & 0.06 & 0.03 & 0.02 & 0.04 & 0.02 & 0.02 & 0.02 & 0.04 & 0.02 & 0.03 & 0.02 & 0.02 & 0.04 \\
3676 & KOI-2916 & 28 & 0.06 & 0.02 & 0.5 & 0.04 & 0.08 & 0.06 & 0.03 & 0.02 & 0.05 & 0.02 & 0.03 & 0.02 & 0.05 & 0.02 & 0.03 & 0.02 & 0.02 & 0.04 \\
3677 & KOI-2561 & 27 & 0.05 & 0.01 & 0.5 & 0.03 & 0.08 & 0.06 & 0.03 & 0.02 & 0.04 & 0.02 & 0.03 & 0.02 & 0.04 & 0.02 & 0.03 & 0.02 & 0.02 & 0.04 \\
3678 & KOI-2516 & 28 & 0.05 & 0.01 & 0.5 & 0.03 & 0.08 & 0.06 & 0.03 & 0.02 & 0.04 & 0.02 & 0.03 & 0.02 & 0.04 & 0.02 & 0.03 & 0.02 & 0.02 & 0.04 \\
3679 & KOI-456 & 29 & 0.06 & 0.02 & 0.6 & 0.04 & 0.10 & 0.07 & 0.04 & 0.02 & 0.05 & 0.03 & 0.03 & 0.02 & 0.05 & 0.02 & 0.04 & 0.02 & 0.02 & 0.05 \\
3680 & KOI-1979 & 28 & 0.05 & 0.01 & 0.5 & 0.03 & 0.08 & 0.06 & 0.03 & 0.02 & 0.04 & 0.02 & 0.03 & 0.02 & 0.04 & 0.02 & 0.03 & 0.02 & 0.02 & 0.04 \\
3681 & KOI-5379 & 29 & 0.06 & 0.02 & 0.6 & 0.04 & 0.09 & 0.07 & 0.04 & 0.02 & 0.05 & 0.03 & 0.03 & 0.02 & 0.05 & 0.02 & 0.04 & 0.02 & 0.02 & 0.05 \\
3682 & KOI-1862 & 27 & 0.05 & 0.01 & 0.5 & 0.03 & 0.08 & 0.06 & 0.03 & 0.02 & 0.04 & 0.02 & 0.02 & 0.02 & 0.04 & 0.02 & 0.03 & 0.02 & 0.02 & 0.04 \\
3683 & KOI-674 & 27 & 0.05 & 0.01 & 0.5 & 0.03 & 0.07 & 0.05 & 0.03 & 0.02 & 0.04 & 0.02 & 0.02 & 0.02 & 0.04 & 0.02 & 0.03 & 0.01 & 0.02 & 0.04 \\
3684 & KOI-373 & 27 & 0.05 & 0.01 & 0.5 & 0.03 & 0.08 & 0.06 & 0.03 & 0.02 & 0.04 & 0.02 & 0.02 & 0.02 & 0.04 & 0.02 & 0.03 & 0.02 & 0.02 & 0.04 \\
3685 & KOI-1378 & 27 & 0.05 & 0.01 & 0.5 & 0.03 & 0.08 & 0.06 & 0.03 & 0.02 & 0.04 & 0.02 & 0.02 & 0.02 & 0.04 & 0.02 & 0.03 & 0.02 & 0.02 & 0.04 \\
3686 & KOI-4864 & 27 & 0.05 & 0.01 & 0.5 & 0.03 & 0.08 & 0.06 & 0.03 & 0.02 & 0.04 & 0.02 & 0.03 & 0.02 & 0.04 & 0.02 & 0.03 & 0.02 & 0.02 & 0.04 \\
3687 & KOI-4665 & 27 & 0.05 & 0.01 & 0.5 & 0.03 & 0.08 & 0.06 & 0.03 & 0.02 & 0.04 & 0.02 & 0.02 & 0.02 & 0.04 & 0.02 & 0.03 & 0.02 & 0.02 & 0.04 \\
3688 & KOI-266 & 28 & 0.05 & 0.01 & 0.5 & 0.04 & 0.08 & 0.06 & 0.03 & 0.02 & 0.04 & 0.02 & 0.03 & 0.02 & 0.04 & 0.02 & 0.03 & 0.02 & 0.02 & 0.04 \\
3689 & KOI-3096 & 27 & 0.05 & 0.01 & 0.5 & 0.03 & 0.08 & 0.06 & 0.03 & 0.02 & 0.04 & 0.02 & 0.02 & 0.02 & 0.04 & 0.02 & 0.03 & 0.02 & 0.02 & 0.04 \\
3690 & KOI-313 & 27 & 0.05 & 0.01 & 0.5 & 0.03 & 0.08 & 0.06 & 0.03 & 0.02 & 0.04 & 0.02 & 0.02 & 0.02 & 0.04 & 0.02 & 0.03 & 0.02 & 0.02 & 0.04 \\
3691 & KOI-884 & 28 & 0.06 & 0.02 & 0.5 & 0.04 & 0.09 & 0.07 & 0.03 & 0.02 & 0.05 & 0.02 & 0.03 & 0.02 & 0.05 & 0.02 & 0.03 & 0.02 & 0.02 & 0.05 \\
3692 & KOI-1848 & 28 & 0.05 & 0.01 & 0.5 & 0.04 & 0.08 & 0.06 & 0.03 & 0.02 & 0.04 & 0.02 & 0.03 & 0.02 & 0.04 & 0.02 & 0.03 & 0.02 & 0.02 & 0.04 \\
3693 & KOI-2357 & 31 & 0.06 & 0.02 & 0.6 & 0.04 & 0.11 & 0.08 & 0.04 & 0.03 & 0.06 & 0.03 & 0.03 & 0.03 & 0.05 & 0.02 & 0.04 & 0.02 & 0.02 & 0.05 \\
3694 & KOI-5393 & 29 & 0.06 & 0.02 & 0.6 & 0.04 & 0.09 & 0.07 & 0.04 & 0.02 & 0.05 & 0.02 & 0.03 & 0.02 & 0.05 & 0.02 & 0.03 & 0.02 & 0.02 & 0.05 \\
3695 & KOI-3193 & 28 & 0.05 & 0.02 & 0.5 & 0.04 & 0.08 & 0.06 & 0.03 & 0.02 & 0.05 & 0.02 & 0.03 & 0.02 & 0.04 & 0.02 & 0.03 & 0.02 & 0.02 & 0.04 \\
3696 & KOI-1890 & 27 & 0.05 & 0.01 & 0.5 & 0.03 & 0.08 & 0.06 & 0.03 & 0.02 & 0.04 & 0.02 & 0.02 & 0.02 & 0.04 & 0.02 & 0.03 & 0.02 & 0.02 & 0.04 \\
3697 & KOI-457 & 27 & 0.05 & 0.01 & 0.5 & 0.03 & 0.07 & 0.06 & 0.03 & 0.02 & 0.04 & 0.02 & 0.02 & 0.02 & 0.04 & 0.02 & 0.03 & 0.02 & 0.02 & 0.04 \\
3698 & KOI-679 & 27 & 0.05 & 0.01 & 0.5 & 0.03 & 0.08 & 0.06 & 0.03 & 0.02 & 0.04 & 0.02 & 0.02 & 0.02 & 0.04 & 0.02 & 0.03 & 0.02 & 0.02 & 0.04 \\
3699 & KOI-678 & 27 & 0.05 & 0.01 & 0.5 & 0.03 & 0.07 & 0.06 & 0.03 & 0.02 & 0.04 & 0.02 & 0.02 & 0.02 & 0.04 & 0.02 & 0.03 & 0.02 & 0.02 & 0.04 \\
3700 & KOI-4663 & 27 & 0.05 & 0.01 & 0.5 & 0.03 & 0.07 & 0.06 & 0.03 & 0.02 & 0.04 & 0.02 & 0.02 & 0.02 & 0.04 & 0.02 & 0.03 & 0.02 & 0.02 & 0.04 \\
3701 & Kepler-435 & 26 & 0.05 & 0.01 & 0.5 & 0.03 & 0.06 & 0.05 & 0.02 & 0.02 & 0.03 & 0.01 & 0.02 & 0.02 & 0.04 & 0.02 & 0.02 & 0.01 & 0.02 & 0.04 \\
3702 & KOI-150 & 27 & 0.05 & 0.01 & 0.5 & 0.03 & 0.08 & 0.06 & 0.03 & 0.02 & 0.04 & 0.02 & 0.02 & 0.02 & 0.04 & 0.02 & 0.03 & 0.02 & 0.02 & 0.04 \\
3703 & KOI-4160 & 27 & 0.05 & 0.01 & 0.5 & 0.03 & 0.08 & 0.06 & 0.03 & 0.02 & 0.04 & 0.02 & 0.02 & 0.02 & 0.04 & 0.02 & 0.03 & 0.02 & 0.02 & 0.04 \\
3704 & KOI-3128 & 27 & 0.05 & 0.01 & 0.5 & 0.03 & 0.08 & 0.06 & 0.03 & 0.02 & 0.04 & 0.02 & 0.02 & 0.02 & 0.04 & 0.02 & 0.03 & 0.02 & 0.02 & 0.04 \\
3705 & Kepler-431 & 25 & 0.05 & 0.01 & 0.5 & 0.03 & 0.06 & 0.04 & 0.02 & 0.02 & 0.03 & 0.01 & 0.02 & 0.02 & 0.04 & 0.02 & 0.02 & 0.01 & 0.01 & 0.03 \\
3706 & KOI-3097 & 27 & 0.05 & 0.01 & 0.5 & 0.03 & 0.08 & 0.06 & 0.03 & 0.02 & 0.04 & 0.02 & 0.02 & 0.02 & 0.04 & 0.02 & 0.03 & 0.02 & 0.02 & 0.04 \\
3707 & KOI-2631 & 27 & 0.05 & 0.01 & 0.5 & 0.03 & 0.08 & 0.06 & 0.03 & 0.02 & 0.04 & 0.02 & 0.02 & 0.02 & 0.04 & 0.02 & 0.03 & 0.02 & 0.02 & 0.04 \\
3708 & KOI-683 & 27 & 0.05 & 0.01 & 0.5 & 0.03 & 0.08 & 0.06 & 0.03 & 0.02 & 0.04 & 0.02 & 0.03 & 0.02 & 0.04 & 0.02 & 0.03 & 0.02 & 0.02 & 0.04 \\
3709 & KOI-1706 & 27 & 0.05 & 0.01 & 0.5 & 0.03 & 0.08 & 0.06 & 0.03 & 0.02 & 0.04 & 0.02 & 0.02 & 0.02 & 0.04 & 0.02 & 0.03 & 0.02 & 0.02 & 0.04 \\
3710 & KOI-568 & 28 & 0.06 & 0.02 & 0.5 & 0.04 & 0.08 & 0.06 & 0.03 & 0.02 & 0.05 & 0.02 & 0.03 & 0.02 & 0.05 & 0.02 & 0.03 & 0.02 & 0.02 & 0.04 \\
3711 & KOI-4614 & 27 & 0.05 & 0.01 & 0.5 & 0.03 & 0.08 & 0.06 & 0.03 & 0.02 & 0.04 & 0.02 & 0.02 & 0.02 & 0.04 & 0.02 & 0.03 & 0.02 & 0.02 & 0.04 \\
3712 & KOI-1898 & 28 & 0.05 & 0.01 & 0.5 & 0.04 & 0.08 & 0.06 & 0.03 & 0.02 & 0.04 & 0.02 & 0.03 & 0.02 & 0.04 & 0.02 & 0.03 & 0.02 & 0.02 & 0.04 \\
3713 & KOI-3943 & 27 & 0.05 & 0.01 & 0.5 & 0.03 & 0.08 & 0.06 & 0.03 & 0.02 & 0.04 & 0.02 & 0.02 & 0.02 & 0.04 & 0.02 & 0.03 & 0.02 & 0.02 & 0.04 \\
3714 & KOI-315 & 27 & 0.05 & 0.01 & 0.5 & 0.03 & 0.07 & 0.06 & 0.03 & 0.02 & 0.04 & 0.02 & 0.02 & 0.02 & 0.04 & 0.02 & 0.03 & 0.02 & 0.02 & 0.04 \\
3715 & KOI-1528 & 28 & 0.05 & 0.01 & 0.5 & 0.04 & 0.08 & 0.06 & 0.03 & 0.02 & 0.04 & 0.02 & 0.03 & 0.02 & 0.04 & 0.02 & 0.03 & 0.02 & 0.02 & 0.04 \\
3716 & KOI-2722 & 28 & 0.05 & 0.01 & 0.5 & 0.04 & 0.08 & 0.06 & 0.03 & 0.02 & 0.04 & 0.02 & 0.03 & 0.02 & 0.04 & 0.02 & 0.03 & 0.02 & 0.02 & 0.04 \\
3717 & Kepler-402 & 26 & 0.05 & 0.01 & 0.5 & 0.03 & 0.06 & 0.05 & 0.02 & 0.02 & 0.03 & 0.01 & 0.02 & 0.02 & 0.04 & 0.02 & 0.02 & 0.01 & 0.01 & 0.03 \\
3718 & KOI-892 & 36 & 0.07 & 0.02 & 0.6 & 0.06 & 0.15 & 0.11 & 0.06 & 0.04 & 0.08 & 0.04 & 0.05 & 0.04 & 0.07 & 0.03 & 0.05 & 0.03 & 0.03 & 0.07 \\
3719 & KOI-2585 & 27 & 0.05 & 0.01 & 0.5 & 0.03 & 0.08 & 0.06 & 0.03 & 0.02 & 0.04 & 0.02 & 0.02 & 0.02 & 0.04 & 0.02 & 0.03 & 0.02 & 0.02 & 0.04 \\
3720 & KOI-269 & 27 & 0.05 & 0.01 & 0.5 & 0.03 & 0.08 & 0.06 & 0.03 & 0.02 & 0.04 & 0.02 & 0.03 & 0.02 & 0.04 & 0.02 & 0.03 & 0.02 & 0.02 & 0.04 \\
3721 & KOI-684 & 27 & 0.05 & 0.01 & 0.5 & 0.03 & 0.07 & 0.06 & 0.03 & 0.02 & 0.04 & 0.02 & 0.02 & 0.02 & 0.04 & 0.02 & 0.03 & 0.02 & 0.02 & 0.04 \\
3722 & KOI-4561 & 27 & 0.05 & 0.01 & 0.5 & 0.03 & 0.08 & 0.06 & 0.03 & 0.02 & 0.04 & 0.02 & 0.02 & 0.02 & 0.04 & 0.02 & 0.03 & 0.02 & 0.02 & 0.04 \\
3723 & KOI-1921 & 28 & 0.05 & 0.01 & 0.5 & 0.03 & 0.08 & 0.06 & 0.03 & 0.02 & 0.04 & 0.02 & 0.03 & 0.02 & 0.04 & 0.02 & 0.03 & 0.02 & 0.02 & 0.04 \\
3724 & KOI-4482 & 27 & 0.05 & 0.01 & 0.5 & 0.03 & 0.08 & 0.06 & 0.03 & 0.02 & 0.04 & 0.02 & 0.02 & 0.02 & 0.04 & 0.02 & 0.03 & 0.02 & 0.02 & 0.04 \\
3725 & KOI-3721 & 27 & 0.05 & 0.01 & 0.5 & 0.03 & 0.08 & 0.06 & 0.03 & 0.02 & 0.04 & 0.02 & 0.02 & 0.02 & 0.04 & 0.02 & 0.03 & 0.02 & 0.02 & 0.04 \\
3726 & KOI-4022 & 27 & 0.05 & 0.01 & 0.5 & 0.03 & 0.08 & 0.06 & 0.03 & 0.02 & 0.04 & 0.02 & 0.02 & 0.02 & 0.04 & 0.02 & 0.03 & 0.02 & 0.02 & 0.04 \\
3727 & KOI-1808 & 27 & 0.05 & 0.01 & 0.5 & 0.03 & 0.08 & 0.06 & 0.03 & 0.02 & 0.04 & 0.02 & 0.02 & 0.02 & 0.04 & 0.02 & 0.03 & 0.02 & 0.02 & 0.04 \\
3728 & KOI-685 & 28 & 0.06 & 0.02 & 0.5 & 0.04 & 0.09 & 0.06 & 0.03 & 0.02 & 0.05 & 0.02 & 0.03 & 0.02 & 0.05 & 0.02 & 0.03 & 0.02 & 0.02 & 0.04 \\
3729 & KOI-3023 & 28 & 0.05 & 0.01 & 0.5 & 0.03 & 0.08 & 0.06 & 0.03 & 0.02 & 0.04 & 0.02 & 0.03 & 0.02 & 0.04 & 0.02 & 0.03 & 0.02 & 0.02 & 0.04 \\
3730 & KOI-4725 & 27 & 0.05 & 0.01 & 0.5 & 0.03 & 0.08 & 0.06 & 0.03 & 0.02 & 0.04 & 0.02 & 0.02 & 0.02 & 0.04 & 0.02 & 0.03 & 0.02 & 0.02 & 0.04 \\
3731 & KOI-2848 & 27 & 0.05 & 0.01 & 0.5 & 0.03 & 0.08 & 0.06 & 0.03 & 0.02 & 0.04 & 0.02 & 0.02 & 0.02 & 0.04 & 0.02 & 0.03 & 0.02 & 0.02 & 0.04 \\
3732 & KOI-3787 & 27 & 0.05 & 0.01 & 0.5 & 0.03 & 0.08 & 0.06 & 0.03 & 0.02 & 0.04 & 0.02 & 0.02 & 0.02 & 0.04 & 0.02 & 0.03 & 0.02 & 0.02 & 0.04 \\
3733 & KOI-171 & 27 & 0.05 & 0.01 & 0.5 & 0.03 & 0.08 & 0.06 & 0.03 & 0.02 & 0.04 & 0.02 & 0.03 & 0.02 & 0.04 & 0.02 & 0.03 & 0.02 & 0.02 & 0.04 \\
3734 & KOI-1533 & 27 & 0.05 & 0.01 & 0.5 & 0.03 & 0.08 & 0.06 & 0.03 & 0.02 & 0.04 & 0.02 & 0.03 & 0.02 & 0.04 & 0.02 & 0.03 & 0.02 & 0.02 & 0.04 \\
3735 & KOI-4582 & 27 & 0.05 & 0.01 & 0.5 & 0.03 & 0.08 & 0.06 & 0.03 & 0.02 & 0.04 & 0.02 & 0.02 & 0.02 & 0.04 & 0.02 & 0.03 & 0.02 & 0.02 & 0.04 \\
3736 & KOI-1964 & 27 & 0.05 & 0.01 & 0.5 & 0.03 & 0.07 & 0.06 & 0.03 & 0.02 & 0.04 & 0.02 & 0.02 & 0.02 & 0.04 & 0.02 & 0.03 & 0.02 & 0.02 & 0.04 \\
3737 & KOI-2984 & 27 & 0.05 & 0.01 & 0.5 & 0.03 & 0.08 & 0.06 & 0.03 & 0.02 & 0.04 & 0.02 & 0.02 & 0.02 & 0.04 & 0.02 & 0.03 & 0.02 & 0.02 & 0.04 \\
3738 & KOI-1818 & 27 & 0.05 & 0.01 & 0.5 & 0.03 & 0.08 & 0.06 & 0.03 & 0.02 & 0.04 & 0.02 & 0.02 & 0.02 & 0.04 & 0.02 & 0.03 & 0.02 & 0.02 & 0.04 \\
3739 & KOI-4257 & 28 & 0.06 & 0.02 & 0.5 & 0.04 & 0.09 & 0.07 & 0.03 & 0.02 & 0.05 & 0.02 & 0.03 & 0.02 & 0.05 & 0.02 & 0.03 & 0.02 & 0.02 & 0.05 \\
3740 & KOI-686 & 27 & 0.05 & 0.01 & 0.5 & 0.03 & 0.08 & 0.06 & 0.03 & 0.02 & 0.04 & 0.02 & 0.02 & 0.02 & 0.04 & 0.02 & 0.03 & 0.02 & 0.02 & 0.04 \\
3741 & KOI-3236 & 28 & 0.05 & 0.01 & 0.5 & 0.04 & 0.08 & 0.06 & 0.03 & 0.02 & 0.04 & 0.02 & 0.03 & 0.02 & 0.04 & 0.02 & 0.03 & 0.02 & 0.02 & 0.04 \\
3742 & KOI-4109 & 29 & 0.06 & 0.02 & 0.5 & 0.04 & 0.09 & 0.07 & 0.03 & 0.02 & 0.05 & 0.02 & 0.03 & 0.02 & 0.05 & 0.02 & 0.03 & 0.02 & 0.02 & 0.05 \\
3743 & KOI-4773 & 28 & 0.06 & 0.02 & 0.5 & 0.04 & 0.09 & 0.07 & 0.03 & 0.02 & 0.05 & 0.02 & 0.03 & 0.02 & 0.05 & 0.02 & 0.03 & 0.02 & 0.02 & 0.04 \\
3744 & KOI-687 & 27 & 0.05 & 0.01 & 0.5 & 0.03 & 0.08 & 0.06 & 0.03 & 0.02 & 0.04 & 0.02 & 0.02 & 0.02 & 0.04 & 0.02 & 0.03 & 0.02 & 0.02 & 0.04 \\
3745 & KOI-459 & 31 & 0.06 & 0.02 & 0.6 & 0.04 & 0.11 & 0.08 & 0.04 & 0.03 & 0.06 & 0.03 & 0.03 & 0.03 & 0.05 & 0.02 & 0.04 & 0.02 & 0.02 & 0.05 \\
3746 & KOI-92 & 27 & 0.05 & 0.01 & 0.5 & 0.03 & 0.08 & 0.06 & 0.03 & 0.02 & 0.04 & 0.02 & 0.02 & 0.02 & 0.04 & 0.02 & 0.03 & 0.02 & 0.02 & 0.04 \\
3747 & KOI-3214 & 27 & 0.05 & 0.01 & 0.5 & 0.03 & 0.08 & 0.06 & 0.03 & 0.02 & 0.04 & 0.02 & 0.02 & 0.02 & 0.04 & 0.02 & 0.03 & 0.02 & 0.02 & 0.04 \\
3748 & KOI-2674 & 27 & 0.05 & 0.01 & 0.5 & 0.03 & 0.08 & 0.06 & 0.03 & 0.02 & 0.04 & 0.02 & 0.02 & 0.02 & 0.04 & 0.02 & 0.03 & 0.02 & 0.02 & 0.04 \\
3749 & KOI-2352 & 28 & 0.05 & 0.01 & 0.5 & 0.03 & 0.08 & 0.06 & 0.03 & 0.02 & 0.04 & 0.02 & 0.03 & 0.02 & 0.04 & 0.02 & 0.03 & 0.02 & 0.02 & 0.04 \\
3750 & KOI-237 & 29 & 0.06 & 0.02 & 0.5 & 0.04 & 0.09 & 0.07 & 0.04 & 0.02 & 0.05 & 0.02 & 0.03 & 0.02 & 0.05 & 0.02 & 0.03 & 0.02 & 0.02 & 0.05 \\
3751 & KOI-520 & 30 & 0.06 & 0.02 & 0.6 & 0.04 & 0.10 & 0.07 & 0.04 & 0.03 & 0.05 & 0.03 & 0.03 & 0.03 & 0.05 & 0.02 & 0.04 & 0.02 & 0.02 & 0.05 \\
3752 & KOI-517 & 29 & 0.06 & 0.02 & 0.5 & 0.04 & 0.09 & 0.07 & 0.04 & 0.02 & 0.05 & 0.02 & 0.03 & 0.02 & 0.05 & 0.02 & 0.03 & 0.02 & 0.02 & 0.05 \\
3753 & KOI-519 & 32 & 0.06 & 0.02 & 0.6 & 0.05 & 0.12 & 0.09 & 0.05 & 0.03 & 0.06 & 0.03 & 0.04 & 0.03 & 0.06 & 0.02 & 0.04 & 0.02 & 0.03 & 0.06 \\
3754 & KOI-155 & 27 & 0.05 & 0.01 & 0.5 & 0.03 & 0.08 & 0.06 & 0.03 & 0.02 & 0.04 & 0.02 & 0.03 & 0.02 & 0.04 & 0.02 & 0.03 & 0.02 & 0.02 & 0.04 \\
3755 & KOI-316 & 27 & 0.05 & 0.01 & 0.5 & 0.03 & 0.08 & 0.06 & 0.03 & 0.02 & 0.04 & 0.02 & 0.02 & 0.02 & 0.04 & 0.02 & 0.03 & 0.02 & 0.02 & 0.04 \\
3756 & KOI-569 & 30 & 0.06 & 0.02 & 0.6 & 0.04 & 0.11 & 0.08 & 0.04 & 0.03 & 0.06 & 0.03 & 0.03 & 0.03 & 0.05 & 0.02 & 0.04 & 0.02 & 0.02 & 0.05 \\
3757 & KOI-2743 & 27 & 0.05 & 0.01 & 0.5 & 0.03 & 0.08 & 0.06 & 0.03 & 0.02 & 0.04 & 0.02 & 0.02 & 0.02 & 0.04 & 0.02 & 0.03 & 0.02 & 0.02 & 0.04 \\
3758 & KOI-3245 & 27 & 0.05 & 0.01 & 0.5 & 0.03 & 0.08 & 0.06 & 0.03 & 0.02 & 0.04 & 0.02 & 0.02 & 0.02 & 0.04 & 0.02 & 0.03 & 0.02 & 0.02 & 0.04 \\
3759 & KOI-2486 & 27 & 0.05 & 0.01 & 0.5 & 0.03 & 0.08 & 0.06 & 0.03 & 0.02 & 0.04 & 0.02 & 0.02 & 0.02 & 0.04 & 0.02 & 0.03 & 0.02 & 0.02 & 0.04 \\
3760 & KOI-2426 & 27 & 0.05 & 0.01 & 0.5 & 0.03 & 0.07 & 0.06 & 0.03 & 0.02 & 0.04 & 0.02 & 0.02 & 0.02 & 0.04 & 0.02 & 0.03 & 0.02 & 0.02 & 0.04 \\
3761 & KOI-4343 & 29 & 0.06 & 0.02 & 0.5 & 0.04 & 0.09 & 0.07 & 0.04 & 0.02 & 0.05 & 0.02 & 0.03 & 0.02 & 0.05 & 0.02 & 0.03 & 0.02 & 0.02 & 0.05 \\
3762 & KOI-1951 & 27 & 0.05 & 0.01 & 0.5 & 0.03 & 0.08 & 0.06 & 0.03 & 0.02 & 0.04 & 0.02 & 0.02 & 0.02 & 0.04 & 0.02 & 0.03 & 0.02 & 0.02 & 0.04 \\
3763 & KOI-162 & 27 & 0.05 & 0.01 & 0.5 & 0.03 & 0.08 & 0.06 & 0.03 & 0.02 & 0.04 & 0.02 & 0.02 & 0.02 & 0.04 & 0.02 & 0.03 & 0.02 & 0.02 & 0.04 \\
3764 & KOI-4656 & 27 & 0.05 & 0.01 & 0.5 & 0.03 & 0.08 & 0.06 & 0.03 & 0.02 & 0.04 & 0.02 & 0.03 & 0.02 & 0.04 & 0.02 & 0.03 & 0.02 & 0.02 & 0.04 \\
3765 & KOI-4881 & 28 & 0.05 & 0.01 & 0.5 & 0.04 & 0.08 & 0.06 & 0.03 & 0.02 & 0.04 & 0.02 & 0.03 & 0.02 & 0.04 & 0.02 & 0.03 & 0.02 & 0.02 & 0.04 \\
3766 & KOI-317 & 27 & 0.05 & 0.01 & 0.5 & 0.03 & 0.08 & 0.06 & 0.03 & 0.02 & 0.04 & 0.02 & 0.03 & 0.02 & 0.04 & 0.02 & 0.03 & 0.02 & 0.02 & 0.04 \\
3767 & KOI-2073 & 30 & 0.06 & 0.02 & 0.6 & 0.04 & 0.10 & 0.07 & 0.04 & 0.03 & 0.05 & 0.03 & 0.03 & 0.03 & 0.05 & 0.02 & 0.04 & 0.02 & 0.02 & 0.05 \\
3768 & KOI-1019 & 27 & 0.05 & 0.01 & 0.5 & 0.03 & 0.07 & 0.06 & 0.03 & 0.02 & 0.04 & 0.02 & 0.02 & 0.02 & 0.04 & 0.02 & 0.03 & 0.02 & 0.02 & 0.04 \\
3769 & KOI-688 & 27 & 0.05 & 0.01 & 0.5 & 0.03 & 0.08 & 0.06 & 0.03 & 0.02 & 0.04 & 0.02 & 0.02 & 0.02 & 0.04 & 0.02 & 0.03 & 0.02 & 0.02 & 0.04 \\
3770 & KOI-4634 & 28 & 0.05 & 0.01 & 0.5 & 0.04 & 0.08 & 0.06 & 0.03 & 0.02 & 0.04 & 0.02 & 0.03 & 0.02 & 0.04 & 0.02 & 0.03 & 0.02 & 0.02 & 0.04 \\
3771 & KOI-3046 & 27 & 0.05 & 0.01 & 0.5 & 0.03 & 0.08 & 0.06 & 0.03 & 0.02 & 0.04 & 0.02 & 0.02 & 0.02 & 0.04 & 0.02 & 0.03 & 0.02 & 0.02 & 0.04 \\
3772 & KOI-318 & 27 & 0.05 & 0.01 & 0.5 & 0.03 & 0.08 & 0.06 & 0.03 & 0.02 & 0.04 & 0.02 & 0.03 & 0.02 & 0.04 & 0.02 & 0.03 & 0.02 & 0.02 & 0.04 \\
3773 & KOI-2781 & 27 & 0.05 & 0.01 & 0.5 & 0.03 & 0.08 & 0.06 & 0.03 & 0.02 & 0.04 & 0.02 & 0.02 & 0.02 & 0.04 & 0.02 & 0.03 & 0.02 & 0.02 & 0.04 \\
3774 & KOI-2105 & 28 & 0.05 & 0.01 & 0.5 & 0.04 & 0.08 & 0.06 & 0.03 & 0.02 & 0.04 & 0.02 & 0.03 & 0.02 & 0.04 & 0.02 & 0.03 & 0.02 & 0.02 & 0.04 \\
3775 & KOI-1985 & 27 & 0.05 & 0.01 & 0.5 & 0.03 & 0.08 & 0.06 & 0.03 & 0.02 & 0.04 & 0.02 & 0.02 & 0.02 & 0.04 & 0.02 & 0.03 & 0.02 & 0.02 & 0.04 \\
3776 & KOI-572 & 27 & 0.05 & 0.01 & 0.5 & 0.03 & 0.08 & 0.06 & 0.03 & 0.02 & 0.04 & 0.02 & 0.03 & 0.02 & 0.04 & 0.02 & 0.03 & 0.02 & 0.02 & 0.04 \\
3777 & KOI-907 & 34 & 0.06 & 0.02 & 0.6 & 0.05 & 0.13 & 0.10 & 0.05 & 0.03 & 0.07 & 0.04 & 0.04 & 0.03 & 0.06 & 0.03 & 0.05 & 0.03 & 0.03 & 0.06 \\
3778 & KOI-1809 & 27 & 0.05 & 0.01 & 0.5 & 0.03 & 0.07 & 0.06 & 0.03 & 0.02 & 0.04 & 0.02 & 0.02 & 0.02 & 0.04 & 0.02 & 0.03 & 0.02 & 0.02 & 0.04 \\
3779 & KOI-1726 & 27 & 0.05 & 0.01 & 0.5 & 0.03 & 0.07 & 0.06 & 0.03 & 0.02 & 0.04 & 0.02 & 0.02 & 0.02 & 0.04 & 0.02 & 0.03 & 0.01 & 0.02 & 0.04 \\
3780 & KOI-2593 & 27 & 0.05 & 0.01 & 0.5 & 0.03 & 0.08 & 0.06 & 0.03 & 0.02 & 0.04 & 0.02 & 0.02 & 0.02 & 0.04 & 0.02 & 0.03 & 0.02 & 0.02 & 0.04 \\
3781 & KOI-4037 & 27 & 0.05 & 0.01 & 0.5 & 0.03 & 0.08 & 0.06 & 0.03 & 0.02 & 0.04 & 0.02 & 0.02 & 0.02 & 0.04 & 0.02 & 0.03 & 0.02 & 0.02 & 0.04 \\
3782 & KOI-4426 & 27 & 0.05 & 0.01 & 0.5 & 0.03 & 0.08 & 0.06 & 0.03 & 0.02 & 0.04 & 0.02 & 0.02 & 0.02 & 0.04 & 0.02 & 0.03 & 0.02 & 0.02 & 0.04 \\
3783 & KOI-4098 & 28 & 0.05 & 0.01 & 0.5 & 0.03 & 0.08 & 0.06 & 0.03 & 0.02 & 0.04 & 0.02 & 0.03 & 0.02 & 0.04 & 0.02 & 0.03 & 0.02 & 0.02 & 0.04 \\
3784 & KOI-1069 & 32 & 0.06 & 0.02 & 0.6 & 0.05 & 0.12 & 0.09 & 0.05 & 0.03 & 0.06 & 0.03 & 0.04 & 0.03 & 0.06 & 0.02 & 0.04 & 0.02 & 0.03 & 0.06 \\
3785 & KOI-3338 & 27 & 0.05 & 0.01 & 0.5 & 0.03 & 0.08 & 0.06 & 0.03 & 0.02 & 0.04 & 0.02 & 0.02 & 0.02 & 0.04 & 0.02 & 0.03 & 0.02 & 0.02 & 0.04 \\
3786 & KOI-4834 & 27 & 0.05 & 0.01 & 0.5 & 0.03 & 0.07 & 0.05 & 0.03 & 0.02 & 0.04 & 0.02 & 0.02 & 0.02 & 0.04 & 0.02 & 0.03 & 0.01 & 0.02 & 0.04 \\
3787 & KOI-4567 & 27 & 0.05 & 0.01 & 0.5 & 0.03 & 0.08 & 0.06 & 0.03 & 0.02 & 0.04 & 0.02 & 0.02 & 0.02 & 0.04 & 0.02 & 0.03 & 0.02 & 0.02 & 0.04 \\
3788 & KOI-4435 & 28 & 0.05 & 0.01 & 0.5 & 0.04 & 0.08 & 0.06 & 0.03 & 0.02 & 0.04 & 0.02 & 0.03 & 0.02 & 0.04 & 0.02 & 0.03 & 0.02 & 0.02 & 0.04 \\
3789 & KOI-1137 & 29 & 0.06 & 0.02 & 0.6 & 0.04 & 0.09 & 0.07 & 0.04 & 0.02 & 0.05 & 0.02 & 0.03 & 0.02 & 0.05 & 0.02 & 0.03 & 0.02 & 0.02 & 0.05 \\
3790 & KOI-3301 & 27 & 0.05 & 0.01 & 0.5 & 0.03 & 0.08 & 0.06 & 0.03 & 0.02 & 0.04 & 0.02 & 0.02 & 0.02 & 0.04 & 0.02 & 0.03 & 0.02 & 0.02 & 0.04 \\
3791 & Kepler-271 & 26 & 0.05 & 0.01 & 0.5 & 0.03 & 0.06 & 0.05 & 0.02 & 0.02 & 0.04 & 0.01 & 0.02 & 0.02 & 0.04 & 0.02 & 0.02 & 0.01 & 0.02 & 0.04 \\
3792 & KOI-1150 & 27 & 0.05 & 0.01 & 0.5 & 0.03 & 0.08 & 0.06 & 0.03 & 0.02 & 0.04 & 0.02 & 0.02 & 0.02 & 0.04 & 0.02 & 0.03 & 0.02 & 0.02 & 0.04 \\
3793 & KOI-1820 & 27 & 0.05 & 0.01 & 0.5 & 0.03 & 0.08 & 0.06 & 0.03 & 0.02 & 0.04 & 0.02 & 0.02 & 0.02 & 0.04 & 0.02 & 0.03 & 0.02 & 0.02 & 0.04 \\
3794 & KOI-4399 & 27 & 0.05 & 0.01 & 0.5 & 0.03 & 0.07 & 0.06 & 0.03 & 0.02 & 0.04 & 0.02 & 0.02 & 0.02 & 0.04 & 0.02 & 0.03 & 0.02 & 0.02 & 0.04 \\
3795 & KOI-574 & 31 & 0.06 & 0.02 & 0.6 & 0.04 & 0.11 & 0.08 & 0.05 & 0.03 & 0.06 & 0.03 & 0.04 & 0.03 & 0.05 & 0.02 & 0.04 & 0.02 & 0.03 & 0.06 \\
3796 & KOI-4763 & 28 & 0.06 & 0.02 & 0.5 & 0.04 & 0.09 & 0.06 & 0.03 & 0.02 & 0.05 & 0.02 & 0.03 & 0.02 & 0.05 & 0.02 & 0.03 & 0.02 & 0.02 & 0.04 \\
3797 & KOI-573 & 29 & 0.06 & 0.02 & 0.6 & 0.04 & 0.10 & 0.07 & 0.04 & 0.02 & 0.05 & 0.03 & 0.03 & 0.02 & 0.05 & 0.02 & 0.04 & 0.02 & 0.02 & 0.05 \\
3798 & KOI-127 & 28 & 0.05 & 0.01 & 0.5 & 0.03 & 0.08 & 0.06 & 0.03 & 0.02 & 0.04 & 0.02 & 0.03 & 0.02 & 0.04 & 0.02 & 0.03 & 0.02 & 0.02 & 0.04 \\
3799 & KOI-4407 & 27 & 0.05 & 0.01 & 0.5 & 0.03 & 0.08 & 0.06 & 0.03 & 0.02 & 0.04 & 0.02 & 0.02 & 0.02 & 0.04 & 0.02 & 0.03 & 0.02 & 0.02 & 0.04 \\
3800 & Kepler-79 & 27 & 0.05 & 0.01 & 0.5 & 0.03 & 0.08 & 0.06 & 0.03 & 0.02 & 0.04 & 0.02 & 0.02 & 0.02 & 0.04 & 0.02 & 0.03 & 0.02 & 0.02 & 0.04 \\
3801 & KOI-152 & 27 & 0.05 & 0.01 & 0.5 & 0.03 & 0.08 & 0.06 & 0.03 & 0.02 & 0.04 & 0.02 & 0.02 & 0.02 & 0.04 & 0.02 & 0.03 & 0.02 & 0.02 & 0.04 \\
3802 & KOI-689 & 27 & 0.05 & 0.01 & 0.5 & 0.03 & 0.08 & 0.06 & 0.03 & 0.02 & 0.04 & 0.02 & 0.02 & 0.02 & 0.04 & 0.02 & 0.03 & 0.02 & 0.02 & 0.04 \\
3803 & KOI-2730 & 27 & 0.05 & 0.01 & 0.5 & 0.03 & 0.08 & 0.06 & 0.03 & 0.02 & 0.04 & 0.02 & 0.02 & 0.02 & 0.04 & 0.02 & 0.03 & 0.02 & 0.02 & 0.04 \\
3804 & KOI-4693 & 27 & 0.05 & 0.01 & 0.5 & 0.03 & 0.08 & 0.06 & 0.03 & 0.02 & 0.04 & 0.02 & 0.03 & 0.02 & 0.04 & 0.02 & 0.03 & 0.02 & 0.02 & 0.04 \\
3805 & KOI-1148 & 27 & 0.05 & 0.01 & 0.5 & 0.03 & 0.08 & 0.06 & 0.03 & 0.02 & 0.04 & 0.02 & 0.02 & 0.02 & 0.04 & 0.02 & 0.03 & 0.02 & 0.02 & 0.04 \\
3806 & KOI-102 & 26 & 0.05 & 0.01 & 0.5 & 0.03 & 0.07 & 0.05 & 0.02 & 0.02 & 0.04 & 0.02 & 0.02 & 0.02 & 0.04 & 0.02 & 0.03 & 0.01 & 0.02 & 0.04 \\
3807 & KOI-4603 & 29 & 0.06 & 0.02 & 0.6 & 0.04 & 0.09 & 0.07 & 0.04 & 0.02 & 0.05 & 0.02 & 0.03 & 0.02 & 0.05 & 0.02 & 0.03 & 0.02 & 0.02 & 0.05 \\
3808 & TYC 2810-1660-1 & 25 & 0.05 & 0.01 & 0.5 & 0.03 & 0.04 & 0.04 & 0.01 & 0.01 & 0.03 & 0.01 & 0.01 & 0.01 & 0.03 & 0.01 & 0.02 & 0.01 & 0.01 & 0.03 \\
3809 & BD+43183 & 25 & 0.05 & 0.01 & 0.5 & 0.03 & 0.04 & 0.04 & 0.01 & 0.01 & 0.03 & 0.01 & 0.01 & 0.01 & 0.03 & 0.01 & 0.02 & 0.01 & 0.01 & 0.03 \\
3810 & KOI-3497 & 27 & 0.05 & 0.01 & 0.5 & 0.03 & 0.07 & 0.05 & 0.03 & 0.02 & 0.04 & 0.02 & 0.02 & 0.02 & 0.04 & 0.02 & 0.03 & 0.01 & 0.02 & 0.04 \\
3811 & KOI-3251 & 27 & 0.05 & 0.01 & 0.5 & 0.03 & 0.08 & 0.06 & 0.03 & 0.02 & 0.04 & 0.02 & 0.02 & 0.02 & 0.04 & 0.02 & 0.03 & 0.02 & 0.02 & 0.04 \\
3812 & KOI-370 & 27 & 0.05 & 0.01 & 0.5 & 0.03 & 0.08 & 0.06 & 0.03 & 0.02 & 0.04 & 0.02 & 0.02 & 0.02 & 0.04 & 0.02 & 0.03 & 0.02 & 0.02 & 0.04 \\
3813 & KOI-2389 & 27 & 0.05 & 0.01 & 0.5 & 0.03 & 0.08 & 0.06 & 0.03 & 0.02 & 0.04 & 0.02 & 0.02 & 0.02 & 0.04 & 0.02 & 0.03 & 0.02 & 0.02 & 0.04 \\
3814 & KOI-4505 & 28 & 0.06 & 0.02 & 0.5 & 0.04 & 0.09 & 0.07 & 0.03 & 0.02 & 0.05 & 0.02 & 0.03 & 0.02 & 0.05 & 0.02 & 0.03 & 0.02 & 0.02 & 0.05 \\
3815 & KOI-2016 & 27 & 0.05 & 0.01 & 0.5 & 0.03 & 0.08 & 0.06 & 0.03 & 0.02 & 0.04 & 0.02 & 0.03 & 0.02 & 0.04 & 0.02 & 0.03 & 0.02 & 0.02 & 0.04 \\
3816 & KOI-691 & 28 & 0.05 & 0.01 & 0.5 & 0.04 & 0.08 & 0.06 & 0.03 & 0.02 & 0.04 & 0.02 & 0.03 & 0.02 & 0.04 & 0.02 & 0.03 & 0.02 & 0.02 & 0.04 \\
3817 & KOI-3315 & 27 & 0.05 & 0.01 & 0.5 & 0.03 & 0.08 & 0.06 & 0.03 & 0.02 & 0.04 & 0.02 & 0.02 & 0.02 & 0.04 & 0.02 & 0.03 & 0.02 & 0.02 & 0.04 \\
3818 & KOI-2022 & 28 & 0.06 & 0.02 & 0.5 & 0.04 & 0.09 & 0.06 & 0.03 & 0.02 & 0.05 & 0.02 & 0.03 & 0.02 & 0.05 & 0.02 & 0.03 & 0.02 & 0.02 & 0.04 \\
3819 & KOI-3111 & 27 & 0.05 & 0.01 & 0.5 & 0.03 & 0.08 & 0.06 & 0.03 & 0.02 & 0.04 & 0.02 & 0.02 & 0.02 & 0.04 & 0.02 & 0.03 & 0.02 & 0.02 & 0.04 \\
3820 & KOI-1792 & 27 & 0.05 & 0.01 & 0.5 & 0.03 & 0.07 & 0.06 & 0.03 & 0.02 & 0.04 & 0.02 & 0.02 & 0.02 & 0.04 & 0.02 & 0.03 & 0.01 & 0.02 & 0.04 \\
3821 & KOI-3890 & 27 & 0.05 & 0.01 & 0.5 & 0.03 & 0.07 & 0.06 & 0.03 & 0.02 & 0.04 & 0.02 & 0.02 & 0.02 & 0.04 & 0.02 & 0.03 & 0.01 & 0.02 & 0.04 \\
3822 & KOI-692 & 27 & 0.05 & 0.01 & 0.5 & 0.03 & 0.08 & 0.06 & 0.03 & 0.02 & 0.04 & 0.02 & 0.02 & 0.02 & 0.04 & 0.02 & 0.03 & 0.02 & 0.02 & 0.04 \\
3823 & KOI-1270 & 28 & 0.06 & 0.02 & 0.5 & 0.04 & 0.09 & 0.07 & 0.03 & 0.02 & 0.05 & 0.02 & 0.03 & 0.02 & 0.05 & 0.02 & 0.03 & 0.02 & 0.02 & 0.04 \\
3824 & KOI-2969 & 27 & 0.05 & 0.01 & 0.5 & 0.03 & 0.08 & 0.06 & 0.03 & 0.02 & 0.04 & 0.02 & 0.02 & 0.02 & 0.04 & 0.02 & 0.03 & 0.02 & 0.02 & 0.04 \\
3825 & KOI-2488 & 27 & 0.05 & 0.01 & 0.5 & 0.03 & 0.08 & 0.06 & 0.03 & 0.02 & 0.04 & 0.02 & 0.03 & 0.02 & 0.04 & 0.02 & 0.03 & 0.02 & 0.02 & 0.04 \\
3826 & KOI-139 & 27 & 0.05 & 0.01 & 0.5 & 0.03 & 0.08 & 0.06 & 0.03 & 0.02 & 0.04 & 0.02 & 0.02 & 0.02 & 0.04 & 0.02 & 0.03 & 0.02 & 0.02 & 0.04 \\
3827 & KOI-1275 & 28 & 0.05 & 0.01 & 0.5 & 0.04 & 0.08 & 0.06 & 0.03 & 0.02 & 0.05 & 0.02 & 0.03 & 0.02 & 0.04 & 0.02 & 0.03 & 0.02 & 0.02 & 0.04 \\
3828 & KOI-981 & 26 & 0.05 & 0.01 & 0.5 & 0.03 & 0.06 & 0.05 & 0.02 & 0.02 & 0.03 & 0.01 & 0.02 & 0.02 & 0.04 & 0.02 & 0.02 & 0.01 & 0.01 & 0.03 \\
3829 & KOI-3946 & 27 & 0.05 & 0.01 & 0.5 & 0.03 & 0.08 & 0.06 & 0.03 & 0.02 & 0.04 & 0.02 & 0.02 & 0.02 & 0.04 & 0.02 & 0.03 & 0.02 & 0.02 & 0.04 \\
3830 & KOI-4580 & 27 & 0.05 & 0.01 & 0.5 & 0.03 & 0.08 & 0.06 & 0.03 & 0.02 & 0.04 & 0.02 & 0.02 & 0.02 & 0.04 & 0.02 & 0.03 & 0.02 & 0.02 & 0.04 \\
3831 & KOI-579 & 28 & 0.05 & 0.01 & 0.5 & 0.03 & 0.08 & 0.06 & 0.03 & 0.02 & 0.04 & 0.02 & 0.03 & 0.02 & 0.04 & 0.02 & 0.03 & 0.02 & 0.02 & 0.04 \\
3832 & KOI-2503 & 27 & 0.05 & 0.01 & 0.5 & 0.03 & 0.07 & 0.06 & 0.03 & 0.02 & 0.04 & 0.02 & 0.02 & 0.02 & 0.04 & 0.02 & 0.03 & 0.01 & 0.02 & 0.04 \\
3833 & KOI-1754 & 27 & 0.05 & 0.01 & 0.5 & 0.03 & 0.08 & 0.06 & 0.03 & 0.02 & 0.04 & 0.02 & 0.02 & 0.02 & 0.04 & 0.02 & 0.03 & 0.02 & 0.02 & 0.04 \\
3834 & KOI-2111 & 30 & 0.06 & 0.02 & 0.6 & 0.04 & 0.10 & 0.07 & 0.04 & 0.03 & 0.05 & 0.03 & 0.03 & 0.03 & 0.05 & 0.02 & 0.04 & 0.02 & 0.02 & 0.05 \\
3835 & KOI-4775 & 27 & 0.05 & 0.01 & 0.5 & 0.03 & 0.07 & 0.06 & 0.03 & 0.02 & 0.04 & 0.02 & 0.02 & 0.02 & 0.04 & 0.02 & 0.03 & 0.01 & 0.02 & 0.04 \\
3836 & KOI-2414 & 27 & 0.05 & 0.01 & 0.5 & 0.03 & 0.08 & 0.06 & 0.03 & 0.02 & 0.04 & 0.02 & 0.02 & 0.02 & 0.04 & 0.02 & 0.03 & 0.02 & 0.02 & 0.04 \\
3837 & KOI-1279 & 27 & 0.05 & 0.01 & 0.5 & 0.03 & 0.08 & 0.06 & 0.03 & 0.02 & 0.04 & 0.02 & 0.02 & 0.02 & 0.04 & 0.02 & 0.03 & 0.02 & 0.02 & 0.04 \\
3838 & KOI-1271 & 27 & 0.05 & 0.01 & 0.5 & 0.03 & 0.08 & 0.06 & 0.03 & 0.02 & 0.04 & 0.02 & 0.03 & 0.02 & 0.04 & 0.02 & 0.03 & 0.02 & 0.02 & 0.04 \\
3839 & KOI-1278 & 33 & 0.06 & 0.02 & 0.6 & 0.05 & 0.12 & 0.09 & 0.05 & 0.03 & 0.06 & 0.03 & 0.04 & 0.03 & 0.06 & 0.03 & 0.04 & 0.02 & 0.03 & 0.06 \\
3840 & Kepler-282 & 29 & 0.06 & 0.02 & 0.6 & 0.04 & 0.09 & 0.07 & 0.04 & 0.02 & 0.05 & 0.02 & 0.03 & 0.02 & 0.05 & 0.02 & 0.04 & 0.02 & 0.02 & 0.05 \\
3841 & KOI-1891 & 29 & 0.06 & 0.02 & 0.6 & 0.04 & 0.09 & 0.07 & 0.04 & 0.02 & 0.05 & 0.03 & 0.03 & 0.02 & 0.05 & 0.02 & 0.04 & 0.02 & 0.02 & 0.05 \\
3842 & KOI-4066 & 27 & 0.05 & 0.01 & 0.5 & 0.03 & 0.08 & 0.06 & 0.03 & 0.02 & 0.04 & 0.02 & 0.02 & 0.02 & 0.04 & 0.02 & 0.03 & 0.02 & 0.02 & 0.04 \\
3843 & KOI-2758 & 27 & 0.05 & 0.01 & 0.5 & 0.03 & 0.07 & 0.06 & 0.03 & 0.02 & 0.04 & 0.02 & 0.02 & 0.02 & 0.04 & 0.02 & 0.03 & 0.02 & 0.02 & 0.04 \\
3844 & KOI-1283 & 27 & 0.05 & 0.01 & 0.5 & 0.03 & 0.08 & 0.06 & 0.03 & 0.02 & 0.04 & 0.02 & 0.02 & 0.02 & 0.04 & 0.02 & 0.03 & 0.02 & 0.02 & 0.04 \\
3845 & KOI-105 & 26 & 0.05 & 0.01 & 0.5 & 0.03 & 0.07 & 0.05 & 0.03 & 0.02 & 0.04 & 0.02 & 0.02 & 0.02 & 0.04 & 0.02 & 0.03 & 0.01 & 0.02 & 0.04 \\
3846 & KOI-921 & 29 & 0.06 & 0.02 & 0.6 & 0.04 & 0.10 & 0.07 & 0.04 & 0.02 & 0.05 & 0.03 & 0.03 & 0.02 & 0.05 & 0.02 & 0.04 & 0.02 & 0.02 & 0.05 \\
3847 & KOI-172 & 27 & 0.05 & 0.01 & 0.5 & 0.03 & 0.08 & 0.06 & 0.03 & 0.02 & 0.04 & 0.02 & 0.02 & 0.02 & 0.04 & 0.02 & 0.03 & 0.02 & 0.02 & 0.04 \\
3848 & KOI-319 & 27 & 0.05 & 0.01 & 0.5 & 0.03 & 0.08 & 0.06 & 0.03 & 0.02 & 0.04 & 0.02 & 0.02 & 0.02 & 0.04 & 0.02 & 0.03 & 0.02 & 0.02 & 0.04 \\
3849 & KOI-374 & 27 & 0.05 & 0.01 & 0.5 & 0.03 & 0.08 & 0.06 & 0.03 & 0.02 & 0.04 & 0.02 & 0.02 & 0.02 & 0.04 & 0.02 & 0.03 & 0.02 & 0.02 & 0.04 \\
3850 & KOI-1629 & 27 & 0.05 & 0.01 & 0.5 & 0.03 & 0.08 & 0.06 & 0.03 & 0.02 & 0.04 & 0.02 & 0.02 & 0.02 & 0.04 & 0.02 & 0.03 & 0.02 & 0.02 & 0.04 \\
3851 & KOI-2749 & 27 & 0.05 & 0.01 & 0.5 & 0.03 & 0.08 & 0.06 & 0.03 & 0.02 & 0.04 & 0.02 & 0.03 & 0.02 & 0.04 & 0.02 & 0.03 & 0.02 & 0.02 & 0.04 \\
3852 & KOI-2473 & 31 & 0.06 & 0.02 & 0.6 & 0.04 & 0.11 & 0.08 & 0.04 & 0.03 & 0.06 & 0.03 & 0.03 & 0.03 & 0.05 & 0.02 & 0.04 & 0.02 & 0.03 & 0.05 \\
3853 & KOI-3891 & 27 & 0.05 & 0.01 & 0.5 & 0.03 & 0.07 & 0.06 & 0.03 & 0.02 & 0.04 & 0.02 & 0.02 & 0.02 & 0.04 & 0.02 & 0.03 & 0.02 & 0.02 & 0.04 \\
3854 & KOI-4301 & 29 & 0.06 & 0.02 & 0.5 & 0.04 & 0.09 & 0.07 & 0.04 & 0.02 & 0.05 & 0.02 & 0.03 & 0.02 & 0.05 & 0.02 & 0.03 & 0.02 & 0.02 & 0.05 \\
3855 & KOI-1257 & 31 & 0.06 & 0.02 & 0.6 & 0.04 & 0.11 & 0.08 & 0.04 & 0.03 & 0.06 & 0.03 & 0.03 & 0.03 & 0.05 & 0.02 & 0.04 & 0.02 & 0.02 & 0.05 \\
3856 & KOI-2017 & 27 & 0.05 & 0.01 & 0.5 & 0.03 & 0.08 & 0.06 & 0.03 & 0.02 & 0.04 & 0.02 & 0.02 & 0.02 & 0.04 & 0.02 & 0.03 & 0.02 & 0.02 & 0.04 \\
3857 & KOI-1904 & 28 & 0.06 & 0.02 & 0.5 & 0.04 & 0.08 & 0.06 & 0.03 & 0.02 & 0.05 & 0.02 & 0.03 & 0.02 & 0.05 & 0.02 & 0.03 & 0.02 & 0.02 & 0.04 \\
3858 & KOI-4251 & 27 & 0.05 & 0.01 & 0.5 & 0.03 & 0.08 & 0.06 & 0.03 & 0.02 & 0.04 & 0.02 & 0.02 & 0.02 & 0.04 & 0.02 & 0.03 & 0.02 & 0.02 & 0.04 \\
3859 & KOI-2159 & 28 & 0.05 & 0.01 & 0.5 & 0.04 & 0.08 & 0.06 & 0.03 & 0.02 & 0.05 & 0.02 & 0.03 & 0.02 & 0.04 & 0.02 & 0.03 & 0.02 & 0.02 & 0.04 \\
3860 & KOI-694 & 27 & 0.05 & 0.01 & 0.5 & 0.03 & 0.08 & 0.06 & 0.03 & 0.02 & 0.04 & 0.02 & 0.03 & 0.02 & 0.04 & 0.02 & 0.03 & 0.02 & 0.02 & 0.04 \\
3861 & KOI-2039 & 30 & 0.06 & 0.02 & 0.6 & 0.04 & 0.10 & 0.08 & 0.04 & 0.03 & 0.05 & 0.03 & 0.03 & 0.03 & 0.05 & 0.02 & 0.04 & 0.02 & 0.02 & 0.05 \\
3862 & KOI-1850 & 28 & 0.05 & 0.01 & 0.5 & 0.03 & 0.08 & 0.06 & 0.03 & 0.02 & 0.04 & 0.02 & 0.03 & 0.02 & 0.04 & 0.02 & 0.03 & 0.02 & 0.02 & 0.04 \\
3863 & KOI-1276 & 29 & 0.06 & 0.02 & 0.6 & 0.04 & 0.10 & 0.07 & 0.04 & 0.02 & 0.05 & 0.03 & 0.03 & 0.02 & 0.05 & 0.02 & 0.04 & 0.02 & 0.02 & 0.05 \\
3864 & KOI-695 & 27 & 0.05 & 0.01 & 0.5 & 0.03 & 0.08 & 0.06 & 0.03 & 0.02 & 0.04 & 0.02 & 0.02 & 0.02 & 0.04 & 0.02 & 0.03 & 0.02 & 0.02 & 0.04 \\
3865 & KOI-3052 & 27 & 0.05 & 0.01 & 0.5 & 0.03 & 0.08 & 0.06 & 0.03 & 0.02 & 0.04 & 0.02 & 0.02 & 0.02 & 0.04 & 0.02 & 0.03 & 0.02 & 0.02 & 0.04 \\
3866 & KOI-2956 & 27 & 0.05 & 0.01 & 0.5 & 0.03 & 0.08 & 0.06 & 0.03 & 0.02 & 0.04 & 0.02 & 0.02 & 0.02 & 0.04 & 0.02 & 0.03 & 0.02 & 0.02 & 0.04 \\
3867 & KOI-3886 & 26 & 0.05 & 0.01 & 0.5 & 0.03 & 0.07 & 0.05 & 0.03 & 0.02 & 0.04 & 0.02 & 0.02 & 0.02 & 0.04 & 0.02 & 0.03 & 0.01 & 0.02 & 0.04 \\
3868 & KOI-1274 & 27 & 0.05 & 0.01 & 0.5 & 0.03 & 0.08 & 0.06 & 0.03 & 0.02 & 0.04 & 0.02 & 0.02 & 0.02 & 0.04 & 0.02 & 0.03 & 0.02 & 0.02 & 0.04 \\
3869 & KOI-4811 & 28 & 0.05 & 0.01 & 0.5 & 0.04 & 0.08 & 0.06 & 0.03 & 0.02 & 0.04 & 0.02 & 0.03 & 0.02 & 0.04 & 0.02 & 0.03 & 0.02 & 0.02 & 0.04 \\
3870 & KOI-2659 & 27 & 0.05 & 0.01 & 0.5 & 0.03 & 0.07 & 0.06 & 0.03 & 0.02 & 0.04 & 0.02 & 0.02 & 0.02 & 0.04 & 0.02 & 0.03 & 0.01 & 0.02 & 0.04 \\
3871 & KOI-464 & 31 & 0.06 & 0.02 & 0.6 & 0.04 & 0.11 & 0.08 & 0.04 & 0.03 & 0.06 & 0.03 & 0.04 & 0.03 & 0.05 & 0.02 & 0.04 & 0.02 & 0.03 & 0.05 \\
3872 & KOI-3541 & 27 & 0.05 & 0.01 & 0.5 & 0.03 & 0.08 & 0.06 & 0.03 & 0.02 & 0.04 & 0.02 & 0.02 & 0.02 & 0.04 & 0.02 & 0.03 & 0.02 & 0.02 & 0.04 \\
3873 & KOI-2641 & 27 & 0.05 & 0.01 & 0.5 & 0.03 & 0.08 & 0.06 & 0.03 & 0.02 & 0.04 & 0.02 & 0.02 & 0.02 & 0.04 & 0.02 & 0.03 & 0.02 & 0.02 & 0.04 \\
3874 & KOI-465 & 29 & 0.06 & 0.02 & 0.6 & 0.04 & 0.09 & 0.07 & 0.04 & 0.02 & 0.05 & 0.03 & 0.03 & 0.02 & 0.05 & 0.02 & 0.04 & 0.02 & 0.02 & 0.05 \\
3875 & KOI-697 & 27 & 0.05 & 0.01 & 0.5 & 0.03 & 0.08 & 0.06 & 0.03 & 0.02 & 0.04 & 0.02 & 0.02 & 0.02 & 0.04 & 0.02 & 0.03 & 0.02 & 0.02 & 0.04 \\
3876 & KOI-4269 & 27 & 0.05 & 0.01 & 0.5 & 0.03 & 0.07 & 0.06 & 0.03 & 0.02 & 0.04 & 0.02 & 0.02 & 0.02 & 0.04 & 0.02 & 0.03 & 0.01 & 0.02 & 0.04 \\
3877 & WASP-58 & 25 & 0.05 & 0.01 & 0.5 & 0.03 & 0.04 & 0.04 & 0.01 & 0.01 & 0.03 & 0.01 & 0.01 & 0.01 & 0.03 & 0.01 & 0.02 & 0.01 & 0.01 & 0.03 \\
3878 & KOI-3473 & 28 & 0.05 & 0.02 & 0.5 & 0.04 & 0.08 & 0.06 & 0.03 & 0.02 & 0.05 & 0.02 & 0.03 & 0.02 & 0.04 & 0.02 & 0.03 & 0.02 & 0.02 & 0.04 \\
3879 & KOI-698 & 28 & 0.05 & 0.01 & 0.5 & 0.03 & 0.08 & 0.06 & 0.03 & 0.02 & 0.04 & 0.02 & 0.03 & 0.02 & 0.04 & 0.02 & 0.03 & 0.02 & 0.02 & 0.04 \\
3880 & KOI-2595 & 28 & 0.05 & 0.01 & 0.5 & 0.04 & 0.08 & 0.06 & 0.03 & 0.02 & 0.04 & 0.02 & 0.03 & 0.02 & 0.04 & 0.02 & 0.03 & 0.02 & 0.02 & 0.04 \\
3881 & KOI-2517 & 30 & 0.06 & 0.02 & 0.6 & 0.04 & 0.10 & 0.07 & 0.04 & 0.03 & 0.05 & 0.03 & 0.03 & 0.03 & 0.05 & 0.02 & 0.04 & 0.02 & 0.02 & 0.05 \\
3882 & KOI-700 & 28 & 0.05 & 0.01 & 0.5 & 0.03 & 0.08 & 0.06 & 0.03 & 0.02 & 0.04 & 0.02 & 0.03 & 0.02 & 0.04 & 0.02 & 0.03 & 0.02 & 0.02 & 0.04 \\
3883 & Kepler-215 & 26 & 0.05 & 0.01 & 0.5 & 0.03 & 0.06 & 0.05 & 0.02 & 0.02 & 0.04 & 0.02 & 0.02 & 0.02 & 0.04 & 0.02 & 0.03 & 0.01 & 0.02 & 0.04 \\
3884 & KOI-1412 & 27 & 0.05 & 0.01 & 0.5 & 0.03 & 0.08 & 0.06 & 0.03 & 0.02 & 0.04 & 0.02 & 0.02 & 0.02 & 0.04 & 0.02 & 0.03 & 0.02 & 0.02 & 0.04 \\
3885 & KOI-159 & 27 & 0.05 & 0.01 & 0.5 & 0.03 & 0.08 & 0.06 & 0.03 & 0.02 & 0.04 & 0.02 & 0.02 & 0.02 & 0.04 & 0.02 & 0.03 & 0.02 & 0.02 & 0.04 \\
3886 & KOI-2038 & 34 & 0.06 & 0.02 & 0.6 & 0.05 & 0.13 & 0.10 & 0.05 & 0.03 & 0.07 & 0.04 & 0.04 & 0.03 & 0.06 & 0.03 & 0.05 & 0.03 & 0.03 & 0.06 \\
3887 & KOI-3227 & 27 & 0.05 & 0.01 & 0.5 & 0.03 & 0.08 & 0.06 & 0.03 & 0.02 & 0.04 & 0.02 & 0.03 & 0.02 & 0.04 & 0.02 & 0.03 & 0.02 & 0.02 & 0.04 \\
3888 & KOI-4585 & 28 & 0.05 & 0.01 & 0.5 & 0.04 & 0.08 & 0.06 & 0.03 & 0.02 & 0.04 & 0.02 & 0.03 & 0.02 & 0.04 & 0.02 & 0.03 & 0.02 & 0.02 & 0.04 \\
3889 & KOI-582 & 29 & 0.06 & 0.02 & 0.6 & 0.04 & 0.10 & 0.07 & 0.04 & 0.02 & 0.05 & 0.03 & 0.03 & 0.02 & 0.05 & 0.02 & 0.04 & 0.02 & 0.02 & 0.05 \\
3890 & KOI-2319 & 28 & 0.05 & 0.01 & 0.5 & 0.04 & 0.08 & 0.06 & 0.03 & 0.02 & 0.05 & 0.02 & 0.03 & 0.02 & 0.04 & 0.02 & 0.03 & 0.02 & 0.02 & 0.04 \\
3891 & KOI-3196 & 26 & 0.05 & 0.01 & 0.5 & 0.03 & 0.06 & 0.05 & 0.02 & 0.02 & 0.03 & 0.01 & 0.02 & 0.02 & 0.04 & 0.02 & 0.02 & 0.01 & 0.01 & 0.03 \\
3892 & KOI-2530 & 27 & 0.05 & 0.01 & 0.5 & 0.03 & 0.08 & 0.06 & 0.03 & 0.02 & 0.04 & 0.02 & 0.03 & 0.02 & 0.04 & 0.02 & 0.03 & 0.02 & 0.02 & 0.04 \\
3893 & KOI-2768 & 30 & 0.06 & 0.02 & 0.6 & 0.04 & 0.10 & 0.07 & 0.04 & 0.03 & 0.05 & 0.03 & 0.03 & 0.03 & 0.05 & 0.02 & 0.04 & 0.02 & 0.02 & 0.05 \\
3894 & KOI-4014 & 28 & 0.06 & 0.02 & 0.5 & 0.04 & 0.09 & 0.07 & 0.03 & 0.02 & 0.05 & 0.02 & 0.03 & 0.02 & 0.05 & 0.02 & 0.03 & 0.02 & 0.02 & 0.04 \\
3895 & KOI-134 & 28 & 0.06 & 0.02 & 0.5 & 0.04 & 0.09 & 0.06 & 0.03 & 0.02 & 0.05 & 0.02 & 0.03 & 0.02 & 0.05 & 0.02 & 0.03 & 0.02 & 0.02 & 0.04 \\
3896 & KOI-1413 & 29 & 0.06 & 0.02 & 0.6 & 0.04 & 0.10 & 0.07 & 0.04 & 0.02 & 0.05 & 0.03 & 0.03 & 0.02 & 0.05 & 0.02 & 0.04 & 0.02 & 0.02 & 0.05 \\
3897 & KOI-1616 & 27 & 0.05 & 0.01 & 0.5 & 0.03 & 0.08 & 0.06 & 0.03 & 0.02 & 0.04 & 0.02 & 0.02 & 0.02 & 0.04 & 0.02 & 0.03 & 0.02 & 0.02 & 0.04 \\
3898 & KOI-2564 & 27 & 0.05 & 0.01 & 0.5 & 0.03 & 0.08 & 0.06 & 0.03 & 0.02 & 0.04 & 0.02 & 0.02 & 0.02 & 0.04 & 0.02 & 0.03 & 0.02 & 0.02 & 0.04 \\
3899 & KOI-2175 & 27 & 0.05 & 0.01 & 0.5 & 0.03 & 0.08 & 0.06 & 0.03 & 0.02 & 0.04 & 0.02 & 0.02 & 0.02 & 0.04 & 0.02 & 0.03 & 0.02 & 0.02 & 0.04 \\
3900 & KOI-2833 & 28 & 0.05 & 0.01 & 0.5 & 0.04 & 0.08 & 0.06 & 0.03 & 0.02 & 0.04 & 0.02 & 0.03 & 0.02 & 0.04 & 0.02 & 0.03 & 0.02 & 0.02 & 0.04 \\
3901 & KOI-2367 & 27 & 0.05 & 0.01 & 0.5 & 0.03 & 0.08 & 0.06 & 0.03 & 0.02 & 0.04 & 0.02 & 0.02 & 0.02 & 0.04 & 0.02 & 0.03 & 0.02 & 0.02 & 0.04 \\
3902 & KOI-2470 & 27 & 0.05 & 0.01 & 0.5 & 0.03 & 0.08 & 0.06 & 0.03 & 0.02 & 0.04 & 0.02 & 0.02 & 0.02 & 0.04 & 0.02 & 0.03 & 0.02 & 0.02 & 0.04 \\
3903 & KOI-3008 & 27 & 0.05 & 0.01 & 0.5 & 0.03 & 0.08 & 0.06 & 0.03 & 0.02 & 0.04 & 0.02 & 0.03 & 0.02 & 0.04 & 0.02 & 0.03 & 0.02 & 0.02 & 0.04 \\
3904 & KOI-2640 & 27 & 0.05 & 0.01 & 0.5 & 0.03 & 0.07 & 0.06 & 0.03 & 0.02 & 0.04 & 0.02 & 0.02 & 0.02 & 0.04 & 0.02 & 0.03 & 0.02 & 0.02 & 0.04 \\
3905 & KOI-4060 & 29 & 0.06 & 0.02 & 0.6 & 0.04 & 0.09 & 0.07 & 0.04 & 0.02 & 0.05 & 0.02 & 0.03 & 0.02 & 0.05 & 0.02 & 0.03 & 0.02 & 0.02 & 0.05 \\
3906 & KOI-3249 & 27 & 0.05 & 0.01 & 0.5 & 0.03 & 0.08 & 0.06 & 0.03 & 0.02 & 0.04 & 0.02 & 0.02 & 0.02 & 0.04 & 0.02 & 0.03 & 0.02 & 0.02 & 0.04 \\
3907 & HAT-P-40 & 25 & 0.05 & 0.01 & 0.5 & 0.03 & 0.04 & 0.04 & 0.01 & 0.01 & 0.03 & 0.01 & 0.01 & 0.01 & 0.03 & 0.01 & 0.02 & 0.01 & 0.01 & 0.03 \\
3908 & KOI-4839 & 27 & 0.05 & 0.01 & 0.5 & 0.03 & 0.08 & 0.06 & 0.03 & 0.02 & 0.04 & 0.02 & 0.02 & 0.02 & 0.04 & 0.02 & 0.03 & 0.02 & 0.02 & 0.04 \\
3909 & KOI-4198 & 27 & 0.05 & 0.01 & 0.5 & 0.03 & 0.08 & 0.06 & 0.03 & 0.02 & 0.04 & 0.02 & 0.02 & 0.02 & 0.04 & 0.02 & 0.03 & 0.02 & 0.02 & 0.04 \\
3910 & KOI-3087 & 27 & 0.05 & 0.01 & 0.5 & 0.03 & 0.07 & 0.06 & 0.03 & 0.02 & 0.04 & 0.02 & 0.02 & 0.02 & 0.04 & 0.02 & 0.03 & 0.01 & 0.02 & 0.04 \\
3911 & KOI-3425 & 27 & 0.05 & 0.01 & 0.5 & 0.03 & 0.08 & 0.06 & 0.03 & 0.02 & 0.04 & 0.02 & 0.02 & 0.02 & 0.04 & 0.02 & 0.03 & 0.02 & 0.02 & 0.04 \\
3912 & KOI-2874 & 30 & 0.06 & 0.02 & 0.6 & 0.04 & 0.10 & 0.07 & 0.04 & 0.03 & 0.05 & 0.03 & 0.03 & 0.03 & 0.05 & 0.02 & 0.04 & 0.02 & 0.02 & 0.05 \\
3913 & KOI-323 & 27 & 0.05 & 0.01 & 0.5 & 0.03 & 0.08 & 0.06 & 0.03 & 0.02 & 0.04 & 0.02 & 0.02 & 0.02 & 0.04 & 0.02 & 0.03 & 0.02 & 0.02 & 0.04 \\
3914 & KOI-703 & 27 & 0.05 & 0.01 & 0.5 & 0.03 & 0.08 & 0.06 & 0.03 & 0.02 & 0.04 & 0.02 & 0.02 & 0.02 & 0.04 & 0.02 & 0.03 & 0.02 & 0.02 & 0.04 \\
3915 & KOI-2522 & 27 & 0.05 & 0.01 & 0.5 & 0.03 & 0.07 & 0.06 & 0.03 & 0.02 & 0.04 & 0.02 & 0.02 & 0.02 & 0.04 & 0.02 & 0.03 & 0.01 & 0.02 & 0.04 \\
3916 & KOI-584 & 27 & 0.05 & 0.01 & 0.5 & 0.03 & 0.08 & 0.06 & 0.03 & 0.02 & 0.04 & 0.02 & 0.03 & 0.02 & 0.04 & 0.02 & 0.03 & 0.02 & 0.02 & 0.04 \\
3917 & Kepler-192 & 26 & 0.05 & 0.01 & 0.5 & 0.03 & 0.07 & 0.05 & 0.02 & 0.02 & 0.04 & 0.02 & 0.02 & 0.02 & 0.04 & 0.02 & 0.03 & 0.01 & 0.02 & 0.04 \\
3918 & KOI-4222 & 28 & 0.05 & 0.01 & 0.5 & 0.04 & 0.08 & 0.06 & 0.03 & 0.02 & 0.05 & 0.02 & 0.03 & 0.02 & 0.04 & 0.02 & 0.03 & 0.02 & 0.02 & 0.04 \\
3919 & KOI-2443 & 28 & 0.05 & 0.01 & 0.5 & 0.04 & 0.08 & 0.06 & 0.03 & 0.02 & 0.04 & 0.02 & 0.03 & 0.02 & 0.04 & 0.02 & 0.03 & 0.02 & 0.02 & 0.04 \\
3920 & KOI-2281 & 27 & 0.05 & 0.01 & 0.5 & 0.03 & 0.07 & 0.06 & 0.03 & 0.02 & 0.04 & 0.02 & 0.02 & 0.02 & 0.04 & 0.02 & 0.03 & 0.01 & 0.02 & 0.04 \\
3921 & KOI-2162 & 27 & 0.05 & 0.01 & 0.5 & 0.03 & 0.08 & 0.06 & 0.03 & 0.02 & 0.04 & 0.02 & 0.03 & 0.02 & 0.04 & 0.02 & 0.03 & 0.02 & 0.02 & 0.04 \\
3922 & KOI-4318 & 27 & 0.05 & 0.01 & 0.5 & 0.03 & 0.08 & 0.06 & 0.03 & 0.02 & 0.04 & 0.02 & 0.02 & 0.02 & 0.04 & 0.02 & 0.03 & 0.02 & 0.02 & 0.04 \\
3923 & KOI-704 & 27 & 0.05 & 0.01 & 0.5 & 0.03 & 0.08 & 0.06 & 0.03 & 0.02 & 0.04 & 0.02 & 0.02 & 0.02 & 0.04 & 0.02 & 0.03 & 0.02 & 0.02 & 0.04 \\
3924 & KOI-2657 & 27 & 0.05 & 0.01 & 0.5 & 0.03 & 0.08 & 0.06 & 0.03 & 0.02 & 0.04 & 0.02 & 0.02 & 0.02 & 0.04 & 0.02 & 0.03 & 0.02 & 0.02 & 0.04 \\
3925 & KOI-3114 & 27 & 0.05 & 0.01 & 0.5 & 0.03 & 0.08 & 0.06 & 0.03 & 0.02 & 0.04 & 0.02 & 0.03 & 0.02 & 0.04 & 0.02 & 0.03 & 0.02 & 0.02 & 0.04 \\
3926 & KOI-3867 & 31 & 0.06 & 0.02 & 0.6 & 0.04 & 0.11 & 0.08 & 0.05 & 0.03 & 0.06 & 0.03 & 0.04 & 0.03 & 0.05 & 0.02 & 0.04 & 0.02 & 0.03 & 0.06 \\
3927 & KOI-4215 & 29 & 0.06 & 0.02 & 0.6 & 0.04 & 0.09 & 0.07 & 0.04 & 0.02 & 0.05 & 0.02 & 0.03 & 0.02 & 0.05 & 0.02 & 0.03 & 0.02 & 0.02 & 0.05 \\
3928 & KOI-2137 & 28 & 0.05 & 0.01 & 0.5 & 0.04 & 0.08 & 0.06 & 0.03 & 0.02 & 0.05 & 0.02 & 0.03 & 0.02 & 0.04 & 0.02 & 0.03 & 0.02 & 0.02 & 0.04 \\
3929 & KOI-1411 & 27 & 0.05 & 0.01 & 0.5 & 0.03 & 0.07 & 0.06 & 0.03 & 0.02 & 0.04 & 0.02 & 0.02 & 0.02 & 0.04 & 0.02 & 0.03 & 0.02 & 0.02 & 0.04 \\
3930 & KOI-4640 & 27 & 0.05 & 0.01 & 0.5 & 0.03 & 0.08 & 0.06 & 0.03 & 0.02 & 0.04 & 0.02 & 0.02 & 0.02 & 0.04 & 0.02 & 0.03 & 0.02 & 0.02 & 0.04 \\
3931 & KOI-1922 & 31 & 0.06 & 0.02 & 0.6 & 0.04 & 0.11 & 0.08 & 0.05 & 0.03 & 0.06 & 0.03 & 0.04 & 0.03 & 0.05 & 0.02 & 0.04 & 0.02 & 0.03 & 0.05 \\
3932 & KOI-974 & 27 & 0.05 & 0.01 & 0.5 & 0.03 & 0.08 & 0.06 & 0.03 & 0.02 & 0.04 & 0.02 & 0.03 & 0.02 & 0.04 & 0.02 & 0.03 & 0.02 & 0.02 & 0.04 \\
3933 & KOI-1835 & 27 & 0.05 & 0.01 & 0.5 & 0.03 & 0.07 & 0.06 & 0.03 & 0.02 & 0.04 & 0.02 & 0.02 & 0.02 & 0.04 & 0.02 & 0.03 & 0.01 & 0.02 & 0.04 \\
3934 & KOI-707 & 27 & 0.05 & 0.01 & 0.5 & 0.03 & 0.08 & 0.06 & 0.03 & 0.02 & 0.04 & 0.02 & 0.03 & 0.02 & 0.04 & 0.02 & 0.03 & 0.02 & 0.02 & 0.04 \\
3935 & Kepler-33 & 26 & 0.05 & 0.01 & 0.5 & 0.03 & 0.07 & 0.05 & 0.03 & 0.02 & 0.04 & 0.02 & 0.02 & 0.02 & 0.04 & 0.02 & 0.03 & 0.01 & 0.02 & 0.04 \\
3936 & KOI-2079 & 27 & 0.05 & 0.01 & 0.5 & 0.03 & 0.08 & 0.06 & 0.03 & 0.02 & 0.04 & 0.02 & 0.02 & 0.02 & 0.04 & 0.02 & 0.03 & 0.02 & 0.02 & 0.04 \\
3937 & KOI-2786 & 28 & 0.05 & 0.01 & 0.5 & 0.03 & 0.08 & 0.06 & 0.03 & 0.02 & 0.04 & 0.02 & 0.03 & 0.02 & 0.04 & 0.02 & 0.03 & 0.02 & 0.02 & 0.04 \\
3938 & KOI-941 & 34 & 0.06 & 0.02 & 0.6 & 0.05 & 0.13 & 0.10 & 0.05 & 0.03 & 0.07 & 0.04 & 0.04 & 0.03 & 0.06 & 0.03 & 0.05 & 0.03 & 0.03 & 0.06 \\
3939 & Kepler-127 & 25 & 0.05 & 0.01 & 0.5 & 0.03 & 0.04 & 0.04 & 0.01 & 0.01 & 0.03 & 0.01 & 0.01 & 0.01 & 0.03 & 0.01 & 0.02 & 0.01 & 0.01 & 0.03 \\
3940 & KOI-271 & 27 & 0.05 & 0.01 & 0.5 & 0.03 & 0.08 & 0.06 & 0.03 & 0.02 & 0.04 & 0.02 & 0.02 & 0.02 & 0.04 & 0.02 & 0.03 & 0.02 & 0.02 & 0.04 \\
3941 & KOI-4637 & 27 & 0.05 & 0.01 & 0.5 & 0.03 & 0.08 & 0.06 & 0.03 & 0.02 & 0.04 & 0.02 & 0.02 & 0.02 & 0.04 & 0.02 & 0.03 & 0.02 & 0.02 & 0.04 \\
3942 & KOI-2029 & 27 & 0.05 & 0.01 & 0.5 & 0.03 & 0.07 & 0.06 & 0.03 & 0.02 & 0.04 & 0.02 & 0.02 & 0.02 & 0.04 & 0.02 & 0.03 & 0.01 & 0.02 & 0.04 \\
3943 & KOI-2694 & 31 & 0.06 & 0.02 & 0.6 & 0.04 & 0.11 & 0.08 & 0.04 & 0.03 & 0.06 & 0.03 & 0.03 & 0.03 & 0.05 & 0.02 & 0.04 & 0.02 & 0.02 & 0.05 \\
3944 & KOI-2246 & 27 & 0.05 & 0.01 & 0.5 & 0.03 & 0.08 & 0.06 & 0.03 & 0.02 & 0.04 & 0.02 & 0.02 & 0.02 & 0.04 & 0.02 & 0.03 & 0.02 & 0.02 & 0.04 \\
3945 & KOI-119 & 27 & 0.05 & 0.01 & 0.5 & 0.03 & 0.08 & 0.06 & 0.03 & 0.02 & 0.04 & 0.02 & 0.02 & 0.02 & 0.04 & 0.02 & 0.03 & 0.02 & 0.02 & 0.04 \\
3946 & KOI-110 & 28 & 0.05 & 0.01 & 0.5 & 0.03 & 0.08 & 0.06 & 0.03 & 0.02 & 0.04 & 0.02 & 0.03 & 0.02 & 0.04 & 0.02 & 0.03 & 0.02 & 0.02 & 0.04 \\
3947 & KOI-1813 & 28 & 0.05 & 0.01 & 0.5 & 0.04 & 0.08 & 0.06 & 0.03 & 0.02 & 0.04 & 0.02 & 0.03 & 0.02 & 0.04 & 0.02 & 0.03 & 0.02 & 0.02 & 0.04 \\
3948 & KOI-2082 & 27 & 0.05 & 0.01 & 0.5 & 0.03 & 0.08 & 0.06 & 0.03 & 0.02 & 0.04 & 0.02 & 0.03 & 0.02 & 0.04 & 0.02 & 0.03 & 0.02 & 0.02 & 0.04 \\
3949 & KOI-939 & 34 & 0.06 & 0.02 & 0.6 & 0.05 & 0.13 & 0.10 & 0.05 & 0.03 & 0.07 & 0.04 & 0.04 & 0.03 & 0.06 & 0.03 & 0.05 & 0.03 & 0.03 & 0.06 \\
3950 & KOI-2717 & 27 & 0.05 & 0.01 & 0.5 & 0.03 & 0.08 & 0.06 & 0.03 & 0.02 & 0.04 & 0.02 & 0.02 & 0.02 & 0.04 & 0.02 & 0.03 & 0.02 & 0.02 & 0.04 \\
3951 & KOI-1978 & 30 & 0.06 & 0.02 & 0.6 & 0.04 & 0.10 & 0.08 & 0.04 & 0.03 & 0.05 & 0.03 & 0.03 & 0.03 & 0.05 & 0.02 & 0.04 & 0.02 & 0.02 & 0.05 \\
3952 & KOI-708 & 27 & 0.05 & 0.01 & 0.5 & 0.03 & 0.08 & 0.06 & 0.03 & 0.02 & 0.04 & 0.02 & 0.02 & 0.02 & 0.04 & 0.02 & 0.03 & 0.02 & 0.02 & 0.04 \\
3953 & KOI-3132 & 28 & 0.05 & 0.01 & 0.5 & 0.03 & 0.08 & 0.06 & 0.03 & 0.02 & 0.04 & 0.02 & 0.03 & 0.02 & 0.04 & 0.02 & 0.03 & 0.02 & 0.02 & 0.04 \\
3954 & KOI-49 & 27 & 0.05 & 0.01 & 0.5 & 0.03 & 0.08 & 0.06 & 0.03 & 0.02 & 0.04 & 0.02 & 0.02 & 0.02 & 0.04 & 0.02 & 0.03 & 0.02 & 0.02 & 0.04 \\
3955 & KOI-1806 & 28 & 0.05 & 0.02 & 0.5 & 0.04 & 0.08 & 0.06 & 0.03 & 0.02 & 0.05 & 0.02 & 0.03 & 0.02 & 0.05 & 0.02 & 0.03 & 0.02 & 0.02 & 0.04 \\
3956 & KOI-165 & 27 & 0.05 & 0.01 & 0.5 & 0.03 & 0.07 & 0.06 & 0.03 & 0.02 & 0.04 & 0.02 & 0.02 & 0.02 & 0.04 & 0.02 & 0.03 & 0.02 & 0.02 & 0.04 \\
3957 & KOI-1886 & 27 & 0.05 & 0.01 & 0.5 & 0.03 & 0.08 & 0.06 & 0.03 & 0.02 & 0.04 & 0.02 & 0.03 & 0.02 & 0.04 & 0.02 & 0.03 & 0.02 & 0.02 & 0.04 \\
3958 & KOI-709 & 27 & 0.05 & 0.01 & 0.5 & 0.03 & 0.08 & 0.06 & 0.03 & 0.02 & 0.04 & 0.02 & 0.02 & 0.02 & 0.04 & 0.02 & 0.03 & 0.02 & 0.02 & 0.04 \\
3959 & KOI-3165 & 25 & 0.05 & 0.01 & 0.5 & 0.03 & 0.04 & 0.04 & 0.01 & 0.01 & 0.03 & 0.01 & 0.01 & 0.01 & 0.03 & 0.01 & 0.02 & 0.01 & 0.01 & 0.03 \\
3960 & KOI-3232 & 27 & 0.05 & 0.01 & 0.5 & 0.03 & 0.08 & 0.06 & 0.03 & 0.02 & 0.04 & 0.02 & 0.02 & 0.02 & 0.04 & 0.02 & 0.03 & 0.02 & 0.02 & 0.04 \\
3961 & KOI-288 & 27 & 0.05 & 0.01 & 0.5 & 0.03 & 0.08 & 0.06 & 0.03 & 0.02 & 0.04 & 0.02 & 0.02 & 0.02 & 0.04 & 0.02 & 0.03 & 0.02 & 0.02 & 0.04 \\
3962 & KOI-1819 & 27 & 0.05 & 0.01 & 0.5 & 0.03 & 0.08 & 0.06 & 0.03 & 0.02 & 0.04 & 0.02 & 0.02 & 0.02 & 0.04 & 0.02 & 0.03 & 0.02 & 0.02 & 0.04 \\
3963 & KOI-3229 & 27 & 0.05 & 0.01 & 0.5 & 0.03 & 0.08 & 0.06 & 0.03 & 0.02 & 0.04 & 0.02 & 0.02 & 0.02 & 0.04 & 0.02 & 0.03 & 0.02 & 0.02 & 0.04 \\
3964 & KOI-711 & 27 & 0.05 & 0.01 & 0.5 & 0.03 & 0.07 & 0.05 & 0.03 & 0.02 & 0.04 & 0.02 & 0.02 & 0.02 & 0.04 & 0.02 & 0.03 & 0.01 & 0.02 & 0.04 \\
3965 & KOI-115 & 26 & 0.05 & 0.01 & 0.5 & 0.03 & 0.06 & 0.05 & 0.02 & 0.02 & 0.04 & 0.01 & 0.02 & 0.02 & 0.04 & 0.02 & 0.02 & 0.01 & 0.02 & 0.04 \\
3966 & KOI-710 & 28 & 0.05 & 0.01 & 0.5 & 0.04 & 0.08 & 0.06 & 0.03 & 0.02 & 0.04 & 0.02 & 0.03 & 0.02 & 0.04 & 0.02 & 0.03 & 0.02 & 0.02 & 0.04 \\
3967 & Kepler-217 & 26 & 0.05 & 0.01 & 0.5 & 0.03 & 0.06 & 0.05 & 0.02 & 0.02 & 0.03 & 0.01 & 0.02 & 0.02 & 0.04 & 0.02 & 0.02 & 0.01 & 0.01 & 0.03 \\
3968 & KOI-2612 & 29 & 0.06 & 0.02 & 0.6 & 0.04 & 0.09 & 0.07 & 0.04 & 0.02 & 0.05 & 0.03 & 0.03 & 0.02 & 0.05 & 0.02 & 0.04 & 0.02 & 0.02 & 0.05 \\
3969 & KOI-2884 & 27 & 0.05 & 0.01 & 0.5 & 0.03 & 0.08 & 0.06 & 0.03 & 0.02 & 0.04 & 0.02 & 0.02 & 0.02 & 0.04 & 0.02 & 0.03 & 0.02 & 0.02 & 0.04 \\
3970 & KOI-1970 & 30 & 0.06 & 0.02 & 0.6 & 0.04 & 0.11 & 0.08 & 0.04 & 0.03 & 0.06 & 0.03 & 0.03 & 0.03 & 0.05 & 0.02 & 0.04 & 0.02 & 0.02 & 0.05 \\
3971 & KOI-4430 & 29 & 0.06 & 0.02 & 0.6 & 0.04 & 0.10 & 0.07 & 0.04 & 0.03 & 0.05 & 0.03 & 0.03 & 0.03 & 0.05 & 0.02 & 0.04 & 0.02 & 0.02 & 0.05 \\
3972 & KOI-179 & 28 & 0.05 & 0.01 & 0.5 & 0.04 & 0.08 & 0.06 & 0.03 & 0.02 & 0.05 & 0.02 & 0.03 & 0.02 & 0.04 & 0.02 & 0.03 & 0.02 & 0.02 & 0.04 \\
3973 & KOI-2049 & 27 & 0.05 & 0.01 & 0.5 & 0.03 & 0.08 & 0.06 & 0.03 & 0.02 & 0.04 & 0.02 & 0.03 & 0.02 & 0.04 & 0.02 & 0.03 & 0.02 & 0.02 & 0.04 \\
3974 & KOI-712 & 27 & 0.05 & 0.01 & 0.5 & 0.03 & 0.08 & 0.06 & 0.03 & 0.02 & 0.04 & 0.02 & 0.02 & 0.02 & 0.04 & 0.02 & 0.03 & 0.02 & 0.02 & 0.04 \\
3975 & KOI-1938 & 27 & 0.05 & 0.01 & 0.5 & 0.03 & 0.08 & 0.06 & 0.03 & 0.02 & 0.04 & 0.02 & 0.03 & 0.02 & 0.04 & 0.02 & 0.03 & 0.02 & 0.02 & 0.04 \\
3976 & KOI-2815 & 28 & 0.05 & 0.01 & 0.5 & 0.03 & 0.08 & 0.06 & 0.03 & 0.02 & 0.04 & 0.02 & 0.03 & 0.02 & 0.04 & 0.02 & 0.03 & 0.02 & 0.02 & 0.04 \\
3977 & Kepler-423 & 26 & 0.05 & 0.01 & 0.5 & 0.03 & 0.06 & 0.05 & 0.02 & 0.02 & 0.04 & 0.02 & 0.02 & 0.02 & 0.04 & 0.02 & 0.03 & 0.01 & 0.02 & 0.04 \\
3978 & KOI-1854 & 27 & 0.05 & 0.01 & 0.5 & 0.03 & 0.08 & 0.06 & 0.03 & 0.02 & 0.04 & 0.02 & 0.02 & 0.02 & 0.04 & 0.02 & 0.03 & 0.02 & 0.02 & 0.04 \\
3979 & KOI-4822 & 28 & 0.05 & 0.01 & 0.5 & 0.03 & 0.08 & 0.06 & 0.03 & 0.02 & 0.04 & 0.02 & 0.03 & 0.02 & 0.04 & 0.02 & 0.03 & 0.02 & 0.02 & 0.04 \\
3980 & KOI-4617 & 28 & 0.06 & 0.02 & 0.5 & 0.04 & 0.09 & 0.07 & 0.03 & 0.02 & 0.05 & 0.02 & 0.03 & 0.02 & 0.05 & 0.02 & 0.03 & 0.02 & 0.02 & 0.05 \\
3981 & KOI-2831 & 27 & 0.05 & 0.01 & 0.5 & 0.03 & 0.08 & 0.06 & 0.03 & 0.02 & 0.04 & 0.02 & 0.02 & 0.02 & 0.04 & 0.02 & 0.03 & 0.02 & 0.02 & 0.04 \\
3982 & KOI-2706 & 25 & 0.05 & 0.01 & 0.5 & 0.03 & 0.04 & 0.04 & 0.01 & 0.01 & 0.03 & 0.01 & 0.01 & 0.01 & 0.03 & 0.01 & 0.02 & 0.01 & 0.01 & 0.03 \\
3983 & KOI-2769 & 27 & 0.05 & 0.01 & 0.5 & 0.03 & 0.08 & 0.06 & 0.03 & 0.02 & 0.04 & 0.02 & 0.02 & 0.02 & 0.04 & 0.02 & 0.03 & 0.02 & 0.02 & 0.04 \\
3984 & KOI-2545 & 27 & 0.05 & 0.01 & 0.5 & 0.03 & 0.08 & 0.06 & 0.03 & 0.02 & 0.04 & 0.02 & 0.03 & 0.02 & 0.04 & 0.02 & 0.03 & 0.02 & 0.02 & 0.04 \\
3985 & KOI-1751 & 29 & 0.06 & 0.02 & 0.6 & 0.04 & 0.10 & 0.07 & 0.04 & 0.02 & 0.05 & 0.03 & 0.03 & 0.02 & 0.05 & 0.02 & 0.04 & 0.02 & 0.02 & 0.05 \\
3986 & KOI-1913 & 27 & 0.05 & 0.01 & 0.5 & 0.03 & 0.08 & 0.06 & 0.03 & 0.02 & 0.04 & 0.02 & 0.02 & 0.02 & 0.04 & 0.02 & 0.03 & 0.02 & 0.02 & 0.04 \\
3987 & KOI-714 & 27 & 0.05 & 0.01 & 0.5 & 0.03 & 0.08 & 0.06 & 0.03 & 0.02 & 0.04 & 0.02 & 0.02 & 0.02 & 0.04 & 0.02 & 0.03 & 0.02 & 0.02 & 0.04 \\
3988 & KOI-2913 & 27 & 0.05 & 0.01 & 0.5 & 0.03 & 0.08 & 0.06 & 0.03 & 0.02 & 0.04 & 0.02 & 0.02 & 0.02 & 0.04 & 0.02 & 0.03 & 0.02 & 0.02 & 0.04 \\
3989 & KOI-2273 & 27 & 0.05 & 0.01 & 0.5 & 0.03 & 0.08 & 0.06 & 0.03 & 0.02 & 0.04 & 0.02 & 0.02 & 0.02 & 0.04 & 0.02 & 0.03 & 0.02 & 0.02 & 0.04 \\
3990 & KOI-2035 & 27 & 0.05 & 0.01 & 0.5 & 0.03 & 0.08 & 0.06 & 0.03 & 0.02 & 0.04 & 0.02 & 0.02 & 0.02 & 0.04 & 0.02 & 0.03 & 0.02 & 0.02 & 0.04 \\
3991 & KOI-2457 & 28 & 0.05 & 0.01 & 0.5 & 0.03 & 0.08 & 0.06 & 0.03 & 0.02 & 0.04 & 0.02 & 0.03 & 0.02 & 0.04 & 0.02 & 0.03 & 0.02 & 0.02 & 0.04 \\
3992 & KOI-3871 & 27 & 0.05 & 0.01 & 0.5 & 0.03 & 0.08 & 0.06 & 0.03 & 0.02 & 0.04 & 0.02 & 0.02 & 0.02 & 0.04 & 0.02 & 0.03 & 0.02 & 0.02 & 0.04 \\
3993 & KOI-3162 & 25 & 0.05 & 0.01 & 0.5 & 0.03 & 0.04 & 0.04 & 0.01 & 0.01 & 0.03 & 0.01 & 0.01 & 0.01 & 0.03 & 0.01 & 0.02 & 0.01 & 0.01 & 0.03 \\
3994 & KOI-3465 & 27 & 0.05 & 0.01 & 0.5 & 0.03 & 0.08 & 0.06 & 0.03 & 0.02 & 0.04 & 0.02 & 0.02 & 0.02 & 0.04 & 0.02 & 0.03 & 0.02 & 0.02 & 0.04 \\
3995 & KOI-3837 & 27 & 0.05 & 0.01 & 0.5 & 0.03 & 0.08 & 0.06 & 0.03 & 0.02 & 0.04 & 0.02 & 0.02 & 0.02 & 0.04 & 0.02 & 0.03 & 0.02 & 0.02 & 0.04 \\
3996 & KOI-1852 & 28 & 0.05 & 0.01 & 0.5 & 0.04 & 0.08 & 0.06 & 0.03 & 0.02 & 0.04 & 0.02 & 0.03 & 0.02 & 0.04 & 0.02 & 0.03 & 0.02 & 0.02 & 0.04 \\
3997 & KOI-1529 & 31 & 0.06 & 0.02 & 0.6 & 0.04 & 0.11 & 0.08 & 0.04 & 0.03 & 0.06 & 0.03 & 0.03 & 0.03 & 0.05 & 0.02 & 0.04 & 0.02 & 0.03 & 0.05 \\
3998 & KOI-2943 & 27 & 0.05 & 0.01 & 0.5 & 0.03 & 0.08 & 0.06 & 0.03 & 0.02 & 0.04 & 0.02 & 0.02 & 0.02 & 0.04 & 0.02 & 0.03 & 0.02 & 0.02 & 0.04 \\
3999 & KOI-135 & 27 & 0.05 & 0.01 & 0.5 & 0.03 & 0.08 & 0.06 & 0.03 & 0.02 & 0.04 & 0.02 & 0.02 & 0.02 & 0.04 & 0.02 & 0.03 & 0.02 & 0.02 & 0.04 \\
4000 & KOI-4421 & 28 & 0.05 & 0.01 & 0.5 & 0.04 & 0.08 & 0.06 & 0.03 & 0.02 & 0.04 & 0.02 & 0.03 & 0.02 & 0.04 & 0.02 & 0.03 & 0.02 & 0.02 & 0.04 \\
4001 & KOI-1715 & 27 & 0.05 & 0.01 & 0.5 & 0.03 & 0.08 & 0.06 & 0.03 & 0.02 & 0.04 & 0.02 & 0.02 & 0.02 & 0.04 & 0.02 & 0.03 & 0.02 & 0.02 & 0.04 \\
4002 & KOI-1958 & 33 & 0.06 & 0.02 & 0.6 & 0.05 & 0.13 & 0.09 & 0.05 & 0.03 & 0.07 & 0.03 & 0.04 & 0.03 & 0.06 & 0.03 & 0.05 & 0.02 & 0.03 & 0.06 \\
4003 & KOI-716 & 27 & 0.05 & 0.01 & 0.5 & 0.03 & 0.08 & 0.06 & 0.03 & 0.02 & 0.04 & 0.02 & 0.02 & 0.02 & 0.04 & 0.02 & 0.03 & 0.02 & 0.02 & 0.04 \\
4004 & KOI-1606 & 27 & 0.05 & 0.01 & 0.5 & 0.03 & 0.07 & 0.06 & 0.03 & 0.02 & 0.04 & 0.02 & 0.02 & 0.02 & 0.04 & 0.02 & 0.03 & 0.01 & 0.02 & 0.04 \\
4005 & KOI-717 & 27 & 0.05 & 0.01 & 0.5 & 0.03 & 0.08 & 0.06 & 0.03 & 0.02 & 0.04 & 0.02 & 0.02 & 0.02 & 0.04 & 0.02 & 0.03 & 0.02 & 0.02 & 0.04 \\
4006 & KOI-4230 & 27 & 0.05 & 0.01 & 0.5 & 0.03 & 0.08 & 0.06 & 0.03 & 0.02 & 0.04 & 0.02 & 0.02 & 0.02 & 0.04 & 0.02 & 0.03 & 0.02 & 0.02 & 0.04 \\
4007 & KOI-3246 & 27 & 0.05 & 0.01 & 0.5 & 0.03 & 0.07 & 0.06 & 0.03 & 0.02 & 0.04 & 0.02 & 0.02 & 0.02 & 0.04 & 0.02 & 0.03 & 0.01 & 0.02 & 0.04 \\
4008 & KOI-1955 & 28 & 0.05 & 0.02 & 0.5 & 0.04 & 0.08 & 0.06 & 0.03 & 0.02 & 0.05 & 0.02 & 0.03 & 0.02 & 0.04 & 0.02 & 0.03 & 0.02 & 0.02 & 0.04 \\
4009 & Kepler-342 & 26 & 0.05 & 0.01 & 0.5 & 0.03 & 0.06 & 0.05 & 0.02 & 0.02 & 0.03 & 0.01 & 0.02 & 0.02 & 0.04 & 0.02 & 0.02 & 0.01 & 0.02 & 0.04 \\
4010 & KOI-2135 & 27 & 0.05 & 0.01 & 0.5 & 0.03 & 0.08 & 0.06 & 0.03 & 0.02 & 0.04 & 0.02 & 0.02 & 0.02 & 0.04 & 0.02 & 0.03 & 0.02 & 0.02 & 0.04 \\
4011 & KOI-2732 & 28 & 0.05 & 0.01 & 0.5 & 0.03 & 0.08 & 0.06 & 0.03 & 0.02 & 0.04 & 0.02 & 0.03 & 0.02 & 0.04 & 0.02 & 0.03 & 0.02 & 0.02 & 0.04 \\
4012 & Kepler-403 & 25 & 0.05 & 0.01 & 0.5 & 0.03 & 0.05 & 0.04 & 0.02 & 0.01 & 0.03 & 0.01 & 0.02 & 0.01 & 0.04 & 0.02 & 0.02 & 0.01 & 0.01 & 0.03 \\
4013 & KOI-4575 & 27 & 0.05 & 0.01 & 0.5 & 0.03 & 0.08 & 0.06 & 0.03 & 0.02 & 0.04 & 0.02 & 0.02 & 0.02 & 0.04 & 0.02 & 0.03 & 0.02 & 0.02 & 0.04 \\
4014 & KOI-718 & 28 & 0.05 & 0.02 & 0.5 & 0.04 & 0.08 & 0.06 & 0.03 & 0.02 & 0.05 & 0.02 & 0.03 & 0.02 & 0.04 & 0.02 & 0.03 & 0.02 & 0.02 & 0.04 \\
4015 & Kepler-219 & 26 & 0.05 & 0.01 & 0.5 & 0.03 & 0.06 & 0.05 & 0.02 & 0.02 & 0.04 & 0.02 & 0.02 & 0.02 & 0.04 & 0.02 & 0.03 & 0.01 & 0.02 & 0.04 \\
4016 & KOI-327 & 27 & 0.05 & 0.01 & 0.5 & 0.03 & 0.08 & 0.06 & 0.03 & 0.02 & 0.04 & 0.02 & 0.03 & 0.02 & 0.04 & 0.02 & 0.03 & 0.02 & 0.02 & 0.04 \\
4017 & KOI-4383 & 28 & 0.05 & 0.01 & 0.5 & 0.04 & 0.08 & 0.06 & 0.03 & 0.02 & 0.05 & 0.02 & 0.03 & 0.02 & 0.04 & 0.02 & 0.03 & 0.02 & 0.02 & 0.04 \\
4018 & KOI-1537 & 27 & 0.05 & 0.01 & 0.5 & 0.03 & 0.08 & 0.06 & 0.03 & 0.02 & 0.04 & 0.02 & 0.03 & 0.02 & 0.04 & 0.02 & 0.03 & 0.02 & 0.02 & 0.04 \\
4019 & KOI-2803 & 27 & 0.05 & 0.01 & 0.5 & 0.03 & 0.08 & 0.06 & 0.03 & 0.02 & 0.04 & 0.02 & 0.02 & 0.02 & 0.04 & 0.02 & 0.03 & 0.02 & 0.02 & 0.04 \\
4020 & KOI-1779 & 28 & 0.05 & 0.01 & 0.5 & 0.03 & 0.08 & 0.06 & 0.03 & 0.02 & 0.04 & 0.02 & 0.03 & 0.02 & 0.04 & 0.02 & 0.03 & 0.02 & 0.02 & 0.04 \\
4021 & KOI-721 & 27 & 0.05 & 0.01 & 0.5 & 0.03 & 0.08 & 0.06 & 0.03 & 0.02 & 0.04 & 0.02 & 0.02 & 0.02 & 0.04 & 0.02 & 0.03 & 0.02 & 0.02 & 0.04 \\
4022 & KOI-720 & 27 & 0.05 & 0.01 & 0.5 & 0.03 & 0.07 & 0.06 & 0.03 & 0.02 & 0.04 & 0.02 & 0.02 & 0.02 & 0.04 & 0.02 & 0.03 & 0.02 & 0.02 & 0.04 \\
4023 & KOI-722 & 27 & 0.05 & 0.01 & 0.5 & 0.03 & 0.08 & 0.06 & 0.03 & 0.02 & 0.04 & 0.02 & 0.02 & 0.02 & 0.04 & 0.02 & 0.03 & 0.02 & 0.02 & 0.04 \\
4024 & KOI-4431 & 27 & 0.05 & 0.01 & 0.5 & 0.03 & 0.08 & 0.06 & 0.03 & 0.02 & 0.04 & 0.02 & 0.02 & 0.02 & 0.04 & 0.02 & 0.03 & 0.02 & 0.02 & 0.04 \\
4025 & KOI-1875 & 30 & 0.06 & 0.02 & 0.6 & 0.04 & 0.10 & 0.07 & 0.04 & 0.03 & 0.05 & 0.03 & 0.03 & 0.03 & 0.05 & 0.02 & 0.04 & 0.02 & 0.02 & 0.05 \\
4026 & KOI-4647 & 28 & 0.06 & 0.02 & 0.5 & 0.04 & 0.09 & 0.06 & 0.03 & 0.02 & 0.05 & 0.02 & 0.03 & 0.02 & 0.05 & 0.02 & 0.03 & 0.02 & 0.02 & 0.04 \\
4027 & KOI-528 & 31 & 0.06 & 0.02 & 0.6 & 0.04 & 0.11 & 0.08 & 0.04 & 0.03 & 0.06 & 0.03 & 0.03 & 0.03 & 0.05 & 0.02 & 0.04 & 0.02 & 0.02 & 0.05 \\
4028 & KOI-2748 & 27 & 0.05 & 0.01 & 0.5 & 0.03 & 0.08 & 0.06 & 0.03 & 0.02 & 0.04 & 0.02 & 0.02 & 0.02 & 0.04 & 0.02 & 0.03 & 0.02 & 0.02 & 0.04 \\
4029 & KOI-2832 & 27 & 0.05 & 0.01 & 0.5 & 0.03 & 0.07 & 0.06 & 0.03 & 0.02 & 0.04 & 0.02 & 0.02 & 0.02 & 0.04 & 0.02 & 0.03 & 0.01 & 0.02 & 0.04 \\
4030 & KOI-2312 & 27 & 0.05 & 0.01 & 0.5 & 0.03 & 0.08 & 0.06 & 0.03 & 0.02 & 0.04 & 0.02 & 0.02 & 0.02 & 0.04 & 0.02 & 0.03 & 0.02 & 0.02 & 0.04 \\
4031 & KOI-4146 & 27 & 0.05 & 0.01 & 0.5 & 0.03 & 0.07 & 0.06 & 0.03 & 0.02 & 0.04 & 0.02 & 0.02 & 0.02 & 0.04 & 0.02 & 0.03 & 0.01 & 0.02 & 0.04 \\
4032 & KOI-4706 & 28 & 0.05 & 0.01 & 0.5 & 0.04 & 0.08 & 0.06 & 0.03 & 0.02 & 0.04 & 0.02 & 0.03 & 0.02 & 0.04 & 0.02 & 0.03 & 0.02 & 0.02 & 0.04 \\
4033 & KOI-3382 & 32 & 0.06 & 0.02 & 0.6 & 0.05 & 0.12 & 0.09 & 0.05 & 0.03 & 0.06 & 0.03 & 0.04 & 0.03 & 0.06 & 0.02 & 0.04 & 0.02 & 0.03 & 0.06 \\
4034 & KOI-723 & 29 & 0.06 & 0.02 & 0.6 & 0.04 & 0.10 & 0.07 & 0.04 & 0.02 & 0.05 & 0.03 & 0.03 & 0.02 & 0.05 & 0.02 & 0.04 & 0.02 & 0.02 & 0.05 \\
4035 & KOI-1796 & 27 & 0.05 & 0.01 & 0.5 & 0.03 & 0.08 & 0.06 & 0.03 & 0.02 & 0.04 & 0.02 & 0.02 & 0.02 & 0.04 & 0.02 & 0.03 & 0.02 & 0.02 & 0.04 \\
4036 & KOI-2785 & 28 & 0.05 & 0.01 & 0.5 & 0.04 & 0.08 & 0.06 & 0.03 & 0.02 & 0.04 & 0.02 & 0.03 & 0.02 & 0.04 & 0.02 & 0.03 & 0.02 & 0.02 & 0.04 \\
4037 & KOI-4469 & 29 & 0.06 & 0.02 & 0.6 & 0.04 & 0.09 & 0.07 & 0.04 & 0.02 & 0.05 & 0.02 & 0.03 & 0.02 & 0.05 & 0.02 & 0.04 & 0.02 & 0.02 & 0.05 \\
4038 & WASP-113 & 25 & 0.05 & 0.01 & 0.5 & 0.03 & 0.04 & 0.04 & 0.01 & 0.01 & 0.03 & 0.01 & 0.01 & 0.01 & 0.03 & 0.01 & 0.02 & 0.01 & 0.01 & 0.03 \\
4039 & KOI-1598 & 30 & 0.06 & 0.02 & 0.6 & 0.04 & 0.10 & 0.07 & 0.04 & 0.03 & 0.05 & 0.03 & 0.03 & 0.03 & 0.05 & 0.02 & 0.04 & 0.02 & 0.02 & 0.05 \\
4040 & Kepler-310 & 26 & 0.05 & 0.01 & 0.5 & 0.03 & 0.07 & 0.05 & 0.02 & 0.02 & 0.04 & 0.02 & 0.02 & 0.02 & 0.04 & 0.02 & 0.03 & 0.01 & 0.02 & 0.04 \\
4041 & KOI-1783 & 28 & 0.05 & 0.02 & 0.5 & 0.04 & 0.08 & 0.06 & 0.03 & 0.02 & 0.05 & 0.02 & 0.03 & 0.02 & 0.04 & 0.02 & 0.03 & 0.02 & 0.02 & 0.04 \\
4042 & KOI-2002 & 27 & 0.05 & 0.01 & 0.5 & 0.03 & 0.08 & 0.06 & 0.03 & 0.02 & 0.04 & 0.02 & 0.02 & 0.02 & 0.04 & 0.02 & 0.03 & 0.02 & 0.02 & 0.04 \\
4043 & KOI-1984 & 28 & 0.05 & 0.01 & 0.5 & 0.03 & 0.08 & 0.06 & 0.03 & 0.02 & 0.04 & 0.02 & 0.03 & 0.02 & 0.04 & 0.02 & 0.03 & 0.02 & 0.02 & 0.04 \\
4044 & HAT-P-44 & 25 & 0.05 & 0.01 & 0.5 & 0.03 & 0.04 & 0.04 & 0.01 & 0.01 & 0.03 & 0.01 & 0.01 & 0.01 & 0.03 & 0.01 & 0.02 & 0.01 & 0.01 & 0.03 \\
4045 & KOI-4292 & 27 & 0.05 & 0.01 & 0.5 & 0.03 & 0.08 & 0.06 & 0.03 & 0.02 & 0.04 & 0.02 & 0.02 & 0.02 & 0.04 & 0.02 & 0.03 & 0.02 & 0.02 & 0.04 \\
4046 & KOI-2891 & 27 & 0.05 & 0.01 & 0.5 & 0.03 & 0.08 & 0.06 & 0.03 & 0.02 & 0.04 & 0.02 & 0.02 & 0.02 & 0.04 & 0.02 & 0.03 & 0.02 & 0.02 & 0.04 \\
4047 & KOI-1917 & 27 & 0.05 & 0.01 & 0.5 & 0.03 & 0.08 & 0.06 & 0.03 & 0.02 & 0.04 & 0.02 & 0.02 & 0.02 & 0.04 & 0.02 & 0.03 & 0.02 & 0.02 & 0.04 \\
4048 & KOI-2964 & 27 & 0.05 & 0.01 & 0.5 & 0.03 & 0.08 & 0.06 & 0.03 & 0.02 & 0.04 & 0.02 & 0.02 & 0.02 & 0.04 & 0.02 & 0.03 & 0.02 & 0.02 & 0.04 \\
4049 & KOI-1608 & 27 & 0.05 & 0.01 & 0.5 & 0.03 & 0.08 & 0.06 & 0.03 & 0.02 & 0.04 & 0.02 & 0.03 & 0.02 & 0.04 & 0.02 & 0.03 & 0.02 & 0.02 & 0.04 \\
4050 & KOI-1888 & 28 & 0.05 & 0.01 & 0.5 & 0.03 & 0.08 & 0.06 & 0.03 & 0.02 & 0.04 & 0.02 & 0.03 & 0.02 & 0.04 & 0.02 & 0.03 & 0.02 & 0.02 & 0.04 \\
4051 & KOI-1909 & 27 & 0.05 & 0.01 & 0.5 & 0.03 & 0.08 & 0.06 & 0.03 & 0.02 & 0.04 & 0.02 & 0.02 & 0.02 & 0.04 & 0.02 & 0.03 & 0.02 & 0.02 & 0.04 \\
4052 & Kepler-334 & 25 & 0.05 & 0.01 & 0.5 & 0.03 & 0.06 & 0.04 & 0.02 & 0.01 & 0.03 & 0.01 & 0.02 & 0.01 & 0.04 & 0.02 & 0.02 & 0.01 & 0.01 & 0.03 \\
4053 & KOI-1929 & 27 & 0.05 & 0.01 & 0.5 & 0.03 & 0.08 & 0.06 & 0.03 & 0.02 & 0.04 & 0.02 & 0.02 & 0.02 & 0.04 & 0.02 & 0.03 & 0.02 & 0.02 & 0.04 \\
4054 & KOI-3195 & 28 & 0.05 & 0.01 & 0.5 & 0.03 & 0.08 & 0.06 & 0.03 & 0.02 & 0.04 & 0.02 & 0.03 & 0.02 & 0.04 & 0.02 & 0.03 & 0.02 & 0.02 & 0.04 \\
4055 & KOI-1784 & 27 & 0.05 & 0.01 & 0.5 & 0.03 & 0.08 & 0.06 & 0.03 & 0.02 & 0.04 & 0.02 & 0.02 & 0.02 & 0.04 & 0.02 & 0.03 & 0.02 & 0.02 & 0.04 \\
4056 & KOI-3208 & 27 & 0.05 & 0.01 & 0.5 & 0.03 & 0.08 & 0.06 & 0.03 & 0.02 & 0.04 & 0.02 & 0.03 & 0.02 & 0.04 & 0.02 & 0.03 & 0.02 & 0.02 & 0.04 \\
4057 & KOI-991 & 28 & 0.05 & 0.01 & 0.5 & 0.03 & 0.08 & 0.06 & 0.03 & 0.02 & 0.04 & 0.02 & 0.03 & 0.02 & 0.04 & 0.02 & 0.03 & 0.02 & 0.02 & 0.04 \\
4058 & KOI-4613 & 27 & 0.05 & 0.01 & 0.5 & 0.03 & 0.08 & 0.06 & 0.03 & 0.02 & 0.04 & 0.02 & 0.02 & 0.02 & 0.04 & 0.02 & 0.03 & 0.02 & 0.02 & 0.04 \\
4059 & KOI-3218 & 27 & 0.05 & 0.01 & 0.5 & 0.03 & 0.08 & 0.06 & 0.03 & 0.02 & 0.04 & 0.02 & 0.02 & 0.02 & 0.04 & 0.02 & 0.03 & 0.02 & 0.02 & 0.04 \\
4060 & KOI-4070 & 29 & 0.06 & 0.02 & 0.6 & 0.04 & 0.09 & 0.07 & 0.04 & 0.02 & 0.05 & 0.02 & 0.03 & 0.02 & 0.05 & 0.02 & 0.03 & 0.02 & 0.02 & 0.05 \\
4061 & KOI-2342 & 28 & 0.05 & 0.01 & 0.5 & 0.04 & 0.08 & 0.06 & 0.03 & 0.02 & 0.04 & 0.02 & 0.03 & 0.02 & 0.04 & 0.02 & 0.03 & 0.02 & 0.02 & 0.04 \\
4062 & KOI-427 & 31 & 0.06 & 0.02 & 0.6 & 0.04 & 0.11 & 0.08 & 0.04 & 0.03 & 0.06 & 0.03 & 0.03 & 0.03 & 0.05 & 0.02 & 0.04 & 0.02 & 0.03 & 0.05 \\
4063 & KOI-3130 & 27 & 0.05 & 0.01 & 0.5 & 0.03 & 0.07 & 0.06 & 0.03 & 0.02 & 0.04 & 0.02 & 0.02 & 0.02 & 0.04 & 0.02 & 0.03 & 0.02 & 0.02 & 0.04 \\
4064 & KOI-5782 & 29 & 0.06 & 0.02 & 0.6 & 0.04 & 0.09 & 0.07 & 0.04 & 0.02 & 0.05 & 0.02 & 0.03 & 0.02 & 0.05 & 0.02 & 0.03 & 0.02 & 0.02 & 0.05 \\
4065 & KOI-331 & 27 & 0.05 & 0.01 & 0.5 & 0.03 & 0.08 & 0.06 & 0.03 & 0.02 & 0.04 & 0.02 & 0.02 & 0.02 & 0.04 & 0.02 & 0.03 & 0.02 & 0.02 & 0.04 \\
4066 & KOI-2390 & 27 & 0.05 & 0.01 & 0.5 & 0.03 & 0.08 & 0.06 & 0.03 & 0.02 & 0.04 & 0.02 & 0.02 & 0.02 & 0.04 & 0.02 & 0.03 & 0.02 & 0.02 & 0.04 \\
4067 & KOI-732 & 29 & 0.06 & 0.02 & 0.6 & 0.04 & 0.10 & 0.07 & 0.04 & 0.02 & 0.05 & 0.03 & 0.03 & 0.02 & 0.05 & 0.02 & 0.04 & 0.02 & 0.02 & 0.05 \\
4068 & KOI-4557 & 28 & 0.05 & 0.01 & 0.5 & 0.04 & 0.08 & 0.06 & 0.03 & 0.02 & 0.04 & 0.02 & 0.03 & 0.02 & 0.04 & 0.02 & 0.03 & 0.02 & 0.02 & 0.04 \\
4069 & KOI-3608 & 27 & 0.05 & 0.01 & 0.5 & 0.03 & 0.08 & 0.06 & 0.03 & 0.02 & 0.04 & 0.02 & 0.02 & 0.02 & 0.04 & 0.02 & 0.03 & 0.02 & 0.02 & 0.04 \\
4070 & KOI-332 & 27 & 0.05 & 0.01 & 0.5 & 0.03 & 0.08 & 0.06 & 0.03 & 0.02 & 0.04 & 0.02 & 0.02 & 0.02 & 0.04 & 0.02 & 0.03 & 0.02 & 0.02 & 0.04 \\
4071 & KOI-2153 & 27 & 0.05 & 0.01 & 0.5 & 0.03 & 0.08 & 0.06 & 0.03 & 0.02 & 0.04 & 0.02 & 0.03 & 0.02 & 0.04 & 0.02 & 0.03 & 0.02 & 0.02 & 0.04 \\
4072 & KOI-333 & 27 & 0.05 & 0.01 & 0.5 & 0.03 & 0.08 & 0.06 & 0.03 & 0.02 & 0.04 & 0.02 & 0.03 & 0.02 & 0.04 & 0.02 & 0.03 & 0.02 & 0.02 & 0.04 \\
4073 & KOI-1905 & 27 & 0.05 & 0.01 & 0.5 & 0.03 & 0.08 & 0.06 & 0.03 & 0.02 & 0.04 & 0.02 & 0.02 & 0.02 & 0.04 & 0.02 & 0.03 & 0.02 & 0.02 & 0.04 \\
4074 & KOI-3216 & 27 & 0.05 & 0.01 & 0.5 & 0.03 & 0.08 & 0.06 & 0.03 & 0.02 & 0.04 & 0.02 & 0.02 & 0.02 & 0.04 & 0.02 & 0.03 & 0.02 & 0.02 & 0.04 \\
4075 & KOI-3908 & 27 & 0.05 & 0.01 & 0.5 & 0.03 & 0.07 & 0.06 & 0.03 & 0.02 & 0.04 & 0.02 & 0.02 & 0.02 & 0.04 & 0.02 & 0.03 & 0.02 & 0.02 & 0.04 \\
4076 & KOI-1175 & 27 & 0.05 & 0.01 & 0.5 & 0.03 & 0.08 & 0.06 & 0.03 & 0.02 & 0.04 & 0.02 & 0.02 & 0.02 & 0.04 & 0.02 & 0.03 & 0.02 & 0.02 & 0.04 \\
4077 & KOI-1169 & 25 & 0.05 & 0.01 & 0.5 & 0.03 & 0.04 & 0.04 & 0.01 & 0.01 & 0.03 & 0.01 & 0.01 & 0.01 & 0.03 & 0.01 & 0.02 & 0.01 & 0.01 & 0.03 \\
4078 & KOI-1165 & 27 & 0.05 & 0.01 & 0.5 & 0.03 & 0.08 & 0.06 & 0.03 & 0.02 & 0.04 & 0.02 & 0.02 & 0.02 & 0.04 & 0.02 & 0.03 & 0.02 & 0.02 & 0.04 \\
4079 & KOI-3991 & 27 & 0.05 & 0.01 & 0.5 & 0.03 & 0.08 & 0.06 & 0.03 & 0.02 & 0.04 & 0.02 & 0.02 & 0.02 & 0.04 & 0.02 & 0.03 & 0.02 & 0.02 & 0.04 \\
4080 & KOI-4446 & 27 & 0.05 & 0.01 & 0.5 & 0.03 & 0.07 & 0.06 & 0.03 & 0.02 & 0.04 & 0.02 & 0.02 & 0.02 & 0.04 & 0.02 & 0.03 & 0.02 & 0.02 & 0.04 \\
4081 & KOI-2147 & 30 & 0.06 & 0.02 & 0.6 & 0.04 & 0.10 & 0.07 & 0.04 & 0.03 & 0.05 & 0.03 & 0.03 & 0.03 & 0.05 & 0.02 & 0.04 & 0.02 & 0.02 & 0.05 \\
4082 & KOI-2859 & 27 & 0.05 & 0.01 & 0.5 & 0.03 & 0.07 & 0.06 & 0.03 & 0.02 & 0.04 & 0.02 & 0.02 & 0.02 & 0.04 & 0.02 & 0.03 & 0.02 & 0.02 & 0.04 \\
4083 & KOI-4556 & 27 & 0.05 & 0.01 & 0.5 & 0.03 & 0.08 & 0.06 & 0.03 & 0.02 & 0.04 & 0.02 & 0.02 & 0.02 & 0.04 & 0.02 & 0.03 & 0.02 & 0.02 & 0.04 \\
4084 & KOI-289 & 28 & 0.05 & 0.01 & 0.5 & 0.04 & 0.08 & 0.06 & 0.03 & 0.02 & 0.04 & 0.02 & 0.03 & 0.02 & 0.04 & 0.02 & 0.03 & 0.02 & 0.02 & 0.04 \\
4085 & KOI-3224 & 27 & 0.05 & 0.01 & 0.5 & 0.03 & 0.07 & 0.06 & 0.03 & 0.02 & 0.04 & 0.02 & 0.02 & 0.02 & 0.04 & 0.02 & 0.03 & 0.02 & 0.02 & 0.04 \\
4086 & KOI-2583 & 27 & 0.05 & 0.01 & 0.5 & 0.03 & 0.08 & 0.06 & 0.03 & 0.02 & 0.04 & 0.02 & 0.02 & 0.02 & 0.04 & 0.02 & 0.03 & 0.02 & 0.02 & 0.04 \\
4087 & KOI-1161 & 29 & 0.06 & 0.02 & 0.6 & 0.04 & 0.09 & 0.07 & 0.04 & 0.02 & 0.05 & 0.03 & 0.03 & 0.02 & 0.05 & 0.02 & 0.04 & 0.02 & 0.02 & 0.05 \\
4088 & KOI-1168 & 27 & 0.05 & 0.01 & 0.5 & 0.03 & 0.08 & 0.06 & 0.03 & 0.02 & 0.04 & 0.02 & 0.03 & 0.02 & 0.04 & 0.02 & 0.03 & 0.02 & 0.02 & 0.04 \\
4089 & KOI-2040 & 28 & 0.05 & 0.01 & 0.5 & 0.04 & 0.08 & 0.06 & 0.03 & 0.02 & 0.04 & 0.02 & 0.03 & 0.02 & 0.04 & 0.02 & 0.03 & 0.02 & 0.02 & 0.04 \\
4090 & KOI-474 & 30 & 0.06 & 0.02 & 0.6 & 0.04 & 0.11 & 0.08 & 0.04 & 0.03 & 0.06 & 0.03 & 0.03 & 0.03 & 0.05 & 0.02 & 0.04 & 0.02 & 0.02 & 0.05 \\
4091 & Kepler-164 & 26 & 0.05 & 0.01 & 0.5 & 0.03 & 0.06 & 0.05 & 0.02 & 0.02 & 0.04 & 0.02 & 0.02 & 0.02 & 0.04 & 0.02 & 0.03 & 0.01 & 0.02 & 0.04 \\
4092 & KOI-2484 & 27 & 0.05 & 0.01 & 0.5 & 0.03 & 0.08 & 0.06 & 0.03 & 0.02 & 0.04 & 0.02 & 0.02 & 0.02 & 0.04 & 0.02 & 0.03 & 0.02 & 0.02 & 0.04 \\
4093 & KOI-3231 & 27 & 0.05 & 0.01 & 0.5 & 0.03 & 0.08 & 0.06 & 0.03 & 0.02 & 0.04 & 0.02 & 0.03 & 0.02 & 0.04 & 0.02 & 0.03 & 0.02 & 0.02 & 0.04 \\
4094 & KOI-4480 & 27 & 0.05 & 0.01 & 0.5 & 0.03 & 0.08 & 0.06 & 0.03 & 0.02 & 0.04 & 0.02 & 0.02 & 0.02 & 0.04 & 0.02 & 0.03 & 0.02 & 0.02 & 0.04 \\
4095 & KOI-2961 & 27 & 0.05 & 0.01 & 0.5 & 0.03 & 0.08 & 0.06 & 0.03 & 0.02 & 0.04 & 0.02 & 0.02 & 0.02 & 0.04 & 0.02 & 0.03 & 0.02 & 0.02 & 0.04 \\
4096 & KOI-1163 & 31 & 0.06 & 0.02 & 0.6 & 0.04 & 0.11 & 0.08 & 0.04 & 0.03 & 0.06 & 0.03 & 0.04 & 0.03 & 0.05 & 0.02 & 0.04 & 0.02 & 0.03 & 0.05 \\
4097 & KOI-2208 & 27 & 0.05 & 0.01 & 0.5 & 0.03 & 0.08 & 0.06 & 0.03 & 0.02 & 0.04 & 0.02 & 0.02 & 0.02 & 0.04 & 0.02 & 0.03 & 0.02 & 0.02 & 0.04 \\
4098 & KOI-338 & 27 & 0.05 & 0.01 & 0.5 & 0.03 & 0.07 & 0.06 & 0.03 & 0.02 & 0.04 & 0.02 & 0.02 & 0.02 & 0.04 & 0.02 & 0.03 & 0.01 & 0.02 & 0.04 \\
4099 & KOI-4345 & 28 & 0.05 & 0.01 & 0.5 & 0.04 & 0.08 & 0.06 & 0.03 & 0.02 & 0.04 & 0.02 & 0.03 & 0.02 & 0.04 & 0.02 & 0.03 & 0.02 & 0.02 & 0.04 \\
4100 & KOI-337 & 28 & 0.05 & 0.01 & 0.5 & 0.04 & 0.08 & 0.06 & 0.03 & 0.02 & 0.04 & 0.02 & 0.03 & 0.02 & 0.04 & 0.02 & 0.03 & 0.02 & 0.02 & 0.04 \\
4101 & KOI-263 B & 28 & 0.05 & 0.01 & 0.5 & 0.03 & 0.08 & 0.06 & 0.03 & 0.02 & 0.04 & 0.02 & 0.03 & 0.02 & 0.04 & 0.02 & 0.03 & 0.02 & 0.02 & 0.04 \\
4102 & KOI-340 & 27 & 0.05 & 0.01 & 0.5 & 0.03 & 0.07 & 0.06 & 0.03 & 0.02 & 0.04 & 0.02 & 0.02 & 0.02 & 0.04 & 0.02 & 0.03 & 0.02 & 0.02 & 0.04 \\
4103 & KOI-2300 & 28 & 0.05 & 0.01 & 0.5 & 0.04 & 0.08 & 0.06 & 0.03 & 0.02 & 0.05 & 0.02 & 0.03 & 0.02 & 0.04 & 0.02 & 0.03 & 0.02 & 0.02 & 0.04 \\
4104 & KOI-203 & 27 & 0.05 & 0.01 & 0.5 & 0.03 & 0.08 & 0.06 & 0.03 & 0.02 & 0.04 & 0.02 & 0.02 & 0.02 & 0.04 & 0.02 & 0.03 & 0.02 & 0.02 & 0.04 \\
4105 & KOI-4765 & 27 & 0.05 & 0.01 & 0.5 & 0.03 & 0.08 & 0.06 & 0.03 & 0.02 & 0.04 & 0.02 & 0.03 & 0.02 & 0.04 & 0.02 & 0.03 & 0.02 & 0.02 & 0.04 \\
4106 & KOI-1308 & 27 & 0.05 & 0.01 & 0.5 & 0.03 & 0.08 & 0.06 & 0.03 & 0.02 & 0.04 & 0.02 & 0.02 & 0.02 & 0.04 & 0.02 & 0.03 & 0.02 & 0.02 & 0.04 \\
4107 & KOI-275 & 27 & 0.05 & 0.01 & 0.5 & 0.03 & 0.08 & 0.06 & 0.03 & 0.02 & 0.04 & 0.02 & 0.02 & 0.02 & 0.04 & 0.02 & 0.03 & 0.02 & 0.02 & 0.04 \\
4108 & KOI-4892 & 27 & 0.05 & 0.01 & 0.5 & 0.03 & 0.08 & 0.06 & 0.03 & 0.02 & 0.04 & 0.02 & 0.02 & 0.02 & 0.04 & 0.02 & 0.03 & 0.02 & 0.02 & 0.04 \\
4109 & KOI-3032 & 34 & 0.06 & 0.02 & 0.6 & 0.05 & 0.13 & 0.10 & 0.05 & 0.03 & 0.07 & 0.04 & 0.04 & 0.03 & 0.06 & 0.03 & 0.05 & 0.03 & 0.03 & 0.06 \\
4110 & KOI-4204 & 28 & 0.06 & 0.02 & 0.5 & 0.04 & 0.08 & 0.06 & 0.03 & 0.02 & 0.05 & 0.02 & 0.03 & 0.02 & 0.05 & 0.02 & 0.03 & 0.02 & 0.02 & 0.04 \\
4111 & KOI-339 & 27 & 0.05 & 0.01 & 0.5 & 0.03 & 0.08 & 0.06 & 0.03 & 0.02 & 0.04 & 0.02 & 0.02 & 0.02 & 0.04 & 0.02 & 0.03 & 0.02 & 0.02 & 0.04 \\
4112 & KOI-749 & 30 & 0.06 & 0.02 & 0.6 & 0.04 & 0.10 & 0.07 & 0.04 & 0.03 & 0.05 & 0.03 & 0.03 & 0.03 & 0.05 & 0.02 & 0.04 & 0.02 & 0.02 & 0.05 \\
4113 & KOI-2149 & 27 & 0.05 & 0.01 & 0.5 & 0.03 & 0.08 & 0.06 & 0.03 & 0.02 & 0.04 & 0.02 & 0.02 & 0.02 & 0.04 & 0.02 & 0.03 & 0.02 & 0.02 & 0.04 \\
4114 & KOI-4833 & 27 & 0.05 & 0.01 & 0.5 & 0.03 & 0.08 & 0.06 & 0.03 & 0.02 & 0.04 & 0.02 & 0.02 & 0.02 & 0.04 & 0.02 & 0.03 & 0.02 & 0.02 & 0.04 \\
4115 & KOI-1837 & 27 & 0.05 & 0.01 & 0.5 & 0.03 & 0.08 & 0.06 & 0.03 & 0.02 & 0.04 & 0.02 & 0.02 & 0.02 & 0.04 & 0.02 & 0.03 & 0.02 & 0.02 & 0.04 \\
4116 & KOI-1797 & 27 & 0.05 & 0.01 & 0.5 & 0.03 & 0.07 & 0.05 & 0.03 & 0.02 & 0.04 & 0.02 & 0.02 & 0.02 & 0.04 & 0.02 & 0.03 & 0.01 & 0.02 & 0.04 \\
4117 & KOI-598 & 30 & 0.06 & 0.02 & 0.6 & 0.04 & 0.10 & 0.07 & 0.04 & 0.03 & 0.05 & 0.03 & 0.03 & 0.03 & 0.05 & 0.02 & 0.04 & 0.02 & 0.02 & 0.05 \\
4118 & KOI-2 & 26 & 0.05 & 0.01 & 0.5 & 0.03 & 0.06 & 0.05 & 0.02 & 0.02 & 0.04 & 0.02 & 0.02 & 0.02 & 0.04 & 0.02 & 0.03 & 0.01 & 0.02 & 0.04 \\
4119 & KOI-4366 & 34 & 0.06 & 0.02 & 0.6 & 0.05 & 0.13 & 0.10 & 0.05 & 0.03 & 0.07 & 0.04 & 0.04 & 0.03 & 0.06 & 0.03 & 0.05 & 0.03 & 0.03 & 0.06 \\
4120 & KOI-211 & 29 & 0.06 & 0.02 & 0.6 & 0.04 & 0.10 & 0.07 & 0.04 & 0.03 & 0.05 & 0.03 & 0.03 & 0.03 & 0.05 & 0.02 & 0.04 & 0.02 & 0.02 & 0.05 \\
4121 & KOI-2046 & 27 & 0.05 & 0.01 & 0.5 & 0.03 & 0.08 & 0.06 & 0.03 & 0.02 & 0.04 & 0.02 & 0.02 & 0.02 & 0.04 & 0.02 & 0.03 & 0.02 & 0.02 & 0.04 \\
4122 & KOI-4312 & 28 & 0.05 & 0.01 & 0.5 & 0.04 & 0.08 & 0.06 & 0.03 & 0.02 & 0.04 & 0.02 & 0.03 & 0.02 & 0.04 & 0.02 & 0.03 & 0.02 & 0.02 & 0.04 \\
4123 & KOI-4335 & 27 & 0.05 & 0.01 & 0.5 & 0.03 & 0.08 & 0.06 & 0.03 & 0.02 & 0.04 & 0.02 & 0.02 & 0.02 & 0.04 & 0.02 & 0.03 & 0.02 & 0.02 & 0.04 \\
4124 & KOI-4024 & 27 & 0.05 & 0.01 & 0.5 & 0.03 & 0.08 & 0.06 & 0.03 & 0.02 & 0.04 & 0.02 & 0.03 & 0.02 & 0.04 & 0.02 & 0.03 & 0.02 & 0.02 & 0.04 \\
4125 & KOI-209 & 27 & 0.05 & 0.01 & 0.5 & 0.03 & 0.08 & 0.06 & 0.03 & 0.02 & 0.04 & 0.02 & 0.03 & 0.02 & 0.04 & 0.02 & 0.03 & 0.02 & 0.02 & 0.04 \\
4126 & KOI-1305 & 29 & 0.06 & 0.02 & 0.6 & 0.04 & 0.09 & 0.07 & 0.04 & 0.02 & 0.05 & 0.02 & 0.03 & 0.02 & 0.05 & 0.02 & 0.03 & 0.02 & 0.02 & 0.05 \\
4127 & KOI-3 & 27 & 0.05 & 0.01 & 0.5 & 0.03 & 0.07 & 0.05 & 0.03 & 0.02 & 0.04 & 0.02 & 0.02 & 0.02 & 0.04 & 0.02 & 0.03 & 0.01 & 0.02 & 0.04 \\
4128 & KOI-3889 & 27 & 0.05 & 0.01 & 0.5 & 0.03 & 0.08 & 0.06 & 0.03 & 0.02 & 0.04 & 0.02 & 0.02 & 0.02 & 0.04 & 0.02 & 0.03 & 0.02 & 0.02 & 0.04 \\
4129 & KOI-1311 & 27 & 0.05 & 0.01 & 0.5 & 0.03 & 0.08 & 0.06 & 0.03 & 0.02 & 0.04 & 0.02 & 0.02 & 0.02 & 0.04 & 0.02 & 0.03 & 0.02 & 0.02 & 0.04 \\
4130 & KOI-1639 & 28 & 0.05 & 0.01 & 0.5 & 0.03 & 0.08 & 0.06 & 0.03 & 0.02 & 0.04 & 0.02 & 0.03 & 0.02 & 0.04 & 0.02 & 0.03 & 0.02 & 0.02 & 0.04 \\
4131 & KOI-2236 & 30 & 0.06 & 0.02 & 0.6 & 0.04 & 0.10 & 0.08 & 0.04 & 0.03 & 0.05 & 0.03 & 0.03 & 0.03 & 0.05 & 0.02 & 0.04 & 0.02 & 0.02 & 0.05 \\
4132 & KOI-1316 & 27 & 0.05 & 0.01 & 0.5 & 0.03 & 0.08 & 0.06 & 0.03 & 0.02 & 0.04 & 0.02 & 0.02 & 0.02 & 0.04 & 0.02 & 0.03 & 0.02 & 0.02 & 0.04 \\
4133 & KOI-1989 & 28 & 0.05 & 0.01 & 0.5 & 0.04 & 0.08 & 0.06 & 0.03 & 0.02 & 0.04 & 0.02 & 0.03 & 0.02 & 0.04 & 0.02 & 0.03 & 0.02 & 0.02 & 0.04 \\
4134 & KOI-752 & 30 & 0.06 & 0.02 & 0.6 & 0.04 & 0.11 & 0.08 & 0.04 & 0.03 & 0.06 & 0.03 & 0.03 & 0.03 & 0.05 & 0.02 & 0.04 & 0.02 & 0.02 & 0.05 \\
4135 & KOI-3451 & 28 & 0.06 & 0.02 & 0.5 & 0.04 & 0.09 & 0.07 & 0.03 & 0.02 & 0.05 & 0.02 & 0.03 & 0.02 & 0.05 & 0.02 & 0.03 & 0.02 & 0.02 & 0.04 \\
4136 & KOI-3925 & 28 & 0.06 & 0.02 & 0.5 & 0.04 & 0.09 & 0.06 & 0.03 & 0.02 & 0.05 & 0.02 & 0.03 & 0.02 & 0.05 & 0.02 & 0.03 & 0.02 & 0.02 & 0.04 \\
4137 & KOI-3683 & 27 & 0.05 & 0.01 & 0.5 & 0.03 & 0.08 & 0.06 & 0.03 & 0.02 & 0.04 & 0.02 & 0.02 & 0.02 & 0.04 & 0.02 & 0.03 & 0.02 & 0.02 & 0.04 \\
4138 & KOI-4235 & 28 & 0.05 & 0.01 & 0.5 & 0.03 & 0.08 & 0.06 & 0.03 & 0.02 & 0.04 & 0.02 & 0.03 & 0.02 & 0.04 & 0.02 & 0.03 & 0.02 & 0.02 & 0.04 \\
4139 & KOI-2228 & 28 & 0.05 & 0.01 & 0.5 & 0.04 & 0.08 & 0.06 & 0.03 & 0.02 & 0.04 & 0.02 & 0.03 & 0.02 & 0.04 & 0.02 & 0.03 & 0.02 & 0.02 & 0.04 \\
4140 & KOI-117 & 27 & 0.05 & 0.01 & 0.5 & 0.03 & 0.08 & 0.06 & 0.03 & 0.02 & 0.04 & 0.02 & 0.02 & 0.02 & 0.04 & 0.02 & 0.03 & 0.02 & 0.02 & 0.04 \\
4141 & Kepler-107 & 25 & 0.05 & 0.01 & 0.5 & 0.03 & 0.06 & 0.04 & 0.02 & 0.02 & 0.03 & 0.01 & 0.02 & 0.02 & 0.04 & 0.02 & 0.02 & 0.01 & 0.01 & 0.03 \\
4142 & KOI-3602 & 27 & 0.05 & 0.01 & 0.5 & 0.03 & 0.08 & 0.06 & 0.03 & 0.02 & 0.04 & 0.02 & 0.02 & 0.02 & 0.04 & 0.02 & 0.03 & 0.02 & 0.02 & 0.04 \\
4143 & KOI-756 & 35 & 0.07 & 0.02 & 0.6 & 0.05 & 0.14 & 0.10 & 0.06 & 0.04 & 0.07 & 0.04 & 0.04 & 0.04 & 0.06 & 0.03 & 0.05 & 0.03 & 0.03 & 0.07 \\
4144 & KOI-2960 & 27 & 0.05 & 0.01 & 0.5 & 0.03 & 0.08 & 0.06 & 0.03 & 0.02 & 0.04 & 0.02 & 0.02 & 0.02 & 0.04 & 0.02 & 0.03 & 0.02 & 0.02 & 0.04 \\
4145 & KOI-341 & 27 & 0.05 & 0.01 & 0.5 & 0.03 & 0.08 & 0.06 & 0.03 & 0.02 & 0.04 & 0.02 & 0.02 & 0.02 & 0.04 & 0.02 & 0.03 & 0.02 & 0.02 & 0.04 \\
4146 & KOI-2075 & 27 & 0.05 & 0.01 & 0.5 & 0.03 & 0.08 & 0.06 & 0.03 & 0.02 & 0.04 & 0.02 & 0.03 & 0.02 & 0.04 & 0.02 & 0.03 & 0.02 & 0.02 & 0.04 \\
4147 & KOI-431 & 30 & 0.06 & 0.02 & 0.6 & 0.04 & 0.10 & 0.08 & 0.04 & 0.03 & 0.05 & 0.03 & 0.03 & 0.03 & 0.05 & 0.02 & 0.04 & 0.02 & 0.02 & 0.05 \\
4148 & KOI-1299 & 26 & 0.05 & 0.01 & 0.5 & 0.03 & 0.06 & 0.05 & 0.02 & 0.02 & 0.04 & 0.02 & 0.02 & 0.02 & 0.04 & 0.02 & 0.03 & 0.01 & 0.02 & 0.04 \\
4149 & KOI-1306 & 34 & 0.06 & 0.02 & 0.6 & 0.05 & 0.13 & 0.10 & 0.05 & 0.03 & 0.07 & 0.04 & 0.04 & 0.03 & 0.06 & 0.03 & 0.05 & 0.03 & 0.03 & 0.06 \\
4150 & KOI-3146 & 27 & 0.05 & 0.01 & 0.5 & 0.03 & 0.08 & 0.06 & 0.03 & 0.02 & 0.04 & 0.02 & 0.02 & 0.02 & 0.04 & 0.02 & 0.03 & 0.02 & 0.02 & 0.04 \\
4151 & KOI-291 & 27 & 0.05 & 0.01 & 0.5 & 0.03 & 0.08 & 0.06 & 0.03 & 0.02 & 0.04 & 0.02 & 0.02 & 0.02 & 0.04 & 0.02 & 0.03 & 0.02 & 0.02 & 0.04 \\
4152 & KOI-2623 & 27 & 0.05 & 0.01 & 0.5 & 0.03 & 0.08 & 0.06 & 0.03 & 0.02 & 0.04 & 0.02 & 0.03 & 0.02 & 0.04 & 0.02 & 0.03 & 0.02 & 0.02 & 0.04 \\
4153 & KOI-46 & 27 & 0.05 & 0.01 & 0.5 & 0.03 & 0.07 & 0.06 & 0.03 & 0.02 & 0.04 & 0.02 & 0.02 & 0.02 & 0.04 & 0.02 & 0.03 & 0.02 & 0.02 & 0.04 \\
4154 & KOI-1963 & 33 & 0.06 & 0.02 & 0.6 & 0.05 & 0.12 & 0.09 & 0.05 & 0.03 & 0.06 & 0.03 & 0.04 & 0.03 & 0.06 & 0.03 & 0.04 & 0.02 & 0.03 & 0.06 \\
4155 & KOI-2754 & 27 & 0.05 & 0.01 & 0.5 & 0.03 & 0.08 & 0.06 & 0.03 & 0.02 & 0.04 & 0.02 & 0.02 & 0.02 & 0.04 & 0.02 & 0.03 & 0.02 & 0.02 & 0.04 \\
4156 & KOI-757 & 33 & 0.06 & 0.02 & 0.6 & 0.05 & 0.13 & 0.09 & 0.05 & 0.03 & 0.07 & 0.03 & 0.04 & 0.03 & 0.06 & 0.03 & 0.05 & 0.02 & 0.03 & 0.06 \\
4157 & KOI-601 & 31 & 0.06 & 0.02 & 0.6 & 0.04 & 0.11 & 0.08 & 0.04 & 0.03 & 0.06 & 0.03 & 0.03 & 0.03 & 0.05 & 0.02 & 0.04 & 0.02 & 0.03 & 0.05 \\
4158 & KOI-1307 & 31 & 0.06 & 0.02 & 0.6 & 0.04 & 0.11 & 0.08 & 0.04 & 0.03 & 0.06 & 0.03 & 0.03 & 0.03 & 0.05 & 0.02 & 0.04 & 0.02 & 0.02 & 0.05 \\
4159 & KOI-4374 & 27 & 0.05 & 0.01 & 0.5 & 0.03 & 0.08 & 0.06 & 0.03 & 0.02 & 0.04 & 0.02 & 0.02 & 0.02 & 0.04 & 0.02 & 0.03 & 0.02 & 0.02 & 0.04 \\
4160 & KOI-1931 & 28 & 0.06 & 0.02 & 0.5 & 0.04 & 0.09 & 0.07 & 0.03 & 0.02 & 0.05 & 0.02 & 0.03 & 0.02 & 0.05 & 0.02 & 0.03 & 0.02 & 0.02 & 0.04 \\
4161 & KOI-343 & 27 & 0.05 & 0.01 & 0.5 & 0.03 & 0.08 & 0.06 & 0.03 & 0.02 & 0.04 & 0.02 & 0.02 & 0.02 & 0.04 & 0.02 & 0.03 & 0.02 & 0.02 & 0.04 \\
4162 & Kepler-142 & 26 & 0.05 & 0.01 & 0.5 & 0.03 & 0.06 & 0.05 & 0.02 & 0.02 & 0.03 & 0.01 & 0.02 & 0.02 & 0.04 & 0.02 & 0.02 & 0.01 & 0.01 & 0.03 \\
4163 & KOI-112 & 27 & 0.05 & 0.01 & 0.5 & 0.03 & 0.08 & 0.06 & 0.03 & 0.02 & 0.04 & 0.02 & 0.02 & 0.02 & 0.04 & 0.02 & 0.03 & 0.02 & 0.02 & 0.04 \\
4164 & KOI-759 & 29 & 0.06 & 0.02 & 0.6 & 0.04 & 0.10 & 0.07 & 0.04 & 0.02 & 0.05 & 0.03 & 0.03 & 0.02 & 0.05 & 0.02 & 0.04 & 0.02 & 0.02 & 0.05 \\
4165 & KOI-3060 & 27 & 0.05 & 0.01 & 0.5 & 0.03 & 0.08 & 0.06 & 0.03 & 0.02 & 0.04 & 0.02 & 0.02 & 0.02 & 0.04 & 0.02 & 0.03 & 0.02 & 0.02 & 0.04 \\
4166 & KOI-344 & 27 & 0.05 & 0.01 & 0.5 & 0.03 & 0.08 & 0.06 & 0.03 & 0.02 & 0.04 & 0.02 & 0.02 & 0.02 & 0.04 & 0.02 & 0.03 & 0.02 & 0.02 & 0.04 \\
4167 & KOI-479 & 27 & 0.05 & 0.01 & 0.5 & 0.03 & 0.08 & 0.06 & 0.03 & 0.02 & 0.04 & 0.02 & 0.02 & 0.02 & 0.04 & 0.02 & 0.03 & 0.02 & 0.02 & 0.04 \\
4168 & KOI-1645 & 27 & 0.05 & 0.01 & 0.5 & 0.03 & 0.08 & 0.06 & 0.03 & 0.02 & 0.04 & 0.02 & 0.02 & 0.02 & 0.04 & 0.02 & 0.03 & 0.02 & 0.02 & 0.04 \\
4169 & KOI-1800 & 27 & 0.05 & 0.01 & 0.5 & 0.03 & 0.08 & 0.06 & 0.03 & 0.02 & 0.04 & 0.02 & 0.02 & 0.02 & 0.04 & 0.02 & 0.03 & 0.02 & 0.02 & 0.04 \\
4170 & KOI-1444 & 29 & 0.06 & 0.02 & 0.5 & 0.04 & 0.09 & 0.07 & 0.04 & 0.02 & 0.05 & 0.02 & 0.03 & 0.02 & 0.05 & 0.02 & 0.03 & 0.02 & 0.02 & 0.05 \\
4171 & Kepler-299 & 29 & 0.06 & 0.02 & 0.6 & 0.04 & 0.10 & 0.07 & 0.04 & 0.02 & 0.05 & 0.03 & 0.03 & 0.02 & 0.05 & 0.02 & 0.04 & 0.02 & 0.02 & 0.05 \\
4172 & KOI-124 & 27 & 0.05 & 0.01 & 0.5 & 0.03 & 0.08 & 0.06 & 0.03 & 0.02 & 0.04 & 0.02 & 0.03 & 0.02 & 0.04 & 0.02 & 0.03 & 0.02 & 0.02 & 0.04 \\
4173 & KOI-1889 & 30 & 0.06 & 0.02 & 0.6 & 0.04 & 0.10 & 0.08 & 0.04 & 0.03 & 0.05 & 0.03 & 0.03 & 0.03 & 0.05 & 0.02 & 0.04 & 0.02 & 0.02 & 0.05 \\
4174 & KOI-2007 & 27 & 0.05 & 0.01 & 0.5 & 0.03 & 0.08 & 0.06 & 0.03 & 0.02 & 0.04 & 0.02 & 0.02 & 0.02 & 0.04 & 0.02 & 0.03 & 0.02 & 0.02 & 0.04 \\
4175 & KOI-2977 & 27 & 0.05 & 0.01 & 0.5 & 0.03 & 0.08 & 0.06 & 0.03 & 0.02 & 0.04 & 0.02 & 0.03 & 0.02 & 0.04 & 0.02 & 0.03 & 0.02 & 0.02 & 0.04 \\
4176 & KOI-2885 & 27 & 0.05 & 0.01 & 0.5 & 0.03 & 0.08 & 0.06 & 0.03 & 0.02 & 0.04 & 0.02 & 0.02 & 0.02 & 0.04 & 0.02 & 0.03 & 0.02 & 0.02 & 0.04 \\
4177 & KOI-2533 & 27 & 0.05 & 0.01 & 0.5 & 0.03 & 0.07 & 0.06 & 0.03 & 0.02 & 0.04 & 0.02 & 0.02 & 0.02 & 0.04 & 0.02 & 0.03 & 0.02 & 0.02 & 0.04 \\
4178 & KOI-4287 & 27 & 0.05 & 0.01 & 0.5 & 0.03 & 0.08 & 0.06 & 0.03 & 0.02 & 0.04 & 0.02 & 0.02 & 0.02 & 0.04 & 0.02 & 0.03 & 0.02 & 0.02 & 0.04 \\
4179 & KOI-2442 & 33 & 0.06 & 0.02 & 0.6 & 0.05 & 0.13 & 0.09 & 0.05 & 0.03 & 0.07 & 0.03 & 0.04 & 0.03 & 0.06 & 0.03 & 0.05 & 0.02 & 0.03 & 0.06 \\
4180 & KOI-2712 & 27 & 0.05 & 0.01 & 0.5 & 0.03 & 0.08 & 0.06 & 0.03 & 0.02 & 0.04 & 0.02 & 0.02 & 0.02 & 0.04 & 0.02 & 0.03 & 0.02 & 0.02 & 0.04 \\
4181 & KOI-2805 & 27 & 0.05 & 0.01 & 0.5 & 0.03 & 0.08 & 0.06 & 0.03 & 0.02 & 0.04 & 0.02 & 0.03 & 0.02 & 0.04 & 0.02 & 0.03 & 0.02 & 0.02 & 0.04 \\
4182 & KOI-276 & 27 & 0.05 & 0.01 & 0.5 & 0.03 & 0.08 & 0.06 & 0.03 & 0.02 & 0.04 & 0.02 & 0.02 & 0.02 & 0.04 & 0.02 & 0.03 & 0.02 & 0.02 & 0.04 \\
4183 & KOI-1863 & 27 & 0.05 & 0.01 & 0.5 & 0.03 & 0.08 & 0.06 & 0.03 & 0.02 & 0.04 & 0.02 & 0.02 & 0.02 & 0.04 & 0.02 & 0.03 & 0.02 & 0.02 & 0.04 \\
4184 & KOI-3371 & 27 & 0.05 & 0.01 & 0.5 & 0.03 & 0.07 & 0.06 & 0.03 & 0.02 & 0.04 & 0.02 & 0.02 & 0.02 & 0.04 & 0.02 & 0.03 & 0.02 & 0.02 & 0.04 \\
4185 & KOI-2792 & 27 & 0.05 & 0.01 & 0.5 & 0.03 & 0.08 & 0.06 & 0.03 & 0.02 & 0.04 & 0.02 & 0.02 & 0.02 & 0.04 & 0.02 & 0.03 & 0.02 & 0.02 & 0.04 \\
4186 & KOI-2333 & 27 & 0.05 & 0.01 & 0.5 & 0.03 & 0.08 & 0.06 & 0.03 & 0.02 & 0.04 & 0.02 & 0.03 & 0.02 & 0.04 & 0.02 & 0.03 & 0.02 & 0.02 & 0.04 \\
4187 & KOI-1647 & 27 & 0.05 & 0.01 & 0.5 & 0.03 & 0.08 & 0.06 & 0.03 & 0.02 & 0.04 & 0.02 & 0.03 & 0.02 & 0.04 & 0.02 & 0.03 & 0.02 & 0.02 & 0.04 \\
4188 & KOI-1426 & 28 & 0.05 & 0.01 & 0.5 & 0.04 & 0.08 & 0.06 & 0.03 & 0.02 & 0.04 & 0.02 & 0.03 & 0.02 & 0.04 & 0.02 & 0.03 & 0.02 & 0.02 & 0.04 \\
4189 & KOI-1438 & 28 & 0.05 & 0.01 & 0.5 & 0.04 & 0.08 & 0.06 & 0.03 & 0.02 & 0.04 & 0.02 & 0.03 & 0.02 & 0.04 & 0.02 & 0.03 & 0.02 & 0.02 & 0.04 \\
4190 & KOI-2813 & 27 & 0.05 & 0.01 & 0.5 & 0.03 & 0.08 & 0.06 & 0.03 & 0.02 & 0.04 & 0.02 & 0.02 & 0.02 & 0.04 & 0.02 & 0.03 & 0.02 & 0.02 & 0.04 \\
4191 & KOI-481 & 29 & 0.06 & 0.02 & 0.6 & 0.04 & 0.10 & 0.07 & 0.04 & 0.03 & 0.05 & 0.03 & 0.03 & 0.03 & 0.05 & 0.02 & 0.04 & 0.02 & 0.02 & 0.05 \\
4192 & KOI-2765 & 27 & 0.05 & 0.01 & 0.5 & 0.03 & 0.08 & 0.06 & 0.03 & 0.02 & 0.04 & 0.02 & 0.02 & 0.02 & 0.04 & 0.02 & 0.03 & 0.02 & 0.02 & 0.04 \\
4193 & KOI-4653 & 27 & 0.05 & 0.01 & 0.5 & 0.03 & 0.08 & 0.06 & 0.03 & 0.02 & 0.04 & 0.02 & 0.02 & 0.02 & 0.04 & 0.02 & 0.03 & 0.02 & 0.02 & 0.04 \\
4194 & KOI-294 & 27 & 0.05 & 0.01 & 0.5 & 0.03 & 0.08 & 0.06 & 0.03 & 0.02 & 0.04 & 0.02 & 0.02 & 0.02 & 0.04 & 0.02 & 0.03 & 0.02 & 0.02 & 0.04 \\
4195 & KOI-2796 & 31 & 0.06 & 0.02 & 0.6 & 0.04 & 0.11 & 0.08 & 0.04 & 0.03 & 0.06 & 0.03 & 0.03 & 0.03 & 0.05 & 0.02 & 0.04 & 0.02 & 0.03 & 0.05 \\
4196 & KOI-3103 & 28 & 0.06 & 0.02 & 0.5 & 0.04 & 0.09 & 0.07 & 0.03 & 0.02 & 0.05 & 0.02 & 0.03 & 0.02 & 0.05 & 0.02 & 0.03 & 0.02 & 0.02 & 0.04 \\
4197 & KOI-2672 & 26 & 0.05 & 0.01 & 0.5 & 0.03 & 0.06 & 0.05 & 0.02 & 0.02 & 0.03 & 0.01 & 0.02 & 0.02 & 0.04 & 0.02 & 0.02 & 0.01 & 0.01 & 0.03 \\
4198 & KOI-107 & 27 & 0.05 & 0.01 & 0.5 & 0.03 & 0.08 & 0.06 & 0.03 & 0.02 & 0.04 & 0.02 & 0.02 & 0.02 & 0.04 & 0.02 & 0.03 & 0.02 & 0.02 & 0.04 \\
4199 & KOI-3346 & 27 & 0.05 & 0.01 & 0.5 & 0.03 & 0.08 & 0.06 & 0.03 & 0.02 & 0.04 & 0.02 & 0.02 & 0.02 & 0.04 & 0.02 & 0.03 & 0.02 & 0.02 & 0.04 \\
4200 & KOI-1857 & 28 & 0.05 & 0.01 & 0.5 & 0.04 & 0.08 & 0.06 & 0.03 & 0.02 & 0.04 & 0.02 & 0.03 & 0.02 & 0.04 & 0.02 & 0.03 & 0.02 & 0.02 & 0.04 \\
4201 & KOI-4716 & 27 & 0.05 & 0.01 & 0.5 & 0.03 & 0.08 & 0.06 & 0.03 & 0.02 & 0.04 & 0.02 & 0.03 & 0.02 & 0.04 & 0.02 & 0.03 & 0.02 & 0.02 & 0.04 \\
4202 & KOI-246 & 27 & 0.05 & 0.01 & 0.5 & 0.03 & 0.08 & 0.06 & 0.03 & 0.02 & 0.04 & 0.02 & 0.02 & 0.02 & 0.04 & 0.02 & 0.03 & 0.02 & 0.02 & 0.04 \\
4203 & KOI-1802 & 28 & 0.06 & 0.02 & 0.5 & 0.04 & 0.09 & 0.07 & 0.03 & 0.02 & 0.05 & 0.02 & 0.03 & 0.02 & 0.05 & 0.02 & 0.03 & 0.02 & 0.02 & 0.04 \\
4204 & KOI-241 & 28 & 0.05 & 0.01 & 0.5 & 0.04 & 0.08 & 0.06 & 0.03 & 0.02 & 0.04 & 0.02 & 0.03 & 0.02 & 0.04 & 0.02 & 0.03 & 0.02 & 0.02 & 0.04 \\
4205 & Kepler-124 & 26 & 0.05 & 0.01 & 0.5 & 0.03 & 0.07 & 0.05 & 0.02 & 0.02 & 0.04 & 0.02 & 0.02 & 0.02 & 0.04 & 0.02 & 0.03 & 0.01 & 0.02 & 0.04 \\
4206 & KOI-2168 & 32 & 0.06 & 0.02 & 0.6 & 0.05 & 0.12 & 0.09 & 0.05 & 0.03 & 0.06 & 0.03 & 0.04 & 0.03 & 0.06 & 0.03 & 0.04 & 0.02 & 0.03 & 0.06 \\
4207 & KOI-2422 & 31 & 0.06 & 0.02 & 0.6 & 0.04 & 0.11 & 0.08 & 0.04 & 0.03 & 0.06 & 0.03 & 0.04 & 0.03 & 0.05 & 0.02 & 0.04 & 0.02 & 0.03 & 0.05 \\
4208 & KOI-2632 & 27 & 0.05 & 0.01 & 0.5 & 0.03 & 0.08 & 0.06 & 0.03 & 0.02 & 0.04 & 0.02 & 0.02 & 0.02 & 0.04 & 0.02 & 0.03 & 0.02 & 0.02 & 0.04 \\
4209 & Kepler-15 & 26 & 0.05 & 0.01 & 0.5 & 0.03 & 0.06 & 0.05 & 0.02 & 0.02 & 0.04 & 0.02 & 0.02 & 0.02 & 0.04 & 0.02 & 0.03 & 0.01 & 0.02 & 0.04 \\
4210 & KOI-128 & 27 & 0.05 & 0.01 & 0.5 & 0.03 & 0.08 & 0.06 & 0.03 & 0.02 & 0.04 & 0.02 & 0.02 & 0.02 & 0.04 & 0.02 & 0.03 & 0.02 & 0.02 & 0.04 \\
4211 & KOI-2366 & 28 & 0.05 & 0.01 & 0.5 & 0.03 & 0.08 & 0.06 & 0.03 & 0.02 & 0.04 & 0.02 & 0.03 & 0.02 & 0.04 & 0.02 & 0.03 & 0.02 & 0.02 & 0.04 \\
4212 & KOI-330 & 28 & 0.06 & 0.02 & 0.5 & 0.04 & 0.09 & 0.07 & 0.03 & 0.02 & 0.05 & 0.02 & 0.03 & 0.02 & 0.05 & 0.02 & 0.03 & 0.02 & 0.02 & 0.04 \\
4213 & KOI-3782 & 27 & 0.05 & 0.01 & 0.5 & 0.03 & 0.07 & 0.05 & 0.03 & 0.02 & 0.04 & 0.02 & 0.02 & 0.02 & 0.04 & 0.02 & 0.03 & 0.01 & 0.02 & 0.04 \\
4214 & KOI-2639 & 31 & 0.06 & 0.02 & 0.6 & 0.04 & 0.11 & 0.08 & 0.04 & 0.03 & 0.06 & 0.03 & 0.03 & 0.03 & 0.05 & 0.02 & 0.04 & 0.02 & 0.02 & 0.05 \\
4215 & KOI-3015 & 27 & 0.05 & 0.01 & 0.5 & 0.03 & 0.08 & 0.06 & 0.03 & 0.02 & 0.04 & 0.02 & 0.02 & 0.02 & 0.04 & 0.02 & 0.03 & 0.02 & 0.02 & 0.04 \\
4216 & KOI-1428 & 31 & 0.06 & 0.02 & 0.6 & 0.04 & 0.11 & 0.08 & 0.04 & 0.03 & 0.06 & 0.03 & 0.03 & 0.03 & 0.05 & 0.02 & 0.04 & 0.02 & 0.02 & 0.05 \\
4217 & KOI-4036 & 27 & 0.05 & 0.01 & 0.5 & 0.03 & 0.08 & 0.06 & 0.03 & 0.02 & 0.04 & 0.02 & 0.02 & 0.02 & 0.04 & 0.02 & 0.03 & 0.02 & 0.02 & 0.04 \\
4218 & KOI-1436 & 30 & 0.06 & 0.02 & 0.6 & 0.04 & 0.10 & 0.07 & 0.04 & 0.03 & 0.05 & 0.03 & 0.03 & 0.03 & 0.05 & 0.02 & 0.04 & 0.02 & 0.02 & 0.05 \\
4219 & Kepler-301 & 27 & 0.05 & 0.01 & 0.5 & 0.03 & 0.07 & 0.05 & 0.03 & 0.02 & 0.04 & 0.02 & 0.02 & 0.02 & 0.04 & 0.02 & 0.03 & 0.01 & 0.02 & 0.04 \\
4220 & KOI-2143 & 27 & 0.05 & 0.01 & 0.5 & 0.03 & 0.07 & 0.06 & 0.03 & 0.02 & 0.04 & 0.02 & 0.02 & 0.02 & 0.04 & 0.02 & 0.03 & 0.02 & 0.02 & 0.04 \\
4221 & KOI-2195 & 31 & 0.06 & 0.02 & 0.6 & 0.04 & 0.11 & 0.08 & 0.04 & 0.03 & 0.06 & 0.03 & 0.03 & 0.03 & 0.05 & 0.02 & 0.04 & 0.02 & 0.03 & 0.05 \\
4222 & KOI-349 & 27 & 0.05 & 0.01 & 0.5 & 0.03 & 0.08 & 0.06 & 0.03 & 0.02 & 0.04 & 0.02 & 0.02 & 0.02 & 0.04 & 0.02 & 0.03 & 0.02 & 0.02 & 0.04 \\
4223 & KOI-350 & 27 & 0.05 & 0.01 & 0.5 & 0.03 & 0.08 & 0.06 & 0.03 & 0.02 & 0.04 & 0.02 & 0.02 & 0.02 & 0.04 & 0.02 & 0.03 & 0.02 & 0.02 & 0.04 \\
4224 & KOI-1623 & 27 & 0.05 & 0.01 & 0.5 & 0.03 & 0.08 & 0.06 & 0.03 & 0.02 & 0.04 & 0.02 & 0.02 & 0.02 & 0.04 & 0.02 & 0.03 & 0.02 & 0.02 & 0.04 \\
4225 & KOI-351 & 26 & 0.05 & 0.01 & 0.5 & 0.03 & 0.06 & 0.05 & 0.02 & 0.02 & 0.04 & 0.02 & 0.02 & 0.02 & 0.04 & 0.02 & 0.03 & 0.01 & 0.02 & 0.04 \\
4226 & KOI-1992 & 30 & 0.06 & 0.02 & 0.6 & 0.04 & 0.11 & 0.08 & 0.04 & 0.03 & 0.06 & 0.03 & 0.03 & 0.03 & 0.05 & 0.02 & 0.04 & 0.02 & 0.02 & 0.05 \\
4227 & KOI-2047 & 27 & 0.05 & 0.01 & 0.5 & 0.03 & 0.08 & 0.06 & 0.03 & 0.02 & 0.04 & 0.02 & 0.03 & 0.02 & 0.04 & 0.02 & 0.03 & 0.02 & 0.02 & 0.04 \\
4228 & KOI-2771 & 27 & 0.05 & 0.01 & 0.5 & 0.03 & 0.08 & 0.06 & 0.03 & 0.02 & 0.04 & 0.02 & 0.02 & 0.02 & 0.04 & 0.02 & 0.03 & 0.02 & 0.02 & 0.04 \\
4229 & KOI-2110 & 27 & 0.05 & 0.01 & 0.5 & 0.03 & 0.08 & 0.06 & 0.03 & 0.02 & 0.04 & 0.02 & 0.03 & 0.02 & 0.04 & 0.02 & 0.03 & 0.02 & 0.02 & 0.04 \\
4230 & KOI-5900 & 28 & 0.05 & 0.01 & 0.5 & 0.03 & 0.08 & 0.06 & 0.03 & 0.02 & 0.04 & 0.02 & 0.03 & 0.02 & 0.04 & 0.02 & 0.03 & 0.02 & 0.02 & 0.04 \\
4231 & KOI-2399 & 27 & 0.05 & 0.01 & 0.5 & 0.03 & 0.07 & 0.06 & 0.03 & 0.02 & 0.04 & 0.02 & 0.02 & 0.02 & 0.04 & 0.02 & 0.03 & 0.02 & 0.02 & 0.04 \\
4232 & KOI-352 & 27 & 0.05 & 0.01 & 0.5 & 0.03 & 0.08 & 0.06 & 0.03 & 0.02 & 0.04 & 0.02 & 0.02 & 0.02 & 0.04 & 0.02 & 0.03 & 0.02 & 0.02 & 0.04 \\
4233 & KOI-2109 & 28 & 0.06 & 0.02 & 0.5 & 0.04 & 0.09 & 0.07 & 0.03 & 0.02 & 0.05 & 0.02 & 0.03 & 0.02 & 0.05 & 0.02 & 0.03 & 0.02 & 0.02 & 0.04 \\
4234 & KOI-3419 & 27 & 0.05 & 0.01 & 0.5 & 0.03 & 0.08 & 0.06 & 0.03 & 0.02 & 0.04 & 0.02 & 0.02 & 0.02 & 0.04 & 0.02 & 0.03 & 0.02 & 0.02 & 0.04 \\
4235 & KOI-168 & 27 & 0.05 & 0.01 & 0.5 & 0.03 & 0.07 & 0.06 & 0.03 & 0.02 & 0.04 & 0.02 & 0.02 & 0.02 & 0.04 & 0.02 & 0.03 & 0.01 & 0.02 & 0.04 \\
4236 & KOI-1856 & 27 & 0.05 & 0.01 & 0.5 & 0.03 & 0.08 & 0.06 & 0.03 & 0.02 & 0.04 & 0.02 & 0.02 & 0.02 & 0.04 & 0.02 & 0.03 & 0.02 & 0.02 & 0.04 \\
4237 & KOI-1655 & 27 & 0.05 & 0.01 & 0.5 & 0.03 & 0.08 & 0.06 & 0.03 & 0.02 & 0.04 & 0.02 & 0.03 & 0.02 & 0.04 & 0.02 & 0.03 & 0.02 & 0.02 & 0.04 \\
4238 & KOI-354 & 27 & 0.05 & 0.01 & 0.5 & 0.03 & 0.08 & 0.06 & 0.03 & 0.02 & 0.04 & 0.02 & 0.02 & 0.02 & 0.04 & 0.02 & 0.03 & 0.02 & 0.02 & 0.04 \\
4239 & KOI-2365 & 27 & 0.05 & 0.01 & 0.5 & 0.03 & 0.08 & 0.06 & 0.03 & 0.02 & 0.04 & 0.02 & 0.02 & 0.02 & 0.04 & 0.02 & 0.03 & 0.02 & 0.02 & 0.04 \\
4240 & KOI-2837 & 28 & 0.05 & 0.01 & 0.5 & 0.03 & 0.08 & 0.06 & 0.03 & 0.02 & 0.04 & 0.02 & 0.03 & 0.02 & 0.04 & 0.02 & 0.03 & 0.02 & 0.02 & 0.04 \\
4241 & KOI-3109 & 27 & 0.05 & 0.01 & 0.5 & 0.03 & 0.08 & 0.06 & 0.03 & 0.02 & 0.04 & 0.02 & 0.02 & 0.02 & 0.04 & 0.02 & 0.03 & 0.02 & 0.02 & 0.04 \\
4242 & KOI-295 & 27 & 0.05 & 0.01 & 0.5 & 0.03 & 0.08 & 0.06 & 0.03 & 0.02 & 0.04 & 0.02 & 0.03 & 0.02 & 0.04 & 0.02 & 0.03 & 0.02 & 0.02 & 0.04 \\
4243 & KOI-4792 & 27 & 0.05 & 0.01 & 0.5 & 0.03 & 0.08 & 0.06 & 0.03 & 0.02 & 0.04 & 0.02 & 0.02 & 0.02 & 0.04 & 0.02 & 0.03 & 0.02 & 0.02 & 0.04 \\
4244 & KOI-356 & 27 & 0.05 & 0.01 & 0.5 & 0.03 & 0.07 & 0.06 & 0.03 & 0.02 & 0.04 & 0.02 & 0.02 & 0.02 & 0.04 & 0.02 & 0.03 & 0.02 & 0.02 & 0.04 \\
4245 & KOI-1831 & 27 & 0.05 & 0.01 & 0.5 & 0.03 & 0.08 & 0.06 & 0.03 & 0.02 & 0.04 & 0.02 & 0.02 & 0.02 & 0.04 & 0.02 & 0.03 & 0.02 & 0.02 & 0.04 \\
4246 & KOI-4304 & 27 & 0.05 & 0.01 & 0.5 & 0.03 & 0.08 & 0.06 & 0.03 & 0.02 & 0.04 & 0.02 & 0.02 & 0.02 & 0.04 & 0.02 & 0.03 & 0.02 & 0.02 & 0.04 \\
4247 & KOI-355 & 27 & 0.05 & 0.01 & 0.5 & 0.03 & 0.08 & 0.06 & 0.03 & 0.02 & 0.04 & 0.02 & 0.03 & 0.02 & 0.04 & 0.02 & 0.03 & 0.02 & 0.02 & 0.04 \\
4248 & KOI-3363 & 27 & 0.05 & 0.01 & 0.5 & 0.03 & 0.08 & 0.06 & 0.03 & 0.02 & 0.04 & 0.02 & 0.02 & 0.02 & 0.04 & 0.02 & 0.03 & 0.02 & 0.02 & 0.04 \\
4249 & KOI-167 & 27 & 0.05 & 0.01 & 0.5 & 0.03 & 0.08 & 0.06 & 0.03 & 0.02 & 0.04 & 0.02 & 0.03 & 0.02 & 0.04 & 0.02 & 0.03 & 0.02 & 0.02 & 0.04 \\
4250 & KOI-1945 & 29 & 0.06 & 0.02 & 0.6 & 0.04 & 0.10 & 0.07 & 0.04 & 0.02 & 0.05 & 0.03 & 0.03 & 0.02 & 0.05 & 0.02 & 0.04 & 0.02 & 0.02 & 0.05 \\
4251 & KOI-1894 & 27 & 0.05 & 0.01 & 0.5 & 0.03 & 0.07 & 0.05 & 0.03 & 0.02 & 0.04 & 0.02 & 0.02 & 0.02 & 0.04 & 0.02 & 0.03 & 0.01 & 0.02 & 0.04 \\
4252 & KOI-1832 & 32 & 0.06 & 0.02 & 0.6 & 0.05 & 0.12 & 0.09 & 0.05 & 0.03 & 0.06 & 0.03 & 0.04 & 0.03 & 0.06 & 0.03 & 0.04 & 0.02 & 0.03 & 0.06 \\
4253 & KOI-1841 & 27 & 0.05 & 0.01 & 0.5 & 0.03 & 0.08 & 0.06 & 0.03 & 0.02 & 0.04 & 0.02 & 0.02 & 0.02 & 0.04 & 0.02 & 0.03 & 0.02 & 0.02 & 0.04 \\
4254 & KOI-2582 & 27 & 0.05 & 0.01 & 0.5 & 0.03 & 0.08 & 0.06 & 0.03 & 0.02 & 0.04 & 0.02 & 0.02 & 0.02 & 0.04 & 0.02 & 0.03 & 0.02 & 0.02 & 0.04 \\
4255 & KOI-620 & 30 & 0.06 & 0.02 & 0.6 & 0.04 & 0.11 & 0.08 & 0.04 & 0.03 & 0.06 & 0.03 & 0.03 & 0.03 & 0.05 & 0.02 & 0.04 & 0.02 & 0.02 & 0.05 \\
4256 & KOI-3403 & 27 & 0.05 & 0.01 & 0.5 & 0.03 & 0.08 & 0.06 & 0.03 & 0.02 & 0.04 & 0.02 & 0.02 & 0.02 & 0.04 & 0.02 & 0.03 & 0.02 & 0.02 & 0.04 \\
4257 & KOI-1883 & 27 & 0.05 & 0.01 & 0.5 & 0.03 & 0.08 & 0.06 & 0.03 & 0.02 & 0.04 & 0.02 & 0.02 & 0.02 & 0.04 & 0.02 & 0.03 & 0.02 & 0.02 & 0.04 \\
4258 & KOI-3892 & 27 & 0.05 & 0.01 & 0.5 & 0.03 & 0.07 & 0.06 & 0.03 & 0.02 & 0.04 & 0.02 & 0.02 & 0.02 & 0.04 & 0.02 & 0.03 & 0.02 & 0.02 & 0.04 \\
4259 & KOI-1980 & 27 & 0.05 & 0.01 & 0.5 & 0.03 & 0.08 & 0.06 & 0.03 & 0.02 & 0.04 & 0.02 & 0.03 & 0.02 & 0.04 & 0.02 & 0.03 & 0.02 & 0.02 & 0.04 \\
4260 & KOI-2173 & 27 & 0.05 & 0.01 & 0.5 & 0.03 & 0.07 & 0.05 & 0.03 & 0.02 & 0.04 & 0.02 & 0.02 & 0.02 & 0.04 & 0.02 & 0.03 & 0.01 & 0.02 & 0.04 \\
4261 & KOI-2492 & 27 & 0.05 & 0.01 & 0.5 & 0.03 & 0.08 & 0.06 & 0.03 & 0.02 & 0.04 & 0.02 & 0.02 & 0.02 & 0.04 & 0.02 & 0.03 & 0.02 & 0.02 & 0.04 \\
4262 & KOI-2260 & 27 & 0.05 & 0.01 & 0.5 & 0.03 & 0.08 & 0.06 & 0.03 & 0.02 & 0.04 & 0.02 & 0.03 & 0.02 & 0.04 & 0.02 & 0.03 & 0.02 & 0.02 & 0.04 \\
4263 & KOI-296 & 27 & 0.05 & 0.01 & 0.5 & 0.03 & 0.08 & 0.06 & 0.03 & 0.02 & 0.04 & 0.02 & 0.02 & 0.02 & 0.04 & 0.02 & 0.03 & 0.02 & 0.02 & 0.04 \\
4264 & KOI-2581 & 27 & 0.05 & 0.01 & 0.5 & 0.03 & 0.08 & 0.06 & 0.03 & 0.02 & 0.04 & 0.02 & 0.02 & 0.02 & 0.04 & 0.02 & 0.03 & 0.02 & 0.02 & 0.04 \\
4265 & KOI-543 & 29 & 0.06 & 0.02 & 0.6 & 0.04 & 0.10 & 0.07 & 0.04 & 0.02 & 0.05 & 0.03 & 0.03 & 0.02 & 0.05 & 0.02 & 0.04 & 0.02 & 0.02 & 0.05 \\
4266 & KOI-4062 & 28 & 0.06 & 0.02 & 0.5 & 0.04 & 0.09 & 0.07 & 0.03 & 0.02 & 0.05 & 0.02 & 0.03 & 0.02 & 0.05 & 0.02 & 0.03 & 0.02 & 0.02 & 0.05 \\
4267 & KOI-3875 & 27 & 0.05 & 0.01 & 0.5 & 0.03 & 0.08 & 0.06 & 0.03 & 0.02 & 0.04 & 0.02 & 0.02 & 0.02 & 0.04 & 0.02 & 0.03 & 0.02 & 0.02 & 0.04 \\
4268 & KOI-72 & 28 & 0.05 & 0.01 & 0.5 & 0.03 & 0.08 & 0.06 & 0.03 & 0.02 & 0.04 & 0.02 & 0.03 & 0.02 & 0.04 & 0.02 & 0.03 & 0.02 & 0.02 & 0.04 \\
4269 & KOI-297 & 28 & 0.06 & 0.02 & 0.5 & 0.04 & 0.09 & 0.06 & 0.03 & 0.02 & 0.05 & 0.02 & 0.03 & 0.02 & 0.05 & 0.02 & 0.03 & 0.02 & 0.02 & 0.04 \\
4270 & KOI-2026 & 27 & 0.05 & 0.01 & 0.5 & 0.03 & 0.08 & 0.06 & 0.03 & 0.02 & 0.04 & 0.02 & 0.02 & 0.02 & 0.04 & 0.02 & 0.03 & 0.02 & 0.02 & 0.04 \\
4271 & KOI-2433 & 34 & 0.06 & 0.02 & 0.6 & 0.05 & 0.13 & 0.10 & 0.05 & 0.03 & 0.07 & 0.04 & 0.04 & 0.03 & 0.06 & 0.03 & 0.05 & 0.03 & 0.03 & 0.06 \\
4272 & KOI-4011 & 27 & 0.05 & 0.01 & 0.5 & 0.03 & 0.08 & 0.06 & 0.03 & 0.02 & 0.04 & 0.02 & 0.02 & 0.02 & 0.04 & 0.02 & 0.03 & 0.02 & 0.02 & 0.04 \\
4273 & KOI-4129 & 27 & 0.05 & 0.01 & 0.5 & 0.03 & 0.07 & 0.06 & 0.03 & 0.02 & 0.04 & 0.02 & 0.02 & 0.02 & 0.04 & 0.02 & 0.03 & 0.02 & 0.02 & 0.04 \\
4274 & KOI-4021 & 27 & 0.05 & 0.01 & 0.5 & 0.03 & 0.08 & 0.06 & 0.03 & 0.02 & 0.04 & 0.02 & 0.03 & 0.02 & 0.04 & 0.02 & 0.03 & 0.02 & 0.02 & 0.04 \\
4275 & KOI-2590 & 28 & 0.05 & 0.01 & 0.5 & 0.03 & 0.08 & 0.06 & 0.03 & 0.02 & 0.04 & 0.02 & 0.03 & 0.02 & 0.04 & 0.02 & 0.03 & 0.02 & 0.02 & 0.04 \\
4276 & KOI-2729 & 27 & 0.05 & 0.01 & 0.5 & 0.03 & 0.08 & 0.06 & 0.03 & 0.02 & 0.04 & 0.02 & 0.02 & 0.02 & 0.04 & 0.02 & 0.03 & 0.02 & 0.02 & 0.04 \\
4277 & KOI-3194 & 27 & 0.05 & 0.01 & 0.5 & 0.03 & 0.08 & 0.06 & 0.03 & 0.02 & 0.04 & 0.02 & 0.03 & 0.02 & 0.04 & 0.02 & 0.03 & 0.02 & 0.02 & 0.04 \\
4278 & Kepler-197 & 25 & 0.05 & 0.01 & 0.5 & 0.03 & 0.04 & 0.04 & 0.01 & 0.01 & 0.03 & 0.01 & 0.01 & 0.01 & 0.03 & 0.01 & 0.02 & 0.01 & 0.01 & 0.03 \\
4279 & KOI-623 & 27 & 0.05 & 0.01 & 0.5 & 0.03 & 0.08 & 0.06 & 0.03 & 0.02 & 0.04 & 0.02 & 0.03 & 0.02 & 0.04 & 0.02 & 0.03 & 0.02 & 0.02 & 0.04 \\
4280 & KOI-3017 & 27 & 0.05 & 0.01 & 0.5 & 0.03 & 0.08 & 0.06 & 0.03 & 0.02 & 0.04 & 0.02 & 0.02 & 0.02 & 0.04 & 0.02 & 0.03 & 0.02 & 0.02 & 0.04 \\
4281 & KOI-546 & 32 & 0.06 & 0.02 & 0.6 & 0.05 & 0.12 & 0.09 & 0.05 & 0.03 & 0.06 & 0.03 & 0.04 & 0.03 & 0.06 & 0.03 & 0.04 & 0.02 & 0.03 & 0.06 \\
4282 & KOI-2072 & 28 & 0.05 & 0.01 & 0.5 & 0.04 & 0.08 & 0.06 & 0.03 & 0.02 & 0.05 & 0.02 & 0.03 & 0.02 & 0.04 & 0.02 & 0.03 & 0.02 & 0.02 & 0.04 \\
4283 & KOI-2407 & 27 & 0.05 & 0.01 & 0.5 & 0.03 & 0.08 & 0.06 & 0.03 & 0.02 & 0.04 & 0.02 & 0.02 & 0.02 & 0.04 & 0.02 & 0.03 & 0.02 & 0.02 & 0.04 \\
4284 & KOI-2396 & 29 & 0.06 & 0.02 & 0.6 & 0.04 & 0.09 & 0.07 & 0.04 & 0.02 & 0.05 & 0.03 & 0.03 & 0.02 & 0.05 & 0.02 & 0.04 & 0.02 & 0.02 & 0.05 \\
4285 & KOI-4457 & 27 & 0.05 & 0.01 & 0.5 & 0.03 & 0.08 & 0.06 & 0.03 & 0.02 & 0.04 & 0.02 & 0.02 & 0.02 & 0.04 & 0.02 & 0.03 & 0.02 & 0.02 & 0.04 \\
4286 & KOI-360 & 28 & 0.05 & 0.01 & 0.5 & 0.03 & 0.08 & 0.06 & 0.03 & 0.02 & 0.04 & 0.02 & 0.03 & 0.02 & 0.04 & 0.02 & 0.03 & 0.02 & 0.02 & 0.04 \\
4287 & KOI-141 & 27 & 0.05 & 0.01 & 0.5 & 0.03 & 0.08 & 0.06 & 0.03 & 0.02 & 0.04 & 0.02 & 0.02 & 0.02 & 0.04 & 0.02 & 0.03 & 0.02 & 0.02 & 0.04 \\
4288 & KOI-2597 & 32 & 0.06 & 0.02 & 0.6 & 0.05 & 0.12 & 0.09 & 0.05 & 0.03 & 0.06 & 0.03 & 0.04 & 0.03 & 0.06 & 0.02 & 0.04 & 0.02 & 0.03 & 0.06 \\
4289 & KOI-2004 & 27 & 0.05 & 0.01 & 0.5 & 0.03 & 0.08 & 0.06 & 0.03 & 0.02 & 0.04 & 0.02 & 0.02 & 0.02 & 0.04 & 0.02 & 0.03 & 0.02 & 0.02 & 0.04 \\
4290 & KOI-2714 & 28 & 0.05 & 0.01 & 0.5 & 0.04 & 0.08 & 0.06 & 0.03 & 0.02 & 0.04 & 0.02 & 0.03 & 0.02 & 0.04 & 0.02 & 0.03 & 0.02 & 0.02 & 0.04 \\
4291 & Kepler-401 & 25 & 0.05 & 0.01 & 0.5 & 0.03 & 0.06 & 0.05 & 0.02 & 0.02 & 0.03 & 0.01 & 0.02 & 0.02 & 0.04 & 0.02 & 0.02 & 0.01 & 0.01 & 0.03 \\
4292 & KOI-1947 & 27 & 0.05 & 0.01 & 0.5 & 0.03 & 0.08 & 0.06 & 0.03 & 0.02 & 0.04 & 0.02 & 0.02 & 0.02 & 0.04 & 0.02 & 0.03 & 0.02 & 0.02 & 0.04 \\
4293 & KOI-2372 & 27 & 0.05 & 0.01 & 0.5 & 0.03 & 0.08 & 0.06 & 0.03 & 0.02 & 0.04 & 0.02 & 0.03 & 0.02 & 0.04 & 0.02 & 0.03 & 0.02 & 0.02 & 0.04 \\
4294 & KOI-3310 & 27 & 0.05 & 0.01 & 0.5 & 0.03 & 0.08 & 0.06 & 0.03 & 0.02 & 0.04 & 0.02 & 0.02 & 0.02 & 0.04 & 0.02 & 0.03 & 0.02 & 0.02 & 0.04 \\
4295 & KOI-3167 & 27 & 0.05 & 0.01 & 0.5 & 0.03 & 0.07 & 0.06 & 0.03 & 0.02 & 0.04 & 0.02 & 0.02 & 0.02 & 0.04 & 0.02 & 0.03 & 0.02 & 0.02 & 0.04 \\
4296 & KOI-279 & 27 & 0.05 & 0.01 & 0.5 & 0.03 & 0.08 & 0.06 & 0.03 & 0.02 & 0.04 & 0.02 & 0.03 & 0.02 & 0.04 & 0.02 & 0.03 & 0.02 & 0.02 & 0.04 \\
4297 & WASP-92 & 25 & 0.05 & 0.01 & 0.5 & 0.03 & 0.04 & 0.04 & 0.01 & 0.01 & 0.03 & 0.01 & 0.01 & 0.01 & 0.03 & 0.01 & 0.02 & 0.01 & 0.01 & 0.03 \\
4298 & KOI-2541 & 27 & 0.05 & 0.01 & 0.5 & 0.03 & 0.07 & 0.06 & 0.03 & 0.02 & 0.04 & 0.02 & 0.02 & 0.02 & 0.04 & 0.02 & 0.03 & 0.02 & 0.02 & 0.04 \\
4299 & KOI-2059 & 27 & 0.05 & 0.01 & 0.5 & 0.03 & 0.07 & 0.06 & 0.03 & 0.02 & 0.04 & 0.02 & 0.02 & 0.02 & 0.04 & 0.02 & 0.03 & 0.01 & 0.02 & 0.04 \\
4300 & KOI-375 & 27 & 0.05 & 0.01 & 0.5 & 0.03 & 0.08 & 0.06 & 0.03 & 0.02 & 0.04 & 0.02 & 0.02 & 0.02 & 0.04 & 0.02 & 0.03 & 0.02 & 0.02 & 0.04 \\
4301 & KOI-1474 & 25 & 0.05 & 0.01 & 0.5 & 0.03 & 0.05 & 0.04 & 0.02 & 0.01 & 0.03 & 0.01 & 0.02 & 0.01 & 0.04 & 0.02 & 0.02 & 0.01 & 0.01 & 0.03 \\
4302 & KOI-3122 & 27 & 0.05 & 0.01 & 0.5 & 0.03 & 0.08 & 0.06 & 0.03 & 0.02 & 0.04 & 0.02 & 0.03 & 0.02 & 0.04 & 0.02 & 0.03 & 0.02 & 0.02 & 0.04 \\
4303 & KOI-3009 & 33 & 0.06 & 0.02 & 0.6 & 0.05 & 0.13 & 0.09 & 0.05 & 0.03 & 0.07 & 0.03 & 0.04 & 0.03 & 0.06 & 0.03 & 0.05 & 0.02 & 0.03 & 0.06 \\
4304 & KOI-4829 & 27 & 0.05 & 0.01 & 0.5 & 0.03 & 0.08 & 0.06 & 0.03 & 0.02 & 0.04 & 0.02 & 0.02 & 0.02 & 0.04 & 0.02 & 0.03 & 0.02 & 0.02 & 0.04 \\
4305 & KOI-2331 & 27 & 0.05 & 0.01 & 0.5 & 0.03 & 0.08 & 0.06 & 0.03 & 0.02 & 0.04 & 0.02 & 0.02 & 0.02 & 0.04 & 0.02 & 0.03 & 0.02 & 0.02 & 0.04 \\
4306 & KOI-361 & 27 & 0.05 & 0.01 & 0.5 & 0.03 & 0.08 & 0.06 & 0.03 & 0.02 & 0.04 & 0.02 & 0.02 & 0.02 & 0.04 & 0.02 & 0.03 & 0.02 & 0.02 & 0.04 \\
4307 & KOI-2463 & 27 & 0.05 & 0.01 & 0.5 & 0.03 & 0.08 & 0.06 & 0.03 & 0.02 & 0.04 & 0.02 & 0.02 & 0.02 & 0.04 & 0.02 & 0.03 & 0.02 & 0.02 & 0.04 \\
4308 & KOI-439 & 27 & 0.05 & 0.01 & 0.5 & 0.03 & 0.07 & 0.06 & 0.03 & 0.02 & 0.04 & 0.02 & 0.02 & 0.02 & 0.04 & 0.02 & 0.03 & 0.02 & 0.02 & 0.04 \\
4309 & KOI-4329 & 27 & 0.05 & 0.01 & 0.5 & 0.03 & 0.08 & 0.06 & 0.03 & 0.02 & 0.04 & 0.02 & 0.02 & 0.02 & 0.04 & 0.02 & 0.03 & 0.02 & 0.02 & 0.04 \\
4310 & KOI-4605 & 28 & 0.05 & 0.01 & 0.5 & 0.04 & 0.08 & 0.06 & 0.03 & 0.02 & 0.05 & 0.02 & 0.03 & 0.02 & 0.04 & 0.02 & 0.03 & 0.02 & 0.02 & 0.04 \\
4311 & KOI-4190 & 28 & 0.06 & 0.02 & 0.5 & 0.04 & 0.09 & 0.07 & 0.03 & 0.02 & 0.05 & 0.02 & 0.03 & 0.02 & 0.05 & 0.02 & 0.03 & 0.02 & 0.02 & 0.04 \\
4312 & KOI-548 & 28 & 0.05 & 0.01 & 0.5 & 0.03 & 0.08 & 0.06 & 0.03 & 0.02 & 0.04 & 0.02 & 0.03 & 0.02 & 0.04 & 0.02 & 0.03 & 0.02 & 0.02 & 0.04 \\
4313 & KOI-3663 & 27 & 0.05 & 0.01 & 0.5 & 0.03 & 0.08 & 0.06 & 0.03 & 0.02 & 0.04 & 0.02 & 0.02 & 0.02 & 0.04 & 0.02 & 0.03 & 0.02 & 0.02 & 0.04 \\
4314 & KOI-4245 & 28 & 0.05 & 0.02 & 0.5 & 0.04 & 0.08 & 0.06 & 0.03 & 0.02 & 0.05 & 0.02 & 0.03 & 0.02 & 0.04 & 0.02 & 0.03 & 0.02 & 0.02 & 0.04 \\
4315 & BD+52_277A & 25 & 0.05 & 0.01 & 0.5 & 0.03 & 0.04 & 0.04 & 0.01 & 0.01 & 0.03 & 0.01 & 0.01 & 0.01 & 0.03 & 0.01 & 0.02 & 0.01 & 0.01 & 0.03 \\
4316 & HD 239643 & 25 & 0.05 & 0.01 & 0.5 & 0.03 & 0.04 & 0.04 & 0.01 & 0.01 & 0.03 & 0.01 & 0.01 & 0.01 & 0.03 & 0.01 & 0.02 & 0.01 & 0.01 & 0.03 \\
4317 & HD 203802 & 25 & 0.05 & 0.01 & 0.5 & 0.03 & 0.04 & 0.04 & 0.01 & 0.01 & 0.03 & 0.01 & 0.01 & 0.01 & 0.03 & 0.01 & 0.02 & 0.01 & 0.01 & 0.03 \\
4318 & HD 240051 & 25 & 0.05 & 0.01 & 0.5 & 0.03 & 0.04 & 0.04 & 0.01 & 0.01 & 0.03 & 0.01 & 0.01 & 0.01 & 0.03 & 0.01 & 0.02 & 0.01 & 0.01 & 0.03 \\
4319 & HD 215714 & 25 & 0.05 & 0.01 & 0.5 & 0.03 & 0.04 & 0.04 & 0.01 & 0.01 & 0.03 & 0.01 & 0.01 & 0.01 & 0.03 & 0.01 & 0.02 & 0.01 & 0.01 & 0.03 \\
\enddata
\end{deluxetable*}

